Dimensional synthesis of spatial manipulators for velocity and force transmission for operation around a specified task point

Dimensional synthesis refers to design of the dimensions of manipulators by optimising different kinds of performance indices. The motivation of this study is to perform dimensional synthesis for a wide set of spatial manipulators by optimising the manipulability of each manipulator around a pre-defined task point in the workspace and to finally give a prescription of manipulators along with their dimensions optimised for velocity and force transmission. A systematic method to formulate Jacobian matrix of a manipulator is presented. Optimisation of manipulability is performed for manipulation of the end-effector around a chosen task point for 96 1-DOF manipulators, 645 2-DOF manipulators, 8 3-DOF manipulators and 15 4-DOF manipulators taken from the result of enumeration of manipulators that is done in its companion paper devoted to enumeration of possible manipulators up to a number of links. Prescriptions for these sets of manipulators are presented along with their scaled condition numbers and their ordered indices. This gives the designer a prescription of manipulators with their optimised dimensions that reflects the performance of the end-effector around the given task point for velocity and force transmission.

==> 2dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/1.png}}{2D-M1}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/2.png}}{2D-M2}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/3.png}}{2D-M3}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/4.png}}{2D-M4}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/5.png}}{2D-M5}

  \end{minipage}
\end{subfigure}
\caption{Class 1 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/6.png}}{2D-M6}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/7.png}}{2D-M7}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/8.png}}{2D-M8}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/9.png}}{2D-M9}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/10.png}}{2D-M10}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/11.png}}{2D-M11}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/12.png}}{2D-M12}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/13.png}}{2D-M13}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/14.png}}{2D-M14}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/15.png}}{2D-M15}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/16.png}}{2D-M16}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/17.png}}{2D-M17}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/18.png}}{2D-M18}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/19.png}}{2D-M19}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/20.png}}{2D-M20}

  \end{minipage}
\end{subfigure}
\caption{Class 2 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/21.png}}{2D-M21}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/22.png}}{2D-M22}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/23.png}}{2D-M23}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/24.png}}{2D-M24}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/25.png}}{2D-M25}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/26.png}}{2D-M26}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/27.png}}{2D-M27}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/28.png}}{2D-M28}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/29.png}}{2D-M29}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/30.png}}{2D-M30}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/31.png}}{2D-M31}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/32.png}}{2D-M32}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/33.png}}{2D-M33}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/34.png}}{2D-M34}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/35.png}}{2D-M35}

  \end{minipage}
\end{subfigure}
\caption{Class 3 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/36.png}}{2D-M36}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/37.png}}{2D-M37}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/38.png}}{2D-M38}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/39.png}}{2D-M39}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/40.png}}{2D-M40}

  \end{minipage}
\end{subfigure}
\caption{Class 4 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/41.png}}{2D-M41}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/42.png}}{2D-M42}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/43.png}}{2D-M43}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/44.png}}{2D-M44}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/45.png}}{2D-M45}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/46.png}}{2D-M46}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/47.png}}{2D-M47}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/48.png}}{2D-M48}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/49.png}}{2D-M49}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/50.png}}{2D-M50}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/51.png}}{2D-M51}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/52.png}}{2D-M52}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/53.png}}{2D-M53}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/54.png}}{2D-M54}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/55.png}}{2D-M55}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/56.png}}{2D-M56}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/57.png}}{2D-M57}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/58.png}}{2D-M58}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/59.png}}{2D-M59}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/60.png}}{2D-M60}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/61.png}}{2D-M61}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/62.png}}{2D-M62}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/63.png}}{2D-M63}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/64.png}}{2D-M64}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/65.png}}{2D-M65}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/66.png}}{2D-M66}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/67.png}}{2D-M67}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/68.png}}{2D-M68}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/69.png}}{2D-M69}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/70.png}}{2D-M70}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/71.png}}{2D-M71}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/72.png}}{2D-M72}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/73.png}}{2D-M73}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/74.png}}{2D-M74}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/75.png}}{2D-M75}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/76.png}}{2D-M76}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/77.png}}{2D-M77}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/78.png}}{2D-M78}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/79.png}}{2D-M79}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/80.png}}{2D-M80}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/81.png}}{2D-M81}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/82.png}}{2D-M82}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/83.png}}{2D-M83}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/84.png}}{2D-M84}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/85.png}}{2D-M85}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/86.png}}{2D-M86}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/87.png}}{2D-M87}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/88.png}}{2D-M88}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/89.png}}{2D-M89}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/90.png}}{2D-M90}

  \end{minipage}
\end{subfigure}
\caption{Class 5 of 2-DOF Manipulators (Part 1)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/91.png}}{2D-M91}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/92.png}}{2D-M92}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/93.png}}{2D-M93}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/94.png}}{2D-M94}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/95.png}}{2D-M95}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/96.png}}{2D-M96}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/97.png}}{2D-M97}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/98.png}}{2D-M98}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/99.png}}{2D-M99}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/100.png}}{2D-M100}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/101.png}}{2D-M101}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/102.png}}{2D-M102}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/103.png}}{2D-M103}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/104.png}}{2D-M104}

  \end{minipage}
\end{subfigure}
\caption{Class 5 of 2-DOF Manipulators (Part 2)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/105.png}}{2D-M105}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/106.png}}{2D-M106}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/107.png}}{2D-M107}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/108.png}}{2D-M108}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/109.png}}{2D-M109}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/110.png}}{2D-M110}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/111.png}}{2D-M111}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/112.png}}{2D-M112}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/113.png}}{2D-M113}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/114.png}}{2D-M114}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/115.png}}{2D-M115}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/116.png}}{2D-M116}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/117.png}}{2D-M117}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/118.png}}{2D-M118}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/119.png}}{2D-M119}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/120.png}}{2D-M120}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/121.png}}{2D-M121}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/122.png}}{2D-M122}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/123.png}}{2D-M123}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/124.png}}{2D-M124}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/125.png}}{2D-M125}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/126.png}}{2D-M126}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/127.png}}{2D-M127}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/128.png}}{2D-M128}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/129.png}}{2D-M129}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/130.png}}{2D-M130}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/131.png}}{2D-M131}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/132.png}}{2D-M132}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/133.png}}{2D-M133}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/134.png}}{2D-M134}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/135.png}}{2D-M135}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/136.png}}{2D-M136}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/137.png}}{2D-M137}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/138.png}}{2D-M138}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/139.png}}{2D-M139}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/140.png}}{2D-M140}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/141.png}}{2D-M141}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/142.png}}{2D-M142}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/143.png}}{2D-M143}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/144.png}}{2D-M144}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/145.png}}{2D-M145}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/146.png}}{2D-M146}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/147.png}}{2D-M147}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/148.png}}{2D-M148}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/149.png}}{2D-M149}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/150.png}}{2D-M150}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/151.png}}{2D-M151}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/152.png}}{2D-M152}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/153.png}}{2D-M153}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/154.png}}{2D-M154}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Part 1)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/155.png}}{2D-M155}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/156.png}}{2D-M156}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/157.png}}{2D-M157}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/158.png}}{2D-M158}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/159.png}}{2D-M159}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/160.png}}{2D-M160}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/161.png}}{2D-M161}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/162.png}}{2D-M162}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/163.png}}{2D-M163}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/164.png}}{2D-M164}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/165.png}}{2D-M165}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/166.png}}{2D-M166}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/167.png}}{2D-M167}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/168.png}}{2D-M168}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/169.png}}{2D-M169}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/170.png}}{2D-M170}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/171.png}}{2D-M171}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/172.png}}{2D-M172}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/173.png}}{2D-M173}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/174.png}}{2D-M174}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/175.png}}{2D-M175}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/176.png}}{2D-M176}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/177.png}}{2D-M177}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/178.png}}{2D-M178}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/179.png}}{2D-M179}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/180.png}}{2D-M180}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/181.png}}{2D-M181}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/182.png}}{2D-M182}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/183.png}}{2D-M183}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/184.png}}{2D-M184}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/185.png}}{2D-M185}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/186.png}}{2D-M186}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/187.png}}{2D-M187}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/188.png}}{2D-M188}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/189.png}}{2D-M189}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/190.png}}{2D-M190}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/191.png}}{2D-M191}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/192.png}}{2D-M192}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/193.png}}{2D-M193}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/194.png}}{2D-M194}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/195.png}}{2D-M195}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/196.png}}{2D-M196}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/197.png}}{2D-M197}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/198.png}}{2D-M198}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/199.png}}{2D-M199}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/200.png}}{2D-M200}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/201.png}}{2D-M201}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/202.png}}{2D-M202}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/203.png}}{2D-M203}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/204.png}}{2D-M204}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Part 2)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/205.png}}{2D-M205}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/206.png}}{2D-M206}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/207.png}}{2D-M207}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/208.png}}{2D-M208}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/209.png}}{2D-M209}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/210.png}}{2D-M210}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/211.png}}{2D-M211}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/212.png}}{2D-M212}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/213.png}}{2D-M213}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/214.png}}{2D-M214}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/215.png}}{2D-M215}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/216.png}}{2D-M216}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/217.png}}{2D-M217}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/218.png}}{2D-M218}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/219.png}}{2D-M219}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/220.png}}{2D-M220}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/221.png}}{2D-M221}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/222.png}}{2D-M222}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/223.png}}{2D-M223}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/224.png}}{2D-M224}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/225.png}}{2D-M225}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/226.png}}{2D-M226}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/227.png}}{2D-M227}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/228.png}}{2D-M228}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/229.png}}{2D-M229}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/230.png}}{2D-M230}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/231.png}}{2D-M231}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/232.png}}{2D-M232}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/233.png}}{2D-M233}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/234.png}}{2D-M234}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/235.png}}{2D-M235}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/236.png}}{2D-M236}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/237.png}}{2D-M237}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/238.png}}{2D-M238}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/239.png}}{2D-M239}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/240.png}}{2D-M240}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/241.png}}{2D-M241}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/242.png}}{2D-M242}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/243.png}}{2D-M243}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/244.png}}{2D-M244}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/245.png}}{2D-M245}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/246.png}}{2D-M246}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/247.png}}{2D-M247}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/248.png}}{2D-M248}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/249.png}}{2D-M249}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/250.png}}{2D-M250}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/251.png}}{2D-M251}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/252.png}}{2D-M252}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/253.png}}{2D-M253}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/254.png}}{2D-M254}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Part 3)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/255.png}}{2D-M255}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/256.png}}{2D-M256}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/257.png}}{2D-M257}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/258.png}}{2D-M258}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/259.png}}{2D-M259}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/260.png}}{2D-M260}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/261.png}}{2D-M261}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/262.png}}{2D-M262}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/263.png}}{2D-M263}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/264.png}}{2D-M264}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/265.png}}{2D-M265}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/266.png}}{2D-M266}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/267.png}}{2D-M267}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/268.png}}{2D-M268}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/269.png}}{2D-M269}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/270.png}}{2D-M270}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/271.png}}{2D-M271}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/272.png}}{2D-M272}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/273.png}}{2D-M273}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/274.png}}{2D-M274}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/275.png}}{2D-M275}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/276.png}}{2D-M276}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/277.png}}{2D-M277}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/278.png}}{2D-M278}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/279.png}}{2D-M279}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/280.png}}{2D-M280}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/281.png}}{2D-M281}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/282.png}}{2D-M282}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/283.png}}{2D-M283}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/284.png}}{2D-M284}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/285.png}}{2D-M285}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/286.png}}{2D-M286}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/287.png}}{2D-M287}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/288.png}}{2D-M288}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/289.png}}{2D-M289}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/290.png}}{2D-M290}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/291.png}}{2D-M291}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/292.png}}{2D-M292}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/293.png}}{2D-M293}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/294.png}}{2D-M294}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/295.png}}{2D-M295}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/296.png}}{2D-M296}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Part 4)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/297.png}}{2D-M297}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/298.png}}{2D-M298}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/299.png}}{2D-M299}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/300.png}}{2D-M300}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/301.png}}{2D-M301}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/302.png}}{2D-M302}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/303.png}}{2D-M303}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/304.png}}{2D-M304}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/305.png}}{2D-M305}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/306.png}}{2D-M306}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/307.png}}{2D-M307}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/308.png}}{2D-M308}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/309.png}}{2D-M309}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/310.png}}{2D-M310}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/311.png}}{2D-M311}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/312.png}}{2D-M312}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/313.png}}{2D-M313}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/314.png}}{2D-M314}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/315.png}}{2D-M315}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/316.png}}{2D-M316}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/317.png}}{2D-M317}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/318.png}}{2D-M318}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/319.png}}{2D-M319}

  \end{minipage}
\end{subfigure}
\caption{Class 7 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/320.png}}{2D-M320}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/321.png}}{2D-M321}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/322.png}}{2D-M322}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/323.png}}{2D-M323}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/324.png}}{2D-M324}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/325.png}}{2D-M325}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/326.png}}{2D-M326}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/327.png}}{2D-M327}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/328.png}}{2D-M328}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/329.png}}{2D-M329}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/330.png}}{2D-M330}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/331.png}}{2D-M331}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/332.png}}{2D-M332}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/333.png}}{2D-M333}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/334.png}}{2D-M334}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/335.png}}{2D-M335}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/336.png}}{2D-M336}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/337.png}}{2D-M337}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/338.png}}{2D-M338}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/339.png}}{2D-M339}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/340.png}}{2D-M340}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/341.png}}{2D-M341}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/342.png}}{2D-M342}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/343.png}}{2D-M343}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/344.png}}{2D-M344}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/345.png}}{2D-M345}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/346.png}}{2D-M346}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/347.png}}{2D-M347}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/348.png}}{2D-M348}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/349.png}}{2D-M349}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/350.png}}{2D-M350}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/351.png}}{2D-M351}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/352.png}}{2D-M352}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/353.png}}{2D-M353}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/354.png}}{2D-M354}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/355.png}}{2D-M355}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/356.png}}{2D-M356}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/357.png}}{2D-M357}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/358.png}}{2D-M358}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/359.png}}{2D-M359}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/360.png}}{2D-M360}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/361.png}}{2D-M361}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/362.png}}{2D-M362}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/363.png}}{2D-M363}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/364.png}}{2D-M364}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/365.png}}{2D-M365}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/366.png}}{2D-M366}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/367.png}}{2D-M367}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/368.png}}{2D-M368}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/369.png}}{2D-M369}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Part 1)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/370.png}}{2D-M370}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/371.png}}{2D-M371}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/372.png}}{2D-M372}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/373.png}}{2D-M373}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/374.png}}{2D-M374}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/375.png}}{2D-M375}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/376.png}}{2D-M376}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/377.png}}{2D-M377}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/378.png}}{2D-M378}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/379.png}}{2D-M379}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/380.png}}{2D-M380}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/381.png}}{2D-M381}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/382.png}}{2D-M382}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/383.png}}{2D-M383}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/384.png}}{2D-M384}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/385.png}}{2D-M385}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/386.png}}{2D-M386}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/387.png}}{2D-M387}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/388.png}}{2D-M388}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/389.png}}{2D-M389}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/390.png}}{2D-M390}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/391.png}}{2D-M391}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/392.png}}{2D-M392}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/393.png}}{2D-M393}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/394.png}}{2D-M394}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/395.png}}{2D-M395}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/396.png}}{2D-M396}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/397.png}}{2D-M397}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/398.png}}{2D-M398}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/399.png}}{2D-M399}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/400.png}}{2D-M400}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/401.png}}{2D-M401}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/402.png}}{2D-M402}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/403.png}}{2D-M403}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/404.png}}{2D-M404}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/405.png}}{2D-M405}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/406.png}}{2D-M406}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/407.png}}{2D-M407}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/408.png}}{2D-M408}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/409.png}}{2D-M409}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/410.png}}{2D-M410}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/411.png}}{2D-M411}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/412.png}}{2D-M412}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/413.png}}{2D-M413}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/414.png}}{2D-M414}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/415.png}}{2D-M415}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/416.png}}{2D-M416}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/417.png}}{2D-M417}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/418.png}}{2D-M418}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/419.png}}{2D-M419}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Part 2)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/420.png}}{2D-M420}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/421.png}}{2D-M421}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/422.png}}{2D-M422}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/423.png}}{2D-M423}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/424.png}}{2D-M424}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/425.png}}{2D-M425}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/426.png}}{2D-M426}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/427.png}}{2D-M427}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/428.png}}{2D-M428}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/429.png}}{2D-M429}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/430.png}}{2D-M430}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/431.png}}{2D-M431}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/432.png}}{2D-M432}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/433.png}}{2D-M433}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/434.png}}{2D-M434}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/435.png}}{2D-M435}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/436.png}}{2D-M436}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/437.png}}{2D-M437}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/438.png}}{2D-M438}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/439.png}}{2D-M439}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/440.png}}{2D-M440}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/441.png}}{2D-M441}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/442.png}}{2D-M442}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/443.png}}{2D-M443}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/444.png}}{2D-M444}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/445.png}}{2D-M445}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/446.png}}{2D-M446}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/447.png}}{2D-M447}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/448.png}}{2D-M448}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/449.png}}{2D-M449}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/450.png}}{2D-M450}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/451.png}}{2D-M451}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/452.png}}{2D-M452}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/453.png}}{2D-M453}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/454.png}}{2D-M454}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/455.png}}{2D-M455}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/456.png}}{2D-M456}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/457.png}}{2D-M457}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/458.png}}{2D-M458}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/459.png}}{2D-M459}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/460.png}}{2D-M460}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/461.png}}{2D-M461}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/462.png}}{2D-M462}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/463.png}}{2D-M463}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/464.png}}{2D-M464}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/465.png}}{2D-M465}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/466.png}}{2D-M466}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/467.png}}{2D-M467}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/468.png}}{2D-M468}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/469.png}}{2D-M469}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Part 3)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/470.png}}{2D-M470}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/471.png}}{2D-M471}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/472.png}}{2D-M472}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/473.png}}{2D-M473}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/474.png}}{2D-M474}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/475.png}}{2D-M475}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/476.png}}{2D-M476}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/477.png}}{2D-M477}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/478.png}}{2D-M478}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/479.png}}{2D-M479}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/480.png}}{2D-M480}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/481.png}}{2D-M481}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/482.png}}{2D-M482}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/483.png}}{2D-M483}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/484.png}}{2D-M484}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/485.png}}{2D-M485}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/486.png}}{2D-M486}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/487.png}}{2D-M487}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/488.png}}{2D-M488}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/489.png}}{2D-M489}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/490.png}}{2D-M490}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/491.png}}{2D-M491}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/492.png}}{2D-M492}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/493.png}}{2D-M493}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/494.png}}{2D-M494}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/495.png}}{2D-M495}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/496.png}}{2D-M496}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/497.png}}{2D-M497}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/498.png}}{2D-M498}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/499.png}}{2D-M499}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/500.png}}{2D-M500}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/501.png}}{2D-M501}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/502.png}}{2D-M502}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/503.png}}{2D-M503}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/504.png}}{2D-M504}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/505.png}}{2D-M505}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/506.png}}{2D-M506}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/507.png}}{2D-M507}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/508.png}}{2D-M508}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/509.png}}{2D-M509}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/510.png}}{2D-M510}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/511.png}}{2D-M511}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Part 4)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/512.png}}{2D-M512}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/513.png}}{2D-M513}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/514.png}}{2D-M514}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/515.png}}{2D-M515}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/516.png}}{2D-M516}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/517.png}}{2D-M517}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/518.png}}{2D-M518}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/519.png}}{2D-M519}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/520.png}}{2D-M520}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/521.png}}{2D-M521}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/522.png}}{2D-M522}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/523.png}}{2D-M523}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/524.png}}{2D-M524}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/525.png}}{2D-M525}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/526.png}}{2D-M526}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/527.png}}{2D-M527}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/528.png}}{2D-M528}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/529.png}}{2D-M529}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/530.png}}{2D-M530}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/531.png}}{2D-M531}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/532.png}}{2D-M532}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/533.png}}{2D-M533}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/534.png}}{2D-M534}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/535.png}}{2D-M535}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/536.png}}{2D-M536}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/537.png}}{2D-M537}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/538.png}}{2D-M538}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/539.png}}{2D-M539}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/540.png}}{2D-M540}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/541.png}}{2D-M541}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/542.png}}{2D-M542}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/543.png}}{2D-M543}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/544.png}}{2D-M544}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/545.png}}{2D-M545}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/546.png}}{2D-M546}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/547.png}}{2D-M547}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/548.png}}{2D-M548}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/549.png}}{2D-M549}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/550.png}}{2D-M550}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/551.png}}{2D-M551}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/552.png}}{2D-M552}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/553.png}}{2D-M553}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/554.png}}{2D-M554}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/555.png}}{2D-M555}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/556.png}}{2D-M556}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/557.png}}{2D-M557}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/558.png}}{2D-M558}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/559.png}}{2D-M559}

  \end{minipage}
\end{subfigure}
\caption{Class 9 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/560.png}}{2D-M560}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/561.png}}{2D-M561}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/562.png}}{2D-M562}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/563.png}}{2D-M563}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/564.png}}{2D-M564}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/565.png}}{2D-M565}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/566.png}}{2D-M566}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/567.png}}{2D-M567}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/568.png}}{2D-M568}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/569.png}}{2D-M569}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/570.png}}{2D-M570}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/571.png}}{2D-M571}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/572.png}}{2D-M572}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/573.png}}{2D-M573}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/574.png}}{2D-M574}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/575.png}}{2D-M575}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/576.png}}{2D-M576}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/577.png}}{2D-M577}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/578.png}}{2D-M578}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/579.png}}{2D-M579}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/580.png}}{2D-M580}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/581.png}}{2D-M581}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/582.png}}{2D-M582}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/583.png}}{2D-M583}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/584.png}}{2D-M584}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/585.png}}{2D-M585}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/586.png}}{2D-M586}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/587.png}}{2D-M587}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/588.png}}{2D-M588}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/589.png}}{2D-M589}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/590.png}}{2D-M590}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/591.png}}{2D-M591}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/592.png}}{2D-M592}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/593.png}}{2D-M593}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/594.png}}{2D-M594}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/595.png}}{2D-M595}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/596.png}}{2D-M596}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/597.png}}{2D-M597}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/598.png}}{2D-M598}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/599.png}}{2D-M599}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/600.png}}{2D-M600}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/601.png}}{2D-M601}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/602.png}}{2D-M602}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/603.png}}{2D-M603}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/604.png}}{2D-M604}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/605.png}}{2D-M605}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/606.png}}{2D-M606}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/607.png}}{2D-M607}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/608.png}}{2D-M608}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/609.png}}{2D-M609}

  \end{minipage}
\end{subfigure}
\caption{Class 10 of 2-DOF Manipulators (Part 1)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/610.png}}{2D-M610}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/611.png}}{2D-M611}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/612.png}}{2D-M612}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/613.png}}{2D-M613}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/614.png}}{2D-M614}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/615.png}}{2D-M615}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/616.png}}{2D-M616}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/617.png}}{2D-M617}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/618.png}}{2D-M618}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/619.png}}{2D-M619}

  \end{minipage}
\end{subfigure}
\caption{Class 10 of 2-DOF Manipulators (Part 2)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/620.png}}{2D-M620}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/621.png}}{2D-M621}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/622.png}}{2D-M622}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/623.png}}{2D-M623}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/624.png}}{2D-M624}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/625.png}}{2D-M625}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/626.png}}{2D-M626}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/627.png}}{2D-M627}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/628.png}}{2D-M628}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/629.png}}{2D-M629}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/630.png}}{2D-M630}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/631.png}}{2D-M631}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/632.png}}{2D-M632}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/633.png}}{2D-M633}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/634.png}}{2D-M634}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/635.png}}{2D-M635}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/636.png}}{2D-M636}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/637.png}}{2D-M637}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/638.png}}{2D-M638}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/639.png}}{2D-M639}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/640.png}}{2D-M640}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/641.png}}{2D-M641}

  \end{minipage}
\end{subfigure}
\caption{Class 11 of 2-DOF Manipulators}
\end{figure}



==> Dimensional Synthesis/2dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/1.png}}{2D-M1}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/2.png}}{2D-M2}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/3.png}}{2D-M3}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/4.png}}{2D-M4}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/5.png}}{2D-M5}

  \end{minipage}
\end{subfigure}
\caption{Class 1 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/6.png}}{2D-M6}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/7.png}}{2D-M7}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/8.png}}{2D-M8}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/9.png}}{2D-M9}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/10.png}}{2D-M10}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/11.png}}{2D-M11}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/12.png}}{2D-M12}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/13.png}}{2D-M13}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/14.png}}{2D-M14}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/15.png}}{2D-M15}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/16.png}}{2D-M16}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/17.png}}{2D-M17}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/18.png}}{2D-M18}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/19.png}}{2D-M19}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/20.png}}{2D-M20}

  \end{minipage}
\end{subfigure}
\caption{Class 2 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/21.png}}{2D-M21}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/22.png}}{2D-M22}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/23.png}}{2D-M23}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/24.png}}{2D-M24}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/25.png}}{2D-M25}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/26.png}}{2D-M26}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/27.png}}{2D-M27}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/28.png}}{2D-M28}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/29.png}}{2D-M29}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/30.png}}{2D-M30}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/31.png}}{2D-M31}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/32.png}}{2D-M32}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/33.png}}{2D-M33}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/34.png}}{2D-M34}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/35.png}}{2D-M35}

  \end{minipage}
\end{subfigure}
\caption{Class 3 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/36.png}}{2D-M36}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/37.png}}{2D-M37}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/38.png}}{2D-M38}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/39.png}}{2D-M39}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/40.png}}{2D-M40}

  \end{minipage}
\end{subfigure}
\caption{Class 4 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/41.png}}{2D-M41}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/42.png}}{2D-M42}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/43.png}}{2D-M43}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/44.png}}{2D-M44}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/45.png}}{2D-M45}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/46.png}}{2D-M46}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/47.png}}{2D-M47}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/48.png}}{2D-M48}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/49.png}}{2D-M49}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/50.png}}{2D-M50}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/51.png}}{2D-M51}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/52.png}}{2D-M52}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/53.png}}{2D-M53}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/54.png}}{2D-M54}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/55.png}}{2D-M55}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/56.png}}{2D-M56}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/57.png}}{2D-M57}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/58.png}}{2D-M58}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/59.png}}{2D-M59}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/60.png}}{2D-M60}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/61.png}}{2D-M61}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/62.png}}{2D-M62}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/63.png}}{2D-M63}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/64.png}}{2D-M64}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/65.png}}{2D-M65}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/66.png}}{2D-M66}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/67.png}}{2D-M67}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/68.png}}{2D-M68}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/69.png}}{2D-M69}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/70.png}}{2D-M70}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/71.png}}{2D-M71}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/72.png}}{2D-M72}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/73.png}}{2D-M73}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/74.png}}{2D-M74}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/75.png}}{2D-M75}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/76.png}}{2D-M76}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/77.png}}{2D-M77}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/78.png}}{2D-M78}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/79.png}}{2D-M79}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/80.png}}{2D-M80}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/81.png}}{2D-M81}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/82.png}}{2D-M82}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/83.png}}{2D-M83}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/84.png}}{2D-M84}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/85.png}}{2D-M85}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/86.png}}{2D-M86}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/87.png}}{2D-M87}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/88.png}}{2D-M88}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/89.png}}{2D-M89}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/90.png}}{2D-M90}

  \end{minipage}
\end{subfigure}
\caption{Class 5 of 2-DOF Manipulators (Part 1)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/91.png}}{2D-M91}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/92.png}}{2D-M92}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/93.png}}{2D-M93}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/94.png}}{2D-M94}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/95.png}}{2D-M95}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/96.png}}{2D-M96}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/97.png}}{2D-M97}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/98.png}}{2D-M98}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/99.png}}{2D-M99}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/100.png}}{2D-M100}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/101.png}}{2D-M101}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/102.png}}{2D-M102}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/103.png}}{2D-M103}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/104.png}}{2D-M104}

  \end{minipage}
\end{subfigure}
\caption{Class 5 of 2-DOF Manipulators (Part 2)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/105.png}}{2D-M105}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/106.png}}{2D-M106}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/107.png}}{2D-M107}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/108.png}}{2D-M108}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/109.png}}{2D-M109}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/110.png}}{2D-M110}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/111.png}}{2D-M111}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/112.png}}{2D-M112}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/113.png}}{2D-M113}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/114.png}}{2D-M114}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/115.png}}{2D-M115}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/116.png}}{2D-M116}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/117.png}}{2D-M117}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/118.png}}{2D-M118}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/119.png}}{2D-M119}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/120.png}}{2D-M120}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/121.png}}{2D-M121}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/122.png}}{2D-M122}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/123.png}}{2D-M123}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/124.png}}{2D-M124}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/125.png}}{2D-M125}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/126.png}}{2D-M126}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/127.png}}{2D-M127}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/128.png}}{2D-M128}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/129.png}}{2D-M129}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/130.png}}{2D-M130}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/131.png}}{2D-M131}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/132.png}}{2D-M132}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/133.png}}{2D-M133}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/134.png}}{2D-M134}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/135.png}}{2D-M135}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/136.png}}{2D-M136}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/137.png}}{2D-M137}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/138.png}}{2D-M138}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/139.png}}{2D-M139}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/140.png}}{2D-M140}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/141.png}}{2D-M141}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/142.png}}{2D-M142}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/143.png}}{2D-M143}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/144.png}}{2D-M144}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/145.png}}{2D-M145}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/146.png}}{2D-M146}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/147.png}}{2D-M147}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/148.png}}{2D-M148}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/149.png}}{2D-M149}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/150.png}}{2D-M150}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/151.png}}{2D-M151}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/152.png}}{2D-M152}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/153.png}}{2D-M153}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/154.png}}{2D-M154}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Part 1)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/155.png}}{2D-M155}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/156.png}}{2D-M156}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/157.png}}{2D-M157}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/158.png}}{2D-M158}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/159.png}}{2D-M159}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/160.png}}{2D-M160}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/161.png}}{2D-M161}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/162.png}}{2D-M162}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/163.png}}{2D-M163}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/164.png}}{2D-M164}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/165.png}}{2D-M165}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/166.png}}{2D-M166}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/167.png}}{2D-M167}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/168.png}}{2D-M168}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/169.png}}{2D-M169}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/170.png}}{2D-M170}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/171.png}}{2D-M171}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/172.png}}{2D-M172}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/173.png}}{2D-M173}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/174.png}}{2D-M174}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/175.png}}{2D-M175}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/176.png}}{2D-M176}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/177.png}}{2D-M177}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/178.png}}{2D-M178}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/179.png}}{2D-M179}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/180.png}}{2D-M180}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/181.png}}{2D-M181}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/182.png}}{2D-M182}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/183.png}}{2D-M183}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/184.png}}{2D-M184}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/185.png}}{2D-M185}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/186.png}}{2D-M186}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/187.png}}{2D-M187}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/188.png}}{2D-M188}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/189.png}}{2D-M189}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/190.png}}{2D-M190}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/191.png}}{2D-M191}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/192.png}}{2D-M192}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/193.png}}{2D-M193}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/194.png}}{2D-M194}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/195.png}}{2D-M195}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/196.png}}{2D-M196}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/197.png}}{2D-M197}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/198.png}}{2D-M198}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/199.png}}{2D-M199}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/200.png}}{2D-M200}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/201.png}}{2D-M201}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/202.png}}{2D-M202}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/203.png}}{2D-M203}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/204.png}}{2D-M204}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Part 2)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/205.png}}{2D-M205}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/206.png}}{2D-M206}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/207.png}}{2D-M207}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/208.png}}{2D-M208}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/209.png}}{2D-M209}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/210.png}}{2D-M210}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/211.png}}{2D-M211}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/212.png}}{2D-M212}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/213.png}}{2D-M213}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/214.png}}{2D-M214}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/215.png}}{2D-M215}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/216.png}}{2D-M216}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/217.png}}{2D-M217}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/218.png}}{2D-M218}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/219.png}}{2D-M219}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/220.png}}{2D-M220}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/221.png}}{2D-M221}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/222.png}}{2D-M222}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/223.png}}{2D-M223}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/224.png}}{2D-M224}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/225.png}}{2D-M225}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/226.png}}{2D-M226}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/227.png}}{2D-M227}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/228.png}}{2D-M228}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/229.png}}{2D-M229}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/230.png}}{2D-M230}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/231.png}}{2D-M231}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/232.png}}{2D-M232}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/233.png}}{2D-M233}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/234.png}}{2D-M234}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/235.png}}{2D-M235}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/236.png}}{2D-M236}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/237.png}}{2D-M237}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/238.png}}{2D-M238}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/239.png}}{2D-M239}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/240.png}}{2D-M240}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/241.png}}{2D-M241}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/242.png}}{2D-M242}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/243.png}}{2D-M243}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/244.png}}{2D-M244}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/245.png}}{2D-M245}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/246.png}}{2D-M246}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/247.png}}{2D-M247}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/248.png}}{2D-M248}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/249.png}}{2D-M249}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/250.png}}{2D-M250}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/251.png}}{2D-M251}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/252.png}}{2D-M252}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/253.png}}{2D-M253}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/254.png}}{2D-M254}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Part 3)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/255.png}}{2D-M255}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/256.png}}{2D-M256}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/257.png}}{2D-M257}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/258.png}}{2D-M258}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/259.png}}{2D-M259}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/260.png}}{2D-M260}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/261.png}}{2D-M261}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/262.png}}{2D-M262}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/263.png}}{2D-M263}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/264.png}}{2D-M264}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/265.png}}{2D-M265}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/266.png}}{2D-M266}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/267.png}}{2D-M267}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/268.png}}{2D-M268}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/269.png}}{2D-M269}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/270.png}}{2D-M270}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/271.png}}{2D-M271}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/272.png}}{2D-M272}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/273.png}}{2D-M273}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/274.png}}{2D-M274}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/275.png}}{2D-M275}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/276.png}}{2D-M276}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/277.png}}{2D-M277}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/278.png}}{2D-M278}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/279.png}}{2D-M279}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/280.png}}{2D-M280}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/281.png}}{2D-M281}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/282.png}}{2D-M282}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/283.png}}{2D-M283}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/284.png}}{2D-M284}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/285.png}}{2D-M285}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/286.png}}{2D-M286}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/287.png}}{2D-M287}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/288.png}}{2D-M288}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/289.png}}{2D-M289}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/290.png}}{2D-M290}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/291.png}}{2D-M291}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/292.png}}{2D-M292}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/293.png}}{2D-M293}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/294.png}}{2D-M294}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/295.png}}{2D-M295}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/296.png}}{2D-M296}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Part 4)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/297.png}}{2D-M297}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/298.png}}{2D-M298}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/299.png}}{2D-M299}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/300.png}}{2D-M300}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/301.png}}{2D-M301}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/302.png}}{2D-M302}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/303.png}}{2D-M303}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/304.png}}{2D-M304}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/305.png}}{2D-M305}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/306.png}}{2D-M306}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/307.png}}{2D-M307}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/308.png}}{2D-M308}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/309.png}}{2D-M309}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/310.png}}{2D-M310}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/311.png}}{2D-M311}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/312.png}}{2D-M312}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/313.png}}{2D-M313}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/314.png}}{2D-M314}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/315.png}}{2D-M315}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/316.png}}{2D-M316}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/317.png}}{2D-M317}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/318.png}}{2D-M318}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/319.png}}{2D-M319}

  \end{minipage}
\end{subfigure}
\caption{Class 7 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/320.png}}{2D-M320}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/321.png}}{2D-M321}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/322.png}}{2D-M322}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/323.png}}{2D-M323}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/324.png}}{2D-M324}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/325.png}}{2D-M325}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/326.png}}{2D-M326}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/327.png}}{2D-M327}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/328.png}}{2D-M328}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/329.png}}{2D-M329}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/330.png}}{2D-M330}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/331.png}}{2D-M331}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/332.png}}{2D-M332}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/333.png}}{2D-M333}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/334.png}}{2D-M334}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/335.png}}{2D-M335}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/336.png}}{2D-M336}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/337.png}}{2D-M337}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/338.png}}{2D-M338}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/339.png}}{2D-M339}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/340.png}}{2D-M340}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/341.png}}{2D-M341}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/342.png}}{2D-M342}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/343.png}}{2D-M343}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/344.png}}{2D-M344}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/345.png}}{2D-M345}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/346.png}}{2D-M346}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/347.png}}{2D-M347}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/348.png}}{2D-M348}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/349.png}}{2D-M349}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/350.png}}{2D-M350}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/351.png}}{2D-M351}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/352.png}}{2D-M352}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/353.png}}{2D-M353}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/354.png}}{2D-M354}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/355.png}}{2D-M355}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/356.png}}{2D-M356}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/357.png}}{2D-M357}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/358.png}}{2D-M358}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/359.png}}{2D-M359}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/360.png}}{2D-M360}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/361.png}}{2D-M361}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/362.png}}{2D-M362}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/363.png}}{2D-M363}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/364.png}}{2D-M364}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/365.png}}{2D-M365}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/366.png}}{2D-M366}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/367.png}}{2D-M367}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/368.png}}{2D-M368}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/369.png}}{2D-M369}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Part 1)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/370.png}}{2D-M370}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/371.png}}{2D-M371}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/372.png}}{2D-M372}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/373.png}}{2D-M373}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/374.png}}{2D-M374}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/375.png}}{2D-M375}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/376.png}}{2D-M376}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/377.png}}{2D-M377}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/378.png}}{2D-M378}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/379.png}}{2D-M379}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/380.png}}{2D-M380}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/381.png}}{2D-M381}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/382.png}}{2D-M382}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/383.png}}{2D-M383}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/384.png}}{2D-M384}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/385.png}}{2D-M385}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/386.png}}{2D-M386}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/387.png}}{2D-M387}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/388.png}}{2D-M388}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/389.png}}{2D-M389}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/390.png}}{2D-M390}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/391.png}}{2D-M391}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/392.png}}{2D-M392}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/393.png}}{2D-M393}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/394.png}}{2D-M394}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/395.png}}{2D-M395}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/396.png}}{2D-M396}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/397.png}}{2D-M397}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/398.png}}{2D-M398}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/399.png}}{2D-M399}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/400.png}}{2D-M400}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/401.png}}{2D-M401}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/402.png}}{2D-M402}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/403.png}}{2D-M403}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/404.png}}{2D-M404}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/405.png}}{2D-M405}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/406.png}}{2D-M406}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/407.png}}{2D-M407}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/408.png}}{2D-M408}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/409.png}}{2D-M409}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/410.png}}{2D-M410}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/411.png}}{2D-M411}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/412.png}}{2D-M412}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/413.png}}{2D-M413}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/414.png}}{2D-M414}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/415.png}}{2D-M415}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/416.png}}{2D-M416}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/417.png}}{2D-M417}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/418.png}}{2D-M418}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/419.png}}{2D-M419}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Part 2)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/420.png}}{2D-M420}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/421.png}}{2D-M421}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/422.png}}{2D-M422}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/423.png}}{2D-M423}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/424.png}}{2D-M424}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/425.png}}{2D-M425}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/426.png}}{2D-M426}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/427.png}}{2D-M427}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/428.png}}{2D-M428}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/429.png}}{2D-M429}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/430.png}}{2D-M430}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/431.png}}{2D-M431}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/432.png}}{2D-M432}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/433.png}}{2D-M433}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/434.png}}{2D-M434}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/435.png}}{2D-M435}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/436.png}}{2D-M436}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/437.png}}{2D-M437}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/438.png}}{2D-M438}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/439.png}}{2D-M439}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/440.png}}{2D-M440}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/441.png}}{2D-M441}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/442.png}}{2D-M442}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/443.png}}{2D-M443}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/444.png}}{2D-M444}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/445.png}}{2D-M445}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/446.png}}{2D-M446}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/447.png}}{2D-M447}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/448.png}}{2D-M448}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/449.png}}{2D-M449}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/450.png}}{2D-M450}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/451.png}}{2D-M451}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/452.png}}{2D-M452}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/453.png}}{2D-M453}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/454.png}}{2D-M454}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/455.png}}{2D-M455}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/456.png}}{2D-M456}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/457.png}}{2D-M457}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/458.png}}{2D-M458}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/459.png}}{2D-M459}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/460.png}}{2D-M460}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/461.png}}{2D-M461}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/462.png}}{2D-M462}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/463.png}}{2D-M463}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/464.png}}{2D-M464}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/465.png}}{2D-M465}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/466.png}}{2D-M466}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/467.png}}{2D-M467}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/468.png}}{2D-M468}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/469.png}}{2D-M469}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Part 3)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/470.png}}{2D-M470}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/471.png}}{2D-M471}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/472.png}}{2D-M472}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/473.png}}{2D-M473}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/474.png}}{2D-M474}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/475.png}}{2D-M475}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/476.png}}{2D-M476}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/477.png}}{2D-M477}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/478.png}}{2D-M478}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/479.png}}{2D-M479}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/480.png}}{2D-M480}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/481.png}}{2D-M481}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/482.png}}{2D-M482}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/483.png}}{2D-M483}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/484.png}}{2D-M484}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/485.png}}{2D-M485}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/486.png}}{2D-M486}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/487.png}}{2D-M487}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/488.png}}{2D-M488}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/489.png}}{2D-M489}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/490.png}}{2D-M490}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/491.png}}{2D-M491}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/492.png}}{2D-M492}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/493.png}}{2D-M493}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/494.png}}{2D-M494}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/495.png}}{2D-M495}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/496.png}}{2D-M496}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/497.png}}{2D-M497}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/498.png}}{2D-M498}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/499.png}}{2D-M499}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/500.png}}{2D-M500}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/501.png}}{2D-M501}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/502.png}}{2D-M502}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/503.png}}{2D-M503}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/504.png}}{2D-M504}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/505.png}}{2D-M505}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/506.png}}{2D-M506}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/507.png}}{2D-M507}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/508.png}}{2D-M508}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/509.png}}{2D-M509}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/510.png}}{2D-M510}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/511.png}}{2D-M511}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Part 4)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/512.png}}{2D-M512}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/513.png}}{2D-M513}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/514.png}}{2D-M514}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/515.png}}{2D-M515}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/516.png}}{2D-M516}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/517.png}}{2D-M517}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/518.png}}{2D-M518}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/519.png}}{2D-M519}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/520.png}}{2D-M520}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/521.png}}{2D-M521}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/522.png}}{2D-M522}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/523.png}}{2D-M523}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/524.png}}{2D-M524}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/525.png}}{2D-M525}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/526.png}}{2D-M526}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/527.png}}{2D-M527}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/528.png}}{2D-M528}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/529.png}}{2D-M529}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/530.png}}{2D-M530}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/531.png}}{2D-M531}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/532.png}}{2D-M532}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/533.png}}{2D-M533}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/534.png}}{2D-M534}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/535.png}}{2D-M535}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/536.png}}{2D-M536}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/537.png}}{2D-M537}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/538.png}}{2D-M538}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/539.png}}{2D-M539}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/540.png}}{2D-M540}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/541.png}}{2D-M541}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/542.png}}{2D-M542}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/543.png}}{2D-M543}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/544.png}}{2D-M544}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/545.png}}{2D-M545}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/546.png}}{2D-M546}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/547.png}}{2D-M547}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/548.png}}{2D-M548}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/549.png}}{2D-M549}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/550.png}}{2D-M550}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/551.png}}{2D-M551}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/552.png}}{2D-M552}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/553.png}}{2D-M553}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/554.png}}{2D-M554}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/555.png}}{2D-M555}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/556.png}}{2D-M556}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/557.png}}{2D-M557}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/558.png}}{2D-M558}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/559.png}}{2D-M559}

  \end{minipage}
\end{subfigure}
\caption{Class 9 of 2-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/560.png}}{2D-M560}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/561.png}}{2D-M561}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/562.png}}{2D-M562}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/563.png}}{2D-M563}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/564.png}}{2D-M564}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/565.png}}{2D-M565}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/566.png}}{2D-M566}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/567.png}}{2D-M567}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/568.png}}{2D-M568}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/569.png}}{2D-M569}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/570.png}}{2D-M570}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/571.png}}{2D-M571}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/572.png}}{2D-M572}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/573.png}}{2D-M573}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/574.png}}{2D-M574}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/575.png}}{2D-M575}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/576.png}}{2D-M576}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/577.png}}{2D-M577}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/578.png}}{2D-M578}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/579.png}}{2D-M579}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/580.png}}{2D-M580}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/581.png}}{2D-M581}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/582.png}}{2D-M582}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/583.png}}{2D-M583}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/584.png}}{2D-M584}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/585.png}}{2D-M585}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/586.png}}{2D-M586}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/587.png}}{2D-M587}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/588.png}}{2D-M588}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/589.png}}{2D-M589}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/590.png}}{2D-M590}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/591.png}}{2D-M591}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/592.png}}{2D-M592}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/593.png}}{2D-M593}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/594.png}}{2D-M594}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/595.png}}{2D-M595}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/596.png}}{2D-M596}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/597.png}}{2D-M597}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/598.png}}{2D-M598}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/599.png}}{2D-M599}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/600.png}}{2D-M600}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/601.png}}{2D-M601}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/602.png}}{2D-M602}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/603.png}}{2D-M603}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/604.png}}{2D-M604}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/605.png}}{2D-M605}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/606.png}}{2D-M606}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/607.png}}{2D-M607}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/608.png}}{2D-M608}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/609.png}}{2D-M609}

  \end{minipage}
\end{subfigure}
\caption{Class 10 of 2-DOF Manipulators (Part 1)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/610.png}}{2D-M610}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/611.png}}{2D-M611}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/612.png}}{2D-M612}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/613.png}}{2D-M613}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/614.png}}{2D-M614}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/615.png}}{2D-M615}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/616.png}}{2D-M616}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/617.png}}{2D-M617}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/618.png}}{2D-M618}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/619.png}}{2D-M619}

  \end{minipage}
\end{subfigure}
\caption{Class 10 of 2-DOF Manipulators (Part 2)}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/620.png}}{2D-M620}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/621.png}}{2D-M621}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/622.png}}{2D-M622}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/623.png}}{2D-M623}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/624.png}}{2D-M624}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/625.png}}{2D-M625}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/626.png}}{2D-M626}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/627.png}}{2D-M627}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/628.png}}{2D-M628}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/629.png}}{2D-M629}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/630.png}}{2D-M630}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/631.png}}{2D-M631}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/632.png}}{2D-M632}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/633.png}}{2D-M633}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/634.png}}{2D-M634}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/635.png}}{2D-M635}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/636.png}}{2D-M636}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/637.png}}{2D-M637}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/638.png}}{2D-M638}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/639.png}}{2D-M639}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/640.png}}{2D-M640}
\qquad\subsubfloat{\includegraphics[width=0.15\textwidth]{pictures/641.png}}{2D-M641}

  \end{minipage}
\end{subfigure}
\caption{Class 11 of 2-DOF Manipulators}
\end{figure}



==> Dimensional Synthesis/classes/1dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/1.png}}{{\tiny 1D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/2.png}}{{\tiny 1D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/3.png}}{{\tiny 1D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/4.png}}{{\tiny 1D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/5.png}}{{\tiny 1D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/6.png}}{{\tiny 1D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/7.png}}{{\tiny 1D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/8.png}}{{\tiny 1D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/9.png}}{{\tiny 1D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/10.png}}{{\tiny 1D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/11.png}}{{\tiny 1D-M11}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/12.png}}{{\tiny 1D-M12}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/13.png}}{{\tiny 1D-M13}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/14.png}}{{\tiny 1D-M14}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/15.png}}{{\tiny 1D-M15}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/16.png}}{{\tiny 1D-M16}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/17.png}}{{\tiny 1D-M17}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/18.png}}{{\tiny 1D-M18}}
\qquad \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/19.png}}{{\tiny 1D-M19}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/20.png}}{{\tiny 1D-M20}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/21.png}}{{\tiny 1D-M21}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/22.png}}{{\tiny 1D-M22}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/23.png}}{{\tiny 1D-M23}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/24.png}}{{\tiny 1D-M24}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/25.png}}{{\tiny 1D-M25}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/26.png}}{{\tiny 1D-M26}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/27.png}}{{\tiny 1D-M27}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/28.png}}{{\tiny 1D-M28}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/29.png}}{{\tiny 1D-M29}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/30.png}}{{\tiny 1D-M30}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/31.png}}{{\tiny 1D-M31}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/32.png}}{{\tiny 1D-M32}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/33.png}}{{\tiny 1D-M33}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/34.png}}{{\tiny 1D-M34}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/35.png}}{{\tiny 1D-M35}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/36.png}}{{\tiny 1D-M36}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/37.png}}{{\tiny 1D-M37}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/38.png}}{{\tiny 1D-M38}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/39.png}}{{\tiny 1D-M39}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/40.png}}{{\tiny 1D-M40}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/41.png}}{{\tiny 1D-M41}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/42.png}}{{\tiny 1D-M42}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/43.png}}{{\tiny 1D-M43}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/44.png}}{{\tiny 1D-M44}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/45.png}}{{\tiny 1D-M45}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/46.png}}{{\tiny 1D-M46}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/47.png}}{{\tiny 1D-M47}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/48.png}}{{\tiny 1D-M48}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/49.png}}{{\tiny 1D-M49}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/50.png}}{{\tiny 1D-M50}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/51.png}}{{\tiny 1D-M51}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/52.png}}{{\tiny 1D-M52}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/53.png}}{{\tiny 1D-M53}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/54.png}}{{\tiny 1D-M54}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/55.png}}{{\tiny 1D-M55}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/56.png}}{{\tiny 1D-M56}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/57.png}}{{\tiny 1D-M57}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/58.png}}{{\tiny 1D-M58}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/59.png}}{{\tiny 1D-M59}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/60.png}}{{\tiny 1D-M60}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/61.png}}{{\tiny 1D-M61}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/62.png}}{{\tiny 1D-M62}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/63.png}}{{\tiny 1D-M63}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/64.png}}{{\tiny 1D-M64}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/65.png}}{{\tiny 1D-M65}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/66.png}}{{\tiny 1D-M66}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/67.png}}{{\tiny 1D-M67}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/68.png}}{{\tiny 1D-M68}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/69.png}}{{\tiny 1D-M69}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/70.png}}{{\tiny 1D-M70}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/71.png}}{{\tiny 1D-M71}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/72.png}}{{\tiny 1D-M72}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/73.png}}{{\tiny 1D-M73}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/74.png}}{{\tiny 1D-M74}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/75.png}}{{\tiny 1D-M75}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/76.png}}{{\tiny 1D-M76}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/77.png}}{{\tiny 1D-M77}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/78.png}}{{\tiny 1D-M78}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/79.png}}{{\tiny 1D-M79}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/80.png}}{{\tiny 1D-M80}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/81.png}}{{\tiny 1D-M81}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/82.png}}{{\tiny 1D-M82}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/83.png}}{{\tiny 1D-M83}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/84.png}}{{\tiny 1D-M84}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/85.png}}{{\tiny 1D-M85}}
\qquad\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/86.png}}{{\tiny 1D-M86}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/87.png}}{{\tiny 1D-M87}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/88.png}}{{\tiny 1D-M88}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/89.png}}{{\tiny 1D-M89}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/90.png}}{{\tiny 1D-M90}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/91.png}}{{\tiny 1D-M91}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/92.png}}{{\tiny 1D-M92}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/93.png}}{{\tiny 1D-M93}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/94.png}}{{\tiny 1D-M94}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/95.png}}{{\tiny 1D-M95}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/96.png}}{{\tiny 1D-M96}}

  \end{minipage}
\end{subfigure}
\caption{Schematic diagrams of 1-DOF Manipulators}
\end{figure}

% \begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering

% \end{minipage}
% \end{subfigure}
% \caption{Class 2 of 1-DOF Manipulators}
% \end{figure}\begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering





%   \end{minipage}
% \end{subfigure}
% \caption{Class 3 of 1-DOF Manipulators}
% \end{figure}

% \begin{figure}[H]\ContinuedFloat
%   \centering
%   \begin{subfigure}{\columnwidth}
%     \begin{minipage}{\textwidth}\footnotesize
%     \centering

  
%     \end{minipage}
%   \end{subfigure}
%   \caption{Class 3 of 1-DOF Manipulators (Contd.)}
%   \end{figure}

% \begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 4 of 1-DOF Manipulators}
% \end{figure}\begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 5 of 1-DOF Manipulators}
% \end{figure}

% \begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 6 of 1-DOF Manipulators}
% \end{figure}

% \begin{figure}[H]\ContinuedFloat
%   \centering
%   \begin{subfigure}{\columnwidth}
%     \begin{minipage}{\textwidth}\footnotesize
%     \centering

  
  
%     \end{minipage}
%   \end{subfigure}
%   \caption{Class 6 of 1-DOF Manipulators (Contd.)}
%   \end{figure}

% \begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 7 of 1-DOF Manipulators}
% \end{figure}\begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 8 of 1-DOF Manipulators}
% \end{figure}

==> Dimensional Synthesis/classes/1dof_classes_old.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/1.png}}{{\tiny 1D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/2.png}}{{\tiny 1D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/3.png}}{{\tiny 1D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/4.png}}{{\tiny 1D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/5.png}}{{\tiny 1D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/6.png}}{{\tiny 1D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/7.png}}{{\tiny 1D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/8.png}}{{\tiny 1D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/9.png}}{{\tiny 1D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/10.png}}{{\tiny 1D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/11.png}}{{\tiny 1D-M11}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/12.png}}{{\tiny 1D-M12}}


  \end{minipage}
\end{subfigure}
\caption{Class 1 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/13.png}}{{\tiny 1D-M13}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/14.png}}{{\tiny 1D-M14}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/15.png}}{{\tiny 1D-M15}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/16.png}}{{\tiny 1D-M16}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/17.png}}{{\tiny 1D-M17}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/18.png}}{{\tiny 1D-M18}}
\qquad \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/19.png}}{{\tiny 1D-M19}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/20.png}}{{\tiny 1D-M20}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/21.png}}{{\tiny 1D-M21}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/22.png}}{{\tiny 1D-M22}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/23.png}}{{\tiny 1D-M23}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/24.png}}{{\tiny 1D-M24}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/25.png}}{{\tiny 1D-M25}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/26.png}}{{\tiny 1D-M26}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/27.png}}{{\tiny 1D-M27}}
\end{minipage}
\end{subfigure}
\caption{Class 2 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering


\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/28.png}}{{\tiny 1D-M28}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/29.png}}{{\tiny 1D-M29}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/30.png}}{{\tiny 1D-M30}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/31.png}}{{\tiny 1D-M31}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/32.png}}{{\tiny 1D-M32}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/33.png}}{{\tiny 1D-M33}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/34.png}}{{\tiny 1D-M34}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/35.png}}{{\tiny 1D-M35}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/36.png}}{{\tiny 1D-M36}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/37.png}}{{\tiny 1D-M37}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/38.png}}{{\tiny 1D-M38}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/39.png}}{{\tiny 1D-M39}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/40.png}}{{\tiny 1D-M40}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/41.png}}{{\tiny 1D-M41}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/42.png}}{{\tiny 1D-M42}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/43.png}}{{\tiny 1D-M43}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/44.png}}{{\tiny 1D-M44}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/45.png}}{{\tiny 1D-M45}}


  \end{minipage}
\end{subfigure}
\caption{Class 3 of 1-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/46.png}}{{\tiny 1D-M46}}
    \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/47.png}}{{\tiny 1D-M47}}
    \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/48.png}}{{\tiny 1D-M48}}
    \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/49.png}}{{\tiny 1D-M49}}
    \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/50.png}}{{\tiny 1D-M50}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/51.png}}{{\tiny 1D-M51}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/52.png}}{{\tiny 1D-M52}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/53.png}}{{\tiny 1D-M53}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/54.png}}{{\tiny 1D-M54}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/55.png}}{{\tiny 1D-M55}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/56.png}}{{\tiny 1D-M56}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/57.png}}{{\tiny 1D-M57}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 3 of 1-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/58.png}}{{\tiny 1D-M58}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/59.png}}{{\tiny 1D-M59}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/60.png}}{{\tiny 1D-M60}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/61.png}}{{\tiny 1D-M61}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/62.png}}{{\tiny 1D-M62}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/63.png}}{{\tiny 1D-M63}}

  \end{minipage}
\end{subfigure}
\caption{Class 4 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/64.png}}{{\tiny 1D-M64}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/65.png}}{{\tiny 1D-M65}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/66.png}}{{\tiny 1D-M66}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/67.png}}{{\tiny 1D-M67}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/68.png}}{{\tiny 1D-M68}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/69.png}}{{\tiny 1D-M69}}

  \end{minipage}
\end{subfigure}
\caption{Class 5 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/70.png}}{{\tiny 1D-M70}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/71.png}}{{\tiny 1D-M71}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/72.png}}{{\tiny 1D-M72}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/73.png}}{{\tiny 1D-M73}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/74.png}}{{\tiny 1D-M74}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/75.png}}{{\tiny 1D-M75}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/76.png}}{{\tiny 1D-M76}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/77.png}}{{\tiny 1D-M77}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/78.png}}{{\tiny 1D-M78}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/79.png}}{{\tiny 1D-M79}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/80.png}}{{\tiny 1D-M80}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/81.png}}{{\tiny 1D-M81}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/82.png}}{{\tiny 1D-M82}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/83.png}}{{\tiny 1D-M83}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/84.png}}{{\tiny 1D-M84}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/85.png}}{{\tiny 1D-M85}}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 1-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/86.png}}{{\tiny 1D-M86}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/87.png}}{{\tiny 1D-M87}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 1-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/88.png}}{{\tiny 1D-M88}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/89.png}}{{\tiny 1D-M89}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/90.png}}{{\tiny 1D-M90}}

  \end{minipage}
\end{subfigure}
\caption{Class 7 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/91.png}}{{\tiny 1D-M91}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/92.png}}{{\tiny 1D-M92}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/93.png}}{{\tiny 1D-M93}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/94.png}}{{\tiny 1D-M94}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/95.png}}{{\tiny 1D-M95}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/96.png}}{{\tiny 1D-M96}}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 1-DOF Manipulators}
\end{figure}

==> Dimensional Synthesis/classes/2dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/1.png}}{{\tiny 2D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/2.png}}{{\tiny 2D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/3.png}}{{\tiny 2D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/4.png}}{{\tiny 2D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/5.png}}{{\tiny 2D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/6.png}}{{\tiny 2D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/7.png}}{{\tiny 2D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/8.png}}{{\tiny 2D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/9.png}}{{\tiny 2D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/10.png}}{{\tiny 2D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/11.png}}{{\tiny 2D-M11}}    
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/12.png}}{{\tiny 2D-M12}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/13.png}}{{\tiny 2D-M13}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/14.png}}{{\tiny 2D-M14}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/15.png}}{{\tiny 2D-M15}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/16.png}}{{\tiny 2D-M16}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/17.png}}{{\tiny 2D-M17}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/18.png}}{{\tiny 2D-M18}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/19.png}}{{\tiny 2D-M19}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/20.png}}{{\tiny 2D-M20}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/21.png}}{{\tiny 2D-M21}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/22.png}}{{\tiny 2D-M22}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/23.png}}{{\tiny 2D-M23}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/24.png}}{{\tiny 2D-M24}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/25.png}}{{\tiny 2D-M25}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/26.png}}{{\tiny 2D-M26}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/27.png}}{{\tiny 2D-M27}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/28.png}}{{\tiny 2D-M28}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/29.png}}{{\tiny 2D-M29}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/30.png}}{{\tiny 2D-M30}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/31.png}}{{\tiny 2D-M31}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/32.png}}{{\tiny 2D-M32}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/33.png}}{{\tiny 2D-M33}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/34.png}}{{\tiny 2D-M34}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/35.png}}{{\tiny 2D-M35}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/36.png}}{{\tiny 2D-M36}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/37.png}}{{\tiny 2D-M37}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/38.png}}{{\tiny 2D-M38}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/39.png}}{{\tiny 2D-M39}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/40.png}}{{\tiny 2D-M40}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/41.png}}{{\tiny 2D-M41}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/42.png}}{{\tiny 2D-M42}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/43.png}}{{\tiny 2D-M43}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/44.png}}{{\tiny 2D-M44}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/45.png}}{{\tiny 2D-M45}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/46.png}}{{\tiny 2D-M46}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/47.png}}{{\tiny 2D-M47}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/48.png}}{{\tiny 2D-M48}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/49.png}}{{\tiny 2D-M49}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/50.png}}{{\tiny 2D-M50}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/51.png}}{{\tiny 2D-M51}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/52.png}}{{\tiny 2D-M52}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/53.png}}{{\tiny 2D-M53}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/54.png}}{{\tiny 2D-M54}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/55.png}}{{\tiny 2D-M55}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/56.png}}{{\tiny 2D-M56}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/57.png}}{{\tiny 2D-M57}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/58.png}}{{\tiny 2D-M58}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/59.png}}{{\tiny 2D-M59}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/60.png}}{{\tiny 2D-M60}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/61.png}}{{\tiny 2D-M61}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/62.png}}{{\tiny 2D-M62}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/63.png}}{{\tiny 2D-M63}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/64.png}}{{\tiny 2D-M64}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/65.png}}{{\tiny 2D-M65}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/66.png}}{{\tiny 2D-M66}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/67.png}}{{\tiny 2D-M67}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/68.png}}{{\tiny 2D-M68}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/69.png}}{{\tiny 2D-M69}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/70.png}}{{\tiny 2D-M70}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/71.png}}{{\tiny 2D-M71}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/72.png}}{{\tiny 2D-M72}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/73.png}}{{\tiny 2D-M73}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/74.png}}{{\tiny 2D-M74}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/75.png}}{{\tiny 2D-M75}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/76.png}}{{\tiny 2D-M76}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/77.png}}{{\tiny 2D-M77}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/78.png}}{{\tiny 2D-M78}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/79.png}}{{\tiny 2D-M79}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/80.png}}{{\tiny 2D-M80}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/81.png}}{{\tiny 2D-M81}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/82.png}}{{\tiny 2D-M82}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/83.png}}{{\tiny 2D-M83}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/84.png}}{{\tiny 2D-M84}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/85.png}}{{\tiny 2D-M85}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/86.png}}{{\tiny 2D-M86}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/87.png}}{{\tiny 2D-M87}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/88.png}}{{\tiny 2D-M88}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/89.png}}{{\tiny 2D-M89}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/90.png}}{{\tiny 2D-M90}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/91.png}}{{\tiny 2D-M91}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/92.png}}{{\tiny 2D-M92}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/93.png}}{{\tiny 2D-M93}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/94.png}}{{\tiny 2D-M94}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/95.png}}{{\tiny 2D-M95}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/96.png}}{{\tiny 2D-M96}} 
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/97.png}}{{\tiny 2D-M97}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/98.png}}{{\tiny 2D-M98}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/99.png}}{{\tiny 2D-M99}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/100.png}}{{\tiny 2D-M100}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/101.png}}{{\tiny 2D-M101}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/102.png}}{{\tiny 2D-M102}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/103.png}}{{\tiny 2D-M103}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/104.png}}{{\tiny 2D-M104}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/105.png}}{{\tiny 2D-M105}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/106.png}}{{\tiny 2D-M106}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/107.png}}{{\tiny 2D-M107}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/108.png}}{{\tiny 2D-M108}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/109.png}}{{\tiny 2D-M109}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/110.png}}{{\tiny 2D-M110}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/111.png}}{{\tiny 2D-M111}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/112.png}}{{\tiny 2D-M112}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/113.png}}{{\tiny 2D-M113}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/114.png}}{{\tiny 2D-M114}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/115.png}}{{\tiny 2D-M115}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/116.png}}{{\tiny 2D-M116}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/117.png}}{{\tiny 2D-M117}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/118.png}}{{\tiny 2D-M118}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/119.png}}{{\tiny 2D-M119}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/120.png}}{{\tiny 2D-M120}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/121.png}}{{\tiny 2D-M121}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/122.png}}{{\tiny 2D-M122}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/123.png}}{{\tiny 2D-M123}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/124.png}}{{\tiny 2D-M124}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/125.png}}{{\tiny 2D-M125}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/126.png}}{{\tiny 2D-M126}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/127.png}}{{\tiny 2D-M127}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/128.png}}{{\tiny 2D-M128}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/129.png}}{{\tiny 2D-M129}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/130.png}}{{\tiny 2D-M130}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/131.png}}{{\tiny 2D-M131}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/132.png}}{{\tiny 2D-M132}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/133.png}}{{\tiny 2D-M133}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/134.png}}{{\tiny 2D-M134}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/135.png}}{{\tiny 2D-M135}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/136.png}}{{\tiny 2D-M136}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/137.png}}{{\tiny 2D-M137}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/138.png}}{{\tiny 2D-M138}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/139.png}}{{\tiny 2D-M139}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/140.png}}{{\tiny 2D-M140}}
\qquad  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/141.png}}{{\tiny 2D-M141}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/142.png}}{{\tiny 2D-M142}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/143.png}}{{\tiny 2D-M143}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/144.png}}{{\tiny 2D-M144}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/145.png}}{{\tiny 2D-M145}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/146.png}}{{\tiny 2D-M146}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/147.png}}{{\tiny 2D-M147}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/148.png}}{{\tiny 2D-M148}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/149.png}}{{\tiny 2D-M149}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/150.png}}{{\tiny 2D-M150}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/151.png}}{{\tiny 2D-M151}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/152.png}}{{\tiny 2D-M152}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/153.png}}{{\tiny 2D-M153}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/154.png}}{{\tiny 2D-M154}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/155.png}}{{\tiny 2D-M155}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/156.png}}{{\tiny 2D-M156}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/157.png}}{{\tiny 2D-M157}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/158.png}}{{\tiny 2D-M158}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/159.png}}{{\tiny 2D-M159}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/160.png}}{{\tiny 2D-M160}} 
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/161.png}}{{\tiny 2D-M161}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/162.png}}{{\tiny 2D-M162}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/163.png}}{{\tiny 2D-M163}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/164.png}}{{\tiny 2D-M164}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/165.png}}{{\tiny 2D-M165}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/166.png}}{{\tiny 2D-M166}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/167.png}}{{\tiny 2D-M167}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/168.png}}{{\tiny 2D-M168}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/169.png}}{{\tiny 2D-M169}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/170.png}}{{\tiny 2D-M170}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/171.png}}{{\tiny 2D-M171}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/172.png}}{{\tiny 2D-M172}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/173.png}}{{\tiny 2D-M173}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/174.png}}{{\tiny 2D-M174}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/175.png}}{{\tiny 2D-M175}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/176.png}}{{\tiny 2D-M176}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/177.png}}{{\tiny 2D-M177}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/178.png}}{{\tiny 2D-M178}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/179.png}}{{\tiny 2D-M179}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/180.png}}{{\tiny 2D-M180}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/181.png}}{{\tiny 2D-M181}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/182.png}}{{\tiny 2D-M182}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/183.png}}{{\tiny 2D-M183}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/184.png}}{{\tiny 2D-M184}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/185.png}}{{\tiny 2D-M185}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/186.png}}{{\tiny 2D-M186}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/187.png}}{{\tiny 2D-M187}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/188.png}}{{\tiny 2D-M188}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/189.png}}{{\tiny 2D-M189}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/190.png}}{{\tiny 2D-M190}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/191.png}}{{\tiny 2D-M191}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/192.png}}{{\tiny 2D-M192}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/193.png}}{{\tiny 2D-M193}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/194.png}}{{\tiny 2D-M194}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/195.png}}{{\tiny 2D-M195}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/196.png}}{{\tiny 2D-M196}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/197.png}}{{\tiny 2D-M197}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/198.png}}{{\tiny 2D-M198}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/199.png}}{{\tiny 2D-M199}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/200.png}}{{\tiny 2D-M200}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/201.png}}{{\tiny 2D-M201}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/202.png}}{{\tiny 2D-M202}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/203.png}}{{\tiny 2D-M203}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/204.png}}{{\tiny 2D-M204}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/205.png}}{{\tiny 2D-M205}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/206.png}}{{\tiny 2D-M206}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/207.png}}{{\tiny 2D-M207}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/208.png}}{{\tiny 2D-M208}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/209.png}}{{\tiny 2D-M209}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/210.png}}{{\tiny 2D-M210}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/211.png}}{{\tiny 2D-M211}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/212.png}}{{\tiny 2D-M212}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/213.png}}{{\tiny 2D-M213}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/214.png}}{{\tiny 2D-M214}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/215.png}}{{\tiny 2D-M215}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/216.png}}{{\tiny 2D-M216}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/217.png}}{{\tiny 2D-M217}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/218.png}}{{\tiny 2D-M218}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/219.png}}{{\tiny 2D-M219}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/220.png}}{{\tiny 2D-M220}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/221.png}}{{\tiny 2D-M221}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/222.png}}{{\tiny 2D-M222}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/223.png}}{{\tiny 2D-M223}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/224.png}}{{\tiny 2D-M224}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/225.png}}{{\tiny 2D-M225}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/226.png}}{{\tiny 2D-M226}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/227.png}}{{\tiny 2D-M227}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/228.png}}{{\tiny 2D-M228}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/229.png}}{{\tiny 2D-M229}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/230.png}}{{\tiny 2D-M230}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/231.png}}{{\tiny 2D-M231}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/232.png}}{{\tiny 2D-M232}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/233.png}}{{\tiny 2D-M233}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/234.png}}{{\tiny 2D-M234}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/235.png}}{{\tiny 2D-M235}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/236.png}}{{\tiny 2D-M236}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/237.png}}{{\tiny 2D-M237}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/238.png}}{{\tiny 2D-M238}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/239.png}}{{\tiny 2D-M239}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/240.png}}{{\tiny 2D-M240}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/241.png}}{{\tiny 2D-M241}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/242.png}}{{\tiny 2D-M242}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/243.png}}{{\tiny 2D-M243}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/244.png}}{{\tiny 2D-M244}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/245.png}}{{\tiny 2D-M245}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/246.png}}{{\tiny 2D-M246}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/247.png}}{{\tiny 2D-M247}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/248.png}}{{\tiny 2D-M248}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/249.png}}{{\tiny 2D-M249}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/250.png}}{{\tiny 2D-M250}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/251.png}}{{\tiny 2D-M251}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/252.png}}{{\tiny 2D-M252}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/253.png}}{{\tiny 2D-M253}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/254.png}}{{\tiny 2D-M254}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/255.png}}{{\tiny 2D-M255}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/256.png}}{{\tiny 2D-M256}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/257.png}}{{\tiny 2D-M257}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/258.png}}{{\tiny 2D-M258}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/259.png}}{{\tiny 2D-M259}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/260.png}}{{\tiny 2D-M260}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/261.png}}{{\tiny 2D-M261}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/262.png}}{{\tiny 2D-M262}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/263.png}}{{\tiny 2D-M263}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/264.png}}{{\tiny 2D-M264}}


  \end{minipage}
\end{subfigure}
\caption{Schematic diagrams of 2-DOF Manipulators}
\end{figure}





  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/265.png}}{{\tiny 2D-M265}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/266.png}}{{\tiny 2D-M266}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/267.png}}{{\tiny 2D-M267}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/268.png}}{{\tiny 2D-M268}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/269.png}}{{\tiny 2D-M269}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/270.png}}{{\tiny 2D-M270}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/271.png}}{{\tiny 2D-M271}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/272.png}}{{\tiny 2D-M272}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/273.png}}{{\tiny 2D-M273}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/274.png}}{{\tiny 2D-M274}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/275.png}}{{\tiny 2D-M275}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/276.png}}{{\tiny 2D-M276}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/277.png}}{{\tiny 2D-M277}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/278.png}}{{\tiny 2D-M278}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/279.png}}{{\tiny 2D-M279}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/280.png}}{{\tiny 2D-M280}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/281.png}}{{\tiny 2D-M281}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/282.png}}{{\tiny 2D-M282}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/283.png}}{{\tiny 2D-M283}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/284.png}}{{\tiny 2D-M284}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/285.png}}{{\tiny 2D-M285}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/286.png}}{{\tiny 2D-M286}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/287.png}}{{\tiny 2D-M287}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/288.png}}{{\tiny 2D-M288}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/289.png}}{{\tiny 2D-M289}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/290.png}}{{\tiny 2D-M290}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/291.png}}{{\tiny 2D-M291}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/292.png}}{{\tiny 2D-M292}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/293.png}}{{\tiny 2D-M293}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/294.png}}{{\tiny 2D-M294}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/295.png}}{{\tiny 2D-M295}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/296.png}}{{\tiny 2D-M296}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/297.png}}{{\tiny 2D-M297}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/298.png}}{{\tiny 2D-M298}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/299.png}}{{\tiny 2D-M299}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/300.png}}{{\tiny 2D-M300}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/301.png}}{{\tiny 2D-M301}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/302.png}}{{\tiny 2D-M302}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/303.png}}{{\tiny 2D-M303}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/304.png}}{{\tiny 2D-M304}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/305.png}}{{\tiny 2D-M305}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/306.png}}{{\tiny 2D-M306}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/307.png}}{{\tiny 2D-M307}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/308.png}}{{\tiny 2D-M308}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/309.png}}{{\tiny 2D-M309}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/310.png}}{{\tiny 2D-M310}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/311.png}}{{\tiny 2D-M311}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/312.png}}{{\tiny 2D-M312}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/313.png}}{{\tiny 2D-M313}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/314.png}}{{\tiny 2D-M314}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/315.png}}{{\tiny 2D-M315}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/316.png}}{{\tiny 2D-M316}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/317.png}}{{\tiny 2D-M317}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/318.png}}{{\tiny 2D-M318}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/319.png}}{{\tiny 2D-M319}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/320.png}}{{\tiny 2D-M320}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/321.png}}{{\tiny 2D-M321}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/322.png}}{{\tiny 2D-M322}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/323.png}}{{\tiny 2D-M323}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/324.png}}{{\tiny 2D-M324}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/325.png}}{{\tiny 2D-M325}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/326.png}}{{\tiny 2D-M326}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/327.png}}{{\tiny 2D-M327}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/328.png}}{{\tiny 2D-M328}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/329.png}}{{\tiny 2D-M329}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/330.png}}{{\tiny 2D-M330}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/331.png}}{{\tiny 2D-M331}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/332.png}}{{\tiny 2D-M332}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/333.png}}{{\tiny 2D-M333}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/334.png}}{{\tiny 2D-M334}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/335.png}}{{\tiny 2D-M335}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/336.png}}{{\tiny 2D-M336}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/337.png}}{{\tiny 2D-M337}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/338.png}}{{\tiny 2D-M338}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/339.png}}{{\tiny 2D-M339}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/340.png}}{{\tiny 2D-M340}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/341.png}}{{\tiny 2D-M341}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/342.png}}{{\tiny 2D-M342}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/343.png}}{{\tiny 2D-M343}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/344.png}}{{\tiny 2D-M344}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/345.png}}{{\tiny 2D-M345}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/346.png}}{{\tiny 2D-M346}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/347.png}}{{\tiny 2D-M347}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/348.png}}{{\tiny 2D-M348}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/349.png}}{{\tiny 2D-M349}}
\qquad  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/350.png}}{{\tiny 2D-M350}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/351.png}}{{\tiny 2D-M351}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/352.png}}{{\tiny 2D-M352}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/353.png}}{{\tiny 2D-M353}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/354.png}}{{\tiny 2D-M354}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/355.png}}{{\tiny 2D-M355}}  
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/356.png}}{{\tiny 2D-M356}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/357.png}}{{\tiny 2D-M357}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/358.png}}{{\tiny 2D-M358}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/359.png}}{{\tiny 2D-M359}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/360.png}}{{\tiny 2D-M360}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/361.png}}{{\tiny 2D-M361}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/362.png}}{{\tiny 2D-M362}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/363.png}}{{\tiny 2D-M363}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/364.png}}{{\tiny 2D-M364}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/365.png}}{{\tiny 2D-M365}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/366.png}}{{\tiny 2D-M366}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/367.png}}{{\tiny 2D-M367}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/368.png}}{{\tiny 2D-M368}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/369.png}}{{\tiny 2D-M369}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/370.png}}{{\tiny 2D-M370}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/371.png}}{{\tiny 2D-M371}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/372.png}}{{\tiny 2D-M372}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/373.png}}{{\tiny 2D-M373}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/374.png}}{{\tiny 2D-M374}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/375.png}}{{\tiny 2D-M375}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/376.png}}{{\tiny 2D-M376}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/377.png}}{{\tiny 2D-M377}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/378.png}}{{\tiny 2D-M378}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/379.png}}{{\tiny 2D-M379}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/380.png}}{{\tiny 2D-M380}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/381.png}}{{\tiny 2D-M381}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/382.png}}{{\tiny 2D-M382}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/383.png}}{{\tiny 2D-M383}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/384.png}}{{\tiny 2D-M384}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/385.png}}{{\tiny 2D-M385}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/386.png}}{{\tiny 2D-M386}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/387.png}}{{\tiny 2D-M387}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/388.png}}{{\tiny 2D-M388}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/389.png}}{{\tiny 2D-M389}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/390.png}}{{\tiny 2D-M390}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/391.png}}{{\tiny 2D-M391}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/392.png}}{{\tiny 2D-M392}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/393.png}}{{\tiny 2D-M393}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/394.png}}{{\tiny 2D-M394}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/395.png}}{{\tiny 2D-M395}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/396.png}}{{\tiny 2D-M396}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/397.png}}{{\tiny 2D-M397}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/398.png}}{{\tiny 2D-M398}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/399.png}}{{\tiny 2D-M399}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/400.png}}{{\tiny 2D-M400}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/401.png}}{{\tiny 2D-M401}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/402.png}}{{\tiny 2D-M402}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/403.png}}{{\tiny 2D-M403}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/404.png}}{{\tiny 2D-M404}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/405.png}}{{\tiny 2D-M405}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/406.png}}{{\tiny 2D-M406}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/407.png}}{{\tiny 2D-M407}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/408.png}}{{\tiny 2D-M408}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/409.png}}{{\tiny 2D-M409}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/410.png}}{{\tiny 2D-M410}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/411.png}}{{\tiny 2D-M411}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/412.png}}{{\tiny 2D-M412}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/413.png}}{{\tiny 2D-M413}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/414.png}}{{\tiny 2D-M414}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/415.png}}{{\tiny 2D-M415}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/416.png}}{{\tiny 2D-M416}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/417.png}}{{\tiny 2D-M417}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/418.png}}{{\tiny 2D-M418}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/419.png}}{{\tiny 2D-M419}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/420.png}}{{\tiny 2D-M420}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/421.png}}{{\tiny 2D-M421}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/422.png}}{{\tiny 2D-M422}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/423.png}}{{\tiny 2D-M423}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/424.png}}{{\tiny 2D-M424}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/425.png}}{{\tiny 2D-M425}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/426.png}}{{\tiny 2D-M426}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/427.png}}{{\tiny 2D-M427}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/428.png}}{{\tiny 2D-M428}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/429.png}}{{\tiny 2D-M429}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/430.png}}{{\tiny 2D-M430}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/431.png}}{{\tiny 2D-M431}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/432.png}}{{\tiny 2D-M432}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/433.png}}{{\tiny 2D-M433}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/434.png}}{{\tiny 2D-M434}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/435.png}}{{\tiny 2D-M435}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/436.png}}{{\tiny 2D-M436}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/437.png}}{{\tiny 2D-M437}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/438.png}}{{\tiny 2D-M438}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/439.png}}{{\tiny 2D-M439}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/440.png}}{{\tiny 2D-M440}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/441.png}}{{\tiny 2D-M441}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/442.png}}{{\tiny 2D-M442}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/443.png}}{{\tiny 2D-M443}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/444.png}}{{\tiny 2D-M444}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/445.png}}{{\tiny 2D-M445}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/446.png}}{{\tiny 2D-M446}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/447.png}}{{\tiny 2D-M447}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/448.png}}{{\tiny 2D-M448}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/449.png}}{{\tiny 2D-M449}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/450.png}}{{\tiny 2D-M450}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/451.png}}{{\tiny 2D-M451}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/452.png}}{{\tiny 2D-M452}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/453.png}}{{\tiny 2D-M453}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/454.png}}{{\tiny 2D-M454}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/455.png}}{{\tiny 2D-M455}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/456.png}}{{\tiny 2D-M456}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/457.png}}{{\tiny 2D-M457}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/458.png}}{{\tiny 2D-M458}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/459.png}}{{\tiny 2D-M459}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/460.png}}{{\tiny 2D-M460}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/461.png}}{{\tiny 2D-M461}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/462.png}}{{\tiny 2D-M462}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/463.png}}{{\tiny 2D-M463}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/464.png}}{{\tiny 2D-M464}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/465.png}}{{\tiny 2D-M465}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/466.png}}{{\tiny 2D-M466}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/467.png}}{{\tiny 2D-M467}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/468.png}}{{\tiny 2D-M468}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/469.png}}{{\tiny 2D-M469}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/470.png}}{{\tiny 2D-M470}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/471.png}}{{\tiny 2D-M471}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/472.png}}{{\tiny 2D-M472}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/473.png}}{{\tiny 2D-M473}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/474.png}}{{\tiny 2D-M474}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/475.png}}{{\tiny 2D-M475}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/476.png}}{{\tiny 2D-M476}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/477.png}}{{\tiny 2D-M477}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/478.png}}{{\tiny 2D-M478}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/479.png}}{{\tiny 2D-M479}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/480.png}}{{\tiny 2D-M480}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/481.png}}{{\tiny 2D-M481}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/482.png}}{{\tiny 2D-M482}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/483.png}}{{\tiny 2D-M483}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/484.png}}{{\tiny 2D-M484}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/485.png}}{{\tiny 2D-M485}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/486.png}}{{\tiny 2D-M486}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/487.png}}{{\tiny 2D-M487}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/488.png}}{{\tiny 2D-M488}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/489.png}}{{\tiny 2D-M489}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/490.png}}{{\tiny 2D-M490}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/491.png}}{{\tiny 2D-M491}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/492.png}}{{\tiny 2D-M492}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/493.png}}{{\tiny 2D-M493}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/494.png}}{{\tiny 2D-M494}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/495.png}}{{\tiny 2D-M495}}  
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/496.png}}{{\tiny 2D-M496}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/497.png}}{{\tiny 2D-M497}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/498.png}}{{\tiny 2D-M498}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/499.png}}{{\tiny 2D-M499}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/500.png}}{{\tiny 2D-M500}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/501.png}}{{\tiny 2D-M501}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/502.png}}{{\tiny 2D-M502}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/503.png}}{{\tiny 2D-M503}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/504.png}}{{\tiny 2D-M504}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/505.png}}{{\tiny 2D-M505}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/506.png}}{{\tiny 2D-M506}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/507.png}}{{\tiny 2D-M507}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/508.png}}{{\tiny 2D-M508}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/509.png}}{{\tiny 2D-M509}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/510.png}}{{\tiny 2D-M510}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/511.png}}{{\tiny 2D-M511}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/512.png}}{{\tiny 2D-M512}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/513.png}}{{\tiny 2D-M513}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/514.png}}{{\tiny 2D-M514}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/515.png}}{{\tiny 2D-M515}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/516.png}}{{\tiny 2D-M516}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/517.png}}{{\tiny 2D-M517}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/518.png}}{{\tiny 2D-M518}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/519.png}}{{\tiny 2D-M519}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/520.png}}{{\tiny 2D-M520}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/521.png}}{{\tiny 2D-M521}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/522.png}}{{\tiny 2D-M522}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/523.png}}{{\tiny 2D-M523}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/524.png}}{{\tiny 2D-M524}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/525.png}}{{\tiny 2D-M525}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/526.png}}{{\tiny 2D-M526}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/527.png}}{{\tiny 2D-M527}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/528.png}}{{\tiny 2D-M528}}

      \end{minipage}
    \end{subfigure}
    \caption{Schematic diagrams of 2-DOF Manipulators (Contd.)}
    \end{figure}










\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering


\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/529.png}}{{\tiny 2D-M529}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/530.png}}{{\tiny 2D-M530}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/531.png}}{{\tiny 2D-M531}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/532.png}}{{\tiny 2D-M532}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/533.png}}{{\tiny 2D-M533}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/534.png}}{{\tiny 2D-M534}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/535.png}}{{\tiny 2D-M535}}
\qquad  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/536.png}}{{\tiny 2D-M536}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/537.png}}{{\tiny 2D-M537}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/538.png}}{{\tiny 2D-M538}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/539.png}}{{\tiny 2D-M539}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/540.png}}{{\tiny 2D-M540}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/541.png}}{{\tiny 2D-M541}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/542.png}}{{\tiny 2D-M542}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/543.png}}{{\tiny 2D-M543}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/544.png}}{{\tiny 2D-M544}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/545.png}}{{\tiny 2D-M545}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/546.png}}{{\tiny 2D-M546}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/547.png}}{{\tiny 2D-M547}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/548.png}}{{\tiny 2D-M548}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/549.png}}{{\tiny 2D-M549}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/550.png}}{{\tiny 2D-M550}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/551.png}}{{\tiny 2D-M551}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/552.png}}{{\tiny 2D-M552}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/553.png}}{{\tiny 2D-M553}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/554.png}}{{\tiny 2D-M554}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/555.png}}{{\tiny 2D-M555}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/556.png}}{{\tiny 2D-M556}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/557.png}}{{\tiny 2D-M557}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/558.png}}{{\tiny 2D-M558}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/559.png}}{{\tiny 2D-M559}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/560.png}}{{\tiny 2D-M560}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/561.png}}{{\tiny 2D-M561}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/562.png}}{{\tiny 2D-M562}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/563.png}}{{\tiny 2D-M563}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/564.png}}{{\tiny 2D-M564}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/565.png}}{{\tiny 2D-M565}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/566.png}}{{\tiny 2D-M566}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/567.png}}{{\tiny 2D-M567}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/568.png}}{{\tiny 2D-M568}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/569.png}}{{\tiny 2D-M569}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/570.png}}{{\tiny 2D-M570}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/571.png}}{{\tiny 2D-M571}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/572.png}}{{\tiny 2D-M572}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/573.png}}{{\tiny 2D-M573}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/574.png}}{{\tiny 2D-M574}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/575.png}}{{\tiny 2D-M575}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/576.png}}{{\tiny 2D-M576}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/577.png}}{{\tiny 2D-M577}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/578.png}}{{\tiny 2D-M578}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/579.png}}{{\tiny 2D-M579}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/580.png}}{{\tiny 2D-M580}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/581.png}}{{\tiny 2D-M581}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/582.png}}{{\tiny 2D-M582}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/583.png}}{{\tiny 2D-M583}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/584.png}}{{\tiny 2D-M584}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/585.png}}{{\tiny 2D-M585}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/586.png}}{{\tiny 2D-M586}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/587.png}}{{\tiny 2D-M587}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/588.png}}{{\tiny 2D-M588}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/589.png}}{{\tiny 2D-M589}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/590.png}}{{\tiny 2D-M590}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/591.png}}{{\tiny 2D-M591}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/592.png}}{{\tiny 2D-M592}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/593.png}}{{\tiny 2D-M593}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/594.png}}{{\tiny 2D-M594}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/595.png}}{{\tiny 2D-M595}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/596.png}}{{\tiny 2D-M596}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/597.png}}{{\tiny 2D-M597}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/598.png}}{{\tiny 2D-M598}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/599.png}}{{\tiny 2D-M599}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/600.png}}{{\tiny 2D-M600}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/601.png}}{{\tiny 2D-M601}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/602.png}}{{\tiny 2D-M602}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/603.png}}{{\tiny 2D-M603}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/604.png}}{{\tiny 2D-M604}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/605.png}}{{\tiny 2D-M605}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/606.png}}{{\tiny 2D-M606}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/607.png}}{{\tiny 2D-M607}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/608.png}}{{\tiny 2D-M608}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/609.png}}{{\tiny 2D-M609}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/610.png}}{{\tiny 2D-M610}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/611.png}}{{\tiny 2D-M611}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/612.png}}{{\tiny 2D-M612}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/613.png}}{{\tiny 2D-M613}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/614.png}}{{\tiny 2D-M614}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/615.png}}{{\tiny 2D-M615}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/616.png}}{{\tiny 2D-M616}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/617.png}}{{\tiny 2D-M617}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/618.png}}{{\tiny 2D-M618}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/619.png}}{{\tiny 2D-M619}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/620.png}}{{\tiny 2D-M620}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/621.png}}{{\tiny 2D-M621}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/622.png}}{{\tiny 2D-M622}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/623.png}}{{\tiny 2D-M623}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/624.png}}{{\tiny 2D-M624}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/625.png}}{{\tiny 2D-M625}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/626.png}}{{\tiny 2D-M626}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/627.png}}{{\tiny 2D-M627}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/628.png}}{{\tiny 2D-M628}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/629.png}}{{\tiny 2D-M629}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/630.png}}{{\tiny 2D-M630}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/631.png}}{{\tiny 2D-M631}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/632.png}}{{\tiny 2D-M632}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/633.png}}{{\tiny 2D-M633}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/634.png}}{{\tiny 2D-M634}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/635.png}}{{\tiny 2D-M635}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/636.png}}{{\tiny 2D-M636}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/637.png}}{{\tiny 2D-M637}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/638.png}}{{\tiny 2D-M638}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/639.png}}{{\tiny 2D-M639}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/640.png}}{{\tiny 2D-M640}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/641.png}}{{\tiny 2D-M641}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/642.png}}{{\tiny 2D-M642}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/643.png}}{{\tiny 2D-M643}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/644.png}}{{\tiny 2D-M644}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/645.png}}{{\tiny 2D-M645}}

  
    \end{minipage}
  \end{subfigure}
  \caption{Schematic diagrams of 2-DOF Manipulators (Contd.)}
  \end{figure}


==> Dimensional Synthesis/classes/2dof_classes_old.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/1.png}}{{\tiny 2D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/2.png}}{{\tiny 2D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/3.png}}{{\tiny 2D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/4.png}}{{\tiny 2D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/5.png}}{{\tiny 2D-M5}}

  \end{minipage}
\end{subfigure}
\caption{Class 1 of 2-DOF Manipulators}
\end{figure}


\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/6.png}}{{\tiny 2D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/7.png}}{{\tiny 2D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/8.png}}{{\tiny 2D-M8}}


  \end{minipage}
\end{subfigure}
\caption{Class 2 of 2-DOF Manipulators}
\end{figure}



\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/9.png}}{{\tiny 2D-M9}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/10.png}}{{\tiny 2D-M10}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/11.png}}{{\tiny 2D-M11}}    
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/12.png}}{{\tiny 2D-M12}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/13.png}}{{\tiny 2D-M13}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/14.png}}{{\tiny 2D-M14}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/15.png}}{{\tiny 2D-M15}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/16.png}}{{\tiny 2D-M16}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/17.png}}{{\tiny 2D-M17}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/18.png}}{{\tiny 2D-M18}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/19.png}}{{\tiny 2D-M19}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/20.png}}{{\tiny 2D-M20}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 2 of 2-DOF Manipulators (Contd.)}
  \end{figure}


  \begin{figure}[H]
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/21.png}}{{\tiny 2D-M21}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/22.png}}{{\tiny 2D-M22}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/23.png}}{{\tiny 2D-M23}}
    
      \end{minipage}
    \end{subfigure}
    \caption{Class 3 of 2-DOF Manipulators}
    \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/24.png}}{{\tiny 2D-M24}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/25.png}}{{\tiny 2D-M25}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/26.png}}{{\tiny 2D-M26}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/27.png}}{{\tiny 2D-M27}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/28.png}}{{\tiny 2D-M28}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/29.png}}{{\tiny 2D-M29}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/30.png}}{{\tiny 2D-M30}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/31.png}}{{\tiny 2D-M31}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/32.png}}{{\tiny 2D-M32}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/33.png}}{{\tiny 2D-M33}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/34.png}}{{\tiny 2D-M34}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/35.png}}{{\tiny 2D-M35}}

  \end{minipage}
\end{subfigure}
\caption{Class 3 of 2-DOF Manipulators (Contd.)}
\end{figure}



\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/36.png}}{{\tiny 2D-M36}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/37.png}}{{\tiny 2D-M37}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/38.png}}{{\tiny 2D-M38}}
  \end{minipage}
\end{subfigure}
\caption{Class 4 of 2-DOF Manipulators}
\end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/39.png}}{{\tiny 2D-M39}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/40.png}}{{\tiny 2D-M40}}
    \end{minipage}
  \end{subfigure}
  \caption{Class 4 of 2-DOF Manipulators (Contd.)}
  \end{figure}

% \begin{figure}[H]\ContinuedFloat
%   \centering
%   \begin{subfigure}{\columnwidth}
%     \begin{minipage}{\textwidth}\footnotesize
%     \centering
  
  
%     \end{minipage}
%   \end{subfigure}
%   \caption{Class 4 of 2-DOF Manipulators (Contd.)}
%   \end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/41.png}}{{\tiny 2D-M41}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/42.png}}{{\tiny 2D-M42}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/43.png}}{{\tiny 2D-M43}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/44.png}}{{\tiny 2D-M44}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/45.png}}{{\tiny 2D-M45}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/46.png}}{{\tiny 2D-M46}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/47.png}}{{\tiny 2D-M47}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/48.png}}{{\tiny 2D-M48}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/49.png}}{{\tiny 2D-M49}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/50.png}}{{\tiny 2D-M50}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/51.png}}{{\tiny 2D-M51}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/52.png}}{{\tiny 2D-M52}}



  \end{minipage}
\end{subfigure}
\caption{Class 5 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/53.png}}{{\tiny 2D-M53}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/54.png}}{{\tiny 2D-M54}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/55.png}}{{\tiny 2D-M55}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/56.png}}{{\tiny 2D-M56}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/57.png}}{{\tiny 2D-M57}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/58.png}}{{\tiny 2D-M58}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/59.png}}{{\tiny 2D-M59}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/60.png}}{{\tiny 2D-M60}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/61.png}}{{\tiny 2D-M61}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/62.png}}{{\tiny 2D-M62}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/63.png}}{{\tiny 2D-M63}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/64.png}}{{\tiny 2D-M64}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/65.png}}{{\tiny 2D-M65}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/66.png}}{{\tiny 2D-M66}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/67.png}}{{\tiny 2D-M67}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/68.png}}{{\tiny 2D-M68}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/69.png}}{{\tiny 2D-M69}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/70.png}}{{\tiny 2D-M70}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/71.png}}{{\tiny 2D-M71}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/72.png}}{{\tiny 2D-M72}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/73.png}}{{\tiny 2D-M73}}

  
    \end{minipage}
  \end{subfigure}
  \caption{Class 5 of 2-DOF Manipulators (Contd.)}
  \end{figure}


  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
    
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/74.png}}{{\tiny 2D-M74}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/75.png}}{{\tiny 2D-M75}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/76.png}}{{\tiny 2D-M76}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/77.png}}{{\tiny 2D-M77}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/78.png}}{{\tiny 2D-M78}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/79.png}}{{\tiny 2D-M79}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/80.png}}{{\tiny 2D-M80}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/81.png}}{{\tiny 2D-M81}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/82.png}}{{\tiny 2D-M82}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/83.png}}{{\tiny 2D-M83}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/84.png}}{{\tiny 2D-M84}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/85.png}}{{\tiny 2D-M85}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/86.png}}{{\tiny 2D-M86}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/87.png}}{{\tiny 2D-M87}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/88.png}}{{\tiny 2D-M88}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/89.png}}{{\tiny 2D-M89}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/90.png}}{{\tiny 2D-M90}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/91.png}}{{\tiny 2D-M91}}
   
      \end{minipage}
    \end{subfigure}
    \caption{Class 5 of 2-DOF Manipulators (Contd.)}
    \end{figure}



  \begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/92.png}}{{\tiny 2D-M92}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/93.png}}{{\tiny 2D-M93}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/94.png}}{{\tiny 2D-M94}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/95.png}}{{\tiny 2D-M95}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/96.png}}{{\tiny 2D-M96}} 
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/97.png}}{{\tiny 2D-M97}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/98.png}}{{\tiny 2D-M98}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/99.png}}{{\tiny 2D-M99}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/100.png}}{{\tiny 2D-M100}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/101.png}}{{\tiny 2D-M101}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/102.png}}{{\tiny 2D-M102}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/103.png}}{{\tiny 2D-M103}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/104.png}}{{\tiny 2D-M104}}

  \end{minipage}
\end{subfigure}
\caption{Class 5 of 2-DOF Manipulators (Contd.)}
\end{figure}


\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/105.png}}{{\tiny 2D-M105}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/106.png}}{{\tiny 2D-M106}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/107.png}}{{\tiny 2D-M107}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/108.png}}{{\tiny 2D-M108}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/109.png}}{{\tiny 2D-M109}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/110.png}}{{\tiny 2D-M110}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/111.png}}{{\tiny 2D-M111}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/112.png}}{{\tiny 2D-M112}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/113.png}}{{\tiny 2D-M113}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/114.png}}{{\tiny 2D-M114}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/115.png}}{{\tiny 2D-M115}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/116.png}}{{\tiny 2D-M116}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/117.png}}{{\tiny 2D-M117}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/118.png}}{{\tiny 2D-M118}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/119.png}}{{\tiny 2D-M119}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/120.png}}{{\tiny 2D-M120}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/121.png}}{{\tiny 2D-M121}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/122.png}}{{\tiny 2D-M122}}





  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/123.png}}{{\tiny 2D-M123}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/124.png}}{{\tiny 2D-M124}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/125.png}}{{\tiny 2D-M125}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/126.png}}{{\tiny 2D-M126}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/127.png}}{{\tiny 2D-M127}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/128.png}}{{\tiny 2D-M128}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/129.png}}{{\tiny 2D-M129}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/130.png}}{{\tiny 2D-M130}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/131.png}}{{\tiny 2D-M131}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/132.png}}{{\tiny 2D-M132}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/133.png}}{{\tiny 2D-M133}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/134.png}}{{\tiny 2D-M134}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/135.png}}{{\tiny 2D-M135}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/136.png}}{{\tiny 2D-M136}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/137.png}}{{\tiny 2D-M137}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/138.png}}{{\tiny 2D-M138}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/139.png}}{{\tiny 2D-M139}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/140.png}}{{\tiny 2D-M140}}
 
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 2-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/141.png}}{{\tiny 2D-M141}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/142.png}}{{\tiny 2D-M142}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/143.png}}{{\tiny 2D-M143}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/144.png}}{{\tiny 2D-M144}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/145.png}}{{\tiny 2D-M145}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/146.png}}{{\tiny 2D-M146}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/147.png}}{{\tiny 2D-M147}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/148.png}}{{\tiny 2D-M148}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/149.png}}{{\tiny 2D-M149}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/150.png}}{{\tiny 2D-M150}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/151.png}}{{\tiny 2D-M151}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/152.png}}{{\tiny 2D-M152}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/153.png}}{{\tiny 2D-M153}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/154.png}}{{\tiny 2D-M154}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/155.png}}{{\tiny 2D-M155}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/156.png}}{{\tiny 2D-M156}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/157.png}}{{\tiny 2D-M157}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/158.png}}{{\tiny 2D-M158}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/159.png}}{{\tiny 2D-M159}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/160.png}}{{\tiny 2D-M160}} 
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/161.png}}{{\tiny 2D-M161}}



  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Contd.)}
\end{figure}\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/162.png}}{{\tiny 2D-M162}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/163.png}}{{\tiny 2D-M163}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/164.png}}{{\tiny 2D-M164}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/165.png}}{{\tiny 2D-M165}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/166.png}}{{\tiny 2D-M166}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/167.png}}{{\tiny 2D-M167}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/168.png}}{{\tiny 2D-M168}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/169.png}}{{\tiny 2D-M169}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/170.png}}{{\tiny 2D-M170}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/171.png}}{{\tiny 2D-M171}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/172.png}}{{\tiny 2D-M172}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/173.png}}{{\tiny 2D-M173}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/174.png}}{{\tiny 2D-M174}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/175.png}}{{\tiny 2D-M175}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/176.png}}{{\tiny 2D-M176}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/177.png}}{{\tiny 2D-M177}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/178.png}}{{\tiny 2D-M178}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/179.png}}{{\tiny 2D-M179}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/180.png}}{{\tiny 2D-M180}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/181.png}}{{\tiny 2D-M181}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/182.png}}{{\tiny 2D-M182}}



  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Contd.)}
\end{figure}


\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/183.png}}{{\tiny 2D-M183}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/184.png}}{{\tiny 2D-M184}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/185.png}}{{\tiny 2D-M185}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/186.png}}{{\tiny 2D-M186}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/187.png}}{{\tiny 2D-M187}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/188.png}}{{\tiny 2D-M188}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/189.png}}{{\tiny 2D-M189}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/190.png}}{{\tiny 2D-M190}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/191.png}}{{\tiny 2D-M191}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/192.png}}{{\tiny 2D-M192}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/193.png}}{{\tiny 2D-M193}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/194.png}}{{\tiny 2D-M194}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/195.png}}{{\tiny 2D-M195}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/196.png}}{{\tiny 2D-M196}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/197.png}}{{\tiny 2D-M197}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/198.png}}{{\tiny 2D-M198}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/199.png}}{{\tiny 2D-M199}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/200.png}}{{\tiny 2D-M200}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/201.png}}{{\tiny 2D-M201}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/202.png}}{{\tiny 2D-M202}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/203.png}}{{\tiny 2D-M203}}



  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Contd.)}
\end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/204.png}}{{\tiny 2D-M204}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/205.png}}{{\tiny 2D-M205}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/206.png}}{{\tiny 2D-M206}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/207.png}}{{\tiny 2D-M207}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/208.png}}{{\tiny 2D-M208}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/209.png}}{{\tiny 2D-M209}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/210.png}}{{\tiny 2D-M210}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/211.png}}{{\tiny 2D-M211}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/212.png}}{{\tiny 2D-M212}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/213.png}}{{\tiny 2D-M213}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/214.png}}{{\tiny 2D-M214}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/215.png}}{{\tiny 2D-M215}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/216.png}}{{\tiny 2D-M216}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/217.png}}{{\tiny 2D-M217}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/218.png}}{{\tiny 2D-M218}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/219.png}}{{\tiny 2D-M219}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/220.png}}{{\tiny 2D-M220}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/221.png}}{{\tiny 2D-M221}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/222.png}}{{\tiny 2D-M222}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/223.png}}{{\tiny 2D-M223}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/224.png}}{{\tiny 2D-M224}}


  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 2-DOF Manipulators (Contd.)}
  \end{figure}


  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
    
  
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/225.png}}{{\tiny 2D-M225}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/226.png}}{{\tiny 2D-M226}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/227.png}}{{\tiny 2D-M227}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/228.png}}{{\tiny 2D-M228}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/229.png}}{{\tiny 2D-M229}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/230.png}}{{\tiny 2D-M230}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/231.png}}{{\tiny 2D-M231}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/232.png}}{{\tiny 2D-M232}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/233.png}}{{\tiny 2D-M233}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/234.png}}{{\tiny 2D-M234}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/235.png}}{{\tiny 2D-M235}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/236.png}}{{\tiny 2D-M236}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/237.png}}{{\tiny 2D-M237}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/238.png}}{{\tiny 2D-M238}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/239.png}}{{\tiny 2D-M239}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/240.png}}{{\tiny 2D-M240}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/241.png}}{{\tiny 2D-M241}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/242.png}}{{\tiny 2D-M242}}

    
      \end{minipage}
    \end{subfigure}
    \caption{Class 6 of 2-DOF Manipulators (Contd.)}
    \end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/243.png}}{{\tiny 2D-M243}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/244.png}}{{\tiny 2D-M244}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/245.png}}{{\tiny 2D-M245}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/246.png}}{{\tiny 2D-M246}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/247.png}}{{\tiny 2D-M247}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/248.png}}{{\tiny 2D-M248}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/249.png}}{{\tiny 2D-M249}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/250.png}}{{\tiny 2D-M250}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/251.png}}{{\tiny 2D-M251}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/252.png}}{{\tiny 2D-M252}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/253.png}}{{\tiny 2D-M253}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/254.png}}{{\tiny 2D-M254}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/255.png}}{{\tiny 2D-M255}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/256.png}}{{\tiny 2D-M256}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/257.png}}{{\tiny 2D-M257}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/258.png}}{{\tiny 2D-M258}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/259.png}}{{\tiny 2D-M259}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/260.png}}{{\tiny 2D-M260}}



  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 2-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/261.png}}{{\tiny 2D-M261}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/262.png}}{{\tiny 2D-M262}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/263.png}}{{\tiny 2D-M263}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/264.png}}{{\tiny 2D-M264}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/265.png}}{{\tiny 2D-M265}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/266.png}}{{\tiny 2D-M266}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/267.png}}{{\tiny 2D-M267}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/268.png}}{{\tiny 2D-M268}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/269.png}}{{\tiny 2D-M269}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/270.png}}{{\tiny 2D-M270}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/271.png}}{{\tiny 2D-M271}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/272.png}}{{\tiny 2D-M272}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/273.png}}{{\tiny 2D-M273}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/274.png}}{{\tiny 2D-M274}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/275.png}}{{\tiny 2D-M275}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/276.png}}{{\tiny 2D-M276}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/277.png}}{{\tiny 2D-M277}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/278.png}}{{\tiny 2D-M278}}



  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 2-DOF Manipulators (Contd.)}
  \end{figure}


  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/279.png}}{{\tiny 2D-M279}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/280.png}}{{\tiny 2D-M280}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/281.png}}{{\tiny 2D-M281}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/282.png}}{{\tiny 2D-M282}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/283.png}}{{\tiny 2D-M283}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/284.png}}{{\tiny 2D-M284}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/285.png}}{{\tiny 2D-M285}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/286.png}}{{\tiny 2D-M286}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/287.png}}{{\tiny 2D-M287}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/288.png}}{{\tiny 2D-M288}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/289.png}}{{\tiny 2D-M289}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/290.png}}{{\tiny 2D-M290}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/291.png}}{{\tiny 2D-M291}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/292.png}}{{\tiny 2D-M292}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/293.png}}{{\tiny 2D-M293}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/294.png}}{{\tiny 2D-M294}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/295.png}}{{\tiny 2D-M295}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/296.png}}{{\tiny 2D-M296}}
    
      \end{minipage}
    \end{subfigure}
    \caption{Class 6 of 2-DOF Manipulators (Contd.)}
    \end{figure}



\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/297.png}}{{\tiny 2D-M297}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/298.png}}{{\tiny 2D-M298}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/299.png}}{{\tiny 2D-M299}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/300.png}}{{\tiny 2D-M300}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/301.png}}{{\tiny 2D-M301}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/302.png}}{{\tiny 2D-M302}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/303.png}}{{\tiny 2D-M303}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/304.png}}{{\tiny 2D-M304}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/305.png}}{{\tiny 2D-M305}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/306.png}}{{\tiny 2D-M306}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/307.png}}{{\tiny 2D-M307}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/308.png}}{{\tiny 2D-M308}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/309.png}}{{\tiny 2D-M309}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/310.png}}{{\tiny 2D-M310}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/311.png}}{{\tiny 2D-M311}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/312.png}}{{\tiny 2D-M312}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/313.png}}{{\tiny 2D-M313}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/314.png}}{{\tiny 2D-M314}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/315.png}}{{\tiny 2D-M315}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/316.png}}{{\tiny 2D-M316}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/317.png}}{{\tiny 2D-M317}}

  \end{minipage}
\end{subfigure}
\caption{Class 7 of 2-DOF Manipulators}
\end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/318.png}}{{\tiny 2D-M318}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/319.png}}{{\tiny 2D-M319}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 7 of 2-DOF Manipulators (Contd.)}
  \end{figure}


\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/320.png}}{{\tiny 2D-M320}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/321.png}}{{\tiny 2D-M321}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/322.png}}{{\tiny 2D-M322}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/323.png}}{{\tiny 2D-M323}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/324.png}}{{\tiny 2D-M324}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/325.png}}{{\tiny 2D-M325}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/326.png}}{{\tiny 2D-M326}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/327.png}}{{\tiny 2D-M327}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/328.png}}{{\tiny 2D-M328}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/329.png}}{{\tiny 2D-M329}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/330.png}}{{\tiny 2D-M330}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/331.png}}{{\tiny 2D-M331}}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators}
\end{figure}



\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering

  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/332.png}}{{\tiny 2D-M332}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/333.png}}{{\tiny 2D-M333}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/334.png}}{{\tiny 2D-M334}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/335.png}}{{\tiny 2D-M335}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/336.png}}{{\tiny 2D-M336}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/337.png}}{{\tiny 2D-M337}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/338.png}}{{\tiny 2D-M338}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/339.png}}{{\tiny 2D-M339}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/340.png}}{{\tiny 2D-M340}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/341.png}}{{\tiny 2D-M341}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/342.png}}{{\tiny 2D-M342}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/343.png}}{{\tiny 2D-M343}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/344.png}}{{\tiny 2D-M344}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/345.png}}{{\tiny 2D-M345}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/346.png}}{{\tiny 2D-M346}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/347.png}}{{\tiny 2D-M347}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/348.png}}{{\tiny 2D-M348}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/349.png}}{{\tiny 2D-M349}}

    \end{minipage}
  \end{subfigure}
  \caption{Class 8 of 2-DOF Manipulators (Contd.)}
  \end{figure}


\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/350.png}}{{\tiny 2D-M350}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/351.png}}{{\tiny 2D-M351}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/352.png}}{{\tiny 2D-M352}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/353.png}}{{\tiny 2D-M353}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/354.png}}{{\tiny 2D-M354}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/355.png}}{{\tiny 2D-M355}}  
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/356.png}}{{\tiny 2D-M356}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/357.png}}{{\tiny 2D-M357}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/358.png}}{{\tiny 2D-M358}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/359.png}}{{\tiny 2D-M359}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/360.png}}{{\tiny 2D-M360}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/361.png}}{{\tiny 2D-M361}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/362.png}}{{\tiny 2D-M362}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/363.png}}{{\tiny 2D-M363}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/364.png}}{{\tiny 2D-M364}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/365.png}}{{\tiny 2D-M365}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/366.png}}{{\tiny 2D-M366}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/367.png}}{{\tiny 2D-M367}}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Contd.)}
\end{figure}


\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/368.png}}{{\tiny 2D-M368}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/369.png}}{{\tiny 2D-M369}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/370.png}}{{\tiny 2D-M370}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/371.png}}{{\tiny 2D-M371}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/372.png}}{{\tiny 2D-M372}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/373.png}}{{\tiny 2D-M373}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/374.png}}{{\tiny 2D-M374}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/375.png}}{{\tiny 2D-M375}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/376.png}}{{\tiny 2D-M376}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/377.png}}{{\tiny 2D-M377}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/378.png}}{{\tiny 2D-M378}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/379.png}}{{\tiny 2D-M379}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/380.png}}{{\tiny 2D-M380}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/381.png}}{{\tiny 2D-M381}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/382.png}}{{\tiny 2D-M382}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/383.png}}{{\tiny 2D-M383}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/384.png}}{{\tiny 2D-M384}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/385.png}}{{\tiny 2D-M385}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/386.png}}{{\tiny 2D-M386}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/387.png}}{{\tiny 2D-M387}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/388.png}}{{\tiny 2D-M388}}



  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Contd.)}
\end{figure}



  

  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/389.png}}{{\tiny 2D-M389}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/390.png}}{{\tiny 2D-M390}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/391.png}}{{\tiny 2D-M391}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/392.png}}{{\tiny 2D-M392}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/393.png}}{{\tiny 2D-M393}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/394.png}}{{\tiny 2D-M394}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/395.png}}{{\tiny 2D-M395}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/396.png}}{{\tiny 2D-M396}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/397.png}}{{\tiny 2D-M397}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/398.png}}{{\tiny 2D-M398}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/399.png}}{{\tiny 2D-M399}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/400.png}}{{\tiny 2D-M400}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/401.png}}{{\tiny 2D-M401}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/402.png}}{{\tiny 2D-M402}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/403.png}}{{\tiny 2D-M403}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/404.png}}{{\tiny 2D-M404}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/405.png}}{{\tiny 2D-M405}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/406.png}}{{\tiny 2D-M406}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/407.png}}{{\tiny 2D-M407}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/408.png}}{{\tiny 2D-M408}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/409.png}}{{\tiny 2D-M409}}

    
      \end{minipage}
    \end{subfigure}
    \caption{Class 8 of 2-DOF Manipulators (Contd.)}
    \end{figure}

    \begin{figure}[H]\ContinuedFloat
      \centering
      \begin{subfigure}{\columnwidth}
        \begin{minipage}{\textwidth}\footnotesize
        \centering
        \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/410.png}}{{\tiny 2D-M410}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/411.png}}{{\tiny 2D-M411}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/412.png}}{{\tiny 2D-M412}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/413.png}}{{\tiny 2D-M413}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/414.png}}{{\tiny 2D-M414}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/415.png}}{{\tiny 2D-M415}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/416.png}}{{\tiny 2D-M416}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/417.png}}{{\tiny 2D-M417}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/418.png}}{{\tiny 2D-M418}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/419.png}}{{\tiny 2D-M419}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/420.png}}{{\tiny 2D-M420}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/421.png}}{{\tiny 2D-M421}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/422.png}}{{\tiny 2D-M422}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/423.png}}{{\tiny 2D-M423}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/424.png}}{{\tiny 2D-M424}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/425.png}}{{\tiny 2D-M425}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/426.png}}{{\tiny 2D-M426}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/427.png}}{{\tiny 2D-M427}}


    \end{minipage}
      \end{subfigure}
      \caption{Class 8 of 2-DOF Manipulators (Contd.)}
      \end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/428.png}}{{\tiny 2D-M428}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/429.png}}{{\tiny 2D-M429}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/430.png}}{{\tiny 2D-M430}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/431.png}}{{\tiny 2D-M431}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/432.png}}{{\tiny 2D-M432}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/433.png}}{{\tiny 2D-M433}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/434.png}}{{\tiny 2D-M434}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/435.png}}{{\tiny 2D-M435}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/436.png}}{{\tiny 2D-M436}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/437.png}}{{\tiny 2D-M437}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/438.png}}{{\tiny 2D-M438}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/439.png}}{{\tiny 2D-M439}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/440.png}}{{\tiny 2D-M440}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/441.png}}{{\tiny 2D-M441}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/442.png}}{{\tiny 2D-M442}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/443.png}}{{\tiny 2D-M443}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/444.png}}{{\tiny 2D-M444}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/445.png}}{{\tiny 2D-M445}}


 
    \end{minipage}
  \end{subfigure}
  \caption{Class 8 of 2-DOF Manipulators (Contd.)}
  \end{figure}

  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/446.png}}{{\tiny 2D-M446}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/447.png}}{{\tiny 2D-M447}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/448.png}}{{\tiny 2D-M448}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/449.png}}{{\tiny 2D-M449}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/450.png}}{{\tiny 2D-M450}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/451.png}}{{\tiny 2D-M451}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/452.png}}{{\tiny 2D-M452}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/453.png}}{{\tiny 2D-M453}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/454.png}}{{\tiny 2D-M454}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/455.png}}{{\tiny 2D-M455}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/456.png}}{{\tiny 2D-M456}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/457.png}}{{\tiny 2D-M457}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/458.png}}{{\tiny 2D-M458}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/459.png}}{{\tiny 2D-M459}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/460.png}}{{\tiny 2D-M460}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/461.png}}{{\tiny 2D-M461}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/462.png}}{{\tiny 2D-M462}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/463.png}}{{\tiny 2D-M463}}




   
      \end{minipage}
    \end{subfigure}
    \caption{Class 8 of 2-DOF Manipulators (Contd.)}
    \end{figure}
  
    \begin{figure}[H]\ContinuedFloat
      \centering
      \begin{subfigure}{\columnwidth}
        \begin{minipage}{\textwidth}\footnotesize
        \centering
        \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/464.png}}{{\tiny 2D-M464}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/465.png}}{{\tiny 2D-M465}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/466.png}}{{\tiny 2D-M466}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/467.png}}{{\tiny 2D-M467}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/468.png}}{{\tiny 2D-M468}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/469.png}}{{\tiny 2D-M469}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/470.png}}{{\tiny 2D-M470}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/471.png}}{{\tiny 2D-M471}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/472.png}}{{\tiny 2D-M472}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/473.png}}{{\tiny 2D-M473}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/474.png}}{{\tiny 2D-M474}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/475.png}}{{\tiny 2D-M475}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/476.png}}{{\tiny 2D-M476}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/477.png}}{{\tiny 2D-M477}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/478.png}}{{\tiny 2D-M478}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/479.png}}{{\tiny 2D-M479}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/480.png}}{{\tiny 2D-M480}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/481.png}}{{\tiny 2D-M481}}



      
     
        \end{minipage}
      \end{subfigure}
      \caption{Class 8 of 2-DOF Manipulators (Contd.)}
      \end{figure}

      \begin{figure}[H]\ContinuedFloat
        \centering
        \begin{subfigure}{\columnwidth}
          \begin{minipage}{\textwidth}\footnotesize
          \centering
          \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/482.png}}{{\tiny 2D-M482}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/483.png}}{{\tiny 2D-M483}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/484.png}}{{\tiny 2D-M484}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/485.png}}{{\tiny 2D-M485}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/486.png}}{{\tiny 2D-M486}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/487.png}}{{\tiny 2D-M487}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/488.png}}{{\tiny 2D-M488}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/489.png}}{{\tiny 2D-M489}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/490.png}}{{\tiny 2D-M490}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/491.png}}{{\tiny 2D-M491}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/492.png}}{{\tiny 2D-M492}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/493.png}}{{\tiny 2D-M493}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/494.png}}{{\tiny 2D-M494}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/495.png}}{{\tiny 2D-M495}}  
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/496.png}}{{\tiny 2D-M496}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/497.png}}{{\tiny 2D-M497}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/498.png}}{{\tiny 2D-M498}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/499.png}}{{\tiny 2D-M499}}


          \end{minipage}
        \end{subfigure}
        \caption{Class 8 of 2-DOF Manipulators (Contd.)}
        \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering


  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/500.png}}{{\tiny 2D-M500}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/501.png}}{{\tiny 2D-M501}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/502.png}}{{\tiny 2D-M502}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/503.png}}{{\tiny 2D-M503}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/504.png}}{{\tiny 2D-M504}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/505.png}}{{\tiny 2D-M505}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/506.png}}{{\tiny 2D-M506}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/507.png}}{{\tiny 2D-M507}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/508.png}}{{\tiny 2D-M508}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/509.png}}{{\tiny 2D-M509}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/510.png}}{{\tiny 2D-M510}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/511.png}}{{\tiny 2D-M511}}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Contd.)}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/512.png}}{{\tiny 2D-M512}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/513.png}}{{\tiny 2D-M513}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/514.png}}{{\tiny 2D-M514}}

  
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 9 of 2-DOF Manipulators}
  \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/515.png}}{{\tiny 2D-M515}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/516.png}}{{\tiny 2D-M516}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/517.png}}{{\tiny 2D-M517}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/518.png}}{{\tiny 2D-M518}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/519.png}}{{\tiny 2D-M519}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/520.png}}{{\tiny 2D-M520}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/521.png}}{{\tiny 2D-M521}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/522.png}}{{\tiny 2D-M522}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/523.png}}{{\tiny 2D-M523}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/524.png}}{{\tiny 2D-M524}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/525.png}}{{\tiny 2D-M525}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/526.png}}{{\tiny 2D-M526}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/527.png}}{{\tiny 2D-M527}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/528.png}}{{\tiny 2D-M528}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/529.png}}{{\tiny 2D-M529}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/530.png}}{{\tiny 2D-M530}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/531.png}}{{\tiny 2D-M531}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/532.png}}{{\tiny 2D-M532}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/533.png}}{{\tiny 2D-M533}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/534.png}}{{\tiny 2D-M534}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/535.png}}{{\tiny 2D-M535}}

  \end{minipage}
\end{subfigure}
\caption{Class 9 of 2-DOF Manipulators (Contd.)}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering


  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/536.png}}{{\tiny 2D-M536}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/537.png}}{{\tiny 2D-M537}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/538.png}}{{\tiny 2D-M538}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/539.png}}{{\tiny 2D-M539}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/540.png}}{{\tiny 2D-M540}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/541.png}}{{\tiny 2D-M541}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/542.png}}{{\tiny 2D-M542}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/543.png}}{{\tiny 2D-M543}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/544.png}}{{\tiny 2D-M544}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/545.png}}{{\tiny 2D-M545}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/546.png}}{{\tiny 2D-M546}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/547.png}}{{\tiny 2D-M547}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/548.png}}{{\tiny 2D-M548}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/549.png}}{{\tiny 2D-M549}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/550.png}}{{\tiny 2D-M550}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/551.png}}{{\tiny 2D-M551}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/552.png}}{{\tiny 2D-M552}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/553.png}}{{\tiny 2D-M553}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/554.png}}{{\tiny 2D-M554}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/555.png}}{{\tiny 2D-M555}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/556.png}}{{\tiny 2D-M556}}

  
    \end{minipage}
  \end{subfigure}
  \caption{Class 9 of 2-DOF Manipulators (Contd.)}
  \end{figure}

  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
  
  
 \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/557.png}}{{\tiny 2D-M557}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/558.png}}{{\tiny 2D-M558}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/559.png}}{{\tiny 2D-M559}}
    
      \end{minipage}
    \end{subfigure}
    \caption{Class 9 of 2-DOF Manipulators (Contd.)}
    \end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/560.png}}{{\tiny 2D-M560}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/561.png}}{{\tiny 2D-M561}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/562.png}}{{\tiny 2D-M562}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/563.png}}{{\tiny 2D-M563}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/564.png}}{{\tiny 2D-M564}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/565.png}}{{\tiny 2D-M565}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/566.png}}{{\tiny 2D-M566}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/567.png}}{{\tiny 2D-M567}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/568.png}}{{\tiny 2D-M568}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/569.png}}{{\tiny 2D-M569}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/570.png}}{{\tiny 2D-M570}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/571.png}}{{\tiny 2D-M571}}




  \end{minipage}
\end{subfigure}
\caption{Class 10 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  


    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/572.png}}{{\tiny 2D-M572}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/573.png}}{{\tiny 2D-M573}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/574.png}}{{\tiny 2D-M574}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/575.png}}{{\tiny 2D-M575}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/576.png}}{{\tiny 2D-M576}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/577.png}}{{\tiny 2D-M577}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/578.png}}{{\tiny 2D-M578}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/579.png}}{{\tiny 2D-M579}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/580.png}}{{\tiny 2D-M580}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/581.png}}{{\tiny 2D-M581}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/582.png}}{{\tiny 2D-M582}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/583.png}}{{\tiny 2D-M583}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/584.png}}{{\tiny 2D-M584}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/585.png}}{{\tiny 2D-M585}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/586.png}}{{\tiny 2D-M586}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/587.png}}{{\tiny 2D-M587}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/588.png}}{{\tiny 2D-M588}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/589.png}}{{\tiny 2D-M589}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/590.png}}{{\tiny 2D-M590}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/591.png}}{{\tiny 2D-M591}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/592.png}}{{\tiny 2D-M592}}
    

    \end{minipage}
  \end{subfigure}
  \caption{Class 10 of 2-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/593.png}}{{\tiny 2D-M593}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/594.png}}{{\tiny 2D-M594}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/595.png}}{{\tiny 2D-M595}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/596.png}}{{\tiny 2D-M596}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/597.png}}{{\tiny 2D-M597}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/598.png}}{{\tiny 2D-M598}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/599.png}}{{\tiny 2D-M599}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/600.png}}{{\tiny 2D-M600}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/601.png}}{{\tiny 2D-M601}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/602.png}}{{\tiny 2D-M602}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/603.png}}{{\tiny 2D-M603}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/604.png}}{{\tiny 2D-M604}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/605.png}}{{\tiny 2D-M605}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/606.png}}{{\tiny 2D-M606}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/607.png}}{{\tiny 2D-M607}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/608.png}}{{\tiny 2D-M608}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/609.png}}{{\tiny 2D-M609}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/610.png}}{{\tiny 2D-M610}}


  \end{minipage}
\end{subfigure}
\caption{Class 10 of 2-DOF Manipulators (Contd.)}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/611.png}}{{\tiny 2D-M611}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/612.png}}{{\tiny 2D-M612}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/613.png}}{{\tiny 2D-M613}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/614.png}}{{\tiny 2D-M614}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/615.png}}{{\tiny 2D-M615}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/616.png}}{{\tiny 2D-M616}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/617.png}}{{\tiny 2D-M617}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/618.png}}{{\tiny 2D-M618}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/619.png}}{{\tiny 2D-M619}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/620.png}}{{\tiny 2D-M620}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/621.png}}{{\tiny 2D-M621}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/622.png}}{{\tiny 2D-M622}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/623.png}}{{\tiny 2D-M623}}
    \end{minipage}
  \end{subfigure}
  \caption{Class 10 of 2-DOF Manipulators (Contd.)}
  \end{figure}


\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering

\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/624.png}}{{\tiny 2D-M624}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/625.png}}{{\tiny 2D-M625}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/626.png}}{{\tiny 2D-M626}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/627.png}}{{\tiny 2D-M627}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/628.png}}{{\tiny 2D-M628}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/629.png}}{{\tiny 2D-M629}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/630.png}}{{\tiny 2D-M630}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/631.png}}{{\tiny 2D-M631}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/632.png}}{{\tiny 2D-M632}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/633.png}}{{\tiny 2D-M633}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/634.png}}{{\tiny 2D-M634}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/635.png}}{{\tiny 2D-M635}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/636.png}}{{\tiny 2D-M636}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/637.png}}{{\tiny 2D-M637}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/638.png}}{{\tiny 2D-M638}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/639.png}}{{\tiny 2D-M639}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/640.png}}{{\tiny 2D-M640}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/641.png}}{{\tiny 2D-M641}}

  \end{minipage}
\end{subfigure}
\caption{Class 11 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/642.png}}{{\tiny 2D-M642}}

    \end{minipage}
  \end{subfigure}
  \caption{Class 12 of 2-DOF Manipulators}
  \end{figure}\begin{figure}[H]
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/643.png}}{{\tiny 2D-M643}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/644.png}}{{\tiny 2D-M644}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 13 of 2-DOF Manipulators}
  \end{figure}\begin{figure}[H]
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/645.png}}{{\tiny 2D-M645}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 14 of 2-DOF Manipulators}
  \end{figure}

==> Dimensional Synthesis/classes/3dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/1.png}}{{\tiny 3D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/2.png}}{{\tiny 3D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/3.png}}{{\tiny 3D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/4.png}}{{\tiny 3D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/5.png}}{{\tiny 3D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/6.png}}{{\tiny 3D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/7.png}}{{\tiny 3D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/8.png}}{{\tiny 3D-M8}}

  \end{minipage}
\end{subfigure}
\caption{Schematic diagrams of 3-DOF Manipulators}
\end{figure}



==> Dimensional Synthesis/classes/3dof_classes_old.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/1.png}}{{\tiny 3D-M1}}

  \end{minipage}
\end{subfigure}
\caption{Class 1 of 3-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/2.png}}{{\tiny 3D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/3.png}}{{\tiny 3D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/4.png}}{{\tiny 3D-M4}}

  \end{minipage}
\end{subfigure}
\caption{Class 2 of 3-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/5.png}}{{\tiny 3D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/6.png}}{{\tiny 3D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/7.png}}{{\tiny 3D-M7}}

  \end{minipage}
\end{subfigure}
\caption{Class 3 of 3-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/8.png}}{{\tiny 3D-M8}}

  \end{minipage}
\end{subfigure}
\caption{Class 4 of 3-DOF Manipulators}
\end{figure}

==> Dimensional Synthesis/classes/4dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/1.png}}{{\tiny 4D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/2.png}}{{\tiny 4D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/3.png}}{{\tiny 4D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/4.png}}{{\tiny 4D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/5.png}}{{\tiny 4D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/6.png}}{{\tiny 4D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/7.png}}{{\tiny 4D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/8.png}}{{\tiny 4D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/9.png}}{{\tiny 4D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/10.png}}{{\tiny 4D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/11.png}}{{\tiny 4D-M11}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/12.png}}{{\tiny 4D-M12}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/13.png}}{{\tiny 4D-M13}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/14.png}}{{\tiny 4D-M14}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/15.png}}{{\tiny 4D-M15}}

  \end{minipage}
\end{subfigure}
\caption{Schematic diagrams of 4-DOF Manipulators}
\end{figure}

==> Dimensional Synthesis/classes/4dof_classes_old.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/1.png}}{{\tiny 4D-M1}}

  \end{minipage}
\end{subfigure}
\caption{Class 1 of 4-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/2.png}}{{\tiny 4D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/3.png}}{{\tiny 4D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/4.png}}{{\tiny 4D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/5.png}}{{\tiny 4D-M5}}

  \end{minipage}
\end{subfigure}
\caption{Class 2 of 4-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/6.png}}{{\tiny 4D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/7.png}}{{\tiny 4D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/8.png}}{{\tiny 4D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/9.png}}{{\tiny 4D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/10.png}}{{\tiny 4D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/11.png}}{{\tiny 4D-M11}}

  \end{minipage}
\end{subfigure}
\caption{Class 3 of 4-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/12.png}}{{\tiny 4D-M12}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/13.png}}{{\tiny 4D-M13}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/14.png}}{{\tiny 4D-M14}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/15.png}}{{\tiny 4D-M15}}

  \end{minipage}
\end{subfigure}
\caption{Class 4 of 4-DOF Manipulators}
\end{figure}

==> Dimensional Synthesis/contentfolder/mechanisms2/1dof_manipulabilitytable_final.tex <==
\small
\begin{center}

\tablefirsthead{%

\hline
%\multicolumn{1}{|c}{\tbsp S.No.} &
\multicolumn{1}{|c|}{S.No.} &
%\tbsp S.No. &
%\multicolumn{1}{c}{Name} &
Name &
$\bar{\mu}$ &
%\multicolumn{1}{c}{$\mu$} &
$\mu$ &
\multicolumn{1}{c|}{$f$} &
AJV \\
\hline}
\tablehead{%
\hline
%\multicolumn{5}{|l|}{\small\sl continued from previous page}\\
\multicolumn{6}{|l|}{\small\sl continuing...}\\
\hline
\multicolumn{1}{|c|}{S.No.} &
Name &
$\bar{\mu}$ &
$\mu$ &
\multicolumn{1}{c|}{$f$} &
AJV \\
\hline}
\tabletail{%
\hline
%\multicolumn{5}{|r|}{\small\sl continued on next page}\\
\multicolumn{6}{|r|}{\small\sl ...continued}\\
\hline}
\tablelasttail{\hline}
\label{Tab:table_dof1mt_1}
%\customlabel{Tab:table_dof1mt_1}{2}
\bottomcaption{Prescription of 1-DOF Manipulators.}



%\tablehead{S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\}

%\begin{supertabular}{||c|c|c|c|c||}
\begin{supertabular}{|r|r|r|r|r|r|}
%\begin{longtable}{||c|c|c|c|c||}
%\hline
%S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\ 
\hline
1 & 1D-M10 & 0.1523 & 8.1 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline2 & 1D-M65 & 0.1376 & 10.5 & $f_2$ & $\dot{\theta}_{14}$ \\
\hline3 & 1D-M8 & 0.1152 & 7.1 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline4 & 1D-M94 & 0.1106 & 1.0 & $f_2$ & $\dot{d}_{24}$ \\
\hline5 & 1D-M28 & 0.1088 & 8.1 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline6 & 1D-M20 & 0.0824 & 10.5 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline7 & 1D-M34 & 0.0798 & 7.1 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline8 & 1D-M95 & 0.0776 & 1.0 & $f_2$ & $\dot{d}_{12}$ \\
\hline9 & 1D-M7 & 0.0774 & 8.4 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline10 & 1D-M29 & 0.0732 & 10.5 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline11 & 1D-M41 & 0.0722 & 9.5 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline12 & 1D-M40 & 0.071 & 7.1 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline13 & 1D-M35 & 0.0706 & 10.5 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline14 & 1D-M11 & 0.062 & 10.5 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline15 & 1D-M64 & 0.0563 & 20.3 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline16 & 1D-M66 & 0.0487 & 19.8 & $f_2$ & $\dot{\theta}_{23}$ \\
\hline17 & 1D-M60 & 0.0475 & 8.4 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline18 & 1D-M93 & 0.0467 & 1.0 & $f_2$ & $\dot{d}_{23}$ \\
\hline19 & 1D-M59 & 0.0462 & 9.5 & $f_1$ & $\dot{\theta}_{14}$ \\
\hline20 & 1D-M91 & 0.0438 & 1.0 & $f_2$ & $\dot{d}_{13}$ \\
\hline21 & 1D-M79 & 0.0335 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline22 & 1D-M25 & 0.0313 & 17.3 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline23 & 1D-M44 & 0.0313 & 17.3 & $f_2$ & $\dot{\theta}_{23}$ \\
\hline24 & 1D-M67 & 0.0306 & 18.3 & $f_2$ & $\dot{\theta}_{24}$ \\
\hline25 & 1D-M15 & 0.0305 & 21.2 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline26 & 1D-M22 & 0.0246 & 17.3 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline27 & 1D-M13 & 0.024 & 15.3 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline28 & 1D-M46 & 0.0237 & 15.3 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline29 & 1D-M45 & 0.0229 & 17.3 & $f_2$ & $\dot{\theta}_{24}$ \\
\hline30 & 1D-M3 & 0.0222 & 15.4 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline31 & 1D-M49 & 0.0219 & 14.1 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline32 & 1D-M68 & 0.0214 & 19.6 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline33 & 1D-M5 & 0.0212 & 14.7 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline34 & 1D-M47 & 0.0212 & 17.3 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline35 & 1D-M24 & 0.0212 & 17.3 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline36 & 1D-M51 & 0.0203 & 14.9 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline37 & 1D-M18 & 0.0194 & 14.6 & $f_2$ & $\dot{\theta}_{24}$ \\
\hline38 & 1D-M69 & 0.019 & 19.0 & $f_2$ & $\dot{\theta}_{24}$ \\
\hline39 & 1D-M48 & 0.0189 & 14.0 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline40 & 1D-M12 & 0.0188 & 12.8 & $f_2$ & $\dot{\theta}_{23}$ \\
\hline41 & 1D-M9 & 0.0185 & 12.8 & $f_2$ & $\dot{\theta}_{23}$ \\
\hline42 & 1D-M23 & 0.0177 & 13.0 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline43 & 1D-M62 & 0.0167 & 9.6 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline44 & 1D-M26 & 0.0167 & 9.6 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline45 & 1D-M14 & 0.0163 & 10.1 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline46 & 1D-M96 & 0.016 & 1.0 & $f_2$ & $\dot{d}_{24}$ \\
\hline47 & 1D-M6 & 0.0159 & 12.0 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline48 & 1D-M4 & 0.0158 & 13.4 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline49 & 1D-M89 & 0.0155 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline50 & 1D-M38 & 0.0153 & 12.9 & $f_2$ & $\dot{\theta}_{23}$ \\
\hline51 & 1D-M58 & 0.0148 & 8.2 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline52 & 1D-M57 & 0.0143 & 11.7 & $f_2$ & $\dot{\theta}_{34}$ \\
\hline53 & 1D-M76 & 0.0138 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline54 & 1D-M17 & 0.0136 & 8.6 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline55 & 1D-M50 & 0.0135 & 11.1 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline56 & 1D-M19 & 0.0134 & 10.3 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline57 & 1D-M56 & 0.0129 & 10.5 & $f_2$ & $\dot{\theta}_{24}$ \\
\hline58 & 1D-M21 & 0.0128 & 10.5 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline59 & 1D-M27 & 0.0127 & 9.3 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline60 & 1D-M77 & 0.0126 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline61 & 1D-M16 & 0.0125 & 9.3 & $f_2$ & $\dot{\theta}_{12}$ \\
\hline62 & 1D-M2 & 0.0116 & 6.7 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline63 & 1D-M1 & 0.0113 & 8.4 & $f_2$ & $\dot{\theta}_{13}$ \\
\hline64 & 1D-M43 & 0.0108 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline65 & 1D-M39 & 0.01 & 8.5 & $f_2$ & $\dot{\theta}_{24}$ \\
\hline66 & 1D-M80 & 0.0082 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline67 & 1D-M36 & 0.0081 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline68 & 1D-M92 & 0.0071 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline69 & 1D-M61 & 0.0051 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline70 & 1D-M42 & 0.0034 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline71 & 1D-M31 & 0.0031 & 1.7 & $f_2$ & $\dot{d}_{13}$ \\
\hline72 & 1D-M37 & 0.0025 & 1 & $f_1$ & $\dot{d}_{14}$ \\
\hline73 & 1D-M86 & 0.0021 & 1.0 & $f_2$ & $\dot{d}_{12}$ \\
\hline74 & 1D-M30 & 0.002 & 1.1 & $f_2$ & $\dot{d}_{13}$ \\
\hline75 & 1D-M53 & 0.0017 & 1.1 & $f_2$ & $\dot{d}_{12}$ \\
\hline76 & 1D-M83 & 0.0016 & 1.0 & $f_2$ & $\dot{d}_{12}$ \\
\hline77 & 1D-M84 & 0.0015 & 1.0 & $f_2$ & $\dot{d}_{12}$ \\
\hline78 & 1D-M87 & 0.0015 & 1.0 & $f_2$ & $\dot{d}_{24}$ \\
\hline79 & 1D-M55 & 0.0015 & 1.3 & $f_2$ & $\dot{d}_{12}$ \\
\hline80 & 1D-M71 & 0.0015 & 1.0 & $f_2$ & $\dot{d}_{13}$ \\
\hline81 & 1D-M73 & 0.0015 & 1.0 & $f_2$ & $\dot{d}_{13}$ \\
\hline82 & 1D-M90 & 0.0015 & 1.0 & $f_2$ & $\dot{d}_{12}$ \\
\hline83 & 1D-M52 & 0.0015 & 1.1 & $f_2$ & $\dot{d}_{12}$ \\
\hline84 & 1D-M82 & 0.0014 & 1.0 & $f_2$ & $\dot{d}_{12}$ \\
\hline85 & 1D-M72 & 0.0014 & 1 & $f_2$ & $\dot{d}_{13}$ \\
\hline86 & 1D-M70 & 0.0014 & 1.0 & $f_2$ & $\dot{d}_{13}$ \\
\hline87 & 1D-M81 & 0.0014 & 1 & $f_2$ & $\dot{d}_{23}$ \\
\hline88 & 1D-M85 & 0.0014 & 1.0 & $f_2$ & $\dot{d}_{12}$ \\
\hline89 & 1D-M88 & 0.0014 & 1.0 & $f_2$ & $\dot{d}_{13}$ \\
\hline90 & 1D-M63 & 0.0013 & 1.1 & $f_2$ & $\dot{d}_{12}$ \\
\hline91 & 1D-M32 & 0.0013 & 0.7 & $f_2$ & $\dot{d}_{13}$ \\
\hline92 & 1D-M54 & 0.0013 & 1.1 & $f_2$ & $\dot{d}_{12}$ \\
\hline93 & 1D-M33 & 0.0012 & 0.8 & $f_2$ & $\dot{d}_{13}$ \\
\hline94 & 1D-M78 & 0.0009 & 0.6 & $f_2$ & $\dot{d}_{23}$ \\
\hline95 & 1D-M74 & 0.0008 & 0.6 & $f_2$ & $\dot{d}_{13}$ \\
\hline96 & 1D-M75 & 0.0006 & 0.4 & $f_2$ & $\dot{d}_{13}$ \\
\hline
%\caption{Manipulability of 1-DOF Manipulators}
%\label{Tab:table_dof1mt_1}

\end{supertabular}
\end{center}

%\end{longtable}

\normalsize

==> Dimensional Synthesis/contentfolder/mechanisms2/2dof_manipulabilitytable_final.tex <==
% \section*{Appendix A}
% \label{AppendixA}

\tiny
\begin{center}
%\label{Tab:table_dof2mt_1}
\tablefirsthead{%
\hline
%\multicolumn{1}{|c}{\tbsp S.No.} &
\multicolumn{1}{|c|}{S.No.} &
%\tbsp S.No. &
%\multicolumn{1}{c}{Name} &
Name &
$\bar{\mu}$ &
$\kappa$ &
$i_{\kappa}$ &
%\multicolumn{1}{c}{$\mu$} &
$\mu$ &
\multicolumn{1}{c|}{$f$} &
AJV \\
\hline}
\tablehead{%
\hline
%\multicolumn{5}{|l|}{\small\sl continued from previous page}\\
\multicolumn{8}{|l|}{\tiny\sl continuing...}\\
\hline
\multicolumn{1}{|c|}{S.No.} &
Name &
$\bar{\mu}$ &
$\kappa$ &
$i_{\kappa}$ &
$\mu$ &
\multicolumn{1}{c|}{$f$} &
AJV \\
\hline}
\tabletail{%
\hline
%\multicolumn{5}{|r|}{\small\sl continued on next page}\\
\multicolumn{8}{|r|}{\tiny\sl ...continued}\\
\hline}
\tablelasttail{\hline}
%\vskip -0.20cm
\bottomcaption{Prescription of 2-DOF Manipulators.}



%\tablehead{S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\}

%\begin{supertabular}{||c|c|c|c|c||}
\begin{supertabular}{|r|r|r|r|r|r|r|r|}
%\begin{longtable}{||c|c|c|c|c||}
%\hline
%S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\ 
\hline

1 & 2D-M645 & 1.0 & 1.0 & 6 & 1.0 & $f_1$ & $\dot{d}_{12},\dot{d}_{23}$ \\
\hline2 & 2D-M315 & 0.7544 & 1.2 & 155 & 87.4 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline3 & 2D-M301 & 0.7058 & 1.2 & 158 & 88.8 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline4 & 2D-M224 & 0.6366 & 1.1 & 127 & 60.2 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline5 & 2D-M308 & 0.6034 & 1.1 & 118 & 340.6 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline6 & 2D-M126 & 0.5855 & 1.3 & 207 & 88.8 & $f_1$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline7 & 2D-M309 & 0.5624 & 1.2 & 135 & 351.6 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline8 & 2D-M319 & 0.5621 & 1.4 & 230 & 283.4 & $f_2$ & $\dot{\theta}_{25},\dot{\theta}_{35}$ \\
\hline9 & 2D-M208 & 0.5495 & 1.2 & 172 & 68.1 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline10 & 2D-M134 & 0.541 & 1.1 & 107 & 100.5 & $f_1$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline11 & 2D-M248 & 0.5381 & 1.4 & 224 & 75.2 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline12 & 2D-M203 & 0.5289 & 1.3 & 198 & 68.1 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline13 & 2D-M634 & 0.5142 & 1.0 & 7 & 1 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline14 & 2D-M458 & 0.5116 & 1.0 & 32 & 1.0 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline15 & 2D-M74 & 0.5114 & 1.1 & 115 & 77.5 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline16 & 2D-M318 & 0.5006 & 1.1 & 130 & 298.9 & $f_2$ & $\dot{\theta}_{24},\dot{\theta}_{35}$ \\
\hline17 & 2D-M213 & 0.4948 & 1.3 & 183 & 60.2 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline18 & 2D-M304 & 0.4879 & 1.8 & 307 & 165.1 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline19 & 2D-M311 & 0.485 & 1.2 & 152 & 88.5 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline20 & 2D-M300 & 0.4831 & 2.1 & 316 & 144.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline21 & 2D-M314 & 0.4683 & 1.2 & 141 & 266.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline22 & 2D-M303 & 0.4571 & 1.6 & 294 & 181.6 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline23 & 2D-M305 & 0.4477 & 1.5 & 266 & 200.5 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline24 & 2D-M98 & 0.4435 & 1.3 & 180 & 88.8 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline25 & 2D-M302 & 0.4376 & 1.8 & 306 & 164.6 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline26 & 2D-M299 & 0.4327 & 1.7 & 298 & 192.7 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline27 & 2D-M86 & 0.4221 & 1.2 & 136 & 100.5 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline28 & 2D-M11 & 0.4196 & 1.1 & 117 & 60.2 & $f_1$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline29 & 2D-M313 & 0.418 & 1.1 & 108 & 232.3 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline30 & 2D-M312 & 0.4138 & 1.2 & 148 & 253.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline31 & 2D-M239 & 0.3908 & 1.1 & 104 & 80.4 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline32 & 2D-M317 & 0.3621 & 1.2 & 131 & 294.7 & $f_2$ & $\dot{\theta}_{24},\dot{\theta}_{25}$ \\
\hline33 & 2D-M237 & 0.3503 & 1.1 & 114 & 100.5 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline34 & 2D-M132 & 0.3441 & 1.4 & 228 & 88.8 & $f_1$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline35 & 2D-M232 & 0.3306 & 1.2 & 157 & 88.8 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline36 & 2D-M227 & 0.3291 & 1.0 & 70 & 204.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline37 & 2D-M286 & 0.3224 & 1.1 & 122 & 194.5 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{45}$ \\
\hline38 & 2D-M138 & 0.3142 & 1.1 & 111 & 100.5 & $f_1$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline39 & 2D-M226 & 0.3127 & 1.5 & 269 & 176.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline40 & 2D-M307 & 0.3125 & 1.5 & 281 & 186.7 & $f_2$ & $\dot{\theta}_{25},\dot{\theta}_{34}$ \\
\hline41 & 2D-M306 & 0.2991 & 1.5 & 259 & 212.1 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{34}$ \\
\hline42 & 2D-M310 & 0.2946 & 1.6 & 290 & 138.7 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline43 & 2D-M521 & 0.2929 & 8.9 & 334 & 8.4 & $f_1$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline44 & 2D-M145 & 0.2902 & 1.4 & 240 & 142.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline45 & 2D-M234 & 0.2884 & 1.1 & 120 & 162.0 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline46 & 2D-M59 & 0.2879 & 1.5 & 276 & 189.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline47 & 2D-M128 & 0.2829 & 1.2 & 133 & 60.2 & $f_1$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline48 & 2D-M187 & 0.2736 & 1.3 & 204 & 220.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline49 & 2D-M293 & 0.273 & 1.3 & 192 & 182.5 & $f_2$ & $\dot{\theta}_{25},\dot{\theta}_{45}$ \\
\hline50 & 2D-M118 & 0.273 & 1.3 & 191 & 182.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline51 & 2D-M135 & 0.273 & 1.3 & 190 & 182.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline52 & 2D-M256 & 0.2719 & 1.1 & 84 & 100.5 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline53 & 2D-M184 & 0.271 & 2.0 & 314 & 164.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline54 & 2D-M140 & 0.2705 & 1.1 & 119 & 75.9 & $f_1$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline55 & 2D-M209 & 0.2696 & 1.4 & 223 & 165.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline56 & 2D-M236 & 0.2691 & 1.9 & 312 & 149.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline57 & 2D-M282 & 0.2688 & 1.7 & 300 & 167.5 & $f_2$ & $\dot{\theta}_{24},\dot{\theta}_{25}$ \\
\hline58 & 2D-M9 & 0.2678 & 1.2 & 153 & 100.5 & $f_1$ & $\dot{\theta}_{14},\dot{\theta}_{45}$ \\
\hline59 & 2D-M182 & 0.2677 & 1.2 & 171 & 168.8 & $f_2$ & $\dot{\theta}_{25},\dot{\theta}_{34}$ \\
\hline60 & 2D-M144 & 0.2665 & 1.3 & 216 & 112.8 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline61 & 2D-M295 & 0.2587 & 1.2 & 174 & 119.2 & $f_2$ & $\dot{\theta}_{24},\dot{\theta}_{35}$ \\
\hline62 & 2D-M524 & 0.2581 & 9.0 & 335 & 8.4 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{23}$ \\
\hline63 & 2D-M316 & 0.256 & 1.2 & 175 & 168.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline64 & 2D-M285 & 0.2533 & 1.1 & 80 & 174.6 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline65 & 2D-M217 & 0.2526 & 1.6 & 284 & 126.4 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline66 & 2D-M116 & 0.2519 & 1.6 & 295 & 123.7 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{35}$ \\
\hline67 & 2D-M264 & 0.2518 & 7.7 & 325 & 7.1 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline68 & 2D-M152 & 0.2506 & 1.1 & 116 & 162.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline69 & 2D-M87 & 0.2471 & 1.4 & 227 & 132.4 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline70 & 2D-M522 & 0.2466 & 7.7 & 326 & 7.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline71 & 2D-M82 & 0.2439 & 1.2 & 173 & 88.8 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline72 & 2D-M88 & 0.2418 & 1.3 & 179 & 182.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline73 & 2D-M298 & 0.2387 & 1.5 & 265 & 202.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline74 & 2D-M526 & 0.2381 & 7.7 & 327 & 7.1 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{25}$ \\
\hline75 & 2D-M215 & 0.2377 & 1.4 & 241 & 100.5 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline76 & 2D-M143 & 0.2369 & 1.1 & 82 & 210.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline77 & 2D-M113 & 0.2355 & 1.4 & 226 & 101.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{35}$ \\
\hline78 & 2D-M61 & 0.233 & 1.8 & 305 & 113.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline79 & 2D-M546 & 0.2319 & 7.7 & 328 & 7.1 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline80 & 2D-M43 & 0.2307 & 1.4 & 246 & 135.8 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline81 & 2D-M71 & 0.2305 & 2.0 & 313 & 173.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline82 & 2D-M181 & 0.2289 & 1.3 & 219 & 142.6 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{34}$ \\
\hline83 & 2D-M80 & 0.2278 & 1.5 & 263 & 124.4 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline84 & 2D-M66 & 0.227 & 1.3 & 178 & 165.4 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline85 & 2D-M527 & 0.2263 & 9.0 & 339 & 8.4 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{34}$ \\
\hline86 & 2D-M185 & 0.2257 & 1.0 & 76 & 149.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline87 & 2D-M63 & 0.2253 & 1.5 & 271 & 134.9 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline88 & 2D-M103 & 0.2251 & 1.3 & 209 & 123.4 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{35}$ \\
\hline89 & 2D-M251 & 0.2246 & 1.3 & 181 & 141.0 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline90 & 2D-M177 & 0.2241 & 1.5 & 279 & 111.0 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline91 & 2D-M555 & 0.224 & 9.0 & 340 & 8.4 & $f_2$ & $\dot{d}_{35},\dot{\theta}_{23}$ \\
\hline92 & 2D-M284 & 0.223 & 2.0 & 315 & 136.6 & $f_2$ & $\dot{\theta}_{25},\dot{\theta}_{35}$ \\
\hline93 & 2D-M130 & 0.2218 & 1.3 & 193 & 126.6 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline94 & 2D-M212 & 0.2218 & 1.6 & 291 & 137.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline95 & 2D-M291 & 0.2201 & 1.6 & 288 & 123.7 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{35}$ \\
\hline96 & 2D-M223 & 0.2201 & 1.6 & 287 & 123.7 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline97 & 2D-M120 & 0.2189 & 1.0 & 61 & 145.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline98 & 2D-M639 & 0.2183 & 1.0 & 18 & 1.0 & $f_2$ & $\dot{d}_{23},\dot{d}_{45}$ \\
\hline99 & 2D-M468 & 0.2157 & 1.0 & 38 & 1.0 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline100 & 2D-M235 & 0.2155 & 1.3 & 199 & 109.6 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline101 & 2D-M525 & 0.2138 & 9.0 & 341 & 8.4 & $f_2$ & $\dot{d}_{34},\dot{\theta}_{23}$ \\
\hline102 & 2D-M188 & 0.2127 & 1.4 & 244 & 139.6 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline103 & 2D-M635 & 0.2096 & 1.0 & 48 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline104 & 2D-M631 & 0.208 & 1.0 & 11 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline105 & 2D-M68 & 0.208 & 1.2 & 164 & 175.5 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline106 & 2D-M514 & 0.2078 & 9.0 & 342 & 8.4 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline107 & 2D-M146 & 0.2056 & 1.2 & 161 & 182.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline108 & 2D-M297 & 0.204 & 1.9 & 310 & 155.9 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline109 & 2D-M56 & 0.2028 & 1.1 & 95 & 159.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline110 & 2D-M100 & 0.2023 & 1.6 & 293 & 178.8 & $f_2$ & $\dot{\theta}_{24},\dot{\theta}_{25}$ \\
\hline111 & 2D-M190 & 0.202 & 10.2 & 351 & 9.5 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline112 & 2D-M137 & 0.2016 & 1.0 & 68 & 149.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline113 & 2D-M629 & 0.2016 & 1.0 & 36 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline114 & 2D-M180 & 0.1995 & 1.4 & 225 & 109.1 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline115 & 2D-M127 & 0.1984 & 1.3 & 201 & 165.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline116 & 2D-M512 & 0.1978 & 9.1 & 343 & 8.4 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{14}$ \\
\hline117 & 2D-M246 & 0.1971 & 1.3 & 184 & 132.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline118 & 2D-M76 & 0.1969 & 2.5 & 321 & 138.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline119 & 2D-M85 & 0.1964 & 1.1 & 121 & 140.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline120 & 2D-M121 & 0.1964 & 1.2 & 132 & 144.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline121 & 2D-M231 & 0.195 & 1.2 & 144 & 143.0 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline122 & 2D-M222 & 0.1949 & 1.4 & 242 & 107.6 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline123 & 2D-M250 & 0.1936 & 1.3 & 185 & 107.3 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline124 & 2D-M210 & 0.1922 & 1.1 & 105 & 135.4 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline125 & 2D-M257 & 0.1919 & 1.4 & 220 & 130.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline126 & 2D-M523 & 0.1895 & 7.8 & 329 & 7.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline127 & 2D-M53 & 0.1889 & 1.0 & 57 & 111.8 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline128 & 2D-M69 & 0.1883 & 1.3 & 212 & 147.5 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline129 & 2D-M529 & 0.1881 & 11.2 & 381 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{34}$ \\
\hline130 & 2D-M276 & 0.1869 & 11.2 & 382 & 10.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline131 & 2D-M216 & 0.1861 & 1.3 & 217 & 104.7 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline132 & 2D-M142 & 0.1846 & 1.2 & 169 & 149.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline133 & 2D-M101 & 0.1844 & 1.2 & 176 & 120.0 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline134 & 2D-M557 & 0.1843 & 10.2 & 352 & 9.5 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{45}$ \\
\hline135 & 2D-M221 & 0.182 & 1.4 & 248 & 130.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline136 & 2D-M183 & 0.1812 & 1.3 & 205 & 101.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline137 & 2D-M141 & 0.1806 & 1.5 & 272 & 81.9 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline138 & 2D-M202 & 0.1799 & 1.1 & 103 & 110.3 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline139 & 2D-M102 & 0.1795 & 1.3 & 213 & 95.2 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{45}$ \\
\hline140 & 2D-M124 & 0.176 & 1.2 & 137 & 119.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline141 & 2D-M513 & 0.1754 & 11.2 & 383 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline142 & 2D-M94 & 0.1753 & 1.4 & 236 & 88.8 & $f_1$ & $\dot{\theta}_{13},\dot{\theta}_{35}$ \\
\hline143 & 2D-M517 & 0.175 & 11.2 & 384 & 10.5 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{14}$ \\
\hline144 & 2D-M99 & 0.1747 & 1.1 & 92 & 132.9 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline145 & 2D-M554 & 0.1742 & 11.2 & 385 & 10.5 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{23}$ \\
\hline146 & 2D-M519 & 0.174 & 11.2 & 386 & 10.5 & $f_2$ & $\dot{d}_{34},\dot{\theta}_{14}$ \\
\hline147 & 2D-M207 & 0.1733 & 1.0 & 52 & 124.9 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline148 & 2D-M60 & 0.1729 & 2.4 & 319 & 130.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline149 & 2D-M559 & 0.1727 & 11.2 & 387 & 10.5 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{25}$ \\
\hline150 & 2D-M62 & 0.1717 & 1.1 & 112 & 120.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline151 & 2D-M632 & 0.171 & 1.0 & 27 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline152 & 2D-M111 & 0.1708 & 1.3 & 211 & 109.6 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline153 & 2D-M545 & 0.1704 & 11.2 & 389 & 10.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline154 & 2D-M48 & 0.17 & 1.3 & 182 & 117.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline155 & 2D-M96 & 0.169 & 1.2 & 156 & 96.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline156 & 2D-M186 & 0.1684 & 1.7 & 297 & 108.9 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline157 & 2D-M214 & 0.1681 & 1.1 & 129 & 101.3 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline158 & 2D-M110 & 0.1679 & 1.1 & 93 & 135.3 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline159 & 2D-M601 & 0.1676 & 1.0 & 34 & 1.0 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline160 & 2D-M46 & 0.1674 & 1.2 & 145 & 100.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline161 & 2D-M518 & 0.1665 & 11.2 & 390 & 10.5 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline162 & 2D-M122 & 0.166 & 1.2 & 142 & 104.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline163 & 2D-M283 & 0.1653 & 1.6 & 292 & 123.1 & $f_2$ & $\dot{\theta}_{24},\dot{\theta}_{35}$ \\
\hline164 & 2D-M97 & 0.1652 & 1.5 & 280 & 112.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline165 & 2D-M627 & 0.1651 & 1.0 & 28 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{24}$ \\
\hline166 & 2D-M204 & 0.1636 & 1.4 & 253 & 92.9 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline167 & 2D-M558 & 0.1626 & 11.2 & 391 & 10.5 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{35}$ \\
\hline168 & 2D-M296 & 0.1625 & 1.2 & 134 & 119.5 & $f_2$ & $\dot{\theta}_{24},\dot{\theta}_{25}$ \\
\hline169 & 2D-M131 & 0.1618 & 1.2 & 143 & 128.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline170 & 2D-M623 & 0.1613 & 1.0 & 14 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline171 & 2D-M640 & 0.1608 & 1.0 & 43 & 1.0 & $f_2$ & $\dot{d}_{23},\dot{d}_{35}$ \\
\hline172 & 2D-M107 & 0.1602 & 1.1 & 83 & 120.8 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline173 & 2D-M515 & 0.1581 & 11.2 & 392 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline174 & 2D-M49 & 0.1576 & 1.1 & 109 & 91.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline175 & 2D-M108 & 0.1576 & 1.1 & 99 & 127.9 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline176 & 2D-M597 & 0.1569 & 1.0 & 41 & 1.0 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline177 & 2D-M136 & 0.1553 & 1.2 & 139 & 126.7 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline178 & 2D-M292 & 0.1543 & 1.2 & 163 & 124.6 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline179 & 2D-M45 & 0.1538 & 1.3 & 218 & 137.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline180 & 2D-M148 & 0.1535 & 1.0 & 56 & 91.6 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline181 & 2D-M243 & 0.1534 & 11.3 & 393 & 10.5 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline182 & 2D-M104 & 0.1515 & 1.1 & 102 & 121.5 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline183 & 2D-M638 & 0.1508 & 1.0 & 31 & 1.0 & $f_2$ & $\dot{d}_{25},\dot{d}_{35}$ \\
\hline184 & 2D-M225 & 0.1494 & 1.1 & 81 & 109.5 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline185 & 2D-M454 & 0.1488 & 10.3 & 354 & 9.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline186 & 2D-M84 & 0.1484 & 1.6 & 283 & 114.9 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline187 & 2D-M47 & 0.1467 & 1.3 & 189 & 103.7 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline188 & 2D-M44 & 0.1466 & 1.4 & 247 & 121.1 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline189 & 2D-M241 & 0.1455 & 1.4 & 257 & 90.4 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline190 & 2D-M114 & 0.1451 & 1.1 & 98 & 116.6 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{35}$ \\
\hline191 & 2D-M528 & 0.1447 & 11.3 & 395 & 10.5 & $f_2$ & $\dot{d}_{34},\dot{\theta}_{25}$ \\
\hline192 & 2D-M621 & 0.1437 & 1.0 & 30 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline193 & 2D-M478 & 0.1431 & 10.3 & 355 & 9.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline194 & 2D-M268 & 0.1428 & 11.3 & 396 & 10.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline195 & 2D-M609 & 0.1385 & 1.0 & 40 & 1.0 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline196 & 2D-M133 & 0.1381 & 1.5 & 277 & 94.7 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline197 & 2D-M90 & 0.1378 & 1.2 & 140 & 100.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline198 & 2D-M51 & 0.1372 & 1.4 & 254 & 104.1 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline199 & 2D-M95 & 0.1364 & 1.2 & 150 & 90.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline200 & 2D-M115 & 0.1354 & 1.1 & 128 & 91.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline201 & 2D-M89 & 0.1353 & 1.5 & 270 & 87.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline202 & 2D-M371 & 0.1352 & 7.7 & 324 & 6.8 & $f_1$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline203 & 2D-M238 & 0.134 & 1.4 & 249 & 85.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline204 & 2D-M129 & 0.1339 & 1.0 & 13 & 91.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline205 & 2D-M81 & 0.1336 & 1.3 & 195 & 98.0 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline206 & 2D-M626 & 0.133 & 1.0 & 49 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline207 & 2D-M625 & 0.1323 & 1.0 & 20 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{45}$ \\
\hline208 & 2D-M516 & 0.1323 & 10.4 & 356 & 9.5 & $f_2$ & $\dot{d}_{34},\dot{\theta}_{14}$ \\
\hline209 & 2D-M5 & 0.1309 & 1.3 & 206 & 100.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline210 & 2D-M52 & 0.1305 & 1.6 & 286 & 100.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline211 & 2D-M247 & 0.1293 & 1.6 & 285 & 88.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline212 & 2D-M109 & 0.1284 & 1.4 & 233 & 105.7 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline213 & 2D-M64 & 0.128 & 1.0 & 75 & 85.3 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline214 & 2D-M83 & 0.1275 & 1.0 & 15 & 111.0 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline215 & 2D-M75 & 0.1272 & 1.3 & 202 & 88.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline216 & 2D-M447 & 0.1272 & 11.4 & 397 & 10.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline217 & 2D-M79 & 0.1264 & 1.6 & 296 & 75.3 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline218 & 2D-M245 & 0.1264 & 1.1 & 100 & 96.5 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline219 & 2D-M65 & 0.1258 & 1.0 & 51 & 90.7 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{25}$ \\
\hline220 & 2D-M8 & 0.1255 & 1.7 & 301 & 86.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline221 & 2D-M54 & 0.125 & 1.2 & 149 & 68.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline222 & 2D-M4 & 0.1247 & 1.9 & 311 & 62.0 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline223 & 2D-M3 & 0.1245 & 1.1 & 123 & 88.7 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline224 & 2D-M72 & 0.1243 & 1.2 & 168 & 74.9 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline225 & 2D-M6 & 0.1242 & 1.0 & 62 & 111.1 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline226 & 2D-M544 & 0.1241 & 17.5 & 604 & 17.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline227 & 2D-M50 & 0.1236 & 1.2 & 151 & 85.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline228 & 2D-M414 & 0.1229 & 10.4 & 359 & 9.5 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline229 & 2D-M151 & 0.1218 & 1.0 & 72 & 93.3 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline230 & 2D-M7 & 0.1216 & 1.4 & 222 & 100.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline231 & 2D-M41 & 0.1211 & 1.2 & 154 & 98.8 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline232 & 2D-M117 & 0.121 & 1.0 & 66 & 92.3 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline233 & 2D-M150 & 0.121 & 1.0 & 67 & 92.3 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline234 & 2D-M106 & 0.1209 & 1.3 & 208 & 92.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline235 & 2D-M211 & 0.1199 & 2.2 & 318 & 87.7 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline236 & 2D-M57 & 0.1189 & 1.5 & 268 & 96.6 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline237 & 2D-M139 & 0.1182 & 1.3 & 177 & 69.6 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline238 & 2D-M240 & 0.1178 & 1.1 & 125 & 88.9 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline239 & 2D-M105 & 0.1177 & 1.2 & 162 & 89.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline240 & 2D-M541 & 0.1172 & 9.3 & 345 & 8.4 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline241 & 2D-M249 & 0.117 & 1.5 & 278 & 95.3 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline242 & 2D-M78 & 0.1165 & 1.1 & 113 & 68.5 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline243 & 2D-M70 & 0.1162 & 1.1 & 101 & 57.4 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline244 & 2D-M530 & 0.1158 & 17.4 & 599 & 17.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline245 & 2D-M58 & 0.1149 & 1.3 & 214 & 63.5 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline246 & 2D-M93 & 0.1146 & 1.5 & 273 & 88.8 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline247 & 2D-M125 & 0.1145 & 1.5 & 260 & 78.1 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline248 & 2D-M10 & 0.1143 & 1.7 & 302 & 86.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline249 & 2D-M112 & 0.1143 & 1.3 & 194 & 72.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline250 & 2D-M15 & 0.1138 & 1.7 & 303 & 86.0 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline251 & 2D-M149 & 0.1138 & 1.0 & 74 & 72.9 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline252 & 2D-M147 & 0.1138 & 1.0 & 73 & 72.9 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline253 & 2D-M294 & 0.1137 & 1.5 & 258 & 85.6 & $f_2$ & $\dot{\theta}_{24},\dot{\theta}_{45}$ \\
\hline254 & 2D-M178 & 0.1129 & 1.1 & 96 & 77.5 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{34}$ \\
\hline255 & 2D-M551 & 0.1124 & 17.4 & 598 & 17.4 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{35}$ \\
\hline256 & 2D-M123 & 0.1121 & 1.2 & 160 & 75.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline257 & 2D-M2 & 0.1115 & 1.2 & 159 & 100.4 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{25}$ \\
\hline258 & 2D-M119 & 0.1105 & 1.3 & 215 & 68.1 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{23}$ \\
\hline259 & 2D-M624 & 0.1091 & 1.0 & 35 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{34}$ \\
\hline260 & 2D-M290 & 0.1086 & 1.1 & 97 & 90.6 & $f_2$ & $\dot{\theta}_{23},\dot{\theta}_{45}$ \\
\hline261 & 2D-M1 & 0.106 & 1.9 & 309 & 74.0 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline262 & 2D-M67 & 0.1059 & 1.5 & 264 & 79.0 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{14}$ \\
\hline263 & 2D-M531 & 0.1058 & 17.6 & 605 & 17.5 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{13}$ \\
\hline264 & 2D-M463 & 0.1045 & 10.5 & 360 & 9.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline265 & 2D-M641 & 0.1036 & 1.0 & 42 & 1.0 & $f_2$ & $\dot{d}_{23},\dot{d}_{25}$ \\
\hline266 & 2D-M532 & 0.1028 & 17.4 & 597 & 17.4 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline267 & 2D-M636 & 0.1026 & 1.0 & 33 & 1.0 & $f_2$ & $\dot{d}_{24},\dot{d}_{25}$ \\
\hline268 & 2D-M630 & 0.1021 & 1.0 & 45 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{23}$ \\
\hline269 & 2D-M434 & 0.1012 & 10.5 & 361 & 9.5 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline270 & 2D-M29 & 0.101 & 8.2 & 331 & 7.1 & $f_1$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline271 & 2D-M637 & 0.1006 & 1.0 & 5 & 1.0 & $f_2$ & $\dot{d}_{24},\dot{d}_{35}$ \\
\hline272 & 2D-M233 & 0.099 & 2.5 & 320 & 82.4 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{25}$ \\
\hline273 & 2D-M77 & 0.099 & 1.4 & 255 & 63.5 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{24}$ \\
\hline274 & 2D-M55 & 0.0984 & 1.5 & 262 & 78.8 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{34}$ \\
\hline275 & 2D-M553 & 0.097 & 16.8 & 575 & 16.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{35}$ \\
\hline276 & 2D-M42 & 0.0964 & 1.4 & 221 & 60.2 & $f_2$ & $\dot{\theta}_{14},\dot{\theta}_{24}$ \\
\hline277 & 2D-M642 & 0.0962 & 1.0 & 9 & 111.0 & $f_1$ & $\dot{\theta}_{12},\dot{\theta}_{23}$ \\
\hline278 & 2D-M255 & 0.0945 & 1.8 & 308 & 76.7 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline279 & 2D-M409 & 0.093 & 10.6 & 362 & 9.5 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline280 & 2D-M620 & 0.0923 & 1.0 & 16 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{24}$ \\
\hline281 & 2D-M452 & 0.0922 & 10.6 & 363 & 9.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline282 & 2D-M471 & 0.091 & 11.6 & 403 & 10.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline283 & 2D-M179 & 0.0906 & 1.0 & 78 & 62.8 & $f_2$ & $\dot{\theta}_{25},\dot{\theta}_{34}$ \\
\hline284 & 2D-M438 & 0.0901 & 9.2 & 344 & 8.1 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline285 & 2D-M92 & 0.0898 & 1.5 & 267 & 62.1 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline286 & 2D-M91 & 0.0896 & 1.4 & 231 & 49.5 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{23}$ \\
\hline287 & 2D-M73 & 0.088 & 1.3 & 197 & 48.2 & $f_2$ & $\dot{\theta}_{13},\dot{\theta}_{45}$ \\
\hline288 & 2D-M622 & 0.0869 & 1.0 & 39 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline289 & 2D-M365 & 0.0868 & 11.6 & 406 & 10.5 & $f_1$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline290 & 2D-M482 & 0.0862 & 1.0 & 44 & 1.0 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline291 & 2D-M547 & 0.0855 & 10.4 & 357 & 9.3 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline292 & 2D-M426 & 0.0843 & 10.6 & 366 & 9.5 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline293 & 2D-M27 & 0.0834 & 11.6 & 408 & 10.5 & $f_1$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline294 & 2D-M538 & 0.0833 & 11.8 & 416 & 10.1 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline295 & 2D-M495 & 0.0823 & 11.6 & 409 & 10.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline296 & 2D-M536 & 0.0805 & 19.8 & 622 & 19.8 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline297 & 2D-M373 & 0.0742 & 11.7 & 412 & 10.5 & $f_1$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline298 & 2D-M280 & 0.0736 & 11.7 & 413 & 10.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline299 & 2D-M476 & 0.073 & 11.7 & 414 & 10.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline300 & 2D-M377 & 0.0705 & 10.8 & 369 & 9.5 & $f_1$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline301 & 2D-M253 & 0.0693 & 11.8 & 415 & 10.5 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline302 & 2D-M540 & 0.0692 & 20.2 & 629 & 20.2 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline303 & 2D-M539 & 0.067 & 20.2 & 630 & 20.2 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline304 & 2D-M549 & 0.0656 & 20.2 & 626 & 20.2 & $f_2$ & $\dot{d}_{35},\dot{\theta}_{24}$ \\
\hline305 & 2D-M552 & 0.0605 & 20.2 & 627 & 20.2 & $f_2$ & $\dot{d}_{35},\dot{\theta}_{25}$ \\
\hline306 & 2D-M537 & 0.0603 & 20.2 & 628 & 20.2 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline307 & 2D-M533 & 0.0579 & 9.0 & 336 & 6.4 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline308 & 2D-M32 & 0.0565 & 1.0 & 22 & 1.0 & $f_1$ & $\dot{d}_{14},\dot{d}_{45}$ \\
\hline309 & 2D-M633 & 0.0525 & 1.0 & 46 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline310 & 2D-M219 & 0.0514 & 8.8 & 333 & 7.1 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline311 & 2D-M422 & 0.0484 & 10.1 & 350 & 8.4 & $f_1$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline312 & 2D-M492 & 0.0458 & 1.0 & 10 & 1 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline313 & 2D-M379 & 0.0441 & 12.2 & 433 & 10.5 & $f_1$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline314 & 2D-M487 & 0.0401 & 12.3 & 436 & 10.5 & $f_1$ & $\dot{d}_{13},\dot{\theta}_{35}$ \\
\hline315 & 2D-M420 & 0.0335 & 14.1 & 512 & 14.2 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{13}$ \\
\hline316 & 2D-M589 & 0.0333 & 1.0 & 37 & 1.0 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline317 & 2D-M613 & 0.0326 & 1.0 & 47 & 1.0 & $f_1$ & $\dot{d}_{13},\dot{d}_{35}$ \\
\hline318 & 2D-M498 & 0.032 & 17.2 & 580 & 17.4 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{25}$ \\
\hline319 & 2D-M352 & 0.0318 & 17.3 & 585 & 17.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{35}$ \\
\hline320 & 2D-M157 & 0.0297 & 20.8 & 636 & 20.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline321 & 2D-M262 & 0.0296 & 11.2 & 388 & 18.1 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline322 & 2D-M218 & 0.0294 & 17.0 & 579 & 16.8 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline323 & 2D-M542 & 0.0293 & 16.8 & 573 & 15.8 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline324 & 2D-M172 & 0.0289 & 17.5 & 601 & 15.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline325 & 2D-M205 & 0.028 & 14.6 & 535 & 18.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline326 & 2D-M394 & 0.0271 & 12.8 & 451 & 8.6 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{34}$ \\
\hline327 & 2D-M520 & 0.027 & 19.4 & 618 & 18.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline328 & 2D-M421 & 0.0268 & 17.3 & 586 & 17.3 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline329 & 2D-M360 & 0.0268 & 17.3 & 582 & 17.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline330 & 2D-M413 & 0.0267 & 13.2 & 472 & 12.9 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline331 & 2D-M355 & 0.0266 & 14.1 & 523 & 14.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{35}$ \\
\hline332 & 2D-M349 & 0.0263 & 14.6 & 536 & 14.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline333 & 2D-M508 & 0.0263 & 17.6 & 606 & 16.4 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{24}$ \\
\hline334 & 2D-M407 & 0.0261 & 14.9 & 541 & 14.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline335 & 2D-M389 & 0.026 & 17.4 & 594 & 6.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline336 & 2D-M424 & 0.0259 & 16.1 & 561 & 18.4 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline337 & 2D-M450 & 0.0258 & 13.1 & 460 & 13.0 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline338 & 2D-M534 & 0.0254 & 19.9 & 624 & 18.6 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{13}$ \\
\hline339 & 2D-M548 & 0.0253 & 19.0 & 615 & 17.8 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{24}$ \\
\hline340 & 2D-M387 & 0.0245 & 17.3 & 590 & 6.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline341 & 2D-M412 & 0.0244 & 13.1 & 463 & 13.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline342 & 2D-M543 & 0.0241 & 18.5 & 610 & 18.0 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline343 & 2D-M556 & 0.024 & 20.4 & 633 & 18.6 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{23}$ \\
\hline344 & 2D-M346 & 0.0239 & 14.8 & 538 & 12.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline345 & 2D-M475 & 0.0238 & 17.0 & 578 & 17.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline346 & 2D-M288 & 0.0238 & 15.0 & 543 & 14.8 & $f_2$ & $\dot{d}_{35},\dot{\theta}_{23}$ \\
\hline347 & 2D-M507 & 0.0235 & 17.3 & 588 & 17.3 & $f_2$ & $\dot{d}_{35},\dot{\theta}_{24}$ \\
\hline348 & 2D-M348 & 0.0235 & 17.3 & 587 & 17.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline349 & 2D-M163 & 0.0234 & 13.7 & 481 & 12.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline350 & 2D-M242 & 0.023 & 18.4 & 609 & 13.8 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline351 & 2D-M550 & 0.023 & 19.1 & 617 & 17.7 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{25}$ \\
\hline352 & 2D-M24 & 0.0228 & 14.5 & 532 & 12.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline353 & 2D-M425 & 0.0226 & 14.1 & 522 & 14.1 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline354 & 2D-M357 & 0.0223 & 17.4 & 595 & 16.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline355 & 2D-M535 & 0.0222 & 19.8 & 623 & 18.4 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline356 & 2D-M406 & 0.0222 & 13.9 & 494 & 15.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline357 & 2D-M156 & 0.0222 & 16.8 & 572 & 13.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline358 & 2D-M252 & 0.0219 & 20.3 & 632 & 14.3 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline359 & 2D-M628 & 0.0217 & 1.0 & 26 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline360 & 2D-M366 & 0.0215 & 13.0 & 458 & 12.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline361 & 2D-M343 & 0.0215 & 12.1 & 429 & 7.8 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline362 & 2D-M155 & 0.0215 & 16.3 & 563 & 13.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline363 & 2D-M194 & 0.0214 & 16.3 & 562 & 13.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline364 & 2D-M502 & 0.0214 & 17.3 & 584 & 17.3 & $f_2$ & $\dot{d}_{35},\dot{\theta}_{23}$ \\
\hline365 & 2D-M374 & 0.0214 & 17.3 & 583 & 17.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline366 & 2D-M192 & 0.0213 & 16.1 & 560 & 13.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline367 & 2D-M354 & 0.021 & 17.0 & 577 & 14.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline368 & 2D-M168 & 0.0209 & 14.0 & 498 & 12.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline369 & 2D-M353 & 0.0208 & 14.3 & 531 & 11.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{35}$ \\
\hline370 & 2D-M465 & 0.0205 & 14.0 & 506 & 14.0 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline371 & 2D-M363 & 0.0203 & 15.1 & 545 & 15.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline372 & 2D-M160 & 0.0202 & 15.2 & 548 & 15.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline373 & 2D-M17 & 0.0202 & 14.1 & 511 & 14.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline374 & 2D-M484 & 0.0201 & 13.0 & 456 & 10.3 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline375 & 2D-M375 & 0.0199 & 10.9 & 378 & 10.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline376 & 2D-M415 & 0.0198 & 15.0 & 542 & 13.4 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline377 & 2D-M361 & 0.0195 & 11.4 & 398 & 11.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline378 & 2D-M411 & 0.0194 & 15.0 & 544 & 15.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline379 & 2D-M170 & 0.0194 & 15.7 & 556 & 11.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline380 & 2D-M164 & 0.0192 & 12.7 & 444 & 8.7 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline381 & 2D-M362 & 0.0192 & 12.5 & 442 & 9.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline382 & 2D-M230 & 0.0191 & 13.7 & 485 & 12.3 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline383 & 2D-M228 & 0.0191 & 12.9 & 452 & 12.9 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline384 & 2D-M16 & 0.0184 & 15.6 & 553 & 10.3 & $f_2$ & $\dot{\theta}_{13},\dot{d}_{45}$ \\
\hline385 & 2D-M267 & 0.0184 & 11.6 & 405 & 12.4 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline386 & 2D-M376 & 0.0184 & 11.4 & 399 & 10.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline387 & 2D-M410 & 0.0183 & 16.5 & 567 & 13.8 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline388 & 2D-M193 & 0.0181 & 10.8 & 370 & 9.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline389 & 2D-M378 & 0.0181 & 14.7 & 537 & 12.7 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline390 & 2D-M278 & 0.0181 & 16.1 & 558 & 10.6 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline391 & 2D-M158 & 0.0179 & 15.3 & 551 & 12.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline392 & 2D-M456 & 0.0178 & 19.8 & 621 & 13.2 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline393 & 2D-M344 & 0.0178 & 13.0 & 454 & 10.0 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline394 & 2D-M175 & 0.0177 & 18.9 & 613 & 10.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline395 & 2D-M474 & 0.0177 & 10.9 & 375 & 10.9 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline396 & 2D-M430 & 0.0175 & 10.4 & 358 & 11.7 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline397 & 2D-M497 & 0.0174 & 20.4 & 634 & 13.0 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{24}$ \\
\hline398 & 2D-M28 & 0.0174 & 14.1 & 524 & 14.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline399 & 2D-M26 & 0.0174 & 14.1 & 525 & 14.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline400 & 2D-M372 & 0.0173 & 10.9 & 376 & 10.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline401 & 2D-M485 & 0.0173 & 20.8 & 635 & 9.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline402 & 2D-M460 & 0.0171 & 12.4 & 439 & 9.4 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline403 & 2D-M503 & 0.017 & 15.2 & 547 & 12.3 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{23}$ \\
\hline404 & 2D-M439 & 0.017 & 15.2 & 546 & 12.3 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline405 & 2D-M489 & 0.017 & 17.8 & 608 & 10.8 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline406 & 2D-M201 & 0.0169 & 14.3 & 530 & 10.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline407 & 2D-M504 & 0.0169 & 13.0 & 457 & 11.3 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{25}$ \\
\hline408 & 2D-M173 & 0.0169 & 15.2 & 549 & 12.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline409 & 2D-M404 & 0.0169 & 13.5 & 475 & 10.7 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline410 & 2D-M277 & 0.0168 & 12.7 & 446 & 9.3 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline411 & 2D-M196 & 0.0166 & 11.8 & 419 & 13.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline412 & 2D-M364 & 0.0166 & 12.4 & 438 & 9.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline413 & 2D-M254 & 0.0166 & 12.2 & 430 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline414 & 2D-M390 & 0.0166 & 17.4 & 596 & 4.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline415 & 2D-M405 & 0.0165 & 11.6 & 404 & 10.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline416 & 2D-M381 & 0.0163 & 14.2 & 526 & 8.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline417 & 2D-M408 & 0.0162 & 10.3 & 353 & 10.3 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline418 & 2D-M477 & 0.0161 & 10.9 & 379 & 10.9 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline419 & 2D-M359 & 0.0161 & 10.9 & 377 & 10.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline420 & 2D-M174 & 0.0161 & 13.8 & 487 & 11.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline421 & 2D-M266 & 0.016 & 12.2 & 435 & 11.3 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline422 & 2D-M263 & 0.016 & 12.5 & 441 & 10.7 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline423 & 2D-M369 & 0.0159 & 9.0 & 337 & 9.0 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline424 & 2D-M199 & 0.0159 & 24.4 & 641 & 9.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline425 & 2D-M453 & 0.0159 & 11.7 & 411 & 10.9 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline426 & 2D-M500 & 0.0159 & 17.5 & 603 & 10.1 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{23}$ \\
\hline427 & 2D-M435 & 0.0158 & 12.0 & 422 & 8.7 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline428 & 2D-M198 & 0.0158 & 12.7 & 445 & 11.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline429 & 2D-M397 & 0.0156 & 14.1 & 514 & 9.3 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{34}$ \\
\hline430 & 2D-M473 & 0.0155 & 17.5 & 602 & 9.9 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline431 & 2D-M229 & 0.0155 & 12.7 & 448 & 9.5 & $f_2$ & $\dot{d}_{35},\dot{\theta}_{13}$ \\
\hline432 & 2D-M260 & 0.0154 & 11.8 & 420 & 8.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline433 & 2D-M23 & 0.0154 & 9.9 & 348 & 10.3 & $f_2$ & $\dot{d}_{34},\dot{\theta}_{14}$ \\
\hline434 & 2D-M461 & 0.0154 & 11.9 & 421 & 9.8 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline435 & 2D-M35 & 0.0153 & 11.5 & 402 & 12.9 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline436 & 2D-M427 & 0.0153 & 13.4 & 473 & 10.1 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline437 & 2D-M165 & 0.0153 & 11.7 & 410 & 7.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline438 & 2D-M200 & 0.0152 & 12.8 & 449 & 10.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline439 & 2D-M383 & 0.0152 & 11.6 & 407 & 10.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline440 & 2D-M385 & 0.0152 & 13.0 & 455 & 8.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline441 & 2D-M220 & 0.0151 & 11.8 & 417 & 8.6 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline442 & 2D-M499 & 0.015 & 13.8 & 489 & 9.3 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{35}$ \\
\hline443 & 2D-M153 & 0.0149 & 13.6 & 478 & 11.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline444 & 2D-M159 & 0.0148 & 14.1 & 520 & 9.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline445 & 2D-M340 & 0.0148 & 17.6 & 607 & 12.0 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline446 & 2D-M466 & 0.0148 & 11.5 & 400 & 10.4 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline447 & 2D-M419 & 0.0147 & 10.7 & 367 & 6.9 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{13}$ \\
\hline448 & 2D-M259 & 0.0146 & 12.2 & 431 & 8.9 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline449 & 2D-M273 & 0.0146 & 12.8 & 450 & 9.7 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline450 & 2D-M244 & 0.0146 & 13.7 & 482 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline451 & 2D-M451 & 0.0145 & 12.9 & 453 & 6.4 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline452 & 2D-M31 & 0.0145 & 8.2 & 330 & 8.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline453 & 2D-M289 & 0.0145 & 11.5 & 401 & 8.6 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{23}$ \\
\hline454 & 2D-M279 & 0.0144 & 12.5 & 440 & 8.7 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline455 & 2D-M417 & 0.0143 & 13.1 & 465 & 11.3 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{13}$ \\
\hline456 & 2D-M386 & 0.0143 & 17.3 & 589 & 5.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline457 & 2D-M342 & 0.0142 & 17.4 & 593 & 5.2 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline458 & 2D-M488 & 0.0141 & 13.1 & 461 & 11.3 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline459 & 2D-M167 & 0.014 & 10.6 & 365 & 7.0 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline460 & 2D-M501 & 0.0139 & 14.0 & 501 & 10.6 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{23}$ \\
\hline461 & 2D-M368 & 0.0139 & 14.0 & 502 & 10.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline462 & 2D-M480 & 0.0139 & 16.4 & 566 & 10.3 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline463 & 2D-M258 & 0.0139 & 9.8 & 346 & 6.8 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline464 & 2D-M392 & 0.0139 & 18.5 & 612 & 4.9 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{23}$ \\
\hline465 & 2D-M189 & 0.0139 & 13.8 & 491 & 10.4 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline466 & 2D-M154 & 0.0138 & 13.6 & 479 & 10.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline467 & 2D-M261 & 0.0138 & 14.0 & 507 & 10.6 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline468 & 2D-M510 & 0.0138 & 9.9 & 347 & 7.1 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{35}$ \\
\hline469 & 2D-M399 & 0.0138 & 16.6 & 568 & 11.0 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline470 & 2D-M14 & 0.0138 & 10.8 & 371 & 6.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline471 & 2D-M324 & 0.0137 & 13.8 & 488 & 10.6 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{14}$ \\
\hline472 & 2D-M382 & 0.0137 & 19.9 & 625 & 5.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline473 & 2D-M271 & 0.0136 & 13.9 & 496 & 10.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline474 & 2D-M403 & 0.0136 & 11.1 & 380 & 7.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline475 & 2D-M333 & 0.0136 & 13.9 & 497 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline476 & 2D-M12 & 0.0136 & 12.2 & 434 & 8.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline477 & 2D-M356 & 0.0136 & 10.8 & 372 & 7.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline478 & 2D-M331 & 0.0132 & 13.1 & 459 & 9.5 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline479 & 2D-M269 & 0.0132 & 13.5 & 476 & 10.8 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline480 & 2D-M281 & 0.0132 & 10.0 & 349 & 7.0 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline481 & 2D-M351 & 0.0132 & 14.2 & 528 & 10.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline482 & 2D-M431 & 0.0132 & 14.2 & 527 & 10.8 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{13}$ \\
\hline483 & 2D-M337 & 0.0132 & 12.0 & 424 & 8.4 & $f_2$ & $\dot{d}_{34},\dot{\theta}_{14}$ \\
\hline484 & 2D-M166 & 0.0132 & 14.0 & 499 & 9.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline485 & 2D-M265 & 0.0131 & 14.0 & 500 & 10.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline486 & 2D-M393 & 0.0131 & 18.5 & 611 & 4.9 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{25}$ \\
\hline487 & 2D-M462 & 0.0131 & 14.0 & 503 & 10.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline488 & 2D-M436 & 0.0131 & 14.0 & 504 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline489 & 2D-M334 & 0.0131 & 14.0 & 505 & 10.5 & $f_2$ & $\dot{d}_{34},\dot{\theta}_{14}$ \\
\hline490 & 2D-M329 & 0.013 & 12.0 & 425 & 8.4 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline491 & 2D-M384 & 0.013 & 21.4 & 639 & 10.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline492 & 2D-M395 & 0.013 & 21.3 & 638 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{23}$ \\
\hline493 & 2D-M396 & 0.013 & 19.7 & 619 & 7.1 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{25}$ \\
\hline494 & 2D-M162 & 0.013 & 10.8 & 368 & 7.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline495 & 2D-M206 & 0.013 & 10.9 & 374 & 8.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline496 & 2D-M274 & 0.013 & 12.0 & 423 & 8.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline497 & 2D-M511 & 0.013 & 13.9 & 495 & 10.6 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{25}$ \\
\hline498 & 2D-M418 & 0.0129 & 14.0 & 508 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline499 & 2D-M350 & 0.0129 & 14.1 & 510 & 10.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline500 & 2D-M370 & 0.0129 & 13.1 & 464 & 9.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline501 & 2D-M339 & 0.0129 & 11.3 & 394 & 7.1 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline502 & 2D-M347 & 0.0129 & 14.0 & 509 & 10.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline503 & 2D-M479 & 0.0129 & 13.8 & 492 & 10.3 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline504 & 2D-M287 & 0.0129 & 14.3 & 529 & 8.8 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{23}$ \\
\hline505 & 2D-M19 & 0.0129 & 10.8 & 373 & 7.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline506 & 2D-M470 & 0.0128 & 13.1 & 466 & 9.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline507 & 2D-M506 & 0.0128 & 11.8 & 418 & 8.1 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{24}$ \\
\hline508 & 2D-M437 & 0.0128 & 12.1 & 426 & 8.4 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline509 & 2D-M401 & 0.0128 & 13.1 & 468 & 9.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline510 & 2D-M338 & 0.0128 & 17.3 & 581 & 9.5 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline511 & 2D-M464 & 0.0127 & 14.1 & 513 & 10.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline512 & 2D-M433 & 0.0127 & 13.1 & 469 & 9.5 & $f_2$ & $\dot{d}_{45},\dot{\theta}_{13}$ \\
\hline513 & 2D-M423 & 0.0127 & 13.8 & 490 & 10.2 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline514 & 2D-M472 & 0.0127 & 13.1 & 462 & 9.6 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline515 & 2D-M336 & 0.0127 & 14.1 & 515 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline516 & 2D-M321 & 0.0126 & 12.1 & 427 & 8.4 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{14}$ \\
\hline517 & 2D-M380 & 0.0126 & 15.7 & 557 & 10.2 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline518 & 2D-M335 & 0.0126 & 14.1 & 516 & 10.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline519 & 2D-M21 & 0.0126 & 12.1 & 428 & 8.4 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{14}$ \\
\hline520 & 2D-M345 & 0.0126 & 13.2 & 470 & 9.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{24}$ \\
\hline521 & 2D-M367 & 0.0126 & 14.1 & 517 & 10.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{45}$ \\
\hline522 & 2D-M25 & 0.0126 & 13.2 & 471 & 9.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline523 & 2D-M320 & 0.0126 & 14.1 & 518 & 10.5 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{14}$ \\
\hline524 & 2D-M30 & 0.0125 & 14.1 & 519 & 10.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline525 & 2D-M323 & 0.0125 & 12.7 & 447 & 7.5 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{14}$ \\
\hline526 & 2D-M428 & 0.0123 & 16.8 & 576 & 10.1 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{13}$ \\
\hline527 & 2D-M496 & 0.0121 & 14.1 & 521 & 9.9 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline528 & 2D-M455 & 0.0121 & 12.6 & 443 & 8.1 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{23}$ \\
\hline529 & 2D-M330 & 0.0121 & 13.7 & 483 & 9.2 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline530 & 2D-M449 & 0.0121 & 9.0 & 338 & 5.1 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline531 & 2D-M169 & 0.012 & 10.6 & 364 & 8.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline532 & 2D-M161 & 0.012 & 15.3 & 550 & 10.1 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline533 & 2D-M402 & 0.0119 & 13.7 & 486 & 8.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline534 & 2D-M446 & 0.0119 & 15.6 & 554 & 9.5 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline535 & 2D-M429 & 0.0119 & 13.8 & 493 & 8.5 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{13}$ \\
\hline536 & 2D-M358 & 0.0117 & 13.5 & 474 & 9.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline537 & 2D-M275 & 0.0117 & 13.7 & 484 & 7.0 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline538 & 2D-M272 & 0.0117 & 13.1 & 467 & 9.2 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline539 & 2D-M327 & 0.0116 & 14.6 & 534 & 9.4 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline540 & 2D-M322 & 0.0116 & 14.6 & 533 & 9.5 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{14}$ \\
\hline541 & 2D-M490 & 0.0115 & 24.5 & 642 & 8.4 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline542 & 2D-M505 & 0.0114 & 24.4 & 640 & 8.4 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{45}$ \\
\hline543 & 2D-M13 & 0.0113 & 13.5 & 477 & 9.3 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline544 & 2D-M18 & 0.0112 & 12.3 & 437 & 8.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline545 & 2D-M432 & 0.0111 & 15.6 & 555 & 7.4 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{13}$ \\
\hline546 & 2D-M341 & 0.011 & 17.3 & 592 & 2.9 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline547 & 2D-M400 & 0.0109 & 26.1 & 644 & 7.8 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline548 & 2D-M191 & 0.0108 & 15.3 & 552 & 8.0 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{13}$ \\
\hline549 & 2D-M20 & 0.0107 & 8.7 & 332 & 6.6 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{35}$ \\
\hline550 & 2D-M388 & 0.0107 & 17.3 & 591 & 2.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline551 & 2D-M448 & 0.0105 & 12.2 & 432 & 5.8 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{25}$ \\
\hline552 & 2D-M325 & 0.0104 & 16.7 & 571 & 8.1 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline553 & 2D-M270 & 0.0098 & 16.7 & 570 & 6.6 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{24}$ \\
\hline554 & 2D-M643 & 0.0091 & 14.8 & 539 & 10.5 & $f_1$ & $\dot{\theta}_{12},\dot{d}_{23}$ \\
\hline555 & 2D-M644 & 0.0091 & 14.8 & 540 & 10.5 & $f_1$ & $\dot{d}_{12},\dot{\theta}_{23}$ \\
\hline556 & 2D-M416 & 0.0088 & 25.6 & 643 & 7.1 & $f_2$ & $\dot{d}_{24},\dot{\theta}_{13}$ \\
\hline557 & 2D-M195 & 0.0085 & 16.7 & 569 & 4.9 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline558 & 2D-M197 & 0.0084 & 13.6 & 480 & 4.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline559 & 2D-M22 & 0.0082 & 18.9 & 614 & 6.1 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline560 & 2D-M326 & 0.0079 & 16.4 & 564 & 5.8 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline561 & 2D-M486 & 0.0079 & 16.4 & 565 & 5.8 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline562 & 2D-M398 & 0.0078 & 27.4 & 645 & 6.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{13}$ \\
\hline563 & 2D-M171 & 0.0077 & 16.1 & 559 & 4.5 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{23}$ \\
\hline564 & 2D-M391 & 0.0073 & 20.2 & 631 & 3.4 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{34}$ \\
\hline565 & 2D-M332 & 0.0066 & 19.0 & 616 & 5.5 & $f_2$ & $\dot{d}_{25},\dot{\theta}_{14}$ \\
\hline566 & 2D-M494 & 0.0062 & 21.2 & 637 & 5.1 & $f_2$ & $\dot{d}_{13},\dot{\theta}_{45}$ \\
\hline567 & 2D-M509 & 0.0057 & 19.7 & 620 & 4.8 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{45}$ \\
\hline568 & 2D-M328 & 0.0055 & 17.5 & 600 & 3.5 & $f_2$ & $\dot{d}_{23},\dot{\theta}_{14}$ \\
\hline569 & 2D-M176 & 0.0041 & 16.8 & 574 & 2.7 & $f_2$ & $\dot{d}_{14},\dot{\theta}_{25}$ \\
\hline570 & 2D-M599 & 0.0028 & 1.0 & 53 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline571 & 2D-M40 & 0.0026 & 1.7 & 304 & 1.7 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline572 & 2D-M469 & 0.0021 & 1.1 & 106 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline573 & 2D-M483 & 0.002 & 1.1 & 79 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline574 & 2D-M565 & 0.002 & 1.0 & 50 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline575 & 2D-M36 & 0.002 & 1.4 & 238 & 1.4 & $f_2$ & $\dot{d}_{14},\dot{d}_{24}$ \\
\hline576 & 2D-M560 & 0.0019 & 1.2 & 147 & 1.2 & $f_2$ & $\dot{d}_{14},\dot{d}_{24}$ \\
\hline577 & 2D-M573 & 0.0018 & 1.2 & 146 & 1.2 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline578 & 2D-M441 & 0.0017 & 1.1 & 124 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline579 & 2D-M39 & 0.0017 & 1.2 & 165 & 1.2 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline580 & 2D-M563 & 0.0017 & 1.1 & 94 & 1.1 & $f_2$ & $\dot{d}_{14},\dot{d}_{24}$ \\
\hline581 & 2D-M576 & 0.0017 & 1.1 & 85 & 1.1 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline582 & 2D-M575 & 0.0017 & 1.1 & 87 & 1.1 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline583 & 2D-M587 & 0.0017 & 1.1 & 91 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline584 & 2D-M615 & 0.0016 & 1.0 & 71 & 1.0 & $f_2$ & $\dot{d}_{24},\dot{d}_{25}$ \\
\hline585 & 2D-M588 & 0.0016 & 1.1 & 86 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline586 & 2D-M34 & 0.0016 & 1.5 & 261 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline587 & 2D-M493 & 0.0016 & 1.1 & 90 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline588 & 2D-M574 & 0.0016 & 1.0 & 12 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{34}$ \\
\hline589 & 2D-M467 & 0.0016 & 1.1 & 126 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline590 & 2D-M571 & 0.0016 & 1.0 & 2 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline591 & 2D-M592 & 0.0016 & 1.7 & 299 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{24}$ \\
\hline592 & 2D-M577 & 0.0015 & 1.2 & 138 & 0.9 & $f_2$ & $\dot{d}_{14},\dot{d}_{34}$ \\
\hline593 & 2D-M605 & 0.0015 & 1.1 & 89 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline594 & 2D-M604 & 0.0015 & 1.1 & 88 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{24}$ \\
\hline595 & 2D-M594 & 0.0015 & 1.0 & 8 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{23}$ \\
\hline596 & 2D-M598 & 0.0015 & 1.0 & 24 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline597 & 2D-M610 & 0.0015 & 1.0 & 3 & 1 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline598 & 2D-M602 & 0.0015 & 1.0 & 60 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline599 & 2D-M590 & 0.0015 & 1.0 & 59 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline600 & 2D-M586 & 0.0015 & 1.0 & 58 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline601 & 2D-M564 & 0.0015 & 1.0 & 55 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{24}$ \\
\hline602 & 2D-M603 & 0.0015 & 1.0 & 54 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{24}$ \\
\hline603 & 2D-M618 & 0.0015 & 1.0 & 29 & 1.0 & $f_2$ & $\dot{d}_{23},\dot{d}_{35}$ \\
\hline604 & 2D-M457 & 0.0015 & 1.4 & 229 & 1.1 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline605 & 2D-M585 & 0.0015 & 1.0 & 23 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline606 & 2D-M569 & 0.0015 & 1.0 & 17 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline607 & 2D-M596 & 0.0014 & 1.0 & 21 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline608 & 2D-M567 & 0.0014 & 1.0 & 19 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline609 & 2D-M570 & 0.0014 & 1.0 & 1 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline610 & 2D-M606 & 0.0014 & 1.0 & 25 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{23}$ \\
\hline611 & 2D-M595 & 0.0014 & 1.0 & 63 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{23}$ \\
\hline612 & 2D-M583 & 0.0014 & 1.0 & 65 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline613 & 2D-M562 & 0.0014 & 1.0 & 64 & 1.0 & $f_2$ & $\dot{d}_{14},\dot{d}_{24}$ \\
\hline614 & 2D-M600 & 0.0014 & 1.0 & 4 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline615 & 2D-M619 & 0.0014 & 1.4 & 235 & 1.0 & $f_2$ & $\dot{d}_{23},\dot{d}_{25}$ \\
\hline616 & 2D-M614 & 0.0014 & 1.4 & 234 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline617 & 2D-M459 & 0.0014 & 1.0 & 77 & 1.0 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline618 & 2D-M33 & 0.0013 & 1.4 & 237 & 1.1 & $f_2$ & $\dot{d}_{14},\dot{d}_{35}$ \\
\hline619 & 2D-M445 & 0.0012 & 1.1 & 110 & 0.8 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline620 & 2D-M444 & 0.0012 & 1.5 & 274 & 0.9 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline621 & 2D-M37 & 0.0012 & 1.2 & 166 & 0.8 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline622 & 2D-M38 & 0.0012 & 1.2 & 167 & 0.8 & $f_2$ & $\dot{d}_{14},\dot{d}_{34}$ \\
\hline623 & 2D-M443 & 0.0012 & 1.2 & 170 & 0.7 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline624 & 2D-M440 & 0.0012 & 2.6 & 322 & 0.9 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline625 & 2D-M593 & 0.0012 & 1.3 & 200 & 0.8 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline626 & 2D-M611 & 0.001 & 1.4 & 232 & 0.6 & $f_2$ & $\dot{d}_{13},\dot{d}_{25}$ \\
\hline627 & 2D-M481 & 0.001 & 1.0 & 69 & 0.7 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline628 & 2D-M616 & 0.001 & 1.6 & 289 & 0.6 & $f_2$ & $\dot{d}_{23},\dot{d}_{25}$ \\
\hline629 & 2D-M442 & 0.001 & 2.2 & 317 & 0.6 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline630 & 2D-M568 & 0.0009 & 1.3 & 187 & 0.6 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline631 & 2D-M582 & 0.0009 & 1.3 & 196 & 0.6 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline632 & 2D-M617 & 0.0009 & 1.3 & 188 & 0.6 & $f_2$ & $\dot{d}_{23},\dot{d}_{45}$ \\
\hline633 & 2D-M580 & 0.0009 & 1.3 & 186 & 0.6 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline634 & 2D-M561 & 0.0009 & 2.6 & 323 & 0.6 & $f_2$ & $\dot{d}_{14},\dot{d}_{24}$ \\
\hline635 & 2D-M578 & 0.0008 & 1.5 & 275 & 0.5 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline636 & 2D-M566 & 0.0008 & 1.4 & 252 & 0.5 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline637 & 2D-M608 & 0.0008 & 1.4 & 251 & 0.5 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline638 & 2D-M581 & 0.0008 & 1.3 & 210 & 0.6 & $f_2$ & $\dot{d}_{23},\dot{d}_{25}$ \\
\hline639 & 2D-M584 & 0.0007 & 1.4 & 250 & 0.5 & $f_2$ & $\dot{d}_{13},\dot{d}_{14}$ \\
\hline640 & 2D-M612 & 0.0007 & 1.4 & 245 & 0.5 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline641 & 2D-M579 & 0.0007 & 1.4 & 243 & 0.5 & $f_2$ & $\dot{d}_{14},\dot{d}_{23}$ \\
\hline642 & 2D-M591 & 0.0007 & 1.4 & 256 & 0.5 & $f_2$ & $\dot{d}_{13},\dot{d}_{24}$ \\
\hline643 & 2D-M572 & 0.0007 & 1.4 & 239 & 0.5 & $f_2$ & $\dot{d}_{14},\dot{d}_{25}$ \\
\hline644 & 2D-M491 & 0.0007 & 1.3 & 203 & 0.5 & $f_2$ & $\dot{d}_{13},\dot{d}_{45}$ \\
\hline645 & 2D-M607 & 0.0006 & 1.6 & 282 & 0.4 & $f_2$ & $\dot{d}_{13},\dot{d}_{23}$ \\
\hline
%\caption{Manipulability of 1-DOF Manipulators}
%\label{Tab:table_dof1mt_1}

\end{supertabular}
\end{center}

%\end{longtable}

\normalsize



















==> Dimensional Synthesis/contentfolder/mechanisms2/manipulabilitytable1.tex <==

\begin{center}

\tablefirsthead{%

\hline
%\multicolumn{1}{|c}{\tbsp S.No.} &
\multicolumn{1}{|c|}{\tbsp S.No.} &
%\tbsp S.No. &
%\multicolumn{1}{c}{Name} &
Name &
$\bar{\mu}$ &
%\multicolumn{1}{c}{$\mu$} &
$\mu$ &
\multicolumn{1}{c|}{$f$} \\
\hline}
\tablehead{%
\hline
%\multicolumn{5}{|l|}{\small\sl continued from previous page}\\
\multicolumn{5}{|l|}{\small\sl continuing...}\\
\hline
\multicolumn{1}{|c|}{\tbsp S.No.} &
Name &
$\bar{\mu}$ &
$\mu$ &
\multicolumn{1}{c|}{$f$} \\
\hline}
\tabletail{%
\hline
%\multicolumn{5}{|r|}{\small\sl continued on next page}\\
\multicolumn{5}{|r|}{\small\sl ...continued}\\
\hline}
\tablelasttail{\hline}
\label{Tab:table_dof1mt_1}
%\customlabel{Tab:table_dof1mt_1}{2}
\bottomcaption{Prescription of 1-DOF Manipulators}



%\tablehead{S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\}

%\begin{supertabular}{||c|c|c|c|c||}
\begin{supertabular}{|r|r|r|r|r|}
%\begin{longtable}{||c|c|c|c|c||}
%\hline
%S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\ 
\hline
1 & 1D-M10 & 0.1523 & 8.1 & $f_1$ \\
\hline2 & 1D-M65 & 0.1376 & 10.5 & $f_2$ \\
\hline3 & 1D-M8 & 0.1152 & 7.1 & $f_1$ \\
\hline4 & 1D-M94 & 0.1106 & 1.0 & $f_2$ \\
\hline5 & 1D-M28 & 0.1088 & 8.1 & $f_1$ \\
\hline6 & 1D-M20 & 0.0824 & 10.5 & $f_1$ \\
\hline7 & 1D-M34 & 0.0798 & 7.1 & $f_1$ \\
\hline8 & 1D-M95 & 0.0776 & 1.0 & $f_2$ \\
\hline9 & 1D-M7 & 0.0774 & 8.4 & $f_1$ \\
\hline10 & 1D-M29 & 0.0732 & 10.5 & $f_1$ \\
\hline11 & 1D-M41 & 0.0722 & 9.5 & $f_1$ \\
\hline12 & 1D-M40 & 0.071 & 7.1 & $f_1$ \\
\hline13 & 1D-M35 & 0.0706 & 10.5 & $f_1$ \\
\hline14 & 1D-M11 & 0.062 & 10.5 & $f_1$ \\
\hline15 & 1D-M64 & 0.0563 & 20.3 & $f_2$ \\
\hline16 & 1D-M66 & 0.0487 & 19.8 & $f_2$ \\
\hline17 & 1D-M60 & 0.0475 & 8.4 & $f_1$ \\
\hline18 & 1D-M93 & 0.0467 & 1.0 & $f_2$ \\
\hline19 & 1D-M59 & 0.0462 & 9.5 & $f_1$ \\
\hline20 & 1D-M91 & 0.0438 & 1.0 & $f_2$ \\
\hline21 & 1D-M79 & 0.0335 & 1 & $f_1$ \\
\hline22 & 1D-M25 & 0.0313 & 17.3 & $f_2$ \\
\hline23 & 1D-M44 & 0.0313 & 17.3 & $f_2$ \\
\hline24 & 1D-M67 & 0.0306 & 18.3 & $f_2$ \\
\hline25 & 1D-M15 & 0.0305 & 21.2 & $f_2$ \\
\hline26 & 1D-M22 & 0.0246 & 17.3 & $f_2$ \\
\hline27 & 1D-M13 & 0.024 & 15.3 & $f_2$ \\
\hline28 & 1D-M46 & 0.0237 & 15.3 & $f_2$ \\
\hline29 & 1D-M45 & 0.0229 & 17.3 & $f_2$ \\
\hline30 & 1D-M3 & 0.0222 & 15.4 & $f_2$ \\
\hline31 & 1D-M49 & 0.0219 & 14.1 & $f_2$ \\
\hline32 & 1D-M68 & 0.0214 & 19.6 & $f_2$ \\
\hline33 & 1D-M5 & 0.0212 & 14.7 & $f_2$ \\
\hline34 & 1D-M47 & 0.0212 & 17.3 & $f_2$ \\
\hline35 & 1D-M24 & 0.0212 & 17.3 & $f_2$ \\
\hline36 & 1D-M51 & 0.0203 & 14.9 & $f_2$ \\
\hline37 & 1D-M18 & 0.0194 & 14.6 & $f_2$ \\
\hline38 & 1D-M69 & 0.019 & 19.0 & $f_2$ \\
\hline39 & 1D-M48 & 0.0189 & 14.0 & $f_2$ \\
\hline40 & 1D-M12 & 0.0188 & 12.8 & $f_2$ \\
\hline41 & 1D-M9 & 0.0185 & 12.8 & $f_2$ \\
\hline42 & 1D-M23 & 0.0177 & 13.0 & $f_2$ \\
\hline43 & 1D-M62 & 0.0167 & 9.6 & $f_2$ \\
\hline44 & 1D-M26 & 0.0167 & 9.6 & $f_2$ \\
\hline45 & 1D-M14 & 0.0163 & 10.1 & $f_2$ \\
\hline46 & 1D-M96 & 0.016 & 1.0 & $f_2$ \\
\hline47 & 1D-M6 & 0.0159 & 12.0 & $f_2$ \\
\hline48 & 1D-M4 & 0.0158 & 13.4 & $f_2$ \\
\hline49 & 1D-M89 & 0.0155 & 1 & $f_1$ \\
\hline50 & 1D-M38 & 0.0153 & 12.9 & $f_2$ \\
\hline51 & 1D-M58 & 0.0148 & 8.2 & $f_2$ \\
\hline52 & 1D-M57 & 0.0143 & 11.7 & $f_2$ \\
\hline53 & 1D-M76 & 0.0138 & 1 & $f_1$ \\
\hline54 & 1D-M17 & 0.0136 & 8.6 & $f_2$ \\
\hline55 & 1D-M50 & 0.0135 & 11.1 & $f_2$ \\
\hline56 & 1D-M19 & 0.0134 & 10.3 & $f_2$ \\
\hline57 & 1D-M56 & 0.0129 & 10.5 & $f_2$ \\
\hline58 & 1D-M21 & 0.0128 & 10.5 & $f_2$ \\
\hline59 & 1D-M27 & 0.0127 & 9.3 & $f_2$ \\
\hline60 & 1D-M77 & 0.0126 & 1 & $f_1$ \\
\hline61 & 1D-M16 & 0.0125 & 9.3 & $f_2$ \\
\hline62 & 1D-M2 & 0.0116 & 6.7 & $f_2$ \\
\hline63 & 1D-M1 & 0.0113 & 8.4 & $f_2$ \\
\hline64 & 1D-M43 & 0.0108 & 1 & $f_1$ \\
\hline65 & 1D-M39 & 0.01 & 8.5 & $f_2$ \\
\hline66 & 1D-M80 & 0.0082 & 1 & $f_1$ \\
\hline67 & 1D-M36 & 0.0081 & 1 & $f_1$ \\
\hline68 & 1D-M92 & 0.0071 & 1 & $f_1$ \\
\hline69 & 1D-M61 & 0.0051 & 1 & $f_1$ \\
\hline70 & 1D-M42 & 0.0034 & 1 & $f_1$ \\
\hline71 & 1D-M31 & 0.0031 & 1.7 & $f_2$ \\
\hline72 & 1D-M37 & 0.0025 & 1 & $f_1$ \\
\hline73 & 1D-M86 & 0.0021 & 1.0 & $f_2$ \\
\hline74 & 1D-M30 & 0.002 & 1.1 & $f_2$ \\
\hline75 & 1D-M53 & 0.0017 & 1.1 & $f_2$ \\
\hline76 & 1D-M83 & 0.0016 & 1.0 & $f_2$ \\
\hline77 & 1D-M84 & 0.0015 & 1.0 & $f_2$ \\
\hline78 & 1D-M87 & 0.0015 & 1.0 & $f_2$ \\
\hline79 & 1D-M55 & 0.0015 & 1.3 & $f_2$ \\
\hline80 & 1D-M71 & 0.0015 & 1.0 & $f_2$ \\
\hline81 & 1D-M73 & 0.0015 & 1.0 & $f_2$ \\
\hline82 & 1D-M90 & 0.0015 & 1.0 & $f_2$ \\
\hline83 & 1D-M52 & 0.0015 & 1.1 & $f_2$ \\
\hline84 & 1D-M82 & 0.0014 & 1.0 & $f_2$ \\
\hline85 & 1D-M72 & 0.0014 & 1 & $f_2$ \\
\hline86 & 1D-M70 & 0.0014 & 1.0 & $f_2$ \\
\hline87 & 1D-M81 & 0.0014 & 1 & $f_2$ \\
\hline88 & 1D-M85 & 0.0014 & 1.0 & $f_2$ \\
\hline89 & 1D-M88 & 0.0014 & 1.0 & $f_2$ \\
\hline90 & 1D-M63 & 0.0013 & 1.1 & $f_2$ \\
\hline91 & 1D-M32 & 0.0013 & 0.7 & $f_2$ \\
\hline92 & 1D-M54 & 0.0013 & 1.1 & $f_2$ \\
\hline93 & 1D-M33 & 0.0012 & 0.8 & $f_2$ \\
\hline94 & 1D-M78 & 0.0009 & 0.6 & $f_2$ \\
\hline95 & 1D-M74 & 0.0008 & 0.6 & $f_2$ \\
\hline96 & 1D-M75 & 0.0006 & 0.4 & $f_2$ \\
\hline
%\caption{Manipulability of 1-DOF Manipulators}
%\label{Tab:table_dof1mt_1}

\end{supertabular}
\end{center}

%\end{longtable}



==> Dimensional Synthesis/contentfolder/mechanisms2/manipulabilitytable2.tex <==
\tiny
\begin{center}
%\label{Tab:table_dof2mt_1}
\tablefirsthead{%
\hline
%\multicolumn{1}{|c}{\tbsp S.No.} &
\multicolumn{1}{|c|}{\tbsp S.No.} &
%\tbsp S.No. &
%\multicolumn{1}{c}{Name} &
Name &
$\bar{\mu}$ &
$\kappa$ &
$i_{\kappa}$ &
%\multicolumn{1}{c}{$\mu$} &
$\mu$ &
\multicolumn{1}{c|}{$f$} \\
\hline}
\tablehead{%
\hline
%\multicolumn{5}{|l|}{\small\sl continued from previous page}\\
\multicolumn{7}{|l|}{\small\sl continuing...}\\
\hline
\multicolumn{1}{|c|}{\tbsp S.No.} &
Name &
$\bar{\mu}$ &
$\kappa$ &
$i_{\kappa}$ &
$\mu$ &
\multicolumn{1}{c|}{$f$} \\
\hline}
\tabletail{%
\hline
%\multicolumn{5}{|r|}{\small\sl continued on next page}\\
\multicolumn{7}{|r|}{\small\sl ...continued}\\
\hline}
\tablelasttail{\hline}
\bottomcaption{Prescription of 2-DOF Manipulators}



%\tablehead{S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\}

%\begin{supertabular}{||c|c|c|c|c||}
\begin{supertabular}{|r|r|r|r|r|r|r|}
%\begin{longtable}{||c|c|c|c|c||}
%\hline
%S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\ 
\hline

1 & 2D-M645 & 1.0 & 1.0 & 6 & 1.0 & $f_1$ \\
\hline2 & 2D-M315 & 0.7544 & 1.2 & 155 & 87.4 & $f_1$ \\
\hline3 & 2D-M301 & 0.7058 & 1.2 & 158 & 88.8 & $f_2$ \\
\hline4 & 2D-M224 & 0.6366 & 1.1 & 127 & 60.2 & $f_1$ \\
\hline5 & 2D-M308 & 0.6034 & 1.1 & 118 & 340.6 & $f_2$ \\
\hline6 & 2D-M126 & 0.5855 & 1.3 & 207 & 88.8 & $f_1$ \\
\hline7 & 2D-M309 & 0.5624 & 1.2 & 135 & 351.6 & $f_2$ \\
\hline8 & 2D-M319 & 0.5621 & 1.4 & 230 & 283.4 & $f_2$ \\
\hline9 & 2D-M208 & 0.5495 & 1.2 & 172 & 68.1 & $f_1$ \\
\hline10 & 2D-M134 & 0.541 & 1.1 & 107 & 100.5 & $f_1$ \\
\hline11 & 2D-M248 & 0.5381 & 1.4 & 224 & 75.2 & $f_1$ \\
\hline12 & 2D-M203 & 0.5289 & 1.3 & 198 & 68.1 & $f_1$ \\
\hline13 & 2D-M634 & 0.5142 & 1.0 & 7 & 1 & $f_1$ \\
\hline14 & 2D-M458 & 0.5116 & 1.0 & 32 & 1.0 & $f_1$ \\
\hline15 & 2D-M74 & 0.5114 & 1.1 & 115 & 77.5 & $f_1$ \\
\hline16 & 2D-M318 & 0.5006 & 1.1 & 130 & 298.9 & $f_2$ \\
\hline17 & 2D-M213 & 0.4948 & 1.3 & 183 & 60.2 & $f_1$ \\
\hline18 & 2D-M304 & 0.4879 & 1.8 & 307 & 165.1 & $f_2$ \\
\hline19 & 2D-M311 & 0.485 & 1.2 & 152 & 88.5 & $f_1$ \\
\hline20 & 2D-M300 & 0.4831 & 2.1 & 316 & 144.2 & $f_2$ \\
\hline21 & 2D-M314 & 0.4683 & 1.2 & 141 & 266.1 & $f_2$ \\
\hline22 & 2D-M303 & 0.4571 & 1.6 & 294 & 181.6 & $f_2$ \\
\hline23 & 2D-M305 & 0.4477 & 1.5 & 266 & 200.5 & $f_2$ \\
\hline24 & 2D-M98 & 0.4435 & 1.3 & 180 & 88.8 & $f_1$ \\
\hline25 & 2D-M302 & 0.4376 & 1.8 & 306 & 164.6 & $f_2$ \\
\hline26 & 2D-M299 & 0.4327 & 1.7 & 298 & 192.7 & $f_2$ \\
\hline27 & 2D-M86 & 0.4221 & 1.2 & 136 & 100.5 & $f_1$ \\
\hline28 & 2D-M11 & 0.4196 & 1.1 & 117 & 60.2 & $f_1$ \\
\hline29 & 2D-M313 & 0.418 & 1.1 & 108 & 232.3 & $f_2$ \\
\hline30 & 2D-M312 & 0.4138 & 1.2 & 148 & 253.8 & $f_2$ \\
\hline31 & 2D-M239 & 0.3908 & 1.1 & 104 & 80.4 & $f_1$ \\
\hline32 & 2D-M317 & 0.3621 & 1.2 & 131 & 294.7 & $f_2$ \\
\hline33 & 2D-M237 & 0.3503 & 1.1 & 114 & 100.5 & $f_1$ \\
\hline34 & 2D-M132 & 0.3441 & 1.4 & 228 & 88.8 & $f_1$ \\
\hline35 & 2D-M232 & 0.3306 & 1.2 & 157 & 88.8 & $f_1$ \\
\hline36 & 2D-M227 & 0.3291 & 1.0 & 70 & 204.1 & $f_2$ \\
\hline37 & 2D-M286 & 0.3224 & 1.1 & 122 & 194.5 & $f_2$ \\
\hline38 & 2D-M138 & 0.3142 & 1.1 & 111 & 100.5 & $f_1$ \\
\hline39 & 2D-M226 & 0.3127 & 1.5 & 269 & 176.2 & $f_2$ \\
\hline40 & 2D-M307 & 0.3125 & 1.5 & 281 & 186.7 & $f_2$ \\
\hline41 & 2D-M306 & 0.2991 & 1.5 & 259 & 212.1 & $f_2$ \\
\hline42 & 2D-M310 & 0.2946 & 1.6 & 290 & 138.7 & $f_2$ \\
\hline43 & 2D-M521 & 0.2929 & 8.9 & 334 & 8.4 & $f_1$ \\
\hline44 & 2D-M145 & 0.2902 & 1.4 & 240 & 142.5 & $f_2$ \\
\hline45 & 2D-M234 & 0.2884 & 1.1 & 120 & 162.0 & $f_2$ \\
\hline46 & 2D-M59 & 0.2879 & 1.5 & 276 & 189.0 & $f_2$ \\
\hline47 & 2D-M128 & 0.2829 & 1.2 & 133 & 60.2 & $f_1$ \\
\hline48 & 2D-M187 & 0.2736 & 1.3 & 204 & 220.1 & $f_2$ \\
\hline49 & 2D-M293 & 0.273 & 1.3 & 192 & 182.5 & $f_2$ \\
\hline50 & 2D-M118 & 0.273 & 1.3 & 191 & 182.5 & $f_2$ \\
\hline51 & 2D-M135 & 0.273 & 1.3 & 190 & 182.5 & $f_2$ \\
\hline52 & 2D-M256 & 0.2719 & 1.1 & 84 & 100.5 & $f_1$ \\
\hline53 & 2D-M184 & 0.271 & 2.0 & 314 & 164.8 & $f_2$ \\
\hline54 & 2D-M140 & 0.2705 & 1.1 & 119 & 75.9 & $f_1$ \\
\hline55 & 2D-M209 & 0.2696 & 1.4 & 223 & 165.2 & $f_2$ \\
\hline56 & 2D-M236 & 0.2691 & 1.9 & 312 & 149.1 & $f_2$ \\
\hline57 & 2D-M282 & 0.2688 & 1.7 & 300 & 167.5 & $f_2$ \\
\hline58 & 2D-M9 & 0.2678 & 1.2 & 153 & 100.5 & $f_1$ \\
\hline59 & 2D-M182 & 0.2677 & 1.2 & 171 & 168.8 & $f_2$ \\
\hline60 & 2D-M144 & 0.2665 & 1.3 & 216 & 112.8 & $f_2$ \\
\hline61 & 2D-M295 & 0.2587 & 1.2 & 174 & 119.2 & $f_2$ \\
\hline62 & 2D-M524 & 0.2581 & 9.0 & 335 & 8.4 & $f_2$ \\
\hline63 & 2D-M316 & 0.256 & 1.2 & 175 & 168.8 & $f_2$ \\
\hline64 & 2D-M285 & 0.2533 & 1.1 & 80 & 174.6 & $f_2$ \\
\hline65 & 2D-M217 & 0.2526 & 1.6 & 284 & 126.4 & $f_2$ \\
\hline66 & 2D-M116 & 0.2519 & 1.6 & 295 & 123.7 & $f_2$ \\
\hline67 & 2D-M264 & 0.2518 & 7.7 & 325 & 7.1 & $f_1$ \\
\hline68 & 2D-M152 & 0.2506 & 1.1 & 116 & 162.4 & $f_2$ \\
\hline69 & 2D-M87 & 0.2471 & 1.4 & 227 & 132.4 & $f_2$ \\
\hline70 & 2D-M522 & 0.2466 & 7.7 & 326 & 7.1 & $f_2$ \\
\hline71 & 2D-M82 & 0.2439 & 1.2 & 173 & 88.8 & $f_1$ \\
\hline72 & 2D-M88 & 0.2418 & 1.3 & 179 & 182.1 & $f_2$ \\
\hline73 & 2D-M298 & 0.2387 & 1.5 & 265 & 202.0 & $f_2$ \\
\hline74 & 2D-M526 & 0.2381 & 7.7 & 327 & 7.1 & $f_2$ \\
\hline75 & 2D-M215 & 0.2377 & 1.4 & 241 & 100.5 & $f_1$ \\
\hline76 & 2D-M143 & 0.2369 & 1.1 & 82 & 210.2 & $f_2$ \\
\hline77 & 2D-M113 & 0.2355 & 1.4 & 226 & 101.2 & $f_2$ \\
\hline78 & 2D-M61 & 0.233 & 1.8 & 305 & 113.4 & $f_2$ \\
\hline79 & 2D-M546 & 0.2319 & 7.7 & 328 & 7.1 & $f_2$ \\
\hline80 & 2D-M43 & 0.2307 & 1.4 & 246 & 135.8 & $f_2$ \\
\hline81 & 2D-M71 & 0.2305 & 2.0 & 313 & 173.2 & $f_2$ \\
\hline82 & 2D-M181 & 0.2289 & 1.3 & 219 & 142.6 & $f_2$ \\
\hline83 & 2D-M80 & 0.2278 & 1.5 & 263 & 124.4 & $f_2$ \\
\hline84 & 2D-M66 & 0.227 & 1.3 & 178 & 165.4 & $f_2$ \\
\hline85 & 2D-M527 & 0.2263 & 9.0 & 339 & 8.4 & $f_2$ \\
\hline86 & 2D-M185 & 0.2257 & 1.0 & 76 & 149.1 & $f_2$ \\
\hline87 & 2D-M63 & 0.2253 & 1.5 & 271 & 134.9 & $f_2$ \\
\hline88 & 2D-M103 & 0.2251 & 1.3 & 209 & 123.4 & $f_2$ \\
\hline89 & 2D-M251 & 0.2246 & 1.3 & 181 & 141.0 & $f_2$ \\
\hline90 & 2D-M177 & 0.2241 & 1.5 & 279 & 111.0 & $f_2$ \\
\hline91 & 2D-M555 & 0.224 & 9.0 & 340 & 8.4 & $f_2$ \\
\hline92 & 2D-M284 & 0.223 & 2.0 & 315 & 136.6 & $f_2$ \\
\hline93 & 2D-M130 & 0.2218 & 1.3 & 193 & 126.6 & $f_2$ \\
\hline94 & 2D-M212 & 0.2218 & 1.6 & 291 & 137.2 & $f_2$ \\
\hline95 & 2D-M291 & 0.2201 & 1.6 & 288 & 123.7 & $f_2$ \\
\hline96 & 2D-M223 & 0.2201 & 1.6 & 287 & 123.7 & $f_2$ \\
\hline97 & 2D-M120 & 0.2189 & 1.0 & 61 & 145.2 & $f_2$ \\
\hline98 & 2D-M639 & 0.2183 & 1.0 & 18 & 1.0 & $f_2$ \\
\hline99 & 2D-M468 & 0.2157 & 1.0 & 38 & 1.0 & $f_1$ \\
\hline100 & 2D-M235 & 0.2155 & 1.3 & 199 & 109.6 & $f_2$ \\
\hline101 & 2D-M525 & 0.2138 & 9.0 & 341 & 8.4 & $f_2$ \\
\hline102 & 2D-M188 & 0.2127 & 1.4 & 244 & 139.6 & $f_2$ \\
\hline103 & 2D-M635 & 0.2096 & 1.0 & 48 & 1.0 & $f_2$ \\
\hline104 & 2D-M631 & 0.208 & 1.0 & 11 & 1.0 & $f_2$ \\
\hline105 & 2D-M68 & 0.208 & 1.2 & 164 & 175.5 & $f_2$ \\
\hline106 & 2D-M514 & 0.2078 & 9.0 & 342 & 8.4 & $f_2$ \\
\hline107 & 2D-M146 & 0.2056 & 1.2 & 161 & 182.5 & $f_2$ \\
\hline108 & 2D-M297 & 0.204 & 1.9 & 310 & 155.9 & $f_2$ \\
\hline109 & 2D-M56 & 0.2028 & 1.1 & 95 & 159.5 & $f_2$ \\
\hline110 & 2D-M100 & 0.2023 & 1.6 & 293 & 178.8 & $f_2$ \\
\hline111 & 2D-M190 & 0.202 & 10.2 & 351 & 9.5 & $f_1$ \\
\hline112 & 2D-M137 & 0.2016 & 1.0 & 68 & 149.0 & $f_2$ \\
\hline113 & 2D-M629 & 0.2016 & 1.0 & 36 & 1.0 & $f_2$ \\
\hline114 & 2D-M180 & 0.1995 & 1.4 & 225 & 109.1 & $f_2$ \\
\hline115 & 2D-M127 & 0.1984 & 1.3 & 201 & 165.2 & $f_2$ \\
\hline116 & 2D-M512 & 0.1978 & 9.1 & 343 & 8.4 & $f_2$ \\
\hline117 & 2D-M246 & 0.1971 & 1.3 & 184 & 132.2 & $f_2$ \\
\hline118 & 2D-M76 & 0.1969 & 2.5 & 321 & 138.2 & $f_2$ \\
\hline119 & 2D-M85 & 0.1964 & 1.1 & 121 & 140.2 & $f_2$ \\
\hline120 & 2D-M121 & 0.1964 & 1.2 & 132 & 144.5 & $f_2$ \\
\hline121 & 2D-M231 & 0.195 & 1.2 & 144 & 143.0 & $f_2$ \\
\hline122 & 2D-M222 & 0.1949 & 1.4 & 242 & 107.6 & $f_2$ \\
\hline123 & 2D-M250 & 0.1936 & 1.3 & 185 & 107.3 & $f_2$ \\
\hline124 & 2D-M210 & 0.1922 & 1.1 & 105 & 135.4 & $f_2$ \\
\hline125 & 2D-M257 & 0.1919 & 1.4 & 220 & 130.8 & $f_2$ \\
\hline126 & 2D-M523 & 0.1895 & 7.8 & 329 & 7.1 & $f_2$ \\
\hline127 & 2D-M53 & 0.1889 & 1.0 & 57 & 111.8 & $f_2$ \\
\hline128 & 2D-M69 & 0.1883 & 1.3 & 212 & 147.5 & $f_2$ \\
\hline129 & 2D-M529 & 0.1881 & 11.2 & 381 & 10.5 & $f_2$ \\
\hline130 & 2D-M276 & 0.1869 & 11.2 & 382 & 10.5 & $f_1$ \\
\hline131 & 2D-M216 & 0.1861 & 1.3 & 217 & 104.7 & $f_2$ \\
\hline132 & 2D-M142 & 0.1846 & 1.2 & 169 & 149.0 & $f_2$ \\
\hline133 & 2D-M101 & 0.1844 & 1.2 & 176 & 120.0 & $f_2$ \\
\hline134 & 2D-M557 & 0.1843 & 10.2 & 352 & 9.5 & $f_2$ \\
\hline135 & 2D-M221 & 0.182 & 1.4 & 248 & 130.1 & $f_2$ \\
\hline136 & 2D-M183 & 0.1812 & 1.3 & 205 & 101.1 & $f_2$ \\
\hline137 & 2D-M141 & 0.1806 & 1.5 & 272 & 81.9 & $f_2$ \\
\hline138 & 2D-M202 & 0.1799 & 1.1 & 103 & 110.3 & $f_2$ \\
\hline139 & 2D-M102 & 0.1795 & 1.3 & 213 & 95.2 & $f_2$ \\
\hline140 & 2D-M124 & 0.176 & 1.2 & 137 & 119.2 & $f_2$ \\
\hline141 & 2D-M513 & 0.1754 & 11.2 & 383 & 10.5 & $f_2$ \\
\hline142 & 2D-M94 & 0.1753 & 1.4 & 236 & 88.8 & $f_1$ \\
\hline143 & 2D-M517 & 0.175 & 11.2 & 384 & 10.5 & $f_2$ \\
\hline144 & 2D-M99 & 0.1747 & 1.1 & 92 & 132.9 & $f_2$ \\
\hline145 & 2D-M554 & 0.1742 & 11.2 & 385 & 10.5 & $f_2$ \\
\hline146 & 2D-M519 & 0.174 & 11.2 & 386 & 10.5 & $f_2$ \\
\hline147 & 2D-M207 & 0.1733 & 1.0 & 52 & 124.9 & $f_2$ \\
\hline148 & 2D-M60 & 0.1729 & 2.4 & 319 & 130.4 & $f_2$ \\
\hline149 & 2D-M559 & 0.1727 & 11.2 & 387 & 10.5 & $f_2$ \\
\hline150 & 2D-M62 & 0.1717 & 1.1 & 112 & 120.5 & $f_2$ \\
\hline151 & 2D-M632 & 0.171 & 1.0 & 27 & 1.0 & $f_2$ \\
\hline152 & 2D-M111 & 0.1708 & 1.3 & 211 & 109.6 & $f_2$ \\
\hline153 & 2D-M545 & 0.1704 & 11.2 & 389 & 10.5 & $f_2$ \\
\hline154 & 2D-M48 & 0.17 & 1.3 & 182 & 117.5 & $f_2$ \\
\hline155 & 2D-M96 & 0.169 & 1.2 & 156 & 96.8 & $f_2$ \\
\hline156 & 2D-M186 & 0.1684 & 1.7 & 297 & 108.9 & $f_2$ \\
\hline157 & 2D-M214 & 0.1681 & 1.1 & 129 & 101.3 & $f_2$ \\
\hline158 & 2D-M110 & 0.1679 & 1.1 & 93 & 135.3 & $f_2$ \\
\hline159 & 2D-M601 & 0.1676 & 1.0 & 34 & 1.0 & $f_1$ \\
\hline160 & 2D-M46 & 0.1674 & 1.2 & 145 & 100.4 & $f_2$ \\
\hline161 & 2D-M518 & 0.1665 & 11.2 & 390 & 10.5 & $f_2$ \\
\hline162 & 2D-M122 & 0.166 & 1.2 & 142 & 104.2 & $f_2$ \\
\hline163 & 2D-M283 & 0.1653 & 1.6 & 292 & 123.1 & $f_2$ \\
\hline164 & 2D-M97 & 0.1652 & 1.5 & 280 & 112.8 & $f_2$ \\
\hline165 & 2D-M627 & 0.1651 & 1.0 & 28 & 1.0 & $f_2$ \\
\hline166 & 2D-M204 & 0.1636 & 1.4 & 253 & 92.9 & $f_2$ \\
\hline167 & 2D-M558 & 0.1626 & 11.2 & 391 & 10.5 & $f_2$ \\
\hline168 & 2D-M296 & 0.1625 & 1.2 & 134 & 119.5 & $f_2$ \\
\hline169 & 2D-M131 & 0.1618 & 1.2 & 143 & 128.4 & $f_2$ \\
\hline170 & 2D-M623 & 0.1613 & 1.0 & 14 & 1.0 & $f_2$ \\
\hline171 & 2D-M640 & 0.1608 & 1.0 & 43 & 1.0 & $f_2$ \\
\hline172 & 2D-M107 & 0.1602 & 1.1 & 83 & 120.8 & $f_2$ \\
\hline173 & 2D-M515 & 0.1581 & 11.2 & 392 & 10.5 & $f_2$ \\
\hline174 & 2D-M49 & 0.1576 & 1.1 & 109 & 91.0 & $f_2$ \\
\hline175 & 2D-M108 & 0.1576 & 1.1 & 99 & 127.9 & $f_2$ \\
\hline176 & 2D-M597 & 0.1569 & 1.0 & 41 & 1.0 & $f_1$ \\
\hline177 & 2D-M136 & 0.1553 & 1.2 & 139 & 126.7 & $f_2$ \\
\hline178 & 2D-M292 & 0.1543 & 1.2 & 163 & 124.6 & $f_2$ \\
\hline179 & 2D-M45 & 0.1538 & 1.3 & 218 & 137.5 & $f_2$ \\
\hline180 & 2D-M148 & 0.1535 & 1.0 & 56 & 91.6 & $f_2$ \\
\hline181 & 2D-M243 & 0.1534 & 11.3 & 393 & 10.5 & $f_1$ \\
\hline182 & 2D-M104 & 0.1515 & 1.1 & 102 & 121.5 & $f_2$ \\
\hline183 & 2D-M638 & 0.1508 & 1.0 & 31 & 1.0 & $f_2$ \\
\hline184 & 2D-M225 & 0.1494 & 1.1 & 81 & 109.5 & $f_2$ \\
\hline185 & 2D-M454 & 0.1488 & 10.3 & 354 & 9.5 & $f_1$ \\
\hline186 & 2D-M84 & 0.1484 & 1.6 & 283 & 114.9 & $f_2$ \\
\hline187 & 2D-M47 & 0.1467 & 1.3 & 189 & 103.7 & $f_2$ \\
\hline188 & 2D-M44 & 0.1466 & 1.4 & 247 & 121.1 & $f_2$ \\
\hline189 & 2D-M241 & 0.1455 & 1.4 & 257 & 90.4 & $f_2$ \\
\hline190 & 2D-M114 & 0.1451 & 1.1 & 98 & 116.6 & $f_2$ \\
\hline191 & 2D-M528 & 0.1447 & 11.3 & 395 & 10.5 & $f_2$ \\
\hline192 & 2D-M621 & 0.1437 & 1.0 & 30 & 1.0 & $f_2$ \\
\hline193 & 2D-M478 & 0.1431 & 10.3 & 355 & 9.5 & $f_1$ \\
\hline194 & 2D-M268 & 0.1428 & 11.3 & 396 & 10.5 & $f_1$ \\
\hline195 & 2D-M609 & 0.1385 & 1.0 & 40 & 1.0 & $f_1$ \\
\hline196 & 2D-M133 & 0.1381 & 1.5 & 277 & 94.7 & $f_2$ \\
\hline197 & 2D-M90 & 0.1378 & 1.2 & 140 & 100.2 & $f_2$ \\
\hline198 & 2D-M51 & 0.1372 & 1.4 & 254 & 104.1 & $f_2$ \\
\hline199 & 2D-M95 & 0.1364 & 1.2 & 150 & 90.2 & $f_2$ \\
\hline200 & 2D-M115 & 0.1354 & 1.1 & 128 & 91.0 & $f_2$ \\
\hline201 & 2D-M89 & 0.1353 & 1.5 & 270 & 87.1 & $f_2$ \\
\hline202 & 2D-M371 & 0.1352 & 7.7 & 324 & 6.8 & $f_1$ \\
\hline203 & 2D-M238 & 0.134 & 1.4 & 249 & 85.2 & $f_2$ \\
\hline204 & 2D-M129 & 0.1339 & 1.0 & 13 & 91.0 & $f_2$ \\
\hline205 & 2D-M81 & 0.1336 & 1.3 & 195 & 98.0 & $f_2$ \\
\hline206 & 2D-M626 & 0.133 & 1.0 & 49 & 1.0 & $f_2$ \\
\hline207 & 2D-M625 & 0.1323 & 1.0 & 20 & 1.0 & $f_2$ \\
\hline208 & 2D-M516 & 0.1323 & 10.4 & 356 & 9.5 & $f_2$ \\
\hline209 & 2D-M5 & 0.1309 & 1.3 & 206 & 100.1 & $f_2$ \\
\hline210 & 2D-M52 & 0.1305 & 1.6 & 286 & 100.4 & $f_2$ \\
\hline211 & 2D-M247 & 0.1293 & 1.6 & 285 & 88.8 & $f_2$ \\
\hline212 & 2D-M109 & 0.1284 & 1.4 & 233 & 105.7 & $f_2$ \\
\hline213 & 2D-M64 & 0.128 & 1.0 & 75 & 85.3 & $f_2$ \\
\hline214 & 2D-M83 & 0.1275 & 1.0 & 15 & 111.0 & $f_2$ \\
\hline215 & 2D-M75 & 0.1272 & 1.3 & 202 & 88.8 & $f_2$ \\
\hline216 & 2D-M447 & 0.1272 & 11.4 & 397 & 10.5 & $f_1$ \\
\hline217 & 2D-M79 & 0.1264 & 1.6 & 296 & 75.3 & $f_2$ \\
\hline218 & 2D-M245 & 0.1264 & 1.1 & 100 & 96.5 & $f_2$ \\
\hline219 & 2D-M65 & 0.1258 & 1.0 & 51 & 90.7 & $f_2$ \\
\hline220 & 2D-M8 & 0.1255 & 1.7 & 301 & 86.0 & $f_2$ \\
\hline221 & 2D-M54 & 0.125 & 1.2 & 149 & 68.0 & $f_2$ \\
\hline222 & 2D-M4 & 0.1247 & 1.9 & 311 & 62.0 & $f_2$ \\
\hline223 & 2D-M3 & 0.1245 & 1.1 & 123 & 88.7 & $f_2$ \\
\hline224 & 2D-M72 & 0.1243 & 1.2 & 168 & 74.9 & $f_2$ \\
\hline225 & 2D-M6 & 0.1242 & 1.0 & 62 & 111.1 & $f_2$ \\
\hline226 & 2D-M544 & 0.1241 & 17.5 & 604 & 17.5 & $f_2$ \\
\hline227 & 2D-M50 & 0.1236 & 1.2 & 151 & 85.4 & $f_2$ \\
\hline228 & 2D-M414 & 0.1229 & 10.4 & 359 & 9.5 & $f_1$ \\
\hline229 & 2D-M151 & 0.1218 & 1.0 & 72 & 93.3 & $f_2$ \\
\hline230 & 2D-M7 & 0.1216 & 1.4 & 222 & 100.5 & $f_2$ \\
\hline231 & 2D-M41 & 0.1211 & 1.2 & 154 & 98.8 & $f_2$ \\
\hline232 & 2D-M117 & 0.121 & 1.0 & 66 & 92.3 & $f_2$ \\
\hline233 & 2D-M150 & 0.121 & 1.0 & 67 & 92.3 & $f_2$ \\
\hline234 & 2D-M106 & 0.1209 & 1.3 & 208 & 92.2 & $f_2$ \\
\hline235 & 2D-M211 & 0.1199 & 2.2 & 318 & 87.7 & $f_2$ \\
\hline236 & 2D-M57 & 0.1189 & 1.5 & 268 & 96.6 & $f_2$ \\
\hline237 & 2D-M139 & 0.1182 & 1.3 & 177 & 69.6 & $f_2$ \\
\hline238 & 2D-M240 & 0.1178 & 1.1 & 125 & 88.9 & $f_2$ \\
\hline239 & 2D-M105 & 0.1177 & 1.2 & 162 & 89.5 & $f_2$ \\
\hline240 & 2D-M541 & 0.1172 & 9.3 & 345 & 8.4 & $f_1$ \\
\hline241 & 2D-M249 & 0.117 & 1.5 & 278 & 95.3 & $f_2$ \\
\hline242 & 2D-M78 & 0.1165 & 1.1 & 113 & 68.5 & $f_2$ \\
\hline243 & 2D-M70 & 0.1162 & 1.1 & 101 & 57.4 & $f_2$ \\
\hline244 & 2D-M530 & 0.1158 & 17.4 & 599 & 17.4 & $f_2$ \\
\hline245 & 2D-M58 & 0.1149 & 1.3 & 214 & 63.5 & $f_2$ \\
\hline246 & 2D-M93 & 0.1146 & 1.5 & 273 & 88.8 & $f_2$ \\
\hline247 & 2D-M125 & 0.1145 & 1.5 & 260 & 78.1 & $f_2$ \\
\hline248 & 2D-M10 & 0.1143 & 1.7 & 302 & 86.0 & $f_2$ \\
\hline249 & 2D-M112 & 0.1143 & 1.3 & 194 & 72.4 & $f_2$ \\
\hline250 & 2D-M15 & 0.1138 & 1.7 & 303 & 86.0 & $f_2$ \\
\hline251 & 2D-M149 & 0.1138 & 1.0 & 74 & 72.9 & $f_2$ \\
\hline252 & 2D-M147 & 0.1138 & 1.0 & 73 & 72.9 & $f_2$ \\
\hline253 & 2D-M294 & 0.1137 & 1.5 & 258 & 85.6 & $f_2$ \\
\hline254 & 2D-M178 & 0.1129 & 1.1 & 96 & 77.5 & $f_2$ \\
\hline255 & 2D-M551 & 0.1124 & 17.4 & 598 & 17.4 & $f_2$ \\
\hline256 & 2D-M123 & 0.1121 & 1.2 & 160 & 75.2 & $f_2$ \\
\hline257 & 2D-M2 & 0.1115 & 1.2 & 159 & 100.4 & $f_2$ \\
\hline258 & 2D-M119 & 0.1105 & 1.3 & 215 & 68.1 & $f_2$ \\
\hline259 & 2D-M624 & 0.1091 & 1.0 & 35 & 1.0 & $f_2$ \\
\hline260 & 2D-M290 & 0.1086 & 1.1 & 97 & 90.6 & $f_2$ \\
\hline261 & 2D-M1 & 0.106 & 1.9 & 309 & 74.0 & $f_2$ \\
\hline262 & 2D-M67 & 0.1059 & 1.5 & 264 & 79.0 & $f_2$ \\
\hline263 & 2D-M531 & 0.1058 & 17.6 & 605 & 17.5 & $f_2$ \\
\hline264 & 2D-M463 & 0.1045 & 10.5 & 360 & 9.5 & $f_1$ \\
\hline265 & 2D-M641 & 0.1036 & 1.0 & 42 & 1.0 & $f_2$ \\
\hline266 & 2D-M532 & 0.1028 & 17.4 & 597 & 17.4 & $f_2$ \\
\hline267 & 2D-M636 & 0.1026 & 1.0 & 33 & 1.0 & $f_2$ \\
\hline268 & 2D-M630 & 0.1021 & 1.0 & 45 & 1.0 & $f_2$ \\
\hline269 & 2D-M434 & 0.1012 & 10.5 & 361 & 9.5 & $f_1$ \\
\hline270 & 2D-M29 & 0.101 & 8.2 & 331 & 7.1 & $f_1$ \\
\hline271 & 2D-M637 & 0.1006 & 1.0 & 5 & 1.0 & $f_2$ \\
\hline272 & 2D-M233 & 0.099 & 2.5 & 320 & 82.4 & $f_2$ \\
\hline273 & 2D-M77 & 0.099 & 1.4 & 255 & 63.5 & $f_2$ \\
\hline274 & 2D-M55 & 0.0984 & 1.5 & 262 & 78.8 & $f_2$ \\
\hline275 & 2D-M553 & 0.097 & 16.8 & 575 & 16.5 & $f_2$ \\
\hline276 & 2D-M42 & 0.0964 & 1.4 & 221 & 60.2 & $f_2$ \\
\hline277 & 2D-M642 & 0.0962 & 1.0 & 9 & 111.0 & $f_1$ \\
\hline278 & 2D-M255 & 0.0945 & 1.8 & 308 & 76.7 & $f_2$ \\
\hline279 & 2D-M409 & 0.093 & 10.6 & 362 & 9.5 & $f_1$ \\
\hline280 & 2D-M620 & 0.0923 & 1.0 & 16 & 1.0 & $f_2$ \\
\hline281 & 2D-M452 & 0.0922 & 10.6 & 363 & 9.5 & $f_1$ \\
\hline282 & 2D-M471 & 0.091 & 11.6 & 403 & 10.5 & $f_1$ \\
\hline283 & 2D-M179 & 0.0906 & 1.0 & 78 & 62.8 & $f_2$ \\
\hline284 & 2D-M438 & 0.0901 & 9.2 & 344 & 8.1 & $f_1$ \\
\hline285 & 2D-M92 & 0.0898 & 1.5 & 267 & 62.1 & $f_2$ \\
\hline286 & 2D-M91 & 0.0896 & 1.4 & 231 & 49.5 & $f_2$ \\
\hline287 & 2D-M73 & 0.088 & 1.3 & 197 & 48.2 & $f_2$ \\
\hline288 & 2D-M622 & 0.0869 & 1.0 & 39 & 1.0 & $f_2$ \\
\hline289 & 2D-M365 & 0.0868 & 11.6 & 406 & 10.5 & $f_1$ \\
\hline290 & 2D-M482 & 0.0862 & 1.0 & 44 & 1.0 & $f_1$ \\
\hline291 & 2D-M547 & 0.0855 & 10.4 & 357 & 9.3 & $f_2$ \\
\hline292 & 2D-M426 & 0.0843 & 10.6 & 366 & 9.5 & $f_1$ \\
\hline293 & 2D-M27 & 0.0834 & 11.6 & 408 & 10.5 & $f_1$ \\
\hline294 & 2D-M538 & 0.0833 & 11.8 & 416 & 10.1 & $f_1$ \\
\hline295 & 2D-M495 & 0.0823 & 11.6 & 409 & 10.5 & $f_1$ \\
\hline296 & 2D-M536 & 0.0805 & 19.8 & 622 & 19.8 & $f_2$ \\
\hline297 & 2D-M373 & 0.0742 & 11.7 & 412 & 10.5 & $f_1$ \\
\hline298 & 2D-M280 & 0.0736 & 11.7 & 413 & 10.5 & $f_1$ \\
\hline299 & 2D-M476 & 0.073 & 11.7 & 414 & 10.5 & $f_1$ \\
\hline300 & 2D-M377 & 0.0705 & 10.8 & 369 & 9.5 & $f_1$ \\
\hline301 & 2D-M253 & 0.0693 & 11.8 & 415 & 10.5 & $f_1$ \\
\hline302 & 2D-M540 & 0.0692 & 20.2 & 629 & 20.2 & $f_2$ \\
\hline303 & 2D-M539 & 0.067 & 20.2 & 630 & 20.2 & $f_2$ \\
\hline304 & 2D-M549 & 0.0656 & 20.2 & 626 & 20.2 & $f_2$ \\
\hline305 & 2D-M552 & 0.0605 & 20.2 & 627 & 20.2 & $f_2$ \\
\hline306 & 2D-M537 & 0.0603 & 20.2 & 628 & 20.2 & $f_2$ \\
\hline307 & 2D-M533 & 0.0579 & 9.0 & 336 & 6.4 & $f_1$ \\
\hline308 & 2D-M32 & 0.0565 & 1.0 & 22 & 1.0 & $f_1$ \\
\hline309 & 2D-M633 & 0.0525 & 1.0 & 46 & 1.0 & $f_2$ \\
\hline310 & 2D-M219 & 0.0514 & 8.8 & 333 & 7.1 & $f_1$ \\
\hline311 & 2D-M422 & 0.0484 & 10.1 & 350 & 8.4 & $f_1$ \\
\hline312 & 2D-M492 & 0.0458 & 1.0 & 10 & 1 & $f_1$ \\
\hline313 & 2D-M379 & 0.0441 & 12.2 & 433 & 10.5 & $f_1$ \\
\hline314 & 2D-M487 & 0.0401 & 12.3 & 436 & 10.5 & $f_1$ \\
\hline315 & 2D-M420 & 0.0335 & 14.1 & 512 & 14.2 & $f_2$ \\
\hline316 & 2D-M589 & 0.0333 & 1.0 & 37 & 1.0 & $f_1$ \\
\hline317 & 2D-M613 & 0.0326 & 1.0 & 47 & 1.0 & $f_1$ \\
\hline318 & 2D-M498 & 0.032 & 17.2 & 580 & 17.4 & $f_2$ \\
\hline319 & 2D-M352 & 0.0318 & 17.3 & 585 & 17.3 & $f_2$ \\
\hline320 & 2D-M157 & 0.0297 & 20.8 & 636 & 20.1 & $f_2$ \\
\hline321 & 2D-M262 & 0.0296 & 11.2 & 388 & 18.1 & $f_2$ \\
\hline322 & 2D-M218 & 0.0294 & 17.0 & 579 & 16.8 & $f_2$ \\
\hline323 & 2D-M542 & 0.0293 & 16.8 & 573 & 15.8 & $f_2$ \\
\hline324 & 2D-M172 & 0.0289 & 17.5 & 601 & 15.1 & $f_2$ \\
\hline325 & 2D-M205 & 0.028 & 14.6 & 535 & 18.9 & $f_2$ \\
\hline326 & 2D-M394 & 0.0271 & 12.8 & 451 & 8.6 & $f_2$ \\
\hline327 & 2D-M520 & 0.027 & 19.4 & 618 & 18.1 & $f_2$ \\
\hline328 & 2D-M421 & 0.0268 & 17.3 & 586 & 17.3 & $f_2$ \\
\hline329 & 2D-M360 & 0.0268 & 17.3 & 582 & 17.3 & $f_2$ \\
\hline330 & 2D-M413 & 0.0267 & 13.2 & 472 & 12.9 & $f_2$ \\
\hline331 & 2D-M355 & 0.0266 & 14.1 & 523 & 14.1 & $f_2$ \\
\hline332 & 2D-M349 & 0.0263 & 14.6 & 536 & 14.5 & $f_2$ \\
\hline333 & 2D-M508 & 0.0263 & 17.6 & 606 & 16.4 & $f_2$ \\
\hline334 & 2D-M407 & 0.0261 & 14.9 & 541 & 14.9 & $f_2$ \\
\hline335 & 2D-M389 & 0.026 & 17.4 & 594 & 6.4 & $f_2$ \\
\hline336 & 2D-M424 & 0.0259 & 16.1 & 561 & 18.4 & $f_2$ \\
\hline337 & 2D-M450 & 0.0258 & 13.1 & 460 & 13.0 & $f_2$ \\
\hline338 & 2D-M534 & 0.0254 & 19.9 & 624 & 18.6 & $f_2$ \\
\hline339 & 2D-M548 & 0.0253 & 19.0 & 615 & 17.8 & $f_2$ \\
\hline340 & 2D-M387 & 0.0245 & 17.3 & 590 & 6.4 & $f_2$ \\
\hline341 & 2D-M412 & 0.0244 & 13.1 & 463 & 13.1 & $f_2$ \\
\hline342 & 2D-M543 & 0.0241 & 18.5 & 610 & 18.0 & $f_2$ \\
\hline343 & 2D-M556 & 0.024 & 20.4 & 633 & 18.6 & $f_2$ \\
\hline344 & 2D-M346 & 0.0239 & 14.8 & 538 & 12.3 & $f_2$ \\
\hline345 & 2D-M475 & 0.0238 & 17.0 & 578 & 17.5 & $f_2$ \\
\hline346 & 2D-M288 & 0.0238 & 15.0 & 543 & 14.8 & $f_2$ \\
\hline347 & 2D-M507 & 0.0235 & 17.3 & 588 & 17.3 & $f_2$ \\
\hline348 & 2D-M348 & 0.0235 & 17.3 & 587 & 17.3 & $f_2$ \\
\hline349 & 2D-M163 & 0.0234 & 13.7 & 481 & 12.6 & $f_2$ \\
\hline350 & 2D-M242 & 0.023 & 18.4 & 609 & 13.8 & $f_2$ \\
\hline351 & 2D-M550 & 0.023 & 19.1 & 617 & 17.7 & $f_2$ \\
\hline352 & 2D-M24 & 0.0228 & 14.5 & 532 & 12.1 & $f_2$ \\
\hline353 & 2D-M425 & 0.0226 & 14.1 & 522 & 14.1 & $f_2$ \\
\hline354 & 2D-M357 & 0.0223 & 17.4 & 595 & 16.9 & $f_2$ \\
\hline355 & 2D-M535 & 0.0222 & 19.8 & 623 & 18.4 & $f_2$ \\
\hline356 & 2D-M406 & 0.0222 & 13.9 & 494 & 15.1 & $f_2$ \\
\hline357 & 2D-M156 & 0.0222 & 16.8 & 572 & 13.6 & $f_2$ \\
\hline358 & 2D-M252 & 0.0219 & 20.3 & 632 & 14.3 & $f_2$ \\
\hline359 & 2D-M628 & 0.0217 & 1.0 & 26 & 1.0 & $f_2$ \\
\hline360 & 2D-M366 & 0.0215 & 13.0 & 458 & 12.9 & $f_2$ \\
\hline361 & 2D-M343 & 0.0215 & 12.1 & 429 & 7.8 & $f_2$ \\
\hline362 & 2D-M155 & 0.0215 & 16.3 & 563 & 13.9 & $f_2$ \\
\hline363 & 2D-M194 & 0.0214 & 16.3 & 562 & 13.6 & $f_2$ \\
\hline364 & 2D-M502 & 0.0214 & 17.3 & 584 & 17.3 & $f_2$ \\
\hline365 & 2D-M374 & 0.0214 & 17.3 & 583 & 17.3 & $f_2$ \\
\hline366 & 2D-M192 & 0.0213 & 16.1 & 560 & 13.2 & $f_2$ \\
\hline367 & 2D-M354 & 0.021 & 17.0 & 577 & 14.6 & $f_2$ \\
\hline368 & 2D-M168 & 0.0209 & 14.0 & 498 & 12.5 & $f_2$ \\
\hline369 & 2D-M353 & 0.0208 & 14.3 & 531 & 11.8 & $f_2$ \\
\hline370 & 2D-M465 & 0.0205 & 14.0 & 506 & 14.0 & $f_2$ \\
\hline371 & 2D-M363 & 0.0203 & 15.1 & 545 & 15.1 & $f_2$ \\
\hline372 & 2D-M160 & 0.0202 & 15.2 & 548 & 15.1 & $f_2$ \\
\hline373 & 2D-M17 & 0.0202 & 14.1 & 511 & 14.8 & $f_2$ \\
\hline374 & 2D-M484 & 0.0201 & 13.0 & 456 & 10.3 & $f_2$ \\
\hline375 & 2D-M375 & 0.0199 & 10.9 & 378 & 10.9 & $f_2$ \\
\hline376 & 2D-M415 & 0.0198 & 15.0 & 542 & 13.4 & $f_2$ \\
\hline377 & 2D-M361 & 0.0195 & 11.4 & 398 & 11.4 & $f_2$ \\
\hline378 & 2D-M411 & 0.0194 & 15.0 & 544 & 15.3 & $f_2$ \\
\hline379 & 2D-M170 & 0.0194 & 15.7 & 556 & 11.6 & $f_2$ \\
\hline380 & 2D-M164 & 0.0192 & 12.7 & 444 & 8.7 & $f_2$ \\
\hline381 & 2D-M362 & 0.0192 & 12.5 & 442 & 9.6 & $f_2$ \\
\hline382 & 2D-M230 & 0.0191 & 13.7 & 485 & 12.3 & $f_2$ \\
\hline383 & 2D-M228 & 0.0191 & 12.9 & 452 & 12.9 & $f_2$ \\
\hline384 & 2D-M16 & 0.0184 & 15.6 & 553 & 10.3 & $f_2$ \\
\hline385 & 2D-M267 & 0.0184 & 11.6 & 405 & 12.4 & $f_2$ \\
\hline386 & 2D-M376 & 0.0184 & 11.4 & 399 & 10.1 & $f_2$ \\
\hline387 & 2D-M410 & 0.0183 & 16.5 & 567 & 13.8 & $f_2$ \\
\hline388 & 2D-M193 & 0.0181 & 10.8 & 370 & 9.6 & $f_2$ \\
\hline389 & 2D-M378 & 0.0181 & 14.7 & 537 & 12.7 & $f_2$ \\
\hline390 & 2D-M278 & 0.0181 & 16.1 & 558 & 10.6 & $f_2$ \\
\hline391 & 2D-M158 & 0.0179 & 15.3 & 551 & 12.9 & $f_2$ \\
\hline392 & 2D-M456 & 0.0178 & 19.8 & 621 & 13.2 & $f_2$ \\
\hline393 & 2D-M344 & 0.0178 & 13.0 & 454 & 10.0 & $f_2$ \\
\hline394 & 2D-M175 & 0.0177 & 18.9 & 613 & 10.5 & $f_2$ \\
\hline395 & 2D-M474 & 0.0177 & 10.9 & 375 & 10.9 & $f_2$ \\
\hline396 & 2D-M430 & 0.0175 & 10.4 & 358 & 11.7 & $f_2$ \\
\hline397 & 2D-M497 & 0.0174 & 20.4 & 634 & 13.0 & $f_2$ \\
\hline398 & 2D-M28 & 0.0174 & 14.1 & 524 & 14.1 & $f_2$ \\
\hline399 & 2D-M26 & 0.0174 & 14.1 & 525 & 14.1 & $f_2$ \\
\hline400 & 2D-M372 & 0.0173 & 10.9 & 376 & 10.9 & $f_2$ \\
\hline401 & 2D-M485 & 0.0173 & 20.8 & 635 & 9.5 & $f_2$ \\
\hline402 & 2D-M460 & 0.0171 & 12.4 & 439 & 9.4 & $f_2$ \\
\hline403 & 2D-M503 & 0.017 & 15.2 & 547 & 12.3 & $f_2$ \\
\hline404 & 2D-M439 & 0.017 & 15.2 & 546 & 12.3 & $f_2$ \\
\hline405 & 2D-M489 & 0.017 & 17.8 & 608 & 10.8 & $f_2$ \\
\hline406 & 2D-M201 & 0.0169 & 14.3 & 530 & 10.4 & $f_2$ \\
\hline407 & 2D-M504 & 0.0169 & 13.0 & 457 & 11.3 & $f_2$ \\
\hline408 & 2D-M173 & 0.0169 & 15.2 & 549 & 12.4 & $f_2$ \\
\hline409 & 2D-M404 & 0.0169 & 13.5 & 475 & 10.7 & $f_2$ \\
\hline410 & 2D-M277 & 0.0168 & 12.7 & 446 & 9.3 & $f_2$ \\
\hline411 & 2D-M196 & 0.0166 & 11.8 & 419 & 13.3 & $f_2$ \\
\hline412 & 2D-M364 & 0.0166 & 12.4 & 438 & 9.3 & $f_2$ \\
\hline413 & 2D-M254 & 0.0166 & 12.2 & 430 & 10.5 & $f_2$ \\
\hline414 & 2D-M390 & 0.0166 & 17.4 & 596 & 4.1 & $f_2$ \\
\hline415 & 2D-M405 & 0.0165 & 11.6 & 404 & 10.2 & $f_2$ \\
\hline416 & 2D-M381 & 0.0163 & 14.2 & 526 & 8.2 & $f_2$ \\
\hline417 & 2D-M408 & 0.0162 & 10.3 & 353 & 10.3 & $f_2$ \\
\hline418 & 2D-M477 & 0.0161 & 10.9 & 379 & 10.9 & $f_2$ \\
\hline419 & 2D-M359 & 0.0161 & 10.9 & 377 & 10.9 & $f_2$ \\
\hline420 & 2D-M174 & 0.0161 & 13.8 & 487 & 11.2 & $f_2$ \\
\hline421 & 2D-M266 & 0.016 & 12.2 & 435 & 11.3 & $f_2$ \\
\hline422 & 2D-M263 & 0.016 & 12.5 & 441 & 10.7 & $f_2$ \\
\hline423 & 2D-M369 & 0.0159 & 9.0 & 337 & 9.0 & $f_2$ \\
\hline424 & 2D-M199 & 0.0159 & 24.4 & 641 & 9.2 & $f_2$ \\
\hline425 & 2D-M453 & 0.0159 & 11.7 & 411 & 10.9 & $f_2$ \\
\hline426 & 2D-M500 & 0.0159 & 17.5 & 603 & 10.1 & $f_2$ \\
\hline427 & 2D-M435 & 0.0158 & 12.0 & 422 & 8.7 & $f_2$ \\
\hline428 & 2D-M198 & 0.0158 & 12.7 & 445 & 11.2 & $f_2$ \\
\hline429 & 2D-M397 & 0.0156 & 14.1 & 514 & 9.3 & $f_2$ \\
\hline430 & 2D-M473 & 0.0155 & 17.5 & 602 & 9.9 & $f_2$ \\
\hline431 & 2D-M229 & 0.0155 & 12.7 & 448 & 9.5 & $f_2$ \\
\hline432 & 2D-M260 & 0.0154 & 11.8 & 420 & 8.5 & $f_2$ \\
\hline433 & 2D-M23 & 0.0154 & 9.9 & 348 & 10.3 & $f_2$ \\
\hline434 & 2D-M461 & 0.0154 & 11.9 & 421 & 9.8 & $f_2$ \\
\hline435 & 2D-M35 & 0.0153 & 11.5 & 402 & 12.9 & $f_2$ \\
\hline436 & 2D-M427 & 0.0153 & 13.4 & 473 & 10.1 & $f_2$ \\
\hline437 & 2D-M165 & 0.0153 & 11.7 & 410 & 7.8 & $f_2$ \\
\hline438 & 2D-M200 & 0.0152 & 12.8 & 449 & 10.8 & $f_2$ \\
\hline439 & 2D-M383 & 0.0152 & 11.6 & 407 & 10.5 & $f_2$ \\
\hline440 & 2D-M385 & 0.0152 & 13.0 & 455 & 8.3 & $f_2$ \\
\hline441 & 2D-M220 & 0.0151 & 11.8 & 417 & 8.6 & $f_2$ \\
\hline442 & 2D-M499 & 0.015 & 13.8 & 489 & 9.3 & $f_2$ \\
\hline443 & 2D-M153 & 0.0149 & 13.6 & 478 & 11.8 & $f_2$ \\
\hline444 & 2D-M159 & 0.0148 & 14.1 & 520 & 9.8 & $f_2$ \\
\hline445 & 2D-M340 & 0.0148 & 17.6 & 607 & 12.0 & $f_2$ \\
\hline446 & 2D-M466 & 0.0148 & 11.5 & 400 & 10.4 & $f_2$ \\
\hline447 & 2D-M419 & 0.0147 & 10.7 & 367 & 6.9 & $f_2$ \\
\hline448 & 2D-M259 & 0.0146 & 12.2 & 431 & 8.9 & $f_2$ \\
\hline449 & 2D-M273 & 0.0146 & 12.8 & 450 & 9.7 & $f_2$ \\
\hline450 & 2D-M244 & 0.0146 & 13.7 & 482 & 10.5 & $f_2$ \\
\hline451 & 2D-M451 & 0.0145 & 12.9 & 453 & 6.4 & $f_2$ \\
\hline452 & 2D-M31 & 0.0145 & 8.2 & 330 & 8.2 & $f_2$ \\
\hline453 & 2D-M289 & 0.0145 & 11.5 & 401 & 8.6 & $f_2$ \\
\hline454 & 2D-M279 & 0.0144 & 12.5 & 440 & 8.7 & $f_2$ \\
\hline455 & 2D-M417 & 0.0143 & 13.1 & 465 & 11.3 & $f_2$ \\
\hline456 & 2D-M386 & 0.0143 & 17.3 & 589 & 5.3 & $f_2$ \\
\hline457 & 2D-M342 & 0.0142 & 17.4 & 593 & 5.2 & $f_2$ \\
\hline458 & 2D-M488 & 0.0141 & 13.1 & 461 & 11.3 & $f_2$ \\
\hline459 & 2D-M167 & 0.014 & 10.6 & 365 & 7.0 & $f_2$ \\
\hline460 & 2D-M501 & 0.0139 & 14.0 & 501 & 10.6 & $f_2$ \\
\hline461 & 2D-M368 & 0.0139 & 14.0 & 502 & 10.6 & $f_2$ \\
\hline462 & 2D-M480 & 0.0139 & 16.4 & 566 & 10.3 & $f_2$ \\
\hline463 & 2D-M258 & 0.0139 & 9.8 & 346 & 6.8 & $f_2$ \\
\hline464 & 2D-M392 & 0.0139 & 18.5 & 612 & 4.9 & $f_2$ \\
\hline465 & 2D-M189 & 0.0139 & 13.8 & 491 & 10.4 & $f_2$ \\
\hline466 & 2D-M154 & 0.0138 & 13.6 & 479 & 10.3 & $f_2$ \\
\hline467 & 2D-M261 & 0.0138 & 14.0 & 507 & 10.6 & $f_2$ \\
\hline468 & 2D-M510 & 0.0138 & 9.9 & 347 & 7.1 & $f_2$ \\
\hline469 & 2D-M399 & 0.0138 & 16.6 & 568 & 11.0 & $f_2$ \\
\hline470 & 2D-M14 & 0.0138 & 10.8 & 371 & 6.9 & $f_2$ \\
\hline471 & 2D-M324 & 0.0137 & 13.8 & 488 & 10.6 & $f_2$ \\
\hline472 & 2D-M382 & 0.0137 & 19.9 & 625 & 5.8 & $f_2$ \\
\hline473 & 2D-M271 & 0.0136 & 13.9 & 496 & 10.5 & $f_2$ \\
\hline474 & 2D-M403 & 0.0136 & 11.1 & 380 & 7.1 & $f_2$ \\
\hline475 & 2D-M333 & 0.0136 & 13.9 & 497 & 10.5 & $f_2$ \\
\hline476 & 2D-M12 & 0.0136 & 12.2 & 434 & 8.9 & $f_2$ \\
\hline477 & 2D-M356 & 0.0136 & 10.8 & 372 & 7.2 & $f_2$ \\
\hline478 & 2D-M331 & 0.0132 & 13.1 & 459 & 9.5 & $f_2$ \\
\hline479 & 2D-M269 & 0.0132 & 13.5 & 476 & 10.8 & $f_2$ \\
\hline480 & 2D-M281 & 0.0132 & 10.0 & 349 & 7.0 & $f_2$ \\
\hline481 & 2D-M351 & 0.0132 & 14.2 & 528 & 10.8 & $f_2$ \\
\hline482 & 2D-M431 & 0.0132 & 14.2 & 527 & 10.8 & $f_2$ \\
\hline483 & 2D-M337 & 0.0132 & 12.0 & 424 & 8.4 & $f_2$ \\
\hline484 & 2D-M166 & 0.0132 & 14.0 & 499 & 9.4 & $f_2$ \\
\hline485 & 2D-M265 & 0.0131 & 14.0 & 500 & 10.5 & $f_2$ \\
\hline486 & 2D-M393 & 0.0131 & 18.5 & 611 & 4.9 & $f_2$ \\
\hline487 & 2D-M462 & 0.0131 & 14.0 & 503 & 10.5 & $f_2$ \\
\hline488 & 2D-M436 & 0.0131 & 14.0 & 504 & 10.5 & $f_2$ \\
\hline489 & 2D-M334 & 0.0131 & 14.0 & 505 & 10.5 & $f_2$ \\
\hline490 & 2D-M329 & 0.013 & 12.0 & 425 & 8.4 & $f_2$ \\
\hline491 & 2D-M384 & 0.013 & 21.4 & 639 & 10.5 & $f_2$ \\
\hline492 & 2D-M395 & 0.013 & 21.3 & 638 & 10.5 & $f_2$ \\
\hline493 & 2D-M396 & 0.013 & 19.7 & 619 & 7.1 & $f_2$ \\
\hline494 & 2D-M162 & 0.013 & 10.8 & 368 & 7.1 & $f_2$ \\
\hline495 & 2D-M206 & 0.013 & 10.9 & 374 & 8.2 & $f_2$ \\
\hline496 & 2D-M274 & 0.013 & 12.0 & 423 & 8.5 & $f_2$ \\
\hline497 & 2D-M511 & 0.013 & 13.9 & 495 & 10.6 & $f_2$ \\
\hline498 & 2D-M418 & 0.0129 & 14.0 & 508 & 10.5 & $f_2$ \\
\hline499 & 2D-M350 & 0.0129 & 14.1 & 510 & 10.5 & $f_2$ \\
\hline500 & 2D-M370 & 0.0129 & 13.1 & 464 & 9.5 & $f_2$ \\
\hline501 & 2D-M339 & 0.0129 & 11.3 & 394 & 7.1 & $f_2$ \\
\hline502 & 2D-M347 & 0.0129 & 14.0 & 509 & 10.5 & $f_2$ \\
\hline503 & 2D-M479 & 0.0129 & 13.8 & 492 & 10.3 & $f_2$ \\
\hline504 & 2D-M287 & 0.0129 & 14.3 & 529 & 8.8 & $f_2$ \\
\hline505 & 2D-M19 & 0.0129 & 10.8 & 373 & 7.1 & $f_2$ \\
\hline506 & 2D-M470 & 0.0128 & 13.1 & 466 & 9.5 & $f_2$ \\
\hline507 & 2D-M506 & 0.0128 & 11.8 & 418 & 8.1 & $f_2$ \\
\hline508 & 2D-M437 & 0.0128 & 12.1 & 426 & 8.4 & $f_2$ \\
\hline509 & 2D-M401 & 0.0128 & 13.1 & 468 & 9.5 & $f_2$ \\
\hline510 & 2D-M338 & 0.0128 & 17.3 & 581 & 9.5 & $f_2$ \\
\hline511 & 2D-M464 & 0.0127 & 14.1 & 513 & 10.5 & $f_2$ \\
\hline512 & 2D-M433 & 0.0127 & 13.1 & 469 & 9.5 & $f_2$ \\
\hline513 & 2D-M423 & 0.0127 & 13.8 & 490 & 10.2 & $f_2$ \\
\hline514 & 2D-M472 & 0.0127 & 13.1 & 462 & 9.6 & $f_2$ \\
\hline515 & 2D-M336 & 0.0127 & 14.1 & 515 & 10.5 & $f_2$ \\
\hline516 & 2D-M321 & 0.0126 & 12.1 & 427 & 8.4 & $f_2$ \\
\hline517 & 2D-M380 & 0.0126 & 15.7 & 557 & 10.2 & $f_2$ \\
\hline518 & 2D-M335 & 0.0126 & 14.1 & 516 & 10.5 & $f_2$ \\
\hline519 & 2D-M21 & 0.0126 & 12.1 & 428 & 8.4 & $f_2$ \\
\hline520 & 2D-M345 & 0.0126 & 13.2 & 470 & 9.5 & $f_2$ \\
\hline521 & 2D-M367 & 0.0126 & 14.1 & 517 & 10.5 & $f_2$ \\
\hline522 & 2D-M25 & 0.0126 & 13.2 & 471 & 9.5 & $f_2$ \\
\hline523 & 2D-M320 & 0.0126 & 14.1 & 518 & 10.5 & $f_2$ \\
\hline524 & 2D-M30 & 0.0125 & 14.1 & 519 & 10.5 & $f_2$ \\
\hline525 & 2D-M323 & 0.0125 & 12.7 & 447 & 7.5 & $f_2$ \\
\hline526 & 2D-M428 & 0.0123 & 16.8 & 576 & 10.1 & $f_2$ \\
\hline527 & 2D-M496 & 0.0121 & 14.1 & 521 & 9.9 & $f_2$ \\
\hline528 & 2D-M455 & 0.0121 & 12.6 & 443 & 8.1 & $f_2$ \\
\hline529 & 2D-M330 & 0.0121 & 13.7 & 483 & 9.2 & $f_2$ \\
\hline530 & 2D-M449 & 0.0121 & 9.0 & 338 & 5.1 & $f_2$ \\
\hline531 & 2D-M169 & 0.012 & 10.6 & 364 & 8.1 & $f_2$ \\
\hline532 & 2D-M161 & 0.012 & 15.3 & 550 & 10.1 & $f_2$ \\
\hline533 & 2D-M402 & 0.0119 & 13.7 & 486 & 8.8 & $f_2$ \\
\hline534 & 2D-M446 & 0.0119 & 15.6 & 554 & 9.5 & $f_2$ \\
\hline535 & 2D-M429 & 0.0119 & 13.8 & 493 & 8.5 & $f_2$ \\
\hline536 & 2D-M358 & 0.0117 & 13.5 & 474 & 9.6 & $f_2$ \\
\hline537 & 2D-M275 & 0.0117 & 13.7 & 484 & 7.0 & $f_2$ \\
\hline538 & 2D-M272 & 0.0117 & 13.1 & 467 & 9.2 & $f_2$ \\
\hline539 & 2D-M327 & 0.0116 & 14.6 & 534 & 9.4 & $f_2$ \\
\hline540 & 2D-M322 & 0.0116 & 14.6 & 533 & 9.5 & $f_2$ \\
\hline541 & 2D-M490 & 0.0115 & 24.5 & 642 & 8.4 & $f_2$ \\
\hline542 & 2D-M505 & 0.0114 & 24.4 & 640 & 8.4 & $f_2$ \\
\hline543 & 2D-M13 & 0.0113 & 13.5 & 477 & 9.3 & $f_2$ \\
\hline544 & 2D-M18 & 0.0112 & 12.3 & 437 & 8.4 & $f_2$ \\
\hline545 & 2D-M432 & 0.0111 & 15.6 & 555 & 7.4 & $f_2$ \\
\hline546 & 2D-M341 & 0.011 & 17.3 & 592 & 2.9 & $f_2$ \\
\hline547 & 2D-M400 & 0.0109 & 26.1 & 644 & 7.8 & $f_2$ \\
\hline548 & 2D-M191 & 0.0108 & 15.3 & 552 & 8.0 & $f_2$ \\
\hline549 & 2D-M20 & 0.0107 & 8.7 & 332 & 6.6 & $f_2$ \\
\hline550 & 2D-M388 & 0.0107 & 17.3 & 591 & 2.9 & $f_2$ \\
\hline551 & 2D-M448 & 0.0105 & 12.2 & 432 & 5.8 & $f_2$ \\
\hline552 & 2D-M325 & 0.0104 & 16.7 & 571 & 8.1 & $f_2$ \\
\hline553 & 2D-M270 & 0.0098 & 16.7 & 570 & 6.6 & $f_2$ \\
\hline554 & 2D-M643 & 0.0091 & 14.8 & 539 & 10.5 & $f_1$ \\
\hline555 & 2D-M644 & 0.0091 & 14.8 & 540 & 10.5 & $f_1$ \\
\hline556 & 2D-M416 & 0.0088 & 25.6 & 643 & 7.1 & $f_2$ \\
\hline557 & 2D-M195 & 0.0085 & 16.7 & 569 & 4.9 & $f_2$ \\
\hline558 & 2D-M197 & 0.0084 & 13.6 & 480 & 4.5 & $f_2$ \\
\hline559 & 2D-M22 & 0.0082 & 18.9 & 614 & 6.1 & $f_2$ \\
\hline560 & 2D-M326 & 0.0079 & 16.4 & 564 & 5.8 & $f_2$ \\
\hline561 & 2D-M486 & 0.0079 & 16.4 & 565 & 5.8 & $f_2$ \\
\hline562 & 2D-M398 & 0.0078 & 27.4 & 645 & 6.4 & $f_2$ \\
\hline563 & 2D-M171 & 0.0077 & 16.1 & 559 & 4.5 & $f_2$ \\
\hline564 & 2D-M391 & 0.0073 & 20.2 & 631 & 3.4 & $f_2$ \\
\hline565 & 2D-M332 & 0.0066 & 19.0 & 616 & 5.5 & $f_2$ \\
\hline566 & 2D-M494 & 0.0062 & 21.2 & 637 & 5.1 & $f_2$ \\
\hline567 & 2D-M509 & 0.0057 & 19.7 & 620 & 4.8 & $f_2$ \\
\hline568 & 2D-M328 & 0.0055 & 17.5 & 600 & 3.5 & $f_2$ \\
\hline569 & 2D-M176 & 0.0041 & 16.8 & 574 & 2.7 & $f_2$ \\
\hline570 & 2D-M599 & 0.0028 & 1.0 & 53 & 1.0 & $f_2$ \\
\hline571 & 2D-M40 & 0.0026 & 1.7 & 304 & 1.7 & $f_2$ \\
\hline572 & 2D-M469 & 0.0021 & 1.1 & 106 & 1.1 & $f_2$ \\
\hline573 & 2D-M483 & 0.002 & 1.1 & 79 & 1.0 & $f_2$ \\
\hline574 & 2D-M565 & 0.002 & 1.0 & 50 & 1.0 & $f_2$ \\
\hline575 & 2D-M36 & 0.002 & 1.4 & 238 & 1.4 & $f_2$ \\
\hline576 & 2D-M560 & 0.0019 & 1.2 & 147 & 1.2 & $f_2$ \\
\hline577 & 2D-M573 & 0.0018 & 1.2 & 146 & 1.2 & $f_2$ \\
\hline578 & 2D-M441 & 0.0017 & 1.1 & 124 & 1.1 & $f_2$ \\
\hline579 & 2D-M39 & 0.0017 & 1.2 & 165 & 1.2 & $f_2$ \\
\hline580 & 2D-M563 & 0.0017 & 1.1 & 94 & 1.1 & $f_2$ \\
\hline581 & 2D-M576 & 0.0017 & 1.1 & 85 & 1.1 & $f_2$ \\
\hline582 & 2D-M575 & 0.0017 & 1.1 & 87 & 1.1 & $f_2$ \\
\hline583 & 2D-M587 & 0.0017 & 1.1 & 91 & 1.1 & $f_2$ \\
\hline584 & 2D-M615 & 0.0016 & 1.0 & 71 & 1.0 & $f_2$ \\
\hline585 & 2D-M588 & 0.0016 & 1.1 & 86 & 1.1 & $f_2$ \\
\hline586 & 2D-M34 & 0.0016 & 1.5 & 261 & 1.0 & $f_2$ \\
\hline587 & 2D-M493 & 0.0016 & 1.1 & 90 & 1.1 & $f_2$ \\
\hline588 & 2D-M574 & 0.0016 & 1.0 & 12 & 1.0 & $f_2$ \\
\hline589 & 2D-M467 & 0.0016 & 1.1 & 126 & 1.1 & $f_2$ \\
\hline590 & 2D-M571 & 0.0016 & 1.0 & 2 & 1.0 & $f_2$ \\
\hline591 & 2D-M592 & 0.0016 & 1.7 & 299 & 1.0 & $f_2$ \\
\hline592 & 2D-M577 & 0.0015 & 1.2 & 138 & 0.9 & $f_2$ \\
\hline593 & 2D-M605 & 0.0015 & 1.1 & 89 & 1.1 & $f_2$ \\
\hline594 & 2D-M604 & 0.0015 & 1.1 & 88 & 1.1 & $f_2$ \\
\hline595 & 2D-M594 & 0.0015 & 1.0 & 8 & 1.0 & $f_2$ \\
\hline596 & 2D-M598 & 0.0015 & 1.0 & 24 & 1.0 & $f_2$ \\
\hline597 & 2D-M610 & 0.0015 & 1.0 & 3 & 1 & $f_2$ \\
\hline598 & 2D-M602 & 0.0015 & 1.0 & 60 & 1.0 & $f_2$ \\
\hline599 & 2D-M590 & 0.0015 & 1.0 & 59 & 1.0 & $f_2$ \\
\hline600 & 2D-M586 & 0.0015 & 1.0 & 58 & 1.0 & $f_2$ \\
\hline601 & 2D-M564 & 0.0015 & 1.0 & 55 & 1.0 & $f_2$ \\
\hline602 & 2D-M603 & 0.0015 & 1.0 & 54 & 1.0 & $f_2$ \\
\hline603 & 2D-M618 & 0.0015 & 1.0 & 29 & 1.0 & $f_2$ \\
\hline604 & 2D-M457 & 0.0015 & 1.4 & 229 & 1.1 & $f_2$ \\
\hline605 & 2D-M585 & 0.0015 & 1.0 & 23 & 1.0 & $f_2$ \\
\hline606 & 2D-M569 & 0.0015 & 1.0 & 17 & 1.0 & $f_2$ \\
\hline607 & 2D-M596 & 0.0014 & 1.0 & 21 & 1.0 & $f_2$ \\
\hline608 & 2D-M567 & 0.0014 & 1.0 & 19 & 1.0 & $f_2$ \\
\hline609 & 2D-M570 & 0.0014 & 1.0 & 1 & 1.0 & $f_2$ \\
\hline610 & 2D-M606 & 0.0014 & 1.0 & 25 & 1.0 & $f_2$ \\
\hline611 & 2D-M595 & 0.0014 & 1.0 & 63 & 1.0 & $f_2$ \\
\hline612 & 2D-M583 & 0.0014 & 1.0 & 65 & 1.0 & $f_2$ \\
\hline613 & 2D-M562 & 0.0014 & 1.0 & 64 & 1.0 & $f_2$ \\
\hline614 & 2D-M600 & 0.0014 & 1.0 & 4 & 1.0 & $f_2$ \\
\hline615 & 2D-M619 & 0.0014 & 1.4 & 235 & 1.0 & $f_2$ \\
\hline616 & 2D-M614 & 0.0014 & 1.4 & 234 & 1.0 & $f_2$ \\
\hline617 & 2D-M459 & 0.0014 & 1.0 & 77 & 1.0 & $f_2$ \\
\hline618 & 2D-M33 & 0.0013 & 1.4 & 237 & 1.1 & $f_2$ \\
\hline619 & 2D-M445 & 0.0012 & 1.1 & 110 & 0.8 & $f_2$ \\
\hline620 & 2D-M444 & 0.0012 & 1.5 & 274 & 0.9 & $f_2$ \\
\hline621 & 2D-M37 & 0.0012 & 1.2 & 166 & 0.8 & $f_2$ \\
\hline622 & 2D-M38 & 0.0012 & 1.2 & 167 & 0.8 & $f_2$ \\
\hline623 & 2D-M443 & 0.0012 & 1.2 & 170 & 0.7 & $f_2$ \\
\hline624 & 2D-M440 & 0.0012 & 2.6 & 322 & 0.9 & $f_2$ \\
\hline625 & 2D-M593 & 0.0012 & 1.3 & 200 & 0.8 & $f_2$ \\
\hline626 & 2D-M611 & 0.001 & 1.4 & 232 & 0.6 & $f_2$ \\
\hline627 & 2D-M481 & 0.001 & 1.0 & 69 & 0.7 & $f_2$ \\
\hline628 & 2D-M616 & 0.001 & 1.6 & 289 & 0.6 & $f_2$ \\
\hline629 & 2D-M442 & 0.001 & 2.2 & 317 & 0.6 & $f_2$ \\
\hline630 & 2D-M568 & 0.0009 & 1.3 & 187 & 0.6 & $f_2$ \\
\hline631 & 2D-M582 & 0.0009 & 1.3 & 196 & 0.6 & $f_2$ \\
\hline632 & 2D-M617 & 0.0009 & 1.3 & 188 & 0.6 & $f_2$ \\
\hline633 & 2D-M580 & 0.0009 & 1.3 & 186 & 0.6 & $f_2$ \\
\hline634 & 2D-M561 & 0.0009 & 2.6 & 323 & 0.6 & $f_2$ \\
\hline635 & 2D-M578 & 0.0008 & 1.5 & 275 & 0.5 & $f_2$ \\
\hline636 & 2D-M566 & 0.0008 & 1.4 & 252 & 0.5 & $f_2$ \\
\hline637 & 2D-M608 & 0.0008 & 1.4 & 251 & 0.5 & $f_2$ \\
\hline638 & 2D-M581 & 0.0008 & 1.3 & 210 & 0.6 & $f_2$ \\
\hline639 & 2D-M584 & 0.0007 & 1.4 & 250 & 0.5 & $f_2$ \\
\hline640 & 2D-M612 & 0.0007 & 1.4 & 245 & 0.5 & $f_2$ \\
\hline641 & 2D-M579 & 0.0007 & 1.4 & 243 & 0.5 & $f_2$ \\
\hline642 & 2D-M591 & 0.0007 & 1.4 & 256 & 0.5 & $f_2$ \\
\hline643 & 2D-M572 & 0.0007 & 1.4 & 239 & 0.5 & $f_2$ \\
\hline644 & 2D-M491 & 0.0007 & 1.3 & 203 & 0.5 & $f_2$ \\
\hline645 & 2D-M607 & 0.0006 & 1.6 & 282 & 0.4 & $f_2$ \\
\hline
%\caption{Manipulability of 1-DOF Manipulators}
%\label{Tab:table_dof1mt_1}

\end{supertabular}
\end{center}

%\end{longtable}

\normalsize

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulabilitytable3.tex <==
\begin{table}[h]  \centering \begin{tabular}{||c|c|c|c|c|c|c||}
\hline
S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ \\ 
\hline
1 & 3D-M1 & 1.0113 & 1.5 & 2 & 1058.9 & $f_1$ \\
\hline2 & 3D-M8 & 1.0 & 1.0 & 1 & 1.0 & $f_1$ \\
\hline3 & 3D-M2 & 0.0962 & 14.8 & 4 & 111.0 & $f_1$ \\
\hline4 & 3D-M3 & 0.0962 & 15.5 & 8 & 111.0 & $f_1$ \\
\hline5 & 3D-M4 & 0.0962 & 14.8 & 7 & 111.0 & $f_1$ \\
\hline6 & 3D-M7 & 0.0091 & 14.8 & 5 & 10.5 & $f_1$ \\
\hline7 & 3D-M5 & 0.0091 & 14.8 & 6 & 10.5 & $f_1$ \\
\hline8 & 3D-M6 & 0.0091 & 14.8 & 3 & 10.5 & $f_1$ \\
\hline\end{tabular} \caption{Prescription of 3-DOF Manipulators} \label{Tab:table_dof3mt_1} \end{table}

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulabilitytable4.tex <==
\begin{table}[h]  \centering \begin{tabular}{||c|c|c|c|c|c|c||}
\hline
S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ \\ 
\hline
1 & 4D-M1 & 2.5607 & 1.5 & 1 & 2074.5 & $f_1$ \\
\hline2 & 4D-M13 & 0.4866 & 3.0 & 2 & 1.0 & $f_1$ \\
\hline3 & 4D-M12 & 0.4048 & 3.1 & 3 & 1 & $f_1$ \\
\hline4 & 4D-M4 & 0.2619 & 15.3 & 14 & 211.0 & $f_1$ \\
\hline5 & 4D-M5 & 0.2619 & 15.3 & 13 & 211.0 & $f_1$ \\
\hline6 & 4D-M2 & 0.2619 & 15.3 & 12 & 211.0 & $f_1$ \\
\hline7 & 4D-M3 & 0.2619 & 15.3 & 15 & 211.0 & $f_1$ \\
\hline8 & 4D-M15 & 0.077 & 4.9 & 4 & 1.0 & $f_1$ \\
\hline9 & 4D-M14 & 0.0538 & 5.5 & 5 & 1.0 & $f_1$ \\
\hline10 & 4D-M9 & 0.0253 & 12.9 & 7 & 17.6 & $f_1$ \\
\hline11 & 4D-M11 & 0.0253 & 12.9 & 10 & 17.6 & $f_1$ \\
\hline12 & 4D-M10 & 0.0253 & 12.9 & 6 & 17.6 & $f_1$ \\
\hline13 & 4D-M7 & 0.0253 & 12.9 & 8 & 17.6 & $f_1$ \\
\hline14 & 4D-M8 & 0.0253 & 12.9 & 9 & 17.6 & $f_1$ \\
\hline15 & 4D-M6 & 0.0253 & 12.9 & 11 & 17.6 & $f_1$ \\
\hline\end{tabular} \caption{Prescription of 4-DOF Manipulators} \label{Tab:table_dof4mt_1} \end{table}

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulabilitytable_new1.tex <==
\begin{longtable}{||c|c|c|c|c||c|c|c|c|c||}
\hline
S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ & S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\ 
\hline
1 & 1D-M10 & 0.1523 & 8.1 & $f_1$ & 49 & 1D-M89 & 0.0155 & 1 & $f_1$ \\
\hline2 & 1D-M65 & 0.1376 & 10.5 & $f_2$ & 50 & 1D-M38 & 0.0153 & 12.9 & $f_2$ \\
\hline3 & 1D-M8 & 0.1152 & 7.1 & $f_1$ & 51 & 1D-M58 & 0.0148 & 8.2 & $f_2$ \\
\hline4 & 1D-M94 & 0.1106 & 1.0 & $f_2$ & 52 & 1D-M57 & 0.0143 & 11.7 & $f_2$ \\
\hline5 & 1D-M28 & 0.1088 & 8.1 & $f_1$ & 53 & 1D-M76 & 0.0138 & 1 & $f_1$ \\
\hline6 & 1D-M20 & 0.0824 & 10.5 & $f_1$ & 54 & 1D-M17 & 0.0136 & 8.6 & $f_2$ \\
\hline7 & 1D-M34 & 0.0798 & 7.1 & $f_1$ & 55 & 1D-M50 & 0.0135 & 11.1 & $f_2$ \\
\hline8 & 1D-M95 & 0.0776 & 1.0 & $f_2$ & 56 & 1D-M19 & 0.0134 & 10.3 & $f_2$ \\
\hline9 & 1D-M7 & 0.0774 & 8.4 & $f_1$ & 57 & 1D-M56 & 0.0129 & 10.5 & $f_2$ \\
\hline10 & 1D-M29 & 0.0732 & 10.5 & $f_1$ & 58 & 1D-M21 & 0.0128 & 10.5 & $f_2$ \\
\hline11 & 1D-M41 & 0.0722 & 9.5 & $f_1$ & 59 & 1D-M27 & 0.0127 & 9.3 & $f_2$ \\
\hline12 & 1D-M40 & 0.071 & 7.1 & $f_1$ & 60 & 1D-M77 & 0.0126 & 1 & $f_1$ \\
\hline13 & 1D-M35 & 0.0706 & 10.5 & $f_1$ & 61 & 1D-M16 & 0.0125 & 9.3 & $f_2$ \\
\hline14 & 1D-M11 & 0.062 & 10.5 & $f_1$ & 62 & 1D-M2 & 0.0116 & 6.7 & $f_2$ \\
\hline15 & 1D-M64 & 0.0563 & 20.3 & $f_2$ & 63 & 1D-M1 & 0.0113 & 8.4 & $f_2$ \\
\hline16 & 1D-M66 & 0.0487 & 19.8 & $f_2$ & 64 & 1D-M43 & 0.0108 & 1 & $f_1$ \\
\hline17 & 1D-M60 & 0.0475 & 8.4 & $f_1$ & 65 & 1D-M39 & 0.01 & 8.5 & $f_2$ \\
\hline18 & 1D-M93 & 0.0467 & 1.0 & $f_2$ & 66 & 1D-M80 & 0.0082 & 1 & $f_1$ \\
\hline19 & 1D-M59 & 0.0462 & 9.5 & $f_1$ & 67 & 1D-M36 & 0.0081 & 1 & $f_1$ \\
\hline20 & 1D-M91 & 0.0438 & 1.0 & $f_2$ & 68 & 1D-M92 & 0.0071 & 1 & $f_1$ \\
\hline21 & 1D-M79 & 0.0335 & 1 & $f_1$ & 69 & 1D-M61 & 0.0051 & 1 & $f_1$ \\
\hline22 & 1D-M25 & 0.0313 & 17.3 & $f_2$ & 70 & 1D-M42 & 0.0034 & 1 & $f_1$ \\
\hline23 & 1D-M44 & 0.0313 & 17.3 & $f_2$ & 71 & 1D-M31 & 0.0031 & 1.7 & $f_2$ \\
\hline24 & 1D-M67 & 0.0306 & 18.3 & $f_2$ & 72 & 1D-M37 & 0.0025 & 1 & $f_1$ \\
\hline25 & 1D-M15 & 0.0305 & 21.2 & $f_2$ & 73 & 1D-M86 & 0.0021 & 1.0 & $f_2$ \\
\hline26 & 1D-M22 & 0.0246 & 17.3 & $f_2$ & 74 & 1D-M30 & 0.002 & 1.1 & $f_2$ \\
\hline27 & 1D-M13 & 0.024 & 15.3 & $f_2$ & 75 & 1D-M53 & 0.0017 & 1.1 & $f_2$ \\
\hline28 & 1D-M46 & 0.0237 & 15.3 & $f_2$ & 76 & 1D-M83 & 0.0016 & 1.0 & $f_2$ \\
\hline29 & 1D-M45 & 0.0229 & 17.3 & $f_2$ & 77 & 1D-M84 & 0.0015 & 1.0 & $f_2$ \\
\hline30 & 1D-M3 & 0.0222 & 15.4 & $f_2$ & 78 & 1D-M87 & 0.0015 & 1.0 & $f_2$ \\
\hline31 & 1D-M49 & 0.0219 & 14.1 & $f_2$ & 79 & 1D-M55 & 0.0015 & 1.3 & $f_2$ \\
\hline32 & 1D-M68 & 0.0214 & 19.6 & $f_2$ & 80 & 1D-M71 & 0.0015 & 1.0 & $f_2$ \\
\hline33 & 1D-M5 & 0.0212 & 14.7 & $f_2$ & 81 & 1D-M73 & 0.0015 & 1.0 & $f_2$ \\
\hline34 & 1D-M47 & 0.0212 & 17.3 & $f_2$ & 82 & 1D-M90 & 0.0015 & 1.0 & $f_2$ \\
\hline35 & 1D-M24 & 0.0212 & 17.3 & $f_2$ & 83 & 1D-M52 & 0.0015 & 1.1 & $f_2$ \\
\hline36 & 1D-M51 & 0.0203 & 14.9 & $f_2$ & 84 & 1D-M82 & 0.0014 & 1.0 & $f_2$ \\
\hline37 & 1D-M18 & 0.0194 & 14.6 & $f_2$ & 85 & 1D-M72 & 0.0014 & 1 & $f_2$ \\
\hline38 & 1D-M69 & 0.019 & 19.0 & $f_2$ & 86 & 1D-M70 & 0.0014 & 1.0 & $f_2$ \\
\hline39 & 1D-M48 & 0.0189 & 14.0 & $f_2$ & 87 & 1D-M81 & 0.0014 & 1 & $f_2$ \\
\hline40 & 1D-M12 & 0.0188 & 12.8 & $f_2$ & 88 & 1D-M85 & 0.0014 & 1.0 & $f_2$ \\
\hline41 & 1D-M9 & 0.0185 & 12.8 & $f_2$ & 89 & 1D-M88 & 0.0014 & 1.0 & $f_2$ \\
\hline42 & 1D-M23 & 0.0177 & 13.0 & $f_2$ & 90 & 1D-M63 & 0.0013 & 1.1 & $f_2$ \\
\hline43 & 1D-M62 & 0.0167 & 9.6 & $f_2$ & 91 & 1D-M32 & 0.0013 & 0.7 & $f_2$ \\
\hline44 & 1D-M26 & 0.0167 & 9.6 & $f_2$ & 92 & 1D-M54 & 0.0013 & 1.1 & $f_2$ \\
\hline45 & 1D-M14 & 0.0163 & 10.1 & $f_2$ & 93 & 1D-M33 & 0.0012 & 0.8 & $f_2$ \\
\hline46 & 1D-M96 & 0.016 & 1.0 & $f_2$ & 94 & 1D-M78 & 0.0009 & 0.6 & $f_2$ \\
\hline47 & 1D-M6 & 0.0159 & 12.0 & $f_2$ & 95 & 1D-M74 & 0.0008 & 0.6 & $f_2$ \\
\hline48 & 1D-M4 & 0.0158 & 13.4 & $f_2$ & 96 & 1D-M75 & 0.0006 & 0.4 & $f_2$ \\
\hline
\caption{Manipulability of 1-DOF Manipulators}
\label{Tab:table_dof1mt_1} \end{longtable}



==> Dimensional Synthesis/contentfolder/mechanisms2/manipulabilitytable_new2.tex <==
%\resizebox{\linewidth}{!}{
\footnotesize
\begin{longtable}{||c|c|c|c|c|c|c||c|c|c|c|c|c|c||}

\hline
S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ & S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ \\ 
\hline
1 & 2D-M645 & 1.0 & 1.0 & 6 & 1.0 & $f_1$ & 324 & 2D-M172 & 0.0289 & 17.5 & 601 & 15.1 & $f_2$ \\
\hline2 & 2D-M315 & 0.7544 & 1.2 & 155 & 87.4 & $f_1$ & 325 & 2D-M205 & 0.028 & 14.6 & 535 & 18.9 & $f_2$ \\
\hline3 & 2D-M301 & 0.7058 & 1.2 & 158 & 88.8 & $f_2$ & 326 & 2D-M394 & 0.0271 & 12.8 & 451 & 8.6 & $f_2$ \\
\hline4 & 2D-M224 & 0.6366 & 1.1 & 127 & 60.2 & $f_1$ & 327 & 2D-M520 & 0.027 & 19.4 & 618 & 18.1 & $f_2$ \\
\hline5 & 2D-M308 & 0.6034 & 1.1 & 118 & 340.6 & $f_2$ & 328 & 2D-M421 & 0.0268 & 17.3 & 586 & 17.3 & $f_2$ \\
\hline6 & 2D-M126 & 0.5855 & 1.3 & 207 & 88.8 & $f_1$ & 329 & 2D-M360 & 0.0268 & 17.3 & 582 & 17.3 & $f_2$ \\
\hline7 & 2D-M309 & 0.5624 & 1.2 & 135 & 351.6 & $f_2$ & 330 & 2D-M413 & 0.0267 & 13.2 & 472 & 12.9 & $f_2$ \\
\hline8 & 2D-M319 & 0.5621 & 1.4 & 230 & 283.4 & $f_2$ & 331 & 2D-M355 & 0.0266 & 14.1 & 523 & 14.1 & $f_2$ \\
\hline9 & 2D-M208 & 0.5495 & 1.2 & 172 & 68.1 & $f_1$ & 332 & 2D-M349 & 0.0263 & 14.6 & 536 & 14.5 & $f_2$ \\
\hline10 & 2D-M134 & 0.541 & 1.1 & 107 & 100.5 & $f_1$ & 333 & 2D-M508 & 0.0263 & 17.6 & 606 & 16.4 & $f_2$ \\
\hline11 & 2D-M248 & 0.5381 & 1.4 & 224 & 75.2 & $f_1$ & 334 & 2D-M407 & 0.0261 & 14.9 & 541 & 14.9 & $f_2$ \\
\hline12 & 2D-M203 & 0.5289 & 1.3 & 198 & 68.1 & $f_1$ & 335 & 2D-M389 & 0.026 & 17.4 & 594 & 6.4 & $f_2$ \\
\hline13 & 2D-M634 & 0.5142 & 1.0 & 7 & 1 & $f_1$ & 336 & 2D-M424 & 0.0259 & 16.1 & 561 & 18.4 & $f_2$ \\
\hline14 & 2D-M458 & 0.5116 & 1.0 & 32 & 1.0 & $f_1$ & 337 & 2D-M450 & 0.0258 & 13.1 & 460 & 13.0 & $f_2$ \\
\hline15 & 2D-M74 & 0.5114 & 1.1 & 115 & 77.5 & $f_1$ & 338 & 2D-M534 & 0.0254 & 19.9 & 624 & 18.6 & $f_2$ \\
\hline16 & 2D-M318 & 0.5006 & 1.1 & 130 & 298.9 & $f_2$ & 339 & 2D-M548 & 0.0253 & 19.0 & 615 & 17.8 & $f_2$ \\
\hline17 & 2D-M213 & 0.4948 & 1.3 & 183 & 60.2 & $f_1$ & 340 & 2D-M387 & 0.0245 & 17.3 & 590 & 6.4 & $f_2$ \\
\hline18 & 2D-M304 & 0.4879 & 1.8 & 307 & 165.1 & $f_2$ & 341 & 2D-M412 & 0.0244 & 13.1 & 463 & 13.1 & $f_2$ \\
\hline19 & 2D-M311 & 0.485 & 1.2 & 152 & 88.5 & $f_1$ & 342 & 2D-M543 & 0.0241 & 18.5 & 610 & 18.0 & $f_2$ \\
\hline20 & 2D-M300 & 0.4831 & 2.1 & 316 & 144.2 & $f_2$ & 343 & 2D-M556 & 0.024 & 20.4 & 633 & 18.6 & $f_2$ \\
\hline21 & 2D-M314 & 0.4683 & 1.2 & 141 & 266.1 & $f_2$ & 344 & 2D-M346 & 0.0239 & 14.8 & 538 & 12.3 & $f_2$ \\
\hline22 & 2D-M303 & 0.4571 & 1.6 & 294 & 181.6 & $f_2$ & 345 & 2D-M475 & 0.0238 & 17.0 & 578 & 17.5 & $f_2$ \\
\hline23 & 2D-M305 & 0.4477 & 1.5 & 266 & 200.5 & $f_2$ & 346 & 2D-M288 & 0.0238 & 15.0 & 543 & 14.8 & $f_2$ \\
\hline24 & 2D-M98 & 0.4435 & 1.3 & 180 & 88.8 & $f_1$ & 347 & 2D-M507 & 0.0235 & 17.3 & 588 & 17.3 & $f_2$ \\
\hline25 & 2D-M302 & 0.4376 & 1.8 & 306 & 164.6 & $f_2$ & 348 & 2D-M348 & 0.0235 & 17.3 & 587 & 17.3 & $f_2$ \\
\hline26 & 2D-M299 & 0.4327 & 1.7 & 298 & 192.7 & $f_2$ & 349 & 2D-M163 & 0.0234 & 13.7 & 481 & 12.6 & $f_2$ \\
\hline27 & 2D-M86 & 0.4221 & 1.2 & 136 & 100.5 & $f_1$ & 350 & 2D-M242 & 0.023 & 18.4 & 609 & 13.8 & $f_2$ \\
\hline28 & 2D-M11 & 0.4196 & 1.1 & 117 & 60.2 & $f_1$ & 351 & 2D-M550 & 0.023 & 19.1 & 617 & 17.7 & $f_2$ \\
\hline29 & 2D-M313 & 0.418 & 1.1 & 108 & 232.3 & $f_2$ & 352 & 2D-M24 & 0.0228 & 14.5 & 532 & 12.1 & $f_2$ \\
\hline30 & 2D-M312 & 0.4138 & 1.2 & 148 & 253.8 & $f_2$ & 353 & 2D-M425 & 0.0226 & 14.1 & 522 & 14.1 & $f_2$ \\
\hline31 & 2D-M239 & 0.3908 & 1.1 & 104 & 80.4 & $f_1$ & 354 & 2D-M357 & 0.0223 & 17.4 & 595 & 16.9 & $f_2$ \\
\hline32 & 2D-M317 & 0.3621 & 1.2 & 131 & 294.7 & $f_2$ & 355 & 2D-M535 & 0.0222 & 19.8 & 623 & 18.4 & $f_2$ \\
\hline33 & 2D-M237 & 0.3503 & 1.1 & 114 & 100.5 & $f_1$ & 356 & 2D-M406 & 0.0222 & 13.9 & 494 & 15.1 & $f_2$ \\
\hline34 & 2D-M132 & 0.3441 & 1.4 & 228 & 88.8 & $f_1$ & 357 & 2D-M156 & 0.0222 & 16.8 & 572 & 13.6 & $f_2$ \\
\hline35 & 2D-M232 & 0.3306 & 1.2 & 157 & 88.8 & $f_1$ & 358 & 2D-M252 & 0.0219 & 20.3 & 632 & 14.3 & $f_2$ \\
\hline36 & 2D-M227 & 0.3291 & 1.0 & 70 & 204.1 & $f_2$ & 359 & 2D-M628 & 0.0217 & 1.0 & 26 & 1.0 & $f_2$ \\
\hline37 & 2D-M286 & 0.3224 & 1.1 & 122 & 194.5 & $f_2$ & 360 & 2D-M366 & 0.0215 & 13.0 & 458 & 12.9 & $f_2$ \\
\hline38 & 2D-M138 & 0.3142 & 1.1 & 111 & 100.5 & $f_1$ & 361 & 2D-M343 & 0.0215 & 12.1 & 429 & 7.8 & $f_2$ \\
\hline39 & 2D-M226 & 0.3127 & 1.5 & 269 & 176.2 & $f_2$ & 362 & 2D-M155 & 0.0215 & 16.3 & 563 & 13.9 & $f_2$ \\
\hline40 & 2D-M307 & 0.3125 & 1.5 & 281 & 186.7 & $f_2$ & 363 & 2D-M194 & 0.0214 & 16.3 & 562 & 13.6 & $f_2$ \\
\hline41 & 2D-M306 & 0.2991 & 1.5 & 259 & 212.1 & $f_2$ & 364 & 2D-M502 & 0.0214 & 17.3 & 584 & 17.3 & $f_2$ \\
\hline42 & 2D-M310 & 0.2946 & 1.6 & 290 & 138.7 & $f_2$ & 365 & 2D-M374 & 0.0214 & 17.3 & 583 & 17.3 & $f_2$ \\
\hline43 & 2D-M521 & 0.2929 & 8.9 & 334 & 8.4 & $f_1$ & 366 & 2D-M192 & 0.0213 & 16.1 & 560 & 13.2 & $f_2$ \\
\hline44 & 2D-M145 & 0.2902 & 1.4 & 240 & 142.5 & $f_2$ & 367 & 2D-M354 & 0.021 & 17.0 & 577 & 14.6 & $f_2$ \\
\hline45 & 2D-M234 & 0.2884 & 1.1 & 120 & 162.0 & $f_2$ & 368 & 2D-M168 & 0.0209 & 14.0 & 498 & 12.5 & $f_2$ \\
\hline46 & 2D-M59 & 0.2879 & 1.5 & 276 & 189.0 & $f_2$ & 369 & 2D-M353 & 0.0208 & 14.3 & 531 & 11.8 & $f_2$ \\
\hline47 & 2D-M128 & 0.2829 & 1.2 & 133 & 60.2 & $f_1$ & 370 & 2D-M465 & 0.0205 & 14.0 & 506 & 14.0 & $f_2$ \\
\hline48 & 2D-M187 & 0.2736 & 1.3 & 204 & 220.1 & $f_2$ & 371 & 2D-M363 & 0.0203 & 15.1 & 545 & 15.1 & $f_2$ \\
\hline49 & 2D-M293 & 0.273 & 1.3 & 192 & 182.5 & $f_2$ & 372 & 2D-M160 & 0.0202 & 15.2 & 548 & 15.1 & $f_2$ \\
\hline50 & 2D-M118 & 0.273 & 1.3 & 191 & 182.5 & $f_2$ & 373 & 2D-M17 & 0.0202 & 14.1 & 511 & 14.8 & $f_2$ \\
\hline51 & 2D-M135 & 0.273 & 1.3 & 190 & 182.5 & $f_2$ & 374 & 2D-M484 & 0.0201 & 13.0 & 456 & 10.3 & $f_2$ \\
\hline52 & 2D-M256 & 0.2719 & 1.1 & 84 & 100.5 & $f_1$ & 375 & 2D-M375 & 0.0199 & 10.9 & 378 & 10.9 & $f_2$ \\
\hline53 & 2D-M184 & 0.271 & 2.0 & 314 & 164.8 & $f_2$ & 376 & 2D-M415 & 0.0198 & 15.0 & 542 & 13.4 & $f_2$ \\
\hline54 & 2D-M140 & 0.2705 & 1.1 & 119 & 75.9 & $f_1$ & 377 & 2D-M361 & 0.0195 & 11.4 & 398 & 11.4 & $f_2$ \\
\hline55 & 2D-M209 & 0.2696 & 1.4 & 223 & 165.2 & $f_2$ & 378 & 2D-M411 & 0.0194 & 15.0 & 544 & 15.3 & $f_2$ \\
\hline56 & 2D-M236 & 0.2691 & 1.9 & 312 & 149.1 & $f_2$ & 379 & 2D-M170 & 0.0194 & 15.7 & 556 & 11.6 & $f_2$ \\
\hline57 & 2D-M282 & 0.2688 & 1.7 & 300 & 167.5 & $f_2$ & 380 & 2D-M164 & 0.0192 & 12.7 & 444 & 8.7 & $f_2$ \\
\hline58 & 2D-M9 & 0.2678 & 1.2 & 153 & 100.5 & $f_1$ & 381 & 2D-M362 & 0.0192 & 12.5 & 442 & 9.6 & $f_2$ \\
\hline59 & 2D-M182 & 0.2677 & 1.2 & 171 & 168.8 & $f_2$ & 382 & 2D-M230 & 0.0191 & 13.7 & 485 & 12.3 & $f_2$ \\
\hline60 & 2D-M144 & 0.2665 & 1.3 & 216 & 112.8 & $f_2$ & 383 & 2D-M228 & 0.0191 & 12.9 & 452 & 12.9 & $f_2$ \\
\hline61 & 2D-M295 & 0.2587 & 1.2 & 174 & 119.2 & $f_2$ & 384 & 2D-M16 & 0.0184 & 15.6 & 553 & 10.3 & $f_2$ \\
\hline62 & 2D-M524 & 0.2581 & 9.0 & 335 & 8.4 & $f_2$ & 385 & 2D-M267 & 0.0184 & 11.6 & 405 & 12.4 & $f_2$ \\
\hline63 & 2D-M316 & 0.256 & 1.2 & 175 & 168.8 & $f_2$ & 386 & 2D-M376 & 0.0184 & 11.4 & 399 & 10.1 & $f_2$ \\
\hline64 & 2D-M285 & 0.2533 & 1.1 & 80 & 174.6 & $f_2$ & 387 & 2D-M410 & 0.0183 & 16.5 & 567 & 13.8 & $f_2$ \\
\hline65 & 2D-M217 & 0.2526 & 1.6 & 284 & 126.4 & $f_2$ & 388 & 2D-M193 & 0.0181 & 10.8 & 370 & 9.6 & $f_2$ \\
\hline66 & 2D-M116 & 0.2519 & 1.6 & 295 & 123.7 & $f_2$ & 389 & 2D-M378 & 0.0181 & 14.7 & 537 & 12.7 & $f_2$ \\
\hline67 & 2D-M264 & 0.2518 & 7.7 & 325 & 7.1 & $f_1$ & 390 & 2D-M278 & 0.0181 & 16.1 & 558 & 10.6 & $f_2$ \\
\hline68 & 2D-M152 & 0.2506 & 1.1 & 116 & 162.4 & $f_2$ & 391 & 2D-M158 & 0.0179 & 15.3 & 551 & 12.9 & $f_2$ \\
\hline69 & 2D-M87 & 0.2471 & 1.4 & 227 & 132.4 & $f_2$ & 392 & 2D-M456 & 0.0178 & 19.8 & 621 & 13.2 & $f_2$ \\
\hline70 & 2D-M522 & 0.2466 & 7.7 & 326 & 7.1 & $f_2$ & 393 & 2D-M344 & 0.0178 & 13.0 & 454 & 10.0 & $f_2$ \\
\hline71 & 2D-M82 & 0.2439 & 1.2 & 173 & 88.8 & $f_1$ & 394 & 2D-M175 & 0.0177 & 18.9 & 613 & 10.5 & $f_2$ \\
\hline72 & 2D-M88 & 0.2418 & 1.3 & 179 & 182.1 & $f_2$ & 395 & 2D-M474 & 0.0177 & 10.9 & 375 & 10.9 & $f_2$ \\
\hline73 & 2D-M298 & 0.2387 & 1.5 & 265 & 202.0 & $f_2$ & 396 & 2D-M430 & 0.0175 & 10.4 & 358 & 11.7 & $f_2$ \\
\hline74 & 2D-M526 & 0.2381 & 7.7 & 327 & 7.1 & $f_2$ & 397 & 2D-M497 & 0.0174 & 20.4 & 634 & 13.0 & $f_2$ \\
\hline75 & 2D-M215 & 0.2377 & 1.4 & 241 & 100.5 & $f_1$ & 398 & 2D-M28 & 0.0174 & 14.1 & 524 & 14.1 & $f_2$ \\
\hline76 & 2D-M143 & 0.2369 & 1.1 & 82 & 210.2 & $f_2$ & 399 & 2D-M26 & 0.0174 & 14.1 & 525 & 14.1 & $f_2$ \\
\hline77 & 2D-M113 & 0.2355 & 1.4 & 226 & 101.2 & $f_2$ & 400 & 2D-M372 & 0.0173 & 10.9 & 376 & 10.9 & $f_2$ \\
\hline78 & 2D-M61 & 0.233 & 1.8 & 305 & 113.4 & $f_2$ & 401 & 2D-M485 & 0.0173 & 20.8 & 635 & 9.5 & $f_2$ \\
\hline79 & 2D-M546 & 0.2319 & 7.7 & 328 & 7.1 & $f_2$ & 402 & 2D-M460 & 0.0171 & 12.4 & 439 & 9.4 & $f_2$ \\
\hline80 & 2D-M43 & 0.2307 & 1.4 & 246 & 135.8 & $f_2$ & 403 & 2D-M503 & 0.017 & 15.2 & 547 & 12.3 & $f_2$ \\
\hline81 & 2D-M71 & 0.2305 & 2.0 & 313 & 173.2 & $f_2$ & 404 & 2D-M439 & 0.017 & 15.2 & 546 & 12.3 & $f_2$ \\
\hline82 & 2D-M181 & 0.2289 & 1.3 & 219 & 142.6 & $f_2$ & 405 & 2D-M489 & 0.017 & 17.8 & 608 & 10.8 & $f_2$ \\
\hline83 & 2D-M80 & 0.2278 & 1.5 & 263 & 124.4 & $f_2$ & 406 & 2D-M201 & 0.0169 & 14.3 & 530 & 10.4 & $f_2$ \\
\hline84 & 2D-M66 & 0.227 & 1.3 & 178 & 165.4 & $f_2$ & 407 & 2D-M504 & 0.0169 & 13.0 & 457 & 11.3 & $f_2$ \\
\hline85 & 2D-M527 & 0.2263 & 9.0 & 339 & 8.4 & $f_2$ & 408 & 2D-M173 & 0.0169 & 15.2 & 549 & 12.4 & $f_2$ \\
\hline86 & 2D-M185 & 0.2257 & 1.0 & 76 & 149.1 & $f_2$ & 409 & 2D-M404 & 0.0169 & 13.5 & 475 & 10.7 & $f_2$ \\
\hline87 & 2D-M63 & 0.2253 & 1.5 & 271 & 134.9 & $f_2$ & 410 & 2D-M277 & 0.0168 & 12.7 & 446 & 9.3 & $f_2$ \\
\hline88 & 2D-M103 & 0.2251 & 1.3 & 209 & 123.4 & $f_2$ & 411 & 2D-M196 & 0.0166 & 11.8 & 419 & 13.3 & $f_2$ \\
\hline89 & 2D-M251 & 0.2246 & 1.3 & 181 & 141.0 & $f_2$ & 412 & 2D-M364 & 0.0166 & 12.4 & 438 & 9.3 & $f_2$ \\
\hline90 & 2D-M177 & 0.2241 & 1.5 & 279 & 111.0 & $f_2$ & 413 & 2D-M254 & 0.0166 & 12.2 & 430 & 10.5 & $f_2$ \\
\hline91 & 2D-M555 & 0.224 & 9.0 & 340 & 8.4 & $f_2$ & 414 & 2D-M390 & 0.0166 & 17.4 & 596 & 4.1 & $f_2$ \\
\hline92 & 2D-M284 & 0.223 & 2.0 & 315 & 136.6 & $f_2$ & 415 & 2D-M405 & 0.0165 & 11.6 & 404 & 10.2 & $f_2$ \\
\hline93 & 2D-M130 & 0.2218 & 1.3 & 193 & 126.6 & $f_2$ & 416 & 2D-M381 & 0.0163 & 14.2 & 526 & 8.2 & $f_2$ \\
\hline94 & 2D-M212 & 0.2218 & 1.6 & 291 & 137.2 & $f_2$ & 417 & 2D-M408 & 0.0162 & 10.3 & 353 & 10.3 & $f_2$ \\
\hline95 & 2D-M291 & 0.2201 & 1.6 & 288 & 123.7 & $f_2$ & 418 & 2D-M477 & 0.0161 & 10.9 & 379 & 10.9 & $f_2$ \\
\hline96 & 2D-M223 & 0.2201 & 1.6 & 287 & 123.7 & $f_2$ & 419 & 2D-M359 & 0.0161 & 10.9 & 377 & 10.9 & $f_2$ \\
\hline97 & 2D-M120 & 0.2189 & 1.0 & 61 & 145.2 & $f_2$ & 420 & 2D-M174 & 0.0161 & 13.8 & 487 & 11.2 & $f_2$ \\
\hline98 & 2D-M639 & 0.2183 & 1.0 & 18 & 1.0 & $f_2$ & 421 & 2D-M266 & 0.016 & 12.2 & 435 & 11.3 & $f_2$ \\
\hline99 & 2D-M468 & 0.2157 & 1.0 & 38 & 1.0 & $f_1$ & 422 & 2D-M263 & 0.016 & 12.5 & 441 & 10.7 & $f_2$ \\
\hline100 & 2D-M235 & 0.2155 & 1.3 & 199 & 109.6 & $f_2$ & 423 & 2D-M369 & 0.0159 & 9.0 & 337 & 9.0 & $f_2$ \\
\hline101 & 2D-M525 & 0.2138 & 9.0 & 341 & 8.4 & $f_2$ & 424 & 2D-M199 & 0.0159 & 24.4 & 641 & 9.2 & $f_2$ \\
\hline102 & 2D-M188 & 0.2127 & 1.4 & 244 & 139.6 & $f_2$ & 425 & 2D-M453 & 0.0159 & 11.7 & 411 & 10.9 & $f_2$ \\
\hline103 & 2D-M635 & 0.2096 & 1.0 & 48 & 1.0 & $f_2$ & 426 & 2D-M500 & 0.0159 & 17.5 & 603 & 10.1 & $f_2$ \\
\hline104 & 2D-M631 & 0.208 & 1.0 & 11 & 1.0 & $f_2$ & 427 & 2D-M435 & 0.0158 & 12.0 & 422 & 8.7 & $f_2$ \\
\hline105 & 2D-M68 & 0.208 & 1.2 & 164 & 175.5 & $f_2$ & 428 & 2D-M198 & 0.0158 & 12.7 & 445 & 11.2 & $f_2$ \\
\hline106 & 2D-M514 & 0.2078 & 9.0 & 342 & 8.4 & $f_2$ & 429 & 2D-M397 & 0.0156 & 14.1 & 514 & 9.3 & $f_2$ \\
\hline107 & 2D-M146 & 0.2056 & 1.2 & 161 & 182.5 & $f_2$ & 430 & 2D-M473 & 0.0155 & 17.5 & 602 & 9.9 & $f_2$ \\
\hline108 & 2D-M297 & 0.204 & 1.9 & 310 & 155.9 & $f_2$ & 431 & 2D-M229 & 0.0155 & 12.7 & 448 & 9.5 & $f_2$ \\
\hline109 & 2D-M56 & 0.2028 & 1.1 & 95 & 159.5 & $f_2$ & 432 & 2D-M260 & 0.0154 & 11.8 & 420 & 8.5 & $f_2$ \\
\hline110 & 2D-M100 & 0.2023 & 1.6 & 293 & 178.8 & $f_2$ & 433 & 2D-M23 & 0.0154 & 9.9 & 348 & 10.3 & $f_2$ \\
\hline111 & 2D-M190 & 0.202 & 10.2 & 351 & 9.5 & $f_1$ & 434 & 2D-M461 & 0.0154 & 11.9 & 421 & 9.8 & $f_2$ \\
\hline112 & 2D-M137 & 0.2016 & 1.0 & 68 & 149.0 & $f_2$ & 435 & 2D-M35 & 0.0153 & 11.5 & 402 & 12.9 & $f_2$ \\
\hline113 & 2D-M629 & 0.2016 & 1.0 & 36 & 1.0 & $f_2$ & 436 & 2D-M427 & 0.0153 & 13.4 & 473 & 10.1 & $f_2$ \\
\hline114 & 2D-M180 & 0.1995 & 1.4 & 225 & 109.1 & $f_2$ & 437 & 2D-M165 & 0.0153 & 11.7 & 410 & 7.8 & $f_2$ \\
\hline115 & 2D-M127 & 0.1984 & 1.3 & 201 & 165.2 & $f_2$ & 438 & 2D-M200 & 0.0152 & 12.8 & 449 & 10.8 & $f_2$ \\
\hline116 & 2D-M512 & 0.1978 & 9.1 & 343 & 8.4 & $f_2$ & 439 & 2D-M383 & 0.0152 & 11.6 & 407 & 10.5 & $f_2$ \\
\hline117 & 2D-M246 & 0.1971 & 1.3 & 184 & 132.2 & $f_2$ & 440 & 2D-M385 & 0.0152 & 13.0 & 455 & 8.3 & $f_2$ \\
\hline118 & 2D-M76 & 0.1969 & 2.5 & 321 & 138.2 & $f_2$ & 441 & 2D-M220 & 0.0151 & 11.8 & 417 & 8.6 & $f_2$ \\
\hline119 & 2D-M85 & 0.1964 & 1.1 & 121 & 140.2 & $f_2$ & 442 & 2D-M499 & 0.015 & 13.8 & 489 & 9.3 & $f_2$ \\
\hline120 & 2D-M121 & 0.1964 & 1.2 & 132 & 144.5 & $f_2$ & 443 & 2D-M153 & 0.0149 & 13.6 & 478 & 11.8 & $f_2$ \\
\hline121 & 2D-M231 & 0.195 & 1.2 & 144 & 143.0 & $f_2$ & 444 & 2D-M159 & 0.0148 & 14.1 & 520 & 9.8 & $f_2$ \\
\hline122 & 2D-M222 & 0.1949 & 1.4 & 242 & 107.6 & $f_2$ & 445 & 2D-M340 & 0.0148 & 17.6 & 607 & 12.0 & $f_2$ \\
\hline123 & 2D-M250 & 0.1936 & 1.3 & 185 & 107.3 & $f_2$ & 446 & 2D-M466 & 0.0148 & 11.5 & 400 & 10.4 & $f_2$ \\
\hline124 & 2D-M210 & 0.1922 & 1.1 & 105 & 135.4 & $f_2$ & 447 & 2D-M419 & 0.0147 & 10.7 & 367 & 6.9 & $f_2$ \\
\hline125 & 2D-M257 & 0.1919 & 1.4 & 220 & 130.8 & $f_2$ & 448 & 2D-M259 & 0.0146 & 12.2 & 431 & 8.9 & $f_2$ \\
\hline126 & 2D-M523 & 0.1895 & 7.8 & 329 & 7.1 & $f_2$ & 449 & 2D-M273 & 0.0146 & 12.8 & 450 & 9.7 & $f_2$ \\
\hline127 & 2D-M53 & 0.1889 & 1.0 & 57 & 111.8 & $f_2$ & 450 & 2D-M244 & 0.0146 & 13.7 & 482 & 10.5 & $f_2$ \\
\hline128 & 2D-M69 & 0.1883 & 1.3 & 212 & 147.5 & $f_2$ & 451 & 2D-M451 & 0.0145 & 12.9 & 453 & 6.4 & $f_2$ \\
\hline129 & 2D-M529 & 0.1881 & 11.2 & 381 & 10.5 & $f_2$ & 452 & 2D-M31 & 0.0145 & 8.2 & 330 & 8.2 & $f_2$ \\
\hline130 & 2D-M276 & 0.1869 & 11.2 & 382 & 10.5 & $f_1$ & 453 & 2D-M289 & 0.0145 & 11.5 & 401 & 8.6 & $f_2$ \\
\hline131 & 2D-M216 & 0.1861 & 1.3 & 217 & 104.7 & $f_2$ & 454 & 2D-M279 & 0.0144 & 12.5 & 440 & 8.7 & $f_2$ \\
\hline132 & 2D-M142 & 0.1846 & 1.2 & 169 & 149.0 & $f_2$ & 455 & 2D-M417 & 0.0143 & 13.1 & 465 & 11.3 & $f_2$ \\
\hline133 & 2D-M101 & 0.1844 & 1.2 & 176 & 120.0 & $f_2$ & 456 & 2D-M386 & 0.0143 & 17.3 & 589 & 5.3 & $f_2$ \\
\hline134 & 2D-M557 & 0.1843 & 10.2 & 352 & 9.5 & $f_2$ & 457 & 2D-M342 & 0.0142 & 17.4 & 593 & 5.2 & $f_2$ \\
\hline135 & 2D-M221 & 0.182 & 1.4 & 248 & 130.1 & $f_2$ & 458 & 2D-M488 & 0.0141 & 13.1 & 461 & 11.3 & $f_2$ \\
\hline136 & 2D-M183 & 0.1812 & 1.3 & 205 & 101.1 & $f_2$ & 459 & 2D-M167 & 0.014 & 10.6 & 365 & 7.0 & $f_2$ \\
\hline137 & 2D-M141 & 0.1806 & 1.5 & 272 & 81.9 & $f_2$ & 460 & 2D-M501 & 0.0139 & 14.0 & 501 & 10.6 & $f_2$ \\
\hline138 & 2D-M202 & 0.1799 & 1.1 & 103 & 110.3 & $f_2$ & 461 & 2D-M368 & 0.0139 & 14.0 & 502 & 10.6 & $f_2$ \\
\hline139 & 2D-M102 & 0.1795 & 1.3 & 213 & 95.2 & $f_2$ & 462 & 2D-M480 & 0.0139 & 16.4 & 566 & 10.3 & $f_2$ \\
\hline140 & 2D-M124 & 0.176 & 1.2 & 137 & 119.2 & $f_2$ & 463 & 2D-M258 & 0.0139 & 9.8 & 346 & 6.8 & $f_2$ \\
\hline141 & 2D-M513 & 0.1754 & 11.2 & 383 & 10.5 & $f_2$ & 464 & 2D-M392 & 0.0139 & 18.5 & 612 & 4.9 & $f_2$ \\
\hline142 & 2D-M94 & 0.1753 & 1.4 & 236 & 88.8 & $f_1$ & 465 & 2D-M189 & 0.0139 & 13.8 & 491 & 10.4 & $f_2$ \\
\hline143 & 2D-M517 & 0.175 & 11.2 & 384 & 10.5 & $f_2$ & 466 & 2D-M154 & 0.0138 & 13.6 & 479 & 10.3 & $f_2$ \\
\hline144 & 2D-M99 & 0.1747 & 1.1 & 92 & 132.9 & $f_2$ & 467 & 2D-M261 & 0.0138 & 14.0 & 507 & 10.6 & $f_2$ \\
\hline145 & 2D-M554 & 0.1742 & 11.2 & 385 & 10.5 & $f_2$ & 468 & 2D-M510 & 0.0138 & 9.9 & 347 & 7.1 & $f_2$ \\
\hline146 & 2D-M519 & 0.174 & 11.2 & 386 & 10.5 & $f_2$ & 469 & 2D-M399 & 0.0138 & 16.6 & 568 & 11.0 & $f_2$ \\
\hline147 & 2D-M207 & 0.1733 & 1.0 & 52 & 124.9 & $f_2$ & 470 & 2D-M14 & 0.0138 & 10.8 & 371 & 6.9 & $f_2$ \\
\hline148 & 2D-M60 & 0.1729 & 2.4 & 319 & 130.4 & $f_2$ & 471 & 2D-M324 & 0.0137 & 13.8 & 488 & 10.6 & $f_2$ \\
\hline149 & 2D-M559 & 0.1727 & 11.2 & 387 & 10.5 & $f_2$ & 472 & 2D-M382 & 0.0137 & 19.9 & 625 & 5.8 & $f_2$ \\
\hline150 & 2D-M62 & 0.1717 & 1.1 & 112 & 120.5 & $f_2$ & 473 & 2D-M271 & 0.0136 & 13.9 & 496 & 10.5 & $f_2$ \\
\hline151 & 2D-M632 & 0.171 & 1.0 & 27 & 1.0 & $f_2$ & 474 & 2D-M403 & 0.0136 & 11.1 & 380 & 7.1 & $f_2$ \\
\hline152 & 2D-M111 & 0.1708 & 1.3 & 211 & 109.6 & $f_2$ & 475 & 2D-M333 & 0.0136 & 13.9 & 497 & 10.5 & $f_2$ \\
\hline153 & 2D-M545 & 0.1704 & 11.2 & 389 & 10.5 & $f_2$ & 476 & 2D-M12 & 0.0136 & 12.2 & 434 & 8.9 & $f_2$ \\
\hline154 & 2D-M48 & 0.17 & 1.3 & 182 & 117.5 & $f_2$ & 477 & 2D-M356 & 0.0136 & 10.8 & 372 & 7.2 & $f_2$ \\
\hline155 & 2D-M96 & 0.169 & 1.2 & 156 & 96.8 & $f_2$ & 478 & 2D-M331 & 0.0132 & 13.1 & 459 & 9.5 & $f_2$ \\
\hline156 & 2D-M186 & 0.1684 & 1.7 & 297 & 108.9 & $f_2$ & 479 & 2D-M269 & 0.0132 & 13.5 & 476 & 10.8 & $f_2$ \\
\hline157 & 2D-M214 & 0.1681 & 1.1 & 129 & 101.3 & $f_2$ & 480 & 2D-M281 & 0.0132 & 10.0 & 349 & 7.0 & $f_2$ \\
\hline158 & 2D-M110 & 0.1679 & 1.1 & 93 & 135.3 & $f_2$ & 481 & 2D-M351 & 0.0132 & 14.2 & 528 & 10.8 & $f_2$ \\
\hline159 & 2D-M601 & 0.1676 & 1.0 & 34 & 1.0 & $f_1$ & 482 & 2D-M431 & 0.0132 & 14.2 & 527 & 10.8 & $f_2$ \\
\hline160 & 2D-M46 & 0.1674 & 1.2 & 145 & 100.4 & $f_2$ & 483 & 2D-M337 & 0.0132 & 12.0 & 424 & 8.4 & $f_2$ \\
\hline161 & 2D-M518 & 0.1665 & 11.2 & 390 & 10.5 & $f_2$ & 484 & 2D-M166 & 0.0132 & 14.0 & 499 & 9.4 & $f_2$ \\
\hline162 & 2D-M122 & 0.166 & 1.2 & 142 & 104.2 & $f_2$ & 485 & 2D-M265 & 0.0131 & 14.0 & 500 & 10.5 & $f_2$ \\
\hline163 & 2D-M283 & 0.1653 & 1.6 & 292 & 123.1 & $f_2$ & 486 & 2D-M393 & 0.0131 & 18.5 & 611 & 4.9 & $f_2$ \\
\hline164 & 2D-M97 & 0.1652 & 1.5 & 280 & 112.8 & $f_2$ & 487 & 2D-M462 & 0.0131 & 14.0 & 503 & 10.5 & $f_2$ \\
\hline165 & 2D-M627 & 0.1651 & 1.0 & 28 & 1.0 & $f_2$ & 488 & 2D-M436 & 0.0131 & 14.0 & 504 & 10.5 & $f_2$ \\
\hline166 & 2D-M204 & 0.1636 & 1.4 & 253 & 92.9 & $f_2$ & 489 & 2D-M334 & 0.0131 & 14.0 & 505 & 10.5 & $f_2$ \\
\hline167 & 2D-M558 & 0.1626 & 11.2 & 391 & 10.5 & $f_2$ & 490 & 2D-M329 & 0.013 & 12.0 & 425 & 8.4 & $f_2$ \\
\hline168 & 2D-M296 & 0.1625 & 1.2 & 134 & 119.5 & $f_2$ & 491 & 2D-M384 & 0.013 & 21.4 & 639 & 10.5 & $f_2$ \\
\hline169 & 2D-M131 & 0.1618 & 1.2 & 143 & 128.4 & $f_2$ & 492 & 2D-M395 & 0.013 & 21.3 & 638 & 10.5 & $f_2$ \\
\hline170 & 2D-M623 & 0.1613 & 1.0 & 14 & 1.0 & $f_2$ & 493 & 2D-M396 & 0.013 & 19.7 & 619 & 7.1 & $f_2$ \\
\hline171 & 2D-M640 & 0.1608 & 1.0 & 43 & 1.0 & $f_2$ & 494 & 2D-M162 & 0.013 & 10.8 & 368 & 7.1 & $f_2$ \\
\hline172 & 2D-M107 & 0.1602 & 1.1 & 83 & 120.8 & $f_2$ & 495 & 2D-M206 & 0.013 & 10.9 & 374 & 8.2 & $f_2$ \\
\hline173 & 2D-M515 & 0.1581 & 11.2 & 392 & 10.5 & $f_2$ & 496 & 2D-M274 & 0.013 & 12.0 & 423 & 8.5 & $f_2$ \\
\hline174 & 2D-M49 & 0.1576 & 1.1 & 109 & 91.0 & $f_2$ & 497 & 2D-M511 & 0.013 & 13.9 & 495 & 10.6 & $f_2$ \\
\hline175 & 2D-M108 & 0.1576 & 1.1 & 99 & 127.9 & $f_2$ & 498 & 2D-M418 & 0.0129 & 14.0 & 508 & 10.5 & $f_2$ \\
\hline176 & 2D-M597 & 0.1569 & 1.0 & 41 & 1.0 & $f_1$ & 499 & 2D-M350 & 0.0129 & 14.1 & 510 & 10.5 & $f_2$ \\
\hline177 & 2D-M136 & 0.1553 & 1.2 & 139 & 126.7 & $f_2$ & 500 & 2D-M370 & 0.0129 & 13.1 & 464 & 9.5 & $f_2$ \\
\hline178 & 2D-M292 & 0.1543 & 1.2 & 163 & 124.6 & $f_2$ & 501 & 2D-M339 & 0.0129 & 11.3 & 394 & 7.1 & $f_2$ \\
\hline179 & 2D-M45 & 0.1538 & 1.3 & 218 & 137.5 & $f_2$ & 502 & 2D-M347 & 0.0129 & 14.0 & 509 & 10.5 & $f_2$ \\
\hline180 & 2D-M148 & 0.1535 & 1.0 & 56 & 91.6 & $f_2$ & 503 & 2D-M479 & 0.0129 & 13.8 & 492 & 10.3 & $f_2$ \\
\hline181 & 2D-M243 & 0.1534 & 11.3 & 393 & 10.5 & $f_1$ & 504 & 2D-M287 & 0.0129 & 14.3 & 529 & 8.8 & $f_2$ \\
\hline182 & 2D-M104 & 0.1515 & 1.1 & 102 & 121.5 & $f_2$ & 505 & 2D-M19 & 0.0129 & 10.8 & 373 & 7.1 & $f_2$ \\
\hline183 & 2D-M638 & 0.1508 & 1.0 & 31 & 1.0 & $f_2$ & 506 & 2D-M470 & 0.0128 & 13.1 & 466 & 9.5 & $f_2$ \\
\hline184 & 2D-M225 & 0.1494 & 1.1 & 81 & 109.5 & $f_2$ & 507 & 2D-M506 & 0.0128 & 11.8 & 418 & 8.1 & $f_2$ \\
\hline185 & 2D-M454 & 0.1488 & 10.3 & 354 & 9.5 & $f_1$ & 508 & 2D-M437 & 0.0128 & 12.1 & 426 & 8.4 & $f_2$ \\
\hline186 & 2D-M84 & 0.1484 & 1.6 & 283 & 114.9 & $f_2$ & 509 & 2D-M401 & 0.0128 & 13.1 & 468 & 9.5 & $f_2$ \\
\hline187 & 2D-M47 & 0.1467 & 1.3 & 189 & 103.7 & $f_2$ & 510 & 2D-M338 & 0.0128 & 17.3 & 581 & 9.5 & $f_2$ \\
\hline188 & 2D-M44 & 0.1466 & 1.4 & 247 & 121.1 & $f_2$ & 511 & 2D-M464 & 0.0127 & 14.1 & 513 & 10.5 & $f_2$ \\
\hline189 & 2D-M241 & 0.1455 & 1.4 & 257 & 90.4 & $f_2$ & 512 & 2D-M433 & 0.0127 & 13.1 & 469 & 9.5 & $f_2$ \\
\hline190 & 2D-M114 & 0.1451 & 1.1 & 98 & 116.6 & $f_2$ & 513 & 2D-M423 & 0.0127 & 13.8 & 490 & 10.2 & $f_2$ \\
\hline191 & 2D-M528 & 0.1447 & 11.3 & 395 & 10.5 & $f_2$ & 514 & 2D-M472 & 0.0127 & 13.1 & 462 & 9.6 & $f_2$ \\
\hline192 & 2D-M621 & 0.1437 & 1.0 & 30 & 1.0 & $f_2$ & 515 & 2D-M336 & 0.0127 & 14.1 & 515 & 10.5 & $f_2$ \\
\hline193 & 2D-M478 & 0.1431 & 10.3 & 355 & 9.5 & $f_1$ & 516 & 2D-M321 & 0.0126 & 12.1 & 427 & 8.4 & $f_2$ \\
\hline194 & 2D-M268 & 0.1428 & 11.3 & 396 & 10.5 & $f_1$ & 517 & 2D-M380 & 0.0126 & 15.7 & 557 & 10.2 & $f_2$ \\
\hline195 & 2D-M609 & 0.1385 & 1.0 & 40 & 1.0 & $f_1$ & 518 & 2D-M335 & 0.0126 & 14.1 & 516 & 10.5 & $f_2$ \\
\hline196 & 2D-M133 & 0.1381 & 1.5 & 277 & 94.7 & $f_2$ & 519 & 2D-M21 & 0.0126 & 12.1 & 428 & 8.4 & $f_2$ \\
\hline197 & 2D-M90 & 0.1378 & 1.2 & 140 & 100.2 & $f_2$ & 520 & 2D-M345 & 0.0126 & 13.2 & 470 & 9.5 & $f_2$ \\
\hline198 & 2D-M51 & 0.1372 & 1.4 & 254 & 104.1 & $f_2$ & 521 & 2D-M367 & 0.0126 & 14.1 & 517 & 10.5 & $f_2$ \\
\hline199 & 2D-M95 & 0.1364 & 1.2 & 150 & 90.2 & $f_2$ & 522 & 2D-M25 & 0.0126 & 13.2 & 471 & 9.5 & $f_2$ \\
\hline200 & 2D-M115 & 0.1354 & 1.1 & 128 & 91.0 & $f_2$ & 523 & 2D-M320 & 0.0126 & 14.1 & 518 & 10.5 & $f_2$ \\
\hline201 & 2D-M89 & 0.1353 & 1.5 & 270 & 87.1 & $f_2$ & 524 & 2D-M30 & 0.0125 & 14.1 & 519 & 10.5 & $f_2$ \\
\hline202 & 2D-M371 & 0.1352 & 7.7 & 324 & 6.8 & $f_1$ & 525 & 2D-M323 & 0.0125 & 12.7 & 447 & 7.5 & $f_2$ \\
\hline203 & 2D-M238 & 0.134 & 1.4 & 249 & 85.2 & $f_2$ & 526 & 2D-M428 & 0.0123 & 16.8 & 576 & 10.1 & $f_2$ \\
\hline204 & 2D-M129 & 0.1339 & 1.0 & 13 & 91.0 & $f_2$ & 527 & 2D-M496 & 0.0121 & 14.1 & 521 & 9.9 & $f_2$ \\
\hline205 & 2D-M81 & 0.1336 & 1.3 & 195 & 98.0 & $f_2$ & 528 & 2D-M455 & 0.0121 & 12.6 & 443 & 8.1 & $f_2$ \\
\hline206 & 2D-M626 & 0.133 & 1.0 & 49 & 1.0 & $f_2$ & 529 & 2D-M330 & 0.0121 & 13.7 & 483 & 9.2 & $f_2$ \\
\hline207 & 2D-M625 & 0.1323 & 1.0 & 20 & 1.0 & $f_2$ & 530 & 2D-M449 & 0.0121 & 9.0 & 338 & 5.1 & $f_2$ \\
\hline208 & 2D-M516 & 0.1323 & 10.4 & 356 & 9.5 & $f_2$ & 531 & 2D-M169 & 0.012 & 10.6 & 364 & 8.1 & $f_2$ \\
\hline209 & 2D-M5 & 0.1309 & 1.3 & 206 & 100.1 & $f_2$ & 532 & 2D-M161 & 0.012 & 15.3 & 550 & 10.1 & $f_2$ \\
\hline210 & 2D-M52 & 0.1305 & 1.6 & 286 & 100.4 & $f_2$ & 533 & 2D-M402 & 0.0119 & 13.7 & 486 & 8.8 & $f_2$ \\
\hline211 & 2D-M247 & 0.1293 & 1.6 & 285 & 88.8 & $f_2$ & 534 & 2D-M446 & 0.0119 & 15.6 & 554 & 9.5 & $f_2$ \\
\hline212 & 2D-M109 & 0.1284 & 1.4 & 233 & 105.7 & $f_2$ & 535 & 2D-M429 & 0.0119 & 13.8 & 493 & 8.5 & $f_2$ \\
\hline213 & 2D-M64 & 0.128 & 1.0 & 75 & 85.3 & $f_2$ & 536 & 2D-M358 & 0.0117 & 13.5 & 474 & 9.6 & $f_2$ \\
\hline214 & 2D-M83 & 0.1275 & 1.0 & 15 & 111.0 & $f_2$ & 537 & 2D-M275 & 0.0117 & 13.7 & 484 & 7.0 & $f_2$ \\
\hline215 & 2D-M75 & 0.1272 & 1.3 & 202 & 88.8 & $f_2$ & 538 & 2D-M272 & 0.0117 & 13.1 & 467 & 9.2 & $f_2$ \\
\hline216 & 2D-M447 & 0.1272 & 11.4 & 397 & 10.5 & $f_1$ & 539 & 2D-M327 & 0.0116 & 14.6 & 534 & 9.4 & $f_2$ \\
\hline217 & 2D-M79 & 0.1264 & 1.6 & 296 & 75.3 & $f_2$ & 540 & 2D-M322 & 0.0116 & 14.6 & 533 & 9.5 & $f_2$ \\
\hline218 & 2D-M245 & 0.1264 & 1.1 & 100 & 96.5 & $f_2$ & 541 & 2D-M490 & 0.0115 & 24.5 & 642 & 8.4 & $f_2$ \\
\hline219 & 2D-M65 & 0.1258 & 1.0 & 51 & 90.7 & $f_2$ & 542 & 2D-M505 & 0.0114 & 24.4 & 640 & 8.4 & $f_2$ \\
\hline220 & 2D-M8 & 0.1255 & 1.7 & 301 & 86.0 & $f_2$ & 543 & 2D-M13 & 0.0113 & 13.5 & 477 & 9.3 & $f_2$ \\
\hline221 & 2D-M54 & 0.125 & 1.2 & 149 & 68.0 & $f_2$ & 544 & 2D-M18 & 0.0112 & 12.3 & 437 & 8.4 & $f_2$ \\
\hline222 & 2D-M4 & 0.1247 & 1.9 & 311 & 62.0 & $f_2$ & 545 & 2D-M432 & 0.0111 & 15.6 & 555 & 7.4 & $f_2$ \\
\hline223 & 2D-M3 & 0.1245 & 1.1 & 123 & 88.7 & $f_2$ & 546 & 2D-M341 & 0.011 & 17.3 & 592 & 2.9 & $f_2$ \\
\hline224 & 2D-M72 & 0.1243 & 1.2 & 168 & 74.9 & $f_2$ & 547 & 2D-M400 & 0.0109 & 26.1 & 644 & 7.8 & $f_2$ \\
\hline225 & 2D-M6 & 0.1242 & 1.0 & 62 & 111.1 & $f_2$ & 548 & 2D-M191 & 0.0108 & 15.3 & 552 & 8.0 & $f_2$ \\
\hline226 & 2D-M544 & 0.1241 & 17.5 & 604 & 17.5 & $f_2$ & 549 & 2D-M20 & 0.0107 & 8.7 & 332 & 6.6 & $f_2$ \\
\hline227 & 2D-M50 & 0.1236 & 1.2 & 151 & 85.4 & $f_2$ & 550 & 2D-M388 & 0.0107 & 17.3 & 591 & 2.9 & $f_2$ \\
\hline228 & 2D-M414 & 0.1229 & 10.4 & 359 & 9.5 & $f_1$ & 551 & 2D-M448 & 0.0105 & 12.2 & 432 & 5.8 & $f_2$ \\
\hline229 & 2D-M151 & 0.1218 & 1.0 & 72 & 93.3 & $f_2$ & 552 & 2D-M325 & 0.0104 & 16.7 & 571 & 8.1 & $f_2$ \\
\hline230 & 2D-M7 & 0.1216 & 1.4 & 222 & 100.5 & $f_2$ & 553 & 2D-M270 & 0.0098 & 16.7 & 570 & 6.6 & $f_2$ \\
\hline231 & 2D-M41 & 0.1211 & 1.2 & 154 & 98.8 & $f_2$ & 554 & 2D-M643 & 0.0091 & 14.8 & 539 & 10.5 & $f_1$ \\
\hline232 & 2D-M117 & 0.121 & 1.0 & 66 & 92.3 & $f_2$ & 555 & 2D-M644 & 0.0091 & 14.8 & 540 & 10.5 & $f_1$ \\
\hline233 & 2D-M150 & 0.121 & 1.0 & 67 & 92.3 & $f_2$ & 556 & 2D-M416 & 0.0088 & 25.6 & 643 & 7.1 & $f_2$ \\
\hline234 & 2D-M106 & 0.1209 & 1.3 & 208 & 92.2 & $f_2$ & 557 & 2D-M195 & 0.0085 & 16.7 & 569 & 4.9 & $f_2$ \\
\hline235 & 2D-M211 & 0.1199 & 2.2 & 318 & 87.7 & $f_2$ & 558 & 2D-M197 & 0.0084 & 13.6 & 480 & 4.5 & $f_2$ \\
\hline236 & 2D-M57 & 0.1189 & 1.5 & 268 & 96.6 & $f_2$ & 559 & 2D-M22 & 0.0082 & 18.9 & 614 & 6.1 & $f_2$ \\
\hline237 & 2D-M139 & 0.1182 & 1.3 & 177 & 69.6 & $f_2$ & 560 & 2D-M326 & 0.0079 & 16.4 & 564 & 5.8 & $f_2$ \\
\hline238 & 2D-M240 & 0.1178 & 1.1 & 125 & 88.9 & $f_2$ & 561 & 2D-M486 & 0.0079 & 16.4 & 565 & 5.8 & $f_2$ \\
\hline239 & 2D-M105 & 0.1177 & 1.2 & 162 & 89.5 & $f_2$ & 562 & 2D-M398 & 0.0078 & 27.4 & 645 & 6.4 & $f_2$ \\
\hline240 & 2D-M541 & 0.1172 & 9.3 & 345 & 8.4 & $f_1$ & 563 & 2D-M171 & 0.0077 & 16.1 & 559 & 4.5 & $f_2$ \\
\hline241 & 2D-M249 & 0.117 & 1.5 & 278 & 95.3 & $f_2$ & 564 & 2D-M391 & 0.0073 & 20.2 & 631 & 3.4 & $f_2$ \\
\hline242 & 2D-M78 & 0.1165 & 1.1 & 113 & 68.5 & $f_2$ & 565 & 2D-M332 & 0.0066 & 19.0 & 616 & 5.5 & $f_2$ \\
\hline243 & 2D-M70 & 0.1162 & 1.1 & 101 & 57.4 & $f_2$ & 566 & 2D-M494 & 0.0062 & 21.2 & 637 & 5.1 & $f_2$ \\
\hline244 & 2D-M530 & 0.1158 & 17.4 & 599 & 17.4 & $f_2$ & 567 & 2D-M509 & 0.0057 & 19.7 & 620 & 4.8 & $f_2$ \\
\hline245 & 2D-M58 & 0.1149 & 1.3 & 214 & 63.5 & $f_2$ & 568 & 2D-M328 & 0.0055 & 17.5 & 600 & 3.5 & $f_2$ \\
\hline246 & 2D-M93 & 0.1146 & 1.5 & 273 & 88.8 & $f_2$ & 569 & 2D-M176 & 0.0041 & 16.8 & 574 & 2.7 & $f_2$ \\
\hline247 & 2D-M125 & 0.1145 & 1.5 & 260 & 78.1 & $f_2$ & 570 & 2D-M599 & 0.0028 & 1.0 & 53 & 1.0 & $f_2$ \\
\hline248 & 2D-M10 & 0.1143 & 1.7 & 302 & 86.0 & $f_2$ & 571 & 2D-M40 & 0.0026 & 1.7 & 304 & 1.7 & $f_2$ \\
\hline249 & 2D-M112 & 0.1143 & 1.3 & 194 & 72.4 & $f_2$ & 572 & 2D-M469 & 0.0021 & 1.1 & 106 & 1.1 & $f_2$ \\
\hline250 & 2D-M15 & 0.1138 & 1.7 & 303 & 86.0 & $f_2$ & 573 & 2D-M483 & 0.002 & 1.1 & 79 & 1.0 & $f_2$ \\
\hline251 & 2D-M149 & 0.1138 & 1.0 & 74 & 72.9 & $f_2$ & 574 & 2D-M565 & 0.002 & 1.0 & 50 & 1.0 & $f_2$ \\
\hline252 & 2D-M147 & 0.1138 & 1.0 & 73 & 72.9 & $f_2$ & 575 & 2D-M36 & 0.002 & 1.4 & 238 & 1.4 & $f_2$ \\
\hline253 & 2D-M294 & 0.1137 & 1.5 & 258 & 85.6 & $f_2$ & 576 & 2D-M560 & 0.0019 & 1.2 & 147 & 1.2 & $f_2$ \\
\hline254 & 2D-M178 & 0.1129 & 1.1 & 96 & 77.5 & $f_2$ & 577 & 2D-M573 & 0.0018 & 1.2 & 146 & 1.2 & $f_2$ \\
\hline255 & 2D-M551 & 0.1124 & 17.4 & 598 & 17.4 & $f_2$ & 578 & 2D-M441 & 0.0017 & 1.1 & 124 & 1.1 & $f_2$ \\
\hline256 & 2D-M123 & 0.1121 & 1.2 & 160 & 75.2 & $f_2$ & 579 & 2D-M39 & 0.0017 & 1.2 & 165 & 1.2 & $f_2$ \\
\hline257 & 2D-M2 & 0.1115 & 1.2 & 159 & 100.4 & $f_2$ & 580 & 2D-M563 & 0.0017 & 1.1 & 94 & 1.1 & $f_2$ \\
\hline258 & 2D-M119 & 0.1105 & 1.3 & 215 & 68.1 & $f_2$ & 581 & 2D-M576 & 0.0017 & 1.1 & 85 & 1.1 & $f_2$ \\
\hline259 & 2D-M624 & 0.1091 & 1.0 & 35 & 1.0 & $f_2$ & 582 & 2D-M575 & 0.0017 & 1.1 & 87 & 1.1 & $f_2$ \\
\hline260 & 2D-M290 & 0.1086 & 1.1 & 97 & 90.6 & $f_2$ & 583 & 2D-M587 & 0.0017 & 1.1 & 91 & 1.1 & $f_2$ \\
\hline261 & 2D-M1 & 0.106 & 1.9 & 309 & 74.0 & $f_2$ & 584 & 2D-M615 & 0.0016 & 1.0 & 71 & 1.0 & $f_2$ \\
\hline262 & 2D-M67 & 0.1059 & 1.5 & 264 & 79.0 & $f_2$ & 585 & 2D-M588 & 0.0016 & 1.1 & 86 & 1.1 & $f_2$ \\
\hline263 & 2D-M531 & 0.1058 & 17.6 & 605 & 17.5 & $f_2$ & 586 & 2D-M34 & 0.0016 & 1.5 & 261 & 1.0 & $f_2$ \\
\hline264 & 2D-M463 & 0.1045 & 10.5 & 360 & 9.5 & $f_1$ & 587 & 2D-M493 & 0.0016 & 1.1 & 90 & 1.1 & $f_2$ \\
\hline265 & 2D-M641 & 0.1036 & 1.0 & 42 & 1.0 & $f_2$ & 588 & 2D-M574 & 0.0016 & 1.0 & 12 & 1.0 & $f_2$ \\
\hline266 & 2D-M532 & 0.1028 & 17.4 & 597 & 17.4 & $f_2$ & 589 & 2D-M467 & 0.0016 & 1.1 & 126 & 1.1 & $f_2$ \\
\hline267 & 2D-M636 & 0.1026 & 1.0 & 33 & 1.0 & $f_2$ & 590 & 2D-M571 & 0.0016 & 1.0 & 2 & 1.0 & $f_2$ \\
\hline268 & 2D-M630 & 0.1021 & 1.0 & 45 & 1.0 & $f_2$ & 591 & 2D-M592 & 0.0016 & 1.7 & 299 & 1.0 & $f_2$ \\
\hline269 & 2D-M434 & 0.1012 & 10.5 & 361 & 9.5 & $f_1$ & 592 & 2D-M577 & 0.0015 & 1.2 & 138 & 0.9 & $f_2$ \\
\hline270 & 2D-M29 & 0.101 & 8.2 & 331 & 7.1 & $f_1$ & 593 & 2D-M605 & 0.0015 & 1.1 & 89 & 1.1 & $f_2$ \\
\hline271 & 2D-M637 & 0.1006 & 1.0 & 5 & 1.0 & $f_2$ & 594 & 2D-M604 & 0.0015 & 1.1 & 88 & 1.1 & $f_2$ \\
\hline272 & 2D-M233 & 0.099 & 2.5 & 320 & 82.4 & $f_2$ & 595 & 2D-M594 & 0.0015 & 1.0 & 8 & 1.0 & $f_2$ \\
\hline273 & 2D-M77 & 0.099 & 1.4 & 255 & 63.5 & $f_2$ & 596 & 2D-M598 & 0.0015 & 1.0 & 24 & 1.0 & $f_2$ \\
\hline274 & 2D-M55 & 0.0984 & 1.5 & 262 & 78.8 & $f_2$ & 597 & 2D-M610 & 0.0015 & 1.0 & 3 & 1 & $f_2$ \\
\hline275 & 2D-M553 & 0.097 & 16.8 & 575 & 16.5 & $f_2$ & 598 & 2D-M602 & 0.0015 & 1.0 & 60 & 1.0 & $f_2$ \\
\hline276 & 2D-M42 & 0.0964 & 1.4 & 221 & 60.2 & $f_2$ & 599 & 2D-M590 & 0.0015 & 1.0 & 59 & 1.0 & $f_2$ \\
\hline277 & 2D-M642 & 0.0962 & 1.0 & 9 & 111.0 & $f_1$ & 600 & 2D-M586 & 0.0015 & 1.0 & 58 & 1.0 & $f_2$ \\
\hline278 & 2D-M255 & 0.0945 & 1.8 & 308 & 76.7 & $f_2$ & 601 & 2D-M564 & 0.0015 & 1.0 & 55 & 1.0 & $f_2$ \\
\hline279 & 2D-M409 & 0.093 & 10.6 & 362 & 9.5 & $f_1$ & 602 & 2D-M603 & 0.0015 & 1.0 & 54 & 1.0 & $f_2$ \\
\hline280 & 2D-M620 & 0.0923 & 1.0 & 16 & 1.0 & $f_2$ & 603 & 2D-M618 & 0.0015 & 1.0 & 29 & 1.0 & $f_2$ \\
\hline281 & 2D-M452 & 0.0922 & 10.6 & 363 & 9.5 & $f_1$ & 604 & 2D-M457 & 0.0015 & 1.4 & 229 & 1.1 & $f_2$ \\
\hline282 & 2D-M471 & 0.091 & 11.6 & 403 & 10.5 & $f_1$ & 605 & 2D-M585 & 0.0015 & 1.0 & 23 & 1.0 & $f_2$ \\
\hline283 & 2D-M179 & 0.0906 & 1.0 & 78 & 62.8 & $f_2$ & 606 & 2D-M569 & 0.0015 & 1.0 & 17 & 1.0 & $f_2$ \\
\hline284 & 2D-M438 & 0.0901 & 9.2 & 344 & 8.1 & $f_1$ & 607 & 2D-M596 & 0.0014 & 1.0 & 21 & 1.0 & $f_2$ \\
\hline285 & 2D-M92 & 0.0898 & 1.5 & 267 & 62.1 & $f_2$ & 608 & 2D-M567 & 0.0014 & 1.0 & 19 & 1.0 & $f_2$ \\
\hline286 & 2D-M91 & 0.0896 & 1.4 & 231 & 49.5 & $f_2$ & 609 & 2D-M570 & 0.0014 & 1.0 & 1 & 1.0 & $f_2$ \\
\hline287 & 2D-M73 & 0.088 & 1.3 & 197 & 48.2 & $f_2$ & 610 & 2D-M606 & 0.0014 & 1.0 & 25 & 1.0 & $f_2$ \\
\hline288 & 2D-M622 & 0.0869 & 1.0 & 39 & 1.0 & $f_2$ & 611 & 2D-M595 & 0.0014 & 1.0 & 63 & 1.0 & $f_2$ \\
\hline289 & 2D-M365 & 0.0868 & 11.6 & 406 & 10.5 & $f_1$ & 612 & 2D-M583 & 0.0014 & 1.0 & 65 & 1.0 & $f_2$ \\
\hline290 & 2D-M482 & 0.0862 & 1.0 & 44 & 1.0 & $f_1$ & 613 & 2D-M562 & 0.0014 & 1.0 & 64 & 1.0 & $f_2$ \\
\hline291 & 2D-M547 & 0.0855 & 10.4 & 357 & 9.3 & $f_2$ & 614 & 2D-M600 & 0.0014 & 1.0 & 4 & 1.0 & $f_2$ \\
\hline292 & 2D-M426 & 0.0843 & 10.6 & 366 & 9.5 & $f_1$ & 615 & 2D-M619 & 0.0014 & 1.4 & 235 & 1.0 & $f_2$ \\
\hline293 & 2D-M27 & 0.0834 & 11.6 & 408 & 10.5 & $f_1$ & 616 & 2D-M614 & 0.0014 & 1.4 & 234 & 1.0 & $f_2$ \\
\hline294 & 2D-M538 & 0.0833 & 11.8 & 416 & 10.1 & $f_1$ & 617 & 2D-M459 & 0.0014 & 1.0 & 77 & 1.0 & $f_2$ \\
\hline295 & 2D-M495 & 0.0823 & 11.6 & 409 & 10.5 & $f_1$ & 618 & 2D-M33 & 0.0013 & 1.4 & 237 & 1.1 & $f_2$ \\
\hline296 & 2D-M536 & 0.0805 & 19.8 & 622 & 19.8 & $f_2$ & 619 & 2D-M445 & 0.0012 & 1.1 & 110 & 0.8 & $f_2$ \\
\hline297 & 2D-M373 & 0.0742 & 11.7 & 412 & 10.5 & $f_1$ & 620 & 2D-M444 & 0.0012 & 1.5 & 274 & 0.9 & $f_2$ \\
\hline298 & 2D-M280 & 0.0736 & 11.7 & 413 & 10.5 & $f_1$ & 621 & 2D-M37 & 0.0012 & 1.2 & 166 & 0.8 & $f_2$ \\
\hline299 & 2D-M476 & 0.073 & 11.7 & 414 & 10.5 & $f_1$ & 622 & 2D-M38 & 0.0012 & 1.2 & 167 & 0.8 & $f_2$ \\
\hline300 & 2D-M377 & 0.0705 & 10.8 & 369 & 9.5 & $f_1$ & 623 & 2D-M443 & 0.0012 & 1.2 & 170 & 0.7 & $f_2$ \\
\hline301 & 2D-M253 & 0.0693 & 11.8 & 415 & 10.5 & $f_1$ & 624 & 2D-M440 & 0.0012 & 2.6 & 322 & 0.9 & $f_2$ \\
\hline302 & 2D-M540 & 0.0692 & 20.2 & 629 & 20.2 & $f_2$ & 625 & 2D-M593 & 0.0012 & 1.3 & 200 & 0.8 & $f_2$ \\
\hline303 & 2D-M539 & 0.067 & 20.2 & 630 & 20.2 & $f_2$ & 626 & 2D-M611 & 0.001 & 1.4 & 232 & 0.6 & $f_2$ \\
\hline304 & 2D-M549 & 0.0656 & 20.2 & 626 & 20.2 & $f_2$ & 627 & 2D-M481 & 0.001 & 1.0 & 69 & 0.7 & $f_2$ \\
\hline305 & 2D-M552 & 0.0605 & 20.2 & 627 & 20.2 & $f_2$ & 628 & 2D-M616 & 0.001 & 1.6 & 289 & 0.6 & $f_2$ \\
\hline306 & 2D-M537 & 0.0603 & 20.2 & 628 & 20.2 & $f_2$ & 629 & 2D-M442 & 0.001 & 2.2 & 317 & 0.6 & $f_2$ \\
\hline307 & 2D-M533 & 0.0579 & 9.0 & 336 & 6.4 & $f_1$ & 630 & 2D-M568 & 0.0009 & 1.3 & 187 & 0.6 & $f_2$ \\
\hline308 & 2D-M32 & 0.0565 & 1.0 & 22 & 1.0 & $f_1$ & 631 & 2D-M582 & 0.0009 & 1.3 & 196 & 0.6 & $f_2$ \\
\hline309 & 2D-M633 & 0.0525 & 1.0 & 46 & 1.0 & $f_2$ & 632 & 2D-M617 & 0.0009 & 1.3 & 188 & 0.6 & $f_2$ \\
\hline310 & 2D-M219 & 0.0514 & 8.8 & 333 & 7.1 & $f_1$ & 633 & 2D-M580 & 0.0009 & 1.3 & 186 & 0.6 & $f_2$ \\
\hline311 & 2D-M422 & 0.0484 & 10.1 & 350 & 8.4 & $f_1$ & 634 & 2D-M561 & 0.0009 & 2.6 & 323 & 0.6 & $f_2$ \\
\hline312 & 2D-M492 & 0.0458 & 1.0 & 10 & 1 & $f_1$ & 635 & 2D-M578 & 0.0008 & 1.5 & 275 & 0.5 & $f_2$ \\
\hline313 & 2D-M379 & 0.0441 & 12.2 & 433 & 10.5 & $f_1$ & 636 & 2D-M566 & 0.0008 & 1.4 & 252 & 0.5 & $f_2$ \\
\hline314 & 2D-M487 & 0.0401 & 12.3 & 436 & 10.5 & $f_1$ & 637 & 2D-M608 & 0.0008 & 1.4 & 251 & 0.5 & $f_2$ \\
\hline315 & 2D-M420 & 0.0335 & 14.1 & 512 & 14.2 & $f_2$ & 638 & 2D-M581 & 0.0008 & 1.3 & 210 & 0.6 & $f_2$ \\
\hline316 & 2D-M589 & 0.0333 & 1.0 & 37 & 1.0 & $f_1$ & 639 & 2D-M584 & 0.0007 & 1.4 & 250 & 0.5 & $f_2$ \\
\hline317 & 2D-M613 & 0.0326 & 1.0 & 47 & 1.0 & $f_1$ & 640 & 2D-M612 & 0.0007 & 1.4 & 245 & 0.5 & $f_2$ \\
\hline318 & 2D-M498 & 0.032 & 17.2 & 580 & 17.4 & $f_2$ & 641 & 2D-M579 & 0.0007 & 1.4 & 243 & 0.5 & $f_2$ \\
\hline319 & 2D-M352 & 0.0318 & 17.3 & 585 & 17.3 & $f_2$ & 642 & 2D-M591 & 0.0007 & 1.4 & 256 & 0.5 & $f_2$ \\
\hline320 & 2D-M157 & 0.0297 & 20.8 & 636 & 20.1 & $f_2$ & 643 & 2D-M572 & 0.0007 & 1.4 & 239 & 0.5 & $f_2$ \\
\hline321 & 2D-M262 & 0.0296 & 11.2 & 388 & 18.1 & $f_2$ & 644 & 2D-M491 & 0.0007 & 1.3 & 203 & 0.5 & $f_2$ \\
\hline322 & 2D-M218 & 0.0294 & 17.0 & 579 & 16.8 & $f_2$ & 645 & 2D-M607 & 0.0006 & 1.6 & 282 & 0.4 & $f_2$ \\
\hline323 & 2D-M542 & 0.0293 & 16.8 & 573 & 15.8 & $f_2$ &  &  &  &  &  &  &  \\
\hline
\caption{Manipulability and Condition Numbers of 2-DOF Manipulators}
\label{Tab:table_dof2mt_1}  \end{longtable}
\normalsize
%}

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulabilitytable_new3.tex <==
\begin{table}[h]  \centering \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ \\ 
\hline
1 & 3D-M1 & 1.0113 & 1.5 & 2 & 1058.9 & $f_1$ \\
\hline2 & 3D-M8 & 1.0 & 1.0 & 1 & 1.0 & $f_1$ \\
\hline3 & 3D-M2 & 0.0962 & 14.8 & 4 & 111.0 & $f_1$ \\
\hline4 & 3D-M3 & 0.0962 & 15.5 & 8 & 111.0 & $f_1$ \\
\hline5 & 3D-M4 & 0.0962 & 14.8 & 7 & 111.0 & $f_1$ \\
\hline6 & 3D-M7 & 0.0091 & 14.8 & 5 & 10.5 & $f_1$ \\
\hline7 & 3D-M5 & 0.0091 & 14.8 & 6 & 10.5 & $f_1$ \\
\hline8 & 3D-M6 & 0.0091 & 14.8 & 3 & 10.5 & $f_1$ \\
\hline\end{tabular} \caption{Prescription of 3-DOF Manipulators.} \label{Tab:table_dof3mt_1} \end{table}

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulabilitytable_new4.tex <==
\begin{table}[h]  \centering \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ \\ 
\hline
1 & 4D-M1 & 2.5607 & 1.5 & 1 & 2074.5 & $f_1$ \\
\hline2 & 4D-M13 & 0.4866 & 3.0 & 2 & 1.0 & $f_1$ \\
\hline3 & 4D-M12 & 0.4048 & 3.1 & 3 & 1 & $f_1$ \\
\hline4 & 4D-M4 & 0.2619 & 15.3 & 14 & 211.0 & $f_1$ \\
\hline5 & 4D-M5 & 0.2619 & 15.3 & 13 & 211.0 & $f_1$ \\
\hline6 & 4D-M2 & 0.2619 & 15.3 & 12 & 211.0 & $f_1$ \\
\hline7 & 4D-M3 & 0.2619 & 15.3 & 15 & 211.0 & $f_1$ \\
\hline8 & 4D-M15 & 0.077 & 4.9 & 4 & 1.0 & $f_1$ \\
\hline9 & 4D-M14 & 0.0538 & 5.5 & 5 & 1.0 & $f_1$ \\
\hline10 & 4D-M9 & 0.0253 & 12.9 & 7 & 17.6 & $f_1$ \\
\hline11 & 4D-M11 & 0.0253 & 12.9 & 10 & 17.6 & $f_1$ \\
\hline12 & 4D-M10 & 0.0253 & 12.9 & 6 & 17.6 & $f_1$ \\
\hline13 & 4D-M7 & 0.0253 & 12.9 & 8 & 17.6 & $f_1$ \\
\hline14 & 4D-M8 & 0.0253 & 12.9 & 9 & 17.6 & $f_1$ \\
\hline15 & 4D-M6 & 0.0253 & 12.9 & 11 & 17.6 & $f_1$ \\
\hline\end{tabular} \caption{Prescription of 4-DOF Manipulators.} \label{Tab:table_dof4mt_1} \end{table}

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulators/dof1/manipulator_3.tex <==
% \emph{Adjacency matrix of manipulator 1D-M3:}

% The adjacency of the manipulator is\[M_{\text{1D-M3}}=\left[\begin{matrix}L_{1}&O&R&C\\O&L_{2}&R&S\\R&R&L_{3}&O\\C&S&O&L_{4}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline


\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/1dof/3.png}
  \caption{Schematic figure of 1D-M3}
  \label{fig_iext_3}
\end{figure}


\emph{Formulation of Jacobian:}

Jacobian of the manipulator is formulated using the steps shown in section \ref{steps_to_formulate_jacobian}. From figure \ref{fig_iext_3}, the various paths that connect the base link and the end-effector link are $L_1-R-L_3-R-L_2-S-L_4$ and $L_1-C-L_4$. The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.


\begin{eqnarray}\label{eqn:eqn_1_3_1_2}\vec{v}=\dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{32} \hat{n}_{32} \times \left( \vec{a} - \vec{r}_{32} \right) + \vec{\omega}_{24} \times \left( \vec{a} - \vec{r}_{24} \right)\end{eqnarray}\begin{eqnarray}\label{eqn:eqn_1_3_1_1}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{d}_{14} \hat{n}_{14}\end{eqnarray}
\begin{dmath}\label{eqn:eqn_1_3_2_2}\vec{\omega}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{32} \hat{n}_{32} + \vec{\omega}_{24}\end{dmath}\begin{dmath}\label{eqn:eqn_1_3_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14}\end{dmath}where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{ij}=\begin{Bmatrix} \omega_{ijx} & \omega_{ijy} & \omega_{ijz} \end{Bmatrix}^T$ represents the relative angular velocity vector of the link $L_j$ relative to the link $L_i$, of the adjacency matrix. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_1_3_1_1} and \eqref{eqn:eqn_1_3_2_1}, the vector of end-effector velocities in terms of both active and passive joint angles is given by
\newline

$$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}0 & n_{14x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 & 0\\0 & n_{14y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & 0 & 0\\0 & n_{14z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & 0 & 0\\0 & 0 & n_{14x} & 0 & 0 & 0 & 0\\0 & 0 & n_{14y} & 0 & 0 & 0 & 0\\0 & 0 & n_{14z} & 0 & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}$$


$$\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}0\\0\\0\\0\\0\\0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\end{Bmatrix}+\left[\begin{matrix}n_{14x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 & 0\\n_{14y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & 0 & 0\\n_{14z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & 0 & 0\\0 & n_{14x} & 0 & 0 & 0 & 0\\0 & n_{14y} & 0 & 0 & 0 & 0\\0 & n_{14z} & 0 & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}$$

\[\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[J_1\right]\{\dot{\theta}_a\}+\left[J_2\right]\{\Omega\}\]where $\{\dot{\theta}_a\}=\begin{Bmatrix}\dot{\theta}_{13}\end{Bmatrix}$ and $\{\Omega\}=\begin{Bmatrix}\dot{d}_{14} & \dot{\theta}_{14}&\dot{\theta}_{32}&\omega_{24x}&\omega_{24y}&\omega_{24z}\end{Bmatrix}^T$ represent the active joint-velocities and the passive joint-velocities, respectively.
\newline
But since the Jacobian should contain the end-effector velocities in terms of active joint angles alone, the passive joint angles must be written in terms of active joint angles. From the two equations \eqref{eqn:eqn_1_3_1_1} and \eqref{eqn:eqn_1_3_1_2}, 
\newline
\begin{eqnarray}
  \label{eqn:eqn_1_3_5_1}
  \dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{32} \hat{n}_{32} \times \left( \vec{a} - \vec{r}_{32} \right) + \vec{\omega}_{24} \times \left( \vec{a} - \vec{r}_{24} \right)=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{d}_{14} \hat{n}_{14}\end{eqnarray}

From the two equations \eqref{eqn:eqn_1_3_2_1} and \eqref{eqn:eqn_1_3_2_2},
\newline
\begin{dmath}
  \label{eqn:eqn_1_3_5_2}
  \dot{\theta}_{14} \hat{n}_{14}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{32} \hat{n}_{32} + \vec{\omega}_{24}\end{dmath}
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & - n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & - n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\n_{13x} & 0 & - n_{14x} & n_{32x} & 1 & 0 & 0\\n_{13y} & 0 & - n_{14y} & n_{32y} & 0 & 1 & 0\\n_{13z} & 0 & - n_{14z} & n_{32z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
%\newline
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right)\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right)\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right)\\n_{13x}\\n_{13y}\\n_{13z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\end{Bmatrix}+\left[\begin{matrix}- n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\- n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\- n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\0 & - n_{14x} & n_{32x} & 1 & 0 & 0\\0 & - n_{14y} & n_{32y} & 0 & 1 & 0\\0 & - n_{14z} & n_{32z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
From the equations \eqref{eqn:eqn_1_3_5_1} and \eqref{eqn:eqn_1_3_5_2}, linear equations in terms of active and passive joint angles can be stacked as shown below, using which the passive joint angles can be written in terms of the active joint angles.
\[
\begin{split}
  %%\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & - n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & - n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\n_{13x} & 0 & - n_{14x} & n_{32x} & 1 & 0 & 0\\n_{13y} & 0 & - n_{14y} & n_{32y} & 0 & 1 & 0\\n_{13z} & 0 & - n_{14z} & n_{32z} & 0 & 0 & 1\end{matrix}\right]
  %\Rightarrow
  \left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & - n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) \\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) \\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & - n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) \\n_{13x} & 0 & - n_{14x} \\n_{13y} & 0 & - n_{14y} \\n_{13z} & 0 & - n_{14z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\ - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\ n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\ n_{32x} & 1 & 0 & 0\\ n_{32y} & 0 & 1 & 0\\ n_{32z} & 0 & 0 & 1\end{matrix}\right]
  %\Rightarrow\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & - n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) \\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) \\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & - n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) \\n_{13x} & 0 & - n_{14x} & n_{32x} \\n_{13y} & 0 & - n_{14y} & n_{32y} \\n_{13z} & 0 & - n_{14z} & n_{32z} \end{matrix}\right.\\\qquad\left.\begin{matrix} 0 & a_z - r_{24z} & - a_y + r_{24y}\\ - a_z + r_{24z} & 0 & a_x - r_{24x}\\ a_y - r_{24y} & - a_x + r_{24x} & 0\\ 1 & 0 & 0\\ 0 & 1 & 0\\ 0 & 0 & 1\end{matrix}\right]
  \begin{Bmatrix}\dot{\theta}_{13}\\\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}
  =
  \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
\end{split}
\]

\[
\begin{split}
  \Rightarrow\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right)\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right)\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right)\\n_{13x}\\n_{13y}\\n_{13z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\end{Bmatrix}
  +
  %\left[\begin{matrix}- n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\- n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\- n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\0 & - n_{14x} & n_{32x} & 1 & 0 & 0\\0 & - n_{14y} & n_{32y} & 0 & 1 & 0\\0 & - n_{14z} & n_{32z} & 0 & 0 & 1\end{matrix}\right]
  \left[\begin{matrix}- n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) \\- n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) \\- n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) \\0 & - n_{14x} \\0 & - n_{14y} \\0 & - n_{14z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\ - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\ n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\ n_{32x} & 1 & 0 & 0\\ n_{32y} & 0 & 1 & 0\\ n_{32z} & 0 & 0 & 1\end{matrix}\right]
  \begin{Bmatrix}\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}
  =
  \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
\end{split}
\]

\[\Rightarrow \left[A_1\right]\{\dot{\theta}_a\}+\left[A_2\right]\{\Omega\}=0\] \[\Rightarrow \{\Omega\}=-\left[A_2\right]^{-1}\left[A_1\right]\{\dot{\theta}_a\}\]\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}=\left[J_1\right] \{\dot{\theta}_a\}+\left[J_2\right] \{\Omega\}=\left[J_1\right] \{\dot{\theta}_a\}-\left[J_2\right]\left[A_2\right]^{-1}\left[A_1\right] \{\dot{\theta}_a\}\]



The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$ would finally be

$$\left[J_1\right]=\left[\begin{matrix}0\\0\\0\\0\\0\\0\end{matrix}\right]$$

$$\left[J_2\right]=\left[\begin{matrix}\sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & 0 & 0 & 0 & 0\\\sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0 & 0 & 0 & 0\\\cos{\left(\beta_{14} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0 & 0 & 0 & 0\\0 & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0 & 0 & 0 & 0\\0 & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & 0 & 0 & 0 & 0\\0 & \cos{\left(\beta_{14} \right)} & 0 & 0 & 0 & 0\end{matrix}\right]$$

$$\left[A_1\right]=\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)}\\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)}\\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)}\\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)}\\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)}\\\cos{\left(\beta_{13} \right)}\end{matrix}\right]$$

%\resizebox{\textwidth}{!}{$\left[A_2\right]=\left[\begin{matrix}- \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 5 - r_{24z} & r_{24y} - 4\\- \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & r_{24z} - 5 & 0 & 3 - r_{24x}\\- \cos{\left(\beta_{14} \right)} & \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} - \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 4 - r_{24y} & r_{24x} - 3 & 0\\0 & - \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 1 & 0 & 0\\0 & - \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 1 & 0\\0 & - \cos{\left(\beta_{14} \right)} & \cos{\left(\beta_{32} \right)} & 0 & 0 & 1\end{matrix}\right]$}
\[
\begin{split}
  \left[A_2\right]
  =
  %\left[\begin{matrix}- \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 5 - r_{24z} & r_{24y} - 4\\- \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & r_{24z} - 5 & 0 & 3 - r_{24x}\\- \cos{\left(\beta_{14} \right)} & \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} - \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 4 - r_{24y} & r_{24x} - 3 & 0\\0 & - \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 1 & 0 & 0\\0 & - \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 1 & 0\\0 & - \cos{\left(\beta_{14} \right)} & \cos{\left(\beta_{32} \right)} & 0 & 0 & 1\end{matrix}\right]
  \left[\begin{matrix}- \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} \\- \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\- \cos{\left(\beta_{14} \right)} & \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} - \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\0 & - \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\0 & - \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} \\0 & - \cos{\left(\beta_{14} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 5 - r_{24z} & r_{24y} - 4\\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & r_{24z} - 5 & 0 & 3 - r_{24x}\\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 4 - r_{24y} & r_{24x} - 3 & 0\\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 1 & 0 & 0\\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 1 & 0\\ \cos{\left(\beta_{32} \right)} & 0 & 0 & 1\end{matrix}\right]
\end{split}
\]

By using the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$, the relation between the active joint velocities and the end-effector velocities can be written as

\[
  %\Rightarrow
  \{\dot{X}\}=\left( \left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] \right) \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]
  
  where $\left[\widetilde{J}\right]=\left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] $ is the Jacobian matrix of the manipulator for the considered actuating joints.
\newline


$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$
Based on the strategy mentioned in section \ref{strategy_used_in_optimisation}, the above optimisation problem is attempted for solution, but it did not pass the criterion mentioned in Step 1. Hence, the modified objective function is taken for optimisation in order to avoid type-2 singularity. The modified optimisation problem would then become
\newline
Maximise\[f_2=\sqrt{\det{\left(\left[\widetilde{A}\right]^T \left[\widetilde{A}\right]\right)} \times \det{\left(\left[\widetilde{B}\right]^T \left[\widetilde{B}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$

\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{13}-\vec{a}\right)\times \hat{n}_{13}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{32}-\vec{a}\right)\times \hat{n}_{32}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{4}=\left|\vec{r}_{24}-\vec{a}\right|  
\end{matrix}
$$

The characteristic length is formulated as follows.
\[L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}+\bar{d}_{4}}{4}\]

By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
\[\left[S\right]=\begin{bmatrix}
  \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
  0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
  0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
  0 & 0 & 0 & 1 & 0 & 0\\
  0 & 0 & 0 & 0 & 1 & 0\\
  0 & 0 & 0 & 0 & 0 & 1\\
  \end{bmatrix}\]
  
  The scaled Jacobian matrix can then be calculated as
  \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
  The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.

\emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in table \ref{Tab:table_3_3} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{13}$ & $\ang{182.04}$ \\
\hline$\phi_{14}$ & $\ang{133.78}$ \\
\hline$\phi_{32}$ & $\ang{245.33}$ \\
\hline$r_{13x}$ & $10.0$ \\
\hline$r_{13y}$ & $10.0$ \\
\hline$r_{13z}$ & $0.0$ \\
\hline$r_{14x}$ & $0.0$ \\
\hline$r_{14y}$ & $0.0$ \\
\hline$r_{14z}$ & $0.0$ \\
\hline$r_{32x}$ & $10.0$ \\
\hline$r_{32y}$ & $0.0$ \\
\hline$r_{32z}$ & $0.0$ \\
\hline$r_{24x}$ & $0.0$ \\
\hline$r_{24y}$ & $10.0$ \\
\hline$r_{24z}$ & $10.0$ \\
\hline$\beta_{13}$ & $\ang{134.98}$ \\
\hline$\beta_{14}$ & $\ang{100.15}$ \\
\hline$\beta_{32}$ & $\ang{63.84}$ \\
\hline\end{tabular} \caption{Result (1D-M3)} \label{Tab:table_3_3} \end{table}
% \begin{table}[h]  \centering \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% Variable & $\phi_{13}$ & $\phi_{14}$ & $\phi_{32}$ & $r_{13x}$ & $r_{13y}$ & $r_{13z}$ & $r_{14x}$ & $r_{14y}$ & $r_{14z}$ & $r_{32x}$ & $r_{32y}$ & $r_{32z}$ & $r_{24x}$ & $r_{24y}$ & $r_{24z}$ & $\beta_{13}$ & $\beta_{14}$ & $\beta_{32}$\\ 
% \hline
% Value & $\ang{182.04}$ & $\ang{133.78}$ & $\ang{245.33}$ & $10.0$ & $10.0$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ & $10.0$ & $0.0$ & $0.0$ & $0.0$ & $10.0$ & $10.0$ & $\ang{134.98}$ & $\ang{100.15}$ & $\ang{63.84}$ \\
% \hline\end{tabular} \caption{Result (1D-M3)} \label{Tab:table_3_3} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{13}=-0.03\hat{i}-0.71\hat{j}-0.71\hat{k} \\
  \hat{n}_{14}=0.71\hat{i}-0.68\hat{j}-0.18\hat{k} \\
  \hat{n}_{32}=-0.82\hat{i}-0.37\hat{j}+0.44\hat{k} \\
  \vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{32}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=15.37\]
And the corresponding condition number is \[\kappa=1\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.0222\]

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulators/dof2/manipulator_1.tex <==
% \emph{Adjacency matrix of manipulator 2D-M1:}

% The adjacency of the manipulator is\[M_{\text{2D-M1}}=\left[\begin{matrix}L_{1}&O&O&R&O\\O&L_{2}&O&R&R\\O&O&L_{3}&S&S\\R&R&S&L_{4}&O\\O&R&S&O&L_{5}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline

\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/2dof/1.png}
  \caption{Schematic figure of 2D-M1}
  \label{fig_2dof_iext_1}
\end{figure}

\emph{Formulation of Jacobian:}

Jacobian of the manipulator is formulated using the steps shown in section \ref{steps_to_formulate_jacobian}. The various paths that connect the base link and the end-effector link are $L_1-R-L_4-R-L_2-R-L_5$ and $L_1-R-L_4-S-L_3-S-L_5$. The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.

%The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.

\begin{eqnarray}\label{eqn:eqn_2_1_1_2}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{\theta}_{42} \hat{n}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}\begin{eqnarray}\label{eqn:eqn_2_1_1_1}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{43} \times \left( \vec{a} - \vec{r}_{43} \right) + \vec{\omega}_{35} \times \left( \vec{a} - \vec{r}_{35} \right)\end{eqnarray}\begin{dmath}\label{eqn:eqn_2_1_2_2}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \dot{\theta}_{42} \hat{n}_{42} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}\begin{dmath}\label{eqn:eqn_2_1_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{43} + \vec{\omega}_{35}\end{dmath}where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{ij}=\begin{Bmatrix} \omega_{ijx} & \omega_{ijy} & \omega_{ijz} \end{Bmatrix}^T$ represents the relative angular velocity vector of the link $L_j$ relative to the link $L_i$, of the adjacency matrix. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_2_1_1_1} and \eqref{eqn:eqn_2_1_2_1}, the vector of end-effector velocities in terms of both active and passive joint angles is given by
\newline
%\resizebox{\textwidth}{!}{$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 & a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & - a_z + r_{43z} & 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & a_y - r_{43y} & - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\n_{14x} & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0\\n_{14y} & 0 & 0 & 0 & 1 & 0 & 0 & 1 & 0\\n_{14z} & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\\\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}$}


%\resizebox{\textwidth}{!}{$\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0\\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0\\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0\\n_{14x} & 0\\n_{14y} & 0\\n_{14z} & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}+\left[\begin{matrix}0 & 0 & a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\0 & - a_z + r_{43z} & 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\0 & a_y - r_{43y} & - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\0 & 1 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}$}

\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    \begin{Bmatrix} \vec{v} \\ \vec{\omega} \end{Bmatrix}
    =
    %\left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 & a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & - a_z + r_{43z} & 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & a_y - r_{43y} & - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\n_{14x} & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0\\n_{14y} & 0 & 0 & 0 & 1 & 0 & 0 & 1 & 0\\n_{14z} & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]
    \left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 \\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & - a_z + r_{43z} \\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & a_y - r_{43y} \\n_{14x} & 0 & 0 & 1 \\n_{14y} & 0 & 0 & 0 \\n_{14z} & 0 & 0 & 0 \end{matrix}\right.\\\qquad\left.\begin{matrix} a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\ 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\ - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\ 0 & 0 & 1 & 0 & 0\\ 1 & 0 & 0 & 1 & 0\\ 0 & 1 & 0 & 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\\\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}
\end{split}
%$}
\]

\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    \Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}
    =
    \left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0\\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0\\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0\\n_{14x} & 0\\n_{14y} & 0\\n_{14z} & 0\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}
    +
    %\left[\begin{matrix}0 & 0 & a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\0 & - a_z + r_{43z} & 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\0 & a_y - r_{43y} & - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\0 & 1 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]
    \left[\begin{matrix}0 & 0 & a_z - r_{43z} \\0 & - a_z + r_{43z} & 0 \\0 & a_y - r_{43y} & - a_x + r_{43x} \\0 & 1 & 0 \\0 & 0 & 1 \\0 & 0 & 0 \end{matrix}\right.\\\qquad\left.\begin{matrix} - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\ a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\ 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\ 0 & 1 & 0 & 0\\ 0 & 0 & 1 & 0\\ 1 & 0 & 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}
  \end{split}
  %$}
\]

\[\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[J_1\right]\{\dot{\theta}_a\}+\left[J_2\right]\{\Omega\}\]where $\{\dot{\theta}_a\}=\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}$ and $\{\Omega\}=\begin{Bmatrix}\dot{\theta}_{25}&\omega_{43x}&\omega_{43y}&\omega_{43z}&\omega_{35x}&\omega_{35y}&\omega_{35z}\end{Bmatrix}^T$ represent the active joint-velocities and the passive joint-velocities, respectively.
\newline
But since the Jacobian should contain the end-effector velocities in terms of active joint angles alone, the passive joint angles must be written in terms of active joint angles. From the two equations \eqref{eqn:eqn_2_1_1_1} and \eqref{eqn:eqn_2_1_1_2},
\newline
\begin{eqnarray}
  \label{eqn:eqn_2_1_5_1}
  \dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{\theta}_{42} \hat{n}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{43} \times \left( \vec{a} - \vec{r}_{43} \right) + \vec{\omega}_{35} \times \left( \vec{a} - \vec{r}_{35} \right)
\end{eqnarray}
From the two equations \eqref{eqn:eqn_2_1_2_1} and \eqref{eqn:eqn_2_1_2_2},
\newline
\begin{dmath}
  \label{eqn:eqn_2_1_5_2}
  \dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{43} + \vec{\omega}_{35}=\dot{\theta}_{14} \hat{n}_{14} + \dot{\theta}_{42} \hat{n}_{42} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}
For this mechanism, there is a superfluous degree of freedom for the link $L_3$. To avoid uncertainty of the velocity of the link during calculations, an additional constraint is considered as shown below, which does not alter the final velocity of the end-effector.
\begin{eqnarray} 
  \label{eq:superfluous_dof_equation}
  \vec{\omega}_{3}\cdot\left(\vec{r}_{35}-\vec{r}_{43}\right)=0
\end{eqnarray}
\[ \Rightarrow \left(r_{43x} - r_{35x}\right) \left(n_{14x} \dot{\theta}_{14} + \omega_{43x}\right) + \left(r_{43y} - r_{35y}\right) \left(n_{14y} \dot{\theta}_{14} + \omega_{43y}\right) + \left(r_{43z} - r_{35z}\right) \left(n_{14z} \dot{\theta}_{14} + \omega_{43z}\right)=0 \]

%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right) & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} & a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right) & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 & - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right) & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} & 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\0 & n_{42x} & n_{25x} & -1 & 0 & 0 & -1 & 0 & 0\\0 & n_{42y} & n_{25y} & 0 & -1 & 0 & 0 & -1 & 0\\0 & n_{42z} & n_{25z} & 0 & 0 & -1 & 0 & 0 & -1\\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0 & 0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} & r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\\\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\\0\end{Bmatrix}$}
%\newline
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right)\\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right)\\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right)\\0 & n_{42x}\\0 & n_{42y}\\0 & n_{42z}\\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}+\left[\begin{matrix}n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} & a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\- n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 & - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} & 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\n_{25x} & -1 & 0 & 0 & -1 & 0 & 0\\n_{25y} & 0 & -1 & 0 & 0 & -1 & 0\\n_{25z} & 0 & 0 & -1 & 0 & 0 & -1\\0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} & r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\\0\end{Bmatrix}$}
From the equations \eqref{eqn:eqn_2_1_5_1}, \eqref{eqn:eqn_2_1_5_2} and \eqref{eq:superfluous_dof_equation}, linear equations in terms of active and passive joint angles can be stacked as shown below, using which the passive joint angles can be written in terms of the active joint angles.
\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
  %\left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right) & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} & a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right) & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 & - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right) & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} & 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\0 & n_{42x} & n_{25x} & -1 & 0 & 0 & -1 & 0 & 0\\0 & n_{42y} & n_{25y} & 0 & -1 & 0 & 0 & -1 & 0\\0 & n_{42z} & n_{25z} & 0 & 0 & -1 & 0 & 0 & -1\\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0 & 0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} & r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]
  %\Rightarrow
  \left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right) \\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right) \\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right) \\0 & n_{42x} \\0 & n_{42y} \\0 & n_{42z} \\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0 \end{matrix}\right.
  \\
  \qquad
  \left.\begin{matrix} n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} \\ - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 \\ n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} \\ n_{25x} & -1 & 0 \\ n_{25y} & 0 & -1 \\ n_{25z} & 0 & 0 \\ 0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} \end{matrix}\right.
  \\
  \qquad
  \left.\begin{matrix} a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\ - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\ 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\ 0 & -1 & 0 & 0\\ 0 & 0 & -1 & 0\\ -1 & 0 & 0 & -1\\ r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]
\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\\\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}
=
\begin{Bmatrix}0\\0\\0\\0\\0\\0\\0\end{Bmatrix}
\end{split}
%$}
\]



\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
  \Rightarrow \left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right)\\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right)\\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right)\\0 & n_{42x}\\0 & n_{42y}\\0 & n_{42z}\\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0\end{matrix}\right]
  \begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}
  + \\
  \left[\begin{matrix}n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} \\- n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 \\n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} \\n_{25x} & -1 & 0 \\n_{25y} & 0 & -1 \\n_{25z} & 0 & 0 \\0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} \end{matrix}\right.\\\qquad\left.\begin{matrix} a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\ - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\ 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\ 0 & -1 & 0 & 0\\ 0 & 0 & -1 & 0\\ -1 & 0 & 0 & -1\\ r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]
  \begin{Bmatrix}\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}
  =
  \begin{Bmatrix}0\\0\\0\\0\\0\\0\\0\end{Bmatrix}
\end{split}
%$}
\]

\[\Rightarrow \left[A_1\right]\{\dot{\theta}_a\}+\left[A_2\right]\{\Omega\}=0\] \[\Rightarrow \{\Omega\}=-\left[A_2\right]^{-1}\left[A_1\right]\{\dot{\theta}_a\}\]\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}=\left[J_1\right] \{\dot{\theta}_a\}+\left[J_2\right] \{\Omega\}=\left[J_1\right] \{\dot{\theta}_a\}-\left[J_2\right]\left[A_2\right]^{-1}\left[A_1\right] \{\dot{\theta}_a\}\]
The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$ would finally be

%\resizebox{\textwidth}{!}{$
$$\left[J_1\right]=\left[\begin{matrix}- \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & 0\\\left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0\\- \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0\\\sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0\\\sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & 0\\\cos{\left(\beta_{14} \right)} & 0\end{matrix}\right]$$
%$}

%\resizebox{\textwidth}{!}{$
$$\left[J_2\right]=\left[\begin{matrix}0 & 0 & 5 - r_{43z} & r_{43y} - 4 & 0 & 5 - r_{35z} & r_{35y} - 4\\0 & r_{43z} - 5 & 0 & 3 - r_{43x} & r_{35z} - 5 & 0 & 3 - r_{35x}\\0 & 4 - r_{43y} & r_{43x} - 3 & 0 & 4 - r_{35y} & r_{35x} - 3 & 0\\0 & 1 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]$$
%$}

%\resizebox{\textwidth}{!}{$\left[A_1\right]=\left[\begin{matrix}0 & - \left(4 - r_{42y}\right) \cos{\left(\beta_{42} \right)} + \left(5 - r_{42z}\right) \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)}\\0 & \left(3 - r_{42x}\right) \cos{\left(\beta_{42} \right)} - \left(5 - r_{42z}\right) \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\0 & - \left(3 - r_{42x}\right) \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)} + \left(4 - r_{42y}\right) \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\0 & \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\0 & \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)}\\0 & \cos{\left(\beta_{42} \right)}\\\left(r_{43x} - r_{35x}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} + \left(r_{43y} - r_{35y}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(r_{43z} - r_{35z}\right) \cos{\left(\beta_{14} \right)} & 0\end{matrix}\right]$}

%\resizebox{\textwidth}{!}{$\left[A_2\right]=\left[\begin{matrix}- \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & 0 & r_{43z} - 5 & 4 - r_{43y} & 0 & r_{35z} - 5 & 4 - r_{35y}\\\left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & 5 - r_{43z} & 0 & r_{43x} - 3 & 5 - r_{35z} & 0 & r_{35x} - 3\\- \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & r_{43y} - 4 & 3 - r_{43x} & 0 & r_{35y} - 4 & 3 - r_{35x} & 0\\\sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & -1 & 0 & 0 & -1 & 0 & 0\\\sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & 0 & -1 & 0 & 0 & -1 & 0\\\cos{\left(\beta_{25} \right)} & 0 & 0 & -1 & 0 & 0 & -1\\0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} & r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]$}

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
  \left[A_1\right]=\left[\begin{matrix}0 \\0 \\0 \\0 \\0 \\0 \\\left(r_{43x} - r_{35x}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} + \left(r_{43y} - r_{35y}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(r_{43z} - r_{35z}\right) \cos{\left(\beta_{14} \right)} \end{matrix}\right.
  \\
  \qquad\left.\begin{matrix} - \left(4 - r_{42y}\right) \cos{\left(\beta_{42} \right)} + \left(5 - r_{42z}\right) \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)}\\ \left(3 - r_{42x}\right) \cos{\left(\beta_{42} \right)} - \left(5 - r_{42z}\right) \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\ - \left(3 - r_{42x}\right) \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)} + \left(4 - r_{42y}\right) \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\ \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\ \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)}\\ \cos{\left(\beta_{42} \right)}\\ 0\end{matrix}\right]
  \end{split}
\]

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \left[A_2\right]=\left[\begin{matrix}- \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & 0 & r_{43z} - 5 \\\left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & 5 - r_{43z} & 0 \\- \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & r_{43y} - 4 & 3 - r_{43x} \\\sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & -1 & 0 \\\sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & 0 & -1 \\\cos{\left(\beta_{25} \right)} & 0 & 0 \\0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} \end{matrix}\right.\\\qquad\left.\begin{matrix} 4 - r_{43y} & 0 & r_{35z} - 5 & 4 - r_{35y}\\ r_{43x} - 3 & 5 - r_{35z} & 0 & r_{35x} - 3\\ 0 & r_{35y} - 4 & 3 - r_{35x} & 0\\ 0 & -1 & 0 & 0\\ 0 & 0 & -1 & 0\\ -1 & 0 & 0 & -1\\ r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]
  \end{split}
\]

By using the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$, the relation between the active joint velocities and the end-effector velocities can be written as

\[
  %\Rightarrow
   \{\dot{X}\}=\left( \left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] \right) \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]
   where $\left[\widetilde{J}\right]=\left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] $ is the Jacobian matrix of the manipulator for the considered actuating joints.
\newline

$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$
Based on the strategy mentioned in section \ref{strategy_used_in_optimisation}, the above optimisation problem is attempted for solution, but it did not pass the criterion mentioned in Step 1. Hence, the modified objective function is taken for optimisation in order to avoid type-2 singularity. The modified optimisation problem would then become
\newline
Maximise\[f_2=\sqrt{\det{\left(\left[\widetilde{A}\right]^T \left[\widetilde{A}\right]\right)} \times \det{\left(\left[\widetilde{B}\right]^T \left[\widetilde{B}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$

\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{42}-\vec{a}\right)\times \hat{n}_{42}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{25}-\vec{a}\right)\times \hat{n}_{25}\right| \\
  \bar{d}_{4}=\left|\vec{r}_{43}-\vec{a}\right| \\
  \bar{d}_{5}=\left|\vec{r}_{35}-\vec{a}\right|
\end{matrix}
$$

The characteristic length is formulated as follows.
\[L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}+\bar{d}_{4}+\bar{d}_{5}}{5}\]



By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
\[\left[S\right]=\begin{bmatrix}
  \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
  0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
  0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
  0 & 0 & 0 & 1 & 0 & 0\\
  0 & 0 & 0 & 0 & 1 & 0\\
  0 & 0 & 0 & 0 & 0 & 1\\
  \end{bmatrix}\]
  
  The scaled Jacobian matrix can then be calculated as
  \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
  The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.

\emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in table \ref{Tab:table_4_1} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{14}$ & $\ang{0.0}$ \\
\hline$\phi_{42}$ & $\ang{292.2}$ \\
\hline$\phi_{25}$ & $\ang{171.62}$ \\
\hline$r_{14x}$ & $0.0$ \\
\hline$r_{14y}$ & $0.0$ \\
\hline$r_{14z}$ & $10.0$ \\
\hline$r_{42x}$ & $10.0$ \\
\hline$r_{42y}$ & $10.0$ \\
\hline$r_{42z}$ & $0.0$ \\
\hline$r_{25x}$ & $10.0$ \\
\hline$r_{25y}$ & $0.0$ \\
\hline$r_{25z}$ & $10.0$ \\
\hline$r_{43x}$ & $0.0$ \\
\hline$r_{43y}$ & $0.0$ \\
\hline$r_{43z}$ & $0.0$ \\
\hline$r_{35x}$ & $10.0$ \\
\hline$r_{35y}$ & $10.0$ \\
\hline$r_{35z}$ & $10.0$ \\
\hline$\beta_{14}$ & $\ang{73.92}$ \\
\hline$\beta_{42}$ & $\ang{121.39}$ \\
\hline$\beta_{25}$ & $\ang{42.39}$ \\
\hline\end{tabular} \caption{Result (2D-M1)} \label{Tab:table_4_1} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{14}=0.0\hat{i}+0.96\hat{j}+0.28\hat{k} \\
  \hat{n}_{42}=-0.79\hat{i}+0.32\hat{j}-0.52\hat{k} \\
  \hat{n}_{25}=0.1\hat{i}-0.67\hat{j}+0.74\hat{k} \\
  \vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{42}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{43}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=73.96\]
And the corresponding condition number is \[\kappa=1.87\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.106\]

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulators/dof2/manipulator_71.tex <==
% \emph{Adjacency matrix of manipulator 2D-M71:}

% The adjacency of the manipulator is\[M_{\text{2D-M71}}=\left[\begin{matrix}L_{1}&O&R&R&O\\O&L_{2}&O&S&R\\R&O&L_{3}&O&C\\R&S&O&L_{4}&O\\O&R&C&O&L_{5}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline

\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/2dof/71.png}
  \caption{Schematic figure of 2D-M71}
  \label{fig_2dof_iext_71}
\end{figure}


\emph{Formulation of Jacobian:}

Jacobian of the manipulator is formulated using the steps shown in section \ref{steps_to_formulate_jacobian}. The various paths that connect the base link and the end-effector link are $L_1-R-L_3-C-L_5$ and $L_1-R-L_4-S-L_2-R-L_5$. The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.
\begin{eqnarray}\label{eqn:eqn_2_71_1_2}\vec{v}=\dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{35} \hat{n}_{35} \times \left( \vec{a} - \vec{r}_{35} \right) + \dot{d}_{35} \hat{n}_{35}\end{eqnarray}\begin{eqnarray}\label{eqn:eqn_2_71_1_1}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}\begin{dmath}\label{eqn:eqn_2_71_2_2}\vec{\omega}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{35} \hat{n}_{35}\end{dmath}\begin{dmath}\label{eqn:eqn_2_71_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{42} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{ij}=\begin{Bmatrix} \omega_{ijx} & \omega_{ijy} & \omega_{ijz} \end{Bmatrix}^T$ represents the relative angular velocity vector of the link $L_j$ relative to the link $L_i$, of the adjacency matrix. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_2_1}, the vector of end-effector velocities in terms of both active and passive joint angles is given by
%From equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_2_1},
\newline
%\resizebox{\textwidth}{!}{$
$$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & 0 & n_{35x} & 0 & n_{35y} \left(a_z - r_{35z}\right) - n_{35z} \left(a_y - r_{35y}\right) & 0 & 0 & 0\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & 0 & n_{35y} & 0 & - n_{35x} \left(a_z - r_{35z}\right) + n_{35z} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & 0 & n_{35z} & 0 & n_{35x} \left(a_y - r_{35y}\right) - n_{35y} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\n_{13x} & 0 & 0 & 0 & n_{35x} & 0 & 0 & 0\\n_{13y} & 0 & 0 & 0 & n_{35y} & 0 & 0 & 0\\n_{13z} & 0 & 0 & 0 & n_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}$$
%$}


\resizebox{\textwidth}{!}{$\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & 0\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & 0\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & 0\\n_{13x} & 0\\n_{13y} & 0\\n_{13z} & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}+\left[\begin{matrix}n_{35x} & 0 & n_{35y} \left(a_z - r_{35z}\right) - n_{35z} \left(a_y - r_{35y}\right) & 0 & 0 & 0\\n_{35y} & 0 & - n_{35x} \left(a_z - r_{35z}\right) + n_{35z} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\n_{35z} & 0 & n_{35x} \left(a_y - r_{35y}\right) - n_{35y} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\0 & 0 & n_{35x} & 0 & 0 & 0\\0 & 0 & n_{35y} & 0 & 0 & 0\\0 & 0 & n_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}$}
\[\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[J_1\right]\{\dot{\theta}_a\}+\left[J_2\right]\{\Omega\}\]where $\{\dot{\theta}_a\}=\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}$ and $\{\Omega\}=\begin{Bmatrix}\dot{d}_{35}&\dot{\theta}_{25}&\dot{\theta}_{35}&\omega_{42x}&\omega_{42y}&\omega_{42z}\end{Bmatrix}^T$ represent the active joint-velocities and the passive joint-velocities, respectively.
\newline
But since the Jacobian should contain the end-effector velocities in terms of active joint angles alone, the passive joint angles must be written in terms of active joint angles. From the two equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_1_2},
%From the equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_1_2},
\newline
\begin{eqnarray}
  \label{eqn:eqn_2_71_5_1}
  \dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{35} \hat{n}_{35} \times \left( \vec{a} - \vec{r}_{35} \right) + \dot{d}_{35} \hat{n}_{35}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}
From the two equations \eqref{eqn:eqn_2_71_2_1} and \eqref{eqn:eqn_2_71_2_2},
\newline
\begin{dmath}
  \label{eqn:eqn_2_71_5_2}
  \dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{42} + \dot{\theta}_{25} \hat{n}_{25}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{35} \hat{n}_{35}\end{dmath}
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\- n_{13x} & n_{14x} & 0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\- n_{13y} & n_{14y} & 0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\- n_{13z} & n_{14z} & 0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
%\newline
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right)\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right)\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right)\\- n_{13x} & n_{14x}\\- n_{13y} & n_{14y}\\- n_{13z} & n_{14z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}+\left[\begin{matrix}- n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\- n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
From the equations \eqref{eqn:eqn_2_71_5_1} and \eqref{eqn:eqn_2_71_5_2}, linear equations in terms of active and passive joint angles can be stacked as shown below, using which the passive joint angles can be written in terms of the active joint angles.
\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    %\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\- n_{13x} & n_{14x} & 0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\- n_{13y} & n_{14y} & 0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\- n_{13z} & n_{14z} & 0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]
    %\Rightarrow\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) \\- n_{13x} & n_{14x} & 0 & n_{25x} \\- n_{13y} & n_{14y} & 0 & n_{25y} \\- n_{13z} & n_{14z} & 0 & n_{25z} \end{matrix}\right.\\\qquad\left.\begin{matrix} - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\ n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\ - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\ - n_{35x} & 1 & 0 & 0\\ - n_{35y} & 0 & 1 & 0\\ - n_{35z} & 0 & 0 & 1\end{matrix}\right]
    %\Rightarrow
    \left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} \\- n_{13x} & n_{14x} & 0 \\- n_{13y} & n_{14y} & 0 \\- n_{13z} & n_{14z} & 0 \end{matrix}\right.
    \\
    \qquad
    \left.\begin{matrix} n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) \\ - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) \\ n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) \\ n_{25x} & - n_{35x} \\ n_{25y} & - n_{35y} \\ n_{25z} & - n_{35z} \end{matrix}\right.\\\qquad\left.\begin{matrix} 0 & a_z - r_{42z} & - a_y + r_{42y}\\ - a_z + r_{42z} & 0 & a_x - r_{42x}\\ a_y - r_{42y} & - a_x + r_{42x} & 0\\ 1 & 0 & 0\\ 0 & 1 & 0\\ 0 & 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}
    =
    \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
  \end{split}
  %$}
\]

\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    \Rightarrow\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right)\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right)\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right)\\- n_{13x} & n_{14x}\\- n_{13y} & n_{14y}\\- n_{13z} & n_{14z}\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}
    + \\
    \left[\begin{matrix}- n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) \\- n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) \\- n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) \\0 & n_{25x} \\0 & n_{25y} \\0 & n_{25z} \end{matrix}\right.\\\qquad\left.\begin{matrix} - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\ n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\ - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\ - n_{35x} & 1 & 0 & 0\\ - n_{35y} & 0 & 1 & 0\\ - n_{35z} & 0 & 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}
    =
    \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
  \end{split}
  %$}
\]

\[\Rightarrow \left[A_1\right]\{\dot{\theta}_a\}+\left[A_2\right]\{\Omega\}=0\] \[\Rightarrow \{\Omega\}=-\left[A_2\right]^{-1}\left[A_1\right]\{\dot{\theta}_a\}\]\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}=\left[J_1\right] \{\dot{\theta}_a\}+\left[J_2\right] \{\Omega\}=\left[J_1\right] \{\dot{\theta}_a\}-\left[J_2\right]\left[A_2\right]^{-1}\left[A_1\right] \{\dot{\theta}_a\}\]
The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$ would finally be

%\resizebox{\textwidth}{!}{$
$$\left[J_1\right]=\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & 0\\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & 0\\\cos{\left(\beta_{13} \right)} & 0\end{matrix}\right]$$
%$}

%\resizebox{\textwidth}{!}{$
$$\left[J_2\right]=\left[\begin{matrix}\sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 & - \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 0 & 0\\\sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 & 0 & 0\\\cos{\left(\beta_{35} \right)} & 0 & - \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} + \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 & 0 & 0\\0 & 0 & \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 & 0 & 0\\0 & 0 & \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 0 & 0\\0 & 0 & \cos{\left(\beta_{35} \right)} & 0 & 0 & 0\end{matrix}\right]$$
%$}

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \left[A_1\right]=\left[\begin{matrix}\left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\- \left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} - \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\- \cos{\left(\beta_{13} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\ \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\ \cos{\left(\beta_{14} \right)}\end{matrix}\right]
  \end{split}
\]

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \left[A_2\right]=\left[\begin{matrix}- \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} \\- \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\- \cos{\left(\beta_{35} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\0 & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\0 & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} \\0 & \cos{\left(\beta_{25} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 5 - r_{42z} & r_{42y} - 4\\ - \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & r_{42z} - 5 & 0 & 3 - r_{42x}\\ \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} - \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 4 - r_{42y} & r_{42x} - 3 & 0\\ - \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 1 & 0 & 0\\ - \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 1 & 0\\ - \cos{\left(\beta_{35} \right)} & 0 & 0 & 1\end{matrix}\right]
  \end{split}
\]

%\resizebox{\textwidth}{!}{$A_1=\left[\begin{matrix}\left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\- \left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\\left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} - \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\- \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\- \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\- \cos{\left(\beta_{13} \right)} & \cos{\left(\beta_{14} \right)}\end{matrix}\right]$}

%\resizebox{\textwidth}{!}{$A_2=\left[\begin{matrix}- \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 5 - r_{42z} & r_{42y} - 4\\- \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & - \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & r_{42z} - 5 & 0 & 3 - r_{42x}\\- \cos{\left(\beta_{35} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} - \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 4 - r_{42y} & r_{42x} - 3 & 0\\0 & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & - \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 1 & 0 & 0\\0 & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & - \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 1 & 0\\0 & \cos{\left(\beta_{25} \right)} & - \cos{\left(\beta_{35} \right)} & 0 & 0 & 1\end{matrix}\right]$}
By using the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$, the relation between the active joint velocities and the end-effector velocities can be written as

\[
  %\Rightarrow
   \{\dot{X}\}=\left( \left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] \right) \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]
   where $\left[\widetilde{J}\right]=\left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] $ is the Jacobian matrix of the manipulator for the considered actuating joints.
\newline

$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$
Based on the strategy mentioned in section \ref{strategy_used_in_optimisation}, the above optimisation problem is attempted for solution, but it did not pass the criterion mentioned in Step 1. Hence, the modified objective function is taken for optimisation in order to avoid type-2 singularity. The modified optimisation problem would then become
\newline
Maximise\[f_2=\sqrt{\det{\left(\left[\widetilde{A}\right]^T \left[\widetilde{A}\right]\right)} \times \det{\left(\left[\widetilde{B}\right]^T \left[\widetilde{B}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$

\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{13}-\vec{a}\right)\times \hat{n}_{13}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{25}-\vec{a}\right)\times \hat{n}_{25}\right| \\
  \bar{d}_{4}=\left|\left(\vec{r}_{35}-\vec{a}\right)\times \hat{n}_{35}\right| \\
  \bar{d}_{5}=\left|\vec{r}_{42}-\vec{a}\right|
\end{matrix}
$$


The characteristic length is formulated as follows.
\[L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}+\bar{d}_{4}+\bar{d}_{5}}{5}\]



By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
\[\left[S\right]=\begin{bmatrix}
  \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
  0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
  0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
  0 & 0 & 0 & 1 & 0 & 0\\
  0 & 0 & 0 & 0 & 1 & 0\\
  0 & 0 & 0 & 0 & 0 & 1\\
  \end{bmatrix}\]
  
  The scaled Jacobian matrix can then be calculated as
  \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
  The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.

\emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in Table \ref{Tab:table_5_71} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{13}$ & $\ang{360.0}$ \\
\hline$\phi_{14}$ & $\ang{104.74}$ \\
\hline$\phi_{25}$ & $\ang{347.83}$ \\
\hline$\phi_{35}$ & $\ang{32.44}$ \\
\hline$r_{13x}$ & $10.0$ \\
\hline$r_{13y}$ & $10.0$ \\
\hline$r_{13z}$ & $10.0$ \\
\hline$r_{14x}$ & $10.0$ \\
\hline$r_{14y}$ & $10.0$ \\
\hline$r_{14z}$ & $0.0$ \\
\hline$r_{42x}$ & $10.0$ \\
\hline$r_{42y}$ & $0.0$ \\
\hline$r_{42z}$ & $10.0$ \\
\hline$r_{25x}$ & $0.0$ \\
\hline$r_{25y}$ & $0.0$ \\
\hline$r_{25z}$ & $0.0$ \\
\hline$r_{35x}$ & $0.0$ \\
\hline$r_{35y}$ & $10.0$ \\
\hline$r_{35z}$ & $0.0$ \\
\hline$\beta_{13}$ & $\ang{137.39}$ \\
\hline$\beta_{14}$ & $\ang{45.96}$ \\
\hline$\beta_{25}$ & $\ang{134.35}$ \\
\hline$\beta_{35}$ & $\ang{68.46}$ \\
\hline\end{tabular} \caption{Result (2D-M71)} \label{Tab:table_5_71} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k} \\
  \hat{n}_{14}=0.7\hat{i}-0.18\hat{j}+0.7\hat{k} \\
  \hat{n}_{25}=-0.15\hat{i}+0.7\hat{j}-0.7\hat{k} \\
  \hat{n}_{35}=0.5\hat{i}+0.78\hat{j}+0.37\hat{k} \\
  \vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{42}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=173.16\]

And the corresponding condition number is \[\kappa=1.98\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.2305\]

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulators/dof2/manipulator_71_edited.tex <==
% \emph{Adjacency matrix:}

% The adjacency of 2D-M71 manipulator is\[M_{\text{2D-M71}}=\left[\begin{matrix}L_{1}&O&R&R&O\\O&L_{2}&O&S&R\\R&O&L_{3}&O&C\\R&S&O&L_{4}&O\\O&R&C&O&L_{5}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link. The schematic diagram of this manipulator is shown in figure \ref{fig_2dof_iext_71}, mentioning the actuator joints in cyan circles.
% % \newline

The schematic diagram of 2D-M71 manipulator is shown in figure \ref{fig_2dof_iext_71}, mentioning the actuator joints in cyan circles.

\begin{figure}[hbt!]
  \centering
  \includegraphics[width=0.6\linewidth]{contentfolder/images/2dof/71.png}
  \caption{Schematic figure of 2D-M71.}
  \label{fig_2dof_iext_71}
\end{figure}


\noindent\emph{Formulation of Jacobian:}

Jacobian of the manipulator is formulated using the steps shown in section \ref{steps_to_formulate_jacobian}. The various paths that connect the base link and the end-effector link are $L_1-R-L_3-C-L_5$ and $L_1-R-L_4-S-L_2-R-L_5$. The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.

%\begin{eqnarray}\label{eqn:eqn_2_71_1_2}\vec{v}=\dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{35} \hat{n}_{35} \times \left( \vec{a} - \vec{r}_{35} \right) + \dot{d}_{35} \hat{n}_{35}\end{eqnarray}

\begin{equation}
%\centering
\begin{array}{cc}
    \vec{v}=\dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{35} \hat{n}_{35} \times \left( \vec{a} - \vec{r}_{35} \right) \\
     + \dot{d}_{35} \hat{n}_{35}
\end{array}
\label{eqn:eqn_2_71_1_2}
\end{equation}

\begin{equation}
%\centering
\begin{array}{cc}
    \vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) \\
    + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)
\end{array}
\label{eqn:eqn_2_71_1_1}
\end{equation}

\begin{dmath}\label{eqn:eqn_2_71_2_2}\vec{\omega}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{35} \hat{n}_{35}\end{dmath}\begin{dmath}\label{eqn:eqn_2_71_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{42} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} \\ r_{ijy} \\ r_{ijz} \end{Bmatrix}$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{ij}=\begin{Bmatrix} \omega_{ijx} \\ \omega_{ijy} \\ \omega_{ijz} \end{Bmatrix}$ represents the relative angular velocity vector of the link $L_j$ relative to the link $L_i$. $\vec{a}=\begin{Bmatrix} a_{x} \\ a_{y} \\ a_{z} \end{Bmatrix}$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_2_71_1_2} and \eqref{eqn:eqn_2_71_2_2}, the vector of end-effector velocities in terms of both active and passive joint angles is given by
%From equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_2_1},
\newline
\resizebox{0.4\textwidth}{!}{$
$$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & 0 & n_{35x} & 0 \\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & 0 & n_{35y} & 0 \\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & 0 & n_{35z} & 0 \\n_{13x} & 0 & 0 & 0 \\n_{13y} & 0 & 0 & 0 \\n_{13z} & 0 & 0 & 0 \end{matrix}\right.
$}
\\\qquad
\resizebox{0.4\textwidth}{!}{$
\left.\begin{matrix} n_{35y} \left(a_z - r_{35z}\right) - n_{35z} \left(a_y - r_{35y}\right) & 0 & 0 & 0\\ - n_{35x} \left(a_z - r_{35z}\right) + n_{35z} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\ n_{35x} \left(a_y - r_{35y}\right) - n_{35y} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\ n_{35x} & 0 & 0 & 0\\ n_{35y} & 0 & 0 & 0\\ n_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}$$
$}


\resizebox{0.45\textwidth}{!}{$
$$\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & 0\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & 0\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & 0\\n_{13x} & 0\\n_{13y} & 0\\n_{13z} & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}+$$
$}
\\\qquad
\resizebox{0.45\textwidth}{!}{$
$$\left[\begin{matrix}n_{35x} & 0 & n_{35y} \left(a_z - r_{35z}\right) - n_{35z} \left(a_y - r_{35y}\right) & 0 & 0 & 0\\n_{35y} & 0 & - n_{35x} \left(a_z - r_{35z}\right) + n_{35z} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\n_{35z} & 0 & n_{35x} \left(a_y - r_{35y}\right) - n_{35y} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\0 & 0 & n_{35x} & 0 & 0 & 0\\0 & 0 & n_{35y} & 0 & 0 & 0\\0 & 0 & n_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}$$
$}

\[\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[J_1\right]\{\dot{\theta}_a\}+\left[J_2\right]\{\Omega\}\]where $\{\dot{\theta}_a\}=\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}$ and $\{\Omega\}=\begin{Bmatrix}\dot{d}_{35} \\ \dot{\theta}_{25} \\ \dot{\theta}_{35} \\ \omega_{42x} \\ \omega_{42y} \\ \omega_{42z}\end{Bmatrix}$ represent the active joint-velocities and the passive joint-velocities, respectively.
\newline
But since the Jacobian should contain the end-effector velocities in terms of active joint angles alone, the passive joint angles must be written in terms of active joint angles. From the two equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_1_2},
%From the equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_1_2},
\newline
% \begin{eqnarray}
%   \label{eqn:eqn_2_71_5_1}
%   \dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{35} \hat{n}_{35} \times \left( \vec{a} - \vec{r}_{35} \right) + \dot{d}_{35} \hat{n}_{35}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}

\begin{equation}
%\centering
\begin{array}{cc}
    \dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{35} \hat{n}_{35} \times \left( \vec{a} - \vec{r}_{35} \right) \\
    + \dot{d}_{35} \hat{n}_{35}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) \\
    + \vec{\omega}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)
\end{array}
\label{eqn:eqn_2_71_5_1}
\end{equation}

From the two equations \eqref{eqn:eqn_2_71_2_1} and \eqref{eqn:eqn_2_71_2_2},
\newline
\begin{dmath}
  \label{eqn:eqn_2_71_5_2}
  \dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{42} + \dot{\theta}_{25} \hat{n}_{25}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{35} \hat{n}_{35}\end{dmath}
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\- n_{13x} & n_{14x} & 0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\- n_{13y} & n_{14y} & 0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\- n_{13z} & n_{14z} & 0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
%\newline
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right)\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right)\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right)\\- n_{13x} & n_{14x}\\- n_{13y} & n_{14y}\\- n_{13z} & n_{14z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}+\left[\begin{matrix}- n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\- n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
From the equations \eqref{eqn:eqn_2_71_5_1} and \eqref{eqn:eqn_2_71_5_2}, linear equations in terms of active and passive joint angles can be stacked as shown below, using which the passive joint angles can be written in terms of the active joint angles.\newline

% \[
%   %\resizebox{\textwidth}{!}{$
%   \begin{split}
%     %\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\- n_{13x} & n_{14x} & 0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\- n_{13y} & n_{14y} & 0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\- n_{13z} & n_{14z} & 0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]
%     %\Rightarrow\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) \\- n_{13x} & n_{14x} & 0 & n_{25x} \\- n_{13y} & n_{14y} & 0 & n_{25y} \\- n_{13z} & n_{14z} & 0 & n_{25z} \end{matrix}\right.\\\qquad\left.\begin{matrix} - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\ n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\ - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\ - n_{35x} & 1 & 0 & 0\\ - n_{35y} & 0 & 1 & 0\\ - n_{35z} & 0 & 0 & 1\end{matrix}\right]
%     %\Rightarrow
%     \left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} \\- n_{13x} & n_{14x} & 0 \\- n_{13y} & n_{14y} & 0 \\- n_{13z} & n_{14z} & 0 \end{matrix}\right.
%     \\
%     \qquad
%     \left.\begin{matrix} n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) \\ - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) \\ n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) \\ n_{25x} & - n_{35x} \\ n_{25y} & - n_{35y} \\ n_{25z} & - n_{35z} \end{matrix}\right.\\\qquad\left.\begin{matrix} 0 & a_z - r_{42z} & - a_y + r_{42y}\\ - a_z + r_{42z} & 0 & a_x - r_{42x}\\ a_y - r_{42y} & - a_x + r_{42x} & 0\\ 1 & 0 & 0\\ 0 & 1 & 0\\ 0 & 0 & 1\end{matrix}\right]
%     \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}
%     =
%     \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
%   \end{split}
%   %$}
% \]

%\[
  %\resizebox{\textwidth}{!}{$
  %\begin{split}
  \resizebox{0.3\textwidth}{!}{$
    %\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) \\- n_{13x} & n_{14x} \\- n_{13y} & n_{14y} \\- n_{13z} & n_{14z} \end{matrix}\right.
    $$\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) \\- n_{13x} \\- n_{13y} \\- n_{13z} \end{matrix}\right.$$
    $}
    \\\qquad
    %\resizebox{0.3\textwidth}{!}{$
    $$\left.\begin{matrix} n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) \\ - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) \\ n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) \\ n_{14x} \\ n_{14y} \\ n_{14z} \end{matrix}\right.$$
    %$}
    \\\qquad
    %\resizebox{0.5\textwidth}{!}{$
    $$\left.\begin{matrix} - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) \\ - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) \\ - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) \\ 0 & n_{25x} \\ 0 & n_{25y} \\ 0 & n_{25z} \end{matrix}\right.$$
    %$}
    \\\qquad
    %\resizebox{0.5\textwidth}{!}{$
    $$\left.\begin{matrix} - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 \\ n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} \\ - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} \\ - n_{35x} & 1 \\ - n_{35y} & 0 \\ - n_{35z} & 0 \end{matrix}\right.$$
    %$}
    \\\qquad
    %\resizebox{0.5\textwidth}{!}{$
    $$\left.\begin{matrix} a_z - r_{42z} & - a_y + r_{42y}\\ 0 & a_x - r_{42x}\\ - a_x + r_{42x} & 0\\ 0 & 0\\ 1 & 0\\ 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}
    %$}
    =
    \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$$
  %\end{split}
  %$}
%\]

%\[
  %\resizebox{\textwidth}{!}{$
  %\begin{split}
    $$\Rightarrow
    %\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right)\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right)\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right)\\- n_{13x} & n_{14x}\\- n_{13y} & n_{14y}\\- n_{13z} & n_{14z}\end{matrix}\right]
    \left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) \\- n_{13x} \\- n_{13y} \\- n_{13z} \end{matrix}\right.$$
    \\\qquad
    $$\left.\begin{matrix} n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right)\\ - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right)\\ n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right)\\ n_{14x}\\ n_{14y}\\ n_{14z}\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix} +$$
    \\\qquad
    $$\left[\begin{matrix}- n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) \\- n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) \\- n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) \\0 & n_{25x} \\0 & n_{25y} \\0 & n_{25z} \end{matrix}\right.$$
    \\\qquad
    $$\left.\begin{matrix} - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 \\ n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} \\ - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} \\ - n_{35x} & 1 \\ - n_{35y} & 0 \\ - n_{35z} & 0 \end{matrix}\right.$$
    \\\qquad
    $$\left.\begin{matrix} a_z - r_{42z} & - a_y + r_{42y}\\ 0 & a_x - r_{42x}\\ - a_x + r_{42x} & 0\\ 0 & 0\\ 1 & 0\\ 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}
    =
    \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$$
  %\end{split}
  %$}
%\]

\[\Rightarrow \left[A_1\right]\{\dot{\theta}_a\}+\left[A_2\right]\{\Omega\}=0\] \[\Rightarrow \{\Omega\}=-\left[A_2\right]^{-1}\left[A_1\right]\{\dot{\theta}_a\}\]\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}=\left[J_1\right] \{\dot{\theta}_a\}+\left[J_2\right] \{\Omega\}\]\[=\left[J_1\right] \{\dot{\theta}_a\}-\left[J_2\right]\left[A_2\right]^{-1}\left[A_1\right] \{\dot{\theta}_a\}\]

The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$ would finally be\newline

\resizebox{0.45\textwidth}{!}{$
$$\left[J_1\right]=\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & 0\\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & 0\\\cos{\left(\beta_{13} \right)} & 0\end{matrix}\right]$$
$}

\resizebox{0.2\textwidth}{!}{$
$$\left[J_2\right]=
\left[\begin{matrix}\sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 \\\sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 \\\cos{\left(\beta_{35} \right)} & 0 \\0 & 0 \\0 & 0 \\0 & 0 \end{matrix}\right.$$
$}
\\\qquad
\resizebox{0.4\textwidth}{!}{$
$$\left.\begin{matrix} - \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} \\ \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} \\ - \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} + \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} \\ \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} \\ \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} \\ \cos{\left(\beta_{35} \right)} \end{matrix}\right.$$
$}
\\\qquad
%\resizebox{0.08\textwidth}{!}{$
$$\resizebox{0.08\textwidth}{!}{$\left.\begin{matrix} 0 & 0 & 0\\ 0 & 0 & 0\\ 0 & 0 & 0\\ 0 & 0 & 0\\ 0 & 0 & 0\\ 0 & 0 & 0\end{matrix}\right]$}
$$
%$}

%\[
  %\resizebox{\textwidth}{!}{$
  %$}
  %\begin{split}
  \resizebox{0.45\textwidth}{!}{$
    $$\left[A_1\right]=\left[\begin{matrix}\left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\- \left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} - \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\- \cos{\left(\beta_{13} \right)} \end{matrix}\right.$$
    $}
    \\\qquad
    \resizebox{0.45\textwidth}{!}{$
    $$\left.\begin{matrix} - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\ \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\ \cos{\left(\beta_{14} \right)}\end{matrix}\right]$$
    $}
  %\end{split}
%\]

%\[
  %\resizebox{\textwidth}{!}{$$}
  %\begin{split}
    \resizebox{0.22\textwidth}{!}{$
    $$\left[A_2\right]=\left[\begin{matrix}- \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} \\- \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} \\- \cos{\left(\beta_{35} \right)} \\0 \\0 \\0 \end{matrix}\right.$$
    $}
    \\\qquad
    \resizebox{0.45\textwidth}{!}{$
    $$\left.\begin{matrix} - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} \\ \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\ - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\ \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\ \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} \\ \cos{\left(\beta_{25} \right)} \end{matrix}\right.$$
    $}
    \\\qquad
    \resizebox{0.45\textwidth}{!}{$
    $$\left.\begin{matrix} \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} \\ - \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} \\ \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} - \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} \\ - \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} \\ - \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} \\ - \cos{\left(\beta_{35} \right)} \end{matrix}\right.$$
    $}
    \\\qquad
    
    %\resizebox{0.2\textwidth}{!}{$
    $$\left.\begin{matrix} 0 & 5 - r_{42z} & r_{42y} - 4\\ r_{42z} - 5 & 0 & 3 - r_{42x}\\ 4 - r_{42y} & r_{42x} - 3 & 0\\ 1 & 0 & 0\\ 0 & 1 & 0\\ 0 & 0 & 1\end{matrix}\right]$$
    %$}
    
  %\end{split}
%\]

%\resizebox{\textwidth}{!}{$A_1=\left[\begin{matrix}\left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\- \left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\\left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} - \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\- \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\- \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\- \cos{\left(\beta_{13} \right)} & \cos{\left(\beta_{14} \right)}\end{matrix}\right]$}

%\resizebox{\textwidth}{!}{$A_2=\left[\begin{matrix}- \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 5 - r_{42z} & r_{42y} - 4\\- \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & - \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & r_{42z} - 5 & 0 & 3 - r_{42x}\\- \cos{\left(\beta_{35} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} - \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 4 - r_{42y} & r_{42x} - 3 & 0\\0 & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & - \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 1 & 0 & 0\\0 & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & - \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 1 & 0\\0 & \cos{\left(\beta_{25} \right)} & - \cos{\left(\beta_{35} \right)} & 0 & 0 & 1\end{matrix}\right]$}
By using the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$, the relation between the active joint velocities and the end-effector velocities can be written as

\[
  %\Rightarrow
   \{\dot{X}\}=\left( \left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] \right) \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]
   where $\left[\widetilde{J}\right]=\left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] $ is the Jacobian matrix of the manipulator for the considered actuating joints.
\newline

Therefore, the formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

\hl{subject} to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10, \\
  0 \leq \beta_{ij} \leq \pi, \\
  0 \leq \phi_{ij} \leq 2\pi.
  \end{matrix}
$$
Based on the strategy mentioned in section \ref{strategy_used_in_optimisation}, the above optimisation problem is attempted for solution, but it did not pass the criterion mentioned in Step 1. Hence, the modified objective function is taken for optimisation in order to avoid type-2 singularity. The modified optimisation problem would then become
\newline
Maximise\[f_2=\sqrt{\det{\left(\left[\widetilde{A}\right]^T \left[\widetilde{A}\right]\right)} \times \det{\left(\left[\widetilde{B}\right]^T \left[\widetilde{B}\right]\right)}}\]

\hl{subject} to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10, \\
  0 \leq \beta_{ij} \leq \pi, \\
  0 \leq \phi_{ij} \leq 2\pi,
  \end{matrix}
$$

\noindent\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{13}-\vec{a}\right)\times \hat{n}_{13}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{25}-\vec{a}\right)\times \hat{n}_{25}\right| \\
  \bar{d}_{4}=\left|\left(\vec{r}_{35}-\vec{a}\right)\times \hat{n}_{35}\right| \\
  \bar{d}_{5}=\left|\vec{r}_{42}-\vec{a}\right|
\end{matrix}
$$


The characteristic length is formulated as follows.
\[L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}+\bar{d}_{4}+\bar{d}_{5}}{5}\]



By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
\[\left[S\right]=\begin{bmatrix}
  \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
  0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
  0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
  0 & 0 & 0 & 1 & 0 & 0\\
  0 & 0 & 0 & 0 & 1 & 0\\
  0 & 0 & 0 & 0 & 0 & 1\\
  \end{bmatrix}\]
  
The scaled Jacobian matrix can then be calculated as
\[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]
The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.

\noindent\emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in Table \ref{Tab:table_5_71} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{13}$ & $\ang{360.0}$ \\
\hline$\phi_{14}$ & $\ang{104.74}$ \\
\hline$\phi_{25}$ & $\ang{347.83}$ \\
\hline$\phi_{35}$ & $\ang{32.44}$ \\
\hline$r_{13x}$ & $10.0$ \\
\hline$r_{13y}$ & $10.0$ \\
\hline$r_{13z}$ & $10.0$ \\
\hline$r_{14x}$ & $10.0$ \\
\hline$r_{14y}$ & $10.0$ \\
\hline$r_{14z}$ & $0.0$ \\
\hline$r_{42x}$ & $10.0$ \\
\hline$r_{42y}$ & $0.0$ \\
\hline$r_{42z}$ & $10.0$ \\
\hline$r_{25x}$ & $0.0$ \\
\hline$r_{25y}$ & $0.0$ \\
\hline$r_{25z}$ & $0.0$ \\
\hline$r_{35x}$ & $0.0$ \\
\hline$r_{35y}$ & $10.0$ \\
\hline$r_{35z}$ & $0.0$ \\
\hline$\beta_{13}$ & $\ang{137.39}$ \\
\hline$\beta_{14}$ & $\ang{45.96}$ \\
\hline$\beta_{25}$ & $\ang{134.35}$ \\
\hline$\beta_{35}$ & $\ang{68.46}$ \\
\hline\end{tabular} \caption{Result of the optimisation problem corresponding to 2D-M71 manipulator.} \label{Tab:table_5_71} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k} \\
  \hat{n}_{14}=0.7\hat{i}-0.18\hat{j}+0.7\hat{k} \\
  \hat{n}_{25}=-0.15\hat{i}+0.7\hat{j}-0.7\hat{k} \\
  \hat{n}_{35}=0.5\hat{i}+0.78\hat{j}+0.37\hat{k} \\
  \vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{42}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=173.16\]

And the corresponding condition number is \[\kappa=1.98\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.2305\]

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulators/dof3/manipulator_1.tex <==
% \emph{Adjacency matrix of manipulator 3D-M1:}

% The adjacency of the manipulator is\[M_{\text{3D-M1}}=\left[\begin{matrix}L_{1}&O&R&O\\O&L_{2}&R&R\\R&R&L_{3}&O\\O&R&O&L_{4}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline

\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/3dof/1.png}
  \caption{Schematic figure of 3D-M1}
  \label{fig_3dof_iext_1}
\end{figure}


\emph{Formulation of Jacobian:}

Since this is a serial manipulator, there would be only one path that connects the base link and the end-effector link. That path is $L_1-R-L_3-R-L_2-R-L_4$. Hence, through this path, the linear velocity of the end-effector link is given by
\begin{eqnarray}\label{eqn:eqn_3_1_1_1}\vec{v}=\dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{32} \hat{n}_{32} \times \left( \vec{a} - \vec{r}_{32} \right) + \dot{\theta}_{24} \hat{n}_{24} \times \left( \vec{a} - \vec{r}_{24} \right)\end{eqnarray}
And the angular velocity of the end-effector link is given by
\begin{dmath}\label{eqn:eqn_3_1_2_1}\vec{\omega}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{32} \hat{n}_{32} + \dot{\theta}_{24} \hat{n}_{24}\end{dmath}\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}\]where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ represents the rotational joint velocity of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
%where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{k}=\begin{Bmatrix} \omega_{kx} & \omega_{ky} & \omega_{kz} \end{Bmatrix}^T$ represents the angular velocity vector of the link $L_k$, of the adjacency matrix. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix.
\newline
From equations \eqref{eqn:eqn_3_1_1_1} and \eqref{eqn:eqn_3_1_2_1}, the vector of end-effector velocities in terms of active passive joint angles is given by
%\newline
%\resizebox{\textwidth}{!}{$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & n_{24y} \left(a_z - r_{24z}\right) - n_{24z} \left(a_y - r_{24y}\right)\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - n_{24x} \left(a_z - r_{24z}\right) + n_{24z} \left(a_x - r_{24x}\right)\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & n_{24x} \left(a_y - r_{24y}\right) - n_{24y} \left(a_x - r_{24x}\right)\\n_{13x} & n_{32x} & n_{24x}\\n_{13y} & n_{32y} & n_{24y}\\n_{13z} & n_{32z} & n_{24z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{32}\\\dot{\theta}_{24}\end{Bmatrix}$}

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}
    =
    \left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) \\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) \\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) \\n_{13x} & n_{32x} \\n_{13y} & n_{32y} \\n_{13z} & n_{32z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{24y} \left(a_z - r_{24z}\right) - n_{24z} \left(a_y - r_{24y}\right)\\ - n_{24x} \left(a_z - r_{24z}\right) + n_{24z} \left(a_x - r_{24x}\right)\\ n_{24x} \left(a_y - r_{24y}\right) - n_{24y} \left(a_x - r_{24x}\right)\\ n_{24x}\\ n_{24y}\\ n_{24z}\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{32}\\\dot{\theta}_{24}\end{Bmatrix}
  \end{split}
\]

The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrix $\left[J_1\right]$ would finally be
%\resizebox{\textwidth}{!}{$J_1=\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{24y}\right) \cos{\left(\beta_{24} \right)} + \left(5 - r_{24z}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{24x}\right) \cos{\left(\beta_{24} \right)} - \left(5 - r_{24z}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{24x}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)} + \left(4 - r_{24y}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\\cos{\left(\beta_{13} \right)} & \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{24} \right)}\end{matrix}\right]$}

\[
  %\resizebox{\textwidth}{!}{$
  \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \begin{split}
    \left[J_1\right]
    =
    %\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\\cos{\left(\beta_{13} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{24y}\right) \cos{\left(\beta_{24} \right)} + \left(5 - r_{24z}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{24x}\right) \cos{\left(\beta_{24} \right)} - \left(5 - r_{24z}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{24x}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)} + \left(4 - r_{24y}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\ \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{24} \right)}\end{matrix}\right]
    %\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\\cos{\left(\beta_{13} \right)} & \cos{\left(\beta_{32} \right)} \end{matrix}\right.
    \left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\\cos{\left(\beta_{13} \right)} \end{matrix}\right.
    \\
    \qquad
    \left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\ \cos{\left(\beta_{32} \right)} \end{matrix}\right.
    \\
    \qquad
    \left.\begin{matrix} - \left(4 - r_{24y}\right) \cos{\left(\beta_{24} \right)} + \left(5 - r_{24z}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\ \left(3 - r_{24x}\right) \cos{\left(\beta_{24} \right)} - \left(5 - r_{24z}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ - \left(3 - r_{24x}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)} + \left(4 - r_{24y}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\ \cos{\left(\beta_{24} \right)}\end{matrix}\right]
  \end{split}
  %$}
\]
Hence, the relation between the active joint velocities and the end-effector velocities can be written as
\[
  %\Rightarrow
  \{\dot{X}\}=\left[J_1\right] \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]where $\left[\widetilde{J}\right]=\left[J_1\right]$.
\newline



$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise
$$f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}$$

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$


\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{13}-\vec{a}\right)\times \hat{n}_{13}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{32}-\vec{a}\right)\times \hat{n}_{32}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{24}-\vec{a}\right)\times \hat{n}_{24}\right|
\end{matrix}
$$

The characteristic length is formulated as follows.
\[
  L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}}{3}
  \]

  By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
  \[\left[S\right]=\begin{bmatrix}
    \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
    0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
    0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
    0 & 0 & 0 & 1 & 0 & 0\\
    0 & 0 & 0 & 0 & 1 & 0\\
    0 & 0 & 0 & 0 & 0 & 1\\
    \end{bmatrix}\]
    
    The scaled Jacobian matrix can then be calculated as
    \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
    The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.
  
  \emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in Table \ref{Tab:table_5_1} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{13}$ & $\ang{278.57}$ \\
\hline$\phi_{32}$ & $\ang{359.53}$ \\
\hline$\phi_{24}$ & $\ang{119.26}$ \\
\hline$r_{13x}$ & $10.0$ \\
\hline$r_{13y}$ & $10.0$ \\
\hline$r_{13z}$ & $0.0$ \\
\hline$r_{23x}$ & $10.0$ \\
\hline$r_{23y}$ & $0.0$ \\
\hline$r_{23z}$ & $10.0$ \\
\hline$r_{24x}$ & $10.0$ \\
\hline$r_{24y}$ & $10.0$ \\
\hline$r_{24z}$ & $10.0$ \\
\hline$\beta_{13}$ & $\ang{134.36}$ \\
\hline$\beta_{32}$ & $\ang{144.59}$ \\
\hline$\beta_{24}$ & $\ang{109.92}$ \\
\hline\end{tabular} \caption{Result (3D-M1)} \label{Tab:table_5_1} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{13}=-0.71\hat{i}+0.11\hat{j}-0.7\hat{k} \\
  \hat{n}_{32}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k} \\
  \hat{n}_{24}=0.82\hat{i}-0.46\hat{j}-0.34\hat{k} \\
  \vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=1058.87\]
And the corresponding condition number is \[\kappa=1.48\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=1.0113\]

==> Dimensional Synthesis/contentfolder/mechanisms2/manipulators/dof4/manipulator_2.tex <==
% \emph{Adjacency matrix of manipulator 4D-M2:}

% The adjacency of the manipulator is\[M_{\text{4D-M2}}=\left[\begin{matrix}L_{1}&O&O&R&O\\O&L_{2}&R&O&R\\O&R&L_{3}&P&O\\R&O&P&L_{4}&O\\O&R&O&O&L_{5}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline

\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/4dof/2.png}
  \caption{Schematic figure of 4D-M2}
  \label{fig_4dof_iext_2}
\end{figure}


\emph{Formulation of Jacobian:}

Since this is a serial manipulator, there would be only one path that connects the base link and the end-effector link. That path is $L_1-R-L_4-P-L_3-R-L_2-R-L_5$. Hence, through this path, the linear velocity of the end-effector link is given by
\begin{eqnarray}\label{eqn:eqn_4_2_1_1}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{d}_{43} \hat{n}_{43} + \dot{\theta}_{32} \hat{n}_{32} \times \left( \vec{a} - \vec{r}_{32} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}
And the angular velocity of the end-effector link is given by
\begin{dmath}\label{eqn:eqn_4_2_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \dot{\theta}_{32} \hat{n}_{32} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}\]where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector. $\dot{\theta}_{ij}$ represents the rotational joint velocity of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$. And $\dot{d}_{ij}$ represents the translational joint velocity of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_4_2_1_1} and \eqref{eqn:eqn_4_2_2_1}, the vector of end-effector velocities in terms of active passive joint angles is given by
\newline
%\resizebox{\textwidth}{!}{$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{43x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right)\\n_{43y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right)\\n_{43z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right)\\0 & n_{14x} & n_{32x} & n_{25x}\\0 & n_{14y} & n_{32y} & n_{25y}\\0 & n_{14z} & n_{32z} & n_{25z}\end{matrix}\right]\begin{Bmatrix}\dot{d}_{43}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\dot{\theta}_{25}\end{Bmatrix}$}

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}
    =
    %\left[\begin{matrix}n_{43x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) \\n_{43y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) \\n_{43z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) \\0 & n_{14x} \\0 & n_{14y} \\0 & n_{14z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right)\\ - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right)\\ n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right)\\ n_{32x} & n_{25x}\\ n_{32y} & n_{25y}\\ n_{32z} & n_{25z}\end{matrix}\right]
    \left[\begin{matrix}n_{43x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) \\n_{43y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) \\n_{43z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) \\0 & n_{14x} & n_{32x} \\0 & n_{14y} & n_{32y} \\0 & n_{14z} & n_{32z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right)\\ - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right)\\ n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right)\\ n_{25x}\\ n_{25y}\\ n_{25z}\end{matrix}\right]
    \begin{Bmatrix}\dot{d}_{43}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\dot{\theta}_{25}\end{Bmatrix}
  \end{split}
\]

The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrix $\left[J_1\right]$ would finally be
%\resizebox{\textwidth}{!}{$J_1=\left[\begin{matrix}\sin{\left(\beta_{43} \right)} \cos{\left(\phi_{43} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\\sin{\left(\phi_{43} \right)} \sin{\left(\beta_{43} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\\cos{\left(\beta_{43} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\0 & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\0 & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\0 & \cos{\left(\beta_{14} \right)} & \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{25} \right)}\end{matrix}\right]$}

\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    \left[J_1\right]
    =
    %\left[\begin{matrix}\sin{\left(\beta_{43} \right)} \cos{\left(\phi_{43} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\\sin{\left(\phi_{43} \right)} \sin{\left(\beta_{43} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\\cos{\left(\beta_{43} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\0 & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\0 & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\0 & \cos{\left(\beta_{14} \right)} & \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{25} \right)}\end{matrix}\right]
    \left[\begin{matrix}\sin{\left(\beta_{43} \right)} \cos{\left(\phi_{43} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} \\\sin{\left(\phi_{43} \right)} \sin{\left(\beta_{43} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\\cos{\left(\beta_{43} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\0 & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\0 & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} \\0 & \cos{\left(\beta_{14} \right)} \end{matrix}\right.
    \\
    \qquad
    %\left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\ \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{25} \right)}\end{matrix}\right]
    \left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\ \cos{\left(\beta_{32} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\ \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\ \cos{\left(\beta_{25} \right)}\end{matrix}\right]
  \end{split}
  %$}
\]

Hence, the relation between the active joint velocities and the end-effector velocities can be written as
\[
  %\Rightarrow
  \{\dot{X}\}=\left[J_1\right] \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]where $\left[\widetilde{J}\right]=\left[J_1\right]$.
\newline


$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$


\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{32}-\vec{a}\right)\times \hat{n}_{32}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{25}-\vec{a}\right)\times \hat{n}_{25}\right|
\end{matrix}
$$

The characteristic length is formulated as follows.
\[
  L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}}{3}
  \]

  By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
  \[\left[S\right]=\begin{bmatrix}
    \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
    0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
    0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
    0 & 0 & 0 & 1 & 0 & 0\\
    0 & 0 & 0 & 0 & 1 & 0\\
    0 & 0 & 0 & 0 & 0 & 1\\
    \end{bmatrix}\]
    
    The scaled Jacobian matrix can then be calculated as
    \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
    The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.
  
  \emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in Table \ref{Tab:table_6_1} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{14}$ & $\ang{59.28}$ \\
\hline$\phi_{32}$ & $\ang{219.46}$ \\
\hline$\phi_{25}$ & $\ang{206.56}$ \\
\hline$\phi_{43}$ & $\ang{39.95}$ \\
\hline$r_{14x}$ & $10.0$ \\
\hline$r_{14y}$ & $0.0$ \\
\hline$r_{14z}$ & $10.0$ \\
\hline$r_{23x}$ & $10.0$ \\
\hline$r_{23y}$ & $10.0$ \\
\hline$r_{23z}$ & $0.0$ \\
\hline$r_{25x}$ & $0.0$ \\
\hline$r_{25y}$ & $10.0$ \\
\hline$r_{25z}$ & $10.0$ \\
\hline$\beta_{14}$ & $\ang{72.57}$ \\
\hline$\beta_{32}$ & $\ang{142.41}$ \\
\hline$\beta_{25}$ & $\ang{108.6}$ \\
\hline$\beta_{43}$ & $\ang{63.44}$ \\
\hline\end{tabular} \caption{Result (4D-M2)} \label{Tab:table_6_1} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{14}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k} \\
  \hat{n}_{32}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k} \\
  \hat{n}_{25}=-0.42\hat{i}-0.85\hat{j}-0.32\hat{k} \\
  \hat{n}_{43}=0.57\hat{i}+0.69\hat{j}+0.45\hat{k} \\
  \vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=210.96\]
And the corresponding condition number is \[\kappa=15.31\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.2619\]

==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result1.tex <==
{\tiny 1D-M1:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.02\hat{i}-0.52\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=0.75\hat{i}-0.51\hat{j}+0.42\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.53\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result10.tex <==
{\tiny 1D-M10:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.84\hat{i}-0.49\hat{j}-0.25\hat{k}$,\;\;\;$\vec{r}_{13}=3.76\hat{i}+5.51\hat{j}+5.34\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+1.6\hat{k}$,\;\;\;$\vec{r}_{23}=4.11\hat{i}+6.4\hat{j}+4.81\hat{k}$,\;\;\;$\vec{r}_{24}=4.67\hat{i}+3.62\hat{j}+5.9\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result11.tex <==
{\tiny 1D-M11:}

$\hat{n}_{14}=0.16\hat{i}-0.66\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{23}=0.89\hat{i}-0.47\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{24}=-0.96\hat{i}-0.28\hat{j}-0.02\hat{k}$,\;\;\;$\vec{r}_{13}=2.15\hat{i}+6.75\hat{j}+2.1\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=1.36\hat{i}+8.7\hat{j}+7.55\hat{k}$,\;\;\;$\vec{r}_{24}=4.88\hat{i}+4.39\hat{j}+4.5\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result12.tex <==
{\tiny 1D-M12:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.76\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{24}=0.21\hat{i}-0.79\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+2.63\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result13.tex <==
{\tiny 1D-M13:}

$\hat{n}_{12}=-0.82\hat{i}-0.54\hat{j}+0.19\hat{k}$,\;\;\;$\hat{n}_{13}=0.82\hat{i}+0.0\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.03\hat{i}-0.82\hat{j}-0.57\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result14.tex <==
{\tiny 1D-M14:}

$\hat{n}_{12}=0.59\hat{i}-0.79\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}+0.02\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.57\hat{j}-0.59\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result15.tex <==
{\tiny 1D-M15:}

$\hat{n}_{12}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{13}=0.88\hat{i}-0.37\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.69\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result16.tex <==
{\tiny 1D-M16:}

$\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.45\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result17.tex <==
{\tiny 1D-M17:}

$\hat{n}_{12}=0.47\hat{i}-0.44\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{24}=0.11\hat{i}+0.39\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{34}=0.69\hat{i}-0.19\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result18.tex <==
{\tiny 1D-M18:}

$\hat{n}_{12}=0.08\hat{i}-0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.45\hat{i}-0.53\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{34}=0.39\hat{i}-0.82\hat{j}-0.42\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result19.tex <==
{\tiny 1D-M19:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.77\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result2.tex <==
{\tiny 1D-M2:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.77\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{24}=0.29\hat{i}+0.95\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result20.tex <==
{\tiny 1D-M20:}

$\hat{n}_{14}=-0.62\hat{i}+0.73\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{24}=0.59\hat{i}-0.56\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=4.05\hat{i}+6.66\hat{j}+3.38\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.38\hat{i}+5.09\hat{j}+3.57\hat{k}$,\;\;\;$\vec{r}_{24}=6.45\hat{i}+6.22\hat{j}+5.3\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result21.tex <==
{\tiny 1D-M21:}

$\hat{n}_{12}=0.78\hat{i}-0.25\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result22.tex <==
{\tiny 1D-M22:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result23.tex <==
{\tiny 1D-M23:}

$\hat{n}_{13}=0.77\hat{i}+0.0\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.92\hat{j}-0.38\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result24.tex <==
{\tiny 1D-M24:}

$\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result25.tex <==
{\tiny 1D-M25:}

$\hat{n}_{13}=0.16\hat{i}+0.61\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{14}=-0.8\hat{i}+0.54\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result26.tex <==
{\tiny 1D-M26:}

$\hat{n}_{13}=-0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.56\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{24}=0.81\hat{i}+0.46\hat{j}-0.36\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result27.tex <==
{\tiny 1D-M27:}

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}-0.6\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+2.83\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result28.tex <==
{\tiny 1D-M28:}

$\hat{n}_{13}=-0.08\hat{i}-0.95\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.44\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+7.16\hat{k}$,\;\;\;$\vec{r}_{23}=4.62\hat{i}+3.55\hat{j}+4.57\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+4.87\hat{j}+4.55\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result29.tex <==
{\tiny 1D-M29:}

$\hat{n}_{13}=0.94\hat{i}-0.34\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{14}=0.36\hat{i}+0.32\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.14\hat{i}-0.99\hat{j}-0.03\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.04\hat{i}+4.16\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{24}=3.09\hat{i}+4.06\hat{j}+2.83\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result3.tex <==
{\tiny 1D-M3:}

$\hat{n}_{13}=-0.03\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.68\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}-0.37\hat{j}+0.44\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result30.tex <==
{\tiny 1D-M30:}

$\hat{n}_{13}=0.0\hat{i}+0.53\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{14}=0.04\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.2\hat{j}+0.79\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result31.tex <==
{\tiny 1D-M31:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.61\hat{i}+0.72\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.74\hat{i}+0.66\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result32.tex <==
{\tiny 1D-M32:}

$\hat{n}_{13}=0.49\hat{i}-0.6\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}+0.25\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{24}=-0.85\hat{i}-0.47\hat{j}-0.22\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result33.tex <==
{\tiny 1D-M33:}

$\hat{n}_{13}=-0.66\hat{i}-0.58\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}+0.44\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{24}=-0.63\hat{i}+0.22\hat{j}+0.75\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result34.tex <==
{\tiny 1D-M34:}

$\hat{n}_{13}=-0.74\hat{i}-0.6\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.35\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.27\hat{i}-0.91\hat{j}-0.32\hat{k}$,\;\;\;$\vec{r}_{13}=1.42\hat{i}+3.47\hat{j}+4.31\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=4.36\hat{i}+8.23\hat{j}+4.01\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result35.tex <==
{\tiny 1D-M35:}

$\hat{n}_{13}=-0.42\hat{i}-0.91\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{14}=0.43\hat{i}+0.25\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{24}=-0.22\hat{i}-0.98\hat{j}-0.01\hat{k}$,\;\;\;$\vec{r}_{13}=4.89\hat{i}+4.28\hat{j}+3.84\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.55\hat{i}+6.12\hat{j}+6.81\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result36.tex <==
{\tiny 1D-M36:}

$\hat{n}_{13}=-0.44\hat{i}-0.72\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{14}=0.83\hat{i}+0.56\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}+0.17\hat{j}+0.83\hat{k}$,\;\;\;$\vec{r}_{13}=4.07\hat{i}+7.49\hat{j}+8.26\hat{k}$,\;\;\;$\vec{r}_{23}=7.9\hat{i}+3.19\hat{j}+5.34\hat{k}$,\;\;\;$\vec{r}_{24}=0.9\hat{i}+1.12\hat{j}+1.36\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result37.tex <==
{\tiny 1D-M37:}

$\hat{n}_{13}=0.01\hat{i}-0.41\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{14}=0.75\hat{i}+0.56\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=0.01\hat{i}+0.03\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{13}=8.51\hat{i}+5.61\hat{j}+9.3\hat{k}$,\;\;\;$\vec{r}_{23}=6.97\hat{i}+5.83\hat{j}+8.15\hat{k}$,\;\;\;$\vec{r}_{24}=8.79\hat{i}+9.89\hat{j}+0.01\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result38.tex <==
{\tiny 1D-M38:}

$\hat{n}_{13}=0.61\hat{i}-0.54\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.37\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=0.2\hat{i}-0.61\hat{j}+0.77\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result39.tex <==
{\tiny 1D-M39:}

$\hat{n}_{13}=-0.95\hat{i}-0.16\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.7\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.9\hat{j}-0.45\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result4.tex <==
{\tiny 1D-M4:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.8\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}+0.6\hat{j}+0.6\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result40.tex <==
{\tiny 1D-M40:}

$\hat{n}_{14}=0.16\hat{i}+0.79\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{23}=-0.6\hat{i}-0.8\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.67\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{13}=1.1\hat{i}+4.9\hat{j}+2.13\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=2.1\hat{i}+1.07\hat{j}+6.29\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result41.tex <==
{\tiny 1D-M41:}

$\hat{n}_{14}=-0.38\hat{i}+0.38\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{23}=-0.1\hat{i}-0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.15\hat{i}-0.92\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{13}=2.65\hat{i}+4.93\hat{j}+7.29\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.5\hat{i}+6.06\hat{j}+4.36\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result42.tex <==
{\tiny 1D-M42:}

$\hat{n}_{14}=0.03\hat{i}+0.04\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.33\hat{i}+0.27\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{24}=0.54\hat{i}+0.31\hat{j}-0.78\hat{k}$,\;\;\;$\vec{r}_{13}=6.21\hat{i}+5.74\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{23}=9.31\hat{i}+7.29\hat{j}+7.38\hat{k}$,\;\;\;$\vec{r}_{24}=0.63\hat{i}+8.6\hat{j}+9.34\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result43.tex <==
{\tiny 1D-M43:}

$\hat{n}_{14}=-0.04\hat{i}-0.47\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{23}=0.88\hat{i}+0.43\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.36\hat{j}-0.9\hat{k}$,\;\;\;$\vec{r}_{13}=1.34\hat{i}+0.31\hat{j}+9.39\hat{k}$,\;\;\;$\vec{r}_{23}=3.01\hat{i}+2.96\hat{j}+3.33\hat{k}$,\;\;\;$\vec{r}_{24}=4.67\hat{i}+6.48\hat{j}+0.25\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result44.tex <==
{\tiny 1D-M44:}

$\hat{n}_{14}=-0.44\hat{i}-0.37\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.69\hat{i}-0.73\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result45.tex <==
{\tiny 1D-M45:}

$\hat{n}_{14}=-0.8\hat{i}-0.26\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.17\hat{i}+0.78\hat{j}-0.61\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result46.tex <==
{\tiny 1D-M46:}

$\hat{n}_{12}=-0.15\hat{i}+0.71\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{13}=-0.42\hat{i}-0.63\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.75\hat{i}+0.29\hat{j}+0.59\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result47.tex <==
{\tiny 1D-M47:}

$\hat{n}_{12}=-0.47\hat{i}+0.81\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.67\hat{i}+0.08\hat{j}-0.74\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result48.tex <==
{\tiny 1D-M48:}

$\hat{n}_{12}=-0.78\hat{i}+0.61\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}-0.61\hat{j}+0.34\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+1.46\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result49.tex <==
{\tiny 1D-M49:}

$\hat{n}_{12}=-0.0\hat{i}+0.94\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.69\hat{j}-0.0\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result5.tex <==
{\tiny 1D-M5:}

$\hat{n}_{13}=-0.08\hat{i}+0.46\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{23}=0.61\hat{i}-0.33\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.79\hat{i}-0.58\hat{j}-0.19\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result50.tex <==
{\tiny 1D-M50:}

$\hat{n}_{12}=0.82\hat{i}-0.44\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.6\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result51.tex <==
{\tiny 1D-M51:}

$\hat{n}_{12}=-0.0\hat{i}+0.62\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.53\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{34}=0.77\hat{i}+0.44\hat{j}+0.47\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result52.tex <==
{\tiny 1D-M52:}

$\hat{n}_{12}=0.69\hat{i}+0.51\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{13}=-0.91\hat{i}-0.28\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result53.tex <==
{\tiny 1D-M53:}

$\hat{n}_{12}=0.61\hat{i}-0.05\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{13}=-0.65\hat{i}-0.37\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{34}=-0.61\hat{i}+0.5\hat{j}+0.61\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result54.tex <==
{\tiny 1D-M54:}

$\hat{n}_{12}=-0.86\hat{i}+0.41\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}-0.48\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}+0.26\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result55.tex <==
{\tiny 1D-M55:}

$\hat{n}_{12}=-0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.96\hat{i}+0.16\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result56.tex <==
{\tiny 1D-M56:}

$\hat{n}_{12}=-0.74\hat{i}+0.08\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=0.77\hat{i}-0.64\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result57.tex <==
{\tiny 1D-M57:}

$\hat{n}_{12}=0.0\hat{i}+0.79\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{24}=0.6\hat{i}+0.48\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result58.tex <==
{\tiny 1D-M58:}

$\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result59.tex <==
{\tiny 1D-M59:}

$\hat{n}_{13}=0.57\hat{i}-0.61\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.66\hat{j}-0.41\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=1.65\hat{i}+1.14\hat{j}+3.04\hat{k}$,\;\;\;$\vec{r}_{24}=3.29\hat{i}+6.44\hat{j}+8.8\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result6.tex <==
{\tiny 1D-M6:}

$\hat{n}_{13}=0.0\hat{i}+0.37\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{23}=0.33\hat{i}-0.66\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{24}=0.84\hat{i}-0.53\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result60.tex <==
{\tiny 1D-M60:}

$\hat{n}_{14}=0.62\hat{i}-0.06\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}-0.53\hat{j}+0.46\hat{k}$,\;\;\;$\vec{r}_{13}=7.06\hat{i}+6.93\hat{j}+6.95\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=2.75\hat{i}+2.12\hat{j}+7.47\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result61.tex <==
{\tiny 1D-M61:}

$\hat{n}_{14}=-0.32\hat{i}-0.19\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}+0.79\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{13}=5.17\hat{i}+7.03\hat{j}+1.54\hat{k}$,\;\;\;$\vec{r}_{23}=9.53\hat{i}+5.41\hat{j}+6.8\hat{k}$,\;\;\;$\vec{r}_{24}=0.37\hat{i}+8.09\hat{j}+7.49\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result62.tex <==
{\tiny 1D-M62:}

$\hat{n}_{12}=0.28\hat{i}+0.64\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.52\hat{j}+0.85\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result63.tex <==
{\tiny 1D-M63:}

$\hat{n}_{12}=-0.46\hat{i}-0.43\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.07\hat{i}-0.66\hat{j}-0.75\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result64.tex <==
{\tiny 1D-M64:}

$\hat{n}_{13}=-0.23\hat{i}+0.23\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.59\hat{i}-0.59\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=0.43\hat{i}-0.43\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.01\hat{i}+5.01\hat{j}+5.01\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result65.tex <==
{\tiny 1D-M65:}

$\hat{n}_{13}=0.31\hat{i}-0.63\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.02\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.89\hat{i}-0.46\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{24}=0.33\hat{i}-0.63\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=5.12\hat{i}+4.88\hat{j}+5.02\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.82\hat{i}+4.82\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{24}=4.86\hat{i}+5.18\hat{j}+4.92\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result66.tex <==
{\tiny 1D-M66:}

$\hat{n}_{13}=0.61\hat{i}-0.61\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.59\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.31\hat{i}-0.31\hat{j}-0.9\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.06\hat{i}+5.03\hat{j}+5.17\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result67.tex <==
{\tiny 1D-M67:}

$\hat{n}_{13}=-0.58\hat{i}+0.8\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.86\hat{i}-0.52\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{24}=-0.44\hat{i}-0.89\hat{j}-0.05\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+3.07\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result68.tex <==
{\tiny 1D-M68:}

$\hat{n}_{12}=0.34\hat{i}-0.89\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{13}=0.56\hat{i}+0.34\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.82\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.85\hat{i}+0.27\hat{j}-0.44\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result69.tex <==
{\tiny 1D-M69:}

$\hat{n}_{12}=-0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}-0.44\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.61\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{34}=-0.82\hat{i}-0.32\hat{j}+0.48\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result7.tex <==
{\tiny 1D-M7:}

$\hat{n}_{13}=-0.21\hat{i}-0.95\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{14}=0.41\hat{i}-0.48\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}-0.96\hat{j}+0.24\hat{k}$,\;\;\;$\vec{r}_{13}=5.38\hat{i}+6.86\hat{j}+4.63\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.61\hat{i}+5.26\hat{j}+5.64\hat{k}$,\;\;\;$\vec{r}_{24}=5.08\hat{i}+5.88\hat{j}+3.64\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result70.tex <==
{\tiny 1D-M70:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.05\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result71.tex <==
{\tiny 1D-M71:}

$\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.12\hat{i}+0.76\hat{j}+0.64\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result72.tex <==
{\tiny 1D-M72:}

$\hat{n}_{13}=-0.21\hat{i}-0.79\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.21\hat{i}+0.79\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result73.tex <==
{\tiny 1D-M73:}

$\hat{n}_{13}=-0.3\hat{i}+0.81\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.3\hat{i}+0.81\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result74.tex <==
{\tiny 1D-M74:}

$\hat{n}_{13}=-0.62\hat{i}-0.77\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result75.tex <==
{\tiny 1D-M75:}

$\hat{n}_{13}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result76.tex <==
{\tiny 1D-M76:}

$\hat{n}_{13}=-0.42\hat{i}-0.11\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{14}=-0.55\hat{i}-0.55\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=-0.4\hat{i}-0.63\hat{j}-0.66\hat{k}$,\;\;\;$\vec{r}_{13}=6.6\hat{i}+0.48\hat{j}+3.49\hat{k}$,\;\;\;$\vec{r}_{24}=4.51\hat{i}+2.41\hat{j}+7.15\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result77.tex <==
{\tiny 1D-M77:}

$\hat{n}_{13}=0.68\hat{i}+0.58\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{14}=-0.84\hat{i}+0.51\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.09\hat{i}+0.07\hat{j}-0.99\hat{k}$,\;\;\;$\vec{r}_{13}=5.88\hat{i}+3.66\hat{j}+8.07\hat{k}$,\;\;\;$\vec{r}_{23}=5.04\hat{i}+4.9\hat{j}+8.77\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result78.tex <==
{\tiny 1D-M78:}

$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result79.tex <==
{\tiny 1D-M79:}

$\hat{n}_{14}=-0.3\hat{i}-0.22\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{23}=0.35\hat{i}+0.04\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=0.17\hat{i}-0.24\hat{j}+0.96\hat{k}$,\;\;\;$\vec{r}_{13}=1.22\hat{i}+2.68\hat{j}+2.58\hat{k}$,\;\;\;$\vec{r}_{24}=3.32\hat{i}+1.52\hat{j}+3.48\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result8.tex <==
{\tiny 1D-M8:}

$\hat{n}_{13}=-0.72\hat{i}-0.39\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=0.31\hat{i}-0.9\hat{j}+0.29\hat{k}$,\;\;\;$\hat{n}_{24}=-0.04\hat{i}-1.0\hat{j}+0.06\hat{k}$,\;\;\;$\vec{r}_{13}=6.43\hat{i}+4.57\hat{j}+5.96\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=3.69\hat{i}+6.29\hat{j}+5.5\hat{k}$,\;\;\;$\vec{r}_{24}=5.32\hat{i}+3.65\hat{j}+6.36\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result80.tex <==
{\tiny 1D-M80:}

$\hat{n}_{14}=-0.07\hat{i}+0.16\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{23}=0.48\hat{i}-0.66\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.04\hat{i}+0.14\hat{j}+0.99\hat{k}$,\;\;\;$\vec{r}_{13}=3.42\hat{i}+7.36\hat{j}+7.95\hat{k}$,\;\;\;$\vec{r}_{23}=5.45\hat{i}+6.86\hat{j}+8.94\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result81.tex <==
{\tiny 1D-M81:}

$\hat{n}_{14}=-0.66\hat{i}+0.09\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{23}=-0.66\hat{i}+0.09\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result82.tex <==
{\tiny 1D-M82:}

$\hat{n}_{12}=-0.67\hat{i}+0.45\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}-0.61\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result83.tex <==
{\tiny 1D-M83:}

$\hat{n}_{12}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+9.32\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.29\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result84.tex <==
{\tiny 1D-M84:}

$\hat{n}_{12}=-0.57\hat{i}-0.49\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.6\hat{j}+0.56\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result85.tex <==
{\tiny 1D-M85:}

$\hat{n}_{12}=-0.77\hat{i}-0.61\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.01\hat{i}-0.7\hat{j}+0.71\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result86.tex <==
{\tiny 1D-M86:}

$\hat{n}_{12}=0.58\hat{i}-0.81\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.75\hat{i}-0.66\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+1.51\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+6.87\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result87.tex <==
{\tiny 1D-M87:}

$\hat{n}_{12}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.55\hat{j}+0.6\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result88.tex <==
{\tiny 1D-M88:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result89.tex <==
{\tiny 1D-M89:}

$\hat{n}_{14}=0.0\hat{i}-0.36\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.26\hat{j}-0.64\hat{k}$,\;\;\;$\vec{r}_{13}=8.34\hat{i}+6.1\hat{j}+5.75\hat{k}$,\;\;\;$\vec{r}_{23}=3.26\hat{i}+4.56\hat{j}+7.14\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result9.tex <==
{\tiny 1D-M9:}

$\hat{n}_{13}=0.44\hat{i}+0.64\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=0.15\hat{i}+0.42\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{24}=0.5\hat{i}+0.61\hat{j}-0.62\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result90.tex <==
{\tiny 1D-M90:}

$\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.92\hat{j}+0.38\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result91.tex <==
{\tiny 1D-M91:}

$\hat{n}_{13}=-0.24\hat{i}-0.85\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{14}=-0.24\hat{i}-0.85\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{23}=-0.35\hat{i}-0.37\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.91\hat{i}-0.37\hat{j}-0.21\hat{k}$,\;\;\;$\vec{r}_{14}=4.82\hat{i}+5.35\hat{j}+4.24\hat{k}$,\;\;\;$\vec{r}_{23}=5.77\hat{i}+5.14\hat{j}+4.2\hat{k}$,\;\;\;$\vec{r}_{24}=5.35\hat{i}+5.81\hat{j}+5.53\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result92.tex <==
{\tiny 1D-M92:}

$\hat{n}_{13}=-0.05\hat{i}-0.21\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{14}=0.19\hat{i}+0.29\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{23}=0.16\hat{i}+0.12\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.67\hat{j}+0.2\hat{k}$,\;\;\;$\vec{r}_{13}=8.59\hat{i}+9.74\hat{j}+5.71\hat{k}$,\;\;\;$\vec{r}_{23}=9.97\hat{i}+5.54\hat{j}+5.15\hat{k}$,\;\;\;$\vec{r}_{24}=3.31\hat{i}+4.3\hat{j}+4.92\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result93.tex <==
{\tiny 1D-M93:}

$\hat{n}_{13}=-0.63\hat{i}+0.17\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=0.76\hat{i}-0.05\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{23}=0.76\hat{i}-0.05\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{24}=-0.14\hat{i}-0.98\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{13}=5.68\hat{i}+5.82\hat{j}+5.13\hat{k}$,\;\;\;$\vec{r}_{14}=4.08\hat{i}+5.92\hat{j}+4.4\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+5.32\hat{j}+5.78\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result94.tex <==
{\tiny 1D-M94:}

$\hat{n}_{13}=0.4\hat{i}-0.48\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{14}=0.26\hat{i}-0.75\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{23}=-0.88\hat{i}-0.45\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.75\hat{j}-0.61\hat{k}$,\;\;\;$\vec{r}_{13}=4.92\hat{i}+4.88\hat{j}+5.04\hat{k}$,\;\;\;$\vec{r}_{14}=4.81\hat{i}+4.88\hat{j}+4.88\hat{k}$,\;\;\;$\vec{r}_{23}=4.93\hat{i}+4.88\hat{j}+5.07\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result95.tex <==
{\tiny 1D-M95:}

$\hat{n}_{12}=-0.89\hat{i}-0.29\hat{j}-0.36\hat{k}$,\;\;\;$\hat{n}_{13}=0.66\hat{i}+0.57\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{24}=-0.16\hat{i}-0.53\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.63\hat{j}+0.26\hat{k}$,\;\;\;$\vec{r}_{13}=4.73\hat{i}+4.26\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+5.47\hat{j}+4.87\hat{k}$,\;\;\;$\vec{r}_{34}=4.74\hat{i}+5.76\hat{j}+4.86\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof1/result96.tex <==
{\tiny 1D-M96:}

$\hat{n}_{12}=-0.52\hat{i}-0.13\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{13}=0.7\hat{i}-0.64\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.18\hat{i}-0.95\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{34}=-0.49\hat{i}-0.76\hat{j}-0.42\hat{k}$,\;\;\;$\vec{r}_{12}=3.53\hat{i}+7.37\hat{j}+5.85\hat{k}$,\;\;\;$\vec{r}_{13}=7.27\hat{i}+7.33\hat{j}+2.16\hat{k}$,\;\;\;$\vec{r}_{34}=3.23\hat{i}+6.27\hat{j}+4.91\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result1.tex <==
Manipulator 1:

$\vec{r}_{12}=0.0\hat{i}+8.21\hat{j}+10.0\hat{k}$\newline
$\vec{r}_{23}=0.02\hat{i}+7.16\hat{j}+6.31\hat{k}$\newline
$\hat{n}_{23}=-0.29\hat{i}-0.45\hat{j}-0.85\hat{k}$\newline
$\hat{n}_{12}=-0.31\hat{i}+0.15\hat{j}+0.94\hat{k}$



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result1_full.tex <==


{\tiny 1D-M1:}   $\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.02\hat{i}-0.52\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=0.75\hat{i}-0.51\hat{j}+0.42\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.53\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M2:}   $\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.77\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{24}=0.29\hat{i}+0.95\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M3:}   $\hat{n}_{13}=-0.03\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.68\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}-0.37\hat{j}+0.44\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M4:}   $\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.8\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}+0.6\hat{j}+0.6\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M5:}   $\hat{n}_{13}=-0.08\hat{i}+0.46\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{23}=0.61\hat{i}-0.33\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.79\hat{i}-0.58\hat{j}-0.19\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M6:}   $\hat{n}_{13}=0.0\hat{i}+0.37\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{23}=0.33\hat{i}-0.66\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{24}=0.84\hat{i}-0.53\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M7:}   $\hat{n}_{13}=-0.21\hat{i}-0.95\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{14}=0.41\hat{i}-0.48\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}-0.96\hat{j}+0.24\hat{k}$,\;\;\;$\vec{r}_{13}=5.38\hat{i}+6.86\hat{j}+4.63\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.61\hat{i}+5.26\hat{j}+5.64\hat{k}$,\;\;\;$\vec{r}_{24}=5.08\hat{i}+5.88\hat{j}+3.64\hat{k}$.

{\tiny 1D-M8:}   $\hat{n}_{13}=-0.72\hat{i}-0.39\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=0.31\hat{i}-0.9\hat{j}+0.29\hat{k}$,\;\;\;$\hat{n}_{24}=-0.04\hat{i}-1.0\hat{j}+0.06\hat{k}$,\;\;\;$\vec{r}_{13}=6.43\hat{i}+4.57\hat{j}+5.96\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=3.69\hat{i}+6.29\hat{j}+5.5\hat{k}$,\;\;\;$\vec{r}_{24}=5.32\hat{i}+3.65\hat{j}+6.36\hat{k}$.

{\tiny 1D-M9:}   $\hat{n}_{13}=0.44\hat{i}+0.64\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=0.15\hat{i}+0.42\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{24}=0.5\hat{i}+0.61\hat{j}-0.62\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M10:}\label{result_1_10}   $\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.84\hat{i}-0.49\hat{j}-0.25\hat{k}$,\;\;\;$\vec{r}_{13}=3.76\hat{i}+5.51\hat{j}+5.34\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+1.6\hat{k}$,\;\;\;$\vec{r}_{23}=4.11\hat{i}+6.4\hat{j}+4.81\hat{k}$,\;\;\;$\vec{r}_{24}=4.67\hat{i}+3.62\hat{j}+5.9\hat{k}$.

{\tiny 1D-M11:}   $\hat{n}_{14}=0.16\hat{i}-0.66\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{23}=0.89\hat{i}-0.47\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{24}=-0.96\hat{i}-0.28\hat{j}-0.02\hat{k}$,\;\;\;$\vec{r}_{13}=2.15\hat{i}+6.75\hat{j}+2.1\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=1.36\hat{i}+8.7\hat{j}+7.55\hat{k}$,\;\;\;$\vec{r}_{24}=4.88\hat{i}+4.39\hat{j}+4.5\hat{k}$.

{\tiny 1D-M12:}   $\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.76\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{24}=0.21\hat{i}-0.79\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+2.63\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M13:}   $\hat{n}_{12}=-0.82\hat{i}-0.54\hat{j}+0.19\hat{k}$,\;\;\;$\hat{n}_{13}=0.82\hat{i}+0.0\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.03\hat{i}-0.82\hat{j}-0.57\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M14:}   $\hat{n}_{12}=0.59\hat{i}-0.79\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}+0.02\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.57\hat{j}-0.59\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M15:}   $\hat{n}_{12}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{13}=0.88\hat{i}-0.37\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.69\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M16:}   $\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.45\hat{k}$.

{\tiny 1D-M17:}   $\hat{n}_{12}=0.47\hat{i}-0.44\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{24}=0.11\hat{i}+0.39\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{34}=0.69\hat{i}-0.19\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M18:}   $\hat{n}_{12}=0.08\hat{i}-0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.45\hat{i}-0.53\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{34}=0.39\hat{i}-0.82\hat{j}-0.42\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M19:}   $\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.77\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M20:}   $\hat{n}_{14}=-0.62\hat{i}+0.73\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{24}=0.59\hat{i}-0.56\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=4.05\hat{i}+6.66\hat{j}+3.38\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.38\hat{i}+5.09\hat{j}+3.57\hat{k}$,\;\;\;$\vec{r}_{24}=6.45\hat{i}+6.22\hat{j}+5.3\hat{k}$.

{\tiny 1D-M21:}   $\hat{n}_{12}=0.78\hat{i}-0.25\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M22:}   $\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M23:}   $\hat{n}_{13}=0.77\hat{i}+0.0\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.92\hat{j}-0.38\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M24:}   $\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M25:}   $\hat{n}_{13}=0.16\hat{i}+0.61\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{14}=-0.8\hat{i}+0.54\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M26:}   $\hat{n}_{13}=-0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.56\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{24}=0.81\hat{i}+0.46\hat{j}-0.36\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M27:}   $\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}-0.6\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+2.83\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M28:}   $\hat{n}_{13}=-0.08\hat{i}-0.95\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.44\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+7.16\hat{k}$,\;\;\;$\vec{r}_{23}=4.62\hat{i}+3.55\hat{j}+4.57\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+4.87\hat{j}+4.55\hat{k}$.

{\tiny 1D-M29:}   $\hat{n}_{13}=0.94\hat{i}-0.34\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{14}=0.36\hat{i}+0.32\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.14\hat{i}-0.99\hat{j}-0.03\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.04\hat{i}+4.16\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{24}=3.09\hat{i}+4.06\hat{j}+2.83\hat{k}$.

{\tiny 1D-M30:}   $\hat{n}_{13}=0.0\hat{i}+0.53\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{14}=0.04\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.2\hat{j}+0.79\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M31:}   $\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.61\hat{i}+0.72\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.74\hat{i}+0.66\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M32:}   $\hat{n}_{13}=0.49\hat{i}-0.6\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}+0.25\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{24}=-0.85\hat{i}-0.47\hat{j}-0.22\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M33:}   $\hat{n}_{13}=-0.66\hat{i}-0.58\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}+0.44\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{24}=-0.63\hat{i}+0.22\hat{j}+0.75\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M34:}   $\hat{n}_{13}=-0.74\hat{i}-0.6\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.35\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.27\hat{i}-0.91\hat{j}-0.32\hat{k}$,\;\;\;$\vec{r}_{13}=1.42\hat{i}+3.47\hat{j}+4.31\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=4.36\hat{i}+8.23\hat{j}+4.01\hat{k}$.

{\tiny 1D-M35:}   $\hat{n}_{13}=-0.42\hat{i}-0.91\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{14}=0.43\hat{i}+0.25\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{24}=-0.22\hat{i}-0.98\hat{j}-0.01\hat{k}$,\;\;\;$\vec{r}_{13}=4.89\hat{i}+4.28\hat{j}+3.84\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.55\hat{i}+6.12\hat{j}+6.81\hat{k}$.

{\tiny 1D-M36:}   $\hat{n}_{13}=-0.44\hat{i}-0.72\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{14}=0.83\hat{i}+0.56\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}+0.17\hat{j}+0.83\hat{k}$,\;\;\;$\vec{r}_{13}=4.07\hat{i}+7.49\hat{j}+8.26\hat{k}$,\;\;\;$\vec{r}_{23}=7.9\hat{i}+3.19\hat{j}+5.34\hat{k}$,\;\;\;$\vec{r}_{24}=0.9\hat{i}+1.12\hat{j}+1.36\hat{k}$.

{\tiny 1D-M37:}   $\hat{n}_{13}=0.01\hat{i}-0.41\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{14}=0.75\hat{i}+0.56\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=0.01\hat{i}+0.03\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{13}=8.51\hat{i}+5.61\hat{j}+9.3\hat{k}$,\;\;\;$\vec{r}_{23}=6.97\hat{i}+5.83\hat{j}+8.15\hat{k}$,\;\;\;$\vec{r}_{24}=8.79\hat{i}+9.89\hat{j}+0.01\hat{k}$.

{\tiny 1D-M38:}   $\hat{n}_{13}=0.61\hat{i}-0.54\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.37\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=0.2\hat{i}-0.61\hat{j}+0.77\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M39:}   $\hat{n}_{13}=-0.95\hat{i}-0.16\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.7\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.9\hat{j}-0.45\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M40:}   $\hat{n}_{14}=0.16\hat{i}+0.79\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{23}=-0.6\hat{i}-0.8\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.67\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{13}=1.1\hat{i}+4.9\hat{j}+2.13\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=2.1\hat{i}+1.07\hat{j}+6.29\hat{k}$.

{\tiny 1D-M41:}   $\hat{n}_{14}=-0.38\hat{i}+0.38\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{23}=-0.1\hat{i}-0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.15\hat{i}-0.92\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{13}=2.65\hat{i}+4.93\hat{j}+7.29\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.5\hat{i}+6.06\hat{j}+4.36\hat{k}$.

{\tiny 1D-M42:}   $\hat{n}_{14}=0.03\hat{i}+0.04\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.33\hat{i}+0.27\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{24}=0.54\hat{i}+0.31\hat{j}-0.78\hat{k}$,\;\;\;$\vec{r}_{13}=6.21\hat{i}+5.74\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{23}=9.31\hat{i}+7.29\hat{j}+7.38\hat{k}$,\;\;\;$\vec{r}_{24}=0.63\hat{i}+8.6\hat{j}+9.34\hat{k}$.

{\tiny 1D-M43:}   $\hat{n}_{14}=-0.04\hat{i}-0.47\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{23}=0.88\hat{i}+0.43\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.36\hat{j}-0.9\hat{k}$,\;\;\;$\vec{r}_{13}=1.34\hat{i}+0.31\hat{j}+9.39\hat{k}$,\;\;\;$\vec{r}_{23}=3.01\hat{i}+2.96\hat{j}+3.33\hat{k}$,\;\;\;$\vec{r}_{24}=4.67\hat{i}+6.48\hat{j}+0.25\hat{k}$.

{\tiny 1D-M44:}   $\hat{n}_{14}=-0.44\hat{i}-0.37\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.69\hat{i}-0.73\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M45:}   $\hat{n}_{14}=-0.8\hat{i}-0.26\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.17\hat{i}+0.78\hat{j}-0.61\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M46:}   $\hat{n}_{12}=-0.15\hat{i}+0.71\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{13}=-0.42\hat{i}-0.63\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.75\hat{i}+0.29\hat{j}+0.59\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M47:}   $\hat{n}_{12}=-0.47\hat{i}+0.81\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.67\hat{i}+0.08\hat{j}-0.74\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M48:}   $\hat{n}_{12}=-0.78\hat{i}+0.61\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}-0.61\hat{j}+0.34\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+1.46\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M49:}   $\hat{n}_{12}=-0.0\hat{i}+0.94\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.69\hat{j}-0.0\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M50:}   $\hat{n}_{12}=0.82\hat{i}-0.44\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.6\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M51:}   $\hat{n}_{12}=-0.0\hat{i}+0.62\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.53\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{34}=0.77\hat{i}+0.44\hat{j}+0.47\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M52:}   $\hat{n}_{12}=0.69\hat{i}+0.51\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{13}=-0.91\hat{i}-0.28\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M53:}   $\hat{n}_{12}=0.61\hat{i}-0.05\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{13}=-0.65\hat{i}-0.37\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{34}=-0.61\hat{i}+0.5\hat{j}+0.61\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M54:}   $\hat{n}_{12}=-0.86\hat{i}+0.41\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}-0.48\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}+0.26\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M55:}   $\hat{n}_{12}=-0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.96\hat{i}+0.16\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M56:}   $\hat{n}_{12}=-0.74\hat{i}+0.08\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=0.77\hat{i}-0.64\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M57:}   $\hat{n}_{12}=0.0\hat{i}+0.79\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{24}=0.6\hat{i}+0.48\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M58:}   $\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M59:}   $\hat{n}_{13}=0.57\hat{i}-0.61\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.66\hat{j}-0.41\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=1.65\hat{i}+1.14\hat{j}+3.04\hat{k}$,\;\;\;$\vec{r}_{24}=3.29\hat{i}+6.44\hat{j}+8.8\hat{k}$.

{\tiny 1D-M60:}   $\hat{n}_{14}=0.62\hat{i}-0.06\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}-0.53\hat{j}+0.46\hat{k}$,\;\;\;$\vec{r}_{13}=7.06\hat{i}+6.93\hat{j}+6.95\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=2.75\hat{i}+2.12\hat{j}+7.47\hat{k}$.

{\tiny 1D-M61:}   $\hat{n}_{14}=-0.32\hat{i}-0.19\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}+0.79\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{13}=5.17\hat{i}+7.03\hat{j}+1.54\hat{k}$,\;\;\;$\vec{r}_{23}=9.53\hat{i}+5.41\hat{j}+6.8\hat{k}$,\;\;\;$\vec{r}_{24}=0.37\hat{i}+8.09\hat{j}+7.49\hat{k}$.

{\tiny 1D-M62:}   $\hat{n}_{12}=0.28\hat{i}+0.64\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.52\hat{j}+0.85\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M63:}   $\hat{n}_{12}=-0.46\hat{i}-0.43\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.07\hat{i}-0.66\hat{j}-0.75\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M64:}   $\hat{n}_{13}=-0.23\hat{i}+0.23\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.59\hat{i}-0.59\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=0.43\hat{i}-0.43\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.01\hat{i}+5.01\hat{j}+5.01\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M65:}\label{result_1_65}   $\hat{n}_{13}=0.31\hat{i}-0.63\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.02\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.89\hat{i}-0.46\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{24}=0.33\hat{i}-0.63\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=5.12\hat{i}+4.88\hat{j}+5.02\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.82\hat{i}+4.82\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{24}=4.86\hat{i}+5.18\hat{j}+4.92\hat{k}$.

{\tiny 1D-M66:}   $\hat{n}_{13}=0.61\hat{i}-0.61\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.59\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.31\hat{i}-0.31\hat{j}-0.9\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.06\hat{i}+5.03\hat{j}+5.17\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M67:}   $\hat{n}_{13}=-0.58\hat{i}+0.8\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.86\hat{i}-0.52\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{24}=-0.44\hat{i}-0.89\hat{j}-0.05\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+3.07\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M68:}   $\hat{n}_{12}=0.34\hat{i}-0.89\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{13}=0.56\hat{i}+0.34\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.82\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.85\hat{i}+0.27\hat{j}-0.44\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M69:}   $\hat{n}_{12}=-0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}-0.44\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.61\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{34}=-0.82\hat{i}-0.32\hat{j}+0.48\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M70:}   $\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.05\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M71:}   $\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.12\hat{i}+0.76\hat{j}+0.64\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M72:}   $\hat{n}_{13}=-0.21\hat{i}-0.79\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.21\hat{i}+0.79\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M73:}   $\hat{n}_{13}=-0.3\hat{i}+0.81\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.3\hat{i}+0.81\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M74:}   $\hat{n}_{13}=-0.62\hat{i}-0.77\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M75:}   $\hat{n}_{13}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M76:}   $\hat{n}_{13}=-0.42\hat{i}-0.11\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{14}=-0.55\hat{i}-0.55\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=-0.4\hat{i}-0.63\hat{j}-0.66\hat{k}$,\;\;\;$\vec{r}_{13}=6.6\hat{i}+0.48\hat{j}+3.49\hat{k}$,\;\;\;$\vec{r}_{24}=4.51\hat{i}+2.41\hat{j}+7.15\hat{k}$.

{\tiny 1D-M77:}   $\hat{n}_{13}=0.68\hat{i}+0.58\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{14}=-0.84\hat{i}+0.51\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.09\hat{i}+0.07\hat{j}-0.99\hat{k}$,\;\;\;$\vec{r}_{13}=5.88\hat{i}+3.66\hat{j}+8.07\hat{k}$,\;\;\;$\vec{r}_{23}=5.04\hat{i}+4.9\hat{j}+8.77\hat{k}$.

{\tiny 1D-M78:}   $\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M79:}   $\hat{n}_{14}=-0.3\hat{i}-0.22\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{23}=0.35\hat{i}+0.04\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=0.17\hat{i}-0.24\hat{j}+0.96\hat{k}$,\;\;\;$\vec{r}_{13}=1.22\hat{i}+2.68\hat{j}+2.58\hat{k}$,\;\;\;$\vec{r}_{24}=3.32\hat{i}+1.52\hat{j}+3.48\hat{k}$.

{\tiny 1D-M80:}   $\hat{n}_{14}=-0.07\hat{i}+0.16\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{23}=0.48\hat{i}-0.66\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.04\hat{i}+0.14\hat{j}+0.99\hat{k}$,\;\;\;$\vec{r}_{13}=3.42\hat{i}+7.36\hat{j}+7.95\hat{k}$,\;\;\;$\vec{r}_{23}=5.45\hat{i}+6.86\hat{j}+8.94\hat{k}$.

{\tiny 1D-M81:}   $\hat{n}_{14}=-0.66\hat{i}+0.09\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{23}=-0.66\hat{i}+0.09\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M82:}   $\hat{n}_{12}=-0.67\hat{i}+0.45\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}-0.61\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M83:}   $\hat{n}_{12}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+9.32\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.29\hat{k}$.

{\tiny 1D-M84:}   $\hat{n}_{12}=-0.57\hat{i}-0.49\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.6\hat{j}+0.56\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M85:}   $\hat{n}_{12}=-0.77\hat{i}-0.61\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.01\hat{i}-0.7\hat{j}+0.71\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M86:}   $\hat{n}_{12}=0.58\hat{i}-0.81\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.75\hat{i}-0.66\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+1.51\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+6.87\hat{k}$.

{\tiny 1D-M87:}   $\hat{n}_{12}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.55\hat{j}+0.6\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M88:}   $\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M89:}   $\hat{n}_{14}=0.0\hat{i}-0.36\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.26\hat{j}-0.64\hat{k}$,\;\;\;$\vec{r}_{13}=8.34\hat{i}+6.1\hat{j}+5.75\hat{k}$,\;\;\;$\vec{r}_{23}=3.26\hat{i}+4.56\hat{j}+7.14\hat{k}$.

{\tiny 1D-M90:}   $\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.92\hat{j}+0.38\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M91:}   $\hat{n}_{13}=-0.24\hat{i}-0.85\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{14}=-0.24\hat{i}-0.85\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{23}=-0.35\hat{i}-0.37\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.91\hat{i}-0.37\hat{j}-0.21\hat{k}$,\;\;\;$\vec{r}_{14}=4.82\hat{i}+5.35\hat{j}+4.24\hat{k}$,\;\;\;$\vec{r}_{23}=5.77\hat{i}+5.14\hat{j}+4.2\hat{k}$,\;\;\;$\vec{r}_{24}=5.35\hat{i}+5.81\hat{j}+5.53\hat{k}$.

{\tiny 1D-M92:}   $\hat{n}_{13}=-0.05\hat{i}-0.21\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{14}=0.19\hat{i}+0.29\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{23}=0.16\hat{i}+0.12\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.67\hat{j}+0.2\hat{k}$,\;\;\;$\vec{r}_{13}=8.59\hat{i}+9.74\hat{j}+5.71\hat{k}$,\;\;\;$\vec{r}_{23}=9.97\hat{i}+5.54\hat{j}+5.15\hat{k}$,\;\;\;$\vec{r}_{24}=3.31\hat{i}+4.3\hat{j}+4.92\hat{k}$.

{\tiny 1D-M93:}   $\hat{n}_{13}=-0.63\hat{i}+0.17\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=0.76\hat{i}-0.05\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{23}=0.76\hat{i}-0.05\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{24}=-0.14\hat{i}-0.98\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{13}=5.68\hat{i}+5.82\hat{j}+5.13\hat{k}$,\;\;\;$\vec{r}_{14}=4.08\hat{i}+5.92\hat{j}+4.4\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+5.32\hat{j}+5.78\hat{k}$.

{\tiny 1D-M94:}   $\hat{n}_{13}=0.4\hat{i}-0.48\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{14}=0.26\hat{i}-0.75\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{23}=-0.88\hat{i}-0.45\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.75\hat{j}-0.61\hat{k}$,\;\;\;$\vec{r}_{13}=4.92\hat{i}+4.88\hat{j}+5.04\hat{k}$,\;\;\;$\vec{r}_{14}=4.81\hat{i}+4.88\hat{j}+4.88\hat{k}$,\;\;\;$\vec{r}_{23}=4.93\hat{i}+4.88\hat{j}+5.07\hat{k}$.

{\tiny 1D-M95:}   $\hat{n}_{12}=-0.89\hat{i}-0.29\hat{j}-0.36\hat{k}$,\;\;\;$\hat{n}_{13}=0.66\hat{i}+0.57\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{24}=-0.16\hat{i}-0.53\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.63\hat{j}+0.26\hat{k}$,\;\;\;$\vec{r}_{13}=4.73\hat{i}+4.26\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+5.47\hat{j}+4.87\hat{k}$,\;\;\;$\vec{r}_{34}=4.74\hat{i}+5.76\hat{j}+4.86\hat{k}$.

{\tiny 1D-M96:}   $\hat{n}_{12}=-0.52\hat{i}-0.13\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{13}=0.7\hat{i}-0.64\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.18\hat{i}-0.95\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{34}=-0.49\hat{i}-0.76\hat{j}-0.42\hat{k}$,\;\;\;$\vec{r}_{12}=3.53\hat{i}+7.37\hat{j}+5.85\hat{k}$,\;\;\;$\vec{r}_{13}=7.27\hat{i}+7.33\hat{j}+2.16\hat{k}$,\;\;\;$\vec{r}_{34}=3.23\hat{i}+6.27\hat{j}+4.91\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result2.tex <==
Manipulator 2:

$\vec{r}_{12}=1.83\hat{i}+2.97\hat{j}+1.26\hat{k}$\newline
$\vec{r}_{23}=0.83\hat{i}+6.09\hat{j}+0.81\hat{k}$\newline
$\hat{n}_{23}=-0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$\newline
$\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result3.tex <==
Manipulator 3:

$\vec{r}_{23}=5.55\hat{i}+9.95\hat{j}+0.02\hat{k}$\newline
$\hat{n}_{23}=0.02\hat{i}+0.79\hat{j}-0.61\hat{k}$\newline
$\hat{n}_{12}=-0.0\hat{i}-0.54\hat{j}-0.84\hat{k}$



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result3_full.tex <==


{\tiny 3D-M1:}\label{result_3_1}   $\hat{n}_{13}=-0.71\hat{i}+0.11\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.46\hat{j}-0.34\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 3D-M2:}   $\hat{n}_{13}=-0.8\hat{i}+0.33\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}+0.67\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.67\hat{j}-0.48\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 3D-M3:}   $\hat{n}_{13}=-0.8\hat{i}+0.58\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{23}=-0.74\hat{i}-0.51\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}+0.16\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 3D-M4:}   $\hat{n}_{13}=-0.57\hat{i}-0.67\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.36\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.76\hat{i}-0.65\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 3D-M5:}   $\hat{n}_{13}=0.5\hat{i}+0.18\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.76\hat{i}-0.61\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{24}=0.03\hat{i}+0.33\hat{j}-0.94\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 3D-M6:}   $\hat{n}_{13}=-0.6\hat{i}-0.76\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=0.26\hat{i}+0.4\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=-0.21\hat{i}-0.17\hat{j}+0.96\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 3D-M7:}   $\hat{n}_{13}=-0.54\hat{i}-0.83\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{23}=0.18\hat{i}-0.26\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{24}=-0.04\hat{i}-0.56\hat{j}-0.83\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 3D-M8:}\label{result_3_8}   $\hat{n}_{13}=0.41\hat{i}+0.89\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}+0.11\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.67\hat{i}+0.44\hat{j}+0.59\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result4.tex <==
Manipulator 4:

$\hat{n}_{23}=0.1\hat{i}-0.12\hat{j}-0.99\hat{k}$\newline
$\hat{n}_{12}=0.0\hat{i}+0.66\hat{j}+0.75\hat{k}$



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result4_full.tex <==


{\tiny 4D-M1:}\label{result_4_1}   $\hat{n}_{14}=-0.29\hat{i}+0.57\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.75\hat{i}-0.53\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.34\hat{i}+0.83\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{34}=-0.72\hat{i}+0.12\hat{j}+0.69\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M2:}   $\hat{n}_{14}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{23}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=-0.42\hat{i}-0.85\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{34}=0.57\hat{i}+0.69\hat{j}+0.45\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M3:}   $\hat{n}_{14}=0.39\hat{i}+0.47\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{23}=-0.42\hat{i}-0.85\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.69\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.49\hat{j}-0.3\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M4:}   $\hat{n}_{14}=0.42\hat{i}+0.85\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{23}=-0.57\hat{i}-0.69\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{25}=-0.39\hat{i}-0.47\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.49\hat{j}-0.3\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M5:}   $\hat{n}_{14}=-0.57\hat{i}-0.69\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}+0.85\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M6:}   $\hat{n}_{14}=-0.54\hat{i}-0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.53\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.81\hat{j}-0.12\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M7:}   $\hat{n}_{14}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.05\hat{i}+0.94\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}+0.22\hat{j}-0.49\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M8:}   $\hat{n}_{14}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}+0.85\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{25}=-0.8\hat{i}-0.46\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M9:}   $\hat{n}_{14}=-0.08\hat{i}-0.96\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{23}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=-0.84\hat{i}-0.08\hat{j}+0.53\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M10:}   $\hat{n}_{14}=-0.63\hat{i}-0.76\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}+0.59\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M11:}   $\hat{n}_{14}=-0.32\hat{i}+0.81\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.78\hat{i}+0.52\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.54\hat{i}+0.84\hat{j}+0.08\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M12:}   $\hat{n}_{14}=0.09\hat{i}-1.0\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{23}=0.67\hat{i}+0.35\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}-0.88\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{34}=-0.75\hat{i}+0.31\hat{j}+0.59\hat{k}$,\;\;\;$\vec{r}_{14}=4.0\hat{i}+2.99\hat{j}+5.94\hat{k}$.

{\tiny 4D-M13:}\label{result_4_13}   $\hat{n}_{14}=-0.94\hat{i}-0.18\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{23}=0.32\hat{i}-0.95\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=-0.03\hat{i}-0.8\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=0.34\hat{i}-0.57\hat{j}-0.75\hat{k}$,\;\;\;$\vec{r}_{23}=7.59\hat{i}+3.33\hat{j}+4.0\hat{k}$.

{\tiny 4D-M14:}   $\hat{n}_{14}=-0.38\hat{i}-0.54\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.53\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=0.34\hat{i}-0.93\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{34}=0.75\hat{i}-0.65\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{25}=3.55\hat{i}+6.33\hat{j}+6.15\hat{k}$.

{\tiny 4D-M15:}   $\hat{n}_{14}=-0.19\hat{i}-0.68\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.56\hat{i}-0.67\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{25}=-0.8\hat{i}-0.3\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}-0.54\hat{j}+0.05\hat{k}$,\;\;\;$\vec{r}_{34}=3.99\hat{i}+5.66\hat{j}+6.62\hat{k}$.

==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result642.tex <==
{\tiny 2D-M642:}

$\hat{n}_{12}=0.05\hat{i}+0.55\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}-0.5\hat{j}-0.28\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result643.tex <==
{\tiny 2D-M643:}

$\hat{n}_{12}=0.73\hat{i}-0.15\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{23}=-0.03\hat{i}-0.63\hat{j}+0.78\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result644.tex <==
{\tiny 2D-M644:}

$\hat{n}_{12}=-0.68\hat{i}-0.48\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{23}=0.55\hat{i}-0.74\hat{j}-0.39\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2/result645.tex <==
{\tiny 2D-M645:}

$\hat{n}_{12}=0.97\hat{i}+0.03\hat{j}+0.24\hat{k}$,\;\;\;$\hat{n}_{23}=0.03\hat{i}-1.0\hat{j}-0.01\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result1.tex <==
{\tiny 2D-M1:}

$\hat{n}_{14}=0.0\hat{i}+0.96\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.32\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=0.1\hat{i}-0.67\hat{j}+0.74\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result10.tex <==
{\tiny 2D-M10:}

$\hat{n}_{14}=0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.57\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result100.tex <==
{\tiny 2D-M100:}

$\hat{n}_{13}=0.86\hat{i}-0.36\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{24}=0.81\hat{i}+0.47\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.05\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.69\hat{j}+0.73\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result101.tex <==
{\tiny 2D-M101:}

$\hat{n}_{13}=-0.5\hat{i}-0.83\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{23}=-0.08\hat{i}-0.53\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.97\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{45}=-0.83\hat{i}-0.4\hat{j}-0.4\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result102.tex <==
{\tiny 2D-M102:}

$\hat{n}_{13}=0.97\hat{i}+0.01\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.36\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=0.48\hat{i}-0.52\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.34\hat{i}-0.57\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result103.tex <==
{\tiny 2D-M103:}

$\hat{n}_{13}=-0.86\hat{i}-0.27\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.68\hat{i}-0.68\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{35}=0.69\hat{i}+0.27\hat{j}-0.67\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result104.tex <==
{\tiny 2D-M104:}

$\hat{n}_{13}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.99\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.39\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}+0.51\hat{j}-0.26\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result105.tex <==
{\tiny 2D-M105:}

$\hat{n}_{14}=-0.0\hat{i}+0.56\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{24}=-0.35\hat{i}+0.49\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.59\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}-0.67\hat{j}-0.13\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result106.tex <==
{\tiny 2D-M106:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.82\hat{i}-0.08\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.6\hat{i}-0.61\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.61\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.01\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result107.tex <==
{\tiny 2D-M107:}

$\hat{n}_{14}=0.53\hat{i}-0.74\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.69\hat{i}+0.12\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{25}=-0.6\hat{i}+0.75\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.63\hat{i}-0.48\hat{j}+0.62\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result108.tex <==
{\tiny 2D-M108:}

$\hat{n}_{14}=0.0\hat{i}+0.64\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.74\hat{i}+0.55\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{35}=-0.54\hat{i}-0.58\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result109.tex <==
{\tiny 2D-M109:}

$\hat{n}_{14}=0.08\hat{i}-0.62\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.67\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.57\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{35}=-0.82\hat{i}+0.38\hat{j}-0.43\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result11.tex <==
{\tiny 2D-M11:}

$\hat{n}_{14}=0.69\hat{i}+0.47\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{34}=0.03\hat{i}-0.89\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{45}=-0.02\hat{i}+0.86\hat{j}+0.5\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=5.17\hat{i}+6.28\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{25}=5.29\hat{i}+3.75\hat{j}+5.48\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result110.tex <==
{\tiny 2D-M110:}

$\hat{n}_{14}=0.82\hat{i}+0.06\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{24}=-0.35\hat{i}-0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{34}=-0.7\hat{i}+0.01\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}+0.58\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result111.tex <==
{\tiny 2D-M111:}

$\hat{n}_{14}=-0.11\hat{i}+0.79\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}-0.33\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{25}=0.66\hat{i}-0.07\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{34}=0.11\hat{i}+0.99\hat{j}-0.08\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result112.tex <==
{\tiny 2D-M112:}

$\hat{n}_{14}=0.32\hat{i}+0.93\hat{j}+0.17\hat{k}$,\;\;\;$\hat{n}_{24}=0.48\hat{i}-0.75\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.65\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{35}=0.19\hat{i}+0.7\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result113.tex <==
{\tiny 2D-M113:}

$\hat{n}_{14}=0.8\hat{i}-0.48\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.95\hat{i}-0.22\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{35}=-0.36\hat{i}+0.36\hat{j}-0.86\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result114.tex <==
{\tiny 2D-M114:}

$\hat{n}_{14}=-0.69\hat{i}+0.71\hat{j}+0.17\hat{k}$,\;\;\;$\hat{n}_{24}=-0.54\hat{i}+0.63\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}+0.7\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result115.tex <==
{\tiny 2D-M115:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.57\hat{i}+0.27\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.86\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{35}=-0.62\hat{i}-0.62\hat{j}-0.48\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+9.95\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result116.tex <==
{\tiny 2D-M116:}

$\hat{n}_{14}=0.76\hat{i}-0.61\hat{j}+0.24\hat{k}$,\;\;\;$\hat{n}_{24}=0.01\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}-0.41\hat{j}-0.4\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result117.tex <==
{\tiny 2D-M117:}

$\hat{n}_{14}=0.23\hat{i}-0.48\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.94\hat{i}-0.33\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{25}=-0.61\hat{i}+0.57\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.69\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result118.tex <==
{\tiny 2D-M118:}

$\hat{n}_{14}=0.02\hat{i}+0.57\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.65\hat{i}-0.75\hat{j}-0.1\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.49\hat{i}-0.32\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result119.tex <==
{\tiny 2D-M119:}

$\hat{n}_{14}=-0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.78\hat{i}+0.01\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{25}=-0.41\hat{i}+0.82\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result12.tex <==
{\tiny 2D-M12:}

$\hat{n}_{14}=0.7\hat{i}+0.53\hat{j}-0.47\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.85\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{25}=-0.05\hat{i}+0.72\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result120.tex <==
{\tiny 2D-M120:}

$\hat{n}_{14}=0.31\hat{i}+0.36\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}-0.4\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=0.83\hat{i}+0.37\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result121.tex <==
{\tiny 2D-M121:}

$\hat{n}_{14}=0.9\hat{i}+0.39\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.93\hat{i}+0.25\hat{j}-0.25\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result122.tex <==
{\tiny 2D-M122:}

$\hat{n}_{14}=-0.66\hat{i}+0.15\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.63\hat{i}+0.55\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=0.77\hat{i}-0.45\hat{j}-0.45\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result123.tex <==
{\tiny 2D-M123:}

$\hat{n}_{14}=0.61\hat{i}+0.04\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.42\hat{i}-0.89\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{34}=0.15\hat{i}+0.62\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result124.tex <==
{\tiny 2D-M124:}

$\hat{n}_{14}=0.25\hat{i}-0.67\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result125.tex <==
{\tiny 2D-M125:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.41\hat{i}-0.82\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{34}=0.31\hat{i}-0.6\hat{j}-0.73\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.67\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result126.tex <==
{\tiny 2D-M126:}

$\hat{n}_{14}=0.43\hat{i}-0.74\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.07\hat{i}-0.94\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{25}=0.07\hat{i}-0.83\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=0.02\hat{i}+0.87\hat{j}+0.5\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=4.06\hat{i}+3.92\hat{j}+4.65\hat{k}$,\;\;\;$\vec{r}_{34}=5.03\hat{i}+4.27\hat{j}+5.76\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result127.tex <==
{\tiny 2D-M127:}

$\hat{n}_{14}=-0.0\hat{i}+0.59\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.72\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{34}=-0.82\hat{i}-0.45\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{45}=-0.06\hat{i}+0.7\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result128.tex <==
{\tiny 2D-M128:}

$\hat{n}_{14}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{23}=-0.2\hat{i}-0.95\hat{j}+0.24\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.81\hat{j}-0.05\hat{k}$,\;\;\;$\hat{n}_{45}=-0.59\hat{i}+0.15\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=6.36\hat{i}+5.69\hat{j}+8.17\hat{k}$,\;\;\;$\vec{r}_{34}=6.17\hat{i}+5.22\hat{j}+2.99\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result129.tex <==
{\tiny 2D-M129:}

$\hat{n}_{14}=-0.71\hat{i}+0.09\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}+0.67\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result13.tex <==
{\tiny 2D-M13:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.07\hat{i}-0.64\hat{j}-0.76\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result130.tex <==
{\tiny 2D-M130:}

$\hat{n}_{14}=-0.53\hat{i}+0.27\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{23}=-0.9\hat{i}+0.11\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.67\hat{i}-0.67\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result131.tex <==
{\tiny 2D-M131:}

$\hat{n}_{14}=-0.09\hat{i}-0.53\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{23}=0.7\hat{i}+0.38\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.69\hat{i}+0.11\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{34}=-0.81\hat{i}+0.56\hat{j}-0.15\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result132.tex <==
{\tiny 2D-M132:}

$\hat{n}_{14}=0.01\hat{i}+0.86\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{23}=0.41\hat{i}-0.89\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{25}=0.09\hat{i}-0.99\hat{j}+0.07\hat{k}$,\;\;\;$\hat{n}_{45}=0.43\hat{i}-0.74\hat{j}+0.51\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=2.99\hat{i}+6.07\hat{j}+3.02\hat{k}$,\;\;\;$\vec{r}_{34}=6.84\hat{i}+4.37\hat{j}+3.84\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result133.tex <==
{\tiny 2D-M133:}

$\hat{n}_{14}=0.81\hat{i}-0.36\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{23}=0.9\hat{i}+0.31\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.44\hat{i}+0.64\hat{j}-0.64\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result134.tex <==
{\tiny 2D-M134:}

$\hat{n}_{14}=0.38\hat{i}+0.67\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.98\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{34}=0.65\hat{i}-0.75\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}-0.1\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.69\hat{i}+5.22\hat{j}+4.09\hat{k}$,\;\;\;$\vec{r}_{25}=3.77\hat{i}+3.77\hat{j}+3.8\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result135.tex <==
{\tiny 2D-M135:}

$\hat{n}_{14}=-0.13\hat{i}+0.65\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{25}=-0.6\hat{i}+0.78\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.56\hat{i}+0.24\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result136.tex <==
{\tiny 2D-M136:}

$\hat{n}_{14}=-0.0\hat{i}+0.57\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{25}=0.69\hat{i}-0.69\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.87\hat{i}+0.21\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.56\hat{j}-0.83\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result137.tex <==
{\tiny 2D-M137:}

$\hat{n}_{14}=-0.43\hat{i}-0.25\hat{j}-0.87\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result138.tex <==
{\tiny 2D-M138:}

$\hat{n}_{14}=0.17\hat{i}-0.5\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{25}=-0.79\hat{i}-0.49\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{34}=-0.35\hat{i}-0.79\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{45}=0.77\hat{i}-0.23\hat{j}+0.6\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.47\hat{i}+3.98\hat{j}+5.17\hat{k}$,\;\;\;$\vec{r}_{34}=9.55\hat{i}+4.3\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result139.tex <==
{\tiny 2D-M139:}

$\hat{n}_{14}=-0.0\hat{i}+0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=0.54\hat{i}-0.14\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{34}=0.17\hat{i}-0.7\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{45}=0.63\hat{i}+0.7\hat{j}-0.34\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result14.tex <==
{\tiny 2D-M14:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}+0.09\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result140.tex <==
{\tiny 2D-M140:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.39\hat{i}+0.27\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{34}=-0.19\hat{i}-0.77\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.74\hat{j}-0.67\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+9.9\hat{k}$,\;\;\;$\vec{r}_{23}=4.36\hat{i}+0.9\hat{j}+3.84\hat{k}$,\;\;\;$\vec{r}_{25}=7.17\hat{i}+1.16\hat{j}+6.63\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result141.tex <==
{\tiny 2D-M141:}

$\hat{n}_{14}=-0.38\hat{i}+0.38\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{15}=0.93\hat{i}-0.2\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.95\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.74\hat{j}+0.67\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result142.tex <==
{\tiny 2D-M142:}

$\hat{n}_{14}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+8.6\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result143.tex <==
{\tiny 2D-M143:}

$\hat{n}_{14}=-0.19\hat{i}+0.78\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{15}=-0.71\hat{i}+0.69\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{23}=-0.68\hat{i}-0.7\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{25}=0.79\hat{i}-0.24\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result144.tex <==
{\tiny 2D-M144:}

$\hat{n}_{14}=0.24\hat{i}+0.8\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{15}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.65\hat{i}+0.74\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{34}=0.9\hat{i}-0.31\hat{j}-0.31\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+9.72\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result145.tex <==
{\tiny 2D-M145:}

$\hat{n}_{14}=0.28\hat{i}-0.8\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{15}=0.69\hat{i}-0.71\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{25}=0.77\hat{i}-0.15\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{34}=0.7\hat{i}+0.68\hat{j}-0.21\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result146.tex <==
{\tiny 2D-M146:}

$\hat{n}_{14}=0.69\hat{i}+0.02\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.43\hat{i}-0.82\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result147.tex <==
{\tiny 2D-M147:}

$\hat{n}_{14}=-0.44\hat{i}-0.86\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.36\hat{i}+0.55\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{25}=0.55\hat{i}-0.62\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{34}=0.54\hat{i}-0.25\hat{j}+0.81\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result148.tex <==
{\tiny 2D-M148:}

$\hat{n}_{14}=0.92\hat{i}+0.25\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{23}=0.14\hat{i}+0.63\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{25}=-0.06\hat{i}+0.68\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{34}=0.59\hat{i}-0.57\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result149.tex <==
{\tiny 2D-M149:}

$\hat{n}_{14}=-0.36\hat{i}+0.55\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{23}=0.55\hat{i}-0.62\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.44\hat{i}+0.86\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{34}=-0.54\hat{i}+0.25\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result15.tex <==
{\tiny 2D-M15:}

$\hat{n}_{13}=-0.46\hat{i}+0.74\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result150.tex <==
{\tiny 2D-M150:}

$\hat{n}_{14}=-0.23\hat{i}+0.48\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.61\hat{i}+0.57\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{34}=-0.94\hat{i}-0.33\hat{j}-0.03\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result151.tex <==
{\tiny 2D-M151:}

$\hat{n}_{14}=0.61\hat{i}-0.2\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.34\hat{i}-0.46\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{25}=0.8\hat{i}+0.48\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{34}=0.62\hat{i}-0.55\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result152.tex <==
{\tiny 2D-M152:}

$\hat{n}_{14}=0.66\hat{i}-0.45\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{23}=-0.5\hat{i}+0.8\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.29\hat{i}+0.06\hat{j}-0.95\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result153.tex <==
{\tiny 2D-M153:}

$\hat{n}_{14}=-0.06\hat{i}+0.99\hat{j}-0.11\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.86\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.73\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result154.tex <==
{\tiny 2D-M154:}

$\hat{n}_{14}=0.49\hat{i}+0.46\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.29\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{25}=-0.55\hat{i}-0.55\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{35}=0.46\hat{i}-0.88\hat{j}-0.05\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result155.tex <==
{\tiny 2D-M155:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.66\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{25}=0.9\hat{i}+0.28\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result156.tex <==
{\tiny 2D-M156:}

$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.73\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.66\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{35}=0.08\hat{i}-0.7\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result157.tex <==
{\tiny 2D-M157:}

$\hat{n}_{14}=-0.0\hat{i}+0.64\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.91\hat{i}+0.32\hat{j}+0.27\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result158.tex <==
{\tiny 2D-M158:}

$\hat{n}_{14}=0.0\hat{i}+0.92\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{24}=0.15\hat{i}+0.34\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{25}=0.44\hat{i}+0.4\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{35}=-0.49\hat{i}-0.72\hat{j}-0.49\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result159.tex <==
{\tiny 2D-M159:}

$\hat{n}_{14}=-0.03\hat{i}+0.83\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{23}=0.54\hat{i}+0.67\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.62\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.1\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result16.tex <==
{\tiny 2D-M16:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.16\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{45}=-0.27\hat{i}+0.32\hat{j}-0.91\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result160.tex <==
{\tiny 2D-M160:}

$\hat{n}_{14}=-0.24\hat{i}-0.94\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{23}=0.65\hat{i}-0.65\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.11\hat{i}-0.7\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{45}=-0.51\hat{i}+0.46\hat{j}+0.73\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result161.tex <==
{\tiny 2D-M161:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.14\hat{i}+0.36\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.48\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{34}=0.66\hat{i}+0.34\hat{j}-0.67\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result162.tex <==
{\tiny 2D-M162:}

$\hat{n}_{14}=0.16\hat{i}+0.5\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{23}=0.65\hat{i}-0.38\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.5\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{45}=0.72\hat{i}-0.35\hat{j}+0.6\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result163.tex <==
{\tiny 2D-M163:}

$\hat{n}_{14}=-0.0\hat{i}+0.64\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.98\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.67\hat{i}-0.3\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.49\hat{j}-0.87\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result164.tex <==
{\tiny 2D-M164:}

$\hat{n}_{14}=0.55\hat{i}+0.44\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}-0.71\hat{j}-0.07\hat{k}$,\;\;\;$\hat{n}_{34}=0.63\hat{i}+0.74\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{45}=-0.73\hat{i}+0.68\hat{j}+0.1\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result165.tex <==
{\tiny 2D-M165:}

$\hat{n}_{14}=-0.98\hat{i}-0.16\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{23}=-0.32\hat{i}-0.84\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.74\hat{i}+0.36\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.65\hat{j}+0.21\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result166.tex <==
{\tiny 2D-M166:}

$\hat{n}_{14}=0.44\hat{i}+0.11\hat{j}-0.89\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.86\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=-0.62\hat{i}+0.14\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.54\hat{j}-0.84\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result167.tex <==
{\tiny 2D-M167:}

$\hat{n}_{14}=-0.83\hat{i}+0.47\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{23}=-0.67\hat{i}-0.68\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{34}=-0.6\hat{i}+0.6\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{45}=0.67\hat{i}-0.57\hat{j}-0.48\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result168.tex <==
{\tiny 2D-M168:}

$\hat{n}_{14}=-0.0\hat{i}+0.74\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.6\hat{i}-0.54\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{34}=-0.64\hat{i}-0.54\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.45\hat{j}-0.89\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result169.tex <==
{\tiny 2D-M169:}

$\hat{n}_{14}=-0.49\hat{i}-0.87\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=0.41\hat{i}+0.91\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.49\hat{i}+0.53\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result17.tex <==
{\tiny 2D-M17:}

$\hat{n}_{13}=0.71\hat{i}-0.11\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result170.tex <==
{\tiny 2D-M170:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.36\hat{i}+0.86\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.92\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result171.tex <==
{\tiny 2D-M171:}

$\hat{n}_{14}=-0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{15}=0.92\hat{i}-0.07\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.48\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result172.tex <==
{\tiny 2D-M172:}

$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{15}=0.0\hat{i}+0.39\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.77\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{34}=-0.8\hat{i}+0.28\hat{j}+0.52\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result173.tex <==
{\tiny 2D-M173:}

$\hat{n}_{14}=0.48\hat{i}+0.68\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{15}=0.02\hat{i}+0.84\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.61\hat{i}-0.78\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.35\hat{j}-0.94\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result174.tex <==
{\tiny 2D-M174:}

$\hat{n}_{14}=0.52\hat{i}-0.77\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{23}=0.4\hat{i}-0.7\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{25}=0.7\hat{i}-0.62\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{34}=0.81\hat{i}+0.29\hat{j}-0.51\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result175.tex <==
{\tiny 2D-M175:}

$\hat{n}_{14}=-0.99\hat{i}+0.16\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{23}=0.8\hat{i}-0.15\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.12\hat{i}-0.53\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{34}=-0.83\hat{i}-0.55\hat{j}-0.09\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result176.tex <==
{\tiny 2D-M176:}

$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.95\hat{i}+0.17\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.22\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{34}=-0.02\hat{i}-0.78\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result177.tex <==
{\tiny 2D-M177:}

$\hat{n}_{14}=0.68\hat{i}+0.71\hat{j}-0.19\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.51\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.26\hat{j}-0.97\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result178.tex <==
{\tiny 2D-M178:}

$\hat{n}_{14}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.87\hat{i}-0.5\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result179.tex <==
{\tiny 2D-M179:}

$\hat{n}_{14}=-0.9\hat{i}-0.44\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.76\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.34\hat{i}+0.93\hat{j}-0.14\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.02\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result18.tex <==
{\tiny 2D-M18:}

$\hat{n}_{13}=-0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.04\hat{i}+0.73\hat{j}+0.68\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result180.tex <==
{\tiny 2D-M180:}

$\hat{n}_{15}=0.92\hat{i}-0.1\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}-0.39\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result181.tex <==
{\tiny 2D-M181:}

$\hat{n}_{15}=-0.71\hat{i}-0.23\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{23}=-0.69\hat{i}+0.02\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{25}=0.68\hat{i}-0.21\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{34}=0.43\hat{i}+0.82\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result182.tex <==
{\tiny 2D-M182:}

$\hat{n}_{15}=-0.62\hat{i}-0.69\hat{j}-0.38\hat{k}$,\;\;\;$\hat{n}_{23}=-0.71\hat{i}+0.67\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{25}=0.78\hat{i}+0.17\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{34}=-0.25\hat{i}-0.8\hat{j}-0.55\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result183.tex <==
{\tiny 2D-M183:}

$\hat{n}_{13}=-0.61\hat{i}-0.5\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{14}=-0.64\hat{i}+0.77\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{25}=0.72\hat{i}-0.69\hat{j}-0.03\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result184.tex <==
{\tiny 2D-M184:}

$\hat{n}_{13}=-0.88\hat{i}-0.06\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{14}=0.48\hat{i}+0.33\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=-0.55\hat{i}-0.59\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{35}=-0.64\hat{i}+0.75\hat{j}-0.19\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result185.tex <==
{\tiny 2D-M185:}

$\hat{n}_{13}=-0.62\hat{i}+0.62\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{14}=0.66\hat{i}-0.03\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.72\hat{i}-0.03\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.57\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result186.tex <==
{\tiny 2D-M186:}

$\hat{n}_{13}=-0.26\hat{i}+0.46\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{14}=-0.66\hat{i}-0.53\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{24}=0.27\hat{i}+0.88\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result187.tex <==
{\tiny 2D-M187:}

$\hat{n}_{13}=0.72\hat{i}-0.48\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{14}=0.8\hat{i}-0.25\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.14\hat{i}+0.67\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{35}=-0.07\hat{i}+0.73\hat{j}-0.68\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result188.tex <==
{\tiny 2D-M188:}

$\hat{n}_{13}=0.0\hat{i}+0.5\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{14}=-0.67\hat{i}+0.67\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{25}=0.9\hat{i}+0.11\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result189.tex <==
{\tiny 2D-M189:}

$\hat{n}_{13}=0.65\hat{i}-0.65\hat{j}-0.38\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}+0.61\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.87\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.84\hat{j}+0.55\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result19.tex <==
{\tiny 2D-M19:}

$\hat{n}_{13}=-0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result190.tex <==
{\tiny 2D-M190:}

$\hat{n}_{13}=0.02\hat{i}-0.58\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{14}=-0.84\hat{i}-0.33\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{23}=-0.13\hat{i}-0.9\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{35}=-0.36\hat{i}+0.37\hat{j}-0.86\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=2.49\hat{i}+4.03\hat{j}+6.6\hat{k}$,\;\;\;$\vec{r}_{23}=2.43\hat{i}+3.38\hat{j}+6.05\hat{k}$,\;\;\;$\vec{r}_{24}=3.44\hat{i}+3.7\hat{j}+2.4\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result191.tex <==
{\tiny 2D-M191:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{23}=-0.88\hat{i}-0.3\hat{j}-0.36\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result192.tex <==
{\tiny 2D-M192:}

$\hat{n}_{13}=0.04\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.48\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.7\hat{i}+0.23\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.89\hat{i}+0.46\hat{j}+0.03\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result193.tex <==
{\tiny 2D-M193:}

$\hat{n}_{13}=-0.0\hat{i}+0.51\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.62\hat{i}-0.48\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result194.tex <==
{\tiny 2D-M194:}

$\hat{n}_{13}=-0.68\hat{i}-0.73\hat{j}+0.06\hat{k}$,\;\;\;$\hat{n}_{14}=-0.46\hat{i}-0.83\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{24}=0.49\hat{i}+0.05\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{25}=-0.33\hat{i}+0.62\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result195.tex <==
{\tiny 2D-M195:}

$\hat{n}_{13}=0.0\hat{i}+0.53\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{14}=-0.76\hat{i}+0.63\hat{j}-0.19\hat{k}$,\;\;\;$\hat{n}_{24}=-0.15\hat{i}-0.45\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{35}=0.64\hat{i}+0.46\hat{j}-0.61\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result196.tex <==
{\tiny 2D-M196:}

$\hat{n}_{13}=-0.38\hat{i}-0.4\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{14}=0.72\hat{i}+0.0\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.7\hat{i}-0.08\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{35}=0.56\hat{i}+0.54\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result197.tex <==
{\tiny 2D-M197:}

$\hat{n}_{13}=-0.17\hat{i}+0.74\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{14}=0.79\hat{i}-0.59\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{25}=0.31\hat{i}+0.6\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{35}=-0.53\hat{i}-0.57\hat{j}-0.63\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result198.tex <==
{\tiny 2D-M198:}

$\hat{n}_{13}=-0.78\hat{i}+0.61\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{14}=-0.68\hat{i}-0.51\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.02\hat{i}+0.69\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{25}=-0.9\hat{i}-0.27\hat{j}+0.33\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result199.tex <==
{\tiny 2D-M199:}

$\hat{n}_{13}=-1.0\hat{i}+0.02\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.46\hat{j}-0.89\hat{k}$,\;\;\;$\hat{n}_{45}=0.09\hat{i}+0.72\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result2.tex <==
{\tiny 2D-M2:}

$\hat{n}_{14}=-0.31\hat{i}+0.43\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}-0.01\hat{j}+0.72\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result20.tex <==
{\tiny 2D-M20:}

$\hat{n}_{13}=0.28\hat{i}-0.83\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+9.95\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result200.tex <==
{\tiny 2D-M200:}

$\hat{n}_{13}=0.66\hat{i}-0.03\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.51\hat{i}-0.45\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.72\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result201.tex <==
{\tiny 2D-M201:}

$\hat{n}_{13}=-0.45\hat{i}+0.37\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.06\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.44\hat{j}-0.9\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result202.tex <==
{\tiny 2D-M202:}

$\hat{n}_{13}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.65\hat{i}+0.11\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{23}=-0.5\hat{i}-0.81\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{45}=0.13\hat{i}-0.77\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result203.tex <==
{\tiny 2D-M203:}

$\hat{n}_{13}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.89\hat{i}-0.4\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.51\hat{i}-0.77\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{35}=0.83\hat{i}+0.55\hat{j}+0.11\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.28\hat{i}+4.6\hat{j}+5.29\hat{k}$,\;\;\;$\vec{r}_{24}=5.29\hat{i}+5.38\hat{j}+4.64\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result204.tex <==
{\tiny 2D-M204:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.68\hat{i}+0.43\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.78\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{25}=0.66\hat{i}-0.02\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+6.32\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result205.tex <==
{\tiny 2D-M205:}

$\hat{n}_{13}=-0.0\hat{i}+0.81\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{14}=-0.51\hat{i}-0.48\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.76\hat{i}-0.0\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{45}=0.72\hat{i}+0.22\hat{j}+0.66\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result206.tex <==
{\tiny 2D-M206:}

$\hat{n}_{13}=-0.0\hat{i}+0.41\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{14}=-0.14\hat{i}+0.59\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.81\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.6\hat{i}+0.18\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result207.tex <==
{\tiny 2D-M207:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.11\hat{i}-0.65\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=0.81\hat{i}+0.5\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{45}=-0.06\hat{i}+0.56\hat{j}+0.83\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result208.tex <==
{\tiny 2D-M208:}

$\hat{n}_{13}=0.36\hat{i}+0.64\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{14}=-0.01\hat{i}-0.52\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{24}=0.52\hat{i}+0.04\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{35}=0.81\hat{i}+0.05\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.3\hat{i}+4.88\hat{j}+5.01\hat{k}$,\;\;\;$\vec{r}_{24}=3.68\hat{i}+4.58\hat{j}+4.75\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result209.tex <==
{\tiny 2D-M209:}

$\hat{n}_{13}=-0.7\hat{i}-0.01\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}-0.82\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}-0.58\hat{j}+0.82\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result21.tex <==
{\tiny 2D-M21:}

$\hat{n}_{14}=0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{24}=-0.68\hat{i}+0.06\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result210.tex <==
{\tiny 2D-M210:}

$\hat{n}_{13}=-0.7\hat{i}-0.7\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{14}=0.46\hat{i}-0.36\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.35\hat{i}-0.4\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.57\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result211.tex <==
{\tiny 2D-M211:}

$\hat{n}_{13}=-0.0\hat{i}+0.59\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{14}=0.62\hat{i}+0.35\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.04\hat{i}+0.83\hat{j}-0.56\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+8.83\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result212.tex <==
{\tiny 2D-M212:}

$\hat{n}_{13}=0.47\hat{i}+0.0\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{14}=-0.94\hat{i}-0.04\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.22\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{25}=0.66\hat{i}+0.54\hat{j}-0.52\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result213.tex <==
{\tiny 2D-M213:}

$\hat{n}_{13}=-0.57\hat{i}-0.42\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.88\hat{i}+0.45\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{24}=-0.82\hat{i}+0.36\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{35}=-0.13\hat{i}+0.77\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.57\hat{i}+2.56\hat{j}+7.35\hat{k}$,\;\;\;$\vec{r}_{25}=2.49\hat{i}+4.52\hat{j}+2.78\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result214.tex <==
{\tiny 2D-M214:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.57\hat{i}+0.52\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.71\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{35}=-0.43\hat{i}-0.46\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result215.tex <==
{\tiny 2D-M215:}

$\hat{n}_{13}=0.46\hat{i}-0.33\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{14}=-0.64\hat{i}+0.67\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{25}=0.79\hat{i}-0.55\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{35}=-0.71\hat{i}+0.12\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=8.26\hat{i}+4.82\hat{j}+7.98\hat{k}$,\;\;\;$\vec{r}_{24}=7.31\hat{i}+1.36\hat{j}+7.25\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result216.tex <==
{\tiny 2D-M216:}

$\hat{n}_{13}=0.68\hat{i}-0.08\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.72\hat{i}-0.69\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}-0.52\hat{j}+0.24\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+5.72\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result217.tex <==
{\tiny 2D-M217:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.81\hat{i}-0.41\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{23}=0.43\hat{i}-0.64\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{45}=-0.01\hat{i}-0.7\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.2\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result218.tex <==
{\tiny 2D-M218:}

$\hat{n}_{13}=0.78\hat{i}+0.17\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{14}=0.02\hat{i}-0.83\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{23}=-0.64\hat{i}-0.64\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{45}=-0.87\hat{i}-0.24\hat{j}+0.44\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result219.tex <==
{\tiny 2D-M219:}

$\hat{n}_{13}=0.67\hat{i}+0.26\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{14}=-0.92\hat{i}-0.37\hat{j}+0.13\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}-0.91\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{35}=0.68\hat{i}+0.46\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=2.68\hat{i}+4.94\hat{j}+6.84\hat{k}$,\;\;\;$\vec{r}_{23}=8.18\hat{i}+7.07\hat{j}+1.99\hat{k}$,\;\;\;$\vec{r}_{24}=8.1\hat{i}+8.25\hat{j}+5.88\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result22.tex <==
{\tiny 2D-M22:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.62\hat{j}+0.79\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.03\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result220.tex <==
{\tiny 2D-M220:}

$\hat{n}_{13}=-0.52\hat{i}+0.15\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.63\hat{i}-0.54\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result221.tex <==
{\tiny 2D-M221:}

$\hat{n}_{13}=-0.0\hat{i}+0.43\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{14}=0.54\hat{i}+0.68\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.52\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result222.tex <==
{\tiny 2D-M222:}

$\hat{n}_{13}=-0.0\hat{i}+0.97\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.6\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=-0.52\hat{i}+0.75\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{45}=-0.82\hat{i}-0.0\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result223.tex <==
{\tiny 2D-M223:}

$\hat{n}_{13}=0.8\hat{i}+0.54\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{14}=-0.17\hat{i}+0.61\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.81\hat{i}-0.44\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result224.tex <==
{\tiny 2D-M224:}

$\hat{n}_{13}=-0.69\hat{i}-0.5\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{14}=-0.91\hat{i}-0.41\hat{j}+0.11\hat{k}$,\;\;\;$\hat{n}_{23}=0.87\hat{i}+0.46\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{35}=-0.03\hat{i}+0.87\hat{j}-0.5\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.02\hat{i}+5.79\hat{j}+6.14\hat{k}$,\;\;\;$\vec{r}_{24}=3.41\hat{i}+5.22\hat{j}+4.98\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result225.tex <==
{\tiny 2D-M225:}

$\hat{n}_{13}=-0.0\hat{i}+0.61\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.99\hat{i}-0.07\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}+0.52\hat{j}-0.25\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result226.tex <==
{\tiny 2D-M226:}

$\hat{n}_{13}=0.62\hat{i}+0.62\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{14}=0.79\hat{i}+0.24\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.59\hat{i}-0.52\hat{j}+0.62\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result227.tex <==
{\tiny 2D-M227:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.79\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.79\hat{i}-0.61\hat{j}+0.03\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result228.tex <==
{\tiny 2D-M228:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.8\hat{i}-0.25\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.05\hat{i}-0.93\hat{j}-0.36\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result229.tex <==
{\tiny 2D-M229:}

$\hat{n}_{13}=0.07\hat{i}+0.61\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.46\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=0.3\hat{i}+0.07\hat{j}+0.95\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result23.tex <==
{\tiny 2D-M23:}

$\hat{n}_{14}=0.0\hat{i}+0.79\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.73\hat{j}+0.69\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result230.tex <==
{\tiny 2D-M230:}

$\hat{n}_{13}=0.5\hat{i}+0.61\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{14}=-0.03\hat{i}-0.73\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.43\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{25}=0.21\hat{i}+0.04\hat{j}+0.98\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result231.tex <==
{\tiny 2D-M231:}

$\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.75\hat{i}-0.43\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.67\hat{i}+0.05\hat{j}+0.74\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result232.tex <==
{\tiny 2D-M232:}

$\hat{n}_{13}=-0.5\hat{i}-0.18\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{14}=-0.45\hat{i}+0.89\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{24}=-0.13\hat{i}+0.94\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{35}=0.05\hat{i}-0.83\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=7.26\hat{i}+2.37\hat{j}+4.72\hat{k}$,\;\;\;$\vec{r}_{23}=0.91\hat{i}+0.23\hat{j}+9.74\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result233.tex <==
{\tiny 2D-M233:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.44\hat{i}+0.36\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{24}=-0.53\hat{i}+0.64\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.44\hat{j}-0.9\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result234.tex <==
{\tiny 2D-M234:}

$\hat{n}_{13}=-0.75\hat{i}+0.66\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}-0.56\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{35}=-0.69\hat{i}+0.72\hat{j}-0.03\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result235.tex <==
{\tiny 2D-M235:}

$\hat{n}_{13}=0.31\hat{i}-0.6\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=0.63\hat{i}+0.55\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.19\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{35}=0.71\hat{i}-0.69\hat{j}-0.13\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result236.tex <==
{\tiny 2D-M236:}

$\hat{n}_{13}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}-0.63\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{25}=0.79\hat{i}+0.56\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{35}=-0.29\hat{i}+0.5\hat{j}-0.82\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result237.tex <==
{\tiny 2D-M237:}

$\hat{n}_{13}=-0.17\hat{i}+0.67\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.19\hat{i}-0.97\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}-0.33\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{35}=-0.71\hat{i}+0.1\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=2.89\hat{i}+3.46\hat{j}+8.02\hat{k}$,\;\;\;$\vec{r}_{25}=3.92\hat{i}+1.58\hat{j}+8.22\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result238.tex <==
{\tiny 2D-M238:}

$\hat{n}_{13}=0.53\hat{i}+0.67\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.83\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=-0.76\hat{i}-0.0\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.45\hat{j}-0.68\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result239.tex <==
{\tiny 2D-M239:}

$\hat{n}_{13}=-0.02\hat{i}+0.57\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=0.47\hat{i}-0.88\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.02\hat{i}-0.98\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{35}=0.68\hat{i}+0.54\hat{j}+0.5\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.13\hat{i}+6.46\hat{j}+3.38\hat{k}$,\;\;\;$\vec{r}_{24}=2.82\hat{i}+5.36\hat{j}+3.17\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result24.tex <==
{\tiny 2D-M24:}

$\hat{n}_{14}=0.21\hat{i}+0.81\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+3.96\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result240.tex <==
{\tiny 2D-M240:}

$\hat{n}_{13}=-0.69\hat{i}-0.54\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.22\hat{i}-0.69\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{45}=-0.78\hat{i}+0.2\hat{j}-0.6\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result241.tex <==
{\tiny 2D-M241:}

$\hat{n}_{13}=-0.03\hat{i}+0.84\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.47\hat{i}-0.59\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.66\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result242.tex <==
{\tiny 2D-M242:}

$\hat{n}_{13}=-0.72\hat{i}+0.05\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{23}=-0.71\hat{i}+0.01\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}-0.54\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{45}=0.27\hat{i}+0.43\hat{j}+0.86\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result243.tex <==
{\tiny 2D-M243:}

$\hat{n}_{13}=-0.45\hat{i}-0.23\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{23}=-0.13\hat{i}-0.92\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{24}=-0.94\hat{i}-0.18\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{35}=0.37\hat{i}+0.14\hat{j}+0.92\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.12\hat{i}+5.39\hat{j}+4.42\hat{k}$,\;\;\;$\vec{r}_{23}=5.78\hat{i}+4.24\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{24}=5.54\hat{i}+5.62\hat{j}+5.4\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result244.tex <==
{\tiny 2D-M244:}

$\hat{n}_{13}=0.22\hat{i}+0.43\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{23}=0.57\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.21\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.14\hat{i}+0.37\hat{j}+0.92\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result245.tex <==
{\tiny 2D-M245:}

$\hat{n}_{13}=0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.64\hat{i}+0.56\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{25}=-0.81\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}+0.49\hat{j}+0.52\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result246.tex <==
{\tiny 2D-M246:}

$\hat{n}_{13}=0.0\hat{i}+0.49\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{23}=0.55\hat{i}+0.63\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.69\hat{i}+0.04\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.91\hat{j}-0.42\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result247.tex <==
{\tiny 2D-M247:}

$\hat{n}_{13}=0.43\hat{i}-0.44\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result248.tex <==
{\tiny 2D-M248:}

$\hat{n}_{13}=0.05\hat{i}+0.84\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{23}=-0.23\hat{i}-0.91\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.96\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{35}=-0.63\hat{i}+0.73\hat{j}-0.26\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.95\hat{i}+3.34\hat{j}+4.38\hat{k}$,\;\;\;$\vec{r}_{24}=3.26\hat{i}+3.75\hat{j}+6.05\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result249.tex <==
{\tiny 2D-M249:}

$\hat{n}_{13}=0.0\hat{i}+0.77\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.5\hat{i}-0.5\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{25}=0.54\hat{i}+0.67\hat{j}-0.51\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result25.tex <==
{\tiny 2D-M25:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.26\hat{i}-0.46\hat{j}+0.85\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result250.tex <==
{\tiny 2D-M250:}

$\hat{n}_{13}=0.52\hat{i}-0.84\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{23}=-0.73\hat{i}+0.01\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{45}=-0.57\hat{i}-0.51\hat{j}-0.64\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result251.tex <==
{\tiny 2D-M251:}

$\hat{n}_{13}=-0.33\hat{i}+0.54\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}+0.73\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{25}=0.2\hat{i}+0.67\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{45}=-0.65\hat{i}-0.65\hat{j}-0.38\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result252.tex <==
{\tiny 2D-M252:}

$\hat{n}_{13}=-0.0\hat{i}+0.64\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.52\hat{i}-0.71\hat{j}-0.47\hat{k}$,\;\;\;$\hat{n}_{24}=-0.08\hat{i}-0.68\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result253.tex <==
{\tiny 2D-M253:}

$\hat{n}_{13}=0.63\hat{i}+0.02\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=0.91\hat{i}+0.23\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{24}=0.88\hat{i}+0.24\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{35}=-0.18\hat{i}-0.57\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=6.56\hat{i}+4.75\hat{j}+6.38\hat{k}$,\;\;\;$\vec{r}_{23}=6.53\hat{i}+2.55\hat{j}+7.74\hat{k}$,\;\;\;$\vec{r}_{24}=5.03\hat{i}+4.39\hat{j}+6.92\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result254.tex <==
{\tiny 2D-M254:}

$\hat{n}_{13}=-0.42\hat{i}-0.76\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{23}=0.37\hat{i}+0.8\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{24}=-0.68\hat{i}+0.68\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{25}=0.85\hat{i}+0.17\hat{j}+0.5\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result255.tex <==
{\tiny 2D-M255:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.76\hat{i}+0.63\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}+0.55\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.64\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result256.tex <==
{\tiny 2D-M256:}

$\hat{n}_{13}=0.01\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.88\hat{i}+0.31\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{24}=-0.8\hat{i}+0.07\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}-0.48\hat{j}-0.32\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.41\hat{i}+1.17\hat{j}+1.95\hat{k}$,\;\;\;$\vec{r}_{23}=6.6\hat{i}+8.7\hat{j}+2.72\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result257.tex <==
{\tiny 2D-M257:}

$\hat{n}_{13}=0.57\hat{i}+0.14\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.64\hat{i}-0.74\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}+0.74\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.61\hat{j}+0.79\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result258.tex <==
{\tiny 2D-M258:}

$\hat{n}_{13}=0.64\hat{i}+0.35\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{14}=0.66\hat{i}-0.05\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.57\hat{j}-0.1\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.76\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result259.tex <==
{\tiny 2D-M259:}

$\hat{n}_{13}=-0.1\hat{i}+0.76\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{14}=-0.93\hat{i}+0.38\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{24}=0.48\hat{i}-0.74\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{35}=0.68\hat{i}+0.44\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result26.tex <==
{\tiny 2D-M26:}

$\hat{n}_{14}=-0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result260.tex <==
{\tiny 2D-M260:}

$\hat{n}_{13}=-0.97\hat{i}+0.07\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{14}=-0.89\hat{i}+0.46\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=0.11\hat{i}+0.76\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{35}=-0.59\hat{i}-0.52\hat{j}+0.62\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result261.tex <==
{\tiny 2D-M261:}

$\hat{n}_{13}=0.0\hat{i}+0.49\hat{j}-0.87\hat{k}$,\;\;\;$\hat{n}_{14}=-0.03\hat{i}+0.4\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.6\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=-0.64\hat{i}+0.54\hat{j}+0.54\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result262.tex <==
{\tiny 2D-M262:}

$\hat{n}_{13}=0.84\hat{i}-0.32\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{14}=0.6\hat{i}-0.43\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{23}=0.79\hat{i}+0.56\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{45}=0.06\hat{i}-0.82\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result263.tex <==
{\tiny 2D-M263:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.73\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.65\hat{j}+0.76\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+8.19\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result264.tex <==
{\tiny 2D-M264:}

$\hat{n}_{13}=-0.33\hat{i}-0.07\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{14}=-0.99\hat{i}-0.15\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=-0.57\hat{i}-0.81\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{35}=0.35\hat{i}+0.65\hat{j}-0.67\hat{k}$,\newline
$\vec{r}_{14}=5.08\hat{i}+4.91\hat{j}+5.17\hat{k}$,\;\;\;$\vec{r}_{23}=4.91\hat{i}+5.3\hat{j}+4.76\hat{k}$,\;\;\;$\vec{r}_{24}=5.32\hat{i}+5.1\hat{j}+5.01\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result265.tex <==
{\tiny 2D-M265:}

$\hat{n}_{13}=0.31\hat{i}+0.52\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.24\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{23}=-0.65\hat{i}-0.39\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=0.26\hat{i}+0.41\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result266.tex <==
{\tiny 2D-M266:}

$\hat{n}_{13}=0.0\hat{i}+0.73\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{14}=0.53\hat{i}-0.66\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{25}=0.76\hat{i}+0.64\hat{j}-0.13\hat{k}$,\;\;\;$\hat{n}_{45}=0.78\hat{i}+0.63\hat{j}-0.01\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result267.tex <==
{\tiny 2D-M267:}

$\hat{n}_{13}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.53\hat{i}+0.6\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.24\hat{i}+0.42\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result268.tex <==
{\tiny 2D-M268:}

$\hat{n}_{13}=-0.03\hat{i}+0.34\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{14}=-0.09\hat{i}-0.97\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{24}=0.91\hat{i}-0.36\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{35}=0.11\hat{i}+0.51\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=4.96\hat{i}+5.0\hat{j}+5.04\hat{k}$,\;\;\;$\vec{r}_{23}=4.9\hat{i}+4.92\hat{j}+5.09\hat{k}$,\;\;\;$\vec{r}_{24}=6.07\hat{i}+5.07\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result269.tex <==
{\tiny 2D-M269:}

$\hat{n}_{13}=-0.58\hat{i}+0.17\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{14}=0.7\hat{i}+0.02\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.31\hat{i}+0.72\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+5.51\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result27.tex <==
{\tiny 2D-M27:}

$\hat{n}_{14}=-0.1\hat{i}-0.04\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{25}=-0.73\hat{i}-0.61\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{45}=-0.27\hat{i}-0.4\hat{j}-0.88\hat{k}$,\;\;\;$\vec{r}_{23}=5.31\hat{i}+4.46\hat{j}+4.41\hat{k}$,\newline
$\vec{r}_{34}=4.99\hat{i}+4.55\hat{j}+5.58\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result270.tex <==
{\tiny 2D-M270:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.02\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.48\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{35}=0.85\hat{i}-0.48\hat{j}+0.22\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result271.tex <==
{\tiny 2D-M271:}

$\hat{n}_{13}=0.0\hat{i}+0.94\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}+0.71\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=0.61\hat{i}+0.64\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{35}=-0.72\hat{i}+0.69\hat{j}+0.02\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result272.tex <==
{\tiny 2D-M272:}

$\hat{n}_{13}=0.27\hat{i}+0.68\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{24}=-0.88\hat{i}+0.48\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=0.12\hat{i}+0.76\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{35}=0.68\hat{i}+0.44\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result273.tex <==
{\tiny 2D-M273:}

$\hat{n}_{13}=0.79\hat{i}-0.46\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{23}=-0.93\hat{i}-0.37\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{25}=-0.59\hat{i}+0.55\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{45}=-0.59\hat{i}+0.2\hat{j}-0.78\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result274.tex <==
{\tiny 2D-M274:}

$\hat{n}_{13}=-0.0\hat{i}+0.95\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{23}=-0.06\hat{i}+0.26\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.31\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{45}=-0.64\hat{i}+0.43\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result275.tex <==
{\tiny 2D-M275:}

$\hat{n}_{13}=-0.77\hat{i}-0.46\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{23}=0.78\hat{i}-0.61\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{24}=-0.43\hat{i}-0.13\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{45}=-0.7\hat{i}+0.1\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result276.tex <==
{\tiny 2D-M276:}

$\hat{n}_{13}=0.28\hat{i}+0.29\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{23}=0.67\hat{i}+0.73\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{24}=-0.52\hat{i}-0.26\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{35}=-0.33\hat{i}-0.35\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=4.74\hat{i}+4.95\hat{j}+5.1\hat{k}$,\;\;\;$\vec{r}_{23}=6.26\hat{i}+5.85\hat{j}+6.44\hat{k}$,\;\;\;$\vec{r}_{24}=4.75\hat{i}+4.71\hat{j}+5.03\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result277.tex <==
{\tiny 2D-M277:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.5\hat{j}+0.86\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result278.tex <==
{\tiny 2D-M278:}

$\hat{n}_{13}=-0.0\hat{i}+0.6\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=0.52\hat{i}-0.72\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.47\hat{i}+0.63\hat{j}-0.63\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result279.tex <==
{\tiny 2D-M279:}

$\hat{n}_{13}=-0.97\hat{i}-0.25\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.64\hat{i}+0.57\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{45}=0.73\hat{i}-0.14\hat{j}+0.67\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result28.tex <==
{\tiny 2D-M28:}

$\hat{n}_{14}=-0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result280.tex <==
{\tiny 2D-M280:}

$\hat{n}_{13}=0.72\hat{i}+0.46\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.57\hat{i}-0.76\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{24}=-0.19\hat{i}-0.67\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{35}=0.65\hat{i}-0.72\hat{j}-0.23\hat{k}$,\newline
$\vec{r}_{14}=6.07\hat{i}+5.03\hat{j}+3.9\hat{k}$,\;\;\;$\vec{r}_{23}=6.94\hat{i}+7.02\hat{j}+2.92\hat{k}$,\;\;\;$\vec{r}_{24}=2.83\hat{i}+3.65\hat{j}+7.09\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result281.tex <==
{\tiny 2D-M281:}

$\hat{n}_{13}=-0.58\hat{i}-0.36\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.9\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{24}=-0.8\hat{i}+0.0\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+6.03\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result282.tex <==
{\tiny 2D-M282:}

$\hat{n}_{13}=0.82\hat{i}+0.52\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{24}=-0.69\hat{i}-0.22\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}+0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{35}=-0.57\hat{i}+0.65\hat{j}-0.51\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result283.tex <==
{\tiny 2D-M283:}

$\hat{n}_{13}=0.2\hat{i}+0.9\hat{j}-0.38\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.38\hat{j}-0.92\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.89\hat{j}+0.46\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result284.tex <==
{\tiny 2D-M284:}

$\hat{n}_{13}=-0.79\hat{i}-0.19\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.5\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.8\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{35}=-0.75\hat{i}-0.19\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result285.tex <==
{\tiny 2D-M285:}

$\hat{n}_{13}=0.0\hat{i}+0.82\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}-0.21\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.66\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{45}=0.97\hat{i}-0.24\hat{j}-0.07\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result286.tex <==
{\tiny 2D-M286:}

$\hat{n}_{13}=-0.43\hat{i}+0.84\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}-0.57\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.77\hat{i}+0.45\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result287.tex <==
{\tiny 2D-M287:}

$\hat{n}_{13}=-0.79\hat{i}+0.51\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{23}=0.08\hat{i}+0.56\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{24}=-0.65\hat{i}+0.37\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result288.tex <==
{\tiny 2D-M288:}

$\hat{n}_{13}=-0.53\hat{i}-0.53\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}-0.62\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.18\hat{i}+0.9\hat{j}-0.4\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.29\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result289.tex <==
{\tiny 2D-M289:}

$\hat{n}_{13}=0.0\hat{i}+0.27\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=-0.53\hat{i}+0.18\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.42\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result29.tex <==
{\tiny 2D-M29:}

$\hat{n}_{14}=0.52\hat{i}-0.5\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{34}=-0.13\hat{i}-0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{45}=-0.25\hat{i}+0.91\hat{j}-0.35\hat{k}$,\;\;\;$\vec{r}_{23}=3.3\hat{i}+3.38\hat{j}+6.5\hat{k}$,\newline
$\vec{r}_{25}=4.87\hat{i}+6.69\hat{j}+6.68\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result290.tex <==
{\tiny 2D-M290:}

$\hat{n}_{13}=0.22\hat{i}+0.8\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{23}=0.51\hat{i}+0.62\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{24}=-0.54\hat{i}+0.58\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.23\hat{i}-0.69\hat{j}-0.69\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result291.tex <==
{\tiny 2D-M291:}

$\hat{n}_{13}=0.36\hat{i}+0.81\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{23}=0.73\hat{i}+0.06\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.24\hat{i}-0.74\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result292.tex <==
{\tiny 2D-M292:}

$\hat{n}_{13}=-0.37\hat{i}-0.55\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{23}=-0.72\hat{i}+0.69\hat{j}-0.07\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}-0.6\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{25}=-0.81\hat{i}-0.57\hat{j}+0.15\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result293.tex <==
{\tiny 2D-M293:}

$\hat{n}_{13}=0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.67\hat{i}+0.05\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{45}=0.41\hat{i}-0.82\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result294.tex <==
{\tiny 2D-M294:}

$\hat{n}_{13}=-0.37\hat{i}+0.44\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.71\hat{i}-0.11\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result295.tex <==
{\tiny 2D-M295:}

$\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.25\hat{i}-0.67\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result296.tex <==
{\tiny 2D-M296:}

$\hat{n}_{13}=0.7\hat{i}-0.01\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.35\hat{i}+0.66\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{25}=-0.61\hat{i}+0.09\hat{j}-0.79\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result297.tex <==
{\tiny 2D-M297:}

$\hat{n}_{14}=-0.0\hat{i}+0.62\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.3\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.92\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}+0.23\hat{j}+0.67\hat{k}$,\newline
$\hat{n}_{35}=-0.73\hat{i}+0.34\hat{j}+0.59\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result298.tex <==
{\tiny 2D-M298:}

$\hat{n}_{14}=-0.47\hat{i}-0.21\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.09\hat{i}-0.59\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=0.78\hat{i}+0.14\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{34}=0.79\hat{i}+0.46\hat{j}-0.39\hat{k}$,\newline
$\hat{n}_{35}=-0.59\hat{i}+0.63\hat{j}-0.51\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result299.tex <==
{\tiny 2D-M299:}

$\hat{n}_{14}=0.57\hat{i}+0.67\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.56\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.23\hat{i}+0.94\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{34}=0.42\hat{i}-0.8\hat{j}-0.42\hat{k}$,\newline
$\hat{n}_{45}=-0.71\hat{i}-0.0\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=5.33\hat{i}+2.14\hat{j}+5.86\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result3.tex <==
{\tiny 2D-M3:}

$\hat{n}_{14}=-0.56\hat{i}+0.74\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.69\hat{i}-0.01\hat{j}+0.73\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result30.tex <==
{\tiny 2D-M30:}

$\hat{n}_{13}=0.81\hat{i}-0.38\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result300.tex <==
{\tiny 2D-M300:}

$\hat{n}_{14}=0.77\hat{i}+0.04\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.56\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.42\hat{i}+0.8\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{34}=-0.23\hat{i}-0.94\hat{j}-0.23\hat{k}$,\newline
$\hat{n}_{45}=0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=4.56\hat{i}+5.47\hat{j}+4.32\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result301.tex <==
{\tiny 2D-M301:}

$\hat{n}_{14}=0.13\hat{i}-0.65\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{23}=0.98\hat{i}-0.18\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.19\hat{i}-0.78\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.04\hat{i}-0.59\hat{j}+0.8\hat{k}$,\newline
$\hat{n}_{45}=0.55\hat{i}-0.24\hat{j}+0.8\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.39\hat{i}+4.79\hat{j}+5.38\hat{k}$,\;\;\;$\vec{r}_{25}=4.53\hat{i}+5.13\hat{j}+7.95\hat{k}$,\newline
$\vec{r}_{34}=5.37\hat{i}+4.62\hat{j}+5.27\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result302.tex <==
{\tiny 2D-M302:}

$\hat{n}_{14}=-0.6\hat{i}-0.79\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{15}=-0.59\hat{i}-0.79\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}-0.43\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.64\hat{i}-0.58\hat{j}+0.5\hat{k}$,\newline
$\hat{n}_{34}=0.45\hat{i}-0.17\hat{j}-0.88\hat{k}$,\;\;\;$\vec{r}_{14}=6.47\hat{i}+3.62\hat{j}+4.11\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result303.tex <==
{\tiny 2D-M303:}

$\hat{n}_{14}=-0.05\hat{i}-0.76\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{15}=-0.8\hat{i}-0.35\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}-0.91\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{25}=0.78\hat{i}+0.38\hat{j}+0.5\hat{k}$,\newline
$\hat{n}_{34}=-0.5\hat{i}-0.12\hat{j}+0.86\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=4.09\hat{i}+6.24\hat{j}+6.18\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result304.tex <==
{\tiny 2D-M304:}

$\hat{n}_{14}=-0.11\hat{i}+0.76\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{15}=0.11\hat{i}-0.76\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{23}=-0.89\hat{i}+0.22\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=0.49\hat{i}+0.6\hat{j}+0.63\hat{k}$,\newline
$\hat{n}_{34}=0.56\hat{i}-0.49\hat{j}-0.67\hat{k}$,\;\;\;$\vec{r}_{14}=4.93\hat{i}+5.16\hat{j}+4.85\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result305.tex <==
{\tiny 2D-M305:}

$\hat{n}_{14}=-0.9\hat{i}-0.42\hat{j}-0.11\hat{k}$,\;\;\;$\hat{n}_{15}=0.34\hat{i}-0.6\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=0.63\hat{i}+0.73\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{25}=-0.36\hat{i}+0.57\hat{j}+0.74\hat{k}$,\newline
$\hat{n}_{34}=-0.27\hat{i}+0.69\hat{j}-0.67\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=4.72\hat{i}+4.85\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result306.tex <==
{\tiny 2D-M306:}

$\hat{n}_{14}=-0.8\hat{i}-0.47\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{15}=0.05\hat{i}-0.66\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}-0.59\hat{j}-0.57\hat{k}$,\newline
$\hat{n}_{34}=0.95\hat{i}-0.24\hat{j}-0.22\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result307.tex <==
{\tiny 2D-M307:}

$\hat{n}_{14}=0.49\hat{i}+0.66\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{15}=-0.04\hat{i}-0.63\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.89\hat{i}-0.36\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}-0.66\hat{j}+0.51\hat{k}$,\newline
$\hat{n}_{34}=-0.0\hat{i}+0.63\hat{j}+0.77\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result308.tex <==
{\tiny 2D-M308:}

$\hat{n}_{13}=-0.7\hat{i}-0.05\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{14}=-0.56\hat{i}-0.56\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{24}=-0.29\hat{i}-0.9\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.61\hat{i}+0.49\hat{j}+0.63\hat{k}$,\newline
$\hat{n}_{35}=0.73\hat{i}+0.02\hat{j}+0.68\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result309.tex <==
{\tiny 2D-M309:}

$\hat{n}_{13}=0.02\hat{i}-0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.8\hat{i}+0.4\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{24}=-0.94\hat{i}+0.25\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}-0.61\hat{j}-0.56\hat{k}$,\newline
$\hat{n}_{35}=-0.05\hat{i}-0.69\hat{j}+0.72\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result31.tex <==
{\tiny 2D-M31:}

$\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.01\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result310.tex <==
{\tiny 2D-M310:}

$\hat{n}_{13}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.57\hat{i}-0.82\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.83\hat{i}+0.06\hat{j}-0.56\hat{k}$,\newline
$\hat{n}_{35}=-0.8\hat{i}+0.61\hat{j}-0.01\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+2.36\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+2.5\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result311.tex <==
{\tiny 2D-M311:}

$\hat{n}_{13}=0.71\hat{i}-0.09\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{14}=-0.48\hat{i}-0.86\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{24}=-0.91\hat{i}-0.42\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{25}=0.47\hat{i}-0.89\hat{j}-0.02\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.44\hat{i}+1.75\hat{j}+1.53\hat{k}$,\;\;\;$\vec{r}_{24}=3.06\hat{i}+6.64\hat{j}+4.6\hat{k}$,\newline
$\vec{r}_{25}=4.99\hat{i}+1.52\hat{j}+1.51\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+7.73\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result312.tex <==
{\tiny 2D-M312:}

$\hat{n}_{13}=-0.54\hat{i}+0.76\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{14}=0.44\hat{i}+0.54\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{23}=0.14\hat{i}+0.63\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{25}=-0.34\hat{i}-0.72\hat{j}+0.61\hat{k}$,\newline
$\hat{n}_{45}=-0.88\hat{i}+0.47\hat{j}+0.12\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result313.tex <==
{\tiny 2D-M313:}

$\hat{n}_{13}=-0.79\hat{i}+0.17\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{14}=-0.42\hat{i}+0.66\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{23}=-0.32\hat{i}+0.5\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=0.84\hat{i}-0.0\hat{j}-0.54\hat{k}$,\newline
$\hat{n}_{45}=0.73\hat{i}+0.68\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result314.tex <==
{\tiny 2D-M314:}

$\hat{n}_{13}=0.9\hat{i}-0.42\hat{j}+0.06\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.83\hat{i}-0.54\hat{j}+0.11\hat{k}$,\;\;\;$\hat{n}_{25}=0.51\hat{i}-0.85\hat{j}+0.09\hat{k}$,\newline
$\hat{n}_{45}=-0.0\hat{i}+0.34\hat{j}+0.94\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+2.38\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result315.tex <==
{\tiny 2D-M315:}

$\hat{n}_{13}=0.0\hat{i}+0.61\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{14}=-0.41\hat{i}-0.02\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}-0.67\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=-0.92\hat{i}-0.37\hat{j}-0.1\hat{k}$,\newline
$\hat{n}_{35}=0.0\hat{i}+0.83\hat{j}-0.56\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.86\hat{i}+5.62\hat{j}+6.15\hat{k}$,\;\;\;$\vec{r}_{23}=5.03\hat{i}+4.98\hat{j}+5.21\hat{k}$,\newline
$\vec{r}_{24}=5.31\hat{i}+5.28\hat{j}+4.75\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result316.tex <==
{\tiny 2D-M316:}

$\hat{n}_{13}=-0.83\hat{i}-0.08\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{14}=-0.31\hat{i}+0.77\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{23}=0.93\hat{i}+0.36\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{24}=0.28\hat{i}-0.5\hat{j}+0.82\hat{k}$,\newline
$\hat{n}_{25}=-0.51\hat{i}+0.74\hat{j}-0.43\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result317.tex <==
{\tiny 2D-M317:}

$\hat{n}_{13}=-0.6\hat{i}+0.68\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{14}=0.18\hat{i}+0.62\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=0.41\hat{i}+0.5\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{25}=0.91\hat{i}-0.38\hat{j}+0.17\hat{k}$,\newline
$\hat{n}_{35}=-0.74\hat{i}-0.37\hat{j}-0.56\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result318.tex <==
{\tiny 2D-M318:}

$\hat{n}_{13}=0.84\hat{i}-0.16\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{14}=0.55\hat{i}+0.26\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.94\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.93\hat{j}-0.36\hat{k}$,\newline
$\hat{n}_{35}=0.78\hat{i}+0.04\hat{j}-0.62\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result319.tex <==
{\tiny 2D-M319:}

$\hat{n}_{13}=0.85\hat{i}+0.13\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{14}=0.51\hat{i}-0.51\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=0.13\hat{i}+0.87\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{25}=-0.3\hat{i}-0.53\hat{j}-0.79\hat{k}$,\newline
$\hat{n}_{35}=-0.88\hat{i}-0.4\hat{j}+0.26\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result32.tex <==
{\tiny 2D-M32:}

$\hat{n}_{13}=0.09\hat{i}-0.77\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{14}=0.21\hat{i}-0.82\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{45}=-0.82\hat{i}-0.45\hat{j}-0.36\hat{k}$,\;\;\;$\vec{r}_{13}=6.51\hat{i}+3.35\hat{j}+4.18\hat{k}$,\newline
$\vec{r}_{23}=4.5\hat{i}+6.92\hat{j}+6.91\hat{k}$,\;\;\;$\vec{r}_{24}=4.66\hat{i}+4.14\hat{j}+6.71\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result320.tex <==
{\tiny 2D-M320:}

$\hat{n}_{14}=-0.2\hat{i}+0.68\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.35\hat{i}+0.47\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.16\hat{i}+0.61\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result321.tex <==
{\tiny 2D-M321:}

$\hat{n}_{14}=0.63\hat{i}+0.7\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=0.78\hat{i}+0.6\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.37\hat{i}+0.45\hat{j}-0.82\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result322.tex <==
{\tiny 2D-M322:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.22\hat{i}+0.64\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{34}=0.52\hat{i}-0.51\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result323.tex <==
{\tiny 2D-M323:}

$\hat{n}_{14}=0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.72\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.78\hat{i}-0.61\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{35}=-0.37\hat{i}+0.74\hat{j}-0.56\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result324.tex <==
{\tiny 2D-M324:}

$\hat{n}_{14}=-0.17\hat{i}-0.47\hat{j}-0.87\hat{k}$,\;\;\;$\hat{n}_{24}=0.31\hat{i}+0.57\hat{j}+0.76\hat{k}$,\;\;\;$\hat{n}_{34}=0.95\hat{i}-0.17\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result325.tex <==
{\tiny 2D-M325:}

$\hat{n}_{14}=0.0\hat{i}+0.63\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{24}=-0.16\hat{i}-0.89\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.42\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result326.tex <==
{\tiny 2D-M326:}

$\hat{n}_{14}=-0.04\hat{i}+0.56\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result327.tex <==
{\tiny 2D-M327:}

$\hat{n}_{14}=-0.0\hat{i}+0.47\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{23}=0.29\hat{i}+0.47\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.61\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.66\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result328.tex <==
{\tiny 2D-M328:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}-0.33\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.73\hat{j}+0.68\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+4.15\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result329.tex <==
{\tiny 2D-M329:}

$\hat{n}_{14}=-0.45\hat{i}-0.89\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.55\hat{i}+0.8\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result33.tex <==
{\tiny 2D-M33:}

$\hat{n}_{13}=-0.7\hat{i}+0.01\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.54\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result330.tex <==
{\tiny 2D-M330:}

$\hat{n}_{14}=0.37\hat{i}-0.39\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.67\hat{i}+0.67\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{45}=-0.34\hat{i}+0.34\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result331.tex <==
{\tiny 2D-M331:}

$\hat{n}_{14}=0.9\hat{i}+0.25\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result332.tex <==
{\tiny 2D-M332:}

$\hat{n}_{14}=-0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{23}=-0.78\hat{i}-0.14\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.87\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.52\hat{j}-0.63\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result333.tex <==
{\tiny 2D-M333:}

$\hat{n}_{14}=-0.79\hat{i}+0.28\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{23}=-0.95\hat{i}+0.21\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result334.tex <==
{\tiny 2D-M334:}

$\hat{n}_{14}=0.36\hat{i}+0.32\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}+0.8\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result335.tex <==
{\tiny 2D-M335:}

$\hat{n}_{14}=-0.79\hat{i}+0.29\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}-0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result336.tex <==
{\tiny 2D-M336:}

$\hat{n}_{14}=-0.81\hat{i}+0.38\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.01\hat{i}+0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result337.tex <==
{\tiny 2D-M337:}

$\hat{n}_{14}=-0.68\hat{i}-0.53\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{25}=0.57\hat{i}+0.23\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result338.tex <==
{\tiny 2D-M338:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{15}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result339.tex <==
{\tiny 2D-M339:}

$\hat{n}_{14}=0.81\hat{i}-0.29\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.81\hat{i}+0.29\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result34.tex <==
{\tiny 2D-M34:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.04\hat{i}-0.73\hat{j}+0.68\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result340.tex <==
{\tiny 2D-M340:}

$\hat{n}_{14}=-0.0\hat{i}+0.48\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{15}=-0.74\hat{i}+0.67\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.63\hat{i}-0.78\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result341.tex <==
{\tiny 2D-M341:}

$\hat{n}_{14}=0.12\hat{i}+0.81\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{14}=5.93\hat{i}+3.77\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result342.tex <==
{\tiny 2D-M342:}

$\hat{n}_{14}=0.91\hat{i}+0.32\hat{j}-0.28\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}-0.43\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.66\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.61\hat{j}+0.54\hat{k}$,\newline
$\vec{r}_{14}=4.11\hat{i}+7.58\hat{j}+7.9\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result343.tex <==
{\tiny 2D-M343:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.85\hat{i}-0.47\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{25}=0.49\hat{i}+0.87\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=0.42\hat{i}+5.85\hat{j}+6.72\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result344.tex <==
{\tiny 2D-M344:}

$\hat{n}_{14}=-0.1\hat{i}+0.5\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.64\hat{i}-0.33\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.97\hat{j}-0.22\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.14\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result345.tex <==
{\tiny 2D-M345:}

$\hat{n}_{14}=0.0\hat{i}+0.03\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.25\hat{i}+0.47\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.64\hat{i}+0.13\hat{j}+0.76\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result346.tex <==
{\tiny 2D-M346:}

$\hat{n}_{14}=0.1\hat{i}-0.09\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.89\hat{i}+0.44\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+5.28\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result347.tex <==
{\tiny 2D-M347:}

$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.31\hat{i}+0.36\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{25}=0.81\hat{i}-0.47\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result348.tex <==
{\tiny 2D-M348:}

$\hat{n}_{14}=0.32\hat{i}-0.67\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}+0.42\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.02\hat{i}+0.7\hat{j}-0.72\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result349.tex <==
{\tiny 2D-M349:}

$\hat{n}_{14}=0.52\hat{i}+0.01\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}+0.06\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.25\hat{i}-0.67\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{35}=-0.03\hat{i}+0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result35.tex <==
{\tiny 2D-M35:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.08\hat{i}+0.62\hat{j}-0.78\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result350.tex <==
{\tiny 2D-M350:}

$\hat{n}_{14}=0.25\hat{i}+0.21\hat{j}+0.94\hat{k}$,\;\;\;$\hat{n}_{24}=0.59\hat{i}+0.57\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.37\hat{i}-0.31\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{34}=-0.78\hat{i}+0.6\hat{j}+0.19\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result351.tex <==
{\tiny 2D-M351:}

$\hat{n}_{14}=-0.12\hat{i}+0.83\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.6\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{35}=-0.04\hat{i}+0.66\hat{j}-0.75\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result352.tex <==
{\tiny 2D-M352:}

$\hat{n}_{14}=0.01\hat{i}+0.02\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.7\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{35}=0.4\hat{i}+0.41\hat{j}+0.82\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result353.tex <==
{\tiny 2D-M353:}

$\hat{n}_{14}=-0.45\hat{i}+0.89\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=-0.62\hat{i}+0.44\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{34}=0.27\hat{i}+0.77\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.71\hat{i}-0.14\hat{j}-0.69\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result354.tex <==
{\tiny 2D-M354:}

$\hat{n}_{14}=0.02\hat{i}+0.98\hat{j}+0.19\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{25}=-0.78\hat{i}+0.27\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}+0.49\hat{j}+0.65\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result355.tex <==
{\tiny 2D-M355:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+9.99\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result356.tex <==
{\tiny 2D-M356:}

$\hat{n}_{14}=0.68\hat{i}-0.52\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.37\hat{i}-0.92\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.6\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{34}=0.69\hat{i}+0.02\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result357.tex <==
{\tiny 2D-M357:}

$\hat{n}_{14}=-0.04\hat{i}+0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.62\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.89\hat{i}+0.1\hat{j}-0.44\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result358.tex <==
{\tiny 2D-M358:}

$\hat{n}_{14}=0.25\hat{i}+0.09\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.49\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{25}=-0.79\hat{i}-0.58\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{34}=0.57\hat{i}-0.56\hat{j}+0.6\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result359.tex <==
{\tiny 2D-M359:}

$\hat{n}_{14}=0.37\hat{i}-0.62\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}+0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.55\hat{i}+0.63\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=-0.45\hat{i}-0.77\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result36.tex <==
{\tiny 2D-M36:}

$\hat{n}_{14}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+1.0\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result360.tex <==
{\tiny 2D-M360:}

$\hat{n}_{14}=0.0\hat{i}+0.28\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}-0.55\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.78\hat{i}-0.6\hat{j}+0.18\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result361.tex <==
{\tiny 2D-M361:}

$\hat{n}_{14}=-0.65\hat{i}+0.76\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}+0.66\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{34}=0.88\hat{i}+0.27\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result362.tex <==
{\tiny 2D-M362:}

$\hat{n}_{14}=-0.01\hat{i}+0.17\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.74\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.93\hat{i}-0.37\hat{j}+0.05\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+9.3\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result363.tex <==
{\tiny 2D-M363:}

$\hat{n}_{14}=0.01\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.93\hat{i}-0.25\hat{j}-0.25\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result364.tex <==
{\tiny 2D-M364:}

$\hat{n}_{14}=-0.5\hat{i}-0.58\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+5.83\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result365.tex <==
{\tiny 2D-M365:}

$\hat{n}_{14}=0.26\hat{i}+0.45\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}-0.78\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.13\hat{i}-0.95\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{45}=-0.44\hat{i}-0.24\hat{j}+0.87\hat{k}$,\newline
$\vec{r}_{25}=6.53\hat{i}+5.84\hat{j}+4.67\hat{k}$,\;\;\;$\vec{r}_{34}=5.22\hat{i}+3.7\hat{j}+6.69\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result366.tex <==
{\tiny 2D-M366:}

$\hat{n}_{14}=-0.31\hat{i}+0.95\hat{j}-0.06\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.63\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.96\hat{j}+0.29\hat{k}$,\;\;\;$\hat{n}_{45}=-0.85\hat{i}-0.1\hat{j}+0.52\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result367.tex <==
{\tiny 2D-M367:}

$\hat{n}_{14}=-0.1\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.95\hat{i}+0.21\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{45}=-0.24\hat{i}-0.42\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result368.tex <==
{\tiny 2D-M368:}

$\hat{n}_{14}=-0.5\hat{i}+0.75\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}-0.19\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.59\hat{i}-0.68\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{34}=-0.59\hat{i}-0.56\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result369.tex <==
{\tiny 2D-M369:}

$\hat{n}_{14}=0.04\hat{i}+0.72\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{23}=-0.9\hat{i}-0.31\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.44\hat{i}+0.64\hat{j}-0.64\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result37.tex <==
{\tiny 2D-M37:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result370.tex <==
{\tiny 2D-M370:}

$\hat{n}_{14}=-0.25\hat{i}+0.84\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=-0.79\hat{i}-0.56\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.56\hat{j}-0.13\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result371.tex <==
{\tiny 2D-M371:}

$\hat{n}_{14}=-0.41\hat{i}+0.2\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.74\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=-0.02\hat{i}-0.11\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{23}=3.16\hat{i}+2.97\hat{j}+6.41\hat{k}$,\;\;\;$\vec{r}_{34}=3.07\hat{i}+6.34\hat{j}+6.83\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+4.66\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result372.tex <==
{\tiny 2D-M372:}

$\hat{n}_{14}=-0.72\hat{i}-0.7\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{23}=0.55\hat{i}-0.55\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{34}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.45\hat{i}-0.45\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result373.tex <==
{\tiny 2D-M373:}

$\hat{n}_{14}=0.62\hat{i}+0.59\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=-0.13\hat{i}-0.8\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.02\hat{i}-0.94\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{45}=0.51\hat{i}-0.74\hat{j}-0.43\hat{k}$,\newline
$\vec{r}_{23}=3.72\hat{i}+3.44\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{25}=6.54\hat{i}+6.37\hat{j}+3.86\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result374.tex <==
{\tiny 2D-M374:}

$\hat{n}_{14}=0.06\hat{i}+0.93\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{25}=-0.63\hat{i}+0.76\hat{j}+0.13\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.52\hat{i}+0.29\hat{j}+0.81\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result375.tex <==
{\tiny 2D-M375:}

$\hat{n}_{14}=-0.74\hat{i}-0.3\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.55\hat{i}-0.55\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{45}=-0.45\hat{i}-0.45\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result376.tex <==
{\tiny 2D-M376:}

$\hat{n}_{14}=0.08\hat{i}+0.11\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{25}=0.57\hat{i}-0.48\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.83\hat{j}+0.55\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.01\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result377.tex <==
{\tiny 2D-M377:}

$\hat{n}_{14}=0.14\hat{i}-0.01\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{25}=-1.0\hat{i}+0.03\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{34}=0.56\hat{i}-0.83\hat{j}-0.06\hat{k}$,\;\;\;$\hat{n}_{45}=0.14\hat{i}-0.52\hat{j}+0.84\hat{k}$,\newline
$\vec{r}_{23}=3.17\hat{i}+3.41\hat{j}+4.4\hat{k}$,\;\;\;$\vec{r}_{34}=7.03\hat{i}+7.38\hat{j}+5.37\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result378.tex <==
{\tiny 2D-M378:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.43\hat{i}+0.46\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{34}=-0.62\hat{i}+0.48\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{45}=-0.11\hat{i}-0.92\hat{j}-0.37\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result379.tex <==
{\tiny 2D-M379:}

$\hat{n}_{14}=-0.75\hat{i}-0.41\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{25}=0.13\hat{i}-0.82\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{34}=-0.29\hat{i}-0.73\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.65\hat{i}-0.72\hat{j}+0.23\hat{k}$,\newline
$\vec{r}_{23}=6.7\hat{i}+6.71\hat{j}+3.56\hat{k}$,\;\;\;$\vec{r}_{25}=3.87\hat{i}+6.71\hat{j}+6.83\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result38.tex <==
{\tiny 2D-M38:}

$\hat{n}_{14}=0.39\hat{i}-0.82\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result380.tex <==
{\tiny 2D-M380:}

$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{15}=-0.0\hat{i}+0.57\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=-0.39\hat{i}-0.43\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{25}=-0.64\hat{i}-0.7\hat{j}-0.31\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result381.tex <==
{\tiny 2D-M381:}

$\hat{n}_{14}=-0.61\hat{i}-0.61\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{15}=-0.18\hat{i}+0.76\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.14\hat{i}+0.55\hat{j}+0.82\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+9.59\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result382.tex <==
{\tiny 2D-M382:}

$\hat{n}_{14}=-0.41\hat{i}-0.41\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{15}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.56\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result383.tex <==
{\tiny 2D-M383:}

$\hat{n}_{14}=0.53\hat{i}-0.85\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{15}=-0.68\hat{i}+0.51\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.53\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result384.tex <==
{\tiny 2D-M384:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result385.tex <==
{\tiny 2D-M385:}

$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{15}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.41\hat{i}+0.41\hat{j}+0.82\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.26\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result386.tex <==
{\tiny 2D-M386:}

$\hat{n}_{14}=-0.62\hat{i}-0.77\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{23}=0.73\hat{i}+0.62\hat{j}-0.28\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.72\hat{i}+3.59\hat{j}+6.36\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result387.tex <==
{\tiny 2D-M387:}

$\hat{n}_{14}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.08\hat{i}+0.62\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.96\hat{i}+4.18\hat{j}+6.17\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result388.tex <==
{\tiny 2D-M388:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.12\hat{i}-0.81\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=3.34\hat{i}+2.57\hat{j}+6.67\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result389.tex <==
{\tiny 2D-M389:}

$\hat{n}_{14}=-0.82\hat{i}+0.43\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.61\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.67\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{34}=-0.82\hat{i}+0.43\hat{j}-0.38\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=3.03\hat{i}+6.87\hat{j}+5.52\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result39.tex <==
{\tiny 2D-M39:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result390.tex <==
{\tiny 2D-M390:}

$\hat{n}_{14}=-0.82\hat{i}-0.38\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=-0.69\hat{i}-0.48\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}+0.54\hat{j}-0.61\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=3.66\hat{i}+6.37\hat{j}+4.46\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result391.tex <==
{\tiny 2D-M391:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.94\hat{i}-0.28\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.88\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{34}=0.12\hat{i}-0.78\hat{j}-0.61\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=1.2\hat{i}+1.39\hat{j}+9.93\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result392.tex <==
{\tiny 2D-M392:}

$\hat{n}_{14}=-0.76\hat{i}-0.65\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{23}=-0.37\hat{i}+0.39\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.59\hat{i}-0.7\hat{j}+0.39\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.57\hat{i}+7.23\hat{j}+6.35\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result393.tex <==
{\tiny 2D-M393:}

$\hat{n}_{14}=0.76\hat{i}+0.65\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.37\hat{i}-0.39\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{34}=0.59\hat{i}-0.7\hat{j}+0.39\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=6.29\hat{i}+5.68\hat{j}+2.58\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result394.tex <==
{\tiny 2D-M394:}

$\hat{n}_{14}=-0.34\hat{i}+0.88\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{23}=-0.93\hat{i}-0.35\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.66\hat{i}+0.03\hat{j}-0.75\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=4.97\hat{i}+5.13\hat{j}+4.93\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result395.tex <==
{\tiny 2D-M395:}

$\hat{n}_{15}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.07\hat{i}+0.74\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{25}=-0.07\hat{i}+0.74\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result396.tex <==
{\tiny 2D-M396:}

$\hat{n}_{15}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.56\hat{i}+0.23\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}+0.23\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result397.tex <==
{\tiny 2D-M397:}

$\hat{n}_{15}=0.0\hat{i}+0.28\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.19\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{25}=-0.74\hat{i}+0.65\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{34}=-0.5\hat{i}+0.31\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result398.tex <==
{\tiny 2D-M398:}

$\hat{n}_{13}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}-0.69\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.79\hat{i}+0.59\hat{j}+0.18\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result399.tex <==
{\tiny 2D-M399:}

$\hat{n}_{13}=-0.72\hat{i}+0.59\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.85\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{24}=-0.55\hat{i}-0.51\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{35}=0.08\hat{i}-0.79\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result4.tex <==
{\tiny 2D-M4:}

$\hat{n}_{13}=-0.59\hat{i}+0.81\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.04\hat{i}-0.74\hat{j}-0.67\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result40.tex <==
{\tiny 2D-M40:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.22\hat{i}+0.97\hat{j}-0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result400.tex <==
{\tiny 2D-M400:}

$\hat{n}_{13}=0.42\hat{i}-0.4\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}+0.76\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.59\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result401.tex <==
2D-M401:

$\hat{n}_{13}=-0.73\hat{i}-0.62\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result402.tex <==
2D-M402:

$\hat{n}_{13}=0.0\hat{i}+0.48\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.72\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{35}=0.17\hat{i}-0.47\hat{j}+0.87\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result403.tex <==
2D-M403:

$\hat{n}_{13}=-0.0\hat{i}+0.82\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.72\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=0.95\hat{i}-0.25\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.73\hat{j}+0.68\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result404.tex <==
2D-M404:

$\hat{n}_{13}=-0.11\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{14}=0.56\hat{i}+0.64\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.54\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.81\hat{i}+0.39\hat{j}-0.44\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result405.tex <==
2D-M405:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.48\hat{i}+0.53\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.52\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.8\hat{j}+0.6\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+6.19\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result406.tex <==
2D-M406:

$\hat{n}_{13}=0.67\hat{i}-0.34\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{14}=-0.27\hat{i}-0.83\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{23}=-0.38\hat{i}+0.86\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result407.tex <==
2D-M407:

$\hat{n}_{13}=0.67\hat{i}+0.67\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{14}=0.8\hat{i}+0.6\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.91\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result408.tex <==
2D-M408:

$\hat{n}_{13}=0.69\hat{i}-0.21\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{14}=-0.59\hat{i}-0.71\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.47\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{45}=0.33\hat{i}+0.21\hat{j}+0.92\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result409.tex <==
2D-M409:

$\hat{n}_{13}=-0.8\hat{i}-0.57\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{14}=0.17\hat{i}-0.72\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.93\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{35}=-0.46\hat{i}+0.71\hat{j}+0.53\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.94\hat{i}+4.88\hat{j}+3.97\hat{k}$,\;\;\;$\vec{r}_{24}=2.96\hat{i}+7.08\hat{j}+6.42\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result41.tex <==
{\tiny 2D-M41:}

$\hat{n}_{14}=0.81\hat{i}-0.55\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.51\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{25}=-0.32\hat{i}+0.65\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{34}=0.36\hat{i}-0.31\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result410.tex <==
2D-M410:

$\hat{n}_{13}=-0.83\hat{i}-0.55\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{14}=0.53\hat{i}-0.48\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.17\hat{i}-0.62\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{25}=0.69\hat{i}-0.72\hat{j}-0.07\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result411.tex <==
2D-M411:

$\hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{14}=0.36\hat{i}+0.72\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.69\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{45}=0.93\hat{i}-0.26\hat{j}-0.24\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result412.tex <==
2D-M412:

$\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.77\hat{i}-0.48\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.81\hat{i}-0.31\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{45}=-0.11\hat{i}+0.76\hat{j}-0.65\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result413.tex <==
2D-M413:

$\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.7\hat{i}+0.7\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.16\hat{i}+0.16\hat{j}-0.97\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result414.tex <==
2D-M414:

$\hat{n}_{13}=-0.16\hat{i}+0.51\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{14}=-0.22\hat{i}-0.97\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{24}=-0.74\hat{i}-0.67\hat{j}-0.06\hat{k}$,\;\;\;$\hat{n}_{35}=-0.16\hat{i}+0.1\hat{j}+0.98\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.3\hat{i}+3.55\hat{j}+5.79\hat{k}$,\;\;\;$\vec{r}_{24}=7.0\hat{i}+7.51\hat{j}+6.9\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result415.tex <==
2D-M415:

$\hat{n}_{13}=-0.35\hat{i}-0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.7\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+5.94\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result416.tex <==
2D-M416:

$\hat{n}_{13}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result417.tex <==
2D-M417:

$\hat{n}_{13}=-0.79\hat{i}+0.28\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{14}=-0.93\hat{i}+0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{24}=0.36\hat{i}+0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result418.tex <==
2D-M418:

$\hat{n}_{13}=0.36\hat{i}+0.32\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{14}=-0.66\hat{i}+0.74\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result419.tex <==
2D-M419:

$\hat{n}_{13}=-0.0\hat{i}+0.8\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.41\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{25}=0.74\hat{i}+0.67\hat{j}+0.09\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+9.66\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result42.tex <==
{\tiny 2D-M42:}

$\hat{n}_{14}=0.0\hat{i}+0.95\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.68\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{35}=0.8\hat{i}+0.57\hat{j}-0.2\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+1.2\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result420.tex <==
2D-M420:

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.61\hat{i}-0.61\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{45}=-0.57\hat{i}-0.57\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+9.49\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result421.tex <==
2D-M421:

$\hat{n}_{13}=-0.41\hat{i}+0.41\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result422.tex <==
2D-M422:

$\hat{n}_{13}=-0.51\hat{i}+0.32\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.9\hat{i}-0.21\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{23}=-0.48\hat{i}-0.56\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{35}=-0.37\hat{i}+0.25\hat{j}+0.89\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.23\hat{i}+2.59\hat{j}+4.81\hat{k}$,\;\;\;$\vec{r}_{24}=6.61\hat{i}+8.27\hat{j}+8.93\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result423.tex <==
2D-M423:

$\hat{n}_{13}=-0.0\hat{i}+0.45\hat{j}+0.9\hat{k}$,\;\;\;$\hat{n}_{14}=0.68\hat{i}-0.71\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{23}=0.49\hat{i}+0.67\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{25}=-0.01\hat{i}+0.25\hat{j}+0.97\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result424.tex <==
2D-M424:

$\hat{n}_{13}=-0.81\hat{i}+0.29\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.93\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{25}=0.37\hat{i}+0.63\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+9.68\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result425.tex <==
2D-M425:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result426.tex <==
2D-M426:

$\hat{n}_{13}=-0.32\hat{i}-0.67\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{14}=-0.46\hat{i}-0.88\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{24}=0.28\hat{i}-0.96\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{35}=0.38\hat{i}+0.55\hat{j}-0.74\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.68\hat{i}+6.31\hat{j}+4.84\hat{k}$,\;\;\;$\vec{r}_{23}=3.98\hat{i}+3.51\hat{j}+1.89\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result427.tex <==
2D-M427:

$\hat{n}_{13}=-0.0\hat{i}+0.18\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.83\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}+0.45\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result428.tex <==
2D-M428:

$\hat{n}_{13}=-0.52\hat{i}-0.11\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{24}=0.04\hat{i}-0.63\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{25}=0.59\hat{i}-0.61\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.65\hat{j}-0.76\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result429.tex <==
2D-M429:

$\hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=-0.91\hat{i}+0.14\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{35}=-0.29\hat{i}-0.6\hat{j}+0.74\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result43.tex <==
{\tiny 2D-M43:}

$\hat{n}_{14}=0.68\hat{i}+0.56\hat{j}-0.47\hat{k}$,\;\;\;$\hat{n}_{24}=-0.42\hat{i}-0.62\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.14\hat{i}+0.82\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.84\hat{j}+0.54\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result430.tex <==
2D-M430:

$\hat{n}_{13}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.9\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.6\hat{i}-0.34\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result431.tex <==
2D-M431:

$\hat{n}_{13}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.6\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=0.04\hat{i}-0.66\hat{j}-0.75\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result432.tex <==
2D-M432:

$\hat{n}_{13}=0.68\hat{i}+0.55\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{23}=-0.78\hat{i}-0.54\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{25}=0.42\hat{i}-0.83\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{45}=-0.59\hat{i}-0.56\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result433.tex <==
2D-M433:

$\hat{n}_{13}=0.26\hat{i}-0.46\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.2\hat{i}-0.59\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result434.tex <==
2D-M434:

$\hat{n}_{13}=0.4\hat{i}+0.67\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{23}=-0.22\hat{i}-0.97\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}-0.76\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}+0.2\hat{j}+0.79\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.67\hat{i}+5.1\hat{j}+4.86\hat{k}$,\;\;\;$\vec{r}_{24}=5.46\hat{i}+4.73\hat{j}+5.25\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result435.tex <==
2D-M435:

$\hat{n}_{13}=0.81\hat{i}-0.22\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.49\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{24}=0.01\hat{i}-0.9\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result436.tex <==
2D-M436:

$\hat{n}_{13}=0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result437.tex <==
2D-M437:

$\hat{n}_{13}=0.63\hat{i}-0.02\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.88\hat{i}+0.35\hat{j}-0.31\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result438.tex <==
2D-M438:

$\hat{n}_{13}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.04\hat{i}-0.67\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{24}=0.13\hat{i}-0.38\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{35}=0.01\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+3.41\hat{k}$,\;\;\;$\vec{r}_{14}=4.67\hat{i}+5.79\hat{j}+5.32\hat{k}$,\;\;\;$\vec{r}_{23}=5.13\hat{i}+3.54\hat{j}+6.94\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result439.tex <==
2D-M439:

$\hat{n}_{13}=0.17\hat{i}+0.67\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{23}=0.72\hat{i}-0.66\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}-0.61\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.01\hat{i}+0.61\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result44.tex <==
{\tiny 2D-M44:}

$\hat{n}_{14}=0.7\hat{i}-0.1\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=0.74\hat{i}-0.18\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=-0.87\hat{i}-0.07\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{35}=-0.19\hat{i}-0.59\hat{j}+0.78\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result440.tex <==
2D-M440:

$\hat{n}_{13}=0.0\hat{i}+0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{14}=-0.21\hat{i}+0.03\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.11\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{25}=-0.49\hat{i}-0.87\hat{j}+0.08\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result441.tex <==
2D-M441:

$\hat{n}_{13}=-0.44\hat{i}-0.65\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{35}=0.06\hat{i}-0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result442.tex <==
2D-M442:

$\hat{n}_{13}=-0.5\hat{i}-0.62\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{14}=-0.78\hat{i}-0.62\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=-0.52\hat{i}+0.61\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.78\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result443.tex <==
2D-M443:

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.72\hat{i}-0.68\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.21\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{35}=0.46\hat{i}-0.61\hat{j}-0.65\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result444.tex <==
2D-M444:

$\hat{n}_{13}=0.0\hat{i}+0.97\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.37\hat{i}-0.66\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{35}=0.34\hat{i}+0.03\hat{j}-0.94\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result445.tex <==
2D-M445:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.5\hat{i}+0.51\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.12\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result446.tex <==
2D-M446:

$\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.44\hat{i}+0.64\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.9\hat{i}+0.31\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{45}=-0.81\hat{i}+0.36\hat{j}-0.46\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result447.tex <==
2D-M447:

$\hat{n}_{13}=-0.33\hat{i}-0.07\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{14}=-0.39\hat{i}-0.92\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{23}=-0.34\hat{i}-0.94\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.09\hat{i}-0.53\hat{j}+0.84\hat{k}$,\newline
$\vec{r}_{23}=6.79\hat{i}+4.98\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=4.49\hat{i}+5.46\hat{j}+4.46\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result448.tex <==
2D-M448:

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.54\hat{i}-0.58\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{23}=-0.77\hat{i}+0.64\hat{j}+0.07\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}-0.43\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result449.tex <==
2D-M449:

$\hat{n}_{13}=0.0\hat{i}+0.02\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.43\hat{i}+0.38\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+9.97\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result45.tex <==
{\tiny 2D-M45:}

$\hat{n}_{14}=-0.4\hat{i}-0.28\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{24}=0.63\hat{i}+0.63\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}-0.2\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{35}=0.12\hat{i}-0.64\hat{j}+0.76\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result450.tex <==
2D-M450:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.55\hat{i}+0.37\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.57\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.65\hat{i}+0.76\hat{j}+0.06\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result451.tex <==
2D-M451:

$\hat{n}_{13}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.52\hat{i}+0.66\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.81\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+9.14\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result452.tex <==
2D-M452:

$\hat{n}_{13}=-0.22\hat{i}-0.25\hat{j}+0.94\hat{k}$,\;\;\;$\hat{n}_{14}=-0.05\hat{i}-0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=-0.13\hat{i}-0.99\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.23\hat{j}-0.78\hat{k}$,\newline
$\vec{r}_{14}=6.43\hat{i}+5.67\hat{j}+3.93\hat{k}$,\;\;\;$\vec{r}_{25}=5.8\hat{i}+5.18\hat{j}+4.73\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result453.tex <==
2D-M453:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.57\hat{i}-0.36\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=0.11\hat{i}-0.7\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}+0.51\hat{j}+0.25\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result454.tex <==
2D-M454:

$\hat{n}_{13}=0.73\hat{i}+0.19\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{14}=-0.07\hat{i}-0.92\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{25}=-0.5\hat{i}-0.75\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{35}=-0.82\hat{i}-0.06\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=3.86\hat{i}+3.2\hat{j}+5.51\hat{k}$,\;\;\;$\vec{r}_{24}=3.91\hat{i}+5.01\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result455.tex <==
2D-M455:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.34\hat{i}+0.34\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{23}=0.46\hat{i}-0.4\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=-0.67\hat{i}+0.67\hat{j}-0.33\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result456.tex <==
2D-M456:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}-0.48\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}-0.55\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{45}=-0.56\hat{i}+0.55\hat{j}+0.62\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result457.tex <==
2D-M457:

$\hat{n}_{13}=0.0\hat{i}+0.81\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.27\hat{i}+0.2\hat{j}+0.94\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result458.tex <==
2D-M458:

$\hat{n}_{13}=-0.71\hat{i}-0.69\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{14}=0.06\hat{i}-0.96\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.95\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{35}=0.66\hat{i}-0.72\hat{j}+0.22\hat{k}$,\newline
$\vec{r}_{14}=3.78\hat{i}+4.2\hat{j}+4.49\hat{k}$,\;\;\;$\vec{r}_{23}=3.7\hat{i}+4.48\hat{j}+5.93\hat{k}$,\;\;\;$\vec{r}_{24}=5.24\hat{i}+4.23\hat{j}+5.86\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result459.tex <==
2D-M459:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.86\hat{i}+0.15\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.2\hat{i}+0.58\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.35\hat{i}+0.93\hat{j}+0.09\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result46.tex <==
{\tiny 2D-M46:}

$\hat{n}_{14}=-0.62\hat{i}-0.71\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.71\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{25}=0.55\hat{i}-0.12\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{35}=0.13\hat{i}-0.7\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result460.tex <==
2D-M460:

$\hat{n}_{13}=0.61\hat{i}-0.59\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.02\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.61\hat{i}+0.77\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{25}=-0.17\hat{i}-0.98\hat{j}+0.06\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result461.tex <==
2D-M461:

$\hat{n}_{13}=0.12\hat{i}+0.65\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=-0.21\hat{i}-0.59\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.65\hat{i}-0.52\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.8\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result462.tex <==
2D-M462:

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.79\hat{i}-0.28\hat{j}+0.55\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result463.tex <==
2D-M463:

$\hat{n}_{13}=-0.24\hat{i}+0.33\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{14}=-0.16\hat{i}-0.98\hat{j}-0.1\hat{k}$,\;\;\;$\hat{n}_{23}=-0.52\hat{i}-0.86\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{35}=-0.3\hat{i}+0.44\hat{j}+0.85\hat{k}$,\newline
$\vec{r}_{14}=5.64\hat{i}+4.51\hat{j}+4.3\hat{k}$,\;\;\;$\vec{r}_{24}=5.55\hat{i}+5.55\hat{j}+4.32\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result464.tex <==
2D-M464:

$\hat{n}_{13}=0.67\hat{i}+0.74\hat{j}-0.07\hat{k}$,\;\;\;$\hat{n}_{14}=0.12\hat{i}+0.76\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.36\hat{i}-0.32\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result465.tex <==
2D-M465:

$\hat{n}_{13}=-0.51\hat{i}-0.51\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{14}=-0.89\hat{i}+0.44\hat{j}-0.07\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.8\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.21\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result466.tex <==
2D-M466:

$\hat{n}_{13}=0.98\hat{i}-0.13\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{14}=-0.91\hat{i}+0.42\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{45}=0.91\hat{i}+0.16\hat{j}-0.38\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result467.tex <==
2D-M467:

$\hat{n}_{13}=-0.28\hat{i}-0.61\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.26\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.2\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.01\hat{i}+0.92\hat{j}-0.4\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result468.tex <==
2D-M468:

$\hat{n}_{13}=0.72\hat{i}+0.09\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{14}=-0.05\hat{i}-0.99\hat{j}+0.09\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.75\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{35}=0.14\hat{i}-0.99\hat{j}-0.01\hat{k}$,\newline
$\vec{r}_{14}=5.58\hat{i}+5.0\hat{j}+5.4\hat{k}$,\;\;\;$\vec{r}_{23}=4.72\hat{i}+4.21\hat{j}+4.43\hat{k}$,\;\;\;$\vec{r}_{24}=4.1\hat{i}+5.81\hat{j}+5.4\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result469.tex <==
2D-M469:

$\hat{n}_{13}=-0.42\hat{i}+0.43\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.25\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}+0.71\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{25}=-0.95\hat{i}-0.14\hat{j}-0.26\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result47.tex <==
{\tiny 2D-M47:}

$\hat{n}_{14}=0.82\hat{i}-0.53\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.85\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.38\hat{i}+0.92\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+9.45\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result470.tex <==
2D-M470:

$\hat{n}_{13}=-0.82\hat{i}-0.39\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}+0.39\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.9\hat{i}+0.27\hat{j}+0.34\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result471.tex <==
2D-M471:

$\hat{n}_{13}=-0.18\hat{i}-0.16\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{14}=-0.93\hat{i}-0.29\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{24}=-0.68\hat{i}-0.67\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{35}=0.28\hat{i}+0.39\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{14}=3.6\hat{i}+6.7\hat{j}+2.67\hat{k}$,\;\;\;$\vec{r}_{23}=3.29\hat{i}+3.72\hat{j}+2.54\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result472.tex <==
2D-M472:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.5\hat{i}+0.32\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.22\hat{i}-0.48\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result473.tex <==
2D-M473:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.07\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.55\hat{i}+0.53\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{35}=0.6\hat{i}+0.79\hat{j}+0.11\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result474.tex <==
2D-M474:

$\hat{n}_{13}=-0.19\hat{i}-0.52\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.63\hat{i}-0.55\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{35}=-0.77\hat{i}-0.45\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result475.tex <==
2D-M475:

$\hat{n}_{13}=0.48\hat{i}-0.68\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}+0.55\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}+0.77\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{35}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result476.tex <==
2D-M476:

$\hat{n}_{13}=0.25\hat{i}-0.31\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{24}=-0.36\hat{i}-0.58\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{25}=-0.53\hat{i}-0.81\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{35}=0.04\hat{i}-0.6\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=3.13\hat{i}+7.06\hat{j}+4.74\hat{k}$,\;\;\;$\vec{r}_{25}=3.36\hat{i}+3.16\hat{j}+7.01\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result477.tex <==
2D-M477:

$\hat{n}_{13}=-0.56\hat{i}-0.15\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=-0.55\hat{i}+0.63\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.45\hat{i}-0.77\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result478.tex <==
2D-M478:

$\hat{n}_{13}=0.02\hat{i}+0.13\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{24}=-0.36\hat{i}-0.76\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.27\hat{i}-0.96\hat{j}-0.11\hat{k}$,\;\;\;$\hat{n}_{35}=-0.18\hat{i}+0.5\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=4.23\hat{i}+5.03\hat{j}+5.58\hat{k}$,\;\;\;$\vec{r}_{24}=4.93\hat{i}+4.37\hat{j}+4.76\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result479.tex <==
2D-M479:

$\hat{n}_{13}=0.47\hat{i}+0.34\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.46\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{25}=0.47\hat{i}+0.68\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{45}=-0.68\hat{i}+0.72\hat{j}-0.16\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result48.tex <==
{\tiny 2D-M48:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.64\hat{i}+0.64\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.09\hat{i}-0.7\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{45}=-0.49\hat{i}+0.5\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result480.tex <==
2D-M480:

$\hat{n}_{13}=0.85\hat{i}-0.29\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{23}=0.83\hat{i}+0.44\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.22\hat{i}+0.56\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{45}=-0.56\hat{i}+0.56\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result481.tex <==
2D-M481:

$\hat{n}_{13}=0.77\hat{i}-0.28\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{23}=0.64\hat{i}-0.74\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.9\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+1.0\hat{j}+0.05\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result482.tex <==
2D-M482:

$\hat{n}_{13}=-0.8\hat{i}-0.4\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.67\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.46\hat{i}-0.89\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.68\hat{j}-0.45\hat{k}$,\newline
$\vec{r}_{14}=2.75\hat{i}+2.95\hat{j}+7.74\hat{k}$,\;\;\;$\vec{r}_{23}=7.76\hat{i}+7.17\hat{j}+2.98\hat{k}$,\;\;\;$\vec{r}_{24}=5.72\hat{i}+2.73\hat{j}+2.31\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result483.tex <==
2D-M483:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.0\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=0.97\hat{i}+0.22\hat{j}-0.07\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result484.tex <==
2D-M484:

$\hat{n}_{13}=0.66\hat{i}-0.71\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}-0.7\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.8\hat{j}-0.13\hat{k}$,\;\;\;$\hat{n}_{45}=-0.16\hat{i}-0.07\hat{j}-0.98\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result485.tex <==
2D-M485:

$\hat{n}_{13}=0.19\hat{i}+0.98\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.92\hat{i}-0.18\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{45}=-0.13\hat{i}+0.76\hat{j}-0.63\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result486.tex <==
2D-M486:

$\hat{n}_{13}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.43\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.57\hat{j}-0.82\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result487.tex <==
2D-M487:

$\hat{n}_{13}=0.02\hat{i}-0.35\hat{j}+0.94\hat{k}$,\;\;\;$\hat{n}_{23}=-0.7\hat{i}-0.67\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{24}=-0.84\hat{i}-0.53\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{35}=0.11\hat{i}+0.51\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=6.14\hat{i}+7.67\hat{j}+6.57\hat{k}$,\;\;\;$\vec{r}_{24}=7.74\hat{i}+4.9\hat{j}+3.93\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result488.tex <==
2D-M488:

$\hat{n}_{13}=-1.0\hat{i}-0.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.93\hat{i}-0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{25}=0.75\hat{i}-0.66\hat{j}+0.02\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result489.tex <==
2D-M489:

$\hat{n}_{13}=-0.59\hat{i}-0.3\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{23}=0.8\hat{i}-0.31\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.18\hat{i}-0.55\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{45}=0.56\hat{i}+0.59\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result49.tex <==
{\tiny 2D-M49:}

$\hat{n}_{14}=0.82\hat{i}+0.55\hat{j}-0.11\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{25}=0.67\hat{i}-0.3\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{34}=-0.71\hat{i}+0.0\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result490.tex <==
2D-M490:

$\hat{n}_{13}=-0.0\hat{i}+0.72\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{23}=0.78\hat{i}+0.43\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{25}=-0.63\hat{i}+0.55\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result491.tex <==
2D-M491:

$\hat{n}_{13}=-0.39\hat{i}+0.89\hat{j}+0.24\hat{k}$,\;\;\;$\hat{n}_{23}=-0.91\hat{i}-0.34\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.77\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result492.tex <==
2D-M492:

$\hat{n}_{13}=-0.73\hat{i}-0.64\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}-0.85\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}-0.76\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{35}=0.62\hat{i}-0.77\hat{j}+0.16\hat{k}$,\newline
$\vec{r}_{14}=4.11\hat{i}+5.6\hat{j}+4.22\hat{k}$,\;\;\;$\vec{r}_{23}=5.14\hat{i}+5.98\hat{j}+5.75\hat{k}$,\;\;\;$\vec{r}_{24}=5.63\hat{i}+5.96\hat{j}+4.02\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result493.tex <==
2D-M493:

$\hat{n}_{13}=0.7\hat{i}+0.36\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{23}=0.29\hat{i}-0.93\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{24}=0.7\hat{i}-0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result494.tex <==
2D-M494:

$\hat{n}_{13}=-0.82\hat{i}-0.38\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.54\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.56\hat{i}-0.74\hat{j}-0.37\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result495.tex <==
2D-M495:

$\hat{n}_{13}=0.64\hat{i}-0.04\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.39\hat{i}-0.8\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{24}=0.14\hat{i}-0.86\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{35}=0.33\hat{i}-0.72\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=4.04\hat{i}+3.89\hat{j}+4.19\hat{k}$,\;\;\;$\vec{r}_{23}=5.86\hat{i}+6.12\hat{j}+4.73\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result496.tex <==
2D-M496:

$\hat{n}_{13}=0.52\hat{i}-0.56\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.76\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}+0.49\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result497.tex <==
2D-M497:

$\hat{n}_{13}=-0.82\hat{i}-0.34\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.64\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.57\hat{i}+0.55\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result498.tex <==
2D-M498:

$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.57\hat{i}+0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}-0.56\hat{j}-0.59\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result499.tex <==
2D-M499:

$\hat{n}_{13}=-0.48\hat{i}-0.31\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=0.38\hat{i}+0.41\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{25}=0.54\hat{i}+0.63\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.63\hat{j}+0.78\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result5.tex <==
{\tiny 2D-M5:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.02\hat{i}-0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{45}=0.71\hat{i}-0.11\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result50.tex <==
{\tiny 2D-M50:}

$\hat{n}_{14}=-0.3\hat{i}+0.61\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.77\hat{i}+0.62\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.53\hat{i}-0.06\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{45}=-0.49\hat{i}-0.54\hat{j}+0.68\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result500.tex <==
2D-M500:

$\hat{n}_{13}=-0.75\hat{i}+0.66\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=0.5\hat{i}+0.0\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.45\hat{i}+0.67\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result501.tex <==
2D-M501:

$\hat{n}_{13}=0.59\hat{i}+0.19\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.68\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{24}=-0.59\hat{i}-0.56\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.14\hat{i}+0.98\hat{j}-0.14\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result502.tex <==
2D-M502:

$\hat{n}_{13}=0.78\hat{i}-0.6\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}+0.55\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.12\hat{i}+0.13\hat{j}-0.98\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result503.tex <==
2D-M503:

$\hat{n}_{13}=0.72\hat{i}-0.66\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{23}=0.17\hat{i}+0.67\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}-0.61\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{25}=0.22\hat{i}-0.58\hat{j}-0.78\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result504.tex <==
2D-M504:

$\hat{n}_{13}=-0.78\hat{i}-0.25\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{25}=-0.09\hat{i}-0.62\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{45}=-0.47\hat{i}+0.17\hat{j}-0.87\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result505.tex <==
2D-M505:

$\hat{n}_{13}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}-0.77\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.62\hat{i}-0.77\hat{j}+0.15\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result506.tex <==
2D-M506:

$\hat{n}_{13}=-0.0\hat{i}+0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+9.98\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result507.tex <==
2D-M507:

$\hat{n}_{13}=-0.37\hat{i}+0.44\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.73\hat{i}+0.69\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{35}=0.24\hat{i}+0.89\hat{j}+0.37\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result508.tex <==
2D-M508:

$\hat{n}_{13}=-0.79\hat{i}-0.58\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result509.tex <==
2D-M509:

$\hat{n}_{13}=0.94\hat{i}+0.17\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.73\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.69\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{45}=-0.2\hat{i}+0.68\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result51.tex <==
{\tiny 2D-M51:}

$\hat{n}_{14}=0.28\hat{i}-0.63\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.37\hat{i}-0.37\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result510.tex <==
2D-M510:

$\hat{n}_{13}=-0.82\hat{i}+0.19\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{23}=-0.85\hat{i}+0.44\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.53\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+3.67\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result511.tex <==
2D-M511:

$\hat{n}_{13}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.57\hat{i}+0.49\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.59\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{25}=-0.38\hat{i}-0.3\hat{j}+0.87\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result512.tex <==
2D-M512:

$\hat{n}_{14}=-0.65\hat{i}-0.65\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{24}=0.97\hat{i}+0.15\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{25}=-0.04\hat{i}-0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}-0.47\hat{j}+0.5\hat{k}$,\newline
$\hat{n}_{35}=0.68\hat{i}-0.54\hat{j}+0.49\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=5.09\hat{i}+4.91\hat{j}+4.99\hat{k}$,\;\;\;$\vec{r}_{34}=5.11\hat{i}+4.91\hat{j}+5.0\hat{k}$,\newline
$\vec{r}_{35}=5.08\hat{i}+5.03\hat{j}+4.93\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result513.tex <==
2D-M513:

$\hat{n}_{14}=0.66\hat{i}-0.72\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{24}=0.5\hat{i}+0.79\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{25}=-0.84\hat{i}+0.35\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{34}=0.67\hat{i}-0.1\hat{j}-0.73\hat{k}$,\newline
$\hat{n}_{35}=-0.55\hat{i}+0.6\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=4.85\hat{i}+4.97\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{34}=4.85\hat{i}+5.11\hat{j}+5.32\hat{k}$,\newline
$\vec{r}_{35}=4.88\hat{i}+5.11\hat{j}+4.95\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result514.tex <==
2D-M514:

$\hat{n}_{14}=-0.69\hat{i}-0.46\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.58\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.58\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=-0.71\hat{i}-0.58\hat{j}+0.41\hat{k}$,\newline
$\hat{n}_{45}=0.0\hat{i}+0.58\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=4.91\hat{i}+5.04\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{34}=4.92\hat{i}+5.13\hat{j}+5.13\hat{k}$,\newline
$\vec{r}_{45}=4.95\hat{i}+4.99\hat{j}+4.77\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result515.tex <==
2D-M515:

$\hat{n}_{14}=-0.79\hat{i}+0.28\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{23}=0.29\hat{i}-0.55\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{25}=0.91\hat{i}-0.11\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{34}=-0.31\hat{i}-0.83\hat{j}-0.47\hat{k}$,\newline
$\hat{n}_{45}=-0.91\hat{i}+0.11\hat{j}+0.41\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.19\hat{i}+4.83\hat{j}+5.04\hat{k}$,\;\;\;$\vec{r}_{34}=5.19\hat{i}+5.16\hat{j}+4.96\hat{k}$,\newline
$\vec{r}_{45}=5.19\hat{i}+5.18\hat{j}+5.07\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result516.tex <==
2D-M516:

$\hat{n}_{14}=-0.4\hat{i}-0.67\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{23}=-0.36\hat{i}+0.04\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}-0.14\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{34}=0.12\hat{i}-0.99\hat{j}-0.08\hat{k}$,\newline
$\hat{n}_{45}=0.12\hat{i}-0.99\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=2.78\hat{i}+7.13\hat{j}+5.98\hat{k}$,\;\;\;$\vec{r}_{25}=2.95\hat{i}+2.59\hat{j}+6.99\hat{k}$,\newline
$\vec{r}_{45}=6.19\hat{i}+6.76\hat{j}+5.93\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result517.tex <==
2D-M517:

$\hat{n}_{14}=0.66\hat{i}-0.72\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{23}=0.29\hat{i}-0.67\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{25}=0.45\hat{i}-0.53\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.84\hat{i}-0.52\hat{j}-0.15\hat{k}$,\newline
$\hat{n}_{45}=0.22\hat{i}-0.97\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.99\hat{i}+4.87\hat{j}+4.99\hat{k}$,\;\;\;$\vec{r}_{25}=4.99\hat{i}+4.93\hat{j}+5.12\hat{k}$,\newline
$\vec{r}_{34}=5.08\hat{i}+5.07\hat{j}+5.09\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result518.tex <==
2D-M518:

$\hat{n}_{14}=0.8\hat{i}-0.31\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{15}=-0.8\hat{i}+0.31\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=-0.8\hat{i}+0.31\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}-0.69\hat{j}+0.45\hat{k}$,\newline
$\hat{n}_{34}=0.22\hat{i}-0.65\hat{j}-0.72\hat{k}$,\;\;\;$\vec{r}_{14}=5.05\hat{i}+5.06\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=5.08\hat{i}+5.01\hat{j}+5.01\hat{k}$,\newline
$\vec{r}_{34}=4.95\hat{i}+5.09\hat{j}+4.94\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result519.tex <==
2D-M519:

$\hat{n}_{14}=0.77\hat{i}-0.64\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{15}=0.77\hat{i}-0.64\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{23}=-0.49\hat{i}-0.62\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.41\hat{i}-0.45\hat{j}-0.79\hat{k}$,\newline
$\hat{n}_{34}=0.77\hat{i}-0.64\hat{j}-0.03\hat{k}$,\;\;\;$\vec{r}_{14}=5.13\hat{i}+4.73\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.73\hat{i}+4.93\hat{j}+5.0\hat{k}$,\newline
$\vec{r}_{25}=5.18\hat{i}+5.26\hat{j}+5.24\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result52.tex <==
{\tiny 2D-M52:}

$\hat{n}_{14}=-0.72\hat{i}+0.08\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}-0.19\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.8\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}+0.17\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result520.tex <==
2D-M520:

$\hat{n}_{14}=0.74\hat{i}-0.53\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{24}=-0.8\hat{i}-0.6\hat{j}-0.05\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}+0.23\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{34}=-0.39\hat{i}+0.73\hat{j}-0.55\hat{k}$,\newline
$\hat{n}_{35}=-0.34\hat{i}+0.42\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result521.tex <==
2D-M521:

$\hat{n}_{14}=-0.28\hat{i}+0.06\hat{j}-0.96\hat{k}$,\;\;\;$\hat{n}_{23}=-0.71\hat{i}-0.71\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.76\hat{i}-0.51\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}-0.55\hat{j}-0.4\hat{k}$,\newline
$\hat{n}_{45}=0.48\hat{i}-0.37\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{23}=3.91\hat{i}+4.94\hat{j}+2.63\hat{k}$,\;\;\;$\vec{r}_{25}=3.26\hat{i}+3.3\hat{j}+4.41\hat{k}$,\;\;\;$\vec{r}_{34}=4.82\hat{i}+8.11\hat{j}+7.6\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result522.tex <==
2D-M522:

$\hat{n}_{14}=-0.66\hat{i}-0.28\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{15}=0.66\hat{i}+0.28\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.66\hat{i}-0.28\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}-0.07\hat{j}+0.7\hat{k}$,\newline
$\hat{n}_{34}=0.24\hat{i}-0.96\hat{j}+0.15\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.9\hat{i}+5.02\hat{j}+4.99\hat{k}$,\;\;\;$\vec{r}_{25}=4.98\hat{i}+4.98\hat{j}+4.98\hat{k}$,\newline
$\vec{r}_{34}=4.77\hat{i}+4.96\hat{j}+4.55\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result523.tex <==
2D-M523:

$\hat{n}_{14}=-0.64\hat{i}-0.31\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{15}=0.64\hat{i}+0.31\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.63\hat{i}+0.31\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.44\hat{i}+0.9\hat{j}+0.0\hat{k}$,\newline
$\hat{n}_{34}=0.64\hat{i}+0.31\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.8\hat{i}+4.95\hat{j}+5.4\hat{k}$,\;\;\;$\vec{r}_{25}=4.13\hat{i}+5.81\hat{j}+5.24\hat{k}$,\newline
$\vec{r}_{34}=5.88\hat{i}+5.51\hat{j}+5.09\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result524.tex <==
2D-M524:

$\hat{n}_{14}=0.97\hat{i}-0.26\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{15}=-0.26\hat{i}-0.93\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{23}=0.26\hat{i}+0.93\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{25}=-0.26\hat{i}-0.93\hat{j}+0.25\hat{k}$,\newline
$\hat{n}_{34}=-0.03\hat{i}-0.25\hat{j}-0.97\hat{k}$,\;\;\;$\vec{r}_{14}=4.83\hat{i}+5.06\hat{j}+4.87\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.76\hat{i}+5.11\hat{j}+4.74\hat{k}$,\newline
$\vec{r}_{34}=4.59\hat{i}+4.77\hat{j}+5.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result525.tex <==
2D-M525:

$\hat{n}_{14}=0.62\hat{i}+0.78\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{15}=-0.52\hat{i}+0.3\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{23}=0.52\hat{i}-0.3\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=-0.59\hat{i}+0.56\hat{j}-0.59\hat{k}$,\newline
$\hat{n}_{34}=0.52\hat{i}-0.3\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{14}=5.42\hat{i}+5.0\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.88\hat{i}+5.04\hat{j}+4.86\hat{k}$,\newline
$\vec{r}_{25}=5.12\hat{i}+5.09\hat{j}+4.89\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result526.tex <==
2D-M526:

$\hat{n}_{14}=-0.54\hat{i}-0.38\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{15}=-0.73\hat{i}+0.65\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.73\hat{i}+0.65\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{25}=-0.73\hat{i}+0.65\hat{j}-0.2\hat{k}$,\newline
$\hat{n}_{34}=0.42\hat{i}+0.66\hat{j}+0.63\hat{k}$,\;\;\;$\vec{r}_{14}=5.0\hat{i}+4.99\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=4.98\hat{i}+5.01\hat{j}+5.0\hat{k}$,\newline
$\vec{r}_{34}=5.0\hat{i}+5.0\hat{j}+5.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result527.tex <==
2D-M527:

$\hat{n}_{14}=-0.67\hat{i}+0.21\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{15}=-0.38\hat{i}-0.92\hat{j}+0.09\hat{k}$,\;\;\;$\hat{n}_{23}=-0.38\hat{i}-0.92\hat{j}+0.09\hat{k}$,\;\;\;$\hat{n}_{25}=0.64\hat{i}-0.34\hat{j}-0.69\hat{k}$,\newline
$\hat{n}_{34}=0.38\hat{i}+0.92\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{14}=5.47\hat{i}+4.86\hat{j}+5.19\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=4.97\hat{i}+4.57\hat{j}+5.17\hat{k}$,\newline
$\vec{r}_{34}=4.95\hat{i}+5.09\hat{j}+4.54\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result528.tex <==
2D-M528:

$\hat{n}_{14}=0.75\hat{i}-0.54\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{15}=0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.66\hat{i}-0.61\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}-0.58\hat{j}-0.81\hat{k}$,\newline
$\hat{n}_{34}=-0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\vec{r}_{14}=5.73\hat{i}+5.7\hat{j}+5.77\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.6\hat{i}+4.7\hat{j}+4.35\hat{k}$,\newline
$\vec{r}_{25}=5.72\hat{i}+4.61\hat{j}+5.19\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result529.tex <==
2D-M529:

$\hat{n}_{14}=0.34\hat{i}-0.16\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{15}=-0.82\hat{i}+0.44\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{23}=0.46\hat{i}+0.89\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}-0.44\hat{j}-0.37\hat{k}$,\newline
$\hat{n}_{34}=0.82\hat{i}-0.44\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{14}=5.06\hat{i}+5.11\hat{j}+5.03\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.14\hat{i}+5.03\hat{j}+5.14\hat{k}$,\newline
$\vec{r}_{34}=5.04\hat{i}+5.0\hat{j}+5.12\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result53.tex <==
{\tiny 2D-M53:}

$\hat{n}_{14}=0.25\hat{i}+0.41\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.21\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{25}=0.66\hat{i}-0.62\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{34}=-0.64\hat{i}+0.56\hat{j}+0.52\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result530.tex <==
2D-M530:

$\hat{n}_{13}=0.03\hat{i}-0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{14}=0.04\hat{i}+0.75\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{24}=0.06\hat{i}-0.67\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{25}=1.0\hat{i}+0.01\hat{j}-0.07\hat{k}$,\newline
$\hat{n}_{35}=-0.05\hat{i}-0.75\hat{j}-0.66\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=5.04\hat{i}+5.04\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{25}=4.93\hat{i}+5.1\hat{j}+5.09\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result531.tex <==
2D-M531:

$\hat{n}_{13}=-0.66\hat{i}-0.72\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{14}=-0.57\hat{i}+0.49\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.81\hat{j}+0.11\hat{k}$,\;\;\;$\hat{n}_{25}=0.59\hat{i}-0.32\hat{j}+0.74\hat{k}$,\newline
$\hat{n}_{35}=-0.56\hat{i}-0.82\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.79\hat{i}+5.0\hat{j}+5.1\hat{k}$,\;\;\;$\vec{r}_{25}=5.07\hat{i}+5.02\hat{j}+4.79\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result532.tex <==
2D-M532:

$\hat{n}_{13}=0.06\hat{i}-0.73\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{14}=-0.5\hat{i}-0.64\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{24}=0.87\hat{i}-0.36\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}-0.68\hat{j}+0.74\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}+0.67\hat{j}-0.74\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.48\hat{i}+4.46\hat{j}+4.21\hat{k}$,\;\;\;$\vec{r}_{24}=4.62\hat{i}+5.53\hat{j}+4.44\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result533.tex <==
2D-M533:

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.06\hat{i}-0.94\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.9\hat{i}-0.44\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{25}=-0.08\hat{i}-0.8\hat{j}-0.59\hat{k}$,\newline
$\hat{n}_{35}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=1.77\hat{i}+2.39\hat{j}+8.5\hat{k}$,\;\;\;$\vec{r}_{24}=6.02\hat{i}+6.41\hat{j}+1.13\hat{k}$,\newline
$\vec{r}_{25}=2.33\hat{i}+7.66\hat{j}+6.24\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result534.tex <==
2D-M534:

$\hat{n}_{13}=0.25\hat{i}-0.91\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{14}=0.4\hat{i}-0.29\hat{j}-0.87\hat{k}$,\;\;\;$\hat{n}_{23}=-0.61\hat{i}+0.45\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=0.55\hat{i}+0.83\hat{j}-0.06\hat{k}$,\newline
$\hat{n}_{45}=0.78\hat{i}-0.36\hat{j}+0.51\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result535.tex <==
2D-M535:

$\hat{n}_{13}=-0.0\hat{i}+0.7\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{14}=0.75\hat{i}-0.43\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{23}=-0.57\hat{i}-0.82\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{25}=-0.44\hat{i}+0.31\hat{j}-0.84\hat{k}$,\newline
$\hat{n}_{45}=0.44\hat{i}-0.27\hat{j}-0.86\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result536.tex <==
2D-M536:

$\hat{n}_{13}=0.71\hat{i}+0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.19\hat{i}-0.6\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{25}=-0.78\hat{i}+0.6\hat{j}-0.19\hat{k}$,\newline
$\hat{n}_{45}=0.48\hat{i}-0.81\hat{j}-0.33\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.21\hat{i}+5.43\hat{j}+4.46\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result537.tex <==
2D-M537:

$\hat{n}_{13}=-0.23\hat{i}-0.94\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}-0.8\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.56\hat{j}+0.58\hat{k}$,\newline
$\hat{n}_{45}=0.01\hat{i}-1.0\hat{j}+0.01\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.01\hat{i}+4.97\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result538.tex <==
2D-M538:

$\hat{n}_{13}=-0.0\hat{i}+0.42\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{14}=-0.55\hat{i}-0.67\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}-0.84\hat{j}-0.09\hat{k}$,\;\;\;$\hat{n}_{24}=-0.99\hat{i}-0.08\hat{j}-0.14\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=6.34\hat{i}+1.41\hat{j}+3.89\hat{k}$,\;\;\;$\vec{r}_{23}=4.42\hat{i}+4.13\hat{j}+2.91\hat{k}$,\newline
$\vec{r}_{24}=2.54\hat{i}+7.19\hat{j}+8.33\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result539.tex <==
2D-M539:

$\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}+0.58\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{24}=-0.23\hat{i}+0.23\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{25}=-0.42\hat{i}+0.42\hat{j}+0.8\hat{k}$,\newline
$\hat{n}_{35}=0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=5.15\hat{i}+5.24\hat{j}+4.97\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result54.tex <==
{\tiny 2D-M54:}

$\hat{n}_{14}=0.41\hat{i}+0.67\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{23}=0.66\hat{i}+0.6\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.71\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{45}=-0.69\hat{i}+0.72\hat{j}-0.04\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result540.tex <==
2D-M540:

$\hat{n}_{13}=0.76\hat{i}-0.46\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{14}=0.8\hat{i}-0.42\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{24}=0.56\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.94\hat{i}-0.23\hat{j}+0.23\hat{k}$,\newline
$\hat{n}_{35}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=5.21\hat{i}+5.03\hat{j}+5.18\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result541.tex <==
2D-M541:

$\hat{n}_{13}=-0.15\hat{i}-0.31\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{14}=0.12\hat{i}-0.88\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{24}=-0.25\hat{i}-0.83\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{25}=0.07\hat{i}-0.68\hat{j}+0.73\hat{k}$,\newline
$\hat{n}_{35}=0.67\hat{i}+0.13\hat{j}+0.73\hat{k}$,\;\;\;$\vec{r}_{14}=6.24\hat{i}+3.46\hat{j}+3.16\hat{k}$,\;\;\;$\vec{r}_{24}=3.45\hat{i}+3.71\hat{j}+3.74\hat{k}$,\;\;\;$\vec{r}_{25}=5.31\hat{i}+6.47\hat{j}+6.68\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result542.tex <==
2D-M542:

$\hat{n}_{13}=0.64\hat{i}-0.4\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.45\hat{i}-0.21\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{23}=0.18\hat{i}-0.93\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=0.49\hat{i}+0.87\hat{j}+0.05\hat{k}$,\newline
$\hat{n}_{45}=0.72\hat{i}-0.46\hat{j}-0.51\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result543.tex <==
2D-M543:

$\hat{n}_{13}=0.57\hat{i}+0.4\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}+0.47\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{23}=0.27\hat{i}+0.74\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{25}=0.16\hat{i}-0.63\hat{j}-0.76\hat{k}$,\newline
$\hat{n}_{45}=-0.54\hat{i}-0.45\hat{j}+0.72\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result544.tex <==
2D-M544:

$\hat{n}_{13}=-0.65\hat{i}-0.74\hat{j}-0.19\hat{k}$,\;\;\;$\hat{n}_{14}=-0.66\hat{i}-0.72\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.76\hat{i}+0.63\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.25\hat{j}-0.97\hat{k}$,\newline
$\hat{n}_{45}=-0.56\hat{i}-0.82\hat{j}-0.1\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.73\hat{i}+2.72\hat{j}+3.96\hat{k}$,\;\;\;$\vec{r}_{25}=3.27\hat{i}+2.79\hat{j}+2.7\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result545.tex <==
2D-M545:

$\hat{n}_{13}=-0.16\hat{i}-0.91\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{14}=-0.16\hat{i}-0.91\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{23}=0.31\hat{i}-0.41\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.94\hat{i}-0.03\hat{j}-0.35\hat{k}$,\newline
$\hat{n}_{45}=0.16\hat{i}-0.66\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{14}=4.95\hat{i}+4.99\hat{j}+5.02\hat{k}$,\;\;\;$\vec{r}_{23}=5.0\hat{i}+5.13\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{24}=5.07\hat{i}+4.88\hat{j}+4.86\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result546.tex <==
2D-M546:

$\hat{n}_{13}=0.19\hat{i}-0.98\hat{j}-0.05\hat{k}$,\;\;\;$\hat{n}_{14}=0.88\hat{i}-0.45\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{23}=-0.4\hat{i}-0.62\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{24}=-0.23\hat{i}-0.64\hat{j}+0.73\hat{k}$,\newline
$\hat{n}_{35}=0.41\hat{i}-0.89\hat{j}+0.21\hat{k}$,\;\;\;$\vec{r}_{14}=4.91\hat{i}+4.92\hat{j}+5.06\hat{k}$,\;\;\;$\vec{r}_{23}=4.99\hat{i}+4.92\hat{j}+4.96\hat{k}$,\;\;\;$\vec{r}_{24}=5.07\hat{i}+5.07\hat{j}+5.17\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result547.tex <==
2D-M547:

$\hat{n}_{13}=-0.01\hat{i}-0.01\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.2\hat{i}-0.98\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.98\hat{i}-0.2\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{24}=-0.01\hat{i}-0.01\hat{j}-1.0\hat{k}$,\newline
$\hat{n}_{25}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{14}=6.43\hat{i}+7.63\hat{j}+2.17\hat{k}$,\;\;\;$\vec{r}_{23}=2.2\hat{i}+5.86\hat{j}+6.27\hat{k}$,\;\;\;$\vec{r}_{24}=2.38\hat{i}+6.94\hat{j}+2.16\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+7.76\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result548.tex <==
2D-M548:

$\hat{n}_{13}=-0.4\hat{i}+0.52\hat{j}+0.76\hat{k}$,\;\;\;$\hat{n}_{14}=-0.9\hat{i}-0.34\hat{j}-0.28\hat{k}$,\;\;\;$\hat{n}_{24}=0.88\hat{i}-0.47\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=0.43\hat{i}-0.75\hat{j}-0.5\hat{k}$,\newline
$\hat{n}_{35}=0.0\hat{i}+0.81\hat{j}-0.59\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result549.tex <==
2D-M549:

$\hat{n}_{13}=0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.23\hat{i}-0.23\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{25}=0.42\hat{i}-0.42\hat{j}+0.8\hat{k}$,\newline
$\hat{n}_{35}=0.7\hat{i}-0.7\hat{j}+0.12\hat{k}$,\;\;\;$\vec{r}_{13}=2.94\hat{i}+5.77\hat{j}+5.56\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result55.tex <==
{\tiny 2D-M55:}

$\hat{n}_{14}=0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.46\hat{i}+0.48\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{34}=0.9\hat{i}-0.44\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.7\hat{i}+0.11\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result550.tex <==
2D-M550:

$\hat{n}_{13}=-0.19\hat{i}+0.86\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{14}=0.67\hat{i}-0.25\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}-0.65\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.26\hat{j}-0.96\hat{k}$,\newline
$\hat{n}_{35}=-0.78\hat{i}-0.45\hat{j}-0.44\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result551.tex <==
2D-M551:

$\hat{n}_{13}=-0.08\hat{i}-0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.61\hat{i}-0.53\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{24}=0.07\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=0.79\hat{i}-0.47\hat{j}-0.39\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}+0.77\hat{j}-0.64\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.99\hat{i}+4.98\hat{j}+4.98\hat{k}$,\;\;\;$\vec{r}_{25}=5.01\hat{i}+4.99\hat{j}+5.01\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result552.tex <==
2D-M552:

$\hat{n}_{13}=-0.71\hat{i}+0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.56\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}-0.8\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{25}=0.23\hat{i}+0.94\hat{j}+0.23\hat{k}$,\newline
$\hat{n}_{35}=-0.05\hat{i}-1.0\hat{j}-0.05\hat{k}$,\;\;\;$\vec{r}_{13}=4.97\hat{i}+4.99\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result553.tex <==
2D-M553:

$\hat{n}_{13}=0.27\hat{i}+0.95\hat{j}-0.13\hat{k}$,\;\;\;$\hat{n}_{14}=0.72\hat{i}-0.1\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=0.66\hat{i}-0.23\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{25}=0.23\hat{i}+0.97\hat{j}-0.09\hat{k}$,\newline
$\hat{n}_{35}=-0.16\hat{i}+0.94\hat{j}+0.29\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.05\hat{i}+4.92\hat{j}+4.92\hat{k}$,\;\;\;$\vec{r}_{24}=5.05\hat{i}+5.0\hat{j}+4.99\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result554.tex <==
2D-M554:

$\hat{n}_{13}=-0.64\hat{i}-0.14\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=0.57\hat{i}-0.74\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{23}=0.57\hat{i}-0.74\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}+0.66\hat{j}+0.56\hat{k}$,\newline
$\hat{n}_{45}=0.03\hat{i}-1.0\hat{j}-0.06\hat{k}$,\;\;\;$\vec{r}_{13}=4.92\hat{i}+5.04\hat{j}+4.91\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.98\hat{i}+4.91\hat{j}+4.97\hat{k}$,\newline
$\vec{r}_{24}=4.94\hat{i}+5.08\hat{j}+4.94\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result555.tex <==
2D-M555:

$\hat{n}_{13}=0.16\hat{i}-0.75\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{14}=0.44\hat{i}-0.53\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.16\hat{i}-0.75\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{24}=-0.89\hat{i}-0.39\hat{j}-0.24\hat{k}$,\newline
$\hat{n}_{35}=0.6\hat{i}-0.8\hat{j}+0.07\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.03\hat{i}+4.83\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.81\hat{i}+4.8\hat{j}+5.08\hat{k}$,\newline
$\vec{r}_{24}=4.89\hat{i}+4.91\hat{j}+5.2\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result556.tex <==
2D-M556:

$\hat{n}_{13}=0.27\hat{i}-0.66\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{14}=-0.64\hat{i}+0.41\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{23}=-0.78\hat{i}-0.36\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.57\hat{j}-0.41\hat{k}$,\newline
$\hat{n}_{25}=-0.73\hat{i}-0.66\hat{j}+0.18\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result557.tex <==
2D-M557:

$\hat{n}_{13}=0.74\hat{i}+0.35\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}+0.67\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{23}=0.62\hat{i}-0.67\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{24}=-0.24\hat{i}-0.65\hat{j}+0.72\hat{k}$,\newline
$\hat{n}_{45}=0.88\hat{i}+0.18\hat{j}+0.44\hat{k}$,\;\;\;$\vec{r}_{13}=4.95\hat{i}+4.94\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.95\hat{i}+4.95\hat{j}+4.95\hat{k}$,\;\;\;$\vec{r}_{24}=5.06\hat{i}+5.05\hat{j}+5.06\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result558.tex <==
2D-M558:

$\hat{n}_{13}=-0.01\hat{i}-0.88\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.38\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.01\hat{i}-0.88\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.28\hat{j}-0.5\hat{k}$,\newline
$\hat{n}_{35}=0.8\hat{i}-0.59\hat{j}+0.14\hat{k}$,\;\;\;$\vec{r}_{13}=5.0\hat{i}+5.04\hat{j}+4.87\hat{k}$,\;\;\;$\vec{r}_{14}=5.14\hat{i}+4.88\hat{j}+4.93\hat{k}$,\;\;\;$\vec{r}_{24}=5.06\hat{i}+5.14\hat{j}+4.94\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result559.tex <==
2D-M559:

$\hat{n}_{13}=-0.52\hat{i}+0.68\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{14}=0.69\hat{i}+0.69\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{23}=-0.39\hat{i}-0.72\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}-0.24\hat{j}+0.83\hat{k}$,\newline
$\hat{n}_{25}=-0.8\hat{i}+0.34\hat{j}-0.49\hat{k}$,\;\;\;$\vec{r}_{13}=5.36\hat{i}+4.71\hat{j}+5.12\hat{k}$,\;\;\;$\vec{r}_{14}=5.38\hat{i}+5.66\hat{j}+5.16\hat{k}$,\;\;\;$\vec{r}_{24}=5.07\hat{i}+4.73\hat{j}+5.36\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result56.tex <==
{\tiny 2D-M56:}

$\hat{n}_{14}=0.82\hat{i}-0.52\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.93\hat{i}-0.25\hat{j}+0.25\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+9.98\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result560.tex <==
2D-M560:

$\hat{n}_{14}=-0.13\hat{i}+0.58\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.6\hat{i}+0.6\hat{j}+0.53\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result561.tex <==
2D-M561:

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.69\hat{i}+0.56\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.82\hat{j}-0.57\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result562.tex <==
2D-M562:

$\hat{n}_{14}=-0.08\hat{i}-0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.48\hat{i}+0.68\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{34}=0.6\hat{i}-0.55\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result563.tex <==
2D-M563:

$\hat{n}_{14}=-0.03\hat{i}+0.77\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{24}=-0.37\hat{i}+0.56\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}-0.17\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result564.tex <==
2D-M564:

$\hat{n}_{14}=-0.26\hat{i}+0.79\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}-0.56\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result565.tex <==
2D-M565:

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.67\hat{i}+0.74\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.72\hat{i}-0.7\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+1.02\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+9.32\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result566.tex <==
2D-M566:

$\hat{n}_{14}=-0.0\hat{i}-0.91\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.59\hat{i}+0.7\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{34}=-0.76\hat{i}-0.65\hat{j}+0.02\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result567.tex <==
2D-M567:

$\hat{n}_{14}=0.27\hat{i}+0.67\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{23}=-0.01\hat{i}-0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.01\hat{i}+0.71\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result568.tex <==
2D-M568:

$\hat{n}_{14}=-0.64\hat{i}+0.57\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result569.tex <==
2D-M569:

$\hat{n}_{14}=-0.01\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.21\hat{i}+0.79\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result57.tex <==
{\tiny 2D-M57:}

$\hat{n}_{14}=-0.7\hat{i}+0.09\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.6\hat{i}+0.6\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}+0.67\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{45}=-0.72\hat{i}-0.5\hat{j}+0.48\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result570.tex <==
2D-M570:

$\hat{n}_{14}=0.98\hat{i}-0.12\hat{j}+0.13\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.7\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result571.tex <==
2D-M571:

$\hat{n}_{14}=-0.05\hat{i}+1.0\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.63\hat{i}+0.63\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result572.tex <==
2D-M572:

$\hat{n}_{14}=-0.68\hat{i}+0.34\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}+0.77\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result573.tex <==
2D-M573:

$\hat{n}_{14}=-0.65\hat{i}+0.76\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.6\hat{i}-0.6\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{25}=-0.38\hat{i}+0.38\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result574.tex <==
2D-M574:

$\hat{n}_{14}=-0.45\hat{i}-0.89\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.63\hat{i}-0.63\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result575.tex <==
2D-M575:

$\hat{n}_{14}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-1.0\hat{i}+0.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.93\hat{i}-0.25\hat{j}-0.25\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result576.tex <==
2D-M576:

$\hat{n}_{14}=-0.95\hat{i}-0.23\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{25}=0.36\hat{i}+0.66\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{34}=-0.93\hat{i}+0.25\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result577.tex <==
2D-M577:

$\hat{n}_{14}=0.15\hat{i}-0.85\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.8\hat{i}+0.33\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.52\hat{j}-0.86\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result578.tex <==
2D-M578:

$\hat{n}_{14}=0.19\hat{i}+0.77\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{15}=-0.84\hat{i}+0.09\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.98\hat{i}-0.15\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.62\hat{j}+0.78\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result579.tex <==
2D-M579:

$\hat{n}_{14}=-0.81\hat{i}-0.27\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{15}=0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{23}=0.12\hat{i}+0.8\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}+0.54\hat{j}-0.61\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result58.tex <==
{\tiny 2D-M58:}

$\hat{n}_{14}=-0.0\hat{i}+0.85\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{25}=0.34\hat{i}-0.23\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{34}=-0.48\hat{i}-0.73\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{45}=-0.76\hat{i}-0.64\hat{j}-0.01\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result580.tex <==
2D-M580:

$\hat{n}_{14}=-0.49\hat{i}+0.81\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.65\hat{i}+0.1\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result581.tex <==
2D-M581:

$\hat{n}_{15}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}+0.42\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.01\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result582.tex <==
2D-M582:

$\hat{n}_{13}=0.23\hat{i}-0.75\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result583.tex <==
2D-M583:

$\hat{n}_{13}=-0.67\hat{i}+0.45\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{14}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=0.56\hat{i}-0.6\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{35}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result584.tex <==
2D-M584:

$\hat{n}_{13}=-0.25\hat{i}-0.55\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}-0.38\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.75\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.54\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result585.tex <==
2D-M585:

$\hat{n}_{13}=-0.02\hat{i}+0.7\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.8\hat{i}+0.52\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result586.tex <==
2D-M586:

$\hat{n}_{13}=-0.57\hat{i}-0.49\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.59\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result587.tex <==
2D-M587:

$\hat{n}_{13}=-0.05\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.36\hat{i}-0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.93\hat{i}-0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result588.tex <==
2D-M588:

$\hat{n}_{13}=0.36\hat{i}+0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.93\hat{i}+0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{45}=-0.05\hat{i}-0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result589.tex <==
2D-M589:

$\hat{n}_{13}=0.97\hat{i}-0.11\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.7\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{23}=0.48\hat{i}-0.87\hat{j}+0.06\hat{k}$,\;\;\;$\hat{n}_{35}=-0.19\hat{i}-0.87\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{23}=4.03\hat{i}+6.0\hat{j}+5.93\hat{k}$,\;\;\;$\vec{r}_{24}=6.07\hat{i}+6.19\hat{j}+4.65\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result59.tex <==
{\tiny 2D-M59:}

$\hat{n}_{14}=-0.79\hat{i}-0.21\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{15}=-0.4\hat{i}-0.12\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{23}=-0.63\hat{i}-0.63\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result590.tex <==
2D-M590:

$\hat{n}_{13}=0.57\hat{i}+0.49\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.59\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.26\hat{i}-0.84\hat{j}+0.47\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result591.tex <==
2D-M591:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=-0.62\hat{i}-0.77\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result592.tex <==
2D-M592:

$\hat{n}_{13}=0.76\hat{i}+0.65\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.63\hat{i}+0.63\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result593.tex <==
2D-M593:

$\hat{n}_{13}=0.03\hat{i}+0.87\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{14}=0.55\hat{i}-0.55\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.45\hat{i}+0.45\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result594.tex <==
2D-M594:

$\hat{n}_{13}=0.01\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.47\hat{i}+0.35\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}+0.42\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result595.tex <==
2D-M595:

$\hat{n}_{13}=0.58\hat{i}-0.82\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.34\hat{i}+0.47\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.6\hat{i}-0.56\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result596.tex <==
2D-M596:

$\hat{n}_{13}=-0.81\hat{i}-0.48\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{14}=-0.81\hat{i}-0.48\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.06\hat{i}+0.64\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result597.tex <==
2D-M597:

$\hat{n}_{13}=-0.84\hat{i}-0.37\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{14}=-0.13\hat{i}-0.99\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{23}=-0.19\hat{i}-0.98\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{35}=0.32\hat{i}-0.93\hat{j}-0.17\hat{k}$,\newline
$\vec{r}_{14}=5.77\hat{i}+4.06\hat{j}+3.99\hat{k}$,\;\;\;$\vec{r}_{24}=5.34\hat{i}+4.63\hat{j}+6.04\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result598.tex <==
2D-M598:

$\hat{n}_{13}=-0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.07\hat{i}-0.67\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result599.tex <==
2D-M599:

$\hat{n}_{13}=0.65\hat{i}+0.55\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.4\hat{i}-0.34\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}+0.71\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+2.98\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+5.77\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result6.tex <==
{\tiny 2D-M6:}

$\hat{n}_{14}=0.74\hat{i}-0.67\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{24}=-0.37\hat{i}-0.31\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.57\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result60.tex <==
{\tiny 2D-M60:}

$\hat{n}_{14}=0.8\hat{i}-0.54\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{15}=0.35\hat{i}+0.91\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.16\hat{i}-0.62\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result600.tex <==
2D-M600:

$\hat{n}_{13}=-0.21\hat{i}+0.58\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{14}=0.21\hat{i}-0.58\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.01\hat{i}+0.81\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result601.tex <==
2D-M601:

$\hat{n}_{13}=-0.77\hat{i}-0.63\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}-0.58\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.35\hat{i}-0.91\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{35}=0.63\hat{i}-0.77\hat{j}+0.03\hat{k}$,\newline
$\vec{r}_{14}=4.03\hat{i}+4.08\hat{j}+4.09\hat{k}$,\;\;\;$\vec{r}_{23}=4.01\hat{i}+5.96\hat{j}+5.94\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result602.tex <==
2D-M602:

$\hat{n}_{13}=0.57\hat{i}+0.49\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.59\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.57\hat{i}+0.29\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result603.tex <==
2D-M603:

$\hat{n}_{13}=-0.57\hat{i}-0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.56\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result604.tex <==
2D-M604:

$\hat{n}_{13}=-0.03\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.36\hat{i}+0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.93\hat{i}+0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result605.tex <==
2D-M605:

$\hat{n}_{13}=0.04\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.93\hat{i}+0.25\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{25}=-0.36\hat{i}+0.66\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result606.tex <==
2D-M606:

$\hat{n}_{13}=0.82\hat{i}+0.38\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{23}=-0.04\hat{i}-0.72\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.07\hat{i}+0.67\hat{j}-0.74\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result607.tex <==
2D-M607:

$\hat{n}_{13}=-0.02\hat{i}+0.65\hat{j}+0.76\hat{k}$,\;\;\;$\hat{n}_{23}=1.0\hat{i}+0.0\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}+0.76\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.53\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result608.tex <==
2D-M608:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.7\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{24}=0.76\hat{i}+0.65\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{45}=-0.1\hat{i}-0.92\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result609.tex <==
2D-M609:

$\hat{n}_{13}=0.79\hat{i}+0.27\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{23}=-0.11\hat{i}-0.98\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{24}=-0.02\hat{i}-0.99\hat{j}+0.11\hat{k}$,\;\;\;$\hat{n}_{35}=-0.6\hat{i}+0.19\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{14}=3.89\hat{i}+5.76\hat{j}+4.46\hat{k}$,\;\;\;$\vec{r}_{24}=3.89\hat{i}+5.39\hat{j}+6.11\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result61.tex <==
{\tiny 2D-M61:}

$\hat{n}_{14}=-0.67\hat{i}-0.3\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{15}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.3\hat{i}+0.67\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+7.65\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result610.tex <==
2D-M610:

$\hat{n}_{13}=0.45\hat{i}+0.36\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.33\hat{i}-0.48\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{25}=-0.44\hat{i}-0.71\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result611.tex <==
2D-M611:

$\hat{n}_{13}=0.37\hat{i}-0.93\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.93\hat{i}+0.37\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.79\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result612.tex <==
2D-M612:

$\hat{n}_{13}=-0.82\hat{i}-0.38\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.75\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.54\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.41\hat{i}+0.36\hat{j}-0.84\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result613.tex <==
2D-M613:

$\hat{n}_{13}=0.76\hat{i}-0.62\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{23}=-0.09\hat{i}-0.83\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.21\hat{i}-0.89\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{35}=-0.55\hat{i}-0.77\hat{j}+0.33\hat{k}$,\newline
$\vec{r}_{14}=6.72\hat{i}+5.99\hat{j}+6.41\hat{k}$,\;\;\;$\vec{r}_{23}=3.54\hat{i}+3.37\hat{j}+3.29\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result614.tex <==
2D-M614:

$\hat{n}_{13}=0.75\hat{i}-0.5\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{23}=-0.13\hat{i}+0.52\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}+0.71\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result615.tex <==
2D-M615:

$\hat{n}_{13}=0.83\hat{i}+0.22\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{24}=0.89\hat{i}+0.46\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.58\hat{j}-0.82\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result616.tex <==
2D-M616:

$\hat{n}_{13}=-0.56\hat{i}+0.63\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{23}=-0.56\hat{i}-0.77\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{25}=0.61\hat{i}-0.13\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result617.tex <==
2D-M617:

$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.03\hat{i}+0.78\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result618.tex <==
2D-M618:

$\hat{n}_{13}=-0.7\hat{i}+0.71\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{23}=0.7\hat{i}-0.71\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.01\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result619.tex <==
2D-M619:

$\hat{n}_{13}=-0.46\hat{i}-0.21\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.67\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{24}=-0.7\hat{i}-0.63\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result62.tex <==
{\tiny 2D-M62:}

$\hat{n}_{14}=0.81\hat{i}-0.54\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{23}=-0.37\hat{i}-0.15\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{25}=0.26\hat{i}+0.72\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{34}=-0.48\hat{i}-0.06\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result620.tex <==
2D-M620:

$\hat{n}_{14}=-0.28\hat{i}-0.96\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.96\hat{i}-0.28\hat{j}+0.07\hat{k}$,\;\;\;$\hat{n}_{25}=-0.18\hat{i}-0.76\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{34}=-0.8\hat{i}-0.26\hat{j}+0.54\hat{k}$,\newline
$\hat{n}_{35}=0.57\hat{i}-0.6\hat{j}+0.56\hat{k}$,\;\;\;$\vec{r}_{25}=5.33\hat{i}+4.37\hat{j}+4.5\hat{k}$,\;\;\;$\vec{r}_{34}=5.5\hat{i}+5.08\hat{j}+4.04\hat{k}$,\;\;\;$\vec{r}_{35}=5.23\hat{i}+5.61\hat{j}+4.85\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result621.tex <==
2D-M621:

$\hat{n}_{14}=-0.12\hat{i}-0.92\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{24}=-0.05\hat{i}-0.64\hat{j}+0.76\hat{k}$,\;\;\;$\hat{n}_{25}=0.99\hat{i}-0.12\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{34}=-0.54\hat{i}-0.63\hat{j}-0.56\hat{k}$,\newline
$\hat{n}_{35}=0.84\hat{i}-0.44\hat{j}-0.32\hat{k}$,\;\;\;$\vec{r}_{24}=5.61\hat{i}+4.52\hat{j}+4.72\hat{k}$,\;\;\;$\vec{r}_{34}=5.32\hat{i}+4.61\hat{j}+5.69\hat{k}$,\;\;\;$\vec{r}_{35}=5.68\hat{i}+4.49\hat{j}+4.87\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result622.tex <==
2D-M622:

$\hat{n}_{14}=0.13\hat{i}-0.96\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.74\hat{i}-0.27\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{25}=-0.55\hat{i}-0.3\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{34}=0.39\hat{i}-0.92\hat{j}-0.07\hat{k}$,\newline
$\hat{n}_{45}=0.74\hat{i}+0.27\hat{j}+0.62\hat{k}$,\;\;\;$\vec{r}_{25}=5.57\hat{i}+2.78\hat{j}+5.57\hat{k}$,\;\;\;$\vec{r}_{34}=5.22\hat{i}+5.68\hat{j}+5.16\hat{k}$,\;\;\;$\vec{r}_{45}=4.79\hat{i}+5.09\hat{j}+5.42\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result623.tex <==
2D-M623:

$\hat{n}_{14}=-0.62\hat{i}-0.79\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=-0.19\hat{i}-0.57\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=0.76\hat{i}-0.59\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{34}=-0.62\hat{i}-0.56\hat{j}+0.55\hat{k}$,\newline
$\hat{n}_{45}=0.76\hat{i}-0.59\hat{j}+0.25\hat{k}$,\;\;\;$\vec{r}_{23}=5.03\hat{i}+5.53\hat{j}+5.53\hat{k}$,\;\;\;$\vec{r}_{34}=5.47\hat{i}+5.5\hat{j}+5.13\hat{k}$,\;\;\;$\vec{r}_{45}=4.75\hat{i}+4.83\hat{j}+4.97\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result624.tex <==
2D-M624:

$\hat{n}_{14}=0.28\hat{i}-0.95\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{23}=-0.65\hat{i}+0.36\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.88\hat{j}-0.47\hat{k}$,\;\;\;$\hat{n}_{34}=-0.76\hat{i}-0.31\hat{j}+0.57\hat{k}$,\newline
$\hat{n}_{45}=0.76\hat{i}+0.31\hat{j}-0.57\hat{k}$,\;\;\;$\vec{r}_{23}=5.46\hat{i}+4.8\hat{j}+4.59\hat{k}$,\;\;\;$\vec{r}_{25}=5.47\hat{i}+5.47\hat{j}+5.46\hat{k}$,\;\;\;$\vec{r}_{45}=5.41\hat{i}+4.87\hat{j}+4.83\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result625.tex <==
2D-M625:

$\hat{n}_{14}=-0.82\hat{i}-0.53\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{23}=-0.72\hat{i}-0.55\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.13\hat{i}-0.71\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{34}=0.68\hat{i}-0.44\hat{j}-0.58\hat{k}$,\newline
$\hat{n}_{45}=0.55\hat{i}-0.83\hat{j}+0.08\hat{k}$,\;\;\;$\vec{r}_{23}=5.29\hat{i}+5.23\hat{j}+4.71\hat{k}$,\;\;\;$\vec{r}_{25}=5.24\hat{i}+4.87\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{34}=5.27\hat{i}+4.71\hat{j}+4.75\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result626.tex <==
2D-M626:

$\hat{n}_{13}=0.92\hat{i}-0.21\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{24}=-0.7\hat{i}+0.38\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{25}=0.72\hat{i}+0.37\hat{j}+0.59\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\vec{r}_{24}=5.1\hat{i}+5.02\hat{j}+4.88\hat{k}$,\;\;\;$\vec{r}_{25}=4.98\hat{i}+4.97\hat{j}+4.7\hat{k}$,\;\;\;$\vec{r}_{35}=5.0\hat{i}+5.34\hat{j}+4.97\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result627.tex <==
2D-M627:

$\hat{n}_{13}=-0.3\hat{i}-0.95\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{14}=-0.14\hat{i}-0.97\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{24}=0.76\hat{i}-0.24\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{25}=0.64\hat{i}+0.07\hat{j}+0.77\hat{k}$,\newline
$\hat{n}_{35}=-0.76\hat{i}+0.24\hat{j}+0.61\hat{k}$,\;\;\;$\vec{r}_{14}=4.84\hat{i}+5.25\hat{j}+5.19\hat{k}$,\;\;\;$\vec{r}_{25}=4.92\hat{i}+4.76\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{35}=5.12\hat{i}+4.84\hat{j}+5.2\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result628.tex <==
2D-M628:

$\hat{n}_{13}=0.29\hat{i}-0.93\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{14}=0.37\hat{i}-0.59\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.12\hat{i}-0.74\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=-0.92\hat{i}-0.33\hat{j}+0.2\hat{k}$,\newline
$\hat{n}_{35}=-0.92\hat{i}-0.33\hat{j}+0.2\hat{k}$,\;\;\;$\vec{r}_{14}=6.32\hat{i}+6.38\hat{j}+4.93\hat{k}$,\;\;\;$\vec{r}_{24}=6.43\hat{i}+6.16\hat{j}+4.07\hat{k}$,\;\;\;$\vec{r}_{35}=6.02\hat{i}+5.53\hat{j}+6.45\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result629.tex <==
2D-M629:

$\hat{n}_{13}=0.74\hat{i}-0.68\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{14}=-0.89\hat{i}-0.36\hat{j}+0.27\hat{k}$,\;\;\;$\hat{n}_{24}=0.12\hat{i}-0.77\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{25}=0.43\hat{i}-0.52\hat{j}+0.73\hat{k}$,\newline
$\hat{n}_{35}=-0.68\hat{i}-0.74\hat{j}-0.01\hat{k}$,\;\;\;$\vec{r}_{14}=5.03\hat{i}+4.8\hat{j}+5.77\hat{k}$,\;\;\;$\vec{r}_{24}=5.76\hat{i}+4.26\hat{j}+5.22\hat{k}$,\;\;\;$\vec{r}_{25}=4.62\hat{i}+4.42\hat{j}+4.9\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result63.tex <==
{\tiny 2D-M63:}

$\hat{n}_{14}=0.68\hat{i}+0.52\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.84\hat{i}+0.1\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.16\hat{j}-0.99\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+1.8\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result630.tex <==
2D-M630:

$\hat{n}_{13}=0.8\hat{i}-0.38\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{14}=-0.48\hat{i}+0.78\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{23}=0.09\hat{i}-0.68\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{25}=0.59\hat{i}+0.62\hat{j}+0.51\hat{k}$,\newline
$\hat{n}_{45}=0.65\hat{i}+0.01\hat{j}-0.76\hat{k}$,\;\;\;$\vec{r}_{14}=4.7\hat{i}+5.66\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{25}=6.03\hat{i}+5.58\hat{j}+4.55\hat{k}$,\;\;\;$\vec{r}_{45}=4.74\hat{i}+5.38\hat{j}+4.36\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result631.tex <==
2D-M631:

$\hat{n}_{13}=-0.6\hat{i}-0.75\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{14}=0.13\hat{i}-0.83\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.68\hat{i}-0.32\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.41\hat{i}-0.57\hat{j}-0.71\hat{k}$,\newline
$\hat{n}_{45}=-0.72\hat{i}-0.45\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{14}=4.8\hat{i}+5.04\hat{j}+5.14\hat{k}$,\;\;\;$\vec{r}_{23}=4.8\hat{i}+5.08\hat{j}+5.19\hat{k}$,\;\;\;$\vec{r}_{45}=4.8\hat{i}+4.92\hat{j}+5.14\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result632.tex <==
2D-M632:

$\hat{n}_{13}=-0.55\hat{i}+0.61\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=0.55\hat{i}-0.61\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{23}=0.66\hat{i}-0.1\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{25}=-0.51\hat{i}-0.79\hat{j}+0.35\hat{k}$,\newline
$\hat{n}_{45}=0.82\hat{i}+0.25\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{14}=5.03\hat{i}+5.08\hat{j}+4.43\hat{k}$,\;\;\;$\vec{r}_{23}=4.96\hat{i}+4.92\hat{j}+4.61\hat{k}$,\;\;\;$\vec{r}_{25}=4.99\hat{i}+5.5\hat{j}+4.97\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result633.tex <==
2D-M633:

$\hat{n}_{13}=-0.22\hat{i}-0.66\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.22\hat{i}-0.66\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.94\hat{i}-0.06\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{24}=0.27\hat{i}-0.74\hat{j}-0.61\hat{k}$,\newline
$\hat{n}_{45}=0.43\hat{i}-0.72\hat{j}-0.54\hat{k}$,\;\;\;$\vec{r}_{14}=5.81\hat{i}+4.94\hat{j}+5.59\hat{k}$,\;\;\;$\vec{r}_{23}=5.82\hat{i}+5.62\hat{j}+5.68\hat{k}$,\;\;\;$\vec{r}_{24}=5.41\hat{i}+5.81\hat{j}+4.83\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result634.tex <==
2D-M634:

$\hat{n}_{13}=-0.36\hat{i}-0.72\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{14}=-0.83\hat{i}-0.54\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{23}=0.14\hat{i}-0.98\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{24}=-0.05\hat{i}-0.98\hat{j}-0.19\hat{k}$,\newline
$\hat{n}_{35}=0.91\hat{i}-0.41\hat{j}-0.05\hat{k}$,\;\;\;$\vec{r}_{14}=5.41\hat{i}+6.3\hat{j}+5.72\hat{k}$,\;\;\;$\vec{r}_{23}=6.29\hat{i}+4.07\hat{j}+4.39\hat{k}$,\;\;\;$\vec{r}_{24}=4.55\hat{i}+5.87\hat{j}+5.73\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result635.tex <==
2D-M635:

$\hat{n}_{13}=-0.64\hat{i}-0.34\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.35\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{23}=-0.56\hat{i}-0.4\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=-0.08\hat{i}-0.85\hat{j}+0.52\hat{k}$,\newline
$\hat{n}_{25}=0.53\hat{i}-0.84\hat{j}+0.08\hat{k}$,\;\;\;$\vec{r}_{14}=5.14\hat{i}+4.94\hat{j}+4.73\hat{k}$,\;\;\;$\vec{r}_{23}=4.92\hat{i}+4.92\hat{j}+5.18\hat{k}$,\;\;\;$\vec{r}_{24}=5.28\hat{i}+5.07\hat{j}+4.34\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result636.tex <==
2D-M636:

$\hat{n}_{13}=0.71\hat{i}+0.58\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{14}=0.1\hat{i}-0.65\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.92\hat{i}-0.23\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{25}=-0.38\hat{i}-0.72\hat{j}-0.58\hat{k}$,\newline
$\hat{n}_{35}=-0.7\hat{i}+0.49\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{13}=5.53\hat{i}+4.39\hat{j}+5.47\hat{k}$,\;\;\;$\vec{r}_{14}=5.67\hat{i}+4.41\hat{j}+5.69\hat{k}$,\;\;\;$\vec{r}_{35}=4.4\hat{i}+5.62\hat{j}+4.11\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result637.tex <==
2D-M637:

$\hat{n}_{13}=-0.23\hat{i}-0.83\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{14}=0.39\hat{i}-0.56\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{24}=-0.23\hat{i}-0.83\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.89\hat{i}+0.03\hat{j}+0.45\hat{k}$,\newline
$\hat{n}_{35}=-0.97\hat{i}+0.18\hat{j}-0.14\hat{k}$,\;\;\;$\vec{r}_{13}=3.21\hat{i}+4.86\hat{j}+5.67\hat{k}$,\;\;\;$\vec{r}_{14}=5.98\hat{i}+4.92\hat{j}+3.95\hat{k}$,\;\;\;$\vec{r}_{25}=5.09\hat{i}+4.22\hat{j}+5.31\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result638.tex <==
2D-M638:

$\hat{n}_{13}=0.38\hat{i}-0.92\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{14}=0.47\hat{i}+0.08\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}-0.4\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{25}=0.38\hat{i}-0.92\hat{j}+0.12\hat{k}$,\newline
$\hat{n}_{35}=-0.91\hat{i}-0.35\hat{j}+0.22\hat{k}$,\;\;\;$\vec{r}_{13}=5.58\hat{i}+5.48\hat{j}+5.37\hat{k}$,\;\;\;$\vec{r}_{14}=5.7\hat{i}+4.44\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{24}=4.21\hat{i}+5.3\hat{j}+5.78\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result639.tex <==
2D-M639:

$\hat{n}_{13}=0.77\hat{i}-0.16\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{14}=0.42\hat{i}-0.6\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}-0.6\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{24}=-0.48\hat{i}-0.79\hat{j}+0.4\hat{k}$,\newline
$\hat{n}_{45}=-0.6\hat{i}-0.75\hat{j}+0.29\hat{k}$,\;\;\;$\vec{r}_{13}=4.51\hat{i}+5.52\hat{j}+4.98\hat{k}$,\;\;\;$\vec{r}_{14}=4.46\hat{i}+5.27\hat{j}+5.44\hat{k}$,\;\;\;$\vec{r}_{24}=4.6\hat{i}+5.54\hat{j}+5.22\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result64.tex <==
{\tiny 2D-M64:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.88\hat{i}+0.23\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{25}=0.47\hat{i}-0.32\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{34}=-0.7\hat{i}-0.67\hat{j}-0.26\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result640.tex <==
2D-M640:

$\hat{n}_{13}=0.83\hat{i}-0.46\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{14}=-0.21\hat{i}-0.78\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{23}=0.83\hat{i}-0.46\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}-0.43\hat{j}+0.74\hat{k}$,\newline
$\hat{n}_{35}=-0.5\hat{i}-0.86\hat{j}+0.06\hat{k}$,\;\;\;$\vec{r}_{13}=4.66\hat{i}+5.31\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{14}=4.67\hat{i}+5.05\hat{j}+4.71\hat{k}$,\;\;\;$\vec{r}_{24}=5.26\hat{i}+4.83\hat{j}+4.96\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result641.tex <==
2D-M641:

$\hat{n}_{13}=-0.59\hat{i}-0.49\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{14}=0.81\hat{i}-0.38\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{23}=0.69\hat{i}-0.72\hat{j}+0.08\hat{k}$,\;\;\;$\hat{n}_{24}=-0.02\hat{i}-0.78\hat{j}-0.62\hat{k}$,\newline
$\hat{n}_{25}=-0.72\hat{i}-0.68\hat{j}+0.09\hat{k}$,\;\;\;$\vec{r}_{13}=5.42\hat{i}+5.52\hat{j}+5.21\hat{k}$,\;\;\;$\vec{r}_{14}=5.48\hat{i}+4.49\hat{j}+5.19\hat{k}$,\;\;\;$\vec{r}_{24}=5.53\hat{i}+5.39\hat{j}+5.46\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result65.tex <==
{\tiny 2D-M65:}

$\hat{n}_{14}=0.31\hat{i}-0.9\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{23}=0.77\hat{i}+0.37\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.32\hat{i}+0.66\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{34}=0.13\hat{i}-0.63\hat{j}-0.76\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result66.tex <==
{\tiny 2D-M66:}

$\hat{n}_{15}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{23}=0.7\hat{i}-0.7\hat{j}+0.17\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.5\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{34}=-0.15\hat{i}-0.62\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result67.tex <==
{\tiny 2D-M67:}

$\hat{n}_{13}=0.14\hat{i}+0.99\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.39\hat{i}+0.52\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=0.79\hat{i}+0.57\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{25}=-0.61\hat{i}-0.01\hat{j}-0.79\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result68.tex <==
{\tiny 2D-M68:}

$\hat{n}_{13}=0.61\hat{i}+0.15\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{14}=0.57\hat{i}-0.22\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}+0.64\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{35}=-0.52\hat{i}-0.82\hat{j}-0.24\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result69.tex <==
{\tiny 2D-M69:}

$\hat{n}_{13}=0.69\hat{i}-0.03\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{14}=-0.33\hat{i}+0.9\hat{j}+0.29\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}-0.85\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{25}=0.34\hat{i}+0.69\hat{j}-0.64\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result7.tex <==
{\tiny 2D-M7:}

$\hat{n}_{14}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.11\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result70.tex <==
{\tiny 2D-M70:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.6\hat{i}+0.54\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{24}=-0.67\hat{i}-0.3\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{35}=0.6\hat{i}+0.49\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+2.68\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result71.tex <==
{\tiny 2D-M71:}

$\hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{14}=0.7\hat{i}-0.18\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{25}=-0.15\hat{i}+0.7\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{35}=0.5\hat{i}+0.78\hat{j}+0.37\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result72.tex <==
{\tiny 2D-M72:}

$\hat{n}_{13}=0.81\hat{i}-0.4\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.73\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{25}=0.95\hat{i}+0.13\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{35}=0.03\hat{i}+0.76\hat{j}+0.65\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result73.tex <==
{\tiny 2D-M73:}

$\hat{n}_{13}=0.0\hat{i}+0.05\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.05\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.46\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.86\hat{j}-0.51\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result74.tex <==
{\tiny 2D-M74:}

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.02\hat{i}-0.9\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{23}=-0.94\hat{i}-0.11\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{35}=-0.87\hat{i}-0.5\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=7.25\hat{i}+5.1\hat{j}+3.87\hat{k}$,\;\;\;$\vec{r}_{23}=8.61\hat{i}+8.77\hat{j}+6.23\hat{k}$,\;\;\;$\vec{r}_{24}=1.63\hat{i}+6.13\hat{j}+3.88\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result75.tex <==
{\tiny 2D-M75:}

$\hat{n}_{13}=0.05\hat{i}+0.55\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{14}=0.65\hat{i}-0.39\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.25\hat{j}-0.97\hat{k}$,\;\;\;$\hat{n}_{25}=0.48\hat{i}-0.37\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result76.tex <==
{\tiny 2D-M76:}

$\hat{n}_{13}=0.7\hat{i}-0.14\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{14}=-0.52\hat{i}+0.82\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{24}=0.22\hat{i}-0.18\hat{j}-0.96\hat{k}$,\;\;\;$\hat{n}_{25}=0.36\hat{i}-0.63\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result77.tex <==
{\tiny 2D-M77:}

$\hat{n}_{13}=0.73\hat{i}+0.15\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{14}=-0.91\hat{i}+0.3\hat{j}-0.28\hat{k}$,\;\;\;$\hat{n}_{24}=-0.47\hat{i}-0.47\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.67\hat{j}+0.74\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result78.tex <==
{\tiny 2D-M78:}

$\hat{n}_{13}=-0.67\hat{i}-0.6\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.18\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.67\hat{i}+0.49\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+9.99\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result79.tex <==
{\tiny 2D-M79:}

$\hat{n}_{13}=0.0\hat{i}+0.62\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{14}=0.43\hat{i}-0.88\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.77\hat{i}+0.12\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result8.tex <==
{\tiny 2D-M8:}

$\hat{n}_{14}=-0.46\hat{i}+0.74\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result80.tex <==
{\tiny 2D-M80:}

$\hat{n}_{13}=0.04\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.86\hat{i}-0.35\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{23}=0.81\hat{i}-0.31\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{45}=0.01\hat{i}-0.72\hat{j}-0.69\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result81.tex <==
{\tiny 2D-M81:}

$\hat{n}_{13}=-0.0\hat{i}+0.87\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.28\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=-0.49\hat{i}-0.73\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{45}=-0.08\hat{i}+0.55\hat{j}+0.83\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result82.tex <==
{\tiny 2D-M82:}

$\hat{n}_{13}=-0.51\hat{i}+0.31\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.04\hat{i}-0.6\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=0.37\hat{i}-0.47\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{35}=-0.02\hat{i}+0.6\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.5\hat{i}+2.54\hat{j}+7.9\hat{k}$,\;\;\;$\vec{r}_{23}=8.09\hat{i}+8.34\hat{j}+4.68\hat{k}$,\;\;\;$\vec{r}_{24}=9.23\hat{i}+8.25\hat{j}+1.09\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result83.tex <==
{\tiny 2D-M83:}

$\hat{n}_{13}=0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{14}=0.79\hat{i}-0.21\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}+0.47\hat{j}+0.33\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result84.tex <==
{\tiny 2D-M84:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.48\hat{i}+0.77\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.0\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{45}=0.5\hat{i}+0.61\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result85.tex <==
{\tiny 2D-M85:}

$\hat{n}_{13}=-0.65\hat{i}+0.65\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{14}=-0.48\hat{i}+0.45\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.63\hat{i}+0.46\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{45}=0.01\hat{i}+0.58\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result86.tex <==
{\tiny 2D-M86:}

$\hat{n}_{13}=-0.16\hat{i}-0.63\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{14}=-0.22\hat{i}-0.92\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{24}=1.0\hat{i}-0.08\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{35}=-0.71\hat{i}+0.1\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=7.61\hat{i}+1.62\hat{j}+8.23\hat{k}$,\;\;\;$\vec{r}_{23}=1.68\hat{i}+5.11\hat{j}+6.63\hat{k}$,\;\;\;$\vec{r}_{24}=5.61\hat{i}+4.8\hat{j}+3.36\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result87.tex <==
{\tiny 2D-M87:}

$\hat{n}_{13}=0.66\hat{i}-0.66\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{14}=0.52\hat{i}-0.42\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.12\hat{i}-0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{25}=0.68\hat{i}+0.16\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result88.tex <==
{\tiny 2D-M88:}

$\hat{n}_{13}=0.0\hat{i}+0.62\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}+0.42\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.7\hat{j}-0.72\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result89.tex <==
{\tiny 2D-M89:}

$\hat{n}_{13}=-0.0\hat{i}-0.58\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}-0.54\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.38\hat{j}-0.92\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}+0.51\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result9.tex <==
{\tiny 2D-M9:}

$\hat{n}_{14}=-0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{25}=-0.36\hat{i}-0.93\hat{j}-0.05\hat{k}$,\;\;\;$\hat{n}_{45}=0.71\hat{i}-0.1\hat{j}+0.7\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=6.41\hat{i}+3.46\hat{j}+3.55\hat{k}$,\;\;\;$\vec{r}_{34}=6.26\hat{i}+6.53\hat{j}+1.95\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result90.tex <==
{\tiny 2D-M90:}

$\hat{n}_{13}=0.71\hat{i}-0.1\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=0.3\hat{i}+0.67\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.03\hat{i}+0.68\hat{j}+0.73\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result91.tex <==
{\tiny 2D-M91:}

$\hat{n}_{13}=-0.85\hat{i}+0.47\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.13\hat{i}-0.63\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{45}=-0.33\hat{i}-0.9\hat{j}+0.29\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result92.tex <==
{\tiny 2D-M92:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}-0.44\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{25}=0.41\hat{i}+0.2\hat{j}-0.89\hat{k}$,\;\;\;$\hat{n}_{45}=0.75\hat{i}-0.65\hat{j}+0.11\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+9.97\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result93.tex <==
{\tiny 2D-M93:}

$\hat{n}_{13}=-0.32\hat{i}+0.6\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{23}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.33\hat{i}-0.33\hat{j}-0.89\hat{k}$,\;\;\;$\hat{n}_{45}=-0.29\hat{i}-0.38\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result94.tex <==
{\tiny 2D-M94:}

$\hat{n}_{13}=0.6\hat{i}-0.11\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{23}=0.13\hat{i}-0.76\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{24}=-0.28\hat{i}+0.27\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{35}=0.13\hat{i}-0.65\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=6.57\hat{i}+7.46\hat{j}+8.53\hat{k}$,\;\;\;$\vec{r}_{23}=7.76\hat{i}+9.05\hat{j}+0.95\hat{k}$,\;\;\;$\vec{r}_{24}=8.61\hat{i}+8.08\hat{j}+6.19\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result95.tex <==
{\tiny 2D-M95:}

$\hat{n}_{13}=0.82\hat{i}-0.38\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.6\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.77\hat{i}-0.22\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{25}=0.3\hat{i}-0.62\hat{j}-0.73\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result96.tex <==
{\tiny 2D-M96:}

$\hat{n}_{13}=0.07\hat{i}-0.81\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.35\hat{i}-0.92\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.39\hat{i}-0.83\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{45}=0.75\hat{i}-0.47\hat{j}+0.47\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result97.tex <==
{\tiny 2D-M97:}

$\hat{n}_{13}=-0.69\hat{i}-0.36\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.36\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.67\hat{i}-0.35\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{45}=0.9\hat{i}+0.28\hat{j}+0.33\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result98.tex <==
{\tiny 2D-M98:}

$\hat{n}_{13}=0.67\hat{i}+0.12\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.83\hat{i}+0.3\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{24}=-0.87\hat{i}+0.24\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{35}=-0.17\hat{i}+0.67\hat{j}-0.73\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.35\hat{i}+7.41\hat{j}+8.14\hat{k}$,\;\;\;$\vec{r}_{23}=2.65\hat{i}+5.33\hat{j}+4.37\hat{k}$,\;\;\;$\vec{r}_{24}=1.81\hat{i}+5.97\hat{j}+8.77\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof2_2/result99.tex <==
{\tiny 2D-M99:}

$\hat{n}_{13}=0.48\hat{i}+0.77\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{23}=-0.7\hat{i}-0.56\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.64\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.48\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof3/result1.tex <==
{\tiny 3D-M1:}

$\hat{n}_{13}=-0.71\hat{i}+0.11\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.46\hat{j}-0.34\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof3/result2.tex <==
{\tiny 3D-M2:}

$\hat{n}_{13}=-0.8\hat{i}+0.33\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}+0.67\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.67\hat{j}-0.48\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof3/result3.tex <==
{\tiny 3D-M3:}

$\hat{n}_{13}=-0.8\hat{i}+0.58\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{23}=-0.74\hat{i}-0.51\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}+0.16\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof3/result4.tex <==
{\tiny 3D-M4:}

$\hat{n}_{13}=-0.57\hat{i}-0.67\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.36\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.76\hat{i}-0.65\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof3/result5.tex <==
{\tiny 3D-M5:}

$\hat{n}_{13}=0.5\hat{i}+0.18\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.76\hat{i}-0.61\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{24}=0.03\hat{i}+0.33\hat{j}-0.94\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof3/result6.tex <==
{\tiny 3D-M6:}

$\hat{n}_{13}=-0.6\hat{i}-0.76\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=0.26\hat{i}+0.4\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=-0.21\hat{i}-0.17\hat{j}+0.96\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof3/result7.tex <==
{\tiny 3D-M7:}

$\hat{n}_{13}=-0.54\hat{i}-0.83\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{23}=0.18\hat{i}-0.26\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{24}=-0.04\hat{i}-0.56\hat{j}-0.83\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof3/result8.tex <==
{\tiny 3D-M8:}

$\hat{n}_{13}=0.41\hat{i}+0.89\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}+0.11\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.67\hat{i}+0.44\hat{j}+0.59\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result1.tex <==
{\tiny 4D-M1:}

$\hat{n}_{14}=-0.29\hat{i}+0.57\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.75\hat{i}-0.53\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.34\hat{i}+0.83\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{34}=-0.72\hat{i}+0.12\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result10.tex <==
{\tiny 4D-M10:}

$\hat{n}_{14}=-0.63\hat{i}-0.76\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}+0.59\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result11.tex <==
{\tiny 4D-M11:}

$\hat{n}_{14}=-0.32\hat{i}+0.81\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.78\hat{i}+0.52\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.54\hat{i}+0.84\hat{j}+0.08\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result12.tex <==
{\tiny 4D-M12:}

$\hat{n}_{14}=0.09\hat{i}-1.0\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{23}=0.67\hat{i}+0.35\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}-0.88\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{34}=-0.75\hat{i}+0.31\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=4.0\hat{i}+2.99\hat{j}+5.94\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result13.tex <==
{\tiny 4D-M13:}

$\hat{n}_{14}=-0.94\hat{i}-0.18\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{23}=0.32\hat{i}-0.95\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=-0.03\hat{i}-0.8\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=0.34\hat{i}-0.57\hat{j}-0.75\hat{k}$,\newline
$\vec{r}_{23}=7.59\hat{i}+3.33\hat{j}+4.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result14.tex <==
{\tiny 4D-M14:}

$\hat{n}_{14}=-0.38\hat{i}-0.54\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.53\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=0.34\hat{i}-0.93\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{34}=0.75\hat{i}-0.65\hat{j}+0.1\hat{k}$,\newline
$\vec{r}_{25}=3.55\hat{i}+6.33\hat{j}+6.15\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result15.tex <==
{\tiny 4D-M15:}

$\hat{n}_{14}=-0.19\hat{i}-0.68\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.56\hat{i}-0.67\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{25}=-0.8\hat{i}-0.3\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}-0.54\hat{j}+0.05\hat{k}$,\newline
$\vec{r}_{34}=3.99\hat{i}+5.66\hat{j}+6.62\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result2.tex <==
{\tiny 4D-M2:}

$\hat{n}_{14}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{23}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=-0.42\hat{i}-0.85\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{34}=0.57\hat{i}+0.69\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result3.tex <==
{\tiny 4D-M3:}

$\hat{n}_{14}=0.39\hat{i}+0.47\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{23}=-0.42\hat{i}-0.85\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.69\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.49\hat{j}-0.3\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result4.tex <==
{\tiny 4D-M4:}

$\hat{n}_{14}=0.42\hat{i}+0.85\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{23}=-0.57\hat{i}-0.69\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{25}=-0.39\hat{i}-0.47\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.49\hat{j}-0.3\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result5.tex <==
{\tiny 4D-M5:}

$\hat{n}_{14}=-0.57\hat{i}-0.69\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}+0.85\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result6.tex <==
{\tiny 4D-M6:}

$\hat{n}_{14}=-0.54\hat{i}-0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.53\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.81\hat{j}-0.12\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result7.tex <==
{\tiny 4D-M7:}

$\hat{n}_{14}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.05\hat{i}+0.94\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}+0.22\hat{j}-0.49\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result8.tex <==
{\tiny 4D-M8:}

$\hat{n}_{14}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}+0.85\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{25}=-0.8\hat{i}-0.46\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> Dimensional Synthesis/contentfolder/mechanisms2/result/dof4/result9.tex <==
{\tiny 4D-M9:}

$\hat{n}_{14}=-0.08\hat{i}-0.96\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{23}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=-0.84\hat{i}-0.08\hat{j}+0.53\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> classes/1dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/1.png}}{{\tiny 1D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/2.png}}{{\tiny 1D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/3.png}}{{\tiny 1D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/4.png}}{{\tiny 1D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/5.png}}{{\tiny 1D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/6.png}}{{\tiny 1D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/7.png}}{{\tiny 1D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/8.png}}{{\tiny 1D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/9.png}}{{\tiny 1D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/10.png}}{{\tiny 1D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/11.png}}{{\tiny 1D-M11}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/12.png}}{{\tiny 1D-M12}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/13.png}}{{\tiny 1D-M13}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/14.png}}{{\tiny 1D-M14}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/15.png}}{{\tiny 1D-M15}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/16.png}}{{\tiny 1D-M16}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/17.png}}{{\tiny 1D-M17}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/18.png}}{{\tiny 1D-M18}}
\qquad \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/19.png}}{{\tiny 1D-M19}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/20.png}}{{\tiny 1D-M20}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/21.png}}{{\tiny 1D-M21}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/22.png}}{{\tiny 1D-M22}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/23.png}}{{\tiny 1D-M23}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/24.png}}{{\tiny 1D-M24}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/25.png}}{{\tiny 1D-M25}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/26.png}}{{\tiny 1D-M26}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/27.png}}{{\tiny 1D-M27}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/28.png}}{{\tiny 1D-M28}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/29.png}}{{\tiny 1D-M29}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/30.png}}{{\tiny 1D-M30}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/31.png}}{{\tiny 1D-M31}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/32.png}}{{\tiny 1D-M32}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/33.png}}{{\tiny 1D-M33}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/34.png}}{{\tiny 1D-M34}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/35.png}}{{\tiny 1D-M35}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/36.png}}{{\tiny 1D-M36}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/37.png}}{{\tiny 1D-M37}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/38.png}}{{\tiny 1D-M38}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/39.png}}{{\tiny 1D-M39}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/40.png}}{{\tiny 1D-M40}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/41.png}}{{\tiny 1D-M41}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/42.png}}{{\tiny 1D-M42}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/43.png}}{{\tiny 1D-M43}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/44.png}}{{\tiny 1D-M44}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/45.png}}{{\tiny 1D-M45}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/46.png}}{{\tiny 1D-M46}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/47.png}}{{\tiny 1D-M47}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/48.png}}{{\tiny 1D-M48}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/49.png}}{{\tiny 1D-M49}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/50.png}}{{\tiny 1D-M50}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/51.png}}{{\tiny 1D-M51}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/52.png}}{{\tiny 1D-M52}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/53.png}}{{\tiny 1D-M53}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/54.png}}{{\tiny 1D-M54}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/55.png}}{{\tiny 1D-M55}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/56.png}}{{\tiny 1D-M56}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/57.png}}{{\tiny 1D-M57}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/58.png}}{{\tiny 1D-M58}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/59.png}}{{\tiny 1D-M59}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/60.png}}{{\tiny 1D-M60}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/61.png}}{{\tiny 1D-M61}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/62.png}}{{\tiny 1D-M62}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/63.png}}{{\tiny 1D-M63}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/64.png}}{{\tiny 1D-M64}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/65.png}}{{\tiny 1D-M65}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/66.png}}{{\tiny 1D-M66}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/67.png}}{{\tiny 1D-M67}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/68.png}}{{\tiny 1D-M68}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/69.png}}{{\tiny 1D-M69}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/70.png}}{{\tiny 1D-M70}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/71.png}}{{\tiny 1D-M71}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/72.png}}{{\tiny 1D-M72}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/73.png}}{{\tiny 1D-M73}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/74.png}}{{\tiny 1D-M74}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/75.png}}{{\tiny 1D-M75}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/76.png}}{{\tiny 1D-M76}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/77.png}}{{\tiny 1D-M77}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/78.png}}{{\tiny 1D-M78}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/79.png}}{{\tiny 1D-M79}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/80.png}}{{\tiny 1D-M80}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/81.png}}{{\tiny 1D-M81}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/82.png}}{{\tiny 1D-M82}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/83.png}}{{\tiny 1D-M83}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/84.png}}{{\tiny 1D-M84}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/85.png}}{{\tiny 1D-M85}}
\qquad\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/86.png}}{{\tiny 1D-M86}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/87.png}}{{\tiny 1D-M87}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/88.png}}{{\tiny 1D-M88}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/89.png}}{{\tiny 1D-M89}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/90.png}}{{\tiny 1D-M90}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/91.png}}{{\tiny 1D-M91}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/92.png}}{{\tiny 1D-M92}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/93.png}}{{\tiny 1D-M93}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/94.png}}{{\tiny 1D-M94}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/95.png}}{{\tiny 1D-M95}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/96.png}}{{\tiny 1D-M96}}

  \end{minipage}
\end{subfigure}
\caption{Schematic diagrams of 1-DOF Manipulators}
\end{figure}

% \begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering

% \end{minipage}
% \end{subfigure}
% \caption{Class 2 of 1-DOF Manipulators}
% \end{figure}\begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering





%   \end{minipage}
% \end{subfigure}
% \caption{Class 3 of 1-DOF Manipulators}
% \end{figure}

% \begin{figure}[H]\ContinuedFloat
%   \centering
%   \begin{subfigure}{\columnwidth}
%     \begin{minipage}{\textwidth}\footnotesize
%     \centering

  
%     \end{minipage}
%   \end{subfigure}
%   \caption{Class 3 of 1-DOF Manipulators (Contd.)}
%   \end{figure}

% \begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 4 of 1-DOF Manipulators}
% \end{figure}\begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 5 of 1-DOF Manipulators}
% \end{figure}

% \begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 6 of 1-DOF Manipulators}
% \end{figure}

% \begin{figure}[H]\ContinuedFloat
%   \centering
%   \begin{subfigure}{\columnwidth}
%     \begin{minipage}{\textwidth}\footnotesize
%     \centering

  
  
%     \end{minipage}
%   \end{subfigure}
%   \caption{Class 6 of 1-DOF Manipulators (Contd.)}
%   \end{figure}

% \begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 7 of 1-DOF Manipulators}
% \end{figure}\begin{figure}[H]
% \centering
% \begin{subfigure}{\columnwidth}
%   \begin{minipage}{\textwidth}\footnotesize
%   \centering


%   \end{minipage}
% \end{subfigure}
% \caption{Class 8 of 1-DOF Manipulators}
% \end{figure}

==> classes/1dof_classes_old.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/1.png}}{{\tiny 1D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/2.png}}{{\tiny 1D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/3.png}}{{\tiny 1D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/4.png}}{{\tiny 1D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/5.png}}{{\tiny 1D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/6.png}}{{\tiny 1D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/7.png}}{{\tiny 1D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/8.png}}{{\tiny 1D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/9.png}}{{\tiny 1D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/10.png}}{{\tiny 1D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/11.png}}{{\tiny 1D-M11}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/12.png}}{{\tiny 1D-M12}}


  \end{minipage}
\end{subfigure}
\caption{Class 1 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/13.png}}{{\tiny 1D-M13}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/14.png}}{{\tiny 1D-M14}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/15.png}}{{\tiny 1D-M15}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/16.png}}{{\tiny 1D-M16}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/17.png}}{{\tiny 1D-M17}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/18.png}}{{\tiny 1D-M18}}
\qquad \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/19.png}}{{\tiny 1D-M19}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/20.png}}{{\tiny 1D-M20}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/21.png}}{{\tiny 1D-M21}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/22.png}}{{\tiny 1D-M22}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/23.png}}{{\tiny 1D-M23}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/24.png}}{{\tiny 1D-M24}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/25.png}}{{\tiny 1D-M25}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/26.png}}{{\tiny 1D-M26}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/27.png}}{{\tiny 1D-M27}}
\end{minipage}
\end{subfigure}
\caption{Class 2 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering


\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/28.png}}{{\tiny 1D-M28}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/29.png}}{{\tiny 1D-M29}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/30.png}}{{\tiny 1D-M30}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/31.png}}{{\tiny 1D-M31}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/32.png}}{{\tiny 1D-M32}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/33.png}}{{\tiny 1D-M33}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/34.png}}{{\tiny 1D-M34}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/35.png}}{{\tiny 1D-M35}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/36.png}}{{\tiny 1D-M36}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/37.png}}{{\tiny 1D-M37}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/38.png}}{{\tiny 1D-M38}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/39.png}}{{\tiny 1D-M39}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/40.png}}{{\tiny 1D-M40}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/41.png}}{{\tiny 1D-M41}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/42.png}}{{\tiny 1D-M42}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/43.png}}{{\tiny 1D-M43}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/44.png}}{{\tiny 1D-M44}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/45.png}}{{\tiny 1D-M45}}


  \end{minipage}
\end{subfigure}
\caption{Class 3 of 1-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/46.png}}{{\tiny 1D-M46}}
    \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/47.png}}{{\tiny 1D-M47}}
    \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/48.png}}{{\tiny 1D-M48}}
    \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/49.png}}{{\tiny 1D-M49}}
    \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/50.png}}{{\tiny 1D-M50}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/51.png}}{{\tiny 1D-M51}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/52.png}}{{\tiny 1D-M52}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/53.png}}{{\tiny 1D-M53}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/54.png}}{{\tiny 1D-M54}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/55.png}}{{\tiny 1D-M55}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/56.png}}{{\tiny 1D-M56}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/57.png}}{{\tiny 1D-M57}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 3 of 1-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/58.png}}{{\tiny 1D-M58}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/59.png}}{{\tiny 1D-M59}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/60.png}}{{\tiny 1D-M60}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/61.png}}{{\tiny 1D-M61}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/62.png}}{{\tiny 1D-M62}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/63.png}}{{\tiny 1D-M63}}

  \end{minipage}
\end{subfigure}
\caption{Class 4 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/64.png}}{{\tiny 1D-M64}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/65.png}}{{\tiny 1D-M65}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/66.png}}{{\tiny 1D-M66}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/67.png}}{{\tiny 1D-M67}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/68.png}}{{\tiny 1D-M68}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/69.png}}{{\tiny 1D-M69}}

  \end{minipage}
\end{subfigure}
\caption{Class 5 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/70.png}}{{\tiny 1D-M70}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/71.png}}{{\tiny 1D-M71}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/72.png}}{{\tiny 1D-M72}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/73.png}}{{\tiny 1D-M73}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/74.png}}{{\tiny 1D-M74}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/75.png}}{{\tiny 1D-M75}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/76.png}}{{\tiny 1D-M76}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/77.png}}{{\tiny 1D-M77}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/78.png}}{{\tiny 1D-M78}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/79.png}}{{\tiny 1D-M79}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/80.png}}{{\tiny 1D-M80}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/81.png}}{{\tiny 1D-M81}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/82.png}}{{\tiny 1D-M82}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/83.png}}{{\tiny 1D-M83}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/84.png}}{{\tiny 1D-M84}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/85.png}}{{\tiny 1D-M85}}

  \end{minipage}
\end{subfigure}
\caption{Class 6 of 1-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/86.png}}{{\tiny 1D-M86}}
  \qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/87.png}}{{\tiny 1D-M87}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 1-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/88.png}}{{\tiny 1D-M88}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/89.png}}{{\tiny 1D-M89}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/90.png}}{{\tiny 1D-M90}}

  \end{minipage}
\end{subfigure}
\caption{Class 7 of 1-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/91.png}}{{\tiny 1D-M91}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/92.png}}{{\tiny 1D-M92}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/93.png}}{{\tiny 1D-M93}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/1dof/94.png}}{{\tiny 1D-M94}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/95.png}}{{\tiny 1D-M95}}
\qquad\subsubfloat{\includegraphics[width=0.04\textwidth]{contentfolder/images/1dof/96.png}}{{\tiny 1D-M96}}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 1-DOF Manipulators}
\end{figure}

==> classes/2dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/1.png}}{{\tiny 2D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/2.png}}{{\tiny 2D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/3.png}}{{\tiny 2D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/4.png}}{{\tiny 2D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/5.png}}{{\tiny 2D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/6.png}}{{\tiny 2D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/7.png}}{{\tiny 2D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/8.png}}{{\tiny 2D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/9.png}}{{\tiny 2D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/10.png}}{{\tiny 2D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/11.png}}{{\tiny 2D-M11}}    
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/12.png}}{{\tiny 2D-M12}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/13.png}}{{\tiny 2D-M13}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/14.png}}{{\tiny 2D-M14}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/15.png}}{{\tiny 2D-M15}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/16.png}}{{\tiny 2D-M16}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/17.png}}{{\tiny 2D-M17}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/18.png}}{{\tiny 2D-M18}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/19.png}}{{\tiny 2D-M19}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/20.png}}{{\tiny 2D-M20}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/21.png}}{{\tiny 2D-M21}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/22.png}}{{\tiny 2D-M22}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/23.png}}{{\tiny 2D-M23}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/24.png}}{{\tiny 2D-M24}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/25.png}}{{\tiny 2D-M25}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/26.png}}{{\tiny 2D-M26}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/27.png}}{{\tiny 2D-M27}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/28.png}}{{\tiny 2D-M28}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/29.png}}{{\tiny 2D-M29}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/30.png}}{{\tiny 2D-M30}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/31.png}}{{\tiny 2D-M31}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/32.png}}{{\tiny 2D-M32}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/33.png}}{{\tiny 2D-M33}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/34.png}}{{\tiny 2D-M34}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/35.png}}{{\tiny 2D-M35}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/36.png}}{{\tiny 2D-M36}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/37.png}}{{\tiny 2D-M37}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/38.png}}{{\tiny 2D-M38}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/39.png}}{{\tiny 2D-M39}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/40.png}}{{\tiny 2D-M40}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/41.png}}{{\tiny 2D-M41}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/42.png}}{{\tiny 2D-M42}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/43.png}}{{\tiny 2D-M43}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/44.png}}{{\tiny 2D-M44}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/45.png}}{{\tiny 2D-M45}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/46.png}}{{\tiny 2D-M46}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/47.png}}{{\tiny 2D-M47}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/48.png}}{{\tiny 2D-M48}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/49.png}}{{\tiny 2D-M49}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/50.png}}{{\tiny 2D-M50}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/51.png}}{{\tiny 2D-M51}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/52.png}}{{\tiny 2D-M52}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/53.png}}{{\tiny 2D-M53}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/54.png}}{{\tiny 2D-M54}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/55.png}}{{\tiny 2D-M55}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/56.png}}{{\tiny 2D-M56}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/57.png}}{{\tiny 2D-M57}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/58.png}}{{\tiny 2D-M58}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/59.png}}{{\tiny 2D-M59}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/60.png}}{{\tiny 2D-M60}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/61.png}}{{\tiny 2D-M61}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/62.png}}{{\tiny 2D-M62}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/63.png}}{{\tiny 2D-M63}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/64.png}}{{\tiny 2D-M64}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/65.png}}{{\tiny 2D-M65}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/66.png}}{{\tiny 2D-M66}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/67.png}}{{\tiny 2D-M67}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/68.png}}{{\tiny 2D-M68}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/69.png}}{{\tiny 2D-M69}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/70.png}}{{\tiny 2D-M70}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/71.png}}{{\tiny 2D-M71}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/72.png}}{{\tiny 2D-M72}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/73.png}}{{\tiny 2D-M73}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/74.png}}{{\tiny 2D-M74}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/75.png}}{{\tiny 2D-M75}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/76.png}}{{\tiny 2D-M76}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/77.png}}{{\tiny 2D-M77}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/78.png}}{{\tiny 2D-M78}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/79.png}}{{\tiny 2D-M79}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/80.png}}{{\tiny 2D-M80}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/81.png}}{{\tiny 2D-M81}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/82.png}}{{\tiny 2D-M82}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/83.png}}{{\tiny 2D-M83}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/84.png}}{{\tiny 2D-M84}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/85.png}}{{\tiny 2D-M85}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/86.png}}{{\tiny 2D-M86}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/87.png}}{{\tiny 2D-M87}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/88.png}}{{\tiny 2D-M88}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/89.png}}{{\tiny 2D-M89}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/90.png}}{{\tiny 2D-M90}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/91.png}}{{\tiny 2D-M91}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/92.png}}{{\tiny 2D-M92}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/93.png}}{{\tiny 2D-M93}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/94.png}}{{\tiny 2D-M94}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/95.png}}{{\tiny 2D-M95}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/96.png}}{{\tiny 2D-M96}} 
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/97.png}}{{\tiny 2D-M97}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/98.png}}{{\tiny 2D-M98}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/99.png}}{{\tiny 2D-M99}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/100.png}}{{\tiny 2D-M100}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/101.png}}{{\tiny 2D-M101}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/102.png}}{{\tiny 2D-M102}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/103.png}}{{\tiny 2D-M103}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/104.png}}{{\tiny 2D-M104}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/105.png}}{{\tiny 2D-M105}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/106.png}}{{\tiny 2D-M106}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/107.png}}{{\tiny 2D-M107}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/108.png}}{{\tiny 2D-M108}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/109.png}}{{\tiny 2D-M109}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/110.png}}{{\tiny 2D-M110}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/111.png}}{{\tiny 2D-M111}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/112.png}}{{\tiny 2D-M112}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/113.png}}{{\tiny 2D-M113}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/114.png}}{{\tiny 2D-M114}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/115.png}}{{\tiny 2D-M115}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/116.png}}{{\tiny 2D-M116}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/117.png}}{{\tiny 2D-M117}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/118.png}}{{\tiny 2D-M118}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/119.png}}{{\tiny 2D-M119}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/120.png}}{{\tiny 2D-M120}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/121.png}}{{\tiny 2D-M121}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/122.png}}{{\tiny 2D-M122}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/123.png}}{{\tiny 2D-M123}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/124.png}}{{\tiny 2D-M124}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/125.png}}{{\tiny 2D-M125}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/126.png}}{{\tiny 2D-M126}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/127.png}}{{\tiny 2D-M127}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/128.png}}{{\tiny 2D-M128}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/129.png}}{{\tiny 2D-M129}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/130.png}}{{\tiny 2D-M130}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/131.png}}{{\tiny 2D-M131}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/132.png}}{{\tiny 2D-M132}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/133.png}}{{\tiny 2D-M133}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/134.png}}{{\tiny 2D-M134}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/135.png}}{{\tiny 2D-M135}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/136.png}}{{\tiny 2D-M136}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/137.png}}{{\tiny 2D-M137}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/138.png}}{{\tiny 2D-M138}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/139.png}}{{\tiny 2D-M139}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/140.png}}{{\tiny 2D-M140}}
\qquad  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/141.png}}{{\tiny 2D-M141}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/142.png}}{{\tiny 2D-M142}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/143.png}}{{\tiny 2D-M143}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/144.png}}{{\tiny 2D-M144}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/145.png}}{{\tiny 2D-M145}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/146.png}}{{\tiny 2D-M146}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/147.png}}{{\tiny 2D-M147}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/148.png}}{{\tiny 2D-M148}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/149.png}}{{\tiny 2D-M149}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/150.png}}{{\tiny 2D-M150}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/151.png}}{{\tiny 2D-M151}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/152.png}}{{\tiny 2D-M152}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/153.png}}{{\tiny 2D-M153}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/154.png}}{{\tiny 2D-M154}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/155.png}}{{\tiny 2D-M155}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/156.png}}{{\tiny 2D-M156}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/157.png}}{{\tiny 2D-M157}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/158.png}}{{\tiny 2D-M158}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/159.png}}{{\tiny 2D-M159}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/160.png}}{{\tiny 2D-M160}} 
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/161.png}}{{\tiny 2D-M161}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/162.png}}{{\tiny 2D-M162}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/163.png}}{{\tiny 2D-M163}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/164.png}}{{\tiny 2D-M164}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/165.png}}{{\tiny 2D-M165}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/166.png}}{{\tiny 2D-M166}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/167.png}}{{\tiny 2D-M167}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/168.png}}{{\tiny 2D-M168}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/169.png}}{{\tiny 2D-M169}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/170.png}}{{\tiny 2D-M170}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/171.png}}{{\tiny 2D-M171}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/172.png}}{{\tiny 2D-M172}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/173.png}}{{\tiny 2D-M173}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/174.png}}{{\tiny 2D-M174}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/175.png}}{{\tiny 2D-M175}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/176.png}}{{\tiny 2D-M176}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/177.png}}{{\tiny 2D-M177}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/178.png}}{{\tiny 2D-M178}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/179.png}}{{\tiny 2D-M179}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/180.png}}{{\tiny 2D-M180}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/181.png}}{{\tiny 2D-M181}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/182.png}}{{\tiny 2D-M182}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/183.png}}{{\tiny 2D-M183}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/184.png}}{{\tiny 2D-M184}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/185.png}}{{\tiny 2D-M185}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/186.png}}{{\tiny 2D-M186}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/187.png}}{{\tiny 2D-M187}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/188.png}}{{\tiny 2D-M188}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/189.png}}{{\tiny 2D-M189}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/190.png}}{{\tiny 2D-M190}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/191.png}}{{\tiny 2D-M191}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/192.png}}{{\tiny 2D-M192}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/193.png}}{{\tiny 2D-M193}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/194.png}}{{\tiny 2D-M194}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/195.png}}{{\tiny 2D-M195}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/196.png}}{{\tiny 2D-M196}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/197.png}}{{\tiny 2D-M197}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/198.png}}{{\tiny 2D-M198}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/199.png}}{{\tiny 2D-M199}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/200.png}}{{\tiny 2D-M200}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/201.png}}{{\tiny 2D-M201}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/202.png}}{{\tiny 2D-M202}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/203.png}}{{\tiny 2D-M203}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/204.png}}{{\tiny 2D-M204}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/205.png}}{{\tiny 2D-M205}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/206.png}}{{\tiny 2D-M206}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/207.png}}{{\tiny 2D-M207}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/208.png}}{{\tiny 2D-M208}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/209.png}}{{\tiny 2D-M209}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/210.png}}{{\tiny 2D-M210}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/211.png}}{{\tiny 2D-M211}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/212.png}}{{\tiny 2D-M212}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/213.png}}{{\tiny 2D-M213}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/214.png}}{{\tiny 2D-M214}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/215.png}}{{\tiny 2D-M215}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/216.png}}{{\tiny 2D-M216}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/217.png}}{{\tiny 2D-M217}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/218.png}}{{\tiny 2D-M218}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/219.png}}{{\tiny 2D-M219}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/220.png}}{{\tiny 2D-M220}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/221.png}}{{\tiny 2D-M221}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/222.png}}{{\tiny 2D-M222}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/223.png}}{{\tiny 2D-M223}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/224.png}}{{\tiny 2D-M224}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/225.png}}{{\tiny 2D-M225}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/226.png}}{{\tiny 2D-M226}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/227.png}}{{\tiny 2D-M227}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/228.png}}{{\tiny 2D-M228}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/229.png}}{{\tiny 2D-M229}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/230.png}}{{\tiny 2D-M230}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/231.png}}{{\tiny 2D-M231}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/232.png}}{{\tiny 2D-M232}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/233.png}}{{\tiny 2D-M233}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/234.png}}{{\tiny 2D-M234}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/235.png}}{{\tiny 2D-M235}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/236.png}}{{\tiny 2D-M236}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/237.png}}{{\tiny 2D-M237}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/238.png}}{{\tiny 2D-M238}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/239.png}}{{\tiny 2D-M239}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/240.png}}{{\tiny 2D-M240}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/241.png}}{{\tiny 2D-M241}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/242.png}}{{\tiny 2D-M242}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/243.png}}{{\tiny 2D-M243}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/244.png}}{{\tiny 2D-M244}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/245.png}}{{\tiny 2D-M245}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/246.png}}{{\tiny 2D-M246}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/247.png}}{{\tiny 2D-M247}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/248.png}}{{\tiny 2D-M248}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/249.png}}{{\tiny 2D-M249}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/250.png}}{{\tiny 2D-M250}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/251.png}}{{\tiny 2D-M251}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/252.png}}{{\tiny 2D-M252}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/253.png}}{{\tiny 2D-M253}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/254.png}}{{\tiny 2D-M254}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/255.png}}{{\tiny 2D-M255}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/256.png}}{{\tiny 2D-M256}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/257.png}}{{\tiny 2D-M257}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/258.png}}{{\tiny 2D-M258}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/259.png}}{{\tiny 2D-M259}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/260.png}}{{\tiny 2D-M260}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/261.png}}{{\tiny 2D-M261}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/262.png}}{{\tiny 2D-M262}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/263.png}}{{\tiny 2D-M263}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/264.png}}{{\tiny 2D-M264}}


  \end{minipage}
\end{subfigure}
\caption{Schematic diagrams of 2-DOF Manipulators}
\end{figure}





  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/265.png}}{{\tiny 2D-M265}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/266.png}}{{\tiny 2D-M266}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/267.png}}{{\tiny 2D-M267}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/268.png}}{{\tiny 2D-M268}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/269.png}}{{\tiny 2D-M269}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/270.png}}{{\tiny 2D-M270}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/271.png}}{{\tiny 2D-M271}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/272.png}}{{\tiny 2D-M272}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/273.png}}{{\tiny 2D-M273}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/274.png}}{{\tiny 2D-M274}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/275.png}}{{\tiny 2D-M275}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/276.png}}{{\tiny 2D-M276}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/277.png}}{{\tiny 2D-M277}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/278.png}}{{\tiny 2D-M278}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/279.png}}{{\tiny 2D-M279}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/280.png}}{{\tiny 2D-M280}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/281.png}}{{\tiny 2D-M281}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/282.png}}{{\tiny 2D-M282}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/283.png}}{{\tiny 2D-M283}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/284.png}}{{\tiny 2D-M284}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/285.png}}{{\tiny 2D-M285}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/286.png}}{{\tiny 2D-M286}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/287.png}}{{\tiny 2D-M287}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/288.png}}{{\tiny 2D-M288}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/289.png}}{{\tiny 2D-M289}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/290.png}}{{\tiny 2D-M290}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/291.png}}{{\tiny 2D-M291}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/292.png}}{{\tiny 2D-M292}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/293.png}}{{\tiny 2D-M293}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/294.png}}{{\tiny 2D-M294}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/295.png}}{{\tiny 2D-M295}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/296.png}}{{\tiny 2D-M296}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/297.png}}{{\tiny 2D-M297}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/298.png}}{{\tiny 2D-M298}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/299.png}}{{\tiny 2D-M299}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/300.png}}{{\tiny 2D-M300}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/301.png}}{{\tiny 2D-M301}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/302.png}}{{\tiny 2D-M302}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/303.png}}{{\tiny 2D-M303}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/304.png}}{{\tiny 2D-M304}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/305.png}}{{\tiny 2D-M305}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/306.png}}{{\tiny 2D-M306}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/307.png}}{{\tiny 2D-M307}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/308.png}}{{\tiny 2D-M308}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/309.png}}{{\tiny 2D-M309}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/310.png}}{{\tiny 2D-M310}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/311.png}}{{\tiny 2D-M311}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/312.png}}{{\tiny 2D-M312}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/313.png}}{{\tiny 2D-M313}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/314.png}}{{\tiny 2D-M314}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/315.png}}{{\tiny 2D-M315}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/316.png}}{{\tiny 2D-M316}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/317.png}}{{\tiny 2D-M317}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/318.png}}{{\tiny 2D-M318}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/319.png}}{{\tiny 2D-M319}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/320.png}}{{\tiny 2D-M320}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/321.png}}{{\tiny 2D-M321}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/322.png}}{{\tiny 2D-M322}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/323.png}}{{\tiny 2D-M323}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/324.png}}{{\tiny 2D-M324}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/325.png}}{{\tiny 2D-M325}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/326.png}}{{\tiny 2D-M326}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/327.png}}{{\tiny 2D-M327}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/328.png}}{{\tiny 2D-M328}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/329.png}}{{\tiny 2D-M329}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/330.png}}{{\tiny 2D-M330}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/331.png}}{{\tiny 2D-M331}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/332.png}}{{\tiny 2D-M332}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/333.png}}{{\tiny 2D-M333}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/334.png}}{{\tiny 2D-M334}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/335.png}}{{\tiny 2D-M335}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/336.png}}{{\tiny 2D-M336}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/337.png}}{{\tiny 2D-M337}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/338.png}}{{\tiny 2D-M338}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/339.png}}{{\tiny 2D-M339}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/340.png}}{{\tiny 2D-M340}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/341.png}}{{\tiny 2D-M341}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/342.png}}{{\tiny 2D-M342}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/343.png}}{{\tiny 2D-M343}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/344.png}}{{\tiny 2D-M344}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/345.png}}{{\tiny 2D-M345}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/346.png}}{{\tiny 2D-M346}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/347.png}}{{\tiny 2D-M347}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/348.png}}{{\tiny 2D-M348}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/349.png}}{{\tiny 2D-M349}}
\qquad  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/350.png}}{{\tiny 2D-M350}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/351.png}}{{\tiny 2D-M351}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/352.png}}{{\tiny 2D-M352}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/353.png}}{{\tiny 2D-M353}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/354.png}}{{\tiny 2D-M354}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/355.png}}{{\tiny 2D-M355}}  
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/356.png}}{{\tiny 2D-M356}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/357.png}}{{\tiny 2D-M357}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/358.png}}{{\tiny 2D-M358}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/359.png}}{{\tiny 2D-M359}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/360.png}}{{\tiny 2D-M360}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/361.png}}{{\tiny 2D-M361}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/362.png}}{{\tiny 2D-M362}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/363.png}}{{\tiny 2D-M363}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/364.png}}{{\tiny 2D-M364}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/365.png}}{{\tiny 2D-M365}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/366.png}}{{\tiny 2D-M366}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/367.png}}{{\tiny 2D-M367}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/368.png}}{{\tiny 2D-M368}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/369.png}}{{\tiny 2D-M369}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/370.png}}{{\tiny 2D-M370}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/371.png}}{{\tiny 2D-M371}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/372.png}}{{\tiny 2D-M372}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/373.png}}{{\tiny 2D-M373}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/374.png}}{{\tiny 2D-M374}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/375.png}}{{\tiny 2D-M375}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/376.png}}{{\tiny 2D-M376}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/377.png}}{{\tiny 2D-M377}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/378.png}}{{\tiny 2D-M378}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/379.png}}{{\tiny 2D-M379}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/380.png}}{{\tiny 2D-M380}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/381.png}}{{\tiny 2D-M381}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/382.png}}{{\tiny 2D-M382}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/383.png}}{{\tiny 2D-M383}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/384.png}}{{\tiny 2D-M384}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/385.png}}{{\tiny 2D-M385}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/386.png}}{{\tiny 2D-M386}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/387.png}}{{\tiny 2D-M387}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/388.png}}{{\tiny 2D-M388}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/389.png}}{{\tiny 2D-M389}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/390.png}}{{\tiny 2D-M390}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/391.png}}{{\tiny 2D-M391}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/392.png}}{{\tiny 2D-M392}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/393.png}}{{\tiny 2D-M393}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/394.png}}{{\tiny 2D-M394}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/395.png}}{{\tiny 2D-M395}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/396.png}}{{\tiny 2D-M396}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/397.png}}{{\tiny 2D-M397}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/398.png}}{{\tiny 2D-M398}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/399.png}}{{\tiny 2D-M399}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/400.png}}{{\tiny 2D-M400}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/401.png}}{{\tiny 2D-M401}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/402.png}}{{\tiny 2D-M402}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/403.png}}{{\tiny 2D-M403}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/404.png}}{{\tiny 2D-M404}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/405.png}}{{\tiny 2D-M405}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/406.png}}{{\tiny 2D-M406}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/407.png}}{{\tiny 2D-M407}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/408.png}}{{\tiny 2D-M408}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/409.png}}{{\tiny 2D-M409}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/410.png}}{{\tiny 2D-M410}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/411.png}}{{\tiny 2D-M411}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/412.png}}{{\tiny 2D-M412}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/413.png}}{{\tiny 2D-M413}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/414.png}}{{\tiny 2D-M414}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/415.png}}{{\tiny 2D-M415}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/416.png}}{{\tiny 2D-M416}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/417.png}}{{\tiny 2D-M417}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/418.png}}{{\tiny 2D-M418}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/419.png}}{{\tiny 2D-M419}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/420.png}}{{\tiny 2D-M420}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/421.png}}{{\tiny 2D-M421}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/422.png}}{{\tiny 2D-M422}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/423.png}}{{\tiny 2D-M423}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/424.png}}{{\tiny 2D-M424}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/425.png}}{{\tiny 2D-M425}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/426.png}}{{\tiny 2D-M426}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/427.png}}{{\tiny 2D-M427}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/428.png}}{{\tiny 2D-M428}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/429.png}}{{\tiny 2D-M429}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/430.png}}{{\tiny 2D-M430}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/431.png}}{{\tiny 2D-M431}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/432.png}}{{\tiny 2D-M432}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/433.png}}{{\tiny 2D-M433}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/434.png}}{{\tiny 2D-M434}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/435.png}}{{\tiny 2D-M435}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/436.png}}{{\tiny 2D-M436}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/437.png}}{{\tiny 2D-M437}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/438.png}}{{\tiny 2D-M438}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/439.png}}{{\tiny 2D-M439}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/440.png}}{{\tiny 2D-M440}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/441.png}}{{\tiny 2D-M441}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/442.png}}{{\tiny 2D-M442}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/443.png}}{{\tiny 2D-M443}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/444.png}}{{\tiny 2D-M444}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/445.png}}{{\tiny 2D-M445}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/446.png}}{{\tiny 2D-M446}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/447.png}}{{\tiny 2D-M447}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/448.png}}{{\tiny 2D-M448}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/449.png}}{{\tiny 2D-M449}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/450.png}}{{\tiny 2D-M450}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/451.png}}{{\tiny 2D-M451}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/452.png}}{{\tiny 2D-M452}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/453.png}}{{\tiny 2D-M453}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/454.png}}{{\tiny 2D-M454}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/455.png}}{{\tiny 2D-M455}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/456.png}}{{\tiny 2D-M456}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/457.png}}{{\tiny 2D-M457}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/458.png}}{{\tiny 2D-M458}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/459.png}}{{\tiny 2D-M459}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/460.png}}{{\tiny 2D-M460}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/461.png}}{{\tiny 2D-M461}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/462.png}}{{\tiny 2D-M462}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/463.png}}{{\tiny 2D-M463}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/464.png}}{{\tiny 2D-M464}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/465.png}}{{\tiny 2D-M465}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/466.png}}{{\tiny 2D-M466}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/467.png}}{{\tiny 2D-M467}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/468.png}}{{\tiny 2D-M468}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/469.png}}{{\tiny 2D-M469}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/470.png}}{{\tiny 2D-M470}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/471.png}}{{\tiny 2D-M471}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/472.png}}{{\tiny 2D-M472}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/473.png}}{{\tiny 2D-M473}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/474.png}}{{\tiny 2D-M474}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/475.png}}{{\tiny 2D-M475}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/476.png}}{{\tiny 2D-M476}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/477.png}}{{\tiny 2D-M477}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/478.png}}{{\tiny 2D-M478}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/479.png}}{{\tiny 2D-M479}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/480.png}}{{\tiny 2D-M480}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/481.png}}{{\tiny 2D-M481}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/482.png}}{{\tiny 2D-M482}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/483.png}}{{\tiny 2D-M483}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/484.png}}{{\tiny 2D-M484}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/485.png}}{{\tiny 2D-M485}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/486.png}}{{\tiny 2D-M486}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/487.png}}{{\tiny 2D-M487}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/488.png}}{{\tiny 2D-M488}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/489.png}}{{\tiny 2D-M489}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/490.png}}{{\tiny 2D-M490}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/491.png}}{{\tiny 2D-M491}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/492.png}}{{\tiny 2D-M492}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/493.png}}{{\tiny 2D-M493}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/494.png}}{{\tiny 2D-M494}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/495.png}}{{\tiny 2D-M495}}  
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/496.png}}{{\tiny 2D-M496}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/497.png}}{{\tiny 2D-M497}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/498.png}}{{\tiny 2D-M498}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/499.png}}{{\tiny 2D-M499}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/500.png}}{{\tiny 2D-M500}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/501.png}}{{\tiny 2D-M501}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/502.png}}{{\tiny 2D-M502}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/503.png}}{{\tiny 2D-M503}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/504.png}}{{\tiny 2D-M504}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/505.png}}{{\tiny 2D-M505}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/506.png}}{{\tiny 2D-M506}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/507.png}}{{\tiny 2D-M507}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/508.png}}{{\tiny 2D-M508}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/509.png}}{{\tiny 2D-M509}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/510.png}}{{\tiny 2D-M510}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/511.png}}{{\tiny 2D-M511}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/512.png}}{{\tiny 2D-M512}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/513.png}}{{\tiny 2D-M513}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/514.png}}{{\tiny 2D-M514}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/515.png}}{{\tiny 2D-M515}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/516.png}}{{\tiny 2D-M516}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/517.png}}{{\tiny 2D-M517}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/518.png}}{{\tiny 2D-M518}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/519.png}}{{\tiny 2D-M519}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/520.png}}{{\tiny 2D-M520}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/521.png}}{{\tiny 2D-M521}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/522.png}}{{\tiny 2D-M522}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/523.png}}{{\tiny 2D-M523}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/524.png}}{{\tiny 2D-M524}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/525.png}}{{\tiny 2D-M525}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/526.png}}{{\tiny 2D-M526}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/527.png}}{{\tiny 2D-M527}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/528.png}}{{\tiny 2D-M528}}

      \end{minipage}
    \end{subfigure}
    \caption{Schematic diagrams of 2-DOF Manipulators (Contd.)}
    \end{figure}










\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering


\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/529.png}}{{\tiny 2D-M529}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/530.png}}{{\tiny 2D-M530}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/531.png}}{{\tiny 2D-M531}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/532.png}}{{\tiny 2D-M532}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/533.png}}{{\tiny 2D-M533}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/534.png}}{{\tiny 2D-M534}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/535.png}}{{\tiny 2D-M535}}
\qquad  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/536.png}}{{\tiny 2D-M536}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/537.png}}{{\tiny 2D-M537}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/538.png}}{{\tiny 2D-M538}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/539.png}}{{\tiny 2D-M539}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/540.png}}{{\tiny 2D-M540}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/541.png}}{{\tiny 2D-M541}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/542.png}}{{\tiny 2D-M542}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/543.png}}{{\tiny 2D-M543}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/544.png}}{{\tiny 2D-M544}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/545.png}}{{\tiny 2D-M545}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/546.png}}{{\tiny 2D-M546}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/547.png}}{{\tiny 2D-M547}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/548.png}}{{\tiny 2D-M548}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/549.png}}{{\tiny 2D-M549}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/550.png}}{{\tiny 2D-M550}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/551.png}}{{\tiny 2D-M551}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/552.png}}{{\tiny 2D-M552}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/553.png}}{{\tiny 2D-M553}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/554.png}}{{\tiny 2D-M554}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/555.png}}{{\tiny 2D-M555}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/556.png}}{{\tiny 2D-M556}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/557.png}}{{\tiny 2D-M557}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/558.png}}{{\tiny 2D-M558}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/559.png}}{{\tiny 2D-M559}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/560.png}}{{\tiny 2D-M560}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/561.png}}{{\tiny 2D-M561}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/562.png}}{{\tiny 2D-M562}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/563.png}}{{\tiny 2D-M563}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/564.png}}{{\tiny 2D-M564}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/565.png}}{{\tiny 2D-M565}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/566.png}}{{\tiny 2D-M566}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/567.png}}{{\tiny 2D-M567}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/568.png}}{{\tiny 2D-M568}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/569.png}}{{\tiny 2D-M569}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/570.png}}{{\tiny 2D-M570}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/571.png}}{{\tiny 2D-M571}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/572.png}}{{\tiny 2D-M572}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/573.png}}{{\tiny 2D-M573}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/574.png}}{{\tiny 2D-M574}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/575.png}}{{\tiny 2D-M575}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/576.png}}{{\tiny 2D-M576}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/577.png}}{{\tiny 2D-M577}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/578.png}}{{\tiny 2D-M578}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/579.png}}{{\tiny 2D-M579}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/580.png}}{{\tiny 2D-M580}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/581.png}}{{\tiny 2D-M581}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/582.png}}{{\tiny 2D-M582}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/583.png}}{{\tiny 2D-M583}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/584.png}}{{\tiny 2D-M584}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/585.png}}{{\tiny 2D-M585}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/586.png}}{{\tiny 2D-M586}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/587.png}}{{\tiny 2D-M587}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/588.png}}{{\tiny 2D-M588}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/589.png}}{{\tiny 2D-M589}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/590.png}}{{\tiny 2D-M590}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/591.png}}{{\tiny 2D-M591}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/592.png}}{{\tiny 2D-M592}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/593.png}}{{\tiny 2D-M593}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/594.png}}{{\tiny 2D-M594}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/595.png}}{{\tiny 2D-M595}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/596.png}}{{\tiny 2D-M596}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/597.png}}{{\tiny 2D-M597}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/598.png}}{{\tiny 2D-M598}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/599.png}}{{\tiny 2D-M599}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/600.png}}{{\tiny 2D-M600}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/601.png}}{{\tiny 2D-M601}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/602.png}}{{\tiny 2D-M602}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/603.png}}{{\tiny 2D-M603}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/604.png}}{{\tiny 2D-M604}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/605.png}}{{\tiny 2D-M605}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/606.png}}{{\tiny 2D-M606}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/607.png}}{{\tiny 2D-M607}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/608.png}}{{\tiny 2D-M608}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/609.png}}{{\tiny 2D-M609}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/610.png}}{{\tiny 2D-M610}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/611.png}}{{\tiny 2D-M611}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/612.png}}{{\tiny 2D-M612}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/613.png}}{{\tiny 2D-M613}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/614.png}}{{\tiny 2D-M614}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/615.png}}{{\tiny 2D-M615}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/616.png}}{{\tiny 2D-M616}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/617.png}}{{\tiny 2D-M617}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/618.png}}{{\tiny 2D-M618}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/619.png}}{{\tiny 2D-M619}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/620.png}}{{\tiny 2D-M620}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/621.png}}{{\tiny 2D-M621}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/622.png}}{{\tiny 2D-M622}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/623.png}}{{\tiny 2D-M623}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/624.png}}{{\tiny 2D-M624}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/625.png}}{{\tiny 2D-M625}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/626.png}}{{\tiny 2D-M626}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/627.png}}{{\tiny 2D-M627}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/628.png}}{{\tiny 2D-M628}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/629.png}}{{\tiny 2D-M629}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/630.png}}{{\tiny 2D-M630}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/631.png}}{{\tiny 2D-M631}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/632.png}}{{\tiny 2D-M632}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/633.png}}{{\tiny 2D-M633}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/634.png}}{{\tiny 2D-M634}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/635.png}}{{\tiny 2D-M635}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/636.png}}{{\tiny 2D-M636}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/637.png}}{{\tiny 2D-M637}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/638.png}}{{\tiny 2D-M638}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/639.png}}{{\tiny 2D-M639}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/640.png}}{{\tiny 2D-M640}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/641.png}}{{\tiny 2D-M641}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/642.png}}{{\tiny 2D-M642}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/643.png}}{{\tiny 2D-M643}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/644.png}}{{\tiny 2D-M644}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/645.png}}{{\tiny 2D-M645}}

  
    \end{minipage}
  \end{subfigure}
  \caption{Schematic diagrams of 2-DOF Manipulators (Contd.)}
  \end{figure}


==> classes/2dof_classes_old.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/1.png}}{{\tiny 2D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/2.png}}{{\tiny 2D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/3.png}}{{\tiny 2D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/4.png}}{{\tiny 2D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/5.png}}{{\tiny 2D-M5}}

  \end{minipage}
\end{subfigure}
\caption{Class 1 of 2-DOF Manipulators}
\end{figure}


\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/6.png}}{{\tiny 2D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/7.png}}{{\tiny 2D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/8.png}}{{\tiny 2D-M8}}


  \end{minipage}
\end{subfigure}
\caption{Class 2 of 2-DOF Manipulators}
\end{figure}



\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/9.png}}{{\tiny 2D-M9}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/10.png}}{{\tiny 2D-M10}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/11.png}}{{\tiny 2D-M11}}    
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/12.png}}{{\tiny 2D-M12}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/13.png}}{{\tiny 2D-M13}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/14.png}}{{\tiny 2D-M14}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/15.png}}{{\tiny 2D-M15}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/16.png}}{{\tiny 2D-M16}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/17.png}}{{\tiny 2D-M17}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/18.png}}{{\tiny 2D-M18}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/19.png}}{{\tiny 2D-M19}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/20.png}}{{\tiny 2D-M20}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 2 of 2-DOF Manipulators (Contd.)}
  \end{figure}


  \begin{figure}[H]
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/21.png}}{{\tiny 2D-M21}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/22.png}}{{\tiny 2D-M22}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/23.png}}{{\tiny 2D-M23}}
    
      \end{minipage}
    \end{subfigure}
    \caption{Class 3 of 2-DOF Manipulators}
    \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/24.png}}{{\tiny 2D-M24}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/25.png}}{{\tiny 2D-M25}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/26.png}}{{\tiny 2D-M26}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/27.png}}{{\tiny 2D-M27}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/28.png}}{{\tiny 2D-M28}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/29.png}}{{\tiny 2D-M29}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/30.png}}{{\tiny 2D-M30}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/31.png}}{{\tiny 2D-M31}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/32.png}}{{\tiny 2D-M32}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/33.png}}{{\tiny 2D-M33}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/34.png}}{{\tiny 2D-M34}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/35.png}}{{\tiny 2D-M35}}

  \end{minipage}
\end{subfigure}
\caption{Class 3 of 2-DOF Manipulators (Contd.)}
\end{figure}



\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/36.png}}{{\tiny 2D-M36}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/37.png}}{{\tiny 2D-M37}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/38.png}}{{\tiny 2D-M38}}
  \end{minipage}
\end{subfigure}
\caption{Class 4 of 2-DOF Manipulators}
\end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/39.png}}{{\tiny 2D-M39}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/40.png}}{{\tiny 2D-M40}}
    \end{minipage}
  \end{subfigure}
  \caption{Class 4 of 2-DOF Manipulators (Contd.)}
  \end{figure}

% \begin{figure}[H]\ContinuedFloat
%   \centering
%   \begin{subfigure}{\columnwidth}
%     \begin{minipage}{\textwidth}\footnotesize
%     \centering
  
  
%     \end{minipage}
%   \end{subfigure}
%   \caption{Class 4 of 2-DOF Manipulators (Contd.)}
%   \end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/41.png}}{{\tiny 2D-M41}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/42.png}}{{\tiny 2D-M42}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/43.png}}{{\tiny 2D-M43}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/44.png}}{{\tiny 2D-M44}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/45.png}}{{\tiny 2D-M45}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/46.png}}{{\tiny 2D-M46}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/47.png}}{{\tiny 2D-M47}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/48.png}}{{\tiny 2D-M48}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/49.png}}{{\tiny 2D-M49}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/50.png}}{{\tiny 2D-M50}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/51.png}}{{\tiny 2D-M51}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/52.png}}{{\tiny 2D-M52}}



  \end{minipage}
\end{subfigure}
\caption{Class 5 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/53.png}}{{\tiny 2D-M53}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/54.png}}{{\tiny 2D-M54}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/55.png}}{{\tiny 2D-M55}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/56.png}}{{\tiny 2D-M56}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/57.png}}{{\tiny 2D-M57}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/58.png}}{{\tiny 2D-M58}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/59.png}}{{\tiny 2D-M59}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/60.png}}{{\tiny 2D-M60}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/61.png}}{{\tiny 2D-M61}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/62.png}}{{\tiny 2D-M62}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/63.png}}{{\tiny 2D-M63}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/64.png}}{{\tiny 2D-M64}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/65.png}}{{\tiny 2D-M65}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/66.png}}{{\tiny 2D-M66}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/67.png}}{{\tiny 2D-M67}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/68.png}}{{\tiny 2D-M68}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/69.png}}{{\tiny 2D-M69}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/70.png}}{{\tiny 2D-M70}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/71.png}}{{\tiny 2D-M71}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/72.png}}{{\tiny 2D-M72}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/73.png}}{{\tiny 2D-M73}}

  
    \end{minipage}
  \end{subfigure}
  \caption{Class 5 of 2-DOF Manipulators (Contd.)}
  \end{figure}


  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
    
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/74.png}}{{\tiny 2D-M74}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/75.png}}{{\tiny 2D-M75}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/76.png}}{{\tiny 2D-M76}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/77.png}}{{\tiny 2D-M77}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/78.png}}{{\tiny 2D-M78}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/79.png}}{{\tiny 2D-M79}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/80.png}}{{\tiny 2D-M80}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/81.png}}{{\tiny 2D-M81}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/82.png}}{{\tiny 2D-M82}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/83.png}}{{\tiny 2D-M83}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/84.png}}{{\tiny 2D-M84}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/85.png}}{{\tiny 2D-M85}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/86.png}}{{\tiny 2D-M86}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/87.png}}{{\tiny 2D-M87}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/88.png}}{{\tiny 2D-M88}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/89.png}}{{\tiny 2D-M89}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/90.png}}{{\tiny 2D-M90}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/91.png}}{{\tiny 2D-M91}}
   
      \end{minipage}
    \end{subfigure}
    \caption{Class 5 of 2-DOF Manipulators (Contd.)}
    \end{figure}



  \begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/92.png}}{{\tiny 2D-M92}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/93.png}}{{\tiny 2D-M93}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/94.png}}{{\tiny 2D-M94}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/95.png}}{{\tiny 2D-M95}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/96.png}}{{\tiny 2D-M96}} 
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/97.png}}{{\tiny 2D-M97}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/98.png}}{{\tiny 2D-M98}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/99.png}}{{\tiny 2D-M99}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/100.png}}{{\tiny 2D-M100}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/101.png}}{{\tiny 2D-M101}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/102.png}}{{\tiny 2D-M102}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/103.png}}{{\tiny 2D-M103}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/104.png}}{{\tiny 2D-M104}}

  \end{minipage}
\end{subfigure}
\caption{Class 5 of 2-DOF Manipulators (Contd.)}
\end{figure}


\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/105.png}}{{\tiny 2D-M105}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/106.png}}{{\tiny 2D-M106}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/107.png}}{{\tiny 2D-M107}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/108.png}}{{\tiny 2D-M108}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/109.png}}{{\tiny 2D-M109}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/110.png}}{{\tiny 2D-M110}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/111.png}}{{\tiny 2D-M111}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/112.png}}{{\tiny 2D-M112}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/113.png}}{{\tiny 2D-M113}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/114.png}}{{\tiny 2D-M114}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/115.png}}{{\tiny 2D-M115}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/116.png}}{{\tiny 2D-M116}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/117.png}}{{\tiny 2D-M117}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/118.png}}{{\tiny 2D-M118}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/119.png}}{{\tiny 2D-M119}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/120.png}}{{\tiny 2D-M120}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/121.png}}{{\tiny 2D-M121}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/122.png}}{{\tiny 2D-M122}}





  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/123.png}}{{\tiny 2D-M123}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/124.png}}{{\tiny 2D-M124}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/125.png}}{{\tiny 2D-M125}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/126.png}}{{\tiny 2D-M126}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/127.png}}{{\tiny 2D-M127}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/128.png}}{{\tiny 2D-M128}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/129.png}}{{\tiny 2D-M129}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/130.png}}{{\tiny 2D-M130}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/131.png}}{{\tiny 2D-M131}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/132.png}}{{\tiny 2D-M132}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/133.png}}{{\tiny 2D-M133}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/134.png}}{{\tiny 2D-M134}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/135.png}}{{\tiny 2D-M135}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/136.png}}{{\tiny 2D-M136}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/137.png}}{{\tiny 2D-M137}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/138.png}}{{\tiny 2D-M138}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/139.png}}{{\tiny 2D-M139}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/140.png}}{{\tiny 2D-M140}}
 
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 2-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/141.png}}{{\tiny 2D-M141}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/142.png}}{{\tiny 2D-M142}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/143.png}}{{\tiny 2D-M143}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/144.png}}{{\tiny 2D-M144}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/145.png}}{{\tiny 2D-M145}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/146.png}}{{\tiny 2D-M146}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/147.png}}{{\tiny 2D-M147}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/148.png}}{{\tiny 2D-M148}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/149.png}}{{\tiny 2D-M149}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/150.png}}{{\tiny 2D-M150}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/151.png}}{{\tiny 2D-M151}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/152.png}}{{\tiny 2D-M152}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/153.png}}{{\tiny 2D-M153}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/154.png}}{{\tiny 2D-M154}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/155.png}}{{\tiny 2D-M155}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/156.png}}{{\tiny 2D-M156}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/157.png}}{{\tiny 2D-M157}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/158.png}}{{\tiny 2D-M158}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/159.png}}{{\tiny 2D-M159}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/160.png}}{{\tiny 2D-M160}} 
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/161.png}}{{\tiny 2D-M161}}



  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Contd.)}
\end{figure}\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/162.png}}{{\tiny 2D-M162}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/163.png}}{{\tiny 2D-M163}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/164.png}}{{\tiny 2D-M164}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/165.png}}{{\tiny 2D-M165}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/166.png}}{{\tiny 2D-M166}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/167.png}}{{\tiny 2D-M167}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/168.png}}{{\tiny 2D-M168}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/169.png}}{{\tiny 2D-M169}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/170.png}}{{\tiny 2D-M170}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/171.png}}{{\tiny 2D-M171}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/172.png}}{{\tiny 2D-M172}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/173.png}}{{\tiny 2D-M173}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/174.png}}{{\tiny 2D-M174}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/175.png}}{{\tiny 2D-M175}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/176.png}}{{\tiny 2D-M176}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/177.png}}{{\tiny 2D-M177}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/178.png}}{{\tiny 2D-M178}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/179.png}}{{\tiny 2D-M179}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/180.png}}{{\tiny 2D-M180}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/181.png}}{{\tiny 2D-M181}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/182.png}}{{\tiny 2D-M182}}



  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Contd.)}
\end{figure}


\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/183.png}}{{\tiny 2D-M183}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/184.png}}{{\tiny 2D-M184}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/185.png}}{{\tiny 2D-M185}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/186.png}}{{\tiny 2D-M186}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/187.png}}{{\tiny 2D-M187}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/188.png}}{{\tiny 2D-M188}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/189.png}}{{\tiny 2D-M189}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/190.png}}{{\tiny 2D-M190}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/191.png}}{{\tiny 2D-M191}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/192.png}}{{\tiny 2D-M192}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/193.png}}{{\tiny 2D-M193}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/194.png}}{{\tiny 2D-M194}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/195.png}}{{\tiny 2D-M195}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/196.png}}{{\tiny 2D-M196}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/197.png}}{{\tiny 2D-M197}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/198.png}}{{\tiny 2D-M198}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/199.png}}{{\tiny 2D-M199}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/200.png}}{{\tiny 2D-M200}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/201.png}}{{\tiny 2D-M201}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/202.png}}{{\tiny 2D-M202}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/203.png}}{{\tiny 2D-M203}}



  \end{minipage}
\end{subfigure}
\caption{Class 6 of 2-DOF Manipulators (Contd.)}
\end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/204.png}}{{\tiny 2D-M204}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/205.png}}{{\tiny 2D-M205}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/206.png}}{{\tiny 2D-M206}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/207.png}}{{\tiny 2D-M207}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/208.png}}{{\tiny 2D-M208}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/209.png}}{{\tiny 2D-M209}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/210.png}}{{\tiny 2D-M210}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/211.png}}{{\tiny 2D-M211}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/212.png}}{{\tiny 2D-M212}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/213.png}}{{\tiny 2D-M213}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/214.png}}{{\tiny 2D-M214}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/215.png}}{{\tiny 2D-M215}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/216.png}}{{\tiny 2D-M216}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/217.png}}{{\tiny 2D-M217}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/218.png}}{{\tiny 2D-M218}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/219.png}}{{\tiny 2D-M219}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/220.png}}{{\tiny 2D-M220}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/221.png}}{{\tiny 2D-M221}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/222.png}}{{\tiny 2D-M222}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/223.png}}{{\tiny 2D-M223}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/224.png}}{{\tiny 2D-M224}}


  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 2-DOF Manipulators (Contd.)}
  \end{figure}


  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
    
  
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/225.png}}{{\tiny 2D-M225}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/226.png}}{{\tiny 2D-M226}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/227.png}}{{\tiny 2D-M227}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/228.png}}{{\tiny 2D-M228}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/229.png}}{{\tiny 2D-M229}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/230.png}}{{\tiny 2D-M230}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/231.png}}{{\tiny 2D-M231}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/232.png}}{{\tiny 2D-M232}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/233.png}}{{\tiny 2D-M233}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/234.png}}{{\tiny 2D-M234}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/235.png}}{{\tiny 2D-M235}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/236.png}}{{\tiny 2D-M236}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/237.png}}{{\tiny 2D-M237}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/238.png}}{{\tiny 2D-M238}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/239.png}}{{\tiny 2D-M239}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/240.png}}{{\tiny 2D-M240}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/241.png}}{{\tiny 2D-M241}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/242.png}}{{\tiny 2D-M242}}

    
      \end{minipage}
    \end{subfigure}
    \caption{Class 6 of 2-DOF Manipulators (Contd.)}
    \end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/243.png}}{{\tiny 2D-M243}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/244.png}}{{\tiny 2D-M244}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/245.png}}{{\tiny 2D-M245}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/246.png}}{{\tiny 2D-M246}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/247.png}}{{\tiny 2D-M247}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/248.png}}{{\tiny 2D-M248}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/249.png}}{{\tiny 2D-M249}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/250.png}}{{\tiny 2D-M250}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/251.png}}{{\tiny 2D-M251}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/252.png}}{{\tiny 2D-M252}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/253.png}}{{\tiny 2D-M253}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/254.png}}{{\tiny 2D-M254}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/255.png}}{{\tiny 2D-M255}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/256.png}}{{\tiny 2D-M256}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/257.png}}{{\tiny 2D-M257}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/258.png}}{{\tiny 2D-M258}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/259.png}}{{\tiny 2D-M259}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/260.png}}{{\tiny 2D-M260}}



  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 2-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/261.png}}{{\tiny 2D-M261}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/262.png}}{{\tiny 2D-M262}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/263.png}}{{\tiny 2D-M263}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/264.png}}{{\tiny 2D-M264}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/265.png}}{{\tiny 2D-M265}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/266.png}}{{\tiny 2D-M266}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/267.png}}{{\tiny 2D-M267}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/268.png}}{{\tiny 2D-M268}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/269.png}}{{\tiny 2D-M269}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/270.png}}{{\tiny 2D-M270}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/271.png}}{{\tiny 2D-M271}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/272.png}}{{\tiny 2D-M272}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/273.png}}{{\tiny 2D-M273}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/274.png}}{{\tiny 2D-M274}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/275.png}}{{\tiny 2D-M275}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/276.png}}{{\tiny 2D-M276}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/277.png}}{{\tiny 2D-M277}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/278.png}}{{\tiny 2D-M278}}



  
    \end{minipage}
  \end{subfigure}
  \caption{Class 6 of 2-DOF Manipulators (Contd.)}
  \end{figure}


  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/279.png}}{{\tiny 2D-M279}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/280.png}}{{\tiny 2D-M280}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/281.png}}{{\tiny 2D-M281}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/282.png}}{{\tiny 2D-M282}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/283.png}}{{\tiny 2D-M283}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/284.png}}{{\tiny 2D-M284}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/285.png}}{{\tiny 2D-M285}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/286.png}}{{\tiny 2D-M286}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/287.png}}{{\tiny 2D-M287}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/288.png}}{{\tiny 2D-M288}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/289.png}}{{\tiny 2D-M289}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/290.png}}{{\tiny 2D-M290}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/291.png}}{{\tiny 2D-M291}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/292.png}}{{\tiny 2D-M292}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/293.png}}{{\tiny 2D-M293}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/294.png}}{{\tiny 2D-M294}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/295.png}}{{\tiny 2D-M295}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/296.png}}{{\tiny 2D-M296}}
    
      \end{minipage}
    \end{subfigure}
    \caption{Class 6 of 2-DOF Manipulators (Contd.)}
    \end{figure}



\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/297.png}}{{\tiny 2D-M297}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/298.png}}{{\tiny 2D-M298}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/299.png}}{{\tiny 2D-M299}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/300.png}}{{\tiny 2D-M300}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/301.png}}{{\tiny 2D-M301}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/302.png}}{{\tiny 2D-M302}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/303.png}}{{\tiny 2D-M303}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/304.png}}{{\tiny 2D-M304}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/305.png}}{{\tiny 2D-M305}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/306.png}}{{\tiny 2D-M306}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/307.png}}{{\tiny 2D-M307}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/308.png}}{{\tiny 2D-M308}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/309.png}}{{\tiny 2D-M309}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/310.png}}{{\tiny 2D-M310}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/311.png}}{{\tiny 2D-M311}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/312.png}}{{\tiny 2D-M312}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/313.png}}{{\tiny 2D-M313}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/314.png}}{{\tiny 2D-M314}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/315.png}}{{\tiny 2D-M315}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/316.png}}{{\tiny 2D-M316}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/317.png}}{{\tiny 2D-M317}}

  \end{minipage}
\end{subfigure}
\caption{Class 7 of 2-DOF Manipulators}
\end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/318.png}}{{\tiny 2D-M318}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/319.png}}{{\tiny 2D-M319}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 7 of 2-DOF Manipulators (Contd.)}
  \end{figure}


\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/320.png}}{{\tiny 2D-M320}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/321.png}}{{\tiny 2D-M321}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/322.png}}{{\tiny 2D-M322}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/323.png}}{{\tiny 2D-M323}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/324.png}}{{\tiny 2D-M324}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/325.png}}{{\tiny 2D-M325}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/326.png}}{{\tiny 2D-M326}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/327.png}}{{\tiny 2D-M327}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/328.png}}{{\tiny 2D-M328}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/329.png}}{{\tiny 2D-M329}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/330.png}}{{\tiny 2D-M330}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/331.png}}{{\tiny 2D-M331}}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators}
\end{figure}



\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering

  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/332.png}}{{\tiny 2D-M332}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/333.png}}{{\tiny 2D-M333}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/334.png}}{{\tiny 2D-M334}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/335.png}}{{\tiny 2D-M335}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/336.png}}{{\tiny 2D-M336}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/337.png}}{{\tiny 2D-M337}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/338.png}}{{\tiny 2D-M338}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/339.png}}{{\tiny 2D-M339}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/340.png}}{{\tiny 2D-M340}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/341.png}}{{\tiny 2D-M341}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/342.png}}{{\tiny 2D-M342}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/343.png}}{{\tiny 2D-M343}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/344.png}}{{\tiny 2D-M344}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/345.png}}{{\tiny 2D-M345}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/346.png}}{{\tiny 2D-M346}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/347.png}}{{\tiny 2D-M347}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/348.png}}{{\tiny 2D-M348}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/349.png}}{{\tiny 2D-M349}}

    \end{minipage}
  \end{subfigure}
  \caption{Class 8 of 2-DOF Manipulators (Contd.)}
  \end{figure}


\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/350.png}}{{\tiny 2D-M350}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/351.png}}{{\tiny 2D-M351}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/352.png}}{{\tiny 2D-M352}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/353.png}}{{\tiny 2D-M353}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/354.png}}{{\tiny 2D-M354}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/355.png}}{{\tiny 2D-M355}}  
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/356.png}}{{\tiny 2D-M356}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/357.png}}{{\tiny 2D-M357}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/358.png}}{{\tiny 2D-M358}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/359.png}}{{\tiny 2D-M359}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/360.png}}{{\tiny 2D-M360}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/361.png}}{{\tiny 2D-M361}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/362.png}}{{\tiny 2D-M362}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/363.png}}{{\tiny 2D-M363}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/364.png}}{{\tiny 2D-M364}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/365.png}}{{\tiny 2D-M365}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/366.png}}{{\tiny 2D-M366}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/367.png}}{{\tiny 2D-M367}}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Contd.)}
\end{figure}


\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/368.png}}{{\tiny 2D-M368}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/369.png}}{{\tiny 2D-M369}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/370.png}}{{\tiny 2D-M370}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/371.png}}{{\tiny 2D-M371}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/372.png}}{{\tiny 2D-M372}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/373.png}}{{\tiny 2D-M373}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/374.png}}{{\tiny 2D-M374}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/375.png}}{{\tiny 2D-M375}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/376.png}}{{\tiny 2D-M376}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/377.png}}{{\tiny 2D-M377}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/378.png}}{{\tiny 2D-M378}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/379.png}}{{\tiny 2D-M379}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/380.png}}{{\tiny 2D-M380}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/381.png}}{{\tiny 2D-M381}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/382.png}}{{\tiny 2D-M382}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/383.png}}{{\tiny 2D-M383}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/384.png}}{{\tiny 2D-M384}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/385.png}}{{\tiny 2D-M385}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/386.png}}{{\tiny 2D-M386}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/387.png}}{{\tiny 2D-M387}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/388.png}}{{\tiny 2D-M388}}



  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Contd.)}
\end{figure}



  

  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/389.png}}{{\tiny 2D-M389}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/390.png}}{{\tiny 2D-M390}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/391.png}}{{\tiny 2D-M391}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/392.png}}{{\tiny 2D-M392}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/393.png}}{{\tiny 2D-M393}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/394.png}}{{\tiny 2D-M394}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/395.png}}{{\tiny 2D-M395}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/396.png}}{{\tiny 2D-M396}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/397.png}}{{\tiny 2D-M397}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/398.png}}{{\tiny 2D-M398}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/399.png}}{{\tiny 2D-M399}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/400.png}}{{\tiny 2D-M400}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/401.png}}{{\tiny 2D-M401}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/402.png}}{{\tiny 2D-M402}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/403.png}}{{\tiny 2D-M403}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/404.png}}{{\tiny 2D-M404}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/405.png}}{{\tiny 2D-M405}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/406.png}}{{\tiny 2D-M406}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/407.png}}{{\tiny 2D-M407}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/408.png}}{{\tiny 2D-M408}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/409.png}}{{\tiny 2D-M409}}

    
      \end{minipage}
    \end{subfigure}
    \caption{Class 8 of 2-DOF Manipulators (Contd.)}
    \end{figure}

    \begin{figure}[H]\ContinuedFloat
      \centering
      \begin{subfigure}{\columnwidth}
        \begin{minipage}{\textwidth}\footnotesize
        \centering
        \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/410.png}}{{\tiny 2D-M410}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/411.png}}{{\tiny 2D-M411}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/412.png}}{{\tiny 2D-M412}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/413.png}}{{\tiny 2D-M413}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/414.png}}{{\tiny 2D-M414}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/415.png}}{{\tiny 2D-M415}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/416.png}}{{\tiny 2D-M416}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/417.png}}{{\tiny 2D-M417}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/418.png}}{{\tiny 2D-M418}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/419.png}}{{\tiny 2D-M419}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/420.png}}{{\tiny 2D-M420}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/421.png}}{{\tiny 2D-M421}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/422.png}}{{\tiny 2D-M422}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/423.png}}{{\tiny 2D-M423}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/424.png}}{{\tiny 2D-M424}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/425.png}}{{\tiny 2D-M425}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/426.png}}{{\tiny 2D-M426}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/427.png}}{{\tiny 2D-M427}}


    \end{minipage}
      \end{subfigure}
      \caption{Class 8 of 2-DOF Manipulators (Contd.)}
      \end{figure}


\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/428.png}}{{\tiny 2D-M428}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/429.png}}{{\tiny 2D-M429}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/430.png}}{{\tiny 2D-M430}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/431.png}}{{\tiny 2D-M431}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/432.png}}{{\tiny 2D-M432}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/433.png}}{{\tiny 2D-M433}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/434.png}}{{\tiny 2D-M434}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/435.png}}{{\tiny 2D-M435}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/436.png}}{{\tiny 2D-M436}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/437.png}}{{\tiny 2D-M437}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/438.png}}{{\tiny 2D-M438}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/439.png}}{{\tiny 2D-M439}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/440.png}}{{\tiny 2D-M440}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/441.png}}{{\tiny 2D-M441}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/442.png}}{{\tiny 2D-M442}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/443.png}}{{\tiny 2D-M443}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/444.png}}{{\tiny 2D-M444}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/445.png}}{{\tiny 2D-M445}}


 
    \end{minipage}
  \end{subfigure}
  \caption{Class 8 of 2-DOF Manipulators (Contd.)}
  \end{figure}

  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
      \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/446.png}}{{\tiny 2D-M446}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/447.png}}{{\tiny 2D-M447}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/448.png}}{{\tiny 2D-M448}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/449.png}}{{\tiny 2D-M449}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/450.png}}{{\tiny 2D-M450}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/451.png}}{{\tiny 2D-M451}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/452.png}}{{\tiny 2D-M452}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/453.png}}{{\tiny 2D-M453}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/454.png}}{{\tiny 2D-M454}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/455.png}}{{\tiny 2D-M455}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/456.png}}{{\tiny 2D-M456}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/457.png}}{{\tiny 2D-M457}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/458.png}}{{\tiny 2D-M458}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/459.png}}{{\tiny 2D-M459}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/460.png}}{{\tiny 2D-M460}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/461.png}}{{\tiny 2D-M461}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/462.png}}{{\tiny 2D-M462}}
      \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/463.png}}{{\tiny 2D-M463}}




   
      \end{minipage}
    \end{subfigure}
    \caption{Class 8 of 2-DOF Manipulators (Contd.)}
    \end{figure}
  
    \begin{figure}[H]\ContinuedFloat
      \centering
      \begin{subfigure}{\columnwidth}
        \begin{minipage}{\textwidth}\footnotesize
        \centering
        \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/464.png}}{{\tiny 2D-M464}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/465.png}}{{\tiny 2D-M465}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/466.png}}{{\tiny 2D-M466}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/467.png}}{{\tiny 2D-M467}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/468.png}}{{\tiny 2D-M468}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/469.png}}{{\tiny 2D-M469}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/470.png}}{{\tiny 2D-M470}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/471.png}}{{\tiny 2D-M471}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/472.png}}{{\tiny 2D-M472}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/473.png}}{{\tiny 2D-M473}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/474.png}}{{\tiny 2D-M474}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/475.png}}{{\tiny 2D-M475}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/476.png}}{{\tiny 2D-M476}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/477.png}}{{\tiny 2D-M477}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/478.png}}{{\tiny 2D-M478}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/479.png}}{{\tiny 2D-M479}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/480.png}}{{\tiny 2D-M480}}
        \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/481.png}}{{\tiny 2D-M481}}



      
     
        \end{minipage}
      \end{subfigure}
      \caption{Class 8 of 2-DOF Manipulators (Contd.)}
      \end{figure}

      \begin{figure}[H]\ContinuedFloat
        \centering
        \begin{subfigure}{\columnwidth}
          \begin{minipage}{\textwidth}\footnotesize
          \centering
          \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/482.png}}{{\tiny 2D-M482}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/483.png}}{{\tiny 2D-M483}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/484.png}}{{\tiny 2D-M484}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/485.png}}{{\tiny 2D-M485}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/486.png}}{{\tiny 2D-M486}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/487.png}}{{\tiny 2D-M487}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/488.png}}{{\tiny 2D-M488}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/489.png}}{{\tiny 2D-M489}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/490.png}}{{\tiny 2D-M490}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/491.png}}{{\tiny 2D-M491}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/492.png}}{{\tiny 2D-M492}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/493.png}}{{\tiny 2D-M493}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/494.png}}{{\tiny 2D-M494}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/495.png}}{{\tiny 2D-M495}}  
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/496.png}}{{\tiny 2D-M496}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/497.png}}{{\tiny 2D-M497}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/498.png}}{{\tiny 2D-M498}}
          \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/499.png}}{{\tiny 2D-M499}}


          \end{minipage}
        \end{subfigure}
        \caption{Class 8 of 2-DOF Manipulators (Contd.)}
        \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering


  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/500.png}}{{\tiny 2D-M500}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/501.png}}{{\tiny 2D-M501}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/502.png}}{{\tiny 2D-M502}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/503.png}}{{\tiny 2D-M503}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/504.png}}{{\tiny 2D-M504}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/505.png}}{{\tiny 2D-M505}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/506.png}}{{\tiny 2D-M506}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/507.png}}{{\tiny 2D-M507}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/508.png}}{{\tiny 2D-M508}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/509.png}}{{\tiny 2D-M509}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/510.png}}{{\tiny 2D-M510}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/511.png}}{{\tiny 2D-M511}}

  \end{minipage}
\end{subfigure}
\caption{Class 8 of 2-DOF Manipulators (Contd.)}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/512.png}}{{\tiny 2D-M512}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/513.png}}{{\tiny 2D-M513}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/514.png}}{{\tiny 2D-M514}}

  
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 9 of 2-DOF Manipulators}
  \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/515.png}}{{\tiny 2D-M515}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/516.png}}{{\tiny 2D-M516}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/517.png}}{{\tiny 2D-M517}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/518.png}}{{\tiny 2D-M518}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/519.png}}{{\tiny 2D-M519}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/520.png}}{{\tiny 2D-M520}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/521.png}}{{\tiny 2D-M521}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/522.png}}{{\tiny 2D-M522}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/523.png}}{{\tiny 2D-M523}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/524.png}}{{\tiny 2D-M524}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/525.png}}{{\tiny 2D-M525}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/526.png}}{{\tiny 2D-M526}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/527.png}}{{\tiny 2D-M527}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/528.png}}{{\tiny 2D-M528}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/529.png}}{{\tiny 2D-M529}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/530.png}}{{\tiny 2D-M530}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/531.png}}{{\tiny 2D-M531}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/532.png}}{{\tiny 2D-M532}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/533.png}}{{\tiny 2D-M533}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/534.png}}{{\tiny 2D-M534}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/535.png}}{{\tiny 2D-M535}}

  \end{minipage}
\end{subfigure}
\caption{Class 9 of 2-DOF Manipulators (Contd.)}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering


  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/536.png}}{{\tiny 2D-M536}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/537.png}}{{\tiny 2D-M537}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/538.png}}{{\tiny 2D-M538}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/539.png}}{{\tiny 2D-M539}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/540.png}}{{\tiny 2D-M540}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/541.png}}{{\tiny 2D-M541}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/542.png}}{{\tiny 2D-M542}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/543.png}}{{\tiny 2D-M543}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/544.png}}{{\tiny 2D-M544}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/545.png}}{{\tiny 2D-M545}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/546.png}}{{\tiny 2D-M546}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/547.png}}{{\tiny 2D-M547}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/548.png}}{{\tiny 2D-M548}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/549.png}}{{\tiny 2D-M549}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/550.png}}{{\tiny 2D-M550}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/551.png}}{{\tiny 2D-M551}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/552.png}}{{\tiny 2D-M552}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/553.png}}{{\tiny 2D-M553}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/554.png}}{{\tiny 2D-M554}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/555.png}}{{\tiny 2D-M555}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/556.png}}{{\tiny 2D-M556}}

  
    \end{minipage}
  \end{subfigure}
  \caption{Class 9 of 2-DOF Manipulators (Contd.)}
  \end{figure}

  \begin{figure}[H]\ContinuedFloat
    \centering
    \begin{subfigure}{\columnwidth}
      \begin{minipage}{\textwidth}\footnotesize
      \centering
  
  
 \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/557.png}}{{\tiny 2D-M557}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/558.png}}{{\tiny 2D-M558}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/559.png}}{{\tiny 2D-M559}}
    
      \end{minipage}
    \end{subfigure}
    \caption{Class 9 of 2-DOF Manipulators (Contd.)}
    \end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/560.png}}{{\tiny 2D-M560}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/561.png}}{{\tiny 2D-M561}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/562.png}}{{\tiny 2D-M562}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/563.png}}{{\tiny 2D-M563}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/564.png}}{{\tiny 2D-M564}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/565.png}}{{\tiny 2D-M565}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/566.png}}{{\tiny 2D-M566}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/567.png}}{{\tiny 2D-M567}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/568.png}}{{\tiny 2D-M568}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/569.png}}{{\tiny 2D-M569}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/570.png}}{{\tiny 2D-M570}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/571.png}}{{\tiny 2D-M571}}




  \end{minipage}
\end{subfigure}
\caption{Class 10 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  


    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/572.png}}{{\tiny 2D-M572}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/573.png}}{{\tiny 2D-M573}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/574.png}}{{\tiny 2D-M574}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/575.png}}{{\tiny 2D-M575}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/576.png}}{{\tiny 2D-M576}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/577.png}}{{\tiny 2D-M577}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/578.png}}{{\tiny 2D-M578}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/579.png}}{{\tiny 2D-M579}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/580.png}}{{\tiny 2D-M580}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/581.png}}{{\tiny 2D-M581}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/582.png}}{{\tiny 2D-M582}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/583.png}}{{\tiny 2D-M583}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/584.png}}{{\tiny 2D-M584}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/585.png}}{{\tiny 2D-M585}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/586.png}}{{\tiny 2D-M586}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/587.png}}{{\tiny 2D-M587}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/588.png}}{{\tiny 2D-M588}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/589.png}}{{\tiny 2D-M589}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/590.png}}{{\tiny 2D-M590}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/591.png}}{{\tiny 2D-M591}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/592.png}}{{\tiny 2D-M592}}
    

    \end{minipage}
  \end{subfigure}
  \caption{Class 10 of 2-DOF Manipulators (Contd.)}
  \end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/593.png}}{{\tiny 2D-M593}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/594.png}}{{\tiny 2D-M594}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/595.png}}{{\tiny 2D-M595}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/596.png}}{{\tiny 2D-M596}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/597.png}}{{\tiny 2D-M597}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/598.png}}{{\tiny 2D-M598}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/599.png}}{{\tiny 2D-M599}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/600.png}}{{\tiny 2D-M600}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/601.png}}{{\tiny 2D-M601}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/602.png}}{{\tiny 2D-M602}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/603.png}}{{\tiny 2D-M603}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/604.png}}{{\tiny 2D-M604}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/605.png}}{{\tiny 2D-M605}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/606.png}}{{\tiny 2D-M606}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/607.png}}{{\tiny 2D-M607}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/608.png}}{{\tiny 2D-M608}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/609.png}}{{\tiny 2D-M609}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/610.png}}{{\tiny 2D-M610}}


  \end{minipage}
\end{subfigure}
\caption{Class 10 of 2-DOF Manipulators (Contd.)}
\end{figure}

\begin{figure}[H]\ContinuedFloat
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  
    \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/611.png}}{{\tiny 2D-M611}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/612.png}}{{\tiny 2D-M612}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/613.png}}{{\tiny 2D-M613}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/614.png}}{{\tiny 2D-M614}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/615.png}}{{\tiny 2D-M615}}
    \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/616.png}}{{\tiny 2D-M616}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/617.png}}{{\tiny 2D-M617}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/618.png}}{{\tiny 2D-M618}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/619.png}}{{\tiny 2D-M619}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/620.png}}{{\tiny 2D-M620}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/621.png}}{{\tiny 2D-M621}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/622.png}}{{\tiny 2D-M622}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/623.png}}{{\tiny 2D-M623}}
    \end{minipage}
  \end{subfigure}
  \caption{Class 10 of 2-DOF Manipulators (Contd.)}
  \end{figure}


\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering

\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/624.png}}{{\tiny 2D-M624}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/625.png}}{{\tiny 2D-M625}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/626.png}}{{\tiny 2D-M626}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/627.png}}{{\tiny 2D-M627}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/628.png}}{{\tiny 2D-M628}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/629.png}}{{\tiny 2D-M629}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/630.png}}{{\tiny 2D-M630}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/631.png}}{{\tiny 2D-M631}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/632.png}}{{\tiny 2D-M632}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/633.png}}{{\tiny 2D-M633}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/634.png}}{{\tiny 2D-M634}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/635.png}}{{\tiny 2D-M635}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/636.png}}{{\tiny 2D-M636}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/637.png}}{{\tiny 2D-M637}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/638.png}}{{\tiny 2D-M638}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/639.png}}{{\tiny 2D-M639}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/640.png}}{{\tiny 2D-M640}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/641.png}}{{\tiny 2D-M641}}

  \end{minipage}
\end{subfigure}
\caption{Class 11 of 2-DOF Manipulators}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/642.png}}{{\tiny 2D-M642}}

    \end{minipage}
  \end{subfigure}
  \caption{Class 12 of 2-DOF Manipulators}
  \end{figure}\begin{figure}[H]
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/643.png}}{{\tiny 2D-M643}}
  \qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/644.png}}{{\tiny 2D-M644}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 13 of 2-DOF Manipulators}
  \end{figure}\begin{figure}[H]
  \centering
  \begin{subfigure}{\columnwidth}
    \begin{minipage}{\textwidth}\footnotesize
    \centering
  \subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/2dof/645.png}}{{\tiny 2D-M645}}
  
    \end{minipage}
  \end{subfigure}
  \caption{Class 14 of 2-DOF Manipulators}
  \end{figure}

==> classes/3dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/1.png}}{{\tiny 3D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/2.png}}{{\tiny 3D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/3.png}}{{\tiny 3D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/4.png}}{{\tiny 3D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/5.png}}{{\tiny 3D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/6.png}}{{\tiny 3D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/7.png}}{{\tiny 3D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/8.png}}{{\tiny 3D-M8}}

  \end{minipage}
\end{subfigure}
\caption{Schematic diagrams of 3-DOF Manipulators}
\end{figure}



==> classes/3dof_classes_old.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/1.png}}{{\tiny 3D-M1}}

  \end{minipage}
\end{subfigure}
\caption{Class 1 of 3-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/2.png}}{{\tiny 3D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/3.png}}{{\tiny 3D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/4.png}}{{\tiny 3D-M4}}

  \end{minipage}
\end{subfigure}
\caption{Class 2 of 3-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/5.png}}{{\tiny 3D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/6.png}}{{\tiny 3D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/7.png}}{{\tiny 3D-M7}}

  \end{minipage}
\end{subfigure}
\caption{Class 3 of 3-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/3dof/8.png}}{{\tiny 3D-M8}}

  \end{minipage}
\end{subfigure}
\caption{Class 4 of 3-DOF Manipulators}
\end{figure}

==> classes/4dof_classes.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/1.png}}{{\tiny 4D-M1}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/2.png}}{{\tiny 4D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/3.png}}{{\tiny 4D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/4.png}}{{\tiny 4D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/5.png}}{{\tiny 4D-M5}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/6.png}}{{\tiny 4D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/7.png}}{{\tiny 4D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/8.png}}{{\tiny 4D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/9.png}}{{\tiny 4D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/10.png}}{{\tiny 4D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/11.png}}{{\tiny 4D-M11}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/12.png}}{{\tiny 4D-M12}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/13.png}}{{\tiny 4D-M13}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/14.png}}{{\tiny 4D-M14}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/15.png}}{{\tiny 4D-M15}}

  \end{minipage}
\end{subfigure}
\caption{Schematic diagrams of 4-DOF Manipulators}
\end{figure}

==> classes/4dof_classes_old.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/1.png}}{{\tiny 4D-M1}}

  \end{minipage}
\end{subfigure}
\caption{Class 1 of 4-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/2.png}}{{\tiny 4D-M2}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/3.png}}{{\tiny 4D-M3}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/4.png}}{{\tiny 4D-M4}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/5.png}}{{\tiny 4D-M5}}

  \end{minipage}
\end{subfigure}
\caption{Class 2 of 4-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/6.png}}{{\tiny 4D-M6}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/7.png}}{{\tiny 4D-M7}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/8.png}}{{\tiny 4D-M8}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/9.png}}{{\tiny 4D-M9}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/10.png}}{{\tiny 4D-M10}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/11.png}}{{\tiny 4D-M11}}

  \end{minipage}
\end{subfigure}
\caption{Class 3 of 4-DOF Manipulators}
\end{figure}\begin{figure}[H]
\centering
\begin{subfigure}{\columnwidth}
  \begin{minipage}{\textwidth}\footnotesize
  \centering
\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/12.png}}{{\tiny 4D-M12}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/13.png}}{{\tiny 4D-M13}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/14.png}}{{\tiny 4D-M14}}
\qquad\subsubfloat{\includegraphics[width=0.05\textwidth]{contentfolder/images/4dof/15.png}}{{\tiny 4D-M15}}

  \end{minipage}
\end{subfigure}
\caption{Class 4 of 4-DOF Manipulators}
\end{figure}

==> contentfolder/mechanisms2/manipulabilitytable1.tex <==

\begin{center}

\tablefirsthead{%

\hline
%\multicolumn{1}{|c}{\tbsp S.No.} &
\multicolumn{1}{|c|}{\tbsp S.No.} &
%\tbsp S.No. &
%\multicolumn{1}{c}{Name} &
Name &
$\bar{\mu}$ &
%\multicolumn{1}{c}{$\mu$} &
$\mu$ &
\multicolumn{1}{c|}{$f$} \\
\hline}
\tablehead{%
\hline
%\multicolumn{5}{|l|}{\small\sl continued from previous page}\\
\multicolumn{5}{|l|}{\small\sl continuing...}\\
\hline
\multicolumn{1}{|c|}{\tbsp S.No.} &
Name &
$\bar{\mu}$ &
$\mu$ &
\multicolumn{1}{c|}{$f$} \\
\hline}
\tabletail{%
\hline
%\multicolumn{5}{|r|}{\small\sl continued on next page}\\
\multicolumn{5}{|r|}{\small\sl ...continued}\\
\hline}
\tablelasttail{\hline}
\label{Tab:table_dof1mt_1}
%\customlabel{Tab:table_dof1mt_1}{2}
\bottomcaption{Prescription of 1-DOF Manipulators}



%\tablehead{S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\}

%\begin{supertabular}{||c|c|c|c|c||}
\begin{supertabular}{|r|r|r|r|r|}
%\begin{longtable}{||c|c|c|c|c||}
%\hline
%S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\ 
\hline
1 & 1D-M10 & 0.1523 & 8.1 & $f_1$ \\
\hline2 & 1D-M65 & 0.1376 & 10.5 & $f_2$ \\
\hline3 & 1D-M8 & 0.1152 & 7.1 & $f_1$ \\
\hline4 & 1D-M94 & 0.1106 & 1.0 & $f_2$ \\
\hline5 & 1D-M28 & 0.1088 & 8.1 & $f_1$ \\
\hline6 & 1D-M20 & 0.0824 & 10.5 & $f_1$ \\
\hline7 & 1D-M34 & 0.0798 & 7.1 & $f_1$ \\
\hline8 & 1D-M95 & 0.0776 & 1.0 & $f_2$ \\
\hline9 & 1D-M7 & 0.0774 & 8.4 & $f_1$ \\
\hline10 & 1D-M29 & 0.0732 & 10.5 & $f_1$ \\
\hline11 & 1D-M41 & 0.0722 & 9.5 & $f_1$ \\
\hline12 & 1D-M40 & 0.071 & 7.1 & $f_1$ \\
\hline13 & 1D-M35 & 0.0706 & 10.5 & $f_1$ \\
\hline14 & 1D-M11 & 0.062 & 10.5 & $f_1$ \\
\hline15 & 1D-M64 & 0.0563 & 20.3 & $f_2$ \\
\hline16 & 1D-M66 & 0.0487 & 19.8 & $f_2$ \\
\hline17 & 1D-M60 & 0.0475 & 8.4 & $f_1$ \\
\hline18 & 1D-M93 & 0.0467 & 1.0 & $f_2$ \\
\hline19 & 1D-M59 & 0.0462 & 9.5 & $f_1$ \\
\hline20 & 1D-M91 & 0.0438 & 1.0 & $f_2$ \\
\hline21 & 1D-M79 & 0.0335 & 1 & $f_1$ \\
\hline22 & 1D-M25 & 0.0313 & 17.3 & $f_2$ \\
\hline23 & 1D-M44 & 0.0313 & 17.3 & $f_2$ \\
\hline24 & 1D-M67 & 0.0306 & 18.3 & $f_2$ \\
\hline25 & 1D-M15 & 0.0305 & 21.2 & $f_2$ \\
\hline26 & 1D-M22 & 0.0246 & 17.3 & $f_2$ \\
\hline27 & 1D-M13 & 0.024 & 15.3 & $f_2$ \\
\hline28 & 1D-M46 & 0.0237 & 15.3 & $f_2$ \\
\hline29 & 1D-M45 & 0.0229 & 17.3 & $f_2$ \\
\hline30 & 1D-M3 & 0.0222 & 15.4 & $f_2$ \\
\hline31 & 1D-M49 & 0.0219 & 14.1 & $f_2$ \\
\hline32 & 1D-M68 & 0.0214 & 19.6 & $f_2$ \\
\hline33 & 1D-M5 & 0.0212 & 14.7 & $f_2$ \\
\hline34 & 1D-M47 & 0.0212 & 17.3 & $f_2$ \\
\hline35 & 1D-M24 & 0.0212 & 17.3 & $f_2$ \\
\hline36 & 1D-M51 & 0.0203 & 14.9 & $f_2$ \\
\hline37 & 1D-M18 & 0.0194 & 14.6 & $f_2$ \\
\hline38 & 1D-M69 & 0.019 & 19.0 & $f_2$ \\
\hline39 & 1D-M48 & 0.0189 & 14.0 & $f_2$ \\
\hline40 & 1D-M12 & 0.0188 & 12.8 & $f_2$ \\
\hline41 & 1D-M9 & 0.0185 & 12.8 & $f_2$ \\
\hline42 & 1D-M23 & 0.0177 & 13.0 & $f_2$ \\
\hline43 & 1D-M62 & 0.0167 & 9.6 & $f_2$ \\
\hline44 & 1D-M26 & 0.0167 & 9.6 & $f_2$ \\
\hline45 & 1D-M14 & 0.0163 & 10.1 & $f_2$ \\
\hline46 & 1D-M96 & 0.016 & 1.0 & $f_2$ \\
\hline47 & 1D-M6 & 0.0159 & 12.0 & $f_2$ \\
\hline48 & 1D-M4 & 0.0158 & 13.4 & $f_2$ \\
\hline49 & 1D-M89 & 0.0155 & 1 & $f_1$ \\
\hline50 & 1D-M38 & 0.0153 & 12.9 & $f_2$ \\
\hline51 & 1D-M58 & 0.0148 & 8.2 & $f_2$ \\
\hline52 & 1D-M57 & 0.0143 & 11.7 & $f_2$ \\
\hline53 & 1D-M76 & 0.0138 & 1 & $f_1$ \\
\hline54 & 1D-M17 & 0.0136 & 8.6 & $f_2$ \\
\hline55 & 1D-M50 & 0.0135 & 11.1 & $f_2$ \\
\hline56 & 1D-M19 & 0.0134 & 10.3 & $f_2$ \\
\hline57 & 1D-M56 & 0.0129 & 10.5 & $f_2$ \\
\hline58 & 1D-M21 & 0.0128 & 10.5 & $f_2$ \\
\hline59 & 1D-M27 & 0.0127 & 9.3 & $f_2$ \\
\hline60 & 1D-M77 & 0.0126 & 1 & $f_1$ \\
\hline61 & 1D-M16 & 0.0125 & 9.3 & $f_2$ \\
\hline62 & 1D-M2 & 0.0116 & 6.7 & $f_2$ \\
\hline63 & 1D-M1 & 0.0113 & 8.4 & $f_2$ \\
\hline64 & 1D-M43 & 0.0108 & 1 & $f_1$ \\
\hline65 & 1D-M39 & 0.01 & 8.5 & $f_2$ \\
\hline66 & 1D-M80 & 0.0082 & 1 & $f_1$ \\
\hline67 & 1D-M36 & 0.0081 & 1 & $f_1$ \\
\hline68 & 1D-M92 & 0.0071 & 1 & $f_1$ \\
\hline69 & 1D-M61 & 0.0051 & 1 & $f_1$ \\
\hline70 & 1D-M42 & 0.0034 & 1 & $f_1$ \\
\hline71 & 1D-M31 & 0.0031 & 1.7 & $f_2$ \\
\hline72 & 1D-M37 & 0.0025 & 1 & $f_1$ \\
\hline73 & 1D-M86 & 0.0021 & 1.0 & $f_2$ \\
\hline74 & 1D-M30 & 0.002 & 1.1 & $f_2$ \\
\hline75 & 1D-M53 & 0.0017 & 1.1 & $f_2$ \\
\hline76 & 1D-M83 & 0.0016 & 1.0 & $f_2$ \\
\hline77 & 1D-M84 & 0.0015 & 1.0 & $f_2$ \\
\hline78 & 1D-M87 & 0.0015 & 1.0 & $f_2$ \\
\hline79 & 1D-M55 & 0.0015 & 1.3 & $f_2$ \\
\hline80 & 1D-M71 & 0.0015 & 1.0 & $f_2$ \\
\hline81 & 1D-M73 & 0.0015 & 1.0 & $f_2$ \\
\hline82 & 1D-M90 & 0.0015 & 1.0 & $f_2$ \\
\hline83 & 1D-M52 & 0.0015 & 1.1 & $f_2$ \\
\hline84 & 1D-M82 & 0.0014 & 1.0 & $f_2$ \\
\hline85 & 1D-M72 & 0.0014 & 1 & $f_2$ \\
\hline86 & 1D-M70 & 0.0014 & 1.0 & $f_2$ \\
\hline87 & 1D-M81 & 0.0014 & 1 & $f_2$ \\
\hline88 & 1D-M85 & 0.0014 & 1.0 & $f_2$ \\
\hline89 & 1D-M88 & 0.0014 & 1.0 & $f_2$ \\
\hline90 & 1D-M63 & 0.0013 & 1.1 & $f_2$ \\
\hline91 & 1D-M32 & 0.0013 & 0.7 & $f_2$ \\
\hline92 & 1D-M54 & 0.0013 & 1.1 & $f_2$ \\
\hline93 & 1D-M33 & 0.0012 & 0.8 & $f_2$ \\
\hline94 & 1D-M78 & 0.0009 & 0.6 & $f_2$ \\
\hline95 & 1D-M74 & 0.0008 & 0.6 & $f_2$ \\
\hline96 & 1D-M75 & 0.0006 & 0.4 & $f_2$ \\
\hline
%\caption{Manipulability of 1-DOF Manipulators}
%\label{Tab:table_dof1mt_1}

\end{supertabular}
\end{center}

%\end{longtable}



==> contentfolder/mechanisms2/manipulabilitytable2.tex <==
\tiny
\begin{center}
%\label{Tab:table_dof2mt_1}
\tablefirsthead{%
\hline
%\multicolumn{1}{|c}{\tbsp S.No.} &
\multicolumn{1}{|c|}{\tbsp S.No.} &
%\tbsp S.No. &
%\multicolumn{1}{c}{Name} &
Name &
$\bar{\mu}$ &
$\kappa$ &
$i_{\kappa}$ &
%\multicolumn{1}{c}{$\mu$} &
$\mu$ &
\multicolumn{1}{c|}{$f$} \\
\hline}
\tablehead{%
\hline
%\multicolumn{5}{|l|}{\small\sl continued from previous page}\\
\multicolumn{7}{|l|}{\small\sl continuing...}\\
\hline
\multicolumn{1}{|c|}{\tbsp S.No.} &
Name &
$\bar{\mu}$ &
$\kappa$ &
$i_{\kappa}$ &
$\mu$ &
\multicolumn{1}{c|}{$f$} \\
\hline}
\tabletail{%
\hline
%\multicolumn{5}{|r|}{\small\sl continued on next page}\\
\multicolumn{7}{|r|}{\small\sl ...continued}\\
\hline}
\tablelasttail{\hline}
\bottomcaption{Prescription of 2-DOF Manipulators}



%\tablehead{S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\}

%\begin{supertabular}{||c|c|c|c|c||}
\begin{supertabular}{|r|r|r|r|r|r|r|}
%\begin{longtable}{||c|c|c|c|c||}
%\hline
%S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\ 
\hline

1 & 2D-M645 & 1.0 & 1.0 & 6 & 1.0 & $f_1$ \\
\hline2 & 2D-M315 & 0.7544 & 1.2 & 155 & 87.4 & $f_1$ \\
\hline3 & 2D-M301 & 0.7058 & 1.2 & 158 & 88.8 & $f_2$ \\
\hline4 & 2D-M224 & 0.6366 & 1.1 & 127 & 60.2 & $f_1$ \\
\hline5 & 2D-M308 & 0.6034 & 1.1 & 118 & 340.6 & $f_2$ \\
\hline6 & 2D-M126 & 0.5855 & 1.3 & 207 & 88.8 & $f_1$ \\
\hline7 & 2D-M309 & 0.5624 & 1.2 & 135 & 351.6 & $f_2$ \\
\hline8 & 2D-M319 & 0.5621 & 1.4 & 230 & 283.4 & $f_2$ \\
\hline9 & 2D-M208 & 0.5495 & 1.2 & 172 & 68.1 & $f_1$ \\
\hline10 & 2D-M134 & 0.541 & 1.1 & 107 & 100.5 & $f_1$ \\
\hline11 & 2D-M248 & 0.5381 & 1.4 & 224 & 75.2 & $f_1$ \\
\hline12 & 2D-M203 & 0.5289 & 1.3 & 198 & 68.1 & $f_1$ \\
\hline13 & 2D-M634 & 0.5142 & 1.0 & 7 & 1 & $f_1$ \\
\hline14 & 2D-M458 & 0.5116 & 1.0 & 32 & 1.0 & $f_1$ \\
\hline15 & 2D-M74 & 0.5114 & 1.1 & 115 & 77.5 & $f_1$ \\
\hline16 & 2D-M318 & 0.5006 & 1.1 & 130 & 298.9 & $f_2$ \\
\hline17 & 2D-M213 & 0.4948 & 1.3 & 183 & 60.2 & $f_1$ \\
\hline18 & 2D-M304 & 0.4879 & 1.8 & 307 & 165.1 & $f_2$ \\
\hline19 & 2D-M311 & 0.485 & 1.2 & 152 & 88.5 & $f_1$ \\
\hline20 & 2D-M300 & 0.4831 & 2.1 & 316 & 144.2 & $f_2$ \\
\hline21 & 2D-M314 & 0.4683 & 1.2 & 141 & 266.1 & $f_2$ \\
\hline22 & 2D-M303 & 0.4571 & 1.6 & 294 & 181.6 & $f_2$ \\
\hline23 & 2D-M305 & 0.4477 & 1.5 & 266 & 200.5 & $f_2$ \\
\hline24 & 2D-M98 & 0.4435 & 1.3 & 180 & 88.8 & $f_1$ \\
\hline25 & 2D-M302 & 0.4376 & 1.8 & 306 & 164.6 & $f_2$ \\
\hline26 & 2D-M299 & 0.4327 & 1.7 & 298 & 192.7 & $f_2$ \\
\hline27 & 2D-M86 & 0.4221 & 1.2 & 136 & 100.5 & $f_1$ \\
\hline28 & 2D-M11 & 0.4196 & 1.1 & 117 & 60.2 & $f_1$ \\
\hline29 & 2D-M313 & 0.418 & 1.1 & 108 & 232.3 & $f_2$ \\
\hline30 & 2D-M312 & 0.4138 & 1.2 & 148 & 253.8 & $f_2$ \\
\hline31 & 2D-M239 & 0.3908 & 1.1 & 104 & 80.4 & $f_1$ \\
\hline32 & 2D-M317 & 0.3621 & 1.2 & 131 & 294.7 & $f_2$ \\
\hline33 & 2D-M237 & 0.3503 & 1.1 & 114 & 100.5 & $f_1$ \\
\hline34 & 2D-M132 & 0.3441 & 1.4 & 228 & 88.8 & $f_1$ \\
\hline35 & 2D-M232 & 0.3306 & 1.2 & 157 & 88.8 & $f_1$ \\
\hline36 & 2D-M227 & 0.3291 & 1.0 & 70 & 204.1 & $f_2$ \\
\hline37 & 2D-M286 & 0.3224 & 1.1 & 122 & 194.5 & $f_2$ \\
\hline38 & 2D-M138 & 0.3142 & 1.1 & 111 & 100.5 & $f_1$ \\
\hline39 & 2D-M226 & 0.3127 & 1.5 & 269 & 176.2 & $f_2$ \\
\hline40 & 2D-M307 & 0.3125 & 1.5 & 281 & 186.7 & $f_2$ \\
\hline41 & 2D-M306 & 0.2991 & 1.5 & 259 & 212.1 & $f_2$ \\
\hline42 & 2D-M310 & 0.2946 & 1.6 & 290 & 138.7 & $f_2$ \\
\hline43 & 2D-M521 & 0.2929 & 8.9 & 334 & 8.4 & $f_1$ \\
\hline44 & 2D-M145 & 0.2902 & 1.4 & 240 & 142.5 & $f_2$ \\
\hline45 & 2D-M234 & 0.2884 & 1.1 & 120 & 162.0 & $f_2$ \\
\hline46 & 2D-M59 & 0.2879 & 1.5 & 276 & 189.0 & $f_2$ \\
\hline47 & 2D-M128 & 0.2829 & 1.2 & 133 & 60.2 & $f_1$ \\
\hline48 & 2D-M187 & 0.2736 & 1.3 & 204 & 220.1 & $f_2$ \\
\hline49 & 2D-M293 & 0.273 & 1.3 & 192 & 182.5 & $f_2$ \\
\hline50 & 2D-M118 & 0.273 & 1.3 & 191 & 182.5 & $f_2$ \\
\hline51 & 2D-M135 & 0.273 & 1.3 & 190 & 182.5 & $f_2$ \\
\hline52 & 2D-M256 & 0.2719 & 1.1 & 84 & 100.5 & $f_1$ \\
\hline53 & 2D-M184 & 0.271 & 2.0 & 314 & 164.8 & $f_2$ \\
\hline54 & 2D-M140 & 0.2705 & 1.1 & 119 & 75.9 & $f_1$ \\
\hline55 & 2D-M209 & 0.2696 & 1.4 & 223 & 165.2 & $f_2$ \\
\hline56 & 2D-M236 & 0.2691 & 1.9 & 312 & 149.1 & $f_2$ \\
\hline57 & 2D-M282 & 0.2688 & 1.7 & 300 & 167.5 & $f_2$ \\
\hline58 & 2D-M9 & 0.2678 & 1.2 & 153 & 100.5 & $f_1$ \\
\hline59 & 2D-M182 & 0.2677 & 1.2 & 171 & 168.8 & $f_2$ \\
\hline60 & 2D-M144 & 0.2665 & 1.3 & 216 & 112.8 & $f_2$ \\
\hline61 & 2D-M295 & 0.2587 & 1.2 & 174 & 119.2 & $f_2$ \\
\hline62 & 2D-M524 & 0.2581 & 9.0 & 335 & 8.4 & $f_2$ \\
\hline63 & 2D-M316 & 0.256 & 1.2 & 175 & 168.8 & $f_2$ \\
\hline64 & 2D-M285 & 0.2533 & 1.1 & 80 & 174.6 & $f_2$ \\
\hline65 & 2D-M217 & 0.2526 & 1.6 & 284 & 126.4 & $f_2$ \\
\hline66 & 2D-M116 & 0.2519 & 1.6 & 295 & 123.7 & $f_2$ \\
\hline67 & 2D-M264 & 0.2518 & 7.7 & 325 & 7.1 & $f_1$ \\
\hline68 & 2D-M152 & 0.2506 & 1.1 & 116 & 162.4 & $f_2$ \\
\hline69 & 2D-M87 & 0.2471 & 1.4 & 227 & 132.4 & $f_2$ \\
\hline70 & 2D-M522 & 0.2466 & 7.7 & 326 & 7.1 & $f_2$ \\
\hline71 & 2D-M82 & 0.2439 & 1.2 & 173 & 88.8 & $f_1$ \\
\hline72 & 2D-M88 & 0.2418 & 1.3 & 179 & 182.1 & $f_2$ \\
\hline73 & 2D-M298 & 0.2387 & 1.5 & 265 & 202.0 & $f_2$ \\
\hline74 & 2D-M526 & 0.2381 & 7.7 & 327 & 7.1 & $f_2$ \\
\hline75 & 2D-M215 & 0.2377 & 1.4 & 241 & 100.5 & $f_1$ \\
\hline76 & 2D-M143 & 0.2369 & 1.1 & 82 & 210.2 & $f_2$ \\
\hline77 & 2D-M113 & 0.2355 & 1.4 & 226 & 101.2 & $f_2$ \\
\hline78 & 2D-M61 & 0.233 & 1.8 & 305 & 113.4 & $f_2$ \\
\hline79 & 2D-M546 & 0.2319 & 7.7 & 328 & 7.1 & $f_2$ \\
\hline80 & 2D-M43 & 0.2307 & 1.4 & 246 & 135.8 & $f_2$ \\
\hline81 & 2D-M71 & 0.2305 & 2.0 & 313 & 173.2 & $f_2$ \\
\hline82 & 2D-M181 & 0.2289 & 1.3 & 219 & 142.6 & $f_2$ \\
\hline83 & 2D-M80 & 0.2278 & 1.5 & 263 & 124.4 & $f_2$ \\
\hline84 & 2D-M66 & 0.227 & 1.3 & 178 & 165.4 & $f_2$ \\
\hline85 & 2D-M527 & 0.2263 & 9.0 & 339 & 8.4 & $f_2$ \\
\hline86 & 2D-M185 & 0.2257 & 1.0 & 76 & 149.1 & $f_2$ \\
\hline87 & 2D-M63 & 0.2253 & 1.5 & 271 & 134.9 & $f_2$ \\
\hline88 & 2D-M103 & 0.2251 & 1.3 & 209 & 123.4 & $f_2$ \\
\hline89 & 2D-M251 & 0.2246 & 1.3 & 181 & 141.0 & $f_2$ \\
\hline90 & 2D-M177 & 0.2241 & 1.5 & 279 & 111.0 & $f_2$ \\
\hline91 & 2D-M555 & 0.224 & 9.0 & 340 & 8.4 & $f_2$ \\
\hline92 & 2D-M284 & 0.223 & 2.0 & 315 & 136.6 & $f_2$ \\
\hline93 & 2D-M130 & 0.2218 & 1.3 & 193 & 126.6 & $f_2$ \\
\hline94 & 2D-M212 & 0.2218 & 1.6 & 291 & 137.2 & $f_2$ \\
\hline95 & 2D-M291 & 0.2201 & 1.6 & 288 & 123.7 & $f_2$ \\
\hline96 & 2D-M223 & 0.2201 & 1.6 & 287 & 123.7 & $f_2$ \\
\hline97 & 2D-M120 & 0.2189 & 1.0 & 61 & 145.2 & $f_2$ \\
\hline98 & 2D-M639 & 0.2183 & 1.0 & 18 & 1.0 & $f_2$ \\
\hline99 & 2D-M468 & 0.2157 & 1.0 & 38 & 1.0 & $f_1$ \\
\hline100 & 2D-M235 & 0.2155 & 1.3 & 199 & 109.6 & $f_2$ \\
\hline101 & 2D-M525 & 0.2138 & 9.0 & 341 & 8.4 & $f_2$ \\
\hline102 & 2D-M188 & 0.2127 & 1.4 & 244 & 139.6 & $f_2$ \\
\hline103 & 2D-M635 & 0.2096 & 1.0 & 48 & 1.0 & $f_2$ \\
\hline104 & 2D-M631 & 0.208 & 1.0 & 11 & 1.0 & $f_2$ \\
\hline105 & 2D-M68 & 0.208 & 1.2 & 164 & 175.5 & $f_2$ \\
\hline106 & 2D-M514 & 0.2078 & 9.0 & 342 & 8.4 & $f_2$ \\
\hline107 & 2D-M146 & 0.2056 & 1.2 & 161 & 182.5 & $f_2$ \\
\hline108 & 2D-M297 & 0.204 & 1.9 & 310 & 155.9 & $f_2$ \\
\hline109 & 2D-M56 & 0.2028 & 1.1 & 95 & 159.5 & $f_2$ \\
\hline110 & 2D-M100 & 0.2023 & 1.6 & 293 & 178.8 & $f_2$ \\
\hline111 & 2D-M190 & 0.202 & 10.2 & 351 & 9.5 & $f_1$ \\
\hline112 & 2D-M137 & 0.2016 & 1.0 & 68 & 149.0 & $f_2$ \\
\hline113 & 2D-M629 & 0.2016 & 1.0 & 36 & 1.0 & $f_2$ \\
\hline114 & 2D-M180 & 0.1995 & 1.4 & 225 & 109.1 & $f_2$ \\
\hline115 & 2D-M127 & 0.1984 & 1.3 & 201 & 165.2 & $f_2$ \\
\hline116 & 2D-M512 & 0.1978 & 9.1 & 343 & 8.4 & $f_2$ \\
\hline117 & 2D-M246 & 0.1971 & 1.3 & 184 & 132.2 & $f_2$ \\
\hline118 & 2D-M76 & 0.1969 & 2.5 & 321 & 138.2 & $f_2$ \\
\hline119 & 2D-M85 & 0.1964 & 1.1 & 121 & 140.2 & $f_2$ \\
\hline120 & 2D-M121 & 0.1964 & 1.2 & 132 & 144.5 & $f_2$ \\
\hline121 & 2D-M231 & 0.195 & 1.2 & 144 & 143.0 & $f_2$ \\
\hline122 & 2D-M222 & 0.1949 & 1.4 & 242 & 107.6 & $f_2$ \\
\hline123 & 2D-M250 & 0.1936 & 1.3 & 185 & 107.3 & $f_2$ \\
\hline124 & 2D-M210 & 0.1922 & 1.1 & 105 & 135.4 & $f_2$ \\
\hline125 & 2D-M257 & 0.1919 & 1.4 & 220 & 130.8 & $f_2$ \\
\hline126 & 2D-M523 & 0.1895 & 7.8 & 329 & 7.1 & $f_2$ \\
\hline127 & 2D-M53 & 0.1889 & 1.0 & 57 & 111.8 & $f_2$ \\
\hline128 & 2D-M69 & 0.1883 & 1.3 & 212 & 147.5 & $f_2$ \\
\hline129 & 2D-M529 & 0.1881 & 11.2 & 381 & 10.5 & $f_2$ \\
\hline130 & 2D-M276 & 0.1869 & 11.2 & 382 & 10.5 & $f_1$ \\
\hline131 & 2D-M216 & 0.1861 & 1.3 & 217 & 104.7 & $f_2$ \\
\hline132 & 2D-M142 & 0.1846 & 1.2 & 169 & 149.0 & $f_2$ \\
\hline133 & 2D-M101 & 0.1844 & 1.2 & 176 & 120.0 & $f_2$ \\
\hline134 & 2D-M557 & 0.1843 & 10.2 & 352 & 9.5 & $f_2$ \\
\hline135 & 2D-M221 & 0.182 & 1.4 & 248 & 130.1 & $f_2$ \\
\hline136 & 2D-M183 & 0.1812 & 1.3 & 205 & 101.1 & $f_2$ \\
\hline137 & 2D-M141 & 0.1806 & 1.5 & 272 & 81.9 & $f_2$ \\
\hline138 & 2D-M202 & 0.1799 & 1.1 & 103 & 110.3 & $f_2$ \\
\hline139 & 2D-M102 & 0.1795 & 1.3 & 213 & 95.2 & $f_2$ \\
\hline140 & 2D-M124 & 0.176 & 1.2 & 137 & 119.2 & $f_2$ \\
\hline141 & 2D-M513 & 0.1754 & 11.2 & 383 & 10.5 & $f_2$ \\
\hline142 & 2D-M94 & 0.1753 & 1.4 & 236 & 88.8 & $f_1$ \\
\hline143 & 2D-M517 & 0.175 & 11.2 & 384 & 10.5 & $f_2$ \\
\hline144 & 2D-M99 & 0.1747 & 1.1 & 92 & 132.9 & $f_2$ \\
\hline145 & 2D-M554 & 0.1742 & 11.2 & 385 & 10.5 & $f_2$ \\
\hline146 & 2D-M519 & 0.174 & 11.2 & 386 & 10.5 & $f_2$ \\
\hline147 & 2D-M207 & 0.1733 & 1.0 & 52 & 124.9 & $f_2$ \\
\hline148 & 2D-M60 & 0.1729 & 2.4 & 319 & 130.4 & $f_2$ \\
\hline149 & 2D-M559 & 0.1727 & 11.2 & 387 & 10.5 & $f_2$ \\
\hline150 & 2D-M62 & 0.1717 & 1.1 & 112 & 120.5 & $f_2$ \\
\hline151 & 2D-M632 & 0.171 & 1.0 & 27 & 1.0 & $f_2$ \\
\hline152 & 2D-M111 & 0.1708 & 1.3 & 211 & 109.6 & $f_2$ \\
\hline153 & 2D-M545 & 0.1704 & 11.2 & 389 & 10.5 & $f_2$ \\
\hline154 & 2D-M48 & 0.17 & 1.3 & 182 & 117.5 & $f_2$ \\
\hline155 & 2D-M96 & 0.169 & 1.2 & 156 & 96.8 & $f_2$ \\
\hline156 & 2D-M186 & 0.1684 & 1.7 & 297 & 108.9 & $f_2$ \\
\hline157 & 2D-M214 & 0.1681 & 1.1 & 129 & 101.3 & $f_2$ \\
\hline158 & 2D-M110 & 0.1679 & 1.1 & 93 & 135.3 & $f_2$ \\
\hline159 & 2D-M601 & 0.1676 & 1.0 & 34 & 1.0 & $f_1$ \\
\hline160 & 2D-M46 & 0.1674 & 1.2 & 145 & 100.4 & $f_2$ \\
\hline161 & 2D-M518 & 0.1665 & 11.2 & 390 & 10.5 & $f_2$ \\
\hline162 & 2D-M122 & 0.166 & 1.2 & 142 & 104.2 & $f_2$ \\
\hline163 & 2D-M283 & 0.1653 & 1.6 & 292 & 123.1 & $f_2$ \\
\hline164 & 2D-M97 & 0.1652 & 1.5 & 280 & 112.8 & $f_2$ \\
\hline165 & 2D-M627 & 0.1651 & 1.0 & 28 & 1.0 & $f_2$ \\
\hline166 & 2D-M204 & 0.1636 & 1.4 & 253 & 92.9 & $f_2$ \\
\hline167 & 2D-M558 & 0.1626 & 11.2 & 391 & 10.5 & $f_2$ \\
\hline168 & 2D-M296 & 0.1625 & 1.2 & 134 & 119.5 & $f_2$ \\
\hline169 & 2D-M131 & 0.1618 & 1.2 & 143 & 128.4 & $f_2$ \\
\hline170 & 2D-M623 & 0.1613 & 1.0 & 14 & 1.0 & $f_2$ \\
\hline171 & 2D-M640 & 0.1608 & 1.0 & 43 & 1.0 & $f_2$ \\
\hline172 & 2D-M107 & 0.1602 & 1.1 & 83 & 120.8 & $f_2$ \\
\hline173 & 2D-M515 & 0.1581 & 11.2 & 392 & 10.5 & $f_2$ \\
\hline174 & 2D-M49 & 0.1576 & 1.1 & 109 & 91.0 & $f_2$ \\
\hline175 & 2D-M108 & 0.1576 & 1.1 & 99 & 127.9 & $f_2$ \\
\hline176 & 2D-M597 & 0.1569 & 1.0 & 41 & 1.0 & $f_1$ \\
\hline177 & 2D-M136 & 0.1553 & 1.2 & 139 & 126.7 & $f_2$ \\
\hline178 & 2D-M292 & 0.1543 & 1.2 & 163 & 124.6 & $f_2$ \\
\hline179 & 2D-M45 & 0.1538 & 1.3 & 218 & 137.5 & $f_2$ \\
\hline180 & 2D-M148 & 0.1535 & 1.0 & 56 & 91.6 & $f_2$ \\
\hline181 & 2D-M243 & 0.1534 & 11.3 & 393 & 10.5 & $f_1$ \\
\hline182 & 2D-M104 & 0.1515 & 1.1 & 102 & 121.5 & $f_2$ \\
\hline183 & 2D-M638 & 0.1508 & 1.0 & 31 & 1.0 & $f_2$ \\
\hline184 & 2D-M225 & 0.1494 & 1.1 & 81 & 109.5 & $f_2$ \\
\hline185 & 2D-M454 & 0.1488 & 10.3 & 354 & 9.5 & $f_1$ \\
\hline186 & 2D-M84 & 0.1484 & 1.6 & 283 & 114.9 & $f_2$ \\
\hline187 & 2D-M47 & 0.1467 & 1.3 & 189 & 103.7 & $f_2$ \\
\hline188 & 2D-M44 & 0.1466 & 1.4 & 247 & 121.1 & $f_2$ \\
\hline189 & 2D-M241 & 0.1455 & 1.4 & 257 & 90.4 & $f_2$ \\
\hline190 & 2D-M114 & 0.1451 & 1.1 & 98 & 116.6 & $f_2$ \\
\hline191 & 2D-M528 & 0.1447 & 11.3 & 395 & 10.5 & $f_2$ \\
\hline192 & 2D-M621 & 0.1437 & 1.0 & 30 & 1.0 & $f_2$ \\
\hline193 & 2D-M478 & 0.1431 & 10.3 & 355 & 9.5 & $f_1$ \\
\hline194 & 2D-M268 & 0.1428 & 11.3 & 396 & 10.5 & $f_1$ \\
\hline195 & 2D-M609 & 0.1385 & 1.0 & 40 & 1.0 & $f_1$ \\
\hline196 & 2D-M133 & 0.1381 & 1.5 & 277 & 94.7 & $f_2$ \\
\hline197 & 2D-M90 & 0.1378 & 1.2 & 140 & 100.2 & $f_2$ \\
\hline198 & 2D-M51 & 0.1372 & 1.4 & 254 & 104.1 & $f_2$ \\
\hline199 & 2D-M95 & 0.1364 & 1.2 & 150 & 90.2 & $f_2$ \\
\hline200 & 2D-M115 & 0.1354 & 1.1 & 128 & 91.0 & $f_2$ \\
\hline201 & 2D-M89 & 0.1353 & 1.5 & 270 & 87.1 & $f_2$ \\
\hline202 & 2D-M371 & 0.1352 & 7.7 & 324 & 6.8 & $f_1$ \\
\hline203 & 2D-M238 & 0.134 & 1.4 & 249 & 85.2 & $f_2$ \\
\hline204 & 2D-M129 & 0.1339 & 1.0 & 13 & 91.0 & $f_2$ \\
\hline205 & 2D-M81 & 0.1336 & 1.3 & 195 & 98.0 & $f_2$ \\
\hline206 & 2D-M626 & 0.133 & 1.0 & 49 & 1.0 & $f_2$ \\
\hline207 & 2D-M625 & 0.1323 & 1.0 & 20 & 1.0 & $f_2$ \\
\hline208 & 2D-M516 & 0.1323 & 10.4 & 356 & 9.5 & $f_2$ \\
\hline209 & 2D-M5 & 0.1309 & 1.3 & 206 & 100.1 & $f_2$ \\
\hline210 & 2D-M52 & 0.1305 & 1.6 & 286 & 100.4 & $f_2$ \\
\hline211 & 2D-M247 & 0.1293 & 1.6 & 285 & 88.8 & $f_2$ \\
\hline212 & 2D-M109 & 0.1284 & 1.4 & 233 & 105.7 & $f_2$ \\
\hline213 & 2D-M64 & 0.128 & 1.0 & 75 & 85.3 & $f_2$ \\
\hline214 & 2D-M83 & 0.1275 & 1.0 & 15 & 111.0 & $f_2$ \\
\hline215 & 2D-M75 & 0.1272 & 1.3 & 202 & 88.8 & $f_2$ \\
\hline216 & 2D-M447 & 0.1272 & 11.4 & 397 & 10.5 & $f_1$ \\
\hline217 & 2D-M79 & 0.1264 & 1.6 & 296 & 75.3 & $f_2$ \\
\hline218 & 2D-M245 & 0.1264 & 1.1 & 100 & 96.5 & $f_2$ \\
\hline219 & 2D-M65 & 0.1258 & 1.0 & 51 & 90.7 & $f_2$ \\
\hline220 & 2D-M8 & 0.1255 & 1.7 & 301 & 86.0 & $f_2$ \\
\hline221 & 2D-M54 & 0.125 & 1.2 & 149 & 68.0 & $f_2$ \\
\hline222 & 2D-M4 & 0.1247 & 1.9 & 311 & 62.0 & $f_2$ \\
\hline223 & 2D-M3 & 0.1245 & 1.1 & 123 & 88.7 & $f_2$ \\
\hline224 & 2D-M72 & 0.1243 & 1.2 & 168 & 74.9 & $f_2$ \\
\hline225 & 2D-M6 & 0.1242 & 1.0 & 62 & 111.1 & $f_2$ \\
\hline226 & 2D-M544 & 0.1241 & 17.5 & 604 & 17.5 & $f_2$ \\
\hline227 & 2D-M50 & 0.1236 & 1.2 & 151 & 85.4 & $f_2$ \\
\hline228 & 2D-M414 & 0.1229 & 10.4 & 359 & 9.5 & $f_1$ \\
\hline229 & 2D-M151 & 0.1218 & 1.0 & 72 & 93.3 & $f_2$ \\
\hline230 & 2D-M7 & 0.1216 & 1.4 & 222 & 100.5 & $f_2$ \\
\hline231 & 2D-M41 & 0.1211 & 1.2 & 154 & 98.8 & $f_2$ \\
\hline232 & 2D-M117 & 0.121 & 1.0 & 66 & 92.3 & $f_2$ \\
\hline233 & 2D-M150 & 0.121 & 1.0 & 67 & 92.3 & $f_2$ \\
\hline234 & 2D-M106 & 0.1209 & 1.3 & 208 & 92.2 & $f_2$ \\
\hline235 & 2D-M211 & 0.1199 & 2.2 & 318 & 87.7 & $f_2$ \\
\hline236 & 2D-M57 & 0.1189 & 1.5 & 268 & 96.6 & $f_2$ \\
\hline237 & 2D-M139 & 0.1182 & 1.3 & 177 & 69.6 & $f_2$ \\
\hline238 & 2D-M240 & 0.1178 & 1.1 & 125 & 88.9 & $f_2$ \\
\hline239 & 2D-M105 & 0.1177 & 1.2 & 162 & 89.5 & $f_2$ \\
\hline240 & 2D-M541 & 0.1172 & 9.3 & 345 & 8.4 & $f_1$ \\
\hline241 & 2D-M249 & 0.117 & 1.5 & 278 & 95.3 & $f_2$ \\
\hline242 & 2D-M78 & 0.1165 & 1.1 & 113 & 68.5 & $f_2$ \\
\hline243 & 2D-M70 & 0.1162 & 1.1 & 101 & 57.4 & $f_2$ \\
\hline244 & 2D-M530 & 0.1158 & 17.4 & 599 & 17.4 & $f_2$ \\
\hline245 & 2D-M58 & 0.1149 & 1.3 & 214 & 63.5 & $f_2$ \\
\hline246 & 2D-M93 & 0.1146 & 1.5 & 273 & 88.8 & $f_2$ \\
\hline247 & 2D-M125 & 0.1145 & 1.5 & 260 & 78.1 & $f_2$ \\
\hline248 & 2D-M10 & 0.1143 & 1.7 & 302 & 86.0 & $f_2$ \\
\hline249 & 2D-M112 & 0.1143 & 1.3 & 194 & 72.4 & $f_2$ \\
\hline250 & 2D-M15 & 0.1138 & 1.7 & 303 & 86.0 & $f_2$ \\
\hline251 & 2D-M149 & 0.1138 & 1.0 & 74 & 72.9 & $f_2$ \\
\hline252 & 2D-M147 & 0.1138 & 1.0 & 73 & 72.9 & $f_2$ \\
\hline253 & 2D-M294 & 0.1137 & 1.5 & 258 & 85.6 & $f_2$ \\
\hline254 & 2D-M178 & 0.1129 & 1.1 & 96 & 77.5 & $f_2$ \\
\hline255 & 2D-M551 & 0.1124 & 17.4 & 598 & 17.4 & $f_2$ \\
\hline256 & 2D-M123 & 0.1121 & 1.2 & 160 & 75.2 & $f_2$ \\
\hline257 & 2D-M2 & 0.1115 & 1.2 & 159 & 100.4 & $f_2$ \\
\hline258 & 2D-M119 & 0.1105 & 1.3 & 215 & 68.1 & $f_2$ \\
\hline259 & 2D-M624 & 0.1091 & 1.0 & 35 & 1.0 & $f_2$ \\
\hline260 & 2D-M290 & 0.1086 & 1.1 & 97 & 90.6 & $f_2$ \\
\hline261 & 2D-M1 & 0.106 & 1.9 & 309 & 74.0 & $f_2$ \\
\hline262 & 2D-M67 & 0.1059 & 1.5 & 264 & 79.0 & $f_2$ \\
\hline263 & 2D-M531 & 0.1058 & 17.6 & 605 & 17.5 & $f_2$ \\
\hline264 & 2D-M463 & 0.1045 & 10.5 & 360 & 9.5 & $f_1$ \\
\hline265 & 2D-M641 & 0.1036 & 1.0 & 42 & 1.0 & $f_2$ \\
\hline266 & 2D-M532 & 0.1028 & 17.4 & 597 & 17.4 & $f_2$ \\
\hline267 & 2D-M636 & 0.1026 & 1.0 & 33 & 1.0 & $f_2$ \\
\hline268 & 2D-M630 & 0.1021 & 1.0 & 45 & 1.0 & $f_2$ \\
\hline269 & 2D-M434 & 0.1012 & 10.5 & 361 & 9.5 & $f_1$ \\
\hline270 & 2D-M29 & 0.101 & 8.2 & 331 & 7.1 & $f_1$ \\
\hline271 & 2D-M637 & 0.1006 & 1.0 & 5 & 1.0 & $f_2$ \\
\hline272 & 2D-M233 & 0.099 & 2.5 & 320 & 82.4 & $f_2$ \\
\hline273 & 2D-M77 & 0.099 & 1.4 & 255 & 63.5 & $f_2$ \\
\hline274 & 2D-M55 & 0.0984 & 1.5 & 262 & 78.8 & $f_2$ \\
\hline275 & 2D-M553 & 0.097 & 16.8 & 575 & 16.5 & $f_2$ \\
\hline276 & 2D-M42 & 0.0964 & 1.4 & 221 & 60.2 & $f_2$ \\
\hline277 & 2D-M642 & 0.0962 & 1.0 & 9 & 111.0 & $f_1$ \\
\hline278 & 2D-M255 & 0.0945 & 1.8 & 308 & 76.7 & $f_2$ \\
\hline279 & 2D-M409 & 0.093 & 10.6 & 362 & 9.5 & $f_1$ \\
\hline280 & 2D-M620 & 0.0923 & 1.0 & 16 & 1.0 & $f_2$ \\
\hline281 & 2D-M452 & 0.0922 & 10.6 & 363 & 9.5 & $f_1$ \\
\hline282 & 2D-M471 & 0.091 & 11.6 & 403 & 10.5 & $f_1$ \\
\hline283 & 2D-M179 & 0.0906 & 1.0 & 78 & 62.8 & $f_2$ \\
\hline284 & 2D-M438 & 0.0901 & 9.2 & 344 & 8.1 & $f_1$ \\
\hline285 & 2D-M92 & 0.0898 & 1.5 & 267 & 62.1 & $f_2$ \\
\hline286 & 2D-M91 & 0.0896 & 1.4 & 231 & 49.5 & $f_2$ \\
\hline287 & 2D-M73 & 0.088 & 1.3 & 197 & 48.2 & $f_2$ \\
\hline288 & 2D-M622 & 0.0869 & 1.0 & 39 & 1.0 & $f_2$ \\
\hline289 & 2D-M365 & 0.0868 & 11.6 & 406 & 10.5 & $f_1$ \\
\hline290 & 2D-M482 & 0.0862 & 1.0 & 44 & 1.0 & $f_1$ \\
\hline291 & 2D-M547 & 0.0855 & 10.4 & 357 & 9.3 & $f_2$ \\
\hline292 & 2D-M426 & 0.0843 & 10.6 & 366 & 9.5 & $f_1$ \\
\hline293 & 2D-M27 & 0.0834 & 11.6 & 408 & 10.5 & $f_1$ \\
\hline294 & 2D-M538 & 0.0833 & 11.8 & 416 & 10.1 & $f_1$ \\
\hline295 & 2D-M495 & 0.0823 & 11.6 & 409 & 10.5 & $f_1$ \\
\hline296 & 2D-M536 & 0.0805 & 19.8 & 622 & 19.8 & $f_2$ \\
\hline297 & 2D-M373 & 0.0742 & 11.7 & 412 & 10.5 & $f_1$ \\
\hline298 & 2D-M280 & 0.0736 & 11.7 & 413 & 10.5 & $f_1$ \\
\hline299 & 2D-M476 & 0.073 & 11.7 & 414 & 10.5 & $f_1$ \\
\hline300 & 2D-M377 & 0.0705 & 10.8 & 369 & 9.5 & $f_1$ \\
\hline301 & 2D-M253 & 0.0693 & 11.8 & 415 & 10.5 & $f_1$ \\
\hline302 & 2D-M540 & 0.0692 & 20.2 & 629 & 20.2 & $f_2$ \\
\hline303 & 2D-M539 & 0.067 & 20.2 & 630 & 20.2 & $f_2$ \\
\hline304 & 2D-M549 & 0.0656 & 20.2 & 626 & 20.2 & $f_2$ \\
\hline305 & 2D-M552 & 0.0605 & 20.2 & 627 & 20.2 & $f_2$ \\
\hline306 & 2D-M537 & 0.0603 & 20.2 & 628 & 20.2 & $f_2$ \\
\hline307 & 2D-M533 & 0.0579 & 9.0 & 336 & 6.4 & $f_1$ \\
\hline308 & 2D-M32 & 0.0565 & 1.0 & 22 & 1.0 & $f_1$ \\
\hline309 & 2D-M633 & 0.0525 & 1.0 & 46 & 1.0 & $f_2$ \\
\hline310 & 2D-M219 & 0.0514 & 8.8 & 333 & 7.1 & $f_1$ \\
\hline311 & 2D-M422 & 0.0484 & 10.1 & 350 & 8.4 & $f_1$ \\
\hline312 & 2D-M492 & 0.0458 & 1.0 & 10 & 1 & $f_1$ \\
\hline313 & 2D-M379 & 0.0441 & 12.2 & 433 & 10.5 & $f_1$ \\
\hline314 & 2D-M487 & 0.0401 & 12.3 & 436 & 10.5 & $f_1$ \\
\hline315 & 2D-M420 & 0.0335 & 14.1 & 512 & 14.2 & $f_2$ \\
\hline316 & 2D-M589 & 0.0333 & 1.0 & 37 & 1.0 & $f_1$ \\
\hline317 & 2D-M613 & 0.0326 & 1.0 & 47 & 1.0 & $f_1$ \\
\hline318 & 2D-M498 & 0.032 & 17.2 & 580 & 17.4 & $f_2$ \\
\hline319 & 2D-M352 & 0.0318 & 17.3 & 585 & 17.3 & $f_2$ \\
\hline320 & 2D-M157 & 0.0297 & 20.8 & 636 & 20.1 & $f_2$ \\
\hline321 & 2D-M262 & 0.0296 & 11.2 & 388 & 18.1 & $f_2$ \\
\hline322 & 2D-M218 & 0.0294 & 17.0 & 579 & 16.8 & $f_2$ \\
\hline323 & 2D-M542 & 0.0293 & 16.8 & 573 & 15.8 & $f_2$ \\
\hline324 & 2D-M172 & 0.0289 & 17.5 & 601 & 15.1 & $f_2$ \\
\hline325 & 2D-M205 & 0.028 & 14.6 & 535 & 18.9 & $f_2$ \\
\hline326 & 2D-M394 & 0.0271 & 12.8 & 451 & 8.6 & $f_2$ \\
\hline327 & 2D-M520 & 0.027 & 19.4 & 618 & 18.1 & $f_2$ \\
\hline328 & 2D-M421 & 0.0268 & 17.3 & 586 & 17.3 & $f_2$ \\
\hline329 & 2D-M360 & 0.0268 & 17.3 & 582 & 17.3 & $f_2$ \\
\hline330 & 2D-M413 & 0.0267 & 13.2 & 472 & 12.9 & $f_2$ \\
\hline331 & 2D-M355 & 0.0266 & 14.1 & 523 & 14.1 & $f_2$ \\
\hline332 & 2D-M349 & 0.0263 & 14.6 & 536 & 14.5 & $f_2$ \\
\hline333 & 2D-M508 & 0.0263 & 17.6 & 606 & 16.4 & $f_2$ \\
\hline334 & 2D-M407 & 0.0261 & 14.9 & 541 & 14.9 & $f_2$ \\
\hline335 & 2D-M389 & 0.026 & 17.4 & 594 & 6.4 & $f_2$ \\
\hline336 & 2D-M424 & 0.0259 & 16.1 & 561 & 18.4 & $f_2$ \\
\hline337 & 2D-M450 & 0.0258 & 13.1 & 460 & 13.0 & $f_2$ \\
\hline338 & 2D-M534 & 0.0254 & 19.9 & 624 & 18.6 & $f_2$ \\
\hline339 & 2D-M548 & 0.0253 & 19.0 & 615 & 17.8 & $f_2$ \\
\hline340 & 2D-M387 & 0.0245 & 17.3 & 590 & 6.4 & $f_2$ \\
\hline341 & 2D-M412 & 0.0244 & 13.1 & 463 & 13.1 & $f_2$ \\
\hline342 & 2D-M543 & 0.0241 & 18.5 & 610 & 18.0 & $f_2$ \\
\hline343 & 2D-M556 & 0.024 & 20.4 & 633 & 18.6 & $f_2$ \\
\hline344 & 2D-M346 & 0.0239 & 14.8 & 538 & 12.3 & $f_2$ \\
\hline345 & 2D-M475 & 0.0238 & 17.0 & 578 & 17.5 & $f_2$ \\
\hline346 & 2D-M288 & 0.0238 & 15.0 & 543 & 14.8 & $f_2$ \\
\hline347 & 2D-M507 & 0.0235 & 17.3 & 588 & 17.3 & $f_2$ \\
\hline348 & 2D-M348 & 0.0235 & 17.3 & 587 & 17.3 & $f_2$ \\
\hline349 & 2D-M163 & 0.0234 & 13.7 & 481 & 12.6 & $f_2$ \\
\hline350 & 2D-M242 & 0.023 & 18.4 & 609 & 13.8 & $f_2$ \\
\hline351 & 2D-M550 & 0.023 & 19.1 & 617 & 17.7 & $f_2$ \\
\hline352 & 2D-M24 & 0.0228 & 14.5 & 532 & 12.1 & $f_2$ \\
\hline353 & 2D-M425 & 0.0226 & 14.1 & 522 & 14.1 & $f_2$ \\
\hline354 & 2D-M357 & 0.0223 & 17.4 & 595 & 16.9 & $f_2$ \\
\hline355 & 2D-M535 & 0.0222 & 19.8 & 623 & 18.4 & $f_2$ \\
\hline356 & 2D-M406 & 0.0222 & 13.9 & 494 & 15.1 & $f_2$ \\
\hline357 & 2D-M156 & 0.0222 & 16.8 & 572 & 13.6 & $f_2$ \\
\hline358 & 2D-M252 & 0.0219 & 20.3 & 632 & 14.3 & $f_2$ \\
\hline359 & 2D-M628 & 0.0217 & 1.0 & 26 & 1.0 & $f_2$ \\
\hline360 & 2D-M366 & 0.0215 & 13.0 & 458 & 12.9 & $f_2$ \\
\hline361 & 2D-M343 & 0.0215 & 12.1 & 429 & 7.8 & $f_2$ \\
\hline362 & 2D-M155 & 0.0215 & 16.3 & 563 & 13.9 & $f_2$ \\
\hline363 & 2D-M194 & 0.0214 & 16.3 & 562 & 13.6 & $f_2$ \\
\hline364 & 2D-M502 & 0.0214 & 17.3 & 584 & 17.3 & $f_2$ \\
\hline365 & 2D-M374 & 0.0214 & 17.3 & 583 & 17.3 & $f_2$ \\
\hline366 & 2D-M192 & 0.0213 & 16.1 & 560 & 13.2 & $f_2$ \\
\hline367 & 2D-M354 & 0.021 & 17.0 & 577 & 14.6 & $f_2$ \\
\hline368 & 2D-M168 & 0.0209 & 14.0 & 498 & 12.5 & $f_2$ \\
\hline369 & 2D-M353 & 0.0208 & 14.3 & 531 & 11.8 & $f_2$ \\
\hline370 & 2D-M465 & 0.0205 & 14.0 & 506 & 14.0 & $f_2$ \\
\hline371 & 2D-M363 & 0.0203 & 15.1 & 545 & 15.1 & $f_2$ \\
\hline372 & 2D-M160 & 0.0202 & 15.2 & 548 & 15.1 & $f_2$ \\
\hline373 & 2D-M17 & 0.0202 & 14.1 & 511 & 14.8 & $f_2$ \\
\hline374 & 2D-M484 & 0.0201 & 13.0 & 456 & 10.3 & $f_2$ \\
\hline375 & 2D-M375 & 0.0199 & 10.9 & 378 & 10.9 & $f_2$ \\
\hline376 & 2D-M415 & 0.0198 & 15.0 & 542 & 13.4 & $f_2$ \\
\hline377 & 2D-M361 & 0.0195 & 11.4 & 398 & 11.4 & $f_2$ \\
\hline378 & 2D-M411 & 0.0194 & 15.0 & 544 & 15.3 & $f_2$ \\
\hline379 & 2D-M170 & 0.0194 & 15.7 & 556 & 11.6 & $f_2$ \\
\hline380 & 2D-M164 & 0.0192 & 12.7 & 444 & 8.7 & $f_2$ \\
\hline381 & 2D-M362 & 0.0192 & 12.5 & 442 & 9.6 & $f_2$ \\
\hline382 & 2D-M230 & 0.0191 & 13.7 & 485 & 12.3 & $f_2$ \\
\hline383 & 2D-M228 & 0.0191 & 12.9 & 452 & 12.9 & $f_2$ \\
\hline384 & 2D-M16 & 0.0184 & 15.6 & 553 & 10.3 & $f_2$ \\
\hline385 & 2D-M267 & 0.0184 & 11.6 & 405 & 12.4 & $f_2$ \\
\hline386 & 2D-M376 & 0.0184 & 11.4 & 399 & 10.1 & $f_2$ \\
\hline387 & 2D-M410 & 0.0183 & 16.5 & 567 & 13.8 & $f_2$ \\
\hline388 & 2D-M193 & 0.0181 & 10.8 & 370 & 9.6 & $f_2$ \\
\hline389 & 2D-M378 & 0.0181 & 14.7 & 537 & 12.7 & $f_2$ \\
\hline390 & 2D-M278 & 0.0181 & 16.1 & 558 & 10.6 & $f_2$ \\
\hline391 & 2D-M158 & 0.0179 & 15.3 & 551 & 12.9 & $f_2$ \\
\hline392 & 2D-M456 & 0.0178 & 19.8 & 621 & 13.2 & $f_2$ \\
\hline393 & 2D-M344 & 0.0178 & 13.0 & 454 & 10.0 & $f_2$ \\
\hline394 & 2D-M175 & 0.0177 & 18.9 & 613 & 10.5 & $f_2$ \\
\hline395 & 2D-M474 & 0.0177 & 10.9 & 375 & 10.9 & $f_2$ \\
\hline396 & 2D-M430 & 0.0175 & 10.4 & 358 & 11.7 & $f_2$ \\
\hline397 & 2D-M497 & 0.0174 & 20.4 & 634 & 13.0 & $f_2$ \\
\hline398 & 2D-M28 & 0.0174 & 14.1 & 524 & 14.1 & $f_2$ \\
\hline399 & 2D-M26 & 0.0174 & 14.1 & 525 & 14.1 & $f_2$ \\
\hline400 & 2D-M372 & 0.0173 & 10.9 & 376 & 10.9 & $f_2$ \\
\hline401 & 2D-M485 & 0.0173 & 20.8 & 635 & 9.5 & $f_2$ \\
\hline402 & 2D-M460 & 0.0171 & 12.4 & 439 & 9.4 & $f_2$ \\
\hline403 & 2D-M503 & 0.017 & 15.2 & 547 & 12.3 & $f_2$ \\
\hline404 & 2D-M439 & 0.017 & 15.2 & 546 & 12.3 & $f_2$ \\
\hline405 & 2D-M489 & 0.017 & 17.8 & 608 & 10.8 & $f_2$ \\
\hline406 & 2D-M201 & 0.0169 & 14.3 & 530 & 10.4 & $f_2$ \\
\hline407 & 2D-M504 & 0.0169 & 13.0 & 457 & 11.3 & $f_2$ \\
\hline408 & 2D-M173 & 0.0169 & 15.2 & 549 & 12.4 & $f_2$ \\
\hline409 & 2D-M404 & 0.0169 & 13.5 & 475 & 10.7 & $f_2$ \\
\hline410 & 2D-M277 & 0.0168 & 12.7 & 446 & 9.3 & $f_2$ \\
\hline411 & 2D-M196 & 0.0166 & 11.8 & 419 & 13.3 & $f_2$ \\
\hline412 & 2D-M364 & 0.0166 & 12.4 & 438 & 9.3 & $f_2$ \\
\hline413 & 2D-M254 & 0.0166 & 12.2 & 430 & 10.5 & $f_2$ \\
\hline414 & 2D-M390 & 0.0166 & 17.4 & 596 & 4.1 & $f_2$ \\
\hline415 & 2D-M405 & 0.0165 & 11.6 & 404 & 10.2 & $f_2$ \\
\hline416 & 2D-M381 & 0.0163 & 14.2 & 526 & 8.2 & $f_2$ \\
\hline417 & 2D-M408 & 0.0162 & 10.3 & 353 & 10.3 & $f_2$ \\
\hline418 & 2D-M477 & 0.0161 & 10.9 & 379 & 10.9 & $f_2$ \\
\hline419 & 2D-M359 & 0.0161 & 10.9 & 377 & 10.9 & $f_2$ \\
\hline420 & 2D-M174 & 0.0161 & 13.8 & 487 & 11.2 & $f_2$ \\
\hline421 & 2D-M266 & 0.016 & 12.2 & 435 & 11.3 & $f_2$ \\
\hline422 & 2D-M263 & 0.016 & 12.5 & 441 & 10.7 & $f_2$ \\
\hline423 & 2D-M369 & 0.0159 & 9.0 & 337 & 9.0 & $f_2$ \\
\hline424 & 2D-M199 & 0.0159 & 24.4 & 641 & 9.2 & $f_2$ \\
\hline425 & 2D-M453 & 0.0159 & 11.7 & 411 & 10.9 & $f_2$ \\
\hline426 & 2D-M500 & 0.0159 & 17.5 & 603 & 10.1 & $f_2$ \\
\hline427 & 2D-M435 & 0.0158 & 12.0 & 422 & 8.7 & $f_2$ \\
\hline428 & 2D-M198 & 0.0158 & 12.7 & 445 & 11.2 & $f_2$ \\
\hline429 & 2D-M397 & 0.0156 & 14.1 & 514 & 9.3 & $f_2$ \\
\hline430 & 2D-M473 & 0.0155 & 17.5 & 602 & 9.9 & $f_2$ \\
\hline431 & 2D-M229 & 0.0155 & 12.7 & 448 & 9.5 & $f_2$ \\
\hline432 & 2D-M260 & 0.0154 & 11.8 & 420 & 8.5 & $f_2$ \\
\hline433 & 2D-M23 & 0.0154 & 9.9 & 348 & 10.3 & $f_2$ \\
\hline434 & 2D-M461 & 0.0154 & 11.9 & 421 & 9.8 & $f_2$ \\
\hline435 & 2D-M35 & 0.0153 & 11.5 & 402 & 12.9 & $f_2$ \\
\hline436 & 2D-M427 & 0.0153 & 13.4 & 473 & 10.1 & $f_2$ \\
\hline437 & 2D-M165 & 0.0153 & 11.7 & 410 & 7.8 & $f_2$ \\
\hline438 & 2D-M200 & 0.0152 & 12.8 & 449 & 10.8 & $f_2$ \\
\hline439 & 2D-M383 & 0.0152 & 11.6 & 407 & 10.5 & $f_2$ \\
\hline440 & 2D-M385 & 0.0152 & 13.0 & 455 & 8.3 & $f_2$ \\
\hline441 & 2D-M220 & 0.0151 & 11.8 & 417 & 8.6 & $f_2$ \\
\hline442 & 2D-M499 & 0.015 & 13.8 & 489 & 9.3 & $f_2$ \\
\hline443 & 2D-M153 & 0.0149 & 13.6 & 478 & 11.8 & $f_2$ \\
\hline444 & 2D-M159 & 0.0148 & 14.1 & 520 & 9.8 & $f_2$ \\
\hline445 & 2D-M340 & 0.0148 & 17.6 & 607 & 12.0 & $f_2$ \\
\hline446 & 2D-M466 & 0.0148 & 11.5 & 400 & 10.4 & $f_2$ \\
\hline447 & 2D-M419 & 0.0147 & 10.7 & 367 & 6.9 & $f_2$ \\
\hline448 & 2D-M259 & 0.0146 & 12.2 & 431 & 8.9 & $f_2$ \\
\hline449 & 2D-M273 & 0.0146 & 12.8 & 450 & 9.7 & $f_2$ \\
\hline450 & 2D-M244 & 0.0146 & 13.7 & 482 & 10.5 & $f_2$ \\
\hline451 & 2D-M451 & 0.0145 & 12.9 & 453 & 6.4 & $f_2$ \\
\hline452 & 2D-M31 & 0.0145 & 8.2 & 330 & 8.2 & $f_2$ \\
\hline453 & 2D-M289 & 0.0145 & 11.5 & 401 & 8.6 & $f_2$ \\
\hline454 & 2D-M279 & 0.0144 & 12.5 & 440 & 8.7 & $f_2$ \\
\hline455 & 2D-M417 & 0.0143 & 13.1 & 465 & 11.3 & $f_2$ \\
\hline456 & 2D-M386 & 0.0143 & 17.3 & 589 & 5.3 & $f_2$ \\
\hline457 & 2D-M342 & 0.0142 & 17.4 & 593 & 5.2 & $f_2$ \\
\hline458 & 2D-M488 & 0.0141 & 13.1 & 461 & 11.3 & $f_2$ \\
\hline459 & 2D-M167 & 0.014 & 10.6 & 365 & 7.0 & $f_2$ \\
\hline460 & 2D-M501 & 0.0139 & 14.0 & 501 & 10.6 & $f_2$ \\
\hline461 & 2D-M368 & 0.0139 & 14.0 & 502 & 10.6 & $f_2$ \\
\hline462 & 2D-M480 & 0.0139 & 16.4 & 566 & 10.3 & $f_2$ \\
\hline463 & 2D-M258 & 0.0139 & 9.8 & 346 & 6.8 & $f_2$ \\
\hline464 & 2D-M392 & 0.0139 & 18.5 & 612 & 4.9 & $f_2$ \\
\hline465 & 2D-M189 & 0.0139 & 13.8 & 491 & 10.4 & $f_2$ \\
\hline466 & 2D-M154 & 0.0138 & 13.6 & 479 & 10.3 & $f_2$ \\
\hline467 & 2D-M261 & 0.0138 & 14.0 & 507 & 10.6 & $f_2$ \\
\hline468 & 2D-M510 & 0.0138 & 9.9 & 347 & 7.1 & $f_2$ \\
\hline469 & 2D-M399 & 0.0138 & 16.6 & 568 & 11.0 & $f_2$ \\
\hline470 & 2D-M14 & 0.0138 & 10.8 & 371 & 6.9 & $f_2$ \\
\hline471 & 2D-M324 & 0.0137 & 13.8 & 488 & 10.6 & $f_2$ \\
\hline472 & 2D-M382 & 0.0137 & 19.9 & 625 & 5.8 & $f_2$ \\
\hline473 & 2D-M271 & 0.0136 & 13.9 & 496 & 10.5 & $f_2$ \\
\hline474 & 2D-M403 & 0.0136 & 11.1 & 380 & 7.1 & $f_2$ \\
\hline475 & 2D-M333 & 0.0136 & 13.9 & 497 & 10.5 & $f_2$ \\
\hline476 & 2D-M12 & 0.0136 & 12.2 & 434 & 8.9 & $f_2$ \\
\hline477 & 2D-M356 & 0.0136 & 10.8 & 372 & 7.2 & $f_2$ \\
\hline478 & 2D-M331 & 0.0132 & 13.1 & 459 & 9.5 & $f_2$ \\
\hline479 & 2D-M269 & 0.0132 & 13.5 & 476 & 10.8 & $f_2$ \\
\hline480 & 2D-M281 & 0.0132 & 10.0 & 349 & 7.0 & $f_2$ \\
\hline481 & 2D-M351 & 0.0132 & 14.2 & 528 & 10.8 & $f_2$ \\
\hline482 & 2D-M431 & 0.0132 & 14.2 & 527 & 10.8 & $f_2$ \\
\hline483 & 2D-M337 & 0.0132 & 12.0 & 424 & 8.4 & $f_2$ \\
\hline484 & 2D-M166 & 0.0132 & 14.0 & 499 & 9.4 & $f_2$ \\
\hline485 & 2D-M265 & 0.0131 & 14.0 & 500 & 10.5 & $f_2$ \\
\hline486 & 2D-M393 & 0.0131 & 18.5 & 611 & 4.9 & $f_2$ \\
\hline487 & 2D-M462 & 0.0131 & 14.0 & 503 & 10.5 & $f_2$ \\
\hline488 & 2D-M436 & 0.0131 & 14.0 & 504 & 10.5 & $f_2$ \\
\hline489 & 2D-M334 & 0.0131 & 14.0 & 505 & 10.5 & $f_2$ \\
\hline490 & 2D-M329 & 0.013 & 12.0 & 425 & 8.4 & $f_2$ \\
\hline491 & 2D-M384 & 0.013 & 21.4 & 639 & 10.5 & $f_2$ \\
\hline492 & 2D-M395 & 0.013 & 21.3 & 638 & 10.5 & $f_2$ \\
\hline493 & 2D-M396 & 0.013 & 19.7 & 619 & 7.1 & $f_2$ \\
\hline494 & 2D-M162 & 0.013 & 10.8 & 368 & 7.1 & $f_2$ \\
\hline495 & 2D-M206 & 0.013 & 10.9 & 374 & 8.2 & $f_2$ \\
\hline496 & 2D-M274 & 0.013 & 12.0 & 423 & 8.5 & $f_2$ \\
\hline497 & 2D-M511 & 0.013 & 13.9 & 495 & 10.6 & $f_2$ \\
\hline498 & 2D-M418 & 0.0129 & 14.0 & 508 & 10.5 & $f_2$ \\
\hline499 & 2D-M350 & 0.0129 & 14.1 & 510 & 10.5 & $f_2$ \\
\hline500 & 2D-M370 & 0.0129 & 13.1 & 464 & 9.5 & $f_2$ \\
\hline501 & 2D-M339 & 0.0129 & 11.3 & 394 & 7.1 & $f_2$ \\
\hline502 & 2D-M347 & 0.0129 & 14.0 & 509 & 10.5 & $f_2$ \\
\hline503 & 2D-M479 & 0.0129 & 13.8 & 492 & 10.3 & $f_2$ \\
\hline504 & 2D-M287 & 0.0129 & 14.3 & 529 & 8.8 & $f_2$ \\
\hline505 & 2D-M19 & 0.0129 & 10.8 & 373 & 7.1 & $f_2$ \\
\hline506 & 2D-M470 & 0.0128 & 13.1 & 466 & 9.5 & $f_2$ \\
\hline507 & 2D-M506 & 0.0128 & 11.8 & 418 & 8.1 & $f_2$ \\
\hline508 & 2D-M437 & 0.0128 & 12.1 & 426 & 8.4 & $f_2$ \\
\hline509 & 2D-M401 & 0.0128 & 13.1 & 468 & 9.5 & $f_2$ \\
\hline510 & 2D-M338 & 0.0128 & 17.3 & 581 & 9.5 & $f_2$ \\
\hline511 & 2D-M464 & 0.0127 & 14.1 & 513 & 10.5 & $f_2$ \\
\hline512 & 2D-M433 & 0.0127 & 13.1 & 469 & 9.5 & $f_2$ \\
\hline513 & 2D-M423 & 0.0127 & 13.8 & 490 & 10.2 & $f_2$ \\
\hline514 & 2D-M472 & 0.0127 & 13.1 & 462 & 9.6 & $f_2$ \\
\hline515 & 2D-M336 & 0.0127 & 14.1 & 515 & 10.5 & $f_2$ \\
\hline516 & 2D-M321 & 0.0126 & 12.1 & 427 & 8.4 & $f_2$ \\
\hline517 & 2D-M380 & 0.0126 & 15.7 & 557 & 10.2 & $f_2$ \\
\hline518 & 2D-M335 & 0.0126 & 14.1 & 516 & 10.5 & $f_2$ \\
\hline519 & 2D-M21 & 0.0126 & 12.1 & 428 & 8.4 & $f_2$ \\
\hline520 & 2D-M345 & 0.0126 & 13.2 & 470 & 9.5 & $f_2$ \\
\hline521 & 2D-M367 & 0.0126 & 14.1 & 517 & 10.5 & $f_2$ \\
\hline522 & 2D-M25 & 0.0126 & 13.2 & 471 & 9.5 & $f_2$ \\
\hline523 & 2D-M320 & 0.0126 & 14.1 & 518 & 10.5 & $f_2$ \\
\hline524 & 2D-M30 & 0.0125 & 14.1 & 519 & 10.5 & $f_2$ \\
\hline525 & 2D-M323 & 0.0125 & 12.7 & 447 & 7.5 & $f_2$ \\
\hline526 & 2D-M428 & 0.0123 & 16.8 & 576 & 10.1 & $f_2$ \\
\hline527 & 2D-M496 & 0.0121 & 14.1 & 521 & 9.9 & $f_2$ \\
\hline528 & 2D-M455 & 0.0121 & 12.6 & 443 & 8.1 & $f_2$ \\
\hline529 & 2D-M330 & 0.0121 & 13.7 & 483 & 9.2 & $f_2$ \\
\hline530 & 2D-M449 & 0.0121 & 9.0 & 338 & 5.1 & $f_2$ \\
\hline531 & 2D-M169 & 0.012 & 10.6 & 364 & 8.1 & $f_2$ \\
\hline532 & 2D-M161 & 0.012 & 15.3 & 550 & 10.1 & $f_2$ \\
\hline533 & 2D-M402 & 0.0119 & 13.7 & 486 & 8.8 & $f_2$ \\
\hline534 & 2D-M446 & 0.0119 & 15.6 & 554 & 9.5 & $f_2$ \\
\hline535 & 2D-M429 & 0.0119 & 13.8 & 493 & 8.5 & $f_2$ \\
\hline536 & 2D-M358 & 0.0117 & 13.5 & 474 & 9.6 & $f_2$ \\
\hline537 & 2D-M275 & 0.0117 & 13.7 & 484 & 7.0 & $f_2$ \\
\hline538 & 2D-M272 & 0.0117 & 13.1 & 467 & 9.2 & $f_2$ \\
\hline539 & 2D-M327 & 0.0116 & 14.6 & 534 & 9.4 & $f_2$ \\
\hline540 & 2D-M322 & 0.0116 & 14.6 & 533 & 9.5 & $f_2$ \\
\hline541 & 2D-M490 & 0.0115 & 24.5 & 642 & 8.4 & $f_2$ \\
\hline542 & 2D-M505 & 0.0114 & 24.4 & 640 & 8.4 & $f_2$ \\
\hline543 & 2D-M13 & 0.0113 & 13.5 & 477 & 9.3 & $f_2$ \\
\hline544 & 2D-M18 & 0.0112 & 12.3 & 437 & 8.4 & $f_2$ \\
\hline545 & 2D-M432 & 0.0111 & 15.6 & 555 & 7.4 & $f_2$ \\
\hline546 & 2D-M341 & 0.011 & 17.3 & 592 & 2.9 & $f_2$ \\
\hline547 & 2D-M400 & 0.0109 & 26.1 & 644 & 7.8 & $f_2$ \\
\hline548 & 2D-M191 & 0.0108 & 15.3 & 552 & 8.0 & $f_2$ \\
\hline549 & 2D-M20 & 0.0107 & 8.7 & 332 & 6.6 & $f_2$ \\
\hline550 & 2D-M388 & 0.0107 & 17.3 & 591 & 2.9 & $f_2$ \\
\hline551 & 2D-M448 & 0.0105 & 12.2 & 432 & 5.8 & $f_2$ \\
\hline552 & 2D-M325 & 0.0104 & 16.7 & 571 & 8.1 & $f_2$ \\
\hline553 & 2D-M270 & 0.0098 & 16.7 & 570 & 6.6 & $f_2$ \\
\hline554 & 2D-M643 & 0.0091 & 14.8 & 539 & 10.5 & $f_1$ \\
\hline555 & 2D-M644 & 0.0091 & 14.8 & 540 & 10.5 & $f_1$ \\
\hline556 & 2D-M416 & 0.0088 & 25.6 & 643 & 7.1 & $f_2$ \\
\hline557 & 2D-M195 & 0.0085 & 16.7 & 569 & 4.9 & $f_2$ \\
\hline558 & 2D-M197 & 0.0084 & 13.6 & 480 & 4.5 & $f_2$ \\
\hline559 & 2D-M22 & 0.0082 & 18.9 & 614 & 6.1 & $f_2$ \\
\hline560 & 2D-M326 & 0.0079 & 16.4 & 564 & 5.8 & $f_2$ \\
\hline561 & 2D-M486 & 0.0079 & 16.4 & 565 & 5.8 & $f_2$ \\
\hline562 & 2D-M398 & 0.0078 & 27.4 & 645 & 6.4 & $f_2$ \\
\hline563 & 2D-M171 & 0.0077 & 16.1 & 559 & 4.5 & $f_2$ \\
\hline564 & 2D-M391 & 0.0073 & 20.2 & 631 & 3.4 & $f_2$ \\
\hline565 & 2D-M332 & 0.0066 & 19.0 & 616 & 5.5 & $f_2$ \\
\hline566 & 2D-M494 & 0.0062 & 21.2 & 637 & 5.1 & $f_2$ \\
\hline567 & 2D-M509 & 0.0057 & 19.7 & 620 & 4.8 & $f_2$ \\
\hline568 & 2D-M328 & 0.0055 & 17.5 & 600 & 3.5 & $f_2$ \\
\hline569 & 2D-M176 & 0.0041 & 16.8 & 574 & 2.7 & $f_2$ \\
\hline570 & 2D-M599 & 0.0028 & 1.0 & 53 & 1.0 & $f_2$ \\
\hline571 & 2D-M40 & 0.0026 & 1.7 & 304 & 1.7 & $f_2$ \\
\hline572 & 2D-M469 & 0.0021 & 1.1 & 106 & 1.1 & $f_2$ \\
\hline573 & 2D-M483 & 0.002 & 1.1 & 79 & 1.0 & $f_2$ \\
\hline574 & 2D-M565 & 0.002 & 1.0 & 50 & 1.0 & $f_2$ \\
\hline575 & 2D-M36 & 0.002 & 1.4 & 238 & 1.4 & $f_2$ \\
\hline576 & 2D-M560 & 0.0019 & 1.2 & 147 & 1.2 & $f_2$ \\
\hline577 & 2D-M573 & 0.0018 & 1.2 & 146 & 1.2 & $f_2$ \\
\hline578 & 2D-M441 & 0.0017 & 1.1 & 124 & 1.1 & $f_2$ \\
\hline579 & 2D-M39 & 0.0017 & 1.2 & 165 & 1.2 & $f_2$ \\
\hline580 & 2D-M563 & 0.0017 & 1.1 & 94 & 1.1 & $f_2$ \\
\hline581 & 2D-M576 & 0.0017 & 1.1 & 85 & 1.1 & $f_2$ \\
\hline582 & 2D-M575 & 0.0017 & 1.1 & 87 & 1.1 & $f_2$ \\
\hline583 & 2D-M587 & 0.0017 & 1.1 & 91 & 1.1 & $f_2$ \\
\hline584 & 2D-M615 & 0.0016 & 1.0 & 71 & 1.0 & $f_2$ \\
\hline585 & 2D-M588 & 0.0016 & 1.1 & 86 & 1.1 & $f_2$ \\
\hline586 & 2D-M34 & 0.0016 & 1.5 & 261 & 1.0 & $f_2$ \\
\hline587 & 2D-M493 & 0.0016 & 1.1 & 90 & 1.1 & $f_2$ \\
\hline588 & 2D-M574 & 0.0016 & 1.0 & 12 & 1.0 & $f_2$ \\
\hline589 & 2D-M467 & 0.0016 & 1.1 & 126 & 1.1 & $f_2$ \\
\hline590 & 2D-M571 & 0.0016 & 1.0 & 2 & 1.0 & $f_2$ \\
\hline591 & 2D-M592 & 0.0016 & 1.7 & 299 & 1.0 & $f_2$ \\
\hline592 & 2D-M577 & 0.0015 & 1.2 & 138 & 0.9 & $f_2$ \\
\hline593 & 2D-M605 & 0.0015 & 1.1 & 89 & 1.1 & $f_2$ \\
\hline594 & 2D-M604 & 0.0015 & 1.1 & 88 & 1.1 & $f_2$ \\
\hline595 & 2D-M594 & 0.0015 & 1.0 & 8 & 1.0 & $f_2$ \\
\hline596 & 2D-M598 & 0.0015 & 1.0 & 24 & 1.0 & $f_2$ \\
\hline597 & 2D-M610 & 0.0015 & 1.0 & 3 & 1 & $f_2$ \\
\hline598 & 2D-M602 & 0.0015 & 1.0 & 60 & 1.0 & $f_2$ \\
\hline599 & 2D-M590 & 0.0015 & 1.0 & 59 & 1.0 & $f_2$ \\
\hline600 & 2D-M586 & 0.0015 & 1.0 & 58 & 1.0 & $f_2$ \\
\hline601 & 2D-M564 & 0.0015 & 1.0 & 55 & 1.0 & $f_2$ \\
\hline602 & 2D-M603 & 0.0015 & 1.0 & 54 & 1.0 & $f_2$ \\
\hline603 & 2D-M618 & 0.0015 & 1.0 & 29 & 1.0 & $f_2$ \\
\hline604 & 2D-M457 & 0.0015 & 1.4 & 229 & 1.1 & $f_2$ \\
\hline605 & 2D-M585 & 0.0015 & 1.0 & 23 & 1.0 & $f_2$ \\
\hline606 & 2D-M569 & 0.0015 & 1.0 & 17 & 1.0 & $f_2$ \\
\hline607 & 2D-M596 & 0.0014 & 1.0 & 21 & 1.0 & $f_2$ \\
\hline608 & 2D-M567 & 0.0014 & 1.0 & 19 & 1.0 & $f_2$ \\
\hline609 & 2D-M570 & 0.0014 & 1.0 & 1 & 1.0 & $f_2$ \\
\hline610 & 2D-M606 & 0.0014 & 1.0 & 25 & 1.0 & $f_2$ \\
\hline611 & 2D-M595 & 0.0014 & 1.0 & 63 & 1.0 & $f_2$ \\
\hline612 & 2D-M583 & 0.0014 & 1.0 & 65 & 1.0 & $f_2$ \\
\hline613 & 2D-M562 & 0.0014 & 1.0 & 64 & 1.0 & $f_2$ \\
\hline614 & 2D-M600 & 0.0014 & 1.0 & 4 & 1.0 & $f_2$ \\
\hline615 & 2D-M619 & 0.0014 & 1.4 & 235 & 1.0 & $f_2$ \\
\hline616 & 2D-M614 & 0.0014 & 1.4 & 234 & 1.0 & $f_2$ \\
\hline617 & 2D-M459 & 0.0014 & 1.0 & 77 & 1.0 & $f_2$ \\
\hline618 & 2D-M33 & 0.0013 & 1.4 & 237 & 1.1 & $f_2$ \\
\hline619 & 2D-M445 & 0.0012 & 1.1 & 110 & 0.8 & $f_2$ \\
\hline620 & 2D-M444 & 0.0012 & 1.5 & 274 & 0.9 & $f_2$ \\
\hline621 & 2D-M37 & 0.0012 & 1.2 & 166 & 0.8 & $f_2$ \\
\hline622 & 2D-M38 & 0.0012 & 1.2 & 167 & 0.8 & $f_2$ \\
\hline623 & 2D-M443 & 0.0012 & 1.2 & 170 & 0.7 & $f_2$ \\
\hline624 & 2D-M440 & 0.0012 & 2.6 & 322 & 0.9 & $f_2$ \\
\hline625 & 2D-M593 & 0.0012 & 1.3 & 200 & 0.8 & $f_2$ \\
\hline626 & 2D-M611 & 0.001 & 1.4 & 232 & 0.6 & $f_2$ \\
\hline627 & 2D-M481 & 0.001 & 1.0 & 69 & 0.7 & $f_2$ \\
\hline628 & 2D-M616 & 0.001 & 1.6 & 289 & 0.6 & $f_2$ \\
\hline629 & 2D-M442 & 0.001 & 2.2 & 317 & 0.6 & $f_2$ \\
\hline630 & 2D-M568 & 0.0009 & 1.3 & 187 & 0.6 & $f_2$ \\
\hline631 & 2D-M582 & 0.0009 & 1.3 & 196 & 0.6 & $f_2$ \\
\hline632 & 2D-M617 & 0.0009 & 1.3 & 188 & 0.6 & $f_2$ \\
\hline633 & 2D-M580 & 0.0009 & 1.3 & 186 & 0.6 & $f_2$ \\
\hline634 & 2D-M561 & 0.0009 & 2.6 & 323 & 0.6 & $f_2$ \\
\hline635 & 2D-M578 & 0.0008 & 1.5 & 275 & 0.5 & $f_2$ \\
\hline636 & 2D-M566 & 0.0008 & 1.4 & 252 & 0.5 & $f_2$ \\
\hline637 & 2D-M608 & 0.0008 & 1.4 & 251 & 0.5 & $f_2$ \\
\hline638 & 2D-M581 & 0.0008 & 1.3 & 210 & 0.6 & $f_2$ \\
\hline639 & 2D-M584 & 0.0007 & 1.4 & 250 & 0.5 & $f_2$ \\
\hline640 & 2D-M612 & 0.0007 & 1.4 & 245 & 0.5 & $f_2$ \\
\hline641 & 2D-M579 & 0.0007 & 1.4 & 243 & 0.5 & $f_2$ \\
\hline642 & 2D-M591 & 0.0007 & 1.4 & 256 & 0.5 & $f_2$ \\
\hline643 & 2D-M572 & 0.0007 & 1.4 & 239 & 0.5 & $f_2$ \\
\hline644 & 2D-M491 & 0.0007 & 1.3 & 203 & 0.5 & $f_2$ \\
\hline645 & 2D-M607 & 0.0006 & 1.6 & 282 & 0.4 & $f_2$ \\
\hline
%\caption{Manipulability of 1-DOF Manipulators}
%\label{Tab:table_dof1mt_1}

\end{supertabular}
\end{center}

%\end{longtable}

\normalsize

==> contentfolder/mechanisms2/manipulabilitytable3.tex <==
\begin{table}[h]  \centering \begin{tabular}{||c|c|c|c|c|c|c||}
\hline
S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ \\ 
\hline
1 & 3D-M1 & 1.0113 & 1.5 & 2 & 1058.9 & $f_1$ \\
\hline2 & 3D-M8 & 1.0 & 1.0 & 1 & 1.0 & $f_1$ \\
\hline3 & 3D-M2 & 0.0962 & 14.8 & 4 & 111.0 & $f_1$ \\
\hline4 & 3D-M3 & 0.0962 & 15.5 & 8 & 111.0 & $f_1$ \\
\hline5 & 3D-M4 & 0.0962 & 14.8 & 7 & 111.0 & $f_1$ \\
\hline6 & 3D-M7 & 0.0091 & 14.8 & 5 & 10.5 & $f_1$ \\
\hline7 & 3D-M5 & 0.0091 & 14.8 & 6 & 10.5 & $f_1$ \\
\hline8 & 3D-M6 & 0.0091 & 14.8 & 3 & 10.5 & $f_1$ \\
\hline\end{tabular} \caption{Prescription of 3-DOF Manipulators} \label{Tab:table_dof3mt_1} \end{table}

==> contentfolder/mechanisms2/manipulabilitytable4.tex <==
\begin{table}[h]  \centering \begin{tabular}{||c|c|c|c|c|c|c||}
\hline
S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ \\ 
\hline
1 & 4D-M1 & 2.5607 & 1.5 & 1 & 2074.5 & $f_1$ \\
\hline2 & 4D-M13 & 0.4866 & 3.0 & 2 & 1.0 & $f_1$ \\
\hline3 & 4D-M12 & 0.4048 & 3.1 & 3 & 1 & $f_1$ \\
\hline4 & 4D-M4 & 0.2619 & 15.3 & 14 & 211.0 & $f_1$ \\
\hline5 & 4D-M5 & 0.2619 & 15.3 & 13 & 211.0 & $f_1$ \\
\hline6 & 4D-M2 & 0.2619 & 15.3 & 12 & 211.0 & $f_1$ \\
\hline7 & 4D-M3 & 0.2619 & 15.3 & 15 & 211.0 & $f_1$ \\
\hline8 & 4D-M15 & 0.077 & 4.9 & 4 & 1.0 & $f_1$ \\
\hline9 & 4D-M14 & 0.0538 & 5.5 & 5 & 1.0 & $f_1$ \\
\hline10 & 4D-M9 & 0.0253 & 12.9 & 7 & 17.6 & $f_1$ \\
\hline11 & 4D-M11 & 0.0253 & 12.9 & 10 & 17.6 & $f_1$ \\
\hline12 & 4D-M10 & 0.0253 & 12.9 & 6 & 17.6 & $f_1$ \\
\hline13 & 4D-M7 & 0.0253 & 12.9 & 8 & 17.6 & $f_1$ \\
\hline14 & 4D-M8 & 0.0253 & 12.9 & 9 & 17.6 & $f_1$ \\
\hline15 & 4D-M6 & 0.0253 & 12.9 & 11 & 17.6 & $f_1$ \\
\hline\end{tabular} \caption{Prescription of 4-DOF Manipulators} \label{Tab:table_dof4mt_1} \end{table}

==> contentfolder/mechanisms2/manipulabilitytable_new1.tex <==
\begin{longtable}{||c|c|c|c|c||c|c|c|c|c||}
\hline
S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ & S.No. & Name & $\bar{\mu}$ & $\mu$ & $f$ \\ 
\hline
1 & 1D-M10 & 0.1523 & 8.1 & $f_1$ & 49 & 1D-M89 & 0.0155 & 1 & $f_1$ \\
\hline2 & 1D-M65 & 0.1376 & 10.5 & $f_2$ & 50 & 1D-M38 & 0.0153 & 12.9 & $f_2$ \\
\hline3 & 1D-M8 & 0.1152 & 7.1 & $f_1$ & 51 & 1D-M58 & 0.0148 & 8.2 & $f_2$ \\
\hline4 & 1D-M94 & 0.1106 & 1.0 & $f_2$ & 52 & 1D-M57 & 0.0143 & 11.7 & $f_2$ \\
\hline5 & 1D-M28 & 0.1088 & 8.1 & $f_1$ & 53 & 1D-M76 & 0.0138 & 1 & $f_1$ \\
\hline6 & 1D-M20 & 0.0824 & 10.5 & $f_1$ & 54 & 1D-M17 & 0.0136 & 8.6 & $f_2$ \\
\hline7 & 1D-M34 & 0.0798 & 7.1 & $f_1$ & 55 & 1D-M50 & 0.0135 & 11.1 & $f_2$ \\
\hline8 & 1D-M95 & 0.0776 & 1.0 & $f_2$ & 56 & 1D-M19 & 0.0134 & 10.3 & $f_2$ \\
\hline9 & 1D-M7 & 0.0774 & 8.4 & $f_1$ & 57 & 1D-M56 & 0.0129 & 10.5 & $f_2$ \\
\hline10 & 1D-M29 & 0.0732 & 10.5 & $f_1$ & 58 & 1D-M21 & 0.0128 & 10.5 & $f_2$ \\
\hline11 & 1D-M41 & 0.0722 & 9.5 & $f_1$ & 59 & 1D-M27 & 0.0127 & 9.3 & $f_2$ \\
\hline12 & 1D-M40 & 0.071 & 7.1 & $f_1$ & 60 & 1D-M77 & 0.0126 & 1 & $f_1$ \\
\hline13 & 1D-M35 & 0.0706 & 10.5 & $f_1$ & 61 & 1D-M16 & 0.0125 & 9.3 & $f_2$ \\
\hline14 & 1D-M11 & 0.062 & 10.5 & $f_1$ & 62 & 1D-M2 & 0.0116 & 6.7 & $f_2$ \\
\hline15 & 1D-M64 & 0.0563 & 20.3 & $f_2$ & 63 & 1D-M1 & 0.0113 & 8.4 & $f_2$ \\
\hline16 & 1D-M66 & 0.0487 & 19.8 & $f_2$ & 64 & 1D-M43 & 0.0108 & 1 & $f_1$ \\
\hline17 & 1D-M60 & 0.0475 & 8.4 & $f_1$ & 65 & 1D-M39 & 0.01 & 8.5 & $f_2$ \\
\hline18 & 1D-M93 & 0.0467 & 1.0 & $f_2$ & 66 & 1D-M80 & 0.0082 & 1 & $f_1$ \\
\hline19 & 1D-M59 & 0.0462 & 9.5 & $f_1$ & 67 & 1D-M36 & 0.0081 & 1 & $f_1$ \\
\hline20 & 1D-M91 & 0.0438 & 1.0 & $f_2$ & 68 & 1D-M92 & 0.0071 & 1 & $f_1$ \\
\hline21 & 1D-M79 & 0.0335 & 1 & $f_1$ & 69 & 1D-M61 & 0.0051 & 1 & $f_1$ \\
\hline22 & 1D-M25 & 0.0313 & 17.3 & $f_2$ & 70 & 1D-M42 & 0.0034 & 1 & $f_1$ \\
\hline23 & 1D-M44 & 0.0313 & 17.3 & $f_2$ & 71 & 1D-M31 & 0.0031 & 1.7 & $f_2$ \\
\hline24 & 1D-M67 & 0.0306 & 18.3 & $f_2$ & 72 & 1D-M37 & 0.0025 & 1 & $f_1$ \\
\hline25 & 1D-M15 & 0.0305 & 21.2 & $f_2$ & 73 & 1D-M86 & 0.0021 & 1.0 & $f_2$ \\
\hline26 & 1D-M22 & 0.0246 & 17.3 & $f_2$ & 74 & 1D-M30 & 0.002 & 1.1 & $f_2$ \\
\hline27 & 1D-M13 & 0.024 & 15.3 & $f_2$ & 75 & 1D-M53 & 0.0017 & 1.1 & $f_2$ \\
\hline28 & 1D-M46 & 0.0237 & 15.3 & $f_2$ & 76 & 1D-M83 & 0.0016 & 1.0 & $f_2$ \\
\hline29 & 1D-M45 & 0.0229 & 17.3 & $f_2$ & 77 & 1D-M84 & 0.0015 & 1.0 & $f_2$ \\
\hline30 & 1D-M3 & 0.0222 & 15.4 & $f_2$ & 78 & 1D-M87 & 0.0015 & 1.0 & $f_2$ \\
\hline31 & 1D-M49 & 0.0219 & 14.1 & $f_2$ & 79 & 1D-M55 & 0.0015 & 1.3 & $f_2$ \\
\hline32 & 1D-M68 & 0.0214 & 19.6 & $f_2$ & 80 & 1D-M71 & 0.0015 & 1.0 & $f_2$ \\
\hline33 & 1D-M5 & 0.0212 & 14.7 & $f_2$ & 81 & 1D-M73 & 0.0015 & 1.0 & $f_2$ \\
\hline34 & 1D-M47 & 0.0212 & 17.3 & $f_2$ & 82 & 1D-M90 & 0.0015 & 1.0 & $f_2$ \\
\hline35 & 1D-M24 & 0.0212 & 17.3 & $f_2$ & 83 & 1D-M52 & 0.0015 & 1.1 & $f_2$ \\
\hline36 & 1D-M51 & 0.0203 & 14.9 & $f_2$ & 84 & 1D-M82 & 0.0014 & 1.0 & $f_2$ \\
\hline37 & 1D-M18 & 0.0194 & 14.6 & $f_2$ & 85 & 1D-M72 & 0.0014 & 1 & $f_2$ \\
\hline38 & 1D-M69 & 0.019 & 19.0 & $f_2$ & 86 & 1D-M70 & 0.0014 & 1.0 & $f_2$ \\
\hline39 & 1D-M48 & 0.0189 & 14.0 & $f_2$ & 87 & 1D-M81 & 0.0014 & 1 & $f_2$ \\
\hline40 & 1D-M12 & 0.0188 & 12.8 & $f_2$ & 88 & 1D-M85 & 0.0014 & 1.0 & $f_2$ \\
\hline41 & 1D-M9 & 0.0185 & 12.8 & $f_2$ & 89 & 1D-M88 & 0.0014 & 1.0 & $f_2$ \\
\hline42 & 1D-M23 & 0.0177 & 13.0 & $f_2$ & 90 & 1D-M63 & 0.0013 & 1.1 & $f_2$ \\
\hline43 & 1D-M62 & 0.0167 & 9.6 & $f_2$ & 91 & 1D-M32 & 0.0013 & 0.7 & $f_2$ \\
\hline44 & 1D-M26 & 0.0167 & 9.6 & $f_2$ & 92 & 1D-M54 & 0.0013 & 1.1 & $f_2$ \\
\hline45 & 1D-M14 & 0.0163 & 10.1 & $f_2$ & 93 & 1D-M33 & 0.0012 & 0.8 & $f_2$ \\
\hline46 & 1D-M96 & 0.016 & 1.0 & $f_2$ & 94 & 1D-M78 & 0.0009 & 0.6 & $f_2$ \\
\hline47 & 1D-M6 & 0.0159 & 12.0 & $f_2$ & 95 & 1D-M74 & 0.0008 & 0.6 & $f_2$ \\
\hline48 & 1D-M4 & 0.0158 & 13.4 & $f_2$ & 96 & 1D-M75 & 0.0006 & 0.4 & $f_2$ \\
\hline
\caption{Manipulability of 1-DOF Manipulators}
\label{Tab:table_dof1mt_1} \end{longtable}



==> contentfolder/mechanisms2/manipulabilitytable_new2.tex <==
%\resizebox{\linewidth}{!}{
\footnotesize
\begin{longtable}{||c|c|c|c|c|c|c||c|c|c|c|c|c|c||}

\hline
S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ & S.No. & Name & $\bar{\mu}$ & $\kappa$ & $i_{\kappa}$ & $\mu$ & $f$ \\ 
\hline
1 & 2D-M645 & 1.0 & 1.0 & 6 & 1.0 & $f_1$ & 324 & 2D-M172 & 0.0289 & 17.5 & 601 & 15.1 & $f_2$ \\
\hline2 & 2D-M315 & 0.7544 & 1.2 & 155 & 87.4 & $f_1$ & 325 & 2D-M205 & 0.028 & 14.6 & 535 & 18.9 & $f_2$ \\
\hline3 & 2D-M301 & 0.7058 & 1.2 & 158 & 88.8 & $f_2$ & 326 & 2D-M394 & 0.0271 & 12.8 & 451 & 8.6 & $f_2$ \\
\hline4 & 2D-M224 & 0.6366 & 1.1 & 127 & 60.2 & $f_1$ & 327 & 2D-M520 & 0.027 & 19.4 & 618 & 18.1 & $f_2$ \\
\hline5 & 2D-M308 & 0.6034 & 1.1 & 118 & 340.6 & $f_2$ & 328 & 2D-M421 & 0.0268 & 17.3 & 586 & 17.3 & $f_2$ \\
\hline6 & 2D-M126 & 0.5855 & 1.3 & 207 & 88.8 & $f_1$ & 329 & 2D-M360 & 0.0268 & 17.3 & 582 & 17.3 & $f_2$ \\
\hline7 & 2D-M309 & 0.5624 & 1.2 & 135 & 351.6 & $f_2$ & 330 & 2D-M413 & 0.0267 & 13.2 & 472 & 12.9 & $f_2$ \\
\hline8 & 2D-M319 & 0.5621 & 1.4 & 230 & 283.4 & $f_2$ & 331 & 2D-M355 & 0.0266 & 14.1 & 523 & 14.1 & $f_2$ \\
\hline9 & 2D-M208 & 0.5495 & 1.2 & 172 & 68.1 & $f_1$ & 332 & 2D-M349 & 0.0263 & 14.6 & 536 & 14.5 & $f_2$ \\
\hline10 & 2D-M134 & 0.541 & 1.1 & 107 & 100.5 & $f_1$ & 333 & 2D-M508 & 0.0263 & 17.6 & 606 & 16.4 & $f_2$ \\
\hline11 & 2D-M248 & 0.5381 & 1.4 & 224 & 75.2 & $f_1$ & 334 & 2D-M407 & 0.0261 & 14.9 & 541 & 14.9 & $f_2$ \\
\hline12 & 2D-M203 & 0.5289 & 1.3 & 198 & 68.1 & $f_1$ & 335 & 2D-M389 & 0.026 & 17.4 & 594 & 6.4 & $f_2$ \\
\hline13 & 2D-M634 & 0.5142 & 1.0 & 7 & 1 & $f_1$ & 336 & 2D-M424 & 0.0259 & 16.1 & 561 & 18.4 & $f_2$ \\
\hline14 & 2D-M458 & 0.5116 & 1.0 & 32 & 1.0 & $f_1$ & 337 & 2D-M450 & 0.0258 & 13.1 & 460 & 13.0 & $f_2$ \\
\hline15 & 2D-M74 & 0.5114 & 1.1 & 115 & 77.5 & $f_1$ & 338 & 2D-M534 & 0.0254 & 19.9 & 624 & 18.6 & $f_2$ \\
\hline16 & 2D-M318 & 0.5006 & 1.1 & 130 & 298.9 & $f_2$ & 339 & 2D-M548 & 0.0253 & 19.0 & 615 & 17.8 & $f_2$ \\
\hline17 & 2D-M213 & 0.4948 & 1.3 & 183 & 60.2 & $f_1$ & 340 & 2D-M387 & 0.0245 & 17.3 & 590 & 6.4 & $f_2$ \\
\hline18 & 2D-M304 & 0.4879 & 1.8 & 307 & 165.1 & $f_2$ & 341 & 2D-M412 & 0.0244 & 13.1 & 463 & 13.1 & $f_2$ \\
\hline19 & 2D-M311 & 0.485 & 1.2 & 152 & 88.5 & $f_1$ & 342 & 2D-M543 & 0.0241 & 18.5 & 610 & 18.0 & $f_2$ \\
\hline20 & 2D-M300 & 0.4831 & 2.1 & 316 & 144.2 & $f_2$ & 343 & 2D-M556 & 0.024 & 20.4 & 633 & 18.6 & $f_2$ \\
\hline21 & 2D-M314 & 0.4683 & 1.2 & 141 & 266.1 & $f_2$ & 344 & 2D-M346 & 0.0239 & 14.8 & 538 & 12.3 & $f_2$ \\
\hline22 & 2D-M303 & 0.4571 & 1.6 & 294 & 181.6 & $f_2$ & 345 & 2D-M475 & 0.0238 & 17.0 & 578 & 17.5 & $f_2$ \\
\hline23 & 2D-M305 & 0.4477 & 1.5 & 266 & 200.5 & $f_2$ & 346 & 2D-M288 & 0.0238 & 15.0 & 543 & 14.8 & $f_2$ \\
\hline24 & 2D-M98 & 0.4435 & 1.3 & 180 & 88.8 & $f_1$ & 347 & 2D-M507 & 0.0235 & 17.3 & 588 & 17.3 & $f_2$ \\
\hline25 & 2D-M302 & 0.4376 & 1.8 & 306 & 164.6 & $f_2$ & 348 & 2D-M348 & 0.0235 & 17.3 & 587 & 17.3 & $f_2$ \\
\hline26 & 2D-M299 & 0.4327 & 1.7 & 298 & 192.7 & $f_2$ & 349 & 2D-M163 & 0.0234 & 13.7 & 481 & 12.6 & $f_2$ \\
\hline27 & 2D-M86 & 0.4221 & 1.2 & 136 & 100.5 & $f_1$ & 350 & 2D-M242 & 0.023 & 18.4 & 609 & 13.8 & $f_2$ \\
\hline28 & 2D-M11 & 0.4196 & 1.1 & 117 & 60.2 & $f_1$ & 351 & 2D-M550 & 0.023 & 19.1 & 617 & 17.7 & $f_2$ \\
\hline29 & 2D-M313 & 0.418 & 1.1 & 108 & 232.3 & $f_2$ & 352 & 2D-M24 & 0.0228 & 14.5 & 532 & 12.1 & $f_2$ \\
\hline30 & 2D-M312 & 0.4138 & 1.2 & 148 & 253.8 & $f_2$ & 353 & 2D-M425 & 0.0226 & 14.1 & 522 & 14.1 & $f_2$ \\
\hline31 & 2D-M239 & 0.3908 & 1.1 & 104 & 80.4 & $f_1$ & 354 & 2D-M357 & 0.0223 & 17.4 & 595 & 16.9 & $f_2$ \\
\hline32 & 2D-M317 & 0.3621 & 1.2 & 131 & 294.7 & $f_2$ & 355 & 2D-M535 & 0.0222 & 19.8 & 623 & 18.4 & $f_2$ \\
\hline33 & 2D-M237 & 0.3503 & 1.1 & 114 & 100.5 & $f_1$ & 356 & 2D-M406 & 0.0222 & 13.9 & 494 & 15.1 & $f_2$ \\
\hline34 & 2D-M132 & 0.3441 & 1.4 & 228 & 88.8 & $f_1$ & 357 & 2D-M156 & 0.0222 & 16.8 & 572 & 13.6 & $f_2$ \\
\hline35 & 2D-M232 & 0.3306 & 1.2 & 157 & 88.8 & $f_1$ & 358 & 2D-M252 & 0.0219 & 20.3 & 632 & 14.3 & $f_2$ \\
\hline36 & 2D-M227 & 0.3291 & 1.0 & 70 & 204.1 & $f_2$ & 359 & 2D-M628 & 0.0217 & 1.0 & 26 & 1.0 & $f_2$ \\
\hline37 & 2D-M286 & 0.3224 & 1.1 & 122 & 194.5 & $f_2$ & 360 & 2D-M366 & 0.0215 & 13.0 & 458 & 12.9 & $f_2$ \\
\hline38 & 2D-M138 & 0.3142 & 1.1 & 111 & 100.5 & $f_1$ & 361 & 2D-M343 & 0.0215 & 12.1 & 429 & 7.8 & $f_2$ \\
\hline39 & 2D-M226 & 0.3127 & 1.5 & 269 & 176.2 & $f_2$ & 362 & 2D-M155 & 0.0215 & 16.3 & 563 & 13.9 & $f_2$ \\
\hline40 & 2D-M307 & 0.3125 & 1.5 & 281 & 186.7 & $f_2$ & 363 & 2D-M194 & 0.0214 & 16.3 & 562 & 13.6 & $f_2$ \\
\hline41 & 2D-M306 & 0.2991 & 1.5 & 259 & 212.1 & $f_2$ & 364 & 2D-M502 & 0.0214 & 17.3 & 584 & 17.3 & $f_2$ \\
\hline42 & 2D-M310 & 0.2946 & 1.6 & 290 & 138.7 & $f_2$ & 365 & 2D-M374 & 0.0214 & 17.3 & 583 & 17.3 & $f_2$ \\
\hline43 & 2D-M521 & 0.2929 & 8.9 & 334 & 8.4 & $f_1$ & 366 & 2D-M192 & 0.0213 & 16.1 & 560 & 13.2 & $f_2$ \\
\hline44 & 2D-M145 & 0.2902 & 1.4 & 240 & 142.5 & $f_2$ & 367 & 2D-M354 & 0.021 & 17.0 & 577 & 14.6 & $f_2$ \\
\hline45 & 2D-M234 & 0.2884 & 1.1 & 120 & 162.0 & $f_2$ & 368 & 2D-M168 & 0.0209 & 14.0 & 498 & 12.5 & $f_2$ \\
\hline46 & 2D-M59 & 0.2879 & 1.5 & 276 & 189.0 & $f_2$ & 369 & 2D-M353 & 0.0208 & 14.3 & 531 & 11.8 & $f_2$ \\
\hline47 & 2D-M128 & 0.2829 & 1.2 & 133 & 60.2 & $f_1$ & 370 & 2D-M465 & 0.0205 & 14.0 & 506 & 14.0 & $f_2$ \\
\hline48 & 2D-M187 & 0.2736 & 1.3 & 204 & 220.1 & $f_2$ & 371 & 2D-M363 & 0.0203 & 15.1 & 545 & 15.1 & $f_2$ \\
\hline49 & 2D-M293 & 0.273 & 1.3 & 192 & 182.5 & $f_2$ & 372 & 2D-M160 & 0.0202 & 15.2 & 548 & 15.1 & $f_2$ \\
\hline50 & 2D-M118 & 0.273 & 1.3 & 191 & 182.5 & $f_2$ & 373 & 2D-M17 & 0.0202 & 14.1 & 511 & 14.8 & $f_2$ \\
\hline51 & 2D-M135 & 0.273 & 1.3 & 190 & 182.5 & $f_2$ & 374 & 2D-M484 & 0.0201 & 13.0 & 456 & 10.3 & $f_2$ \\
\hline52 & 2D-M256 & 0.2719 & 1.1 & 84 & 100.5 & $f_1$ & 375 & 2D-M375 & 0.0199 & 10.9 & 378 & 10.9 & $f_2$ \\
\hline53 & 2D-M184 & 0.271 & 2.0 & 314 & 164.8 & $f_2$ & 376 & 2D-M415 & 0.0198 & 15.0 & 542 & 13.4 & $f_2$ \\
\hline54 & 2D-M140 & 0.2705 & 1.1 & 119 & 75.9 & $f_1$ & 377 & 2D-M361 & 0.0195 & 11.4 & 398 & 11.4 & $f_2$ \\
\hline55 & 2D-M209 & 0.2696 & 1.4 & 223 & 165.2 & $f_2$ & 378 & 2D-M411 & 0.0194 & 15.0 & 544 & 15.3 & $f_2$ \\
\hline56 & 2D-M236 & 0.2691 & 1.9 & 312 & 149.1 & $f_2$ & 379 & 2D-M170 & 0.0194 & 15.7 & 556 & 11.6 & $f_2$ \\
\hline57 & 2D-M282 & 0.2688 & 1.7 & 300 & 167.5 & $f_2$ & 380 & 2D-M164 & 0.0192 & 12.7 & 444 & 8.7 & $f_2$ \\
\hline58 & 2D-M9 & 0.2678 & 1.2 & 153 & 100.5 & $f_1$ & 381 & 2D-M362 & 0.0192 & 12.5 & 442 & 9.6 & $f_2$ \\
\hline59 & 2D-M182 & 0.2677 & 1.2 & 171 & 168.8 & $f_2$ & 382 & 2D-M230 & 0.0191 & 13.7 & 485 & 12.3 & $f_2$ \\
\hline60 & 2D-M144 & 0.2665 & 1.3 & 216 & 112.8 & $f_2$ & 383 & 2D-M228 & 0.0191 & 12.9 & 452 & 12.9 & $f_2$ \\
\hline61 & 2D-M295 & 0.2587 & 1.2 & 174 & 119.2 & $f_2$ & 384 & 2D-M16 & 0.0184 & 15.6 & 553 & 10.3 & $f_2$ \\
\hline62 & 2D-M524 & 0.2581 & 9.0 & 335 & 8.4 & $f_2$ & 385 & 2D-M267 & 0.0184 & 11.6 & 405 & 12.4 & $f_2$ \\
\hline63 & 2D-M316 & 0.256 & 1.2 & 175 & 168.8 & $f_2$ & 386 & 2D-M376 & 0.0184 & 11.4 & 399 & 10.1 & $f_2$ \\
\hline64 & 2D-M285 & 0.2533 & 1.1 & 80 & 174.6 & $f_2$ & 387 & 2D-M410 & 0.0183 & 16.5 & 567 & 13.8 & $f_2$ \\
\hline65 & 2D-M217 & 0.2526 & 1.6 & 284 & 126.4 & $f_2$ & 388 & 2D-M193 & 0.0181 & 10.8 & 370 & 9.6 & $f_2$ \\
\hline66 & 2D-M116 & 0.2519 & 1.6 & 295 & 123.7 & $f_2$ & 389 & 2D-M378 & 0.0181 & 14.7 & 537 & 12.7 & $f_2$ \\
\hline67 & 2D-M264 & 0.2518 & 7.7 & 325 & 7.1 & $f_1$ & 390 & 2D-M278 & 0.0181 & 16.1 & 558 & 10.6 & $f_2$ \\
\hline68 & 2D-M152 & 0.2506 & 1.1 & 116 & 162.4 & $f_2$ & 391 & 2D-M158 & 0.0179 & 15.3 & 551 & 12.9 & $f_2$ \\
\hline69 & 2D-M87 & 0.2471 & 1.4 & 227 & 132.4 & $f_2$ & 392 & 2D-M456 & 0.0178 & 19.8 & 621 & 13.2 & $f_2$ \\
\hline70 & 2D-M522 & 0.2466 & 7.7 & 326 & 7.1 & $f_2$ & 393 & 2D-M344 & 0.0178 & 13.0 & 454 & 10.0 & $f_2$ \\
\hline71 & 2D-M82 & 0.2439 & 1.2 & 173 & 88.8 & $f_1$ & 394 & 2D-M175 & 0.0177 & 18.9 & 613 & 10.5 & $f_2$ \\
\hline72 & 2D-M88 & 0.2418 & 1.3 & 179 & 182.1 & $f_2$ & 395 & 2D-M474 & 0.0177 & 10.9 & 375 & 10.9 & $f_2$ \\
\hline73 & 2D-M298 & 0.2387 & 1.5 & 265 & 202.0 & $f_2$ & 396 & 2D-M430 & 0.0175 & 10.4 & 358 & 11.7 & $f_2$ \\
\hline74 & 2D-M526 & 0.2381 & 7.7 & 327 & 7.1 & $f_2$ & 397 & 2D-M497 & 0.0174 & 20.4 & 634 & 13.0 & $f_2$ \\
\hline75 & 2D-M215 & 0.2377 & 1.4 & 241 & 100.5 & $f_1$ & 398 & 2D-M28 & 0.0174 & 14.1 & 524 & 14.1 & $f_2$ \\
\hline76 & 2D-M143 & 0.2369 & 1.1 & 82 & 210.2 & $f_2$ & 399 & 2D-M26 & 0.0174 & 14.1 & 525 & 14.1 & $f_2$ \\
\hline77 & 2D-M113 & 0.2355 & 1.4 & 226 & 101.2 & $f_2$ & 400 & 2D-M372 & 0.0173 & 10.9 & 376 & 10.9 & $f_2$ \\
\hline78 & 2D-M61 & 0.233 & 1.8 & 305 & 113.4 & $f_2$ & 401 & 2D-M485 & 0.0173 & 20.8 & 635 & 9.5 & $f_2$ \\
\hline79 & 2D-M546 & 0.2319 & 7.7 & 328 & 7.1 & $f_2$ & 402 & 2D-M460 & 0.0171 & 12.4 & 439 & 9.4 & $f_2$ \\
\hline80 & 2D-M43 & 0.2307 & 1.4 & 246 & 135.8 & $f_2$ & 403 & 2D-M503 & 0.017 & 15.2 & 547 & 12.3 & $f_2$ \\
\hline81 & 2D-M71 & 0.2305 & 2.0 & 313 & 173.2 & $f_2$ & 404 & 2D-M439 & 0.017 & 15.2 & 546 & 12.3 & $f_2$ \\
\hline82 & 2D-M181 & 0.2289 & 1.3 & 219 & 142.6 & $f_2$ & 405 & 2D-M489 & 0.017 & 17.8 & 608 & 10.8 & $f_2$ \\
\hline83 & 2D-M80 & 0.2278 & 1.5 & 263 & 124.4 & $f_2$ & 406 & 2D-M201 & 0.0169 & 14.3 & 530 & 10.4 & $f_2$ \\
\hline84 & 2D-M66 & 0.227 & 1.3 & 178 & 165.4 & $f_2$ & 407 & 2D-M504 & 0.0169 & 13.0 & 457 & 11.3 & $f_2$ \\
\hline85 & 2D-M527 & 0.2263 & 9.0 & 339 & 8.4 & $f_2$ & 408 & 2D-M173 & 0.0169 & 15.2 & 549 & 12.4 & $f_2$ \\
\hline86 & 2D-M185 & 0.2257 & 1.0 & 76 & 149.1 & $f_2$ & 409 & 2D-M404 & 0.0169 & 13.5 & 475 & 10.7 & $f_2$ \\
\hline87 & 2D-M63 & 0.2253 & 1.5 & 271 & 134.9 & $f_2$ & 410 & 2D-M277 & 0.0168 & 12.7 & 446 & 9.3 & $f_2$ \\
\hline88 & 2D-M103 & 0.2251 & 1.3 & 209 & 123.4 & $f_2$ & 411 & 2D-M196 & 0.0166 & 11.8 & 419 & 13.3 & $f_2$ \\
\hline89 & 2D-M251 & 0.2246 & 1.3 & 181 & 141.0 & $f_2$ & 412 & 2D-M364 & 0.0166 & 12.4 & 438 & 9.3 & $f_2$ \\
\hline90 & 2D-M177 & 0.2241 & 1.5 & 279 & 111.0 & $f_2$ & 413 & 2D-M254 & 0.0166 & 12.2 & 430 & 10.5 & $f_2$ \\
\hline91 & 2D-M555 & 0.224 & 9.0 & 340 & 8.4 & $f_2$ & 414 & 2D-M390 & 0.0166 & 17.4 & 596 & 4.1 & $f_2$ \\
\hline92 & 2D-M284 & 0.223 & 2.0 & 315 & 136.6 & $f_2$ & 415 & 2D-M405 & 0.0165 & 11.6 & 404 & 10.2 & $f_2$ \\
\hline93 & 2D-M130 & 0.2218 & 1.3 & 193 & 126.6 & $f_2$ & 416 & 2D-M381 & 0.0163 & 14.2 & 526 & 8.2 & $f_2$ \\
\hline94 & 2D-M212 & 0.2218 & 1.6 & 291 & 137.2 & $f_2$ & 417 & 2D-M408 & 0.0162 & 10.3 & 353 & 10.3 & $f_2$ \\
\hline95 & 2D-M291 & 0.2201 & 1.6 & 288 & 123.7 & $f_2$ & 418 & 2D-M477 & 0.0161 & 10.9 & 379 & 10.9 & $f_2$ \\
\hline96 & 2D-M223 & 0.2201 & 1.6 & 287 & 123.7 & $f_2$ & 419 & 2D-M359 & 0.0161 & 10.9 & 377 & 10.9 & $f_2$ \\
\hline97 & 2D-M120 & 0.2189 & 1.0 & 61 & 145.2 & $f_2$ & 420 & 2D-M174 & 0.0161 & 13.8 & 487 & 11.2 & $f_2$ \\
\hline98 & 2D-M639 & 0.2183 & 1.0 & 18 & 1.0 & $f_2$ & 421 & 2D-M266 & 0.016 & 12.2 & 435 & 11.3 & $f_2$ \\
\hline99 & 2D-M468 & 0.2157 & 1.0 & 38 & 1.0 & $f_1$ & 422 & 2D-M263 & 0.016 & 12.5 & 441 & 10.7 & $f_2$ \\
\hline100 & 2D-M235 & 0.2155 & 1.3 & 199 & 109.6 & $f_2$ & 423 & 2D-M369 & 0.0159 & 9.0 & 337 & 9.0 & $f_2$ \\
\hline101 & 2D-M525 & 0.2138 & 9.0 & 341 & 8.4 & $f_2$ & 424 & 2D-M199 & 0.0159 & 24.4 & 641 & 9.2 & $f_2$ \\
\hline102 & 2D-M188 & 0.2127 & 1.4 & 244 & 139.6 & $f_2$ & 425 & 2D-M453 & 0.0159 & 11.7 & 411 & 10.9 & $f_2$ \\
\hline103 & 2D-M635 & 0.2096 & 1.0 & 48 & 1.0 & $f_2$ & 426 & 2D-M500 & 0.0159 & 17.5 & 603 & 10.1 & $f_2$ \\
\hline104 & 2D-M631 & 0.208 & 1.0 & 11 & 1.0 & $f_2$ & 427 & 2D-M435 & 0.0158 & 12.0 & 422 & 8.7 & $f_2$ \\
\hline105 & 2D-M68 & 0.208 & 1.2 & 164 & 175.5 & $f_2$ & 428 & 2D-M198 & 0.0158 & 12.7 & 445 & 11.2 & $f_2$ \\
\hline106 & 2D-M514 & 0.2078 & 9.0 & 342 & 8.4 & $f_2$ & 429 & 2D-M397 & 0.0156 & 14.1 & 514 & 9.3 & $f_2$ \\
\hline107 & 2D-M146 & 0.2056 & 1.2 & 161 & 182.5 & $f_2$ & 430 & 2D-M473 & 0.0155 & 17.5 & 602 & 9.9 & $f_2$ \\
\hline108 & 2D-M297 & 0.204 & 1.9 & 310 & 155.9 & $f_2$ & 431 & 2D-M229 & 0.0155 & 12.7 & 448 & 9.5 & $f_2$ \\
\hline109 & 2D-M56 & 0.2028 & 1.1 & 95 & 159.5 & $f_2$ & 432 & 2D-M260 & 0.0154 & 11.8 & 420 & 8.5 & $f_2$ \\
\hline110 & 2D-M100 & 0.2023 & 1.6 & 293 & 178.8 & $f_2$ & 433 & 2D-M23 & 0.0154 & 9.9 & 348 & 10.3 & $f_2$ \\
\hline111 & 2D-M190 & 0.202 & 10.2 & 351 & 9.5 & $f_1$ & 434 & 2D-M461 & 0.0154 & 11.9 & 421 & 9.8 & $f_2$ \\
\hline112 & 2D-M137 & 0.2016 & 1.0 & 68 & 149.0 & $f_2$ & 435 & 2D-M35 & 0.0153 & 11.5 & 402 & 12.9 & $f_2$ \\
\hline113 & 2D-M629 & 0.2016 & 1.0 & 36 & 1.0 & $f_2$ & 436 & 2D-M427 & 0.0153 & 13.4 & 473 & 10.1 & $f_2$ \\
\hline114 & 2D-M180 & 0.1995 & 1.4 & 225 & 109.1 & $f_2$ & 437 & 2D-M165 & 0.0153 & 11.7 & 410 & 7.8 & $f_2$ \\
\hline115 & 2D-M127 & 0.1984 & 1.3 & 201 & 165.2 & $f_2$ & 438 & 2D-M200 & 0.0152 & 12.8 & 449 & 10.8 & $f_2$ \\
\hline116 & 2D-M512 & 0.1978 & 9.1 & 343 & 8.4 & $f_2$ & 439 & 2D-M383 & 0.0152 & 11.6 & 407 & 10.5 & $f_2$ \\
\hline117 & 2D-M246 & 0.1971 & 1.3 & 184 & 132.2 & $f_2$ & 440 & 2D-M385 & 0.0152 & 13.0 & 455 & 8.3 & $f_2$ \\
\hline118 & 2D-M76 & 0.1969 & 2.5 & 321 & 138.2 & $f_2$ & 441 & 2D-M220 & 0.0151 & 11.8 & 417 & 8.6 & $f_2$ \\
\hline119 & 2D-M85 & 0.1964 & 1.1 & 121 & 140.2 & $f_2$ & 442 & 2D-M499 & 0.015 & 13.8 & 489 & 9.3 & $f_2$ \\
\hline120 & 2D-M121 & 0.1964 & 1.2 & 132 & 144.5 & $f_2$ & 443 & 2D-M153 & 0.0149 & 13.6 & 478 & 11.8 & $f_2$ \\
\hline121 & 2D-M231 & 0.195 & 1.2 & 144 & 143.0 & $f_2$ & 444 & 2D-M159 & 0.0148 & 14.1 & 520 & 9.8 & $f_2$ \\
\hline122 & 2D-M222 & 0.1949 & 1.4 & 242 & 107.6 & $f_2$ & 445 & 2D-M340 & 0.0148 & 17.6 & 607 & 12.0 & $f_2$ \\
\hline123 & 2D-M250 & 0.1936 & 1.3 & 185 & 107.3 & $f_2$ & 446 & 2D-M466 & 0.0148 & 11.5 & 400 & 10.4 & $f_2$ \\
\hline124 & 2D-M210 & 0.1922 & 1.1 & 105 & 135.4 & $f_2$ & 447 & 2D-M419 & 0.0147 & 10.7 & 367 & 6.9 & $f_2$ \\
\hline125 & 2D-M257 & 0.1919 & 1.4 & 220 & 130.8 & $f_2$ & 448 & 2D-M259 & 0.0146 & 12.2 & 431 & 8.9 & $f_2$ \\
\hline126 & 2D-M523 & 0.1895 & 7.8 & 329 & 7.1 & $f_2$ & 449 & 2D-M273 & 0.0146 & 12.8 & 450 & 9.7 & $f_2$ \\
\hline127 & 2D-M53 & 0.1889 & 1.0 & 57 & 111.8 & $f_2$ & 450 & 2D-M244 & 0.0146 & 13.7 & 482 & 10.5 & $f_2$ \\
\hline128 & 2D-M69 & 0.1883 & 1.3 & 212 & 147.5 & $f_2$ & 451 & 2D-M451 & 0.0145 & 12.9 & 453 & 6.4 & $f_2$ \\
\hline129 & 2D-M529 & 0.1881 & 11.2 & 381 & 10.5 & $f_2$ & 452 & 2D-M31 & 0.0145 & 8.2 & 330 & 8.2 & $f_2$ \\
\hline130 & 2D-M276 & 0.1869 & 11.2 & 382 & 10.5 & $f_1$ & 453 & 2D-M289 & 0.0145 & 11.5 & 401 & 8.6 & $f_2$ \\
\hline131 & 2D-M216 & 0.1861 & 1.3 & 217 & 104.7 & $f_2$ & 454 & 2D-M279 & 0.0144 & 12.5 & 440 & 8.7 & $f_2$ \\
\hline132 & 2D-M142 & 0.1846 & 1.2 & 169 & 149.0 & $f_2$ & 455 & 2D-M417 & 0.0143 & 13.1 & 465 & 11.3 & $f_2$ \\
\hline133 & 2D-M101 & 0.1844 & 1.2 & 176 & 120.0 & $f_2$ & 456 & 2D-M386 & 0.0143 & 17.3 & 589 & 5.3 & $f_2$ \\
\hline134 & 2D-M557 & 0.1843 & 10.2 & 352 & 9.5 & $f_2$ & 457 & 2D-M342 & 0.0142 & 17.4 & 593 & 5.2 & $f_2$ \\
\hline135 & 2D-M221 & 0.182 & 1.4 & 248 & 130.1 & $f_2$ & 458 & 2D-M488 & 0.0141 & 13.1 & 461 & 11.3 & $f_2$ \\
\hline136 & 2D-M183 & 0.1812 & 1.3 & 205 & 101.1 & $f_2$ & 459 & 2D-M167 & 0.014 & 10.6 & 365 & 7.0 & $f_2$ \\
\hline137 & 2D-M141 & 0.1806 & 1.5 & 272 & 81.9 & $f_2$ & 460 & 2D-M501 & 0.0139 & 14.0 & 501 & 10.6 & $f_2$ \\
\hline138 & 2D-M202 & 0.1799 & 1.1 & 103 & 110.3 & $f_2$ & 461 & 2D-M368 & 0.0139 & 14.0 & 502 & 10.6 & $f_2$ \\
\hline139 & 2D-M102 & 0.1795 & 1.3 & 213 & 95.2 & $f_2$ & 462 & 2D-M480 & 0.0139 & 16.4 & 566 & 10.3 & $f_2$ \\
\hline140 & 2D-M124 & 0.176 & 1.2 & 137 & 119.2 & $f_2$ & 463 & 2D-M258 & 0.0139 & 9.8 & 346 & 6.8 & $f_2$ \\
\hline141 & 2D-M513 & 0.1754 & 11.2 & 383 & 10.5 & $f_2$ & 464 & 2D-M392 & 0.0139 & 18.5 & 612 & 4.9 & $f_2$ \\
\hline142 & 2D-M94 & 0.1753 & 1.4 & 236 & 88.8 & $f_1$ & 465 & 2D-M189 & 0.0139 & 13.8 & 491 & 10.4 & $f_2$ \\
\hline143 & 2D-M517 & 0.175 & 11.2 & 384 & 10.5 & $f_2$ & 466 & 2D-M154 & 0.0138 & 13.6 & 479 & 10.3 & $f_2$ \\
\hline144 & 2D-M99 & 0.1747 & 1.1 & 92 & 132.9 & $f_2$ & 467 & 2D-M261 & 0.0138 & 14.0 & 507 & 10.6 & $f_2$ \\
\hline145 & 2D-M554 & 0.1742 & 11.2 & 385 & 10.5 & $f_2$ & 468 & 2D-M510 & 0.0138 & 9.9 & 347 & 7.1 & $f_2$ \\
\hline146 & 2D-M519 & 0.174 & 11.2 & 386 & 10.5 & $f_2$ & 469 & 2D-M399 & 0.0138 & 16.6 & 568 & 11.0 & $f_2$ \\
\hline147 & 2D-M207 & 0.1733 & 1.0 & 52 & 124.9 & $f_2$ & 470 & 2D-M14 & 0.0138 & 10.8 & 371 & 6.9 & $f_2$ \\
\hline148 & 2D-M60 & 0.1729 & 2.4 & 319 & 130.4 & $f_2$ & 471 & 2D-M324 & 0.0137 & 13.8 & 488 & 10.6 & $f_2$ \\
\hline149 & 2D-M559 & 0.1727 & 11.2 & 387 & 10.5 & $f_2$ & 472 & 2D-M382 & 0.0137 & 19.9 & 625 & 5.8 & $f_2$ \\
\hline150 & 2D-M62 & 0.1717 & 1.1 & 112 & 120.5 & $f_2$ & 473 & 2D-M271 & 0.0136 & 13.9 & 496 & 10.5 & $f_2$ \\
\hline151 & 2D-M632 & 0.171 & 1.0 & 27 & 1.0 & $f_2$ & 474 & 2D-M403 & 0.0136 & 11.1 & 380 & 7.1 & $f_2$ \\
\hline152 & 2D-M111 & 0.1708 & 1.3 & 211 & 109.6 & $f_2$ & 475 & 2D-M333 & 0.0136 & 13.9 & 497 & 10.5 & $f_2$ \\
\hline153 & 2D-M545 & 0.1704 & 11.2 & 389 & 10.5 & $f_2$ & 476 & 2D-M12 & 0.0136 & 12.2 & 434 & 8.9 & $f_2$ \\
\hline154 & 2D-M48 & 0.17 & 1.3 & 182 & 117.5 & $f_2$ & 477 & 2D-M356 & 0.0136 & 10.8 & 372 & 7.2 & $f_2$ \\
\hline155 & 2D-M96 & 0.169 & 1.2 & 156 & 96.8 & $f_2$ & 478 & 2D-M331 & 0.0132 & 13.1 & 459 & 9.5 & $f_2$ \\
\hline156 & 2D-M186 & 0.1684 & 1.7 & 297 & 108.9 & $f_2$ & 479 & 2D-M269 & 0.0132 & 13.5 & 476 & 10.8 & $f_2$ \\
\hline157 & 2D-M214 & 0.1681 & 1.1 & 129 & 101.3 & $f_2$ & 480 & 2D-M281 & 0.0132 & 10.0 & 349 & 7.0 & $f_2$ \\
\hline158 & 2D-M110 & 0.1679 & 1.1 & 93 & 135.3 & $f_2$ & 481 & 2D-M351 & 0.0132 & 14.2 & 528 & 10.8 & $f_2$ \\
\hline159 & 2D-M601 & 0.1676 & 1.0 & 34 & 1.0 & $f_1$ & 482 & 2D-M431 & 0.0132 & 14.2 & 527 & 10.8 & $f_2$ \\
\hline160 & 2D-M46 & 0.1674 & 1.2 & 145 & 100.4 & $f_2$ & 483 & 2D-M337 & 0.0132 & 12.0 & 424 & 8.4 & $f_2$ \\
\hline161 & 2D-M518 & 0.1665 & 11.2 & 390 & 10.5 & $f_2$ & 484 & 2D-M166 & 0.0132 & 14.0 & 499 & 9.4 & $f_2$ \\
\hline162 & 2D-M122 & 0.166 & 1.2 & 142 & 104.2 & $f_2$ & 485 & 2D-M265 & 0.0131 & 14.0 & 500 & 10.5 & $f_2$ \\
\hline163 & 2D-M283 & 0.1653 & 1.6 & 292 & 123.1 & $f_2$ & 486 & 2D-M393 & 0.0131 & 18.5 & 611 & 4.9 & $f_2$ \\
\hline164 & 2D-M97 & 0.1652 & 1.5 & 280 & 112.8 & $f_2$ & 487 & 2D-M462 & 0.0131 & 14.0 & 503 & 10.5 & $f_2$ \\
\hline165 & 2D-M627 & 0.1651 & 1.0 & 28 & 1.0 & $f_2$ & 488 & 2D-M436 & 0.0131 & 14.0 & 504 & 10.5 & $f_2$ \\
\hline166 & 2D-M204 & 0.1636 & 1.4 & 253 & 92.9 & $f_2$ & 489 & 2D-M334 & 0.0131 & 14.0 & 505 & 10.5 & $f_2$ \\
\hline167 & 2D-M558 & 0.1626 & 11.2 & 391 & 10.5 & $f_2$ & 490 & 2D-M329 & 0.013 & 12.0 & 425 & 8.4 & $f_2$ \\
\hline168 & 2D-M296 & 0.1625 & 1.2 & 134 & 119.5 & $f_2$ & 491 & 2D-M384 & 0.013 & 21.4 & 639 & 10.5 & $f_2$ \\
\hline169 & 2D-M131 & 0.1618 & 1.2 & 143 & 128.4 & $f_2$ & 492 & 2D-M395 & 0.013 & 21.3 & 638 & 10.5 & $f_2$ \\
\hline170 & 2D-M623 & 0.1613 & 1.0 & 14 & 1.0 & $f_2$ & 493 & 2D-M396 & 0.013 & 19.7 & 619 & 7.1 & $f_2$ \\
\hline171 & 2D-M640 & 0.1608 & 1.0 & 43 & 1.0 & $f_2$ & 494 & 2D-M162 & 0.013 & 10.8 & 368 & 7.1 & $f_2$ \\
\hline172 & 2D-M107 & 0.1602 & 1.1 & 83 & 120.8 & $f_2$ & 495 & 2D-M206 & 0.013 & 10.9 & 374 & 8.2 & $f_2$ \\
\hline173 & 2D-M515 & 0.1581 & 11.2 & 392 & 10.5 & $f_2$ & 496 & 2D-M274 & 0.013 & 12.0 & 423 & 8.5 & $f_2$ \\
\hline174 & 2D-M49 & 0.1576 & 1.1 & 109 & 91.0 & $f_2$ & 497 & 2D-M511 & 0.013 & 13.9 & 495 & 10.6 & $f_2$ \\
\hline175 & 2D-M108 & 0.1576 & 1.1 & 99 & 127.9 & $f_2$ & 498 & 2D-M418 & 0.0129 & 14.0 & 508 & 10.5 & $f_2$ \\
\hline176 & 2D-M597 & 0.1569 & 1.0 & 41 & 1.0 & $f_1$ & 499 & 2D-M350 & 0.0129 & 14.1 & 510 & 10.5 & $f_2$ \\
\hline177 & 2D-M136 & 0.1553 & 1.2 & 139 & 126.7 & $f_2$ & 500 & 2D-M370 & 0.0129 & 13.1 & 464 & 9.5 & $f_2$ \\
\hline178 & 2D-M292 & 0.1543 & 1.2 & 163 & 124.6 & $f_2$ & 501 & 2D-M339 & 0.0129 & 11.3 & 394 & 7.1 & $f_2$ \\
\hline179 & 2D-M45 & 0.1538 & 1.3 & 218 & 137.5 & $f_2$ & 502 & 2D-M347 & 0.0129 & 14.0 & 509 & 10.5 & $f_2$ \\
\hline180 & 2D-M148 & 0.1535 & 1.0 & 56 & 91.6 & $f_2$ & 503 & 2D-M479 & 0.0129 & 13.8 & 492 & 10.3 & $f_2$ \\
\hline181 & 2D-M243 & 0.1534 & 11.3 & 393 & 10.5 & $f_1$ & 504 & 2D-M287 & 0.0129 & 14.3 & 529 & 8.8 & $f_2$ \\
\hline182 & 2D-M104 & 0.1515 & 1.1 & 102 & 121.5 & $f_2$ & 505 & 2D-M19 & 0.0129 & 10.8 & 373 & 7.1 & $f_2$ \\
\hline183 & 2D-M638 & 0.1508 & 1.0 & 31 & 1.0 & $f_2$ & 506 & 2D-M470 & 0.0128 & 13.1 & 466 & 9.5 & $f_2$ \\
\hline184 & 2D-M225 & 0.1494 & 1.1 & 81 & 109.5 & $f_2$ & 507 & 2D-M506 & 0.0128 & 11.8 & 418 & 8.1 & $f_2$ \\
\hline185 & 2D-M454 & 0.1488 & 10.3 & 354 & 9.5 & $f_1$ & 508 & 2D-M437 & 0.0128 & 12.1 & 426 & 8.4 & $f_2$ \\
\hline186 & 2D-M84 & 0.1484 & 1.6 & 283 & 114.9 & $f_2$ & 509 & 2D-M401 & 0.0128 & 13.1 & 468 & 9.5 & $f_2$ \\
\hline187 & 2D-M47 & 0.1467 & 1.3 & 189 & 103.7 & $f_2$ & 510 & 2D-M338 & 0.0128 & 17.3 & 581 & 9.5 & $f_2$ \\
\hline188 & 2D-M44 & 0.1466 & 1.4 & 247 & 121.1 & $f_2$ & 511 & 2D-M464 & 0.0127 & 14.1 & 513 & 10.5 & $f_2$ \\
\hline189 & 2D-M241 & 0.1455 & 1.4 & 257 & 90.4 & $f_2$ & 512 & 2D-M433 & 0.0127 & 13.1 & 469 & 9.5 & $f_2$ \\
\hline190 & 2D-M114 & 0.1451 & 1.1 & 98 & 116.6 & $f_2$ & 513 & 2D-M423 & 0.0127 & 13.8 & 490 & 10.2 & $f_2$ \\
\hline191 & 2D-M528 & 0.1447 & 11.3 & 395 & 10.5 & $f_2$ & 514 & 2D-M472 & 0.0127 & 13.1 & 462 & 9.6 & $f_2$ \\
\hline192 & 2D-M621 & 0.1437 & 1.0 & 30 & 1.0 & $f_2$ & 515 & 2D-M336 & 0.0127 & 14.1 & 515 & 10.5 & $f_2$ \\
\hline193 & 2D-M478 & 0.1431 & 10.3 & 355 & 9.5 & $f_1$ & 516 & 2D-M321 & 0.0126 & 12.1 & 427 & 8.4 & $f_2$ \\
\hline194 & 2D-M268 & 0.1428 & 11.3 & 396 & 10.5 & $f_1$ & 517 & 2D-M380 & 0.0126 & 15.7 & 557 & 10.2 & $f_2$ \\
\hline195 & 2D-M609 & 0.1385 & 1.0 & 40 & 1.0 & $f_1$ & 518 & 2D-M335 & 0.0126 & 14.1 & 516 & 10.5 & $f_2$ \\
\hline196 & 2D-M133 & 0.1381 & 1.5 & 277 & 94.7 & $f_2$ & 519 & 2D-M21 & 0.0126 & 12.1 & 428 & 8.4 & $f_2$ \\
\hline197 & 2D-M90 & 0.1378 & 1.2 & 140 & 100.2 & $f_2$ & 520 & 2D-M345 & 0.0126 & 13.2 & 470 & 9.5 & $f_2$ \\
\hline198 & 2D-M51 & 0.1372 & 1.4 & 254 & 104.1 & $f_2$ & 521 & 2D-M367 & 0.0126 & 14.1 & 517 & 10.5 & $f_2$ \\
\hline199 & 2D-M95 & 0.1364 & 1.2 & 150 & 90.2 & $f_2$ & 522 & 2D-M25 & 0.0126 & 13.2 & 471 & 9.5 & $f_2$ \\
\hline200 & 2D-M115 & 0.1354 & 1.1 & 128 & 91.0 & $f_2$ & 523 & 2D-M320 & 0.0126 & 14.1 & 518 & 10.5 & $f_2$ \\
\hline201 & 2D-M89 & 0.1353 & 1.5 & 270 & 87.1 & $f_2$ & 524 & 2D-M30 & 0.0125 & 14.1 & 519 & 10.5 & $f_2$ \\
\hline202 & 2D-M371 & 0.1352 & 7.7 & 324 & 6.8 & $f_1$ & 525 & 2D-M323 & 0.0125 & 12.7 & 447 & 7.5 & $f_2$ \\
\hline203 & 2D-M238 & 0.134 & 1.4 & 249 & 85.2 & $f_2$ & 526 & 2D-M428 & 0.0123 & 16.8 & 576 & 10.1 & $f_2$ \\
\hline204 & 2D-M129 & 0.1339 & 1.0 & 13 & 91.0 & $f_2$ & 527 & 2D-M496 & 0.0121 & 14.1 & 521 & 9.9 & $f_2$ \\
\hline205 & 2D-M81 & 0.1336 & 1.3 & 195 & 98.0 & $f_2$ & 528 & 2D-M455 & 0.0121 & 12.6 & 443 & 8.1 & $f_2$ \\
\hline206 & 2D-M626 & 0.133 & 1.0 & 49 & 1.0 & $f_2$ & 529 & 2D-M330 & 0.0121 & 13.7 & 483 & 9.2 & $f_2$ \\
\hline207 & 2D-M625 & 0.1323 & 1.0 & 20 & 1.0 & $f_2$ & 530 & 2D-M449 & 0.0121 & 9.0 & 338 & 5.1 & $f_2$ \\
\hline208 & 2D-M516 & 0.1323 & 10.4 & 356 & 9.5 & $f_2$ & 531 & 2D-M169 & 0.012 & 10.6 & 364 & 8.1 & $f_2$ \\
\hline209 & 2D-M5 & 0.1309 & 1.3 & 206 & 100.1 & $f_2$ & 532 & 2D-M161 & 0.012 & 15.3 & 550 & 10.1 & $f_2$ \\
\hline210 & 2D-M52 & 0.1305 & 1.6 & 286 & 100.4 & $f_2$ & 533 & 2D-M402 & 0.0119 & 13.7 & 486 & 8.8 & $f_2$ \\
\hline211 & 2D-M247 & 0.1293 & 1.6 & 285 & 88.8 & $f_2$ & 534 & 2D-M446 & 0.0119 & 15.6 & 554 & 9.5 & $f_2$ \\
\hline212 & 2D-M109 & 0.1284 & 1.4 & 233 & 105.7 & $f_2$ & 535 & 2D-M429 & 0.0119 & 13.8 & 493 & 8.5 & $f_2$ \\
\hline213 & 2D-M64 & 0.128 & 1.0 & 75 & 85.3 & $f_2$ & 536 & 2D-M358 & 0.0117 & 13.5 & 474 & 9.6 & $f_2$ \\
\hline214 & 2D-M83 & 0.1275 & 1.0 & 15 & 111.0 & $f_2$ & 537 & 2D-M275 & 0.0117 & 13.7 & 484 & 7.0 & $f_2$ \\
\hline215 & 2D-M75 & 0.1272 & 1.3 & 202 & 88.8 & $f_2$ & 538 & 2D-M272 & 0.0117 & 13.1 & 467 & 9.2 & $f_2$ \\
\hline216 & 2D-M447 & 0.1272 & 11.4 & 397 & 10.5 & $f_1$ & 539 & 2D-M327 & 0.0116 & 14.6 & 534 & 9.4 & $f_2$ \\
\hline217 & 2D-M79 & 0.1264 & 1.6 & 296 & 75.3 & $f_2$ & 540 & 2D-M322 & 0.0116 & 14.6 & 533 & 9.5 & $f_2$ \\
\hline218 & 2D-M245 & 0.1264 & 1.1 & 100 & 96.5 & $f_2$ & 541 & 2D-M490 & 0.0115 & 24.5 & 642 & 8.4 & $f_2$ \\
\hline219 & 2D-M65 & 0.1258 & 1.0 & 51 & 90.7 & $f_2$ & 542 & 2D-M505 & 0.0114 & 24.4 & 640 & 8.4 & $f_2$ \\
\hline220 & 2D-M8 & 0.1255 & 1.7 & 301 & 86.0 & $f_2$ & 543 & 2D-M13 & 0.0113 & 13.5 & 477 & 9.3 & $f_2$ \\
\hline221 & 2D-M54 & 0.125 & 1.2 & 149 & 68.0 & $f_2$ & 544 & 2D-M18 & 0.0112 & 12.3 & 437 & 8.4 & $f_2$ \\
\hline222 & 2D-M4 & 0.1247 & 1.9 & 311 & 62.0 & $f_2$ & 545 & 2D-M432 & 0.0111 & 15.6 & 555 & 7.4 & $f_2$ \\
\hline223 & 2D-M3 & 0.1245 & 1.1 & 123 & 88.7 & $f_2$ & 546 & 2D-M341 & 0.011 & 17.3 & 592 & 2.9 & $f_2$ \\
\hline224 & 2D-M72 & 0.1243 & 1.2 & 168 & 74.9 & $f_2$ & 547 & 2D-M400 & 0.0109 & 26.1 & 644 & 7.8 & $f_2$ \\
\hline225 & 2D-M6 & 0.1242 & 1.0 & 62 & 111.1 & $f_2$ & 548 & 2D-M191 & 0.0108 & 15.3 & 552 & 8.0 & $f_2$ \\
\hline226 & 2D-M544 & 0.1241 & 17.5 & 604 & 17.5 & $f_2$ & 549 & 2D-M20 & 0.0107 & 8.7 & 332 & 6.6 & $f_2$ \\
\hline227 & 2D-M50 & 0.1236 & 1.2 & 151 & 85.4 & $f_2$ & 550 & 2D-M388 & 0.0107 & 17.3 & 591 & 2.9 & $f_2$ \\
\hline228 & 2D-M414 & 0.1229 & 10.4 & 359 & 9.5 & $f_1$ & 551 & 2D-M448 & 0.0105 & 12.2 & 432 & 5.8 & $f_2$ \\
\hline229 & 2D-M151 & 0.1218 & 1.0 & 72 & 93.3 & $f_2$ & 552 & 2D-M325 & 0.0104 & 16.7 & 571 & 8.1 & $f_2$ \\
\hline230 & 2D-M7 & 0.1216 & 1.4 & 222 & 100.5 & $f_2$ & 553 & 2D-M270 & 0.0098 & 16.7 & 570 & 6.6 & $f_2$ \\
\hline231 & 2D-M41 & 0.1211 & 1.2 & 154 & 98.8 & $f_2$ & 554 & 2D-M643 & 0.0091 & 14.8 & 539 & 10.5 & $f_1$ \\
\hline232 & 2D-M117 & 0.121 & 1.0 & 66 & 92.3 & $f_2$ & 555 & 2D-M644 & 0.0091 & 14.8 & 540 & 10.5 & $f_1$ \\
\hline233 & 2D-M150 & 0.121 & 1.0 & 67 & 92.3 & $f_2$ & 556 & 2D-M416 & 0.0088 & 25.6 & 643 & 7.1 & $f_2$ \\
\hline234 & 2D-M106 & 0.1209 & 1.3 & 208 & 92.2 & $f_2$ & 557 & 2D-M195 & 0.0085 & 16.7 & 569 & 4.9 & $f_2$ \\
\hline235 & 2D-M211 & 0.1199 & 2.2 & 318 & 87.7 & $f_2$ & 558 & 2D-M197 & 0.0084 & 13.6 & 480 & 4.5 & $f_2$ \\
\hline236 & 2D-M57 & 0.1189 & 1.5 & 268 & 96.6 & $f_2$ & 559 & 2D-M22 & 0.0082 & 18.9 & 614 & 6.1 & $f_2$ \\
\hline237 & 2D-M139 & 0.1182 & 1.3 & 177 & 69.6 & $f_2$ & 560 & 2D-M326 & 0.0079 & 16.4 & 564 & 5.8 & $f_2$ \\
\hline238 & 2D-M240 & 0.1178 & 1.1 & 125 & 88.9 & $f_2$ & 561 & 2D-M486 & 0.0079 & 16.4 & 565 & 5.8 & $f_2$ \\
\hline239 & 2D-M105 & 0.1177 & 1.2 & 162 & 89.5 & $f_2$ & 562 & 2D-M398 & 0.0078 & 27.4 & 645 & 6.4 & $f_2$ \\
\hline240 & 2D-M541 & 0.1172 & 9.3 & 345 & 8.4 & $f_1$ & 563 & 2D-M171 & 0.0077 & 16.1 & 559 & 4.5 & $f_2$ \\
\hline241 & 2D-M249 & 0.117 & 1.5 & 278 & 95.3 & $f_2$ & 564 & 2D-M391 & 0.0073 & 20.2 & 631 & 3.4 & $f_2$ \\
\hline242 & 2D-M78 & 0.1165 & 1.1 & 113 & 68.5 & $f_2$ & 565 & 2D-M332 & 0.0066 & 19.0 & 616 & 5.5 & $f_2$ \\
\hline243 & 2D-M70 & 0.1162 & 1.1 & 101 & 57.4 & $f_2$ & 566 & 2D-M494 & 0.0062 & 21.2 & 637 & 5.1 & $f_2$ \\
\hline244 & 2D-M530 & 0.1158 & 17.4 & 599 & 17.4 & $f_2$ & 567 & 2D-M509 & 0.0057 & 19.7 & 620 & 4.8 & $f_2$ \\
\hline245 & 2D-M58 & 0.1149 & 1.3 & 214 & 63.5 & $f_2$ & 568 & 2D-M328 & 0.0055 & 17.5 & 600 & 3.5 & $f_2$ \\
\hline246 & 2D-M93 & 0.1146 & 1.5 & 273 & 88.8 & $f_2$ & 569 & 2D-M176 & 0.0041 & 16.8 & 574 & 2.7 & $f_2$ \\
\hline247 & 2D-M125 & 0.1145 & 1.5 & 260 & 78.1 & $f_2$ & 570 & 2D-M599 & 0.0028 & 1.0 & 53 & 1.0 & $f_2$ \\
\hline248 & 2D-M10 & 0.1143 & 1.7 & 302 & 86.0 & $f_2$ & 571 & 2D-M40 & 0.0026 & 1.7 & 304 & 1.7 & $f_2$ \\
\hline249 & 2D-M112 & 0.1143 & 1.3 & 194 & 72.4 & $f_2$ & 572 & 2D-M469 & 0.0021 & 1.1 & 106 & 1.1 & $f_2$ \\
\hline250 & 2D-M15 & 0.1138 & 1.7 & 303 & 86.0 & $f_2$ & 573 & 2D-M483 & 0.002 & 1.1 & 79 & 1.0 & $f_2$ \\
\hline251 & 2D-M149 & 0.1138 & 1.0 & 74 & 72.9 & $f_2$ & 574 & 2D-M565 & 0.002 & 1.0 & 50 & 1.0 & $f_2$ \\
\hline252 & 2D-M147 & 0.1138 & 1.0 & 73 & 72.9 & $f_2$ & 575 & 2D-M36 & 0.002 & 1.4 & 238 & 1.4 & $f_2$ \\
\hline253 & 2D-M294 & 0.1137 & 1.5 & 258 & 85.6 & $f_2$ & 576 & 2D-M560 & 0.0019 & 1.2 & 147 & 1.2 & $f_2$ \\
\hline254 & 2D-M178 & 0.1129 & 1.1 & 96 & 77.5 & $f_2$ & 577 & 2D-M573 & 0.0018 & 1.2 & 146 & 1.2 & $f_2$ \\
\hline255 & 2D-M551 & 0.1124 & 17.4 & 598 & 17.4 & $f_2$ & 578 & 2D-M441 & 0.0017 & 1.1 & 124 & 1.1 & $f_2$ \\
\hline256 & 2D-M123 & 0.1121 & 1.2 & 160 & 75.2 & $f_2$ & 579 & 2D-M39 & 0.0017 & 1.2 & 165 & 1.2 & $f_2$ \\
\hline257 & 2D-M2 & 0.1115 & 1.2 & 159 & 100.4 & $f_2$ & 580 & 2D-M563 & 0.0017 & 1.1 & 94 & 1.1 & $f_2$ \\
\hline258 & 2D-M119 & 0.1105 & 1.3 & 215 & 68.1 & $f_2$ & 581 & 2D-M576 & 0.0017 & 1.1 & 85 & 1.1 & $f_2$ \\
\hline259 & 2D-M624 & 0.1091 & 1.0 & 35 & 1.0 & $f_2$ & 582 & 2D-M575 & 0.0017 & 1.1 & 87 & 1.1 & $f_2$ \\
\hline260 & 2D-M290 & 0.1086 & 1.1 & 97 & 90.6 & $f_2$ & 583 & 2D-M587 & 0.0017 & 1.1 & 91 & 1.1 & $f_2$ \\
\hline261 & 2D-M1 & 0.106 & 1.9 & 309 & 74.0 & $f_2$ & 584 & 2D-M615 & 0.0016 & 1.0 & 71 & 1.0 & $f_2$ \\
\hline262 & 2D-M67 & 0.1059 & 1.5 & 264 & 79.0 & $f_2$ & 585 & 2D-M588 & 0.0016 & 1.1 & 86 & 1.1 & $f_2$ \\
\hline263 & 2D-M531 & 0.1058 & 17.6 & 605 & 17.5 & $f_2$ & 586 & 2D-M34 & 0.0016 & 1.5 & 261 & 1.0 & $f_2$ \\
\hline264 & 2D-M463 & 0.1045 & 10.5 & 360 & 9.5 & $f_1$ & 587 & 2D-M493 & 0.0016 & 1.1 & 90 & 1.1 & $f_2$ \\
\hline265 & 2D-M641 & 0.1036 & 1.0 & 42 & 1.0 & $f_2$ & 588 & 2D-M574 & 0.0016 & 1.0 & 12 & 1.0 & $f_2$ \\
\hline266 & 2D-M532 & 0.1028 & 17.4 & 597 & 17.4 & $f_2$ & 589 & 2D-M467 & 0.0016 & 1.1 & 126 & 1.1 & $f_2$ \\
\hline267 & 2D-M636 & 0.1026 & 1.0 & 33 & 1.0 & $f_2$ & 590 & 2D-M571 & 0.0016 & 1.0 & 2 & 1.0 & $f_2$ \\
\hline268 & 2D-M630 & 0.1021 & 1.0 & 45 & 1.0 & $f_2$ & 591 & 2D-M592 & 0.0016 & 1.7 & 299 & 1.0 & $f_2$ \\
\hline269 & 2D-M434 & 0.1012 & 10.5 & 361 & 9.5 & $f_1$ & 592 & 2D-M577 & 0.0015 & 1.2 & 138 & 0.9 & $f_2$ \\
\hline270 & 2D-M29 & 0.101 & 8.2 & 331 & 7.1 & $f_1$ & 593 & 2D-M605 & 0.0015 & 1.1 & 89 & 1.1 & $f_2$ \\
\hline271 & 2D-M637 & 0.1006 & 1.0 & 5 & 1.0 & $f_2$ & 594 & 2D-M604 & 0.0015 & 1.1 & 88 & 1.1 & $f_2$ \\
\hline272 & 2D-M233 & 0.099 & 2.5 & 320 & 82.4 & $f_2$ & 595 & 2D-M594 & 0.0015 & 1.0 & 8 & 1.0 & $f_2$ \\
\hline273 & 2D-M77 & 0.099 & 1.4 & 255 & 63.5 & $f_2$ & 596 & 2D-M598 & 0.0015 & 1.0 & 24 & 1.0 & $f_2$ \\
\hline274 & 2D-M55 & 0.0984 & 1.5 & 262 & 78.8 & $f_2$ & 597 & 2D-M610 & 0.0015 & 1.0 & 3 & 1 & $f_2$ \\
\hline275 & 2D-M553 & 0.097 & 16.8 & 575 & 16.5 & $f_2$ & 598 & 2D-M602 & 0.0015 & 1.0 & 60 & 1.0 & $f_2$ \\
\hline276 & 2D-M42 & 0.0964 & 1.4 & 221 & 60.2 & $f_2$ & 599 & 2D-M590 & 0.0015 & 1.0 & 59 & 1.0 & $f_2$ \\
\hline277 & 2D-M642 & 0.0962 & 1.0 & 9 & 111.0 & $f_1$ & 600 & 2D-M586 & 0.0015 & 1.0 & 58 & 1.0 & $f_2$ \\
\hline278 & 2D-M255 & 0.0945 & 1.8 & 308 & 76.7 & $f_2$ & 601 & 2D-M564 & 0.0015 & 1.0 & 55 & 1.0 & $f_2$ \\
\hline279 & 2D-M409 & 0.093 & 10.6 & 362 & 9.5 & $f_1$ & 602 & 2D-M603 & 0.0015 & 1.0 & 54 & 1.0 & $f_2$ \\
\hline280 & 2D-M620 & 0.0923 & 1.0 & 16 & 1.0 & $f_2$ & 603 & 2D-M618 & 0.0015 & 1.0 & 29 & 1.0 & $f_2$ \\
\hline281 & 2D-M452 & 0.0922 & 10.6 & 363 & 9.5 & $f_1$ & 604 & 2D-M457 & 0.0015 & 1.4 & 229 & 1.1 & $f_2$ \\
\hline282 & 2D-M471 & 0.091 & 11.6 & 403 & 10.5 & $f_1$ & 605 & 2D-M585 & 0.0015 & 1.0 & 23 & 1.0 & $f_2$ \\
\hline283 & 2D-M179 & 0.0906 & 1.0 & 78 & 62.8 & $f_2$ & 606 & 2D-M569 & 0.0015 & 1.0 & 17 & 1.0 & $f_2$ \\
\hline284 & 2D-M438 & 0.0901 & 9.2 & 344 & 8.1 & $f_1$ & 607 & 2D-M596 & 0.0014 & 1.0 & 21 & 1.0 & $f_2$ \\
\hline285 & 2D-M92 & 0.0898 & 1.5 & 267 & 62.1 & $f_2$ & 608 & 2D-M567 & 0.0014 & 1.0 & 19 & 1.0 & $f_2$ \\
\hline286 & 2D-M91 & 0.0896 & 1.4 & 231 & 49.5 & $f_2$ & 609 & 2D-M570 & 0.0014 & 1.0 & 1 & 1.0 & $f_2$ \\
\hline287 & 2D-M73 & 0.088 & 1.3 & 197 & 48.2 & $f_2$ & 610 & 2D-M606 & 0.0014 & 1.0 & 25 & 1.0 & $f_2$ \\
\hline288 & 2D-M622 & 0.0869 & 1.0 & 39 & 1.0 & $f_2$ & 611 & 2D-M595 & 0.0014 & 1.0 & 63 & 1.0 & $f_2$ \\
\hline289 & 2D-M365 & 0.0868 & 11.6 & 406 & 10.5 & $f_1$ & 612 & 2D-M583 & 0.0014 & 1.0 & 65 & 1.0 & $f_2$ \\
\hline290 & 2D-M482 & 0.0862 & 1.0 & 44 & 1.0 & $f_1$ & 613 & 2D-M562 & 0.0014 & 1.0 & 64 & 1.0 & $f_2$ \\
\hline291 & 2D-M547 & 0.0855 & 10.4 & 357 & 9.3 & $f_2$ & 614 & 2D-M600 & 0.0014 & 1.0 & 4 & 1.0 & $f_2$ \\
\hline292 & 2D-M426 & 0.0843 & 10.6 & 366 & 9.5 & $f_1$ & 615 & 2D-M619 & 0.0014 & 1.4 & 235 & 1.0 & $f_2$ \\
\hline293 & 2D-M27 & 0.0834 & 11.6 & 408 & 10.5 & $f_1$ & 616 & 2D-M614 & 0.0014 & 1.4 & 234 & 1.0 & $f_2$ \\
\hline294 & 2D-M538 & 0.0833 & 11.8 & 416 & 10.1 & $f_1$ & 617 & 2D-M459 & 0.0014 & 1.0 & 77 & 1.0 & $f_2$ \\
\hline295 & 2D-M495 & 0.0823 & 11.6 & 409 & 10.5 & $f_1$ & 618 & 2D-M33 & 0.0013 & 1.4 & 237 & 1.1 & $f_2$ \\
\hline296 & 2D-M536 & 0.0805 & 19.8 & 622 & 19.8 & $f_2$ & 619 & 2D-M445 & 0.0012 & 1.1 & 110 & 0.8 & $f_2$ \\
\hline297 & 2D-M373 & 0.0742 & 11.7 & 412 & 10.5 & $f_1$ & 620 & 2D-M444 & 0.0012 & 1.5 & 274 & 0.9 & $f_2$ \\
\hline298 & 2D-M280 & 0.0736 & 11.7 & 413 & 10.5 & $f_1$ & 621 & 2D-M37 & 0.0012 & 1.2 & 166 & 0.8 & $f_2$ \\
\hline299 & 2D-M476 & 0.073 & 11.7 & 414 & 10.5 & $f_1$ & 622 & 2D-M38 & 0.0012 & 1.2 & 167 & 0.8 & $f_2$ \\
\hline300 & 2D-M377 & 0.0705 & 10.8 & 369 & 9.5 & $f_1$ & 623 & 2D-M443 & 0.0012 & 1.2 & 170 & 0.7 & $f_2$ \\
\hline301 & 2D-M253 & 0.0693 & 11.8 & 415 & 10.5 & $f_1$ & 624 & 2D-M440 & 0.0012 & 2.6 & 322 & 0.9 & $f_2$ \\
\hline302 & 2D-M540 & 0.0692 & 20.2 & 629 & 20.2 & $f_2$ & 625 & 2D-M593 & 0.0012 & 1.3 & 200 & 0.8 & $f_2$ \\
\hline303 & 2D-M539 & 0.067 & 20.2 & 630 & 20.2 & $f_2$ & 626 & 2D-M611 & 0.001 & 1.4 & 232 & 0.6 & $f_2$ \\
\hline304 & 2D-M549 & 0.0656 & 20.2 & 626 & 20.2 & $f_2$ & 627 & 2D-M481 & 0.001 & 1.0 & 69 & 0.7 & $f_2$ \\
\hline305 & 2D-M552 & 0.0605 & 20.2 & 627 & 20.2 & $f_2$ & 628 & 2D-M616 & 0.001 & 1.6 & 289 & 0.6 & $f_2$ \\
\hline306 & 2D-M537 & 0.0603 & 20.2 & 628 & 20.2 & $f_2$ & 629 & 2D-M442 & 0.001 & 2.2 & 317 & 0.6 & $f_2$ \\
\hline307 & 2D-M533 & 0.0579 & 9.0 & 336 & 6.4 & $f_1$ & 630 & 2D-M568 & 0.0009 & 1.3 & 187 & 0.6 & $f_2$ \\
\hline308 & 2D-M32 & 0.0565 & 1.0 & 22 & 1.0 & $f_1$ & 631 & 2D-M582 & 0.0009 & 1.3 & 196 & 0.6 & $f_2$ \\
\hline309 & 2D-M633 & 0.0525 & 1.0 & 46 & 1.0 & $f_2$ & 632 & 2D-M617 & 0.0009 & 1.3 & 188 & 0.6 & $f_2$ \\
\hline310 & 2D-M219 & 0.0514 & 8.8 & 333 & 7.1 & $f_1$ & 633 & 2D-M580 & 0.0009 & 1.3 & 186 & 0.6 & $f_2$ \\
\hline311 & 2D-M422 & 0.0484 & 10.1 & 350 & 8.4 & $f_1$ & 634 & 2D-M561 & 0.0009 & 2.6 & 323 & 0.6 & $f_2$ \\
\hline312 & 2D-M492 & 0.0458 & 1.0 & 10 & 1 & $f_1$ & 635 & 2D-M578 & 0.0008 & 1.5 & 275 & 0.5 & $f_2$ \\
\hline313 & 2D-M379 & 0.0441 & 12.2 & 433 & 10.5 & $f_1$ & 636 & 2D-M566 & 0.0008 & 1.4 & 252 & 0.5 & $f_2$ \\
\hline314 & 2D-M487 & 0.0401 & 12.3 & 436 & 10.5 & $f_1$ & 637 & 2D-M608 & 0.0008 & 1.4 & 251 & 0.5 & $f_2$ \\
\hline315 & 2D-M420 & 0.0335 & 14.1 & 512 & 14.2 & $f_2$ & 638 & 2D-M581 & 0.0008 & 1.3 & 210 & 0.6 & $f_2$ \\
\hline316 & 2D-M589 & 0.0333 & 1.0 & 37 & 1.0 & $f_1$ & 639 & 2D-M584 & 0.0007 & 1.4 & 250 & 0.5 & $f_2$ \\
\hline317 & 2D-M613 & 0.0326 & 1.0 & 47 & 1.0 & $f_1$ & 640 & 2D-M612 & 0.0007 & 1.4 & 245 & 0.5 & $f_2$ \\
\hline318 & 2D-M498 & 0.032 & 17.2 & 580 & 17.4 & $f_2$ & 641 & 2D-M579 & 0.0007 & 1.4 & 243 & 0.5 & $f_2$ \\
\hline319 & 2D-M352 & 0.0318 & 17.3 & 585 & 17.3 & $f_2$ & 642 & 2D-M591 & 0.0007 & 1.4 & 256 & 0.5 & $f_2$ \\
\hline320 & 2D-M157 & 0.0297 & 20.8 & 636 & 20.1 & $f_2$ & 643 & 2D-M572 & 0.0007 & 1.4 & 239 & 0.5 & $f_2$ \\
\hline321 & 2D-M262 & 0.0296 & 11.2 & 388 & 18.1 & $f_2$ & 644 & 2D-M491 & 0.0007 & 1.3 & 203 & 0.5 & $f_2$ \\
\hline322 & 2D-M218 & 0.0294 & 17.0 & 579 & 16.8 & $f_2$ & 645 & 2D-M607 & 0.0006 & 1.6 & 282 & 0.4 & $f_2$ \\
\hline323 & 2D-M542 & 0.0293 & 16.8 & 573 & 15.8 & $f_2$ &  &  &  &  &  &  &  \\
\hline
\caption{Manipulability and Condition Numbers of 2-DOF Manipulators}
\label{Tab:table_dof2mt_1}  \end{longtable}
\normalsize
%}

==> contentfolder/mechanisms2/manipulators/dof1/manipulator_3.tex <==
% \emph{Adjacency matrix of manipulator 1D-M3:}

% The adjacency of the manipulator is\[M_{\text{1D-M3}}=\left[\begin{matrix}L_{1}&O&R&C\\O&L_{2}&R&S\\R&R&L_{3}&O\\C&S&O&L_{4}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline


\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/1dof/3.png}
  \caption{Schematic figure of 1D-M3}
  \label{fig_iext_3}
\end{figure}


\emph{Formulation of Jacobian:}

Jacobian of the manipulator is formulated using the steps shown in section \ref{steps_to_formulate_jacobian}. From figure \ref{fig_iext_3}, the various paths that connect the base link and the end-effector link are $L_1-R-L_3-R-L_2-S-L_4$ and $L_1-C-L_4$. The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.


\begin{eqnarray}\label{eqn:eqn_1_3_1_2}\vec{v}=\dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{32} \hat{n}_{32} \times \left( \vec{a} - \vec{r}_{32} \right) + \vec{\omega}_{24} \times \left( \vec{a} - \vec{r}_{24} \right)\end{eqnarray}\begin{eqnarray}\label{eqn:eqn_1_3_1_1}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{d}_{14} \hat{n}_{14}\end{eqnarray}
\begin{dmath}\label{eqn:eqn_1_3_2_2}\vec{\omega}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{32} \hat{n}_{32} + \vec{\omega}_{24}\end{dmath}\begin{dmath}\label{eqn:eqn_1_3_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14}\end{dmath}where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{ij}=\begin{Bmatrix} \omega_{ijx} & \omega_{ijy} & \omega_{ijz} \end{Bmatrix}^T$ represents the relative angular velocity vector of the link $L_j$ relative to the link $L_i$, of the adjacency matrix. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_1_3_1_1} and \eqref{eqn:eqn_1_3_2_1}, the vector of end-effector velocities in terms of both active and passive joint angles is given by
\newline

$$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}0 & n_{14x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 & 0\\0 & n_{14y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & 0 & 0\\0 & n_{14z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & 0 & 0\\0 & 0 & n_{14x} & 0 & 0 & 0 & 0\\0 & 0 & n_{14y} & 0 & 0 & 0 & 0\\0 & 0 & n_{14z} & 0 & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}$$


$$\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}0\\0\\0\\0\\0\\0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\end{Bmatrix}+\left[\begin{matrix}n_{14x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 & 0\\n_{14y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & 0 & 0\\n_{14z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & 0 & 0\\0 & n_{14x} & 0 & 0 & 0 & 0\\0 & n_{14y} & 0 & 0 & 0 & 0\\0 & n_{14z} & 0 & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}$$

\[\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[J_1\right]\{\dot{\theta}_a\}+\left[J_2\right]\{\Omega\}\]where $\{\dot{\theta}_a\}=\begin{Bmatrix}\dot{\theta}_{13}\end{Bmatrix}$ and $\{\Omega\}=\begin{Bmatrix}\dot{d}_{14} & \dot{\theta}_{14}&\dot{\theta}_{32}&\omega_{24x}&\omega_{24y}&\omega_{24z}\end{Bmatrix}^T$ represent the active joint-velocities and the passive joint-velocities, respectively.
\newline
But since the Jacobian should contain the end-effector velocities in terms of active joint angles alone, the passive joint angles must be written in terms of active joint angles. From the two equations \eqref{eqn:eqn_1_3_1_1} and \eqref{eqn:eqn_1_3_1_2}, 
\newline
\begin{eqnarray}
  \label{eqn:eqn_1_3_5_1}
  \dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{32} \hat{n}_{32} \times \left( \vec{a} - \vec{r}_{32} \right) + \vec{\omega}_{24} \times \left( \vec{a} - \vec{r}_{24} \right)=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{d}_{14} \hat{n}_{14}\end{eqnarray}

From the two equations \eqref{eqn:eqn_1_3_2_1} and \eqref{eqn:eqn_1_3_2_2},
\newline
\begin{dmath}
  \label{eqn:eqn_1_3_5_2}
  \dot{\theta}_{14} \hat{n}_{14}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{32} \hat{n}_{32} + \vec{\omega}_{24}\end{dmath}
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & - n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & - n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\n_{13x} & 0 & - n_{14x} & n_{32x} & 1 & 0 & 0\\n_{13y} & 0 & - n_{14y} & n_{32y} & 0 & 1 & 0\\n_{13z} & 0 & - n_{14z} & n_{32z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
%\newline
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right)\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right)\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right)\\n_{13x}\\n_{13y}\\n_{13z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\end{Bmatrix}+\left[\begin{matrix}- n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\- n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\- n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\0 & - n_{14x} & n_{32x} & 1 & 0 & 0\\0 & - n_{14y} & n_{32y} & 0 & 1 & 0\\0 & - n_{14z} & n_{32z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
From the equations \eqref{eqn:eqn_1_3_5_1} and \eqref{eqn:eqn_1_3_5_2}, linear equations in terms of active and passive joint angles can be stacked as shown below, using which the passive joint angles can be written in terms of the active joint angles.
\[
\begin{split}
  %%\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & - n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & - n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\n_{13x} & 0 & - n_{14x} & n_{32x} & 1 & 0 & 0\\n_{13y} & 0 & - n_{14y} & n_{32y} & 0 & 1 & 0\\n_{13z} & 0 & - n_{14z} & n_{32z} & 0 & 0 & 1\end{matrix}\right]
  %\Rightarrow
  \left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & - n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) \\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) \\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & - n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) \\n_{13x} & 0 & - n_{14x} \\n_{13y} & 0 & - n_{14y} \\n_{13z} & 0 & - n_{14z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\ - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\ n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\ n_{32x} & 1 & 0 & 0\\ n_{32y} & 0 & 1 & 0\\ n_{32z} & 0 & 0 & 1\end{matrix}\right]
  %\Rightarrow\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & - n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) \\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) \\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & - n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) \\n_{13x} & 0 & - n_{14x} & n_{32x} \\n_{13y} & 0 & - n_{14y} & n_{32y} \\n_{13z} & 0 & - n_{14z} & n_{32z} \end{matrix}\right.\\\qquad\left.\begin{matrix} 0 & a_z - r_{24z} & - a_y + r_{24y}\\ - a_z + r_{24z} & 0 & a_x - r_{24x}\\ a_y - r_{24y} & - a_x + r_{24x} & 0\\ 1 & 0 & 0\\ 0 & 1 & 0\\ 0 & 0 & 1\end{matrix}\right]
  \begin{Bmatrix}\dot{\theta}_{13}\\\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}
  =
  \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
\end{split}
\]

\[
\begin{split}
  \Rightarrow\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right)\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right)\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right)\\n_{13x}\\n_{13y}\\n_{13z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\end{Bmatrix}
  +
  %\left[\begin{matrix}- n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\- n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\- n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\0 & - n_{14x} & n_{32x} & 1 & 0 & 0\\0 & - n_{14y} & n_{32y} & 0 & 1 & 0\\0 & - n_{14z} & n_{32z} & 0 & 0 & 1\end{matrix}\right]
  \left[\begin{matrix}- n_{14x} & - n_{14y} \left(a_z - r_{14z}\right) + n_{14z} \left(a_y - r_{14y}\right) \\- n_{14y} & n_{14x} \left(a_z - r_{14z}\right) - n_{14z} \left(a_x - r_{14x}\right) \\- n_{14z} & - n_{14x} \left(a_y - r_{14y}\right) + n_{14y} \left(a_x - r_{14x}\right) \\0 & - n_{14x} \\0 & - n_{14y} \\0 & - n_{14z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & 0 & a_z - r_{24z} & - a_y + r_{24y}\\ - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - a_z + r_{24z} & 0 & a_x - r_{24x}\\ n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & a_y - r_{24y} & - a_x + r_{24x} & 0\\ n_{32x} & 1 & 0 & 0\\ n_{32y} & 0 & 1 & 0\\ n_{32z} & 0 & 0 & 1\end{matrix}\right]
  \begin{Bmatrix}\dot{d}_{14}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\omega_{24x}\\\omega_{24y}\\\omega_{24z}\end{Bmatrix}
  =
  \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
\end{split}
\]

\[\Rightarrow \left[A_1\right]\{\dot{\theta}_a\}+\left[A_2\right]\{\Omega\}=0\] \[\Rightarrow \{\Omega\}=-\left[A_2\right]^{-1}\left[A_1\right]\{\dot{\theta}_a\}\]\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}=\left[J_1\right] \{\dot{\theta}_a\}+\left[J_2\right] \{\Omega\}=\left[J_1\right] \{\dot{\theta}_a\}-\left[J_2\right]\left[A_2\right]^{-1}\left[A_1\right] \{\dot{\theta}_a\}\]



The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$ would finally be

$$\left[J_1\right]=\left[\begin{matrix}0\\0\\0\\0\\0\\0\end{matrix}\right]$$

$$\left[J_2\right]=\left[\begin{matrix}\sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & 0 & 0 & 0 & 0\\\sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0 & 0 & 0 & 0\\\cos{\left(\beta_{14} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0 & 0 & 0 & 0\\0 & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0 & 0 & 0 & 0\\0 & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & 0 & 0 & 0 & 0\\0 & \cos{\left(\beta_{14} \right)} & 0 & 0 & 0 & 0\end{matrix}\right]$$

$$\left[A_1\right]=\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)}\\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)}\\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)}\\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)}\\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)}\\\cos{\left(\beta_{13} \right)}\end{matrix}\right]$$

%\resizebox{\textwidth}{!}{$\left[A_2\right]=\left[\begin{matrix}- \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 5 - r_{24z} & r_{24y} - 4\\- \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & r_{24z} - 5 & 0 & 3 - r_{24x}\\- \cos{\left(\beta_{14} \right)} & \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} - \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 4 - r_{24y} & r_{24x} - 3 & 0\\0 & - \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 1 & 0 & 0\\0 & - \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 1 & 0\\0 & - \cos{\left(\beta_{14} \right)} & \cos{\left(\beta_{32} \right)} & 0 & 0 & 1\end{matrix}\right]$}
\[
\begin{split}
  \left[A_2\right]
  =
  %\left[\begin{matrix}- \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 5 - r_{24z} & r_{24y} - 4\\- \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & r_{24z} - 5 & 0 & 3 - r_{24x}\\- \cos{\left(\beta_{14} \right)} & \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} - \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 4 - r_{24y} & r_{24x} - 3 & 0\\0 & - \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 1 & 0 & 0\\0 & - \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 1 & 0\\0 & - \cos{\left(\beta_{14} \right)} & \cos{\left(\beta_{32} \right)} & 0 & 0 & 1\end{matrix}\right]
  \left[\begin{matrix}- \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} \\- \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\- \cos{\left(\beta_{14} \right)} & \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} - \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\0 & - \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\0 & - \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} \\0 & - \cos{\left(\beta_{14} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 5 - r_{24z} & r_{24y} - 4\\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & r_{24z} - 5 & 0 & 3 - r_{24x}\\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 4 - r_{24y} & r_{24x} - 3 & 0\\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & 1 & 0 & 0\\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & 0 & 1 & 0\\ \cos{\left(\beta_{32} \right)} & 0 & 0 & 1\end{matrix}\right]
\end{split}
\]

By using the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$, the relation between the active joint velocities and the end-effector velocities can be written as

\[
  %\Rightarrow
  \{\dot{X}\}=\left( \left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] \right) \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]
  
  where $\left[\widetilde{J}\right]=\left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] $ is the Jacobian matrix of the manipulator for the considered actuating joints.
\newline


$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$
Based on the strategy mentioned in section \ref{strategy_used_in_optimisation}, the above optimisation problem is attempted for solution, but it did not pass the criterion mentioned in Step 1. Hence, the modified objective function is taken for optimisation in order to avoid type-2 singularity. The modified optimisation problem would then become
\newline
Maximise\[f_2=\sqrt{\det{\left(\left[\widetilde{A}\right]^T \left[\widetilde{A}\right]\right)} \times \det{\left(\left[\widetilde{B}\right]^T \left[\widetilde{B}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$

\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{13}-\vec{a}\right)\times \hat{n}_{13}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{32}-\vec{a}\right)\times \hat{n}_{32}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{4}=\left|\vec{r}_{24}-\vec{a}\right|  
\end{matrix}
$$

The characteristic length is formulated as follows.
\[L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}+\bar{d}_{4}}{4}\]

By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
\[\left[S\right]=\begin{bmatrix}
  \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
  0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
  0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
  0 & 0 & 0 & 1 & 0 & 0\\
  0 & 0 & 0 & 0 & 1 & 0\\
  0 & 0 & 0 & 0 & 0 & 1\\
  \end{bmatrix}\]
  
  The scaled Jacobian matrix can then be calculated as
  \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
  The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.

\emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in table \ref{Tab:table_3_3} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{13}$ & $\ang{182.04}$ \\
\hline$\phi_{14}$ & $\ang{133.78}$ \\
\hline$\phi_{32}$ & $\ang{245.33}$ \\
\hline$r_{13x}$ & $10.0$ \\
\hline$r_{13y}$ & $10.0$ \\
\hline$r_{13z}$ & $0.0$ \\
\hline$r_{14x}$ & $0.0$ \\
\hline$r_{14y}$ & $0.0$ \\
\hline$r_{14z}$ & $0.0$ \\
\hline$r_{32x}$ & $10.0$ \\
\hline$r_{32y}$ & $0.0$ \\
\hline$r_{32z}$ & $0.0$ \\
\hline$r_{24x}$ & $0.0$ \\
\hline$r_{24y}$ & $10.0$ \\
\hline$r_{24z}$ & $10.0$ \\
\hline$\beta_{13}$ & $\ang{134.98}$ \\
\hline$\beta_{14}$ & $\ang{100.15}$ \\
\hline$\beta_{32}$ & $\ang{63.84}$ \\
\hline\end{tabular} \caption{Result (1D-M3)} \label{Tab:table_3_3} \end{table}
% \begin{table}[h]  \centering \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% Variable & $\phi_{13}$ & $\phi_{14}$ & $\phi_{32}$ & $r_{13x}$ & $r_{13y}$ & $r_{13z}$ & $r_{14x}$ & $r_{14y}$ & $r_{14z}$ & $r_{32x}$ & $r_{32y}$ & $r_{32z}$ & $r_{24x}$ & $r_{24y}$ & $r_{24z}$ & $\beta_{13}$ & $\beta_{14}$ & $\beta_{32}$\\ 
% \hline
% Value & $\ang{182.04}$ & $\ang{133.78}$ & $\ang{245.33}$ & $10.0$ & $10.0$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ & $10.0$ & $0.0$ & $0.0$ & $0.0$ & $10.0$ & $10.0$ & $\ang{134.98}$ & $\ang{100.15}$ & $\ang{63.84}$ \\
% \hline\end{tabular} \caption{Result (1D-M3)} \label{Tab:table_3_3} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{13}=-0.03\hat{i}-0.71\hat{j}-0.71\hat{k} \\
  \hat{n}_{14}=0.71\hat{i}-0.68\hat{j}-0.18\hat{k} \\
  \hat{n}_{32}=-0.82\hat{i}-0.37\hat{j}+0.44\hat{k} \\
  \vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{32}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=15.37\]
And the corresponding condition number is \[\kappa=1\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.0222\]

==> contentfolder/mechanisms2/manipulators/dof2/manipulator_1.tex <==
% \emph{Adjacency matrix of manipulator 2D-M1:}

% The adjacency of the manipulator is\[M_{\text{2D-M1}}=\left[\begin{matrix}L_{1}&O&O&R&O\\O&L_{2}&O&R&R\\O&O&L_{3}&S&S\\R&R&S&L_{4}&O\\O&R&S&O&L_{5}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline

\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/2dof/1.png}
  \caption{Schematic figure of 2D-M1}
  \label{fig_2dof_iext_1}
\end{figure}

\emph{Formulation of Jacobian:}

Jacobian of the manipulator is formulated using the steps shown in section \ref{steps_to_formulate_jacobian}. The various paths that connect the base link and the end-effector link are $L_1-R-L_4-R-L_2-R-L_5$ and $L_1-R-L_4-S-L_3-S-L_5$. The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.

%The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.

\begin{eqnarray}\label{eqn:eqn_2_1_1_2}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{\theta}_{42} \hat{n}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}\begin{eqnarray}\label{eqn:eqn_2_1_1_1}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{43} \times \left( \vec{a} - \vec{r}_{43} \right) + \vec{\omega}_{35} \times \left( \vec{a} - \vec{r}_{35} \right)\end{eqnarray}\begin{dmath}\label{eqn:eqn_2_1_2_2}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \dot{\theta}_{42} \hat{n}_{42} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}\begin{dmath}\label{eqn:eqn_2_1_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{43} + \vec{\omega}_{35}\end{dmath}where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{ij}=\begin{Bmatrix} \omega_{ijx} & \omega_{ijy} & \omega_{ijz} \end{Bmatrix}^T$ represents the relative angular velocity vector of the link $L_j$ relative to the link $L_i$, of the adjacency matrix. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_2_1_1_1} and \eqref{eqn:eqn_2_1_2_1}, the vector of end-effector velocities in terms of both active and passive joint angles is given by
\newline
%\resizebox{\textwidth}{!}{$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 & a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & - a_z + r_{43z} & 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & a_y - r_{43y} & - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\n_{14x} & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0\\n_{14y} & 0 & 0 & 0 & 1 & 0 & 0 & 1 & 0\\n_{14z} & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\\\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}$}


%\resizebox{\textwidth}{!}{$\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0\\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0\\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0\\n_{14x} & 0\\n_{14y} & 0\\n_{14z} & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}+\left[\begin{matrix}0 & 0 & a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\0 & - a_z + r_{43z} & 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\0 & a_y - r_{43y} & - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\0 & 1 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}$}

\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    \begin{Bmatrix} \vec{v} \\ \vec{\omega} \end{Bmatrix}
    =
    %\left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 & a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & - a_z + r_{43z} & 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & a_y - r_{43y} & - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\n_{14x} & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0\\n_{14y} & 0 & 0 & 0 & 1 & 0 & 0 & 1 & 0\\n_{14z} & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]
    \left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0 & 0 & 0 \\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0 & 0 & - a_z + r_{43z} \\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0 & 0 & a_y - r_{43y} \\n_{14x} & 0 & 0 & 1 \\n_{14y} & 0 & 0 & 0 \\n_{14z} & 0 & 0 & 0 \end{matrix}\right.\\\qquad\left.\begin{matrix} a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\ 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\ - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\ 0 & 0 & 1 & 0 & 0\\ 1 & 0 & 0 & 1 & 0\\ 0 & 1 & 0 & 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\\\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}
\end{split}
%$}
\]

\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    \Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}
    =
    \left[\begin{matrix}n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & 0\\- n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & 0\\n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & 0\\n_{14x} & 0\\n_{14y} & 0\\n_{14z} & 0\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}
    +
    %\left[\begin{matrix}0 & 0 & a_z - r_{43z} & - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\0 & - a_z + r_{43z} & 0 & a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\0 & a_y - r_{43y} & - a_x + r_{43x} & 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\0 & 1 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]
    \left[\begin{matrix}0 & 0 & a_z - r_{43z} \\0 & - a_z + r_{43z} & 0 \\0 & a_y - r_{43y} & - a_x + r_{43x} \\0 & 1 & 0 \\0 & 0 & 1 \\0 & 0 & 0 \end{matrix}\right.\\\qquad\left.\begin{matrix} - a_y + r_{43y} & 0 & a_z - r_{35z} & - a_y + r_{35y}\\ a_x - r_{43x} & - a_z + r_{35z} & 0 & a_x - r_{35x}\\ 0 & a_y - r_{35y} & - a_x + r_{35x} & 0\\ 0 & 1 & 0 & 0\\ 0 & 0 & 1 & 0\\ 1 & 0 & 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}
  \end{split}
  %$}
\]

\[\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[J_1\right]\{\dot{\theta}_a\}+\left[J_2\right]\{\Omega\}\]where $\{\dot{\theta}_a\}=\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}$ and $\{\Omega\}=\begin{Bmatrix}\dot{\theta}_{25}&\omega_{43x}&\omega_{43y}&\omega_{43z}&\omega_{35x}&\omega_{35y}&\omega_{35z}\end{Bmatrix}^T$ represent the active joint-velocities and the passive joint-velocities, respectively.
\newline
But since the Jacobian should contain the end-effector velocities in terms of active joint angles alone, the passive joint angles must be written in terms of active joint angles. From the two equations \eqref{eqn:eqn_2_1_1_1} and \eqref{eqn:eqn_2_1_1_2},
\newline
\begin{eqnarray}
  \label{eqn:eqn_2_1_5_1}
  \dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{\theta}_{42} \hat{n}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{43} \times \left( \vec{a} - \vec{r}_{43} \right) + \vec{\omega}_{35} \times \left( \vec{a} - \vec{r}_{35} \right)
\end{eqnarray}
From the two equations \eqref{eqn:eqn_2_1_2_1} and \eqref{eqn:eqn_2_1_2_2},
\newline
\begin{dmath}
  \label{eqn:eqn_2_1_5_2}
  \dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{43} + \vec{\omega}_{35}=\dot{\theta}_{14} \hat{n}_{14} + \dot{\theta}_{42} \hat{n}_{42} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}
For this mechanism, there is a superfluous degree of freedom for the link $L_3$. To avoid uncertainty of the velocity of the link during calculations, an additional constraint is considered as shown below, which does not alter the final velocity of the end-effector.
\begin{eqnarray} 
  \label{eq:superfluous_dof_equation}
  \vec{\omega}_{3}\cdot\left(\vec{r}_{35}-\vec{r}_{43}\right)=0
\end{eqnarray}
\[ \Rightarrow \left(r_{43x} - r_{35x}\right) \left(n_{14x} \dot{\theta}_{14} + \omega_{43x}\right) + \left(r_{43y} - r_{35y}\right) \left(n_{14y} \dot{\theta}_{14} + \omega_{43y}\right) + \left(r_{43z} - r_{35z}\right) \left(n_{14z} \dot{\theta}_{14} + \omega_{43z}\right)=0 \]

%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right) & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} & a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right) & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 & - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right) & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} & 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\0 & n_{42x} & n_{25x} & -1 & 0 & 0 & -1 & 0 & 0\\0 & n_{42y} & n_{25y} & 0 & -1 & 0 & 0 & -1 & 0\\0 & n_{42z} & n_{25z} & 0 & 0 & -1 & 0 & 0 & -1\\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0 & 0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} & r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\\\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\\0\end{Bmatrix}$}
%\newline
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right)\\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right)\\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right)\\0 & n_{42x}\\0 & n_{42y}\\0 & n_{42z}\\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}+\left[\begin{matrix}n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} & a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\- n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 & - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} & 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\n_{25x} & -1 & 0 & 0 & -1 & 0 & 0\\n_{25y} & 0 & -1 & 0 & 0 & -1 & 0\\n_{25z} & 0 & 0 & -1 & 0 & 0 & -1\\0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} & r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\\0\end{Bmatrix}$}
From the equations \eqref{eqn:eqn_2_1_5_1}, \eqref{eqn:eqn_2_1_5_2} and \eqref{eq:superfluous_dof_equation}, linear equations in terms of active and passive joint angles can be stacked as shown below, using which the passive joint angles can be written in terms of the active joint angles.
\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
  %\left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right) & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} & a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right) & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 & - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right) & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} & 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\0 & n_{42x} & n_{25x} & -1 & 0 & 0 & -1 & 0 & 0\\0 & n_{42y} & n_{25y} & 0 & -1 & 0 & 0 & -1 & 0\\0 & n_{42z} & n_{25z} & 0 & 0 & -1 & 0 & 0 & -1\\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0 & 0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} & r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]
  %\Rightarrow
  \left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right) \\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right) \\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right) \\0 & n_{42x} \\0 & n_{42y} \\0 & n_{42z} \\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0 \end{matrix}\right.
  \\
  \qquad
  \left.\begin{matrix} n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} \\ - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 \\ n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} \\ n_{25x} & -1 & 0 \\ n_{25y} & 0 & -1 \\ n_{25z} & 0 & 0 \\ 0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} \end{matrix}\right.
  \\
  \qquad
  \left.\begin{matrix} a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\ - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\ 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\ 0 & -1 & 0 & 0\\ 0 & 0 & -1 & 0\\ -1 & 0 & 0 & -1\\ r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]
\begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\\\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}
=
\begin{Bmatrix}0\\0\\0\\0\\0\\0\\0\end{Bmatrix}
\end{split}
%$}
\]



\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
  \Rightarrow \left[\begin{matrix}0 & n_{42y} \left(a_z - r_{42z}\right) - n_{42z} \left(a_y - r_{42y}\right)\\0 & - n_{42x} \left(a_z - r_{42z}\right) + n_{42z} \left(a_x - r_{42x}\right)\\0 & n_{42x} \left(a_y - r_{42y}\right) - n_{42y} \left(a_x - r_{42x}\right)\\0 & n_{42x}\\0 & n_{42y}\\0 & n_{42z}\\n_{14x} \left(r_{43x} - r_{35x}\right) + n_{14y} \left(r_{43y} - r_{35y}\right) + n_{14z} \left(r_{43z} - r_{35z}\right) & 0\end{matrix}\right]
  \begin{Bmatrix}\dot{\theta}_{14}\\\dot{\theta}_{42}\end{Bmatrix}
  + \\
  \left[\begin{matrix}n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & 0 & - a_z + r_{43z} \\- n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & a_z - r_{43z} & 0 \\n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - a_y + r_{43y} & a_x - r_{43x} \\n_{25x} & -1 & 0 \\n_{25y} & 0 & -1 \\n_{25z} & 0 & 0 \\0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} \end{matrix}\right.\\\qquad\left.\begin{matrix} a_y - r_{43y} & 0 & - a_z + r_{35z} & a_y - r_{35y}\\ - a_x + r_{43x} & a_z - r_{35z} & 0 & - a_x + r_{35x}\\ 0 & - a_y + r_{35y} & a_x - r_{35x} & 0\\ 0 & -1 & 0 & 0\\ 0 & 0 & -1 & 0\\ -1 & 0 & 0 & -1\\ r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]
  \begin{Bmatrix}\dot{\theta}_{25}\\\omega_{43x}\\\omega_{43y}\\\omega_{43z}\\\omega_{35x}\\\omega_{35y}\\\omega_{35z}\end{Bmatrix}
  =
  \begin{Bmatrix}0\\0\\0\\0\\0\\0\\0\end{Bmatrix}
\end{split}
%$}
\]

\[\Rightarrow \left[A_1\right]\{\dot{\theta}_a\}+\left[A_2\right]\{\Omega\}=0\] \[\Rightarrow \{\Omega\}=-\left[A_2\right]^{-1}\left[A_1\right]\{\dot{\theta}_a\}\]\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}=\left[J_1\right] \{\dot{\theta}_a\}+\left[J_2\right] \{\Omega\}=\left[J_1\right] \{\dot{\theta}_a\}-\left[J_2\right]\left[A_2\right]^{-1}\left[A_1\right] \{\dot{\theta}_a\}\]
The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$ would finally be

%\resizebox{\textwidth}{!}{$
$$\left[J_1\right]=\left[\begin{matrix}- \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & 0\\\left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0\\- \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0\\\sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & 0\\\sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & 0\\\cos{\left(\beta_{14} \right)} & 0\end{matrix}\right]$$
%$}

%\resizebox{\textwidth}{!}{$
$$\left[J_2\right]=\left[\begin{matrix}0 & 0 & 5 - r_{43z} & r_{43y} - 4 & 0 & 5 - r_{35z} & r_{35y} - 4\\0 & r_{43z} - 5 & 0 & 3 - r_{43x} & r_{35z} - 5 & 0 & 3 - r_{35x}\\0 & 4 - r_{43y} & r_{43x} - 3 & 0 & 4 - r_{35y} & r_{35x} - 3 & 0\\0 & 1 & 0 & 0 & 1 & 0 & 0\\0 & 0 & 1 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 1 & 0 & 0 & 1\end{matrix}\right]$$
%$}

%\resizebox{\textwidth}{!}{$\left[A_1\right]=\left[\begin{matrix}0 & - \left(4 - r_{42y}\right) \cos{\left(\beta_{42} \right)} + \left(5 - r_{42z}\right) \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)}\\0 & \left(3 - r_{42x}\right) \cos{\left(\beta_{42} \right)} - \left(5 - r_{42z}\right) \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\0 & - \left(3 - r_{42x}\right) \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)} + \left(4 - r_{42y}\right) \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\0 & \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\0 & \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)}\\0 & \cos{\left(\beta_{42} \right)}\\\left(r_{43x} - r_{35x}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} + \left(r_{43y} - r_{35y}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(r_{43z} - r_{35z}\right) \cos{\left(\beta_{14} \right)} & 0\end{matrix}\right]$}

%\resizebox{\textwidth}{!}{$\left[A_2\right]=\left[\begin{matrix}- \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & 0 & r_{43z} - 5 & 4 - r_{43y} & 0 & r_{35z} - 5 & 4 - r_{35y}\\\left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & 5 - r_{43z} & 0 & r_{43x} - 3 & 5 - r_{35z} & 0 & r_{35x} - 3\\- \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & r_{43y} - 4 & 3 - r_{43x} & 0 & r_{35y} - 4 & 3 - r_{35x} & 0\\\sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & -1 & 0 & 0 & -1 & 0 & 0\\\sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & 0 & -1 & 0 & 0 & -1 & 0\\\cos{\left(\beta_{25} \right)} & 0 & 0 & -1 & 0 & 0 & -1\\0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} & r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]$}

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
  \left[A_1\right]=\left[\begin{matrix}0 \\0 \\0 \\0 \\0 \\0 \\\left(r_{43x} - r_{35x}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} + \left(r_{43y} - r_{35y}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(r_{43z} - r_{35z}\right) \cos{\left(\beta_{14} \right)} \end{matrix}\right.
  \\
  \qquad\left.\begin{matrix} - \left(4 - r_{42y}\right) \cos{\left(\beta_{42} \right)} + \left(5 - r_{42z}\right) \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)}\\ \left(3 - r_{42x}\right) \cos{\left(\beta_{42} \right)} - \left(5 - r_{42z}\right) \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\ - \left(3 - r_{42x}\right) \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)} + \left(4 - r_{42y}\right) \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\ \sin{\left(\beta_{42} \right)} \cos{\left(\phi_{42} \right)}\\ \sin{\left(\phi_{42} \right)} \sin{\left(\beta_{42} \right)}\\ \cos{\left(\beta_{42} \right)}\\ 0\end{matrix}\right]
  \end{split}
\]

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \left[A_2\right]=\left[\begin{matrix}- \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & 0 & r_{43z} - 5 \\\left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & 5 - r_{43z} & 0 \\- \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & r_{43y} - 4 & 3 - r_{43x} \\\sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & -1 & 0 \\\sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & 0 & -1 \\\cos{\left(\beta_{25} \right)} & 0 & 0 \\0 & r_{43x} - r_{35x} & r_{43y} - r_{35y} \end{matrix}\right.\\\qquad\left.\begin{matrix} 4 - r_{43y} & 0 & r_{35z} - 5 & 4 - r_{35y}\\ r_{43x} - 3 & 5 - r_{35z} & 0 & r_{35x} - 3\\ 0 & r_{35y} - 4 & 3 - r_{35x} & 0\\ 0 & -1 & 0 & 0\\ 0 & 0 & -1 & 0\\ -1 & 0 & 0 & -1\\ r_{43z} - r_{35z} & 0 & 0 & 0\end{matrix}\right]
  \end{split}
\]

By using the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$, the relation between the active joint velocities and the end-effector velocities can be written as

\[
  %\Rightarrow
   \{\dot{X}\}=\left( \left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] \right) \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]
   where $\left[\widetilde{J}\right]=\left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] $ is the Jacobian matrix of the manipulator for the considered actuating joints.
\newline

$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$
Based on the strategy mentioned in section \ref{strategy_used_in_optimisation}, the above optimisation problem is attempted for solution, but it did not pass the criterion mentioned in Step 1. Hence, the modified objective function is taken for optimisation in order to avoid type-2 singularity. The modified optimisation problem would then become
\newline
Maximise\[f_2=\sqrt{\det{\left(\left[\widetilde{A}\right]^T \left[\widetilde{A}\right]\right)} \times \det{\left(\left[\widetilde{B}\right]^T \left[\widetilde{B}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$

\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{42}-\vec{a}\right)\times \hat{n}_{42}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{25}-\vec{a}\right)\times \hat{n}_{25}\right| \\
  \bar{d}_{4}=\left|\vec{r}_{43}-\vec{a}\right| \\
  \bar{d}_{5}=\left|\vec{r}_{35}-\vec{a}\right|
\end{matrix}
$$

The characteristic length is formulated as follows.
\[L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}+\bar{d}_{4}+\bar{d}_{5}}{5}\]



By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
\[\left[S\right]=\begin{bmatrix}
  \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
  0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
  0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
  0 & 0 & 0 & 1 & 0 & 0\\
  0 & 0 & 0 & 0 & 1 & 0\\
  0 & 0 & 0 & 0 & 0 & 1\\
  \end{bmatrix}\]
  
  The scaled Jacobian matrix can then be calculated as
  \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
  The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.

\emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in table \ref{Tab:table_4_1} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{14}$ & $\ang{0.0}$ \\
\hline$\phi_{42}$ & $\ang{292.2}$ \\
\hline$\phi_{25}$ & $\ang{171.62}$ \\
\hline$r_{14x}$ & $0.0$ \\
\hline$r_{14y}$ & $0.0$ \\
\hline$r_{14z}$ & $10.0$ \\
\hline$r_{42x}$ & $10.0$ \\
\hline$r_{42y}$ & $10.0$ \\
\hline$r_{42z}$ & $0.0$ \\
\hline$r_{25x}$ & $10.0$ \\
\hline$r_{25y}$ & $0.0$ \\
\hline$r_{25z}$ & $10.0$ \\
\hline$r_{43x}$ & $0.0$ \\
\hline$r_{43y}$ & $0.0$ \\
\hline$r_{43z}$ & $0.0$ \\
\hline$r_{35x}$ & $10.0$ \\
\hline$r_{35y}$ & $10.0$ \\
\hline$r_{35z}$ & $10.0$ \\
\hline$\beta_{14}$ & $\ang{73.92}$ \\
\hline$\beta_{42}$ & $\ang{121.39}$ \\
\hline$\beta_{25}$ & $\ang{42.39}$ \\
\hline\end{tabular} \caption{Result (2D-M1)} \label{Tab:table_4_1} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{14}=0.0\hat{i}+0.96\hat{j}+0.28\hat{k} \\
  \hat{n}_{42}=-0.79\hat{i}+0.32\hat{j}-0.52\hat{k} \\
  \hat{n}_{25}=0.1\hat{i}-0.67\hat{j}+0.74\hat{k} \\
  \vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{42}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{43}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=73.96\]
And the corresponding condition number is \[\kappa=1.87\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.106\]

==> contentfolder/mechanisms2/manipulators/dof2/manipulator_71.tex <==
% \emph{Adjacency matrix of manipulator 2D-M71:}

% The adjacency of the manipulator is\[M_{\text{2D-M71}}=\left[\begin{matrix}L_{1}&O&R&R&O\\O&L_{2}&O&S&R\\R&O&L_{3}&O&C\\R&S&O&L_{4}&O\\O&R&C&O&L_{5}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline

\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/2dof/71.png}
  \caption{Schematic figure of 2D-M71}
  \label{fig_2dof_iext_71}
\end{figure}


\emph{Formulation of Jacobian:}

Jacobian of the manipulator is formulated using the steps shown in section \ref{steps_to_formulate_jacobian}. The various paths that connect the base link and the end-effector link are $L_1-R-L_3-C-L_5$ and $L_1-R-L_4-S-L_2-R-L_5$. The descriptions of linear and angular velocities of the end-effector is formulated using various paths from the end-effector link to the base link, and shown by the equations below.
\begin{eqnarray}\label{eqn:eqn_2_71_1_2}\vec{v}=\dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{35} \hat{n}_{35} \times \left( \vec{a} - \vec{r}_{35} \right) + \dot{d}_{35} \hat{n}_{35}\end{eqnarray}\begin{eqnarray}\label{eqn:eqn_2_71_1_1}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}\begin{dmath}\label{eqn:eqn_2_71_2_2}\vec{\omega}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{35} \hat{n}_{35}\end{dmath}\begin{dmath}\label{eqn:eqn_2_71_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{42} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{ij}=\begin{Bmatrix} \omega_{ijx} & \omega_{ijy} & \omega_{ijz} \end{Bmatrix}^T$ represents the relative angular velocity vector of the link $L_j$ relative to the link $L_i$, of the adjacency matrix. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_2_1}, the vector of end-effector velocities in terms of both active and passive joint angles is given by
%From equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_2_1},
\newline
%\resizebox{\textwidth}{!}{$
$$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & 0 & n_{35x} & 0 & n_{35y} \left(a_z - r_{35z}\right) - n_{35z} \left(a_y - r_{35y}\right) & 0 & 0 & 0\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & 0 & n_{35y} & 0 & - n_{35x} \left(a_z - r_{35z}\right) + n_{35z} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & 0 & n_{35z} & 0 & n_{35x} \left(a_y - r_{35y}\right) - n_{35y} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\n_{13x} & 0 & 0 & 0 & n_{35x} & 0 & 0 & 0\\n_{13y} & 0 & 0 & 0 & n_{35y} & 0 & 0 & 0\\n_{13z} & 0 & 0 & 0 & n_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}$$
%$}


\resizebox{\textwidth}{!}{$\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & 0\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & 0\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & 0\\n_{13x} & 0\\n_{13y} & 0\\n_{13z} & 0\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}+\left[\begin{matrix}n_{35x} & 0 & n_{35y} \left(a_z - r_{35z}\right) - n_{35z} \left(a_y - r_{35y}\right) & 0 & 0 & 0\\n_{35y} & 0 & - n_{35x} \left(a_z - r_{35z}\right) + n_{35z} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\n_{35z} & 0 & n_{35x} \left(a_y - r_{35y}\right) - n_{35y} \left(a_x - r_{35x}\right) & 0 & 0 & 0\\0 & 0 & n_{35x} & 0 & 0 & 0\\0 & 0 & n_{35y} & 0 & 0 & 0\\0 & 0 & n_{35z} & 0 & 0 & 0\end{matrix}\right]\begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}$}
\[\Rightarrow \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[J_1\right]\{\dot{\theta}_a\}+\left[J_2\right]\{\Omega\}\]where $\{\dot{\theta}_a\}=\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}$ and $\{\Omega\}=\begin{Bmatrix}\dot{d}_{35}&\dot{\theta}_{25}&\dot{\theta}_{35}&\omega_{42x}&\omega_{42y}&\omega_{42z}\end{Bmatrix}^T$ represent the active joint-velocities and the passive joint-velocities, respectively.
\newline
But since the Jacobian should contain the end-effector velocities in terms of active joint angles alone, the passive joint angles must be written in terms of active joint angles. From the two equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_1_2},
%From the equations \eqref{eqn:eqn_2_71_1_1} and \eqref{eqn:eqn_2_71_1_2},
\newline
\begin{eqnarray}
  \label{eqn:eqn_2_71_5_1}
  \dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{35} \hat{n}_{35} \times \left( \vec{a} - \vec{r}_{35} \right) + \dot{d}_{35} \hat{n}_{35}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \vec{\omega}_{42} \times \left( \vec{a} - \vec{r}_{42} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}
From the two equations \eqref{eqn:eqn_2_71_2_1} and \eqref{eqn:eqn_2_71_2_2},
\newline
\begin{dmath}
  \label{eqn:eqn_2_71_5_2}
  \dot{\theta}_{14} \hat{n}_{14} + \vec{\omega}_{42} + \dot{\theta}_{25} \hat{n}_{25}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{35} \hat{n}_{35}\end{dmath}
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\- n_{13x} & n_{14x} & 0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\- n_{13y} & n_{14y} & 0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\- n_{13z} & n_{14z} & 0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
%\newline
%$\Rightarrow$\resizebox{\textwidth}{!}{$\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right)\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right)\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right)\\- n_{13x} & n_{14x}\\- n_{13y} & n_{14y}\\- n_{13z} & n_{14z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}+\left[\begin{matrix}- n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\- n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]\begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}=\begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}$}
From the equations \eqref{eqn:eqn_2_71_5_1} and \eqref{eqn:eqn_2_71_5_2}, linear equations in terms of active and passive joint angles can be stacked as shown below, using which the passive joint angles can be written in terms of the active joint angles.
\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    %\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\- n_{13x} & n_{14x} & 0 & n_{25x} & - n_{35x} & 1 & 0 & 0\\- n_{13y} & n_{14y} & 0 & n_{25y} & - n_{35y} & 0 & 1 & 0\\- n_{13z} & n_{14z} & 0 & n_{25z} & - n_{35z} & 0 & 0 & 1\end{matrix}\right]
    %\Rightarrow\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) \\- n_{13x} & n_{14x} & 0 & n_{25x} \\- n_{13y} & n_{14y} & 0 & n_{25y} \\- n_{13z} & n_{14z} & 0 & n_{25z} \end{matrix}\right.\\\qquad\left.\begin{matrix} - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\ n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\ - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\ - n_{35x} & 1 & 0 & 0\\ - n_{35y} & 0 & 1 & 0\\ - n_{35z} & 0 & 0 & 1\end{matrix}\right]
    %\Rightarrow
    \left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & - n_{35x} \\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{35y} \\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & - n_{35z} \\- n_{13x} & n_{14x} & 0 \\- n_{13y} & n_{14y} & 0 \\- n_{13z} & n_{14z} & 0 \end{matrix}\right.
    \\
    \qquad
    \left.\begin{matrix} n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) & - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) \\ - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) & n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) \\ n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) & - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) \\ n_{25x} & - n_{35x} \\ n_{25y} & - n_{35y} \\ n_{25z} & - n_{35z} \end{matrix}\right.\\\qquad\left.\begin{matrix} 0 & a_z - r_{42z} & - a_y + r_{42y}\\ - a_z + r_{42z} & 0 & a_x - r_{42x}\\ a_y - r_{42y} & - a_x + r_{42x} & 0\\ 1 & 0 & 0\\ 0 & 1 & 0\\ 0 & 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\\\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}
    =
    \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
  \end{split}
  %$}
\]

\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    \Rightarrow\left[\begin{matrix}- n_{13y} \left(a_z - r_{13z}\right) + n_{13z} \left(a_y - r_{13y}\right) & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right)\\n_{13x} \left(a_z - r_{13z}\right) - n_{13z} \left(a_x - r_{13x}\right) & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right)\\- n_{13x} \left(a_y - r_{13y}\right) + n_{13y} \left(a_x - r_{13x}\right) & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right)\\- n_{13x} & n_{14x}\\- n_{13y} & n_{14y}\\- n_{13z} & n_{14z}\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{14}\end{Bmatrix}
    + \\
    \left[\begin{matrix}- n_{35x} & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right) \\- n_{35y} & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right) \\- n_{35z} & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right) \\0 & n_{25x} \\0 & n_{25y} \\0 & n_{25z} \end{matrix}\right.\\\qquad\left.\begin{matrix} - n_{35y} \left(a_z - r_{35z}\right) + n_{35z} \left(a_y - r_{35y}\right) & 0 & a_z - r_{42z} & - a_y + r_{42y}\\ n_{35x} \left(a_z - r_{35z}\right) - n_{35z} \left(a_x - r_{35x}\right) & - a_z + r_{42z} & 0 & a_x - r_{42x}\\ - n_{35x} \left(a_y - r_{35y}\right) + n_{35y} \left(a_x - r_{35x}\right) & a_y - r_{42y} & - a_x + r_{42x} & 0\\ - n_{35x} & 1 & 0 & 0\\ - n_{35y} & 0 & 1 & 0\\ - n_{35z} & 0 & 0 & 1\end{matrix}\right]
    \begin{Bmatrix}\dot{d}_{35}\\\dot{\theta}_{25}\\\dot{\theta}_{35}\\\omega_{42x}\\\omega_{42y}\\\omega_{42z}\end{Bmatrix}
    =
    \begin{Bmatrix}0\\0\\0\\0\\0\\0\end{Bmatrix}
  \end{split}
  %$}
\]

\[\Rightarrow \left[A_1\right]\{\dot{\theta}_a\}+\left[A_2\right]\{\Omega\}=0\] \[\Rightarrow \{\Omega\}=-\left[A_2\right]^{-1}\left[A_1\right]\{\dot{\theta}_a\}\]\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}=\left[J_1\right] \{\dot{\theta}_a\}+\left[J_2\right] \{\Omega\}=\left[J_1\right] \{\dot{\theta}_a\}-\left[J_2\right]\left[A_2\right]^{-1}\left[A_1\right] \{\dot{\theta}_a\}\]
The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$ would finally be

%\resizebox{\textwidth}{!}{$
$$\left[J_1\right]=\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & 0\\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & 0\\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & 0\\\cos{\left(\beta_{13} \right)} & 0\end{matrix}\right]$$
%$}

%\resizebox{\textwidth}{!}{$
$$\left[J_2\right]=\left[\begin{matrix}\sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 & - \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 0 & 0\\\sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 & 0 & 0\\\cos{\left(\beta_{35} \right)} & 0 & - \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} + \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 & 0 & 0\\0 & 0 & \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 0 & 0 & 0\\0 & 0 & \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 0 & 0\\0 & 0 & \cos{\left(\beta_{35} \right)} & 0 & 0 & 0\end{matrix}\right]$$
%$}

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \left[A_1\right]=\left[\begin{matrix}\left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\- \left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} - \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\- \cos{\left(\beta_{13} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\ \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\ \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\ \cos{\left(\beta_{14} \right)}\end{matrix}\right]
  \end{split}
\]

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \left[A_2\right]=\left[\begin{matrix}- \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} \\- \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\- \cos{\left(\beta_{35} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\0 & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} \\0 & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} \\0 & \cos{\left(\beta_{25} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 5 - r_{42z} & r_{42y} - 4\\ - \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & r_{42z} - 5 & 0 & 3 - r_{42x}\\ \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} - \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 4 - r_{42y} & r_{42x} - 3 & 0\\ - \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 1 & 0 & 0\\ - \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 1 & 0\\ - \cos{\left(\beta_{35} \right)} & 0 & 0 & 1\end{matrix}\right]
  \end{split}
\]

%\resizebox{\textwidth}{!}{$A_1=\left[\begin{matrix}\left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\- \left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\\left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} - \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\- \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)}\\- \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)}\\- \cos{\left(\beta_{13} \right)} & \cos{\left(\beta_{14} \right)}\end{matrix}\right]$}

%\resizebox{\textwidth}{!}{$A_2=\left[\begin{matrix}- \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & \left(4 - r_{35y}\right) \cos{\left(\beta_{35} \right)} - \left(5 - r_{35z}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 5 - r_{42z} & r_{42y} - 4\\- \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & - \left(3 - r_{35x}\right) \cos{\left(\beta_{35} \right)} + \left(5 - r_{35z}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & r_{42z} - 5 & 0 & 3 - r_{42x}\\- \cos{\left(\beta_{35} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & \left(3 - r_{35x}\right) \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} - \left(4 - r_{35y}\right) \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 4 - r_{42y} & r_{42x} - 3 & 0\\0 & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)} & - \sin{\left(\beta_{35} \right)} \cos{\left(\phi_{35} \right)} & 1 & 0 & 0\\0 & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} & - \sin{\left(\phi_{35} \right)} \sin{\left(\beta_{35} \right)} & 0 & 1 & 0\\0 & \cos{\left(\beta_{25} \right)} & - \cos{\left(\beta_{35} \right)} & 0 & 0 & 1\end{matrix}\right]$}
By using the matrices $\left[J_1\right]$, $\left[J_2\right]$, $\left[A_1\right]$ and $\left[A_2\right]$, the relation between the active joint velocities and the end-effector velocities can be written as

\[
  %\Rightarrow
   \{\dot{X}\}=\left( \left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] \right) \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]
   where $\left[\widetilde{J}\right]=\left[J_1\right]-\left[J_2\right] \left[A_2\right]^{-1} \left[A_1\right] $ is the Jacobian matrix of the manipulator for the considered actuating joints.
\newline

$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$
Based on the strategy mentioned in section \ref{strategy_used_in_optimisation}, the above optimisation problem is attempted for solution, but it did not pass the criterion mentioned in Step 1. Hence, the modified objective function is taken for optimisation in order to avoid type-2 singularity. The modified optimisation problem would then become
\newline
Maximise\[f_2=\sqrt{\det{\left(\left[\widetilde{A}\right]^T \left[\widetilde{A}\right]\right)} \times \det{\left(\left[\widetilde{B}\right]^T \left[\widetilde{B}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$

\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{13}-\vec{a}\right)\times \hat{n}_{13}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{25}-\vec{a}\right)\times \hat{n}_{25}\right| \\
  \bar{d}_{4}=\left|\left(\vec{r}_{35}-\vec{a}\right)\times \hat{n}_{35}\right| \\
  \bar{d}_{5}=\left|\vec{r}_{42}-\vec{a}\right|
\end{matrix}
$$


The characteristic length is formulated as follows.
\[L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}+\bar{d}_{4}+\bar{d}_{5}}{5}\]



By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
\[\left[S\right]=\begin{bmatrix}
  \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
  0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
  0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
  0 & 0 & 0 & 1 & 0 & 0\\
  0 & 0 & 0 & 0 & 1 & 0\\
  0 & 0 & 0 & 0 & 0 & 1\\
  \end{bmatrix}\]
  
  The scaled Jacobian matrix can then be calculated as
  \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
  The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.

\emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in Table \ref{Tab:table_5_71} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{13}$ & $\ang{360.0}$ \\
\hline$\phi_{14}$ & $\ang{104.74}$ \\
\hline$\phi_{25}$ & $\ang{347.83}$ \\
\hline$\phi_{35}$ & $\ang{32.44}$ \\
\hline$r_{13x}$ & $10.0$ \\
\hline$r_{13y}$ & $10.0$ \\
\hline$r_{13z}$ & $10.0$ \\
\hline$r_{14x}$ & $10.0$ \\
\hline$r_{14y}$ & $10.0$ \\
\hline$r_{14z}$ & $0.0$ \\
\hline$r_{42x}$ & $10.0$ \\
\hline$r_{42y}$ & $0.0$ \\
\hline$r_{42z}$ & $10.0$ \\
\hline$r_{25x}$ & $0.0$ \\
\hline$r_{25y}$ & $0.0$ \\
\hline$r_{25z}$ & $0.0$ \\
\hline$r_{35x}$ & $0.0$ \\
\hline$r_{35y}$ & $10.0$ \\
\hline$r_{35z}$ & $0.0$ \\
\hline$\beta_{13}$ & $\ang{137.39}$ \\
\hline$\beta_{14}$ & $\ang{45.96}$ \\
\hline$\beta_{25}$ & $\ang{134.35}$ \\
\hline$\beta_{35}$ & $\ang{68.46}$ \\
\hline\end{tabular} \caption{Result (2D-M71)} \label{Tab:table_5_71} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k} \\
  \hat{n}_{14}=0.7\hat{i}-0.18\hat{j}+0.7\hat{k} \\
  \hat{n}_{25}=-0.15\hat{i}+0.7\hat{j}-0.7\hat{k} \\
  \hat{n}_{35}=0.5\hat{i}+0.78\hat{j}+0.37\hat{k} \\
  \vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{42}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=173.16\]

And the corresponding condition number is \[\kappa=1.98\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.2305\]

==> contentfolder/mechanisms2/manipulators/dof3/manipulator_1.tex <==
% \emph{Adjacency matrix of manipulator 3D-M1:}

% The adjacency of the manipulator is\[M_{\text{3D-M1}}=\left[\begin{matrix}L_{1}&O&R&O\\O&L_{2}&R&R\\R&R&L_{3}&O\\O&R&O&L_{4}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline

\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/3dof/1.png}
  \caption{Schematic figure of 3D-M1}
  \label{fig_3dof_iext_1}
\end{figure}


\emph{Formulation of Jacobian:}

Since this is a serial manipulator, there would be only one path that connects the base link and the end-effector link. That path is $L_1-R-L_3-R-L_2-R-L_4$. Hence, through this path, the linear velocity of the end-effector link is given by
\begin{eqnarray}\label{eqn:eqn_3_1_1_1}\vec{v}=\dot{\theta}_{13} \hat{n}_{13} \times \left( \vec{a} - \vec{r}_{13} \right) + \dot{\theta}_{32} \hat{n}_{32} \times \left( \vec{a} - \vec{r}_{32} \right) + \dot{\theta}_{24} \hat{n}_{24} \times \left( \vec{a} - \vec{r}_{24} \right)\end{eqnarray}
And the angular velocity of the end-effector link is given by
\begin{dmath}\label{eqn:eqn_3_1_2_1}\vec{\omega}=\dot{\theta}_{13} \hat{n}_{13} + \dot{\theta}_{32} \hat{n}_{32} + \dot{\theta}_{24} \hat{n}_{24}\end{dmath}\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}\]where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ represents the rotational joint velocity of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
%where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$, and $\vec{\omega}_{k}=\begin{Bmatrix} \omega_{kx} & \omega_{ky} & \omega_{kz} \end{Bmatrix}^T$ represents the angular velocity vector of the link $L_k$, of the adjacency matrix. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector, and $\dot{\theta}_{ij}$ and $\dot{d}_{ij}$ represent the translational and the rotational joint velocities respectively, of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix.
\newline
From equations \eqref{eqn:eqn_3_1_1_1} and \eqref{eqn:eqn_3_1_2_1}, the vector of end-effector velocities in terms of active passive joint angles is given by
%\newline
%\resizebox{\textwidth}{!}{$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & n_{24y} \left(a_z - r_{24z}\right) - n_{24z} \left(a_y - r_{24y}\right)\\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - n_{24x} \left(a_z - r_{24z}\right) + n_{24z} \left(a_x - r_{24x}\right)\\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & n_{24x} \left(a_y - r_{24y}\right) - n_{24y} \left(a_x - r_{24x}\right)\\n_{13x} & n_{32x} & n_{24x}\\n_{13y} & n_{32y} & n_{24y}\\n_{13z} & n_{32z} & n_{24z}\end{matrix}\right]\begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{32}\\\dot{\theta}_{24}\end{Bmatrix}$}

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}
    =
    \left[\begin{matrix}n_{13y} \left(a_z - r_{13z}\right) - n_{13z} \left(a_y - r_{13y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) \\- n_{13x} \left(a_z - r_{13z}\right) + n_{13z} \left(a_x - r_{13x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) \\n_{13x} \left(a_y - r_{13y}\right) - n_{13y} \left(a_x - r_{13x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) \\n_{13x} & n_{32x} \\n_{13y} & n_{32y} \\n_{13z} & n_{32z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{24y} \left(a_z - r_{24z}\right) - n_{24z} \left(a_y - r_{24y}\right)\\ - n_{24x} \left(a_z - r_{24z}\right) + n_{24z} \left(a_x - r_{24x}\right)\\ n_{24x} \left(a_y - r_{24y}\right) - n_{24y} \left(a_x - r_{24x}\right)\\ n_{24x}\\ n_{24y}\\ n_{24z}\end{matrix}\right]
    \begin{Bmatrix}\dot{\theta}_{13}\\\dot{\theta}_{32}\\\dot{\theta}_{24}\end{Bmatrix}
  \end{split}
\]

The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrix $\left[J_1\right]$ would finally be
%\resizebox{\textwidth}{!}{$J_1=\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{24y}\right) \cos{\left(\beta_{24} \right)} + \left(5 - r_{24z}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{24x}\right) \cos{\left(\beta_{24} \right)} - \left(5 - r_{24z}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{24x}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)} + \left(4 - r_{24y}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\\cos{\left(\beta_{13} \right)} & \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{24} \right)}\end{matrix}\right]$}

\[
  %\resizebox{\textwidth}{!}{$
  \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \begin{split}
    \left[J_1\right]
    =
    %\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\\cos{\left(\beta_{13} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{24y}\right) \cos{\left(\beta_{24} \right)} + \left(5 - r_{24z}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{24x}\right) \cos{\left(\beta_{24} \right)} - \left(5 - r_{24z}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{24x}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)} + \left(4 - r_{24y}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\ \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{24} \right)}\end{matrix}\right]
    %\left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\\cos{\left(\beta_{13} \right)} & \cos{\left(\beta_{32} \right)} \end{matrix}\right.
    \left[\begin{matrix}- \left(4 - r_{13y}\right) \cos{\left(\beta_{13} \right)} + \left(5 - r_{13z}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\\left(3 - r_{13x}\right) \cos{\left(\beta_{13} \right)} - \left(5 - r_{13z}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\- \left(3 - r_{13x}\right) \sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} + \left(4 - r_{13y}\right) \sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\sin{\left(\beta_{13} \right)} \cos{\left(\phi_{13} \right)} \\\sin{\left(\phi_{13} \right)} \sin{\left(\beta_{13} \right)} \\\cos{\left(\beta_{13} \right)} \end{matrix}\right.
    \\
    \qquad
    \left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\ \cos{\left(\beta_{32} \right)} \end{matrix}\right.
    \\
    \qquad
    \left.\begin{matrix} - \left(4 - r_{24y}\right) \cos{\left(\beta_{24} \right)} + \left(5 - r_{24z}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\ \left(3 - r_{24x}\right) \cos{\left(\beta_{24} \right)} - \left(5 - r_{24z}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ - \left(3 - r_{24x}\right) \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)} + \left(4 - r_{24y}\right) \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ \sin{\left(\beta_{24} \right)} \cos{\left(\phi_{24} \right)}\\ \sin{\left(\phi_{24} \right)} \sin{\left(\beta_{24} \right)}\\ \cos{\left(\beta_{24} \right)}\end{matrix}\right]
  \end{split}
  %$}
\]
Hence, the relation between the active joint velocities and the end-effector velocities can be written as
\[
  %\Rightarrow
  \{\dot{X}\}=\left[J_1\right] \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]where $\left[\widetilde{J}\right]=\left[J_1\right]$.
\newline



$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise
$$f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}$$

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$


\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{13}-\vec{a}\right)\times \hat{n}_{13}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{32}-\vec{a}\right)\times \hat{n}_{32}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{24}-\vec{a}\right)\times \hat{n}_{24}\right|
\end{matrix}
$$

The characteristic length is formulated as follows.
\[
  L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}}{3}
  \]

  By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
  \[\left[S\right]=\begin{bmatrix}
    \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
    0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
    0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
    0 & 0 & 0 & 1 & 0 & 0\\
    0 & 0 & 0 & 0 & 1 & 0\\
    0 & 0 & 0 & 0 & 0 & 1\\
    \end{bmatrix}\]
    
    The scaled Jacobian matrix can then be calculated as
    \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
    The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.
  
  \emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in Table \ref{Tab:table_5_1} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{13}$ & $\ang{278.57}$ \\
\hline$\phi_{32}$ & $\ang{359.53}$ \\
\hline$\phi_{24}$ & $\ang{119.26}$ \\
\hline$r_{13x}$ & $10.0$ \\
\hline$r_{13y}$ & $10.0$ \\
\hline$r_{13z}$ & $0.0$ \\
\hline$r_{23x}$ & $10.0$ \\
\hline$r_{23y}$ & $0.0$ \\
\hline$r_{23z}$ & $10.0$ \\
\hline$r_{24x}$ & $10.0$ \\
\hline$r_{24y}$ & $10.0$ \\
\hline$r_{24z}$ & $10.0$ \\
\hline$\beta_{13}$ & $\ang{134.36}$ \\
\hline$\beta_{32}$ & $\ang{144.59}$ \\
\hline$\beta_{24}$ & $\ang{109.92}$ \\
\hline\end{tabular} \caption{Result (3D-M1)} \label{Tab:table_5_1} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{13}=-0.71\hat{i}+0.11\hat{j}-0.7\hat{k} \\
  \hat{n}_{32}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k} \\
  \hat{n}_{24}=0.82\hat{i}-0.46\hat{j}-0.34\hat{k} \\
  \vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=1058.87\]
And the corresponding condition number is \[\kappa=1.48\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=1.0113\]

==> contentfolder/mechanisms2/manipulators/dof4/manipulator_2.tex <==
% \emph{Adjacency matrix of manipulator 4D-M2:}

% The adjacency of the manipulator is\[M_{\text{4D-M2}}=\left[\begin{matrix}L_{1}&O&O&R&O\\O&L_{2}&R&O&R\\O&R&L_{3}&P&O\\R&O&P&L_{4}&O\\O&R&O&O&L_{5}\end{matrix}\right]\] where $L_1$ is the base-link and $L_4$ is the end-effector link.
% \newline

\begin{figure}[hb]
  \centering
  \includegraphics[width=0.4\linewidth]{contentfolder/images/4dof/2.png}
  \caption{Schematic figure of 4D-M2}
  \label{fig_4dof_iext_2}
\end{figure}


\emph{Formulation of Jacobian:}

Since this is a serial manipulator, there would be only one path that connects the base link and the end-effector link. That path is $L_1-R-L_4-P-L_3-R-L_2-R-L_5$. Hence, through this path, the linear velocity of the end-effector link is given by
\begin{eqnarray}\label{eqn:eqn_4_2_1_1}\vec{v}=\dot{\theta}_{14} \hat{n}_{14} \times \left( \vec{a} - \vec{r}_{14} \right) + \dot{d}_{43} \hat{n}_{43} + \dot{\theta}_{32} \hat{n}_{32} \times \left( \vec{a} - \vec{r}_{32} \right) + \dot{\theta}_{25} \hat{n}_{25} \times \left( \vec{a} - \vec{r}_{25} \right)\end{eqnarray}
And the angular velocity of the end-effector link is given by
\begin{dmath}\label{eqn:eqn_4_2_2_1}\vec{\omega}=\dot{\theta}_{14} \hat{n}_{14} + \dot{\theta}_{32} \hat{n}_{32} + \dot{\theta}_{25} \hat{n}_{25}\end{dmath}\[\therefore \{\dot{X}\}=\left[J\right] \{\dot{\theta}\}\]where $\vec{r}_{ij}=\begin{Bmatrix} r_{ijx} & r_{ijy} & r_{ijz} \end{Bmatrix}^T$ and $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ represent the position vector of the instantaneous location and the axis of the instantaneous motion respectively, of the joint connected to the links $L_i$ \& $L_j$. $\vec{a}=\begin{Bmatrix} a_{x} & a_{y} & a_{z} \end{Bmatrix}^T$ is the position vector of the end-effector. $\dot{\theta}_{ij}$ represents the rotational joint velocity of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$. And $\dot{d}_{ij}$ represents the translational joint velocity of the joint connected to the links $L_i$ and $L_j$ of the adjacency matrix, measured relative to the link $L_i$.
\newline
From equations \eqref{eqn:eqn_4_2_1_1} and \eqref{eqn:eqn_4_2_2_1}, the vector of end-effector velocities in terms of active passive joint angles is given by
\newline
%\resizebox{\textwidth}{!}{$\begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}=\left[\begin{matrix}n_{43x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right)\\n_{43y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right)\\n_{43z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right)\\0 & n_{14x} & n_{32x} & n_{25x}\\0 & n_{14y} & n_{32y} & n_{25y}\\0 & n_{14z} & n_{32z} & n_{25z}\end{matrix}\right]\begin{Bmatrix}\dot{d}_{43}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\dot{\theta}_{25}\end{Bmatrix}$}

\[
  %\resizebox{\textwidth}{!}{$$}
  \begin{split}
    \begin{Bmatrix}\vec{v} \\ \vec{\omega} \end{Bmatrix}
    =
    %\left[\begin{matrix}n_{43x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) \\n_{43y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) \\n_{43z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) \\0 & n_{14x} \\0 & n_{14y} \\0 & n_{14z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) & n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right)\\ - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) & - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right)\\ n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) & n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right)\\ n_{32x} & n_{25x}\\ n_{32y} & n_{25y}\\ n_{32z} & n_{25z}\end{matrix}\right]
    \left[\begin{matrix}n_{43x} & n_{14y} \left(a_z - r_{14z}\right) - n_{14z} \left(a_y - r_{14y}\right) & n_{32y} \left(a_z - r_{32z}\right) - n_{32z} \left(a_y - r_{32y}\right) \\n_{43y} & - n_{14x} \left(a_z - r_{14z}\right) + n_{14z} \left(a_x - r_{14x}\right) & - n_{32x} \left(a_z - r_{32z}\right) + n_{32z} \left(a_x - r_{32x}\right) \\n_{43z} & n_{14x} \left(a_y - r_{14y}\right) - n_{14y} \left(a_x - r_{14x}\right) & n_{32x} \left(a_y - r_{32y}\right) - n_{32y} \left(a_x - r_{32x}\right) \\0 & n_{14x} & n_{32x} \\0 & n_{14y} & n_{32y} \\0 & n_{14z} & n_{32z} \end{matrix}\right.\\\qquad\left.\begin{matrix} n_{25y} \left(a_z - r_{25z}\right) - n_{25z} \left(a_y - r_{25y}\right)\\ - n_{25x} \left(a_z - r_{25z}\right) + n_{25z} \left(a_x - r_{25x}\right)\\ n_{25x} \left(a_y - r_{25y}\right) - n_{25y} \left(a_x - r_{25x}\right)\\ n_{25x}\\ n_{25y}\\ n_{25z}\end{matrix}\right]
    \begin{Bmatrix}\dot{d}_{43}\\\dot{\theta}_{14}\\\dot{\theta}_{32}\\\dot{\theta}_{25}\end{Bmatrix}
  \end{split}
\]

The elements of $\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} & n_{ijy} & n_{ijz} \end{Bmatrix}^T$ should always satisfy the equation $n_{ijx}^2+n_{ijy}^2+n_{ijz}^2=1$. For this to be satisfied, the elements are considered as below: \[\hat{n}_{ij}=\begin{Bmatrix} n_{ijx} \\ n_{ijy} \\ n_{ijz} \end{Bmatrix}=\begin{Bmatrix} \sin{\left(\beta_{ij}\right)} \cos{\left(\phi_{ij}\right)} \\ \sin{\left(\beta_{ij}\right)} \sin{\left(\phi_{ij}\right)} \\ \cos{\left(\beta_{ij}\right)} \end{Bmatrix}\]
For the chosen end-effector location $\vec{a}=\begin{Bmatrix} 3 & 4 & 5 \end{Bmatrix}^T$, the matrix $\left[J_1\right]$ would finally be
%\resizebox{\textwidth}{!}{$J_1=\left[\begin{matrix}\sin{\left(\beta_{43} \right)} \cos{\left(\phi_{43} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\\sin{\left(\phi_{43} \right)} \sin{\left(\beta_{43} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\\cos{\left(\beta_{43} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\0 & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\0 & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\0 & \cos{\left(\beta_{14} \right)} & \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{25} \right)}\end{matrix}\right]$}

\[
  %\resizebox{\textwidth}{!}{$
  \begin{split}
    \left[J_1\right]
    =
    %\left[\begin{matrix}\sin{\left(\beta_{43} \right)} \cos{\left(\phi_{43} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\\sin{\left(\phi_{43} \right)} \sin{\left(\beta_{43} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\\cos{\left(\beta_{43} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\0 & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} & \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\0 & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} & \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\0 & \cos{\left(\beta_{14} \right)} & \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{25} \right)}\end{matrix}\right]
    \left[\begin{matrix}\sin{\left(\beta_{43} \right)} \cos{\left(\phi_{43} \right)} & - \left(4 - r_{14y}\right) \cos{\left(\beta_{14} \right)} + \left(5 - r_{14z}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} \\\sin{\left(\phi_{43} \right)} \sin{\left(\beta_{43} \right)} & \left(3 - r_{14x}\right) \cos{\left(\beta_{14} \right)} - \left(5 - r_{14z}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\\cos{\left(\beta_{43} \right)} & - \left(3 - r_{14x}\right) \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} + \left(4 - r_{14y}\right) \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\0 & \sin{\left(\beta_{14} \right)} \cos{\left(\phi_{14} \right)} \\0 & \sin{\left(\phi_{14} \right)} \sin{\left(\beta_{14} \right)} \\0 & \cos{\left(\beta_{14} \right)} \end{matrix}\right.
    \\
    \qquad
    %\left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} & \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} & \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\ \cos{\left(\beta_{32} \right)} & \cos{\left(\beta_{25} \right)}\end{matrix}\right]
    \left.\begin{matrix} - \left(4 - r_{32y}\right) \cos{\left(\beta_{32} \right)} + \left(5 - r_{32z}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\ \left(3 - r_{32x}\right) \cos{\left(\beta_{32} \right)} - \left(5 - r_{32z}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ - \left(3 - r_{32x}\right) \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} + \left(4 - r_{32y}\right) \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ \sin{\left(\beta_{32} \right)} \cos{\left(\phi_{32} \right)} \\ \sin{\left(\phi_{32} \right)} \sin{\left(\beta_{32} \right)} \\ \cos{\left(\beta_{32} \right)} \end{matrix}\right.\\\qquad\left.\begin{matrix} - \left(4 - r_{25y}\right) \cos{\left(\beta_{25} \right)} + \left(5 - r_{25z}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\ \left(3 - r_{25x}\right) \cos{\left(\beta_{25} \right)} - \left(5 - r_{25z}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ - \left(3 - r_{25x}\right) \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)} + \left(4 - r_{25y}\right) \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ \sin{\left(\beta_{25} \right)} \cos{\left(\phi_{25} \right)}\\ \sin{\left(\phi_{25} \right)} \sin{\left(\beta_{25} \right)}\\ \cos{\left(\beta_{25} \right)}\end{matrix}\right]
  \end{split}
  %$}
\]

Hence, the relation between the active joint velocities and the end-effector velocities can be written as
\[
  %\Rightarrow
  \{\dot{X}\}=\left[J_1\right] \{\dot{\theta}_a\}=\left[\widetilde{J}\right] \{\dot{\theta}_a\} \]where $\left[\widetilde{J}\right]=\left[J_1\right]$.
\newline


$\therefore$The formulation of the optimisation problem would then be
\newline
Maximise\[f_1=\sqrt{\det{\left(\left[\widetilde{J}\right]^T \left[\widetilde{J}\right]\right)}}\]

Subject to the bounds
$$\begin{matrix}
  0 \leq r_{ijk} \leq 10 \\
  0 \leq \beta_{ij} \leq \pi \\
  0 \leq \phi_{ij} \leq 2\pi
  \end{matrix}
$$


\emph{Condition number formulation:}

Scaled Jacobian matrix is formulated based on the methodology explained in section \ref{methodology_of_scaled_matrix}, as shown below.

The effective distances are formulated as follows.

$$\begin{matrix}
  \bar{d}_{1}=\left|\left(\vec{r}_{14}-\vec{a}\right)\times \hat{n}_{14}\right| \\
  \bar{d}_{2}=\left|\left(\vec{r}_{32}-\vec{a}\right)\times \hat{n}_{32}\right| \\
  \bar{d}_{3}=\left|\left(\vec{r}_{25}-\vec{a}\right)\times \hat{n}_{25}\right|
\end{matrix}
$$

The characteristic length is formulated as follows.
\[
  L=\frac{\bar{d}_{1}+\bar{d}_{2}+\bar{d}_{3}}{3}
  \]

  By using the above characteristic length, the scaling matrix $\left[S\right]$ can be calculated as follows.
  \[\left[S\right]=\begin{bmatrix}
    \frac{1}{L} & 0 & 0 & 0 & 0 & 0\\
    0 & \frac{1}{L} & 0 & 0 & 0 & 0\\
    0 & 0 & \frac{1}{L} & 0 & 0 & 0\\
    0 & 0 & 0 & 1 & 0 & 0\\
    0 & 0 & 0 & 0 & 1 & 0\\
    0 & 0 & 0 & 0 & 0 & 1\\
    \end{bmatrix}\]
    
    The scaled Jacobian matrix can then be calculated as
    \[\left[\widetilde{J}_s\right]=\left[S\right]\left[\widetilde{J}\right]\]\newline
    The condition number of $\left[\widetilde{J}_s\right]$ is used for comparison.
  
  \emph{Result of the optimisation problem:}

Solution to the optimisation problem is shown in Table \ref{Tab:table_6_1} (with the values rounded up to two decimal places).
\begin{table}[h]  \centering \begin{tabular}{|c|c|}
\hline
Variable & Value \\ 
\hline
$\phi_{14}$ & $\ang{59.28}$ \\
\hline$\phi_{32}$ & $\ang{219.46}$ \\
\hline$\phi_{25}$ & $\ang{206.56}$ \\
\hline$\phi_{43}$ & $\ang{39.95}$ \\
\hline$r_{14x}$ & $10.0$ \\
\hline$r_{14y}$ & $0.0$ \\
\hline$r_{14z}$ & $10.0$ \\
\hline$r_{23x}$ & $10.0$ \\
\hline$r_{23y}$ & $10.0$ \\
\hline$r_{23z}$ & $0.0$ \\
\hline$r_{25x}$ & $0.0$ \\
\hline$r_{25y}$ & $10.0$ \\
\hline$r_{25z}$ & $10.0$ \\
\hline$\beta_{14}$ & $\ang{72.57}$ \\
\hline$\beta_{32}$ & $\ang{142.41}$ \\
\hline$\beta_{25}$ & $\ang{108.6}$ \\
\hline$\beta_{43}$ & $\ang{63.44}$ \\
\hline\end{tabular} \caption{Result (4D-M2)} \label{Tab:table_6_1} \end{table}
\newline
Therefore, the locations and orientations of the joints are shown below.
\newline
$$\begin{matrix}
  \hat{n}_{14}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k} \\
  \hat{n}_{32}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k} \\
  \hat{n}_{25}=-0.42\hat{i}-0.85\hat{j}-0.32\hat{k} \\
  \hat{n}_{43}=0.57\hat{i}+0.69\hat{j}+0.45\hat{k} \\
  \vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k} \\
  \vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k} \\
  \vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}
\end{matrix}
$$

The corresponding optimum manipulability is given by \[\mu=210.96\]
And the corresponding condition number is \[\kappa=15.31\]

And the corresponding scaled manipulability index, which is the product of singular values of the scaled Jacobian $\left[\widetilde{J}_s\right]$, is \[\bar{\mu}=0.2619\]

==> contentfolder/mechanisms2/result/dof1/result1.tex <==
{\tiny 1D-M1:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.02\hat{i}-0.52\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=0.75\hat{i}-0.51\hat{j}+0.42\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.53\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result10.tex <==
{\tiny 1D-M10:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.84\hat{i}-0.49\hat{j}-0.25\hat{k}$,\;\;\;$\vec{r}_{13}=3.76\hat{i}+5.51\hat{j}+5.34\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+1.6\hat{k}$,\;\;\;$\vec{r}_{23}=4.11\hat{i}+6.4\hat{j}+4.81\hat{k}$,\;\;\;$\vec{r}_{24}=4.67\hat{i}+3.62\hat{j}+5.9\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result11.tex <==
{\tiny 1D-M11:}

$\hat{n}_{14}=0.16\hat{i}-0.66\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{23}=0.89\hat{i}-0.47\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{24}=-0.96\hat{i}-0.28\hat{j}-0.02\hat{k}$,\;\;\;$\vec{r}_{13}=2.15\hat{i}+6.75\hat{j}+2.1\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=1.36\hat{i}+8.7\hat{j}+7.55\hat{k}$,\;\;\;$\vec{r}_{24}=4.88\hat{i}+4.39\hat{j}+4.5\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result12.tex <==
{\tiny 1D-M12:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.76\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{24}=0.21\hat{i}-0.79\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+2.63\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result13.tex <==
{\tiny 1D-M13:}

$\hat{n}_{12}=-0.82\hat{i}-0.54\hat{j}+0.19\hat{k}$,\;\;\;$\hat{n}_{13}=0.82\hat{i}+0.0\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.03\hat{i}-0.82\hat{j}-0.57\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result14.tex <==
{\tiny 1D-M14:}

$\hat{n}_{12}=0.59\hat{i}-0.79\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}+0.02\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.57\hat{j}-0.59\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result15.tex <==
{\tiny 1D-M15:}

$\hat{n}_{12}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{13}=0.88\hat{i}-0.37\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.69\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result16.tex <==
{\tiny 1D-M16:}

$\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.45\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result17.tex <==
{\tiny 1D-M17:}

$\hat{n}_{12}=0.47\hat{i}-0.44\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{24}=0.11\hat{i}+0.39\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{34}=0.69\hat{i}-0.19\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result18.tex <==
{\tiny 1D-M18:}

$\hat{n}_{12}=0.08\hat{i}-0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.45\hat{i}-0.53\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{34}=0.39\hat{i}-0.82\hat{j}-0.42\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result19.tex <==
{\tiny 1D-M19:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.77\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result2.tex <==
{\tiny 1D-M2:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.77\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{24}=0.29\hat{i}+0.95\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result20.tex <==
{\tiny 1D-M20:}

$\hat{n}_{14}=-0.62\hat{i}+0.73\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{24}=0.59\hat{i}-0.56\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=4.05\hat{i}+6.66\hat{j}+3.38\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.38\hat{i}+5.09\hat{j}+3.57\hat{k}$,\;\;\;$\vec{r}_{24}=6.45\hat{i}+6.22\hat{j}+5.3\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result21.tex <==
{\tiny 1D-M21:}

$\hat{n}_{12}=0.78\hat{i}-0.25\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result22.tex <==
{\tiny 1D-M22:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result23.tex <==
{\tiny 1D-M23:}

$\hat{n}_{13}=0.77\hat{i}+0.0\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.92\hat{j}-0.38\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result24.tex <==
{\tiny 1D-M24:}

$\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result25.tex <==
{\tiny 1D-M25:}

$\hat{n}_{13}=0.16\hat{i}+0.61\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{14}=-0.8\hat{i}+0.54\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result26.tex <==
{\tiny 1D-M26:}

$\hat{n}_{13}=-0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.56\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{24}=0.81\hat{i}+0.46\hat{j}-0.36\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result27.tex <==
{\tiny 1D-M27:}

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}-0.6\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+2.83\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result28.tex <==
{\tiny 1D-M28:}

$\hat{n}_{13}=-0.08\hat{i}-0.95\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.44\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+7.16\hat{k}$,\;\;\;$\vec{r}_{23}=4.62\hat{i}+3.55\hat{j}+4.57\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+4.87\hat{j}+4.55\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result29.tex <==
{\tiny 1D-M29:}

$\hat{n}_{13}=0.94\hat{i}-0.34\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{14}=0.36\hat{i}+0.32\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.14\hat{i}-0.99\hat{j}-0.03\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.04\hat{i}+4.16\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{24}=3.09\hat{i}+4.06\hat{j}+2.83\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result3.tex <==
{\tiny 1D-M3:}

$\hat{n}_{13}=-0.03\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.68\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}-0.37\hat{j}+0.44\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result30.tex <==
{\tiny 1D-M30:}

$\hat{n}_{13}=0.0\hat{i}+0.53\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{14}=0.04\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.2\hat{j}+0.79\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result31.tex <==
{\tiny 1D-M31:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.61\hat{i}+0.72\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.74\hat{i}+0.66\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result32.tex <==
{\tiny 1D-M32:}

$\hat{n}_{13}=0.49\hat{i}-0.6\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}+0.25\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{24}=-0.85\hat{i}-0.47\hat{j}-0.22\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result33.tex <==
{\tiny 1D-M33:}

$\hat{n}_{13}=-0.66\hat{i}-0.58\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}+0.44\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{24}=-0.63\hat{i}+0.22\hat{j}+0.75\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result34.tex <==
{\tiny 1D-M34:}

$\hat{n}_{13}=-0.74\hat{i}-0.6\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.35\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.27\hat{i}-0.91\hat{j}-0.32\hat{k}$,\;\;\;$\vec{r}_{13}=1.42\hat{i}+3.47\hat{j}+4.31\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=4.36\hat{i}+8.23\hat{j}+4.01\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result35.tex <==
{\tiny 1D-M35:}

$\hat{n}_{13}=-0.42\hat{i}-0.91\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{14}=0.43\hat{i}+0.25\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{24}=-0.22\hat{i}-0.98\hat{j}-0.01\hat{k}$,\;\;\;$\vec{r}_{13}=4.89\hat{i}+4.28\hat{j}+3.84\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.55\hat{i}+6.12\hat{j}+6.81\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result36.tex <==
{\tiny 1D-M36:}

$\hat{n}_{13}=-0.44\hat{i}-0.72\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{14}=0.83\hat{i}+0.56\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}+0.17\hat{j}+0.83\hat{k}$,\;\;\;$\vec{r}_{13}=4.07\hat{i}+7.49\hat{j}+8.26\hat{k}$,\;\;\;$\vec{r}_{23}=7.9\hat{i}+3.19\hat{j}+5.34\hat{k}$,\;\;\;$\vec{r}_{24}=0.9\hat{i}+1.12\hat{j}+1.36\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result37.tex <==
{\tiny 1D-M37:}

$\hat{n}_{13}=0.01\hat{i}-0.41\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{14}=0.75\hat{i}+0.56\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=0.01\hat{i}+0.03\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{13}=8.51\hat{i}+5.61\hat{j}+9.3\hat{k}$,\;\;\;$\vec{r}_{23}=6.97\hat{i}+5.83\hat{j}+8.15\hat{k}$,\;\;\;$\vec{r}_{24}=8.79\hat{i}+9.89\hat{j}+0.01\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result38.tex <==
{\tiny 1D-M38:}

$\hat{n}_{13}=0.61\hat{i}-0.54\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.37\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=0.2\hat{i}-0.61\hat{j}+0.77\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result39.tex <==
{\tiny 1D-M39:}

$\hat{n}_{13}=-0.95\hat{i}-0.16\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.7\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.9\hat{j}-0.45\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result4.tex <==
{\tiny 1D-M4:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.8\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}+0.6\hat{j}+0.6\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result40.tex <==
{\tiny 1D-M40:}

$\hat{n}_{14}=0.16\hat{i}+0.79\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{23}=-0.6\hat{i}-0.8\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.67\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{13}=1.1\hat{i}+4.9\hat{j}+2.13\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=2.1\hat{i}+1.07\hat{j}+6.29\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result41.tex <==
{\tiny 1D-M41:}

$\hat{n}_{14}=-0.38\hat{i}+0.38\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{23}=-0.1\hat{i}-0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.15\hat{i}-0.92\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{13}=2.65\hat{i}+4.93\hat{j}+7.29\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.5\hat{i}+6.06\hat{j}+4.36\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result42.tex <==
{\tiny 1D-M42:}

$\hat{n}_{14}=0.03\hat{i}+0.04\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.33\hat{i}+0.27\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{24}=0.54\hat{i}+0.31\hat{j}-0.78\hat{k}$,\;\;\;$\vec{r}_{13}=6.21\hat{i}+5.74\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{23}=9.31\hat{i}+7.29\hat{j}+7.38\hat{k}$,\;\;\;$\vec{r}_{24}=0.63\hat{i}+8.6\hat{j}+9.34\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result43.tex <==
{\tiny 1D-M43:}

$\hat{n}_{14}=-0.04\hat{i}-0.47\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{23}=0.88\hat{i}+0.43\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.36\hat{j}-0.9\hat{k}$,\;\;\;$\vec{r}_{13}=1.34\hat{i}+0.31\hat{j}+9.39\hat{k}$,\;\;\;$\vec{r}_{23}=3.01\hat{i}+2.96\hat{j}+3.33\hat{k}$,\;\;\;$\vec{r}_{24}=4.67\hat{i}+6.48\hat{j}+0.25\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result44.tex <==
{\tiny 1D-M44:}

$\hat{n}_{14}=-0.44\hat{i}-0.37\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.69\hat{i}-0.73\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result45.tex <==
{\tiny 1D-M45:}

$\hat{n}_{14}=-0.8\hat{i}-0.26\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.17\hat{i}+0.78\hat{j}-0.61\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result46.tex <==
{\tiny 1D-M46:}

$\hat{n}_{12}=-0.15\hat{i}+0.71\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{13}=-0.42\hat{i}-0.63\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.75\hat{i}+0.29\hat{j}+0.59\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result47.tex <==
{\tiny 1D-M47:}

$\hat{n}_{12}=-0.47\hat{i}+0.81\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.67\hat{i}+0.08\hat{j}-0.74\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result48.tex <==
{\tiny 1D-M48:}

$\hat{n}_{12}=-0.78\hat{i}+0.61\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}-0.61\hat{j}+0.34\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+1.46\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result49.tex <==
{\tiny 1D-M49:}

$\hat{n}_{12}=-0.0\hat{i}+0.94\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.69\hat{j}-0.0\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result5.tex <==
{\tiny 1D-M5:}

$\hat{n}_{13}=-0.08\hat{i}+0.46\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{23}=0.61\hat{i}-0.33\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.79\hat{i}-0.58\hat{j}-0.19\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result50.tex <==
{\tiny 1D-M50:}

$\hat{n}_{12}=0.82\hat{i}-0.44\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.6\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result51.tex <==
{\tiny 1D-M51:}

$\hat{n}_{12}=-0.0\hat{i}+0.62\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.53\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{34}=0.77\hat{i}+0.44\hat{j}+0.47\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result52.tex <==
{\tiny 1D-M52:}

$\hat{n}_{12}=0.69\hat{i}+0.51\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{13}=-0.91\hat{i}-0.28\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result53.tex <==
{\tiny 1D-M53:}

$\hat{n}_{12}=0.61\hat{i}-0.05\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{13}=-0.65\hat{i}-0.37\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{34}=-0.61\hat{i}+0.5\hat{j}+0.61\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result54.tex <==
{\tiny 1D-M54:}

$\hat{n}_{12}=-0.86\hat{i}+0.41\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}-0.48\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}+0.26\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result55.tex <==
{\tiny 1D-M55:}

$\hat{n}_{12}=-0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.96\hat{i}+0.16\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result56.tex <==
{\tiny 1D-M56:}

$\hat{n}_{12}=-0.74\hat{i}+0.08\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=0.77\hat{i}-0.64\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result57.tex <==
{\tiny 1D-M57:}

$\hat{n}_{12}=0.0\hat{i}+0.79\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{24}=0.6\hat{i}+0.48\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result58.tex <==
{\tiny 1D-M58:}

$\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result59.tex <==
{\tiny 1D-M59:}

$\hat{n}_{13}=0.57\hat{i}-0.61\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.66\hat{j}-0.41\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=1.65\hat{i}+1.14\hat{j}+3.04\hat{k}$,\;\;\;$\vec{r}_{24}=3.29\hat{i}+6.44\hat{j}+8.8\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result6.tex <==
{\tiny 1D-M6:}

$\hat{n}_{13}=0.0\hat{i}+0.37\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{23}=0.33\hat{i}-0.66\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{24}=0.84\hat{i}-0.53\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result60.tex <==
{\tiny 1D-M60:}

$\hat{n}_{14}=0.62\hat{i}-0.06\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}-0.53\hat{j}+0.46\hat{k}$,\;\;\;$\vec{r}_{13}=7.06\hat{i}+6.93\hat{j}+6.95\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=2.75\hat{i}+2.12\hat{j}+7.47\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result61.tex <==
{\tiny 1D-M61:}

$\hat{n}_{14}=-0.32\hat{i}-0.19\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}+0.79\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{13}=5.17\hat{i}+7.03\hat{j}+1.54\hat{k}$,\;\;\;$\vec{r}_{23}=9.53\hat{i}+5.41\hat{j}+6.8\hat{k}$,\;\;\;$\vec{r}_{24}=0.37\hat{i}+8.09\hat{j}+7.49\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result62.tex <==
{\tiny 1D-M62:}

$\hat{n}_{12}=0.28\hat{i}+0.64\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.52\hat{j}+0.85\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result63.tex <==
{\tiny 1D-M63:}

$\hat{n}_{12}=-0.46\hat{i}-0.43\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.07\hat{i}-0.66\hat{j}-0.75\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result64.tex <==
{\tiny 1D-M64:}

$\hat{n}_{13}=-0.23\hat{i}+0.23\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.59\hat{i}-0.59\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=0.43\hat{i}-0.43\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.01\hat{i}+5.01\hat{j}+5.01\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result65.tex <==
{\tiny 1D-M65:}

$\hat{n}_{13}=0.31\hat{i}-0.63\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.02\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.89\hat{i}-0.46\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{24}=0.33\hat{i}-0.63\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=5.12\hat{i}+4.88\hat{j}+5.02\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.82\hat{i}+4.82\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{24}=4.86\hat{i}+5.18\hat{j}+4.92\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result66.tex <==
{\tiny 1D-M66:}

$\hat{n}_{13}=0.61\hat{i}-0.61\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.59\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.31\hat{i}-0.31\hat{j}-0.9\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.06\hat{i}+5.03\hat{j}+5.17\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result67.tex <==
{\tiny 1D-M67:}

$\hat{n}_{13}=-0.58\hat{i}+0.8\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.86\hat{i}-0.52\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{24}=-0.44\hat{i}-0.89\hat{j}-0.05\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+3.07\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result68.tex <==
{\tiny 1D-M68:}

$\hat{n}_{12}=0.34\hat{i}-0.89\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{13}=0.56\hat{i}+0.34\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.82\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.85\hat{i}+0.27\hat{j}-0.44\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result69.tex <==
{\tiny 1D-M69:}

$\hat{n}_{12}=-0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}-0.44\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.61\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{34}=-0.82\hat{i}-0.32\hat{j}+0.48\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result7.tex <==
{\tiny 1D-M7:}

$\hat{n}_{13}=-0.21\hat{i}-0.95\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{14}=0.41\hat{i}-0.48\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}-0.96\hat{j}+0.24\hat{k}$,\;\;\;$\vec{r}_{13}=5.38\hat{i}+6.86\hat{j}+4.63\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.61\hat{i}+5.26\hat{j}+5.64\hat{k}$,\;\;\;$\vec{r}_{24}=5.08\hat{i}+5.88\hat{j}+3.64\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result70.tex <==
{\tiny 1D-M70:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.05\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result71.tex <==
{\tiny 1D-M71:}

$\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.12\hat{i}+0.76\hat{j}+0.64\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result72.tex <==
{\tiny 1D-M72:}

$\hat{n}_{13}=-0.21\hat{i}-0.79\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.21\hat{i}+0.79\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result73.tex <==
{\tiny 1D-M73:}

$\hat{n}_{13}=-0.3\hat{i}+0.81\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.3\hat{i}+0.81\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result74.tex <==
{\tiny 1D-M74:}

$\hat{n}_{13}=-0.62\hat{i}-0.77\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result75.tex <==
{\tiny 1D-M75:}

$\hat{n}_{13}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result76.tex <==
{\tiny 1D-M76:}

$\hat{n}_{13}=-0.42\hat{i}-0.11\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{14}=-0.55\hat{i}-0.55\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=-0.4\hat{i}-0.63\hat{j}-0.66\hat{k}$,\;\;\;$\vec{r}_{13}=6.6\hat{i}+0.48\hat{j}+3.49\hat{k}$,\;\;\;$\vec{r}_{24}=4.51\hat{i}+2.41\hat{j}+7.15\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result77.tex <==
{\tiny 1D-M77:}

$\hat{n}_{13}=0.68\hat{i}+0.58\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{14}=-0.84\hat{i}+0.51\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.09\hat{i}+0.07\hat{j}-0.99\hat{k}$,\;\;\;$\vec{r}_{13}=5.88\hat{i}+3.66\hat{j}+8.07\hat{k}$,\;\;\;$\vec{r}_{23}=5.04\hat{i}+4.9\hat{j}+8.77\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result78.tex <==
{\tiny 1D-M78:}

$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result79.tex <==
{\tiny 1D-M79:}

$\hat{n}_{14}=-0.3\hat{i}-0.22\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{23}=0.35\hat{i}+0.04\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=0.17\hat{i}-0.24\hat{j}+0.96\hat{k}$,\;\;\;$\vec{r}_{13}=1.22\hat{i}+2.68\hat{j}+2.58\hat{k}$,\;\;\;$\vec{r}_{24}=3.32\hat{i}+1.52\hat{j}+3.48\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result8.tex <==
{\tiny 1D-M8:}

$\hat{n}_{13}=-0.72\hat{i}-0.39\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=0.31\hat{i}-0.9\hat{j}+0.29\hat{k}$,\;\;\;$\hat{n}_{24}=-0.04\hat{i}-1.0\hat{j}+0.06\hat{k}$,\;\;\;$\vec{r}_{13}=6.43\hat{i}+4.57\hat{j}+5.96\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=3.69\hat{i}+6.29\hat{j}+5.5\hat{k}$,\;\;\;$\vec{r}_{24}=5.32\hat{i}+3.65\hat{j}+6.36\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result80.tex <==
{\tiny 1D-M80:}

$\hat{n}_{14}=-0.07\hat{i}+0.16\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{23}=0.48\hat{i}-0.66\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.04\hat{i}+0.14\hat{j}+0.99\hat{k}$,\;\;\;$\vec{r}_{13}=3.42\hat{i}+7.36\hat{j}+7.95\hat{k}$,\;\;\;$\vec{r}_{23}=5.45\hat{i}+6.86\hat{j}+8.94\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result81.tex <==
{\tiny 1D-M81:}

$\hat{n}_{14}=-0.66\hat{i}+0.09\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{23}=-0.66\hat{i}+0.09\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result82.tex <==
{\tiny 1D-M82:}

$\hat{n}_{12}=-0.67\hat{i}+0.45\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}-0.61\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result83.tex <==
{\tiny 1D-M83:}

$\hat{n}_{12}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+9.32\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.29\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result84.tex <==
{\tiny 1D-M84:}

$\hat{n}_{12}=-0.57\hat{i}-0.49\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.6\hat{j}+0.56\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result85.tex <==
{\tiny 1D-M85:}

$\hat{n}_{12}=-0.77\hat{i}-0.61\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.01\hat{i}-0.7\hat{j}+0.71\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result86.tex <==
{\tiny 1D-M86:}

$\hat{n}_{12}=0.58\hat{i}-0.81\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.75\hat{i}-0.66\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+1.51\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+6.87\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result87.tex <==
{\tiny 1D-M87:}

$\hat{n}_{12}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.55\hat{j}+0.6\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result88.tex <==
{\tiny 1D-M88:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result89.tex <==
{\tiny 1D-M89:}

$\hat{n}_{14}=0.0\hat{i}-0.36\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.26\hat{j}-0.64\hat{k}$,\;\;\;$\vec{r}_{13}=8.34\hat{i}+6.1\hat{j}+5.75\hat{k}$,\;\;\;$\vec{r}_{23}=3.26\hat{i}+4.56\hat{j}+7.14\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result9.tex <==
{\tiny 1D-M9:}

$\hat{n}_{13}=0.44\hat{i}+0.64\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=0.15\hat{i}+0.42\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{24}=0.5\hat{i}+0.61\hat{j}-0.62\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result90.tex <==
{\tiny 1D-M90:}

$\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.92\hat{j}+0.38\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result91.tex <==
{\tiny 1D-M91:}

$\hat{n}_{13}=-0.24\hat{i}-0.85\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{14}=-0.24\hat{i}-0.85\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{23}=-0.35\hat{i}-0.37\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.91\hat{i}-0.37\hat{j}-0.21\hat{k}$,\;\;\;$\vec{r}_{14}=4.82\hat{i}+5.35\hat{j}+4.24\hat{k}$,\;\;\;$\vec{r}_{23}=5.77\hat{i}+5.14\hat{j}+4.2\hat{k}$,\;\;\;$\vec{r}_{24}=5.35\hat{i}+5.81\hat{j}+5.53\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result92.tex <==
{\tiny 1D-M92:}

$\hat{n}_{13}=-0.05\hat{i}-0.21\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{14}=0.19\hat{i}+0.29\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{23}=0.16\hat{i}+0.12\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.67\hat{j}+0.2\hat{k}$,\;\;\;$\vec{r}_{13}=8.59\hat{i}+9.74\hat{j}+5.71\hat{k}$,\;\;\;$\vec{r}_{23}=9.97\hat{i}+5.54\hat{j}+5.15\hat{k}$,\;\;\;$\vec{r}_{24}=3.31\hat{i}+4.3\hat{j}+4.92\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result93.tex <==
{\tiny 1D-M93:}

$\hat{n}_{13}=-0.63\hat{i}+0.17\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=0.76\hat{i}-0.05\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{23}=0.76\hat{i}-0.05\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{24}=-0.14\hat{i}-0.98\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{13}=5.68\hat{i}+5.82\hat{j}+5.13\hat{k}$,\;\;\;$\vec{r}_{14}=4.08\hat{i}+5.92\hat{j}+4.4\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+5.32\hat{j}+5.78\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result94.tex <==
{\tiny 1D-M94:}

$\hat{n}_{13}=0.4\hat{i}-0.48\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{14}=0.26\hat{i}-0.75\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{23}=-0.88\hat{i}-0.45\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.75\hat{j}-0.61\hat{k}$,\;\;\;$\vec{r}_{13}=4.92\hat{i}+4.88\hat{j}+5.04\hat{k}$,\;\;\;$\vec{r}_{14}=4.81\hat{i}+4.88\hat{j}+4.88\hat{k}$,\;\;\;$\vec{r}_{23}=4.93\hat{i}+4.88\hat{j}+5.07\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result95.tex <==
{\tiny 1D-M95:}

$\hat{n}_{12}=-0.89\hat{i}-0.29\hat{j}-0.36\hat{k}$,\;\;\;$\hat{n}_{13}=0.66\hat{i}+0.57\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{24}=-0.16\hat{i}-0.53\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.63\hat{j}+0.26\hat{k}$,\;\;\;$\vec{r}_{13}=4.73\hat{i}+4.26\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+5.47\hat{j}+4.87\hat{k}$,\;\;\;$\vec{r}_{34}=4.74\hat{i}+5.76\hat{j}+4.86\hat{k}$.



==> contentfolder/mechanisms2/result/dof1/result96.tex <==
{\tiny 1D-M96:}

$\hat{n}_{12}=-0.52\hat{i}-0.13\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{13}=0.7\hat{i}-0.64\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.18\hat{i}-0.95\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{34}=-0.49\hat{i}-0.76\hat{j}-0.42\hat{k}$,\;\;\;$\vec{r}_{12}=3.53\hat{i}+7.37\hat{j}+5.85\hat{k}$,\;\;\;$\vec{r}_{13}=7.27\hat{i}+7.33\hat{j}+2.16\hat{k}$,\;\;\;$\vec{r}_{34}=3.23\hat{i}+6.27\hat{j}+4.91\hat{k}$.



==> contentfolder/mechanisms2/result/dof2/result1.tex <==
Manipulator 1:

$\vec{r}_{12}=0.0\hat{i}+8.21\hat{j}+10.0\hat{k}$\newline
$\vec{r}_{23}=0.02\hat{i}+7.16\hat{j}+6.31\hat{k}$\newline
$\hat{n}_{23}=-0.29\hat{i}-0.45\hat{j}-0.85\hat{k}$\newline
$\hat{n}_{12}=-0.31\hat{i}+0.15\hat{j}+0.94\hat{k}$



==> contentfolder/mechanisms2/result/dof2/result1_full.tex <==


{\tiny 1D-M1:}   $\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.02\hat{i}-0.52\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=0.75\hat{i}-0.51\hat{j}+0.42\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.53\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M2:}   $\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.77\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{24}=0.29\hat{i}+0.95\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M3:}   $\hat{n}_{13}=-0.03\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.68\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}-0.37\hat{j}+0.44\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M4:}   $\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.8\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}+0.6\hat{j}+0.6\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M5:}   $\hat{n}_{13}=-0.08\hat{i}+0.46\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{23}=0.61\hat{i}-0.33\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.79\hat{i}-0.58\hat{j}-0.19\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M6:}   $\hat{n}_{13}=0.0\hat{i}+0.37\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{23}=0.33\hat{i}-0.66\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{24}=0.84\hat{i}-0.53\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M7:}   $\hat{n}_{13}=-0.21\hat{i}-0.95\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{14}=0.41\hat{i}-0.48\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}-0.96\hat{j}+0.24\hat{k}$,\;\;\;$\vec{r}_{13}=5.38\hat{i}+6.86\hat{j}+4.63\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.61\hat{i}+5.26\hat{j}+5.64\hat{k}$,\;\;\;$\vec{r}_{24}=5.08\hat{i}+5.88\hat{j}+3.64\hat{k}$.

{\tiny 1D-M8:}   $\hat{n}_{13}=-0.72\hat{i}-0.39\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=0.31\hat{i}-0.9\hat{j}+0.29\hat{k}$,\;\;\;$\hat{n}_{24}=-0.04\hat{i}-1.0\hat{j}+0.06\hat{k}$,\;\;\;$\vec{r}_{13}=6.43\hat{i}+4.57\hat{j}+5.96\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=3.69\hat{i}+6.29\hat{j}+5.5\hat{k}$,\;\;\;$\vec{r}_{24}=5.32\hat{i}+3.65\hat{j}+6.36\hat{k}$.

{\tiny 1D-M9:}   $\hat{n}_{13}=0.44\hat{i}+0.64\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=0.15\hat{i}+0.42\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{24}=0.5\hat{i}+0.61\hat{j}-0.62\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M10:}\label{result_1_10}   $\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.84\hat{i}-0.49\hat{j}-0.25\hat{k}$,\;\;\;$\vec{r}_{13}=3.76\hat{i}+5.51\hat{j}+5.34\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+1.6\hat{k}$,\;\;\;$\vec{r}_{23}=4.11\hat{i}+6.4\hat{j}+4.81\hat{k}$,\;\;\;$\vec{r}_{24}=4.67\hat{i}+3.62\hat{j}+5.9\hat{k}$.

{\tiny 1D-M11:}   $\hat{n}_{14}=0.16\hat{i}-0.66\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{23}=0.89\hat{i}-0.47\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{24}=-0.96\hat{i}-0.28\hat{j}-0.02\hat{k}$,\;\;\;$\vec{r}_{13}=2.15\hat{i}+6.75\hat{j}+2.1\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=1.36\hat{i}+8.7\hat{j}+7.55\hat{k}$,\;\;\;$\vec{r}_{24}=4.88\hat{i}+4.39\hat{j}+4.5\hat{k}$.

{\tiny 1D-M12:}   $\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.76\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{24}=0.21\hat{i}-0.79\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+2.63\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M13:}   $\hat{n}_{12}=-0.82\hat{i}-0.54\hat{j}+0.19\hat{k}$,\;\;\;$\hat{n}_{13}=0.82\hat{i}+0.0\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.03\hat{i}-0.82\hat{j}-0.57\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M14:}   $\hat{n}_{12}=0.59\hat{i}-0.79\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}+0.02\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.57\hat{j}-0.59\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M15:}   $\hat{n}_{12}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{13}=0.88\hat{i}-0.37\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.69\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M16:}   $\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.45\hat{k}$.

{\tiny 1D-M17:}   $\hat{n}_{12}=0.47\hat{i}-0.44\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{24}=0.11\hat{i}+0.39\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{34}=0.69\hat{i}-0.19\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M18:}   $\hat{n}_{12}=0.08\hat{i}-0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.45\hat{i}-0.53\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{34}=0.39\hat{i}-0.82\hat{j}-0.42\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M19:}   $\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.77\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M20:}   $\hat{n}_{14}=-0.62\hat{i}+0.73\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{24}=0.59\hat{i}-0.56\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=4.05\hat{i}+6.66\hat{j}+3.38\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.38\hat{i}+5.09\hat{j}+3.57\hat{k}$,\;\;\;$\vec{r}_{24}=6.45\hat{i}+6.22\hat{j}+5.3\hat{k}$.

{\tiny 1D-M21:}   $\hat{n}_{12}=0.78\hat{i}-0.25\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M22:}   $\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M23:}   $\hat{n}_{13}=0.77\hat{i}+0.0\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.92\hat{j}-0.38\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M24:}   $\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M25:}   $\hat{n}_{13}=0.16\hat{i}+0.61\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{14}=-0.8\hat{i}+0.54\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M26:}   $\hat{n}_{13}=-0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.56\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{24}=0.81\hat{i}+0.46\hat{j}-0.36\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M27:}   $\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}-0.6\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+2.83\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M28:}   $\hat{n}_{13}=-0.08\hat{i}-0.95\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.44\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+7.16\hat{k}$,\;\;\;$\vec{r}_{23}=4.62\hat{i}+3.55\hat{j}+4.57\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+4.87\hat{j}+4.55\hat{k}$.

{\tiny 1D-M29:}   $\hat{n}_{13}=0.94\hat{i}-0.34\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{14}=0.36\hat{i}+0.32\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.14\hat{i}-0.99\hat{j}-0.03\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.04\hat{i}+4.16\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{24}=3.09\hat{i}+4.06\hat{j}+2.83\hat{k}$.

{\tiny 1D-M30:}   $\hat{n}_{13}=0.0\hat{i}+0.53\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{14}=0.04\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.2\hat{j}+0.79\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M31:}   $\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.61\hat{i}+0.72\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.74\hat{i}+0.66\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M32:}   $\hat{n}_{13}=0.49\hat{i}-0.6\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}+0.25\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{24}=-0.85\hat{i}-0.47\hat{j}-0.22\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M33:}   $\hat{n}_{13}=-0.66\hat{i}-0.58\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}+0.44\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{24}=-0.63\hat{i}+0.22\hat{j}+0.75\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M34:}   $\hat{n}_{13}=-0.74\hat{i}-0.6\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.35\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.27\hat{i}-0.91\hat{j}-0.32\hat{k}$,\;\;\;$\vec{r}_{13}=1.42\hat{i}+3.47\hat{j}+4.31\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=4.36\hat{i}+8.23\hat{j}+4.01\hat{k}$.

{\tiny 1D-M35:}   $\hat{n}_{13}=-0.42\hat{i}-0.91\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{14}=0.43\hat{i}+0.25\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{24}=-0.22\hat{i}-0.98\hat{j}-0.01\hat{k}$,\;\;\;$\vec{r}_{13}=4.89\hat{i}+4.28\hat{j}+3.84\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.55\hat{i}+6.12\hat{j}+6.81\hat{k}$.

{\tiny 1D-M36:}   $\hat{n}_{13}=-0.44\hat{i}-0.72\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{14}=0.83\hat{i}+0.56\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}+0.17\hat{j}+0.83\hat{k}$,\;\;\;$\vec{r}_{13}=4.07\hat{i}+7.49\hat{j}+8.26\hat{k}$,\;\;\;$\vec{r}_{23}=7.9\hat{i}+3.19\hat{j}+5.34\hat{k}$,\;\;\;$\vec{r}_{24}=0.9\hat{i}+1.12\hat{j}+1.36\hat{k}$.

{\tiny 1D-M37:}   $\hat{n}_{13}=0.01\hat{i}-0.41\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{14}=0.75\hat{i}+0.56\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=0.01\hat{i}+0.03\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{13}=8.51\hat{i}+5.61\hat{j}+9.3\hat{k}$,\;\;\;$\vec{r}_{23}=6.97\hat{i}+5.83\hat{j}+8.15\hat{k}$,\;\;\;$\vec{r}_{24}=8.79\hat{i}+9.89\hat{j}+0.01\hat{k}$.

{\tiny 1D-M38:}   $\hat{n}_{13}=0.61\hat{i}-0.54\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.37\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=0.2\hat{i}-0.61\hat{j}+0.77\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M39:}   $\hat{n}_{13}=-0.95\hat{i}-0.16\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.7\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.9\hat{j}-0.45\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M40:}   $\hat{n}_{14}=0.16\hat{i}+0.79\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{23}=-0.6\hat{i}-0.8\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.67\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{13}=1.1\hat{i}+4.9\hat{j}+2.13\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=2.1\hat{i}+1.07\hat{j}+6.29\hat{k}$.

{\tiny 1D-M41:}   $\hat{n}_{14}=-0.38\hat{i}+0.38\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{23}=-0.1\hat{i}-0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.15\hat{i}-0.92\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{13}=2.65\hat{i}+4.93\hat{j}+7.29\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.5\hat{i}+6.06\hat{j}+4.36\hat{k}$.

{\tiny 1D-M42:}   $\hat{n}_{14}=0.03\hat{i}+0.04\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.33\hat{i}+0.27\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{24}=0.54\hat{i}+0.31\hat{j}-0.78\hat{k}$,\;\;\;$\vec{r}_{13}=6.21\hat{i}+5.74\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{23}=9.31\hat{i}+7.29\hat{j}+7.38\hat{k}$,\;\;\;$\vec{r}_{24}=0.63\hat{i}+8.6\hat{j}+9.34\hat{k}$.

{\tiny 1D-M43:}   $\hat{n}_{14}=-0.04\hat{i}-0.47\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{23}=0.88\hat{i}+0.43\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.36\hat{j}-0.9\hat{k}$,\;\;\;$\vec{r}_{13}=1.34\hat{i}+0.31\hat{j}+9.39\hat{k}$,\;\;\;$\vec{r}_{23}=3.01\hat{i}+2.96\hat{j}+3.33\hat{k}$,\;\;\;$\vec{r}_{24}=4.67\hat{i}+6.48\hat{j}+0.25\hat{k}$.

{\tiny 1D-M44:}   $\hat{n}_{14}=-0.44\hat{i}-0.37\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.69\hat{i}-0.73\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M45:}   $\hat{n}_{14}=-0.8\hat{i}-0.26\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.17\hat{i}+0.78\hat{j}-0.61\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M46:}   $\hat{n}_{12}=-0.15\hat{i}+0.71\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{13}=-0.42\hat{i}-0.63\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.75\hat{i}+0.29\hat{j}+0.59\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M47:}   $\hat{n}_{12}=-0.47\hat{i}+0.81\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.67\hat{i}+0.08\hat{j}-0.74\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M48:}   $\hat{n}_{12}=-0.78\hat{i}+0.61\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}-0.61\hat{j}+0.34\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+1.46\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M49:}   $\hat{n}_{12}=-0.0\hat{i}+0.94\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.69\hat{j}-0.0\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M50:}   $\hat{n}_{12}=0.82\hat{i}-0.44\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.6\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M51:}   $\hat{n}_{12}=-0.0\hat{i}+0.62\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.53\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{34}=0.77\hat{i}+0.44\hat{j}+0.47\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M52:}   $\hat{n}_{12}=0.69\hat{i}+0.51\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{13}=-0.91\hat{i}-0.28\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M53:}   $\hat{n}_{12}=0.61\hat{i}-0.05\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{13}=-0.65\hat{i}-0.37\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{34}=-0.61\hat{i}+0.5\hat{j}+0.61\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M54:}   $\hat{n}_{12}=-0.86\hat{i}+0.41\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}-0.48\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}+0.26\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M55:}   $\hat{n}_{12}=-0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.96\hat{i}+0.16\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M56:}   $\hat{n}_{12}=-0.74\hat{i}+0.08\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=0.77\hat{i}-0.64\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M57:}   $\hat{n}_{12}=0.0\hat{i}+0.79\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{24}=0.6\hat{i}+0.48\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M58:}   $\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M59:}   $\hat{n}_{13}=0.57\hat{i}-0.61\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.66\hat{j}-0.41\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=1.65\hat{i}+1.14\hat{j}+3.04\hat{k}$,\;\;\;$\vec{r}_{24}=3.29\hat{i}+6.44\hat{j}+8.8\hat{k}$.

{\tiny 1D-M60:}   $\hat{n}_{14}=0.62\hat{i}-0.06\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}-0.53\hat{j}+0.46\hat{k}$,\;\;\;$\vec{r}_{13}=7.06\hat{i}+6.93\hat{j}+6.95\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=2.75\hat{i}+2.12\hat{j}+7.47\hat{k}$.

{\tiny 1D-M61:}   $\hat{n}_{14}=-0.32\hat{i}-0.19\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}+0.79\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{13}=5.17\hat{i}+7.03\hat{j}+1.54\hat{k}$,\;\;\;$\vec{r}_{23}=9.53\hat{i}+5.41\hat{j}+6.8\hat{k}$,\;\;\;$\vec{r}_{24}=0.37\hat{i}+8.09\hat{j}+7.49\hat{k}$.

{\tiny 1D-M62:}   $\hat{n}_{12}=0.28\hat{i}+0.64\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.52\hat{j}+0.85\hat{k}$,\;\;\;$\vec{r}_{12}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M63:}   $\hat{n}_{12}=-0.46\hat{i}-0.43\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.07\hat{i}-0.66\hat{j}-0.75\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M64:}   $\hat{n}_{13}=-0.23\hat{i}+0.23\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.59\hat{i}-0.59\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=0.43\hat{i}-0.43\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.01\hat{i}+5.01\hat{j}+5.01\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M65:}\label{result_1_65}   $\hat{n}_{13}=0.31\hat{i}-0.63\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.02\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.89\hat{i}-0.46\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{24}=0.33\hat{i}-0.63\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=5.12\hat{i}+4.88\hat{j}+5.02\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.82\hat{i}+4.82\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{24}=4.86\hat{i}+5.18\hat{j}+4.92\hat{k}$.

{\tiny 1D-M66:}   $\hat{n}_{13}=0.61\hat{i}-0.61\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.59\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.31\hat{i}-0.31\hat{j}-0.9\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.06\hat{i}+5.03\hat{j}+5.17\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M67:}   $\hat{n}_{13}=-0.58\hat{i}+0.8\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.86\hat{i}-0.52\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{24}=-0.44\hat{i}-0.89\hat{j}-0.05\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+3.07\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M68:}   $\hat{n}_{12}=0.34\hat{i}-0.89\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{13}=0.56\hat{i}+0.34\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.82\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.85\hat{i}+0.27\hat{j}-0.44\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M69:}   $\hat{n}_{12}=-0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}-0.44\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.61\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{34}=-0.82\hat{i}-0.32\hat{j}+0.48\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M70:}   $\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.05\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M71:}   $\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.12\hat{i}+0.76\hat{j}+0.64\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M72:}   $\hat{n}_{13}=-0.21\hat{i}-0.79\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.21\hat{i}+0.79\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M73:}   $\hat{n}_{13}=-0.3\hat{i}+0.81\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.3\hat{i}+0.81\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M74:}   $\hat{n}_{13}=-0.62\hat{i}-0.77\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M75:}   $\hat{n}_{13}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M76:}   $\hat{n}_{13}=-0.42\hat{i}-0.11\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{14}=-0.55\hat{i}-0.55\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=-0.4\hat{i}-0.63\hat{j}-0.66\hat{k}$,\;\;\;$\vec{r}_{13}=6.6\hat{i}+0.48\hat{j}+3.49\hat{k}$,\;\;\;$\vec{r}_{24}=4.51\hat{i}+2.41\hat{j}+7.15\hat{k}$.

{\tiny 1D-M77:}   $\hat{n}_{13}=0.68\hat{i}+0.58\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{14}=-0.84\hat{i}+0.51\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.09\hat{i}+0.07\hat{j}-0.99\hat{k}$,\;\;\;$\vec{r}_{13}=5.88\hat{i}+3.66\hat{j}+8.07\hat{k}$,\;\;\;$\vec{r}_{23}=5.04\hat{i}+4.9\hat{j}+8.77\hat{k}$.

{\tiny 1D-M78:}   $\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M79:}   $\hat{n}_{14}=-0.3\hat{i}-0.22\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{23}=0.35\hat{i}+0.04\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=0.17\hat{i}-0.24\hat{j}+0.96\hat{k}$,\;\;\;$\vec{r}_{13}=1.22\hat{i}+2.68\hat{j}+2.58\hat{k}$,\;\;\;$\vec{r}_{24}=3.32\hat{i}+1.52\hat{j}+3.48\hat{k}$.

{\tiny 1D-M80:}   $\hat{n}_{14}=-0.07\hat{i}+0.16\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{23}=0.48\hat{i}-0.66\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.04\hat{i}+0.14\hat{j}+0.99\hat{k}$,\;\;\;$\vec{r}_{13}=3.42\hat{i}+7.36\hat{j}+7.95\hat{k}$,\;\;\;$\vec{r}_{23}=5.45\hat{i}+6.86\hat{j}+8.94\hat{k}$.

{\tiny 1D-M81:}   $\hat{n}_{14}=-0.66\hat{i}+0.09\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{23}=-0.66\hat{i}+0.09\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M82:}   $\hat{n}_{12}=-0.67\hat{i}+0.45\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{13}=0.55\hat{i}-0.61\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M83:}   $\hat{n}_{12}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+9.32\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.29\hat{k}$.

{\tiny 1D-M84:}   $\hat{n}_{12}=-0.57\hat{i}-0.49\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.6\hat{j}+0.56\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M85:}   $\hat{n}_{12}=-0.77\hat{i}-0.61\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.01\hat{i}-0.7\hat{j}+0.71\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M86:}   $\hat{n}_{12}=0.58\hat{i}-0.81\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.75\hat{i}-0.66\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+1.51\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+6.87\hat{k}$.

{\tiny 1D-M87:}   $\hat{n}_{12}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.55\hat{j}+0.6\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 1D-M88:}   $\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M89:}   $\hat{n}_{14}=0.0\hat{i}-0.36\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.26\hat{j}-0.64\hat{k}$,\;\;\;$\vec{r}_{13}=8.34\hat{i}+6.1\hat{j}+5.75\hat{k}$,\;\;\;$\vec{r}_{23}=3.26\hat{i}+4.56\hat{j}+7.14\hat{k}$.

{\tiny 1D-M90:}   $\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.92\hat{j}+0.38\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 1D-M91:}   $\hat{n}_{13}=-0.24\hat{i}-0.85\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{14}=-0.24\hat{i}-0.85\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{23}=-0.35\hat{i}-0.37\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.91\hat{i}-0.37\hat{j}-0.21\hat{k}$,\;\;\;$\vec{r}_{14}=4.82\hat{i}+5.35\hat{j}+4.24\hat{k}$,\;\;\;$\vec{r}_{23}=5.77\hat{i}+5.14\hat{j}+4.2\hat{k}$,\;\;\;$\vec{r}_{24}=5.35\hat{i}+5.81\hat{j}+5.53\hat{k}$.

{\tiny 1D-M92:}   $\hat{n}_{13}=-0.05\hat{i}-0.21\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{14}=0.19\hat{i}+0.29\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{23}=0.16\hat{i}+0.12\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.67\hat{j}+0.2\hat{k}$,\;\;\;$\vec{r}_{13}=8.59\hat{i}+9.74\hat{j}+5.71\hat{k}$,\;\;\;$\vec{r}_{23}=9.97\hat{i}+5.54\hat{j}+5.15\hat{k}$,\;\;\;$\vec{r}_{24}=3.31\hat{i}+4.3\hat{j}+4.92\hat{k}$.

{\tiny 1D-M93:}   $\hat{n}_{13}=-0.63\hat{i}+0.17\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=0.76\hat{i}-0.05\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{23}=0.76\hat{i}-0.05\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{24}=-0.14\hat{i}-0.98\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{13}=5.68\hat{i}+5.82\hat{j}+5.13\hat{k}$,\;\;\;$\vec{r}_{14}=4.08\hat{i}+5.92\hat{j}+4.4\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+5.32\hat{j}+5.78\hat{k}$.

{\tiny 1D-M94:}   $\hat{n}_{13}=0.4\hat{i}-0.48\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{14}=0.26\hat{i}-0.75\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{23}=-0.88\hat{i}-0.45\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.75\hat{j}-0.61\hat{k}$,\;\;\;$\vec{r}_{13}=4.92\hat{i}+4.88\hat{j}+5.04\hat{k}$,\;\;\;$\vec{r}_{14}=4.81\hat{i}+4.88\hat{j}+4.88\hat{k}$,\;\;\;$\vec{r}_{23}=4.93\hat{i}+4.88\hat{j}+5.07\hat{k}$.

{\tiny 1D-M95:}   $\hat{n}_{12}=-0.89\hat{i}-0.29\hat{j}-0.36\hat{k}$,\;\;\;$\hat{n}_{13}=0.66\hat{i}+0.57\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{24}=-0.16\hat{i}-0.53\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.63\hat{j}+0.26\hat{k}$,\;\;\;$\vec{r}_{13}=4.73\hat{i}+4.26\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=5.36\hat{i}+5.47\hat{j}+4.87\hat{k}$,\;\;\;$\vec{r}_{34}=4.74\hat{i}+5.76\hat{j}+4.86\hat{k}$.

{\tiny 1D-M96:}   $\hat{n}_{12}=-0.52\hat{i}-0.13\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{13}=0.7\hat{i}-0.64\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.18\hat{i}-0.95\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{34}=-0.49\hat{i}-0.76\hat{j}-0.42\hat{k}$,\;\;\;$\vec{r}_{12}=3.53\hat{i}+7.37\hat{j}+5.85\hat{k}$,\;\;\;$\vec{r}_{13}=7.27\hat{i}+7.33\hat{j}+2.16\hat{k}$,\;\;\;$\vec{r}_{34}=3.23\hat{i}+6.27\hat{j}+4.91\hat{k}$.



==> contentfolder/mechanisms2/result/dof2/result2.tex <==
Manipulator 2:

$\vec{r}_{12}=1.83\hat{i}+2.97\hat{j}+1.26\hat{k}$\newline
$\vec{r}_{23}=0.83\hat{i}+6.09\hat{j}+0.81\hat{k}$\newline
$\hat{n}_{23}=-0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$\newline
$\hat{n}_{12}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$



==> contentfolder/mechanisms2/result/dof2/result3.tex <==
Manipulator 3:

$\vec{r}_{23}=5.55\hat{i}+9.95\hat{j}+0.02\hat{k}$\newline
$\hat{n}_{23}=0.02\hat{i}+0.79\hat{j}-0.61\hat{k}$\newline
$\hat{n}_{12}=-0.0\hat{i}-0.54\hat{j}-0.84\hat{k}$



==> contentfolder/mechanisms2/result/dof2/result3_full.tex <==


{\tiny 3D-M1:}\label{result_3_1}   $\hat{n}_{13}=-0.71\hat{i}+0.11\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.46\hat{j}-0.34\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 3D-M2:}   $\hat{n}_{13}=-0.8\hat{i}+0.33\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}+0.67\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.67\hat{j}-0.48\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 3D-M3:}   $\hat{n}_{13}=-0.8\hat{i}+0.58\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{23}=-0.74\hat{i}-0.51\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}+0.16\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 3D-M4:}   $\hat{n}_{13}=-0.57\hat{i}-0.67\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.36\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.76\hat{i}-0.65\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 3D-M5:}   $\hat{n}_{13}=0.5\hat{i}+0.18\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.76\hat{i}-0.61\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{24}=0.03\hat{i}+0.33\hat{j}-0.94\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 3D-M6:}   $\hat{n}_{13}=-0.6\hat{i}-0.76\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=0.26\hat{i}+0.4\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=-0.21\hat{i}-0.17\hat{j}+0.96\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 3D-M7:}   $\hat{n}_{13}=-0.54\hat{i}-0.83\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{23}=0.18\hat{i}-0.26\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{24}=-0.04\hat{i}-0.56\hat{j}-0.83\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 3D-M8:}\label{result_3_8}   $\hat{n}_{13}=0.41\hat{i}+0.89\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}+0.11\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.67\hat{i}+0.44\hat{j}+0.59\hat{k}$.



==> contentfolder/mechanisms2/result/dof2/result4.tex <==
Manipulator 4:

$\hat{n}_{23}=0.1\hat{i}-0.12\hat{j}-0.99\hat{k}$\newline
$\hat{n}_{12}=0.0\hat{i}+0.66\hat{j}+0.75\hat{k}$



==> contentfolder/mechanisms2/result/dof2/result4_full.tex <==


{\tiny 4D-M1:}\label{result_4_1}   $\hat{n}_{14}=-0.29\hat{i}+0.57\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.75\hat{i}-0.53\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.34\hat{i}+0.83\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{34}=-0.72\hat{i}+0.12\hat{j}+0.69\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M2:}   $\hat{n}_{14}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{23}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=-0.42\hat{i}-0.85\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{34}=0.57\hat{i}+0.69\hat{j}+0.45\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M3:}   $\hat{n}_{14}=0.39\hat{i}+0.47\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{23}=-0.42\hat{i}-0.85\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.69\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.49\hat{j}-0.3\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M4:}   $\hat{n}_{14}=0.42\hat{i}+0.85\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{23}=-0.57\hat{i}-0.69\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{25}=-0.39\hat{i}-0.47\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.49\hat{j}-0.3\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M5:}   $\hat{n}_{14}=-0.57\hat{i}-0.69\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}+0.85\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M6:}   $\hat{n}_{14}=-0.54\hat{i}-0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.53\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.81\hat{j}-0.12\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M7:}   $\hat{n}_{14}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.05\hat{i}+0.94\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}+0.22\hat{j}-0.49\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M8:}   $\hat{n}_{14}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}+0.85\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{25}=-0.8\hat{i}-0.46\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M9:}   $\hat{n}_{14}=-0.08\hat{i}-0.96\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{23}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=-0.84\hat{i}-0.08\hat{j}+0.53\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M10:}   $\hat{n}_{14}=-0.63\hat{i}-0.76\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}+0.59\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.

{\tiny 4D-M11:}   $\hat{n}_{14}=-0.32\hat{i}+0.81\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.78\hat{i}+0.52\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.54\hat{i}+0.84\hat{j}+0.08\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.

{\tiny 4D-M12:}   $\hat{n}_{14}=0.09\hat{i}-1.0\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{23}=0.67\hat{i}+0.35\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}-0.88\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{34}=-0.75\hat{i}+0.31\hat{j}+0.59\hat{k}$,\;\;\;$\vec{r}_{14}=4.0\hat{i}+2.99\hat{j}+5.94\hat{k}$.

{\tiny 4D-M13:}\label{result_4_13}   $\hat{n}_{14}=-0.94\hat{i}-0.18\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{23}=0.32\hat{i}-0.95\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=-0.03\hat{i}-0.8\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=0.34\hat{i}-0.57\hat{j}-0.75\hat{k}$,\;\;\;$\vec{r}_{23}=7.59\hat{i}+3.33\hat{j}+4.0\hat{k}$.

{\tiny 4D-M14:}   $\hat{n}_{14}=-0.38\hat{i}-0.54\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.53\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=0.34\hat{i}-0.93\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{34}=0.75\hat{i}-0.65\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{25}=3.55\hat{i}+6.33\hat{j}+6.15\hat{k}$.

{\tiny 4D-M15:}   $\hat{n}_{14}=-0.19\hat{i}-0.68\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.56\hat{i}-0.67\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{25}=-0.8\hat{i}-0.3\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}-0.54\hat{j}+0.05\hat{k}$,\;\;\;$\vec{r}_{34}=3.99\hat{i}+5.66\hat{j}+6.62\hat{k}$.

==> contentfolder/mechanisms2/result/dof2/result642.tex <==
{\tiny 2D-M642:}

$\hat{n}_{12}=0.05\hat{i}+0.55\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}-0.5\hat{j}-0.28\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2/result643.tex <==
{\tiny 2D-M643:}

$\hat{n}_{12}=0.73\hat{i}-0.15\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{23}=-0.03\hat{i}-0.63\hat{j}+0.78\hat{k}$,\;\;\;$\vec{r}_{12}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2/result644.tex <==
{\tiny 2D-M644:}

$\hat{n}_{12}=-0.68\hat{i}-0.48\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{23}=0.55\hat{i}-0.74\hat{j}-0.39\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2/result645.tex <==
{\tiny 2D-M645:}

$\hat{n}_{12}=0.97\hat{i}+0.03\hat{j}+0.24\hat{k}$,\;\;\;$\hat{n}_{23}=0.03\hat{i}-1.0\hat{j}-0.01\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result1.tex <==
{\tiny 2D-M1:}

$\hat{n}_{14}=0.0\hat{i}+0.96\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.32\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=0.1\hat{i}-0.67\hat{j}+0.74\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result10.tex <==
{\tiny 2D-M10:}

$\hat{n}_{14}=0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.57\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result100.tex <==
{\tiny 2D-M100:}

$\hat{n}_{13}=0.86\hat{i}-0.36\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{24}=0.81\hat{i}+0.47\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.05\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.69\hat{j}+0.73\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result101.tex <==
{\tiny 2D-M101:}

$\hat{n}_{13}=-0.5\hat{i}-0.83\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{23}=-0.08\hat{i}-0.53\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.97\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{45}=-0.83\hat{i}-0.4\hat{j}-0.4\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result102.tex <==
{\tiny 2D-M102:}

$\hat{n}_{13}=0.97\hat{i}+0.01\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.36\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=0.48\hat{i}-0.52\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.34\hat{i}-0.57\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result103.tex <==
{\tiny 2D-M103:}

$\hat{n}_{13}=-0.86\hat{i}-0.27\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.68\hat{i}-0.68\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{35}=0.69\hat{i}+0.27\hat{j}-0.67\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result104.tex <==
{\tiny 2D-M104:}

$\hat{n}_{13}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.99\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.39\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}+0.51\hat{j}-0.26\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result105.tex <==
{\tiny 2D-M105:}

$\hat{n}_{14}=-0.0\hat{i}+0.56\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{24}=-0.35\hat{i}+0.49\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.59\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}-0.67\hat{j}-0.13\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result106.tex <==
{\tiny 2D-M106:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.82\hat{i}-0.08\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.6\hat{i}-0.61\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.61\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.01\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result107.tex <==
{\tiny 2D-M107:}

$\hat{n}_{14}=0.53\hat{i}-0.74\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.69\hat{i}+0.12\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{25}=-0.6\hat{i}+0.75\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.63\hat{i}-0.48\hat{j}+0.62\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result108.tex <==
{\tiny 2D-M108:}

$\hat{n}_{14}=0.0\hat{i}+0.64\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.74\hat{i}+0.55\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{35}=-0.54\hat{i}-0.58\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result109.tex <==
{\tiny 2D-M109:}

$\hat{n}_{14}=0.08\hat{i}-0.62\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.67\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.57\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{35}=-0.82\hat{i}+0.38\hat{j}-0.43\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result11.tex <==
{\tiny 2D-M11:}

$\hat{n}_{14}=0.69\hat{i}+0.47\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{34}=0.03\hat{i}-0.89\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{45}=-0.02\hat{i}+0.86\hat{j}+0.5\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=5.17\hat{i}+6.28\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{25}=5.29\hat{i}+3.75\hat{j}+5.48\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result110.tex <==
{\tiny 2D-M110:}

$\hat{n}_{14}=0.82\hat{i}+0.06\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{24}=-0.35\hat{i}-0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{34}=-0.7\hat{i}+0.01\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}+0.58\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result111.tex <==
{\tiny 2D-M111:}

$\hat{n}_{14}=-0.11\hat{i}+0.79\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}-0.33\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{25}=0.66\hat{i}-0.07\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{34}=0.11\hat{i}+0.99\hat{j}-0.08\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result112.tex <==
{\tiny 2D-M112:}

$\hat{n}_{14}=0.32\hat{i}+0.93\hat{j}+0.17\hat{k}$,\;\;\;$\hat{n}_{24}=0.48\hat{i}-0.75\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.65\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{35}=0.19\hat{i}+0.7\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result113.tex <==
{\tiny 2D-M113:}

$\hat{n}_{14}=0.8\hat{i}-0.48\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.95\hat{i}-0.22\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{35}=-0.36\hat{i}+0.36\hat{j}-0.86\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result114.tex <==
{\tiny 2D-M114:}

$\hat{n}_{14}=-0.69\hat{i}+0.71\hat{j}+0.17\hat{k}$,\;\;\;$\hat{n}_{24}=-0.54\hat{i}+0.63\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}+0.7\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result115.tex <==
{\tiny 2D-M115:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.57\hat{i}+0.27\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.86\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{35}=-0.62\hat{i}-0.62\hat{j}-0.48\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+9.95\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result116.tex <==
{\tiny 2D-M116:}

$\hat{n}_{14}=0.76\hat{i}-0.61\hat{j}+0.24\hat{k}$,\;\;\;$\hat{n}_{24}=0.01\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}-0.41\hat{j}-0.4\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result117.tex <==
{\tiny 2D-M117:}

$\hat{n}_{14}=0.23\hat{i}-0.48\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.94\hat{i}-0.33\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{25}=-0.61\hat{i}+0.57\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.69\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result118.tex <==
{\tiny 2D-M118:}

$\hat{n}_{14}=0.02\hat{i}+0.57\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.65\hat{i}-0.75\hat{j}-0.1\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.49\hat{i}-0.32\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result119.tex <==
{\tiny 2D-M119:}

$\hat{n}_{14}=-0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.78\hat{i}+0.01\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{25}=-0.41\hat{i}+0.82\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result12.tex <==
{\tiny 2D-M12:}

$\hat{n}_{14}=0.7\hat{i}+0.53\hat{j}-0.47\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.85\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{25}=-0.05\hat{i}+0.72\hat{j}-0.69\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result120.tex <==
{\tiny 2D-M120:}

$\hat{n}_{14}=0.31\hat{i}+0.36\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}-0.4\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=0.83\hat{i}+0.37\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result121.tex <==
{\tiny 2D-M121:}

$\hat{n}_{14}=0.9\hat{i}+0.39\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.93\hat{i}+0.25\hat{j}-0.25\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result122.tex <==
{\tiny 2D-M122:}

$\hat{n}_{14}=-0.66\hat{i}+0.15\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.63\hat{i}+0.55\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=0.77\hat{i}-0.45\hat{j}-0.45\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result123.tex <==
{\tiny 2D-M123:}

$\hat{n}_{14}=0.61\hat{i}+0.04\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.42\hat{i}-0.89\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{34}=0.15\hat{i}+0.62\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result124.tex <==
{\tiny 2D-M124:}

$\hat{n}_{14}=0.25\hat{i}-0.67\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result125.tex <==
{\tiny 2D-M125:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.41\hat{i}-0.82\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{34}=0.31\hat{i}-0.6\hat{j}-0.73\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.67\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result126.tex <==
{\tiny 2D-M126:}

$\hat{n}_{14}=0.43\hat{i}-0.74\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.07\hat{i}-0.94\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{25}=0.07\hat{i}-0.83\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=0.02\hat{i}+0.87\hat{j}+0.5\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=4.06\hat{i}+3.92\hat{j}+4.65\hat{k}$,\;\;\;$\vec{r}_{34}=5.03\hat{i}+4.27\hat{j}+5.76\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result127.tex <==
{\tiny 2D-M127:}

$\hat{n}_{14}=-0.0\hat{i}+0.59\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.72\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{34}=-0.82\hat{i}-0.45\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{45}=-0.06\hat{i}+0.7\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result128.tex <==
{\tiny 2D-M128:}

$\hat{n}_{14}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{23}=-0.2\hat{i}-0.95\hat{j}+0.24\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.81\hat{j}-0.05\hat{k}$,\;\;\;$\hat{n}_{45}=-0.59\hat{i}+0.15\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=6.36\hat{i}+5.69\hat{j}+8.17\hat{k}$,\;\;\;$\vec{r}_{34}=6.17\hat{i}+5.22\hat{j}+2.99\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result129.tex <==
{\tiny 2D-M129:}

$\hat{n}_{14}=-0.71\hat{i}+0.09\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}+0.67\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result13.tex <==
{\tiny 2D-M13:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.07\hat{i}-0.64\hat{j}-0.76\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result130.tex <==
{\tiny 2D-M130:}

$\hat{n}_{14}=-0.53\hat{i}+0.27\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{23}=-0.9\hat{i}+0.11\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.67\hat{i}-0.67\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result131.tex <==
{\tiny 2D-M131:}

$\hat{n}_{14}=-0.09\hat{i}-0.53\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{23}=0.7\hat{i}+0.38\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.69\hat{i}+0.11\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{34}=-0.81\hat{i}+0.56\hat{j}-0.15\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result132.tex <==
{\tiny 2D-M132:}

$\hat{n}_{14}=0.01\hat{i}+0.86\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{23}=0.41\hat{i}-0.89\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{25}=0.09\hat{i}-0.99\hat{j}+0.07\hat{k}$,\;\;\;$\hat{n}_{45}=0.43\hat{i}-0.74\hat{j}+0.51\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=2.99\hat{i}+6.07\hat{j}+3.02\hat{k}$,\;\;\;$\vec{r}_{34}=6.84\hat{i}+4.37\hat{j}+3.84\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result133.tex <==
{\tiny 2D-M133:}

$\hat{n}_{14}=0.81\hat{i}-0.36\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{23}=0.9\hat{i}+0.31\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.44\hat{i}+0.64\hat{j}-0.64\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result134.tex <==
{\tiny 2D-M134:}

$\hat{n}_{14}=0.38\hat{i}+0.67\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.98\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{34}=0.65\hat{i}-0.75\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}-0.1\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.69\hat{i}+5.22\hat{j}+4.09\hat{k}$,\;\;\;$\vec{r}_{25}=3.77\hat{i}+3.77\hat{j}+3.8\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result135.tex <==
{\tiny 2D-M135:}

$\hat{n}_{14}=-0.13\hat{i}+0.65\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{25}=-0.6\hat{i}+0.78\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.56\hat{i}+0.24\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result136.tex <==
{\tiny 2D-M136:}

$\hat{n}_{14}=-0.0\hat{i}+0.57\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{25}=0.69\hat{i}-0.69\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.87\hat{i}+0.21\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.56\hat{j}-0.83\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result137.tex <==
{\tiny 2D-M137:}

$\hat{n}_{14}=-0.43\hat{i}-0.25\hat{j}-0.87\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result138.tex <==
{\tiny 2D-M138:}

$\hat{n}_{14}=0.17\hat{i}-0.5\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{25}=-0.79\hat{i}-0.49\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{34}=-0.35\hat{i}-0.79\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{45}=0.77\hat{i}-0.23\hat{j}+0.6\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.47\hat{i}+3.98\hat{j}+5.17\hat{k}$,\;\;\;$\vec{r}_{34}=9.55\hat{i}+4.3\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result139.tex <==
{\tiny 2D-M139:}

$\hat{n}_{14}=-0.0\hat{i}+0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=0.54\hat{i}-0.14\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{34}=0.17\hat{i}-0.7\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{45}=0.63\hat{i}+0.7\hat{j}-0.34\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result14.tex <==
{\tiny 2D-M14:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}+0.09\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result140.tex <==
{\tiny 2D-M140:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.39\hat{i}+0.27\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{34}=-0.19\hat{i}-0.77\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.74\hat{j}-0.67\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+9.9\hat{k}$,\;\;\;$\vec{r}_{23}=4.36\hat{i}+0.9\hat{j}+3.84\hat{k}$,\;\;\;$\vec{r}_{25}=7.17\hat{i}+1.16\hat{j}+6.63\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result141.tex <==
{\tiny 2D-M141:}

$\hat{n}_{14}=-0.38\hat{i}+0.38\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{15}=0.93\hat{i}-0.2\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.95\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.74\hat{j}+0.67\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result142.tex <==
{\tiny 2D-M142:}

$\hat{n}_{14}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+8.6\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result143.tex <==
{\tiny 2D-M143:}

$\hat{n}_{14}=-0.19\hat{i}+0.78\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{15}=-0.71\hat{i}+0.69\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{23}=-0.68\hat{i}-0.7\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{25}=0.79\hat{i}-0.24\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result144.tex <==
{\tiny 2D-M144:}

$\hat{n}_{14}=0.24\hat{i}+0.8\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{15}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.65\hat{i}+0.74\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{34}=0.9\hat{i}-0.31\hat{j}-0.31\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+9.72\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result145.tex <==
{\tiny 2D-M145:}

$\hat{n}_{14}=0.28\hat{i}-0.8\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{15}=0.69\hat{i}-0.71\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{25}=0.77\hat{i}-0.15\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{34}=0.7\hat{i}+0.68\hat{j}-0.21\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result146.tex <==
{\tiny 2D-M146:}

$\hat{n}_{14}=0.69\hat{i}+0.02\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.43\hat{i}-0.82\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result147.tex <==
{\tiny 2D-M147:}

$\hat{n}_{14}=-0.44\hat{i}-0.86\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.36\hat{i}+0.55\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{25}=0.55\hat{i}-0.62\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{34}=0.54\hat{i}-0.25\hat{j}+0.81\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result148.tex <==
{\tiny 2D-M148:}

$\hat{n}_{14}=0.92\hat{i}+0.25\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{23}=0.14\hat{i}+0.63\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{25}=-0.06\hat{i}+0.68\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{34}=0.59\hat{i}-0.57\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result149.tex <==
{\tiny 2D-M149:}

$\hat{n}_{14}=-0.36\hat{i}+0.55\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{23}=0.55\hat{i}-0.62\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.44\hat{i}+0.86\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{34}=-0.54\hat{i}+0.25\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result15.tex <==
{\tiny 2D-M15:}

$\hat{n}_{13}=-0.46\hat{i}+0.74\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result150.tex <==
{\tiny 2D-M150:}

$\hat{n}_{14}=-0.23\hat{i}+0.48\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.61\hat{i}+0.57\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{34}=-0.94\hat{i}-0.33\hat{j}-0.03\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result151.tex <==
{\tiny 2D-M151:}

$\hat{n}_{14}=0.61\hat{i}-0.2\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.34\hat{i}-0.46\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{25}=0.8\hat{i}+0.48\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{34}=0.62\hat{i}-0.55\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result152.tex <==
{\tiny 2D-M152:}

$\hat{n}_{14}=0.66\hat{i}-0.45\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{23}=-0.5\hat{i}+0.8\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.29\hat{i}+0.06\hat{j}-0.95\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result153.tex <==
{\tiny 2D-M153:}

$\hat{n}_{14}=-0.06\hat{i}+0.99\hat{j}-0.11\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.86\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.73\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result154.tex <==
{\tiny 2D-M154:}

$\hat{n}_{14}=0.49\hat{i}+0.46\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.29\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{25}=-0.55\hat{i}-0.55\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{35}=0.46\hat{i}-0.88\hat{j}-0.05\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result155.tex <==
{\tiny 2D-M155:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.66\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{25}=0.9\hat{i}+0.28\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result156.tex <==
{\tiny 2D-M156:}

$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.73\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.66\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{35}=0.08\hat{i}-0.7\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result157.tex <==
{\tiny 2D-M157:}

$\hat{n}_{14}=-0.0\hat{i}+0.64\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.91\hat{i}+0.32\hat{j}+0.27\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result158.tex <==
{\tiny 2D-M158:}

$\hat{n}_{14}=0.0\hat{i}+0.92\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{24}=0.15\hat{i}+0.34\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{25}=0.44\hat{i}+0.4\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{35}=-0.49\hat{i}-0.72\hat{j}-0.49\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result159.tex <==
{\tiny 2D-M159:}

$\hat{n}_{14}=-0.03\hat{i}+0.83\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{23}=0.54\hat{i}+0.67\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.62\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.1\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result16.tex <==
{\tiny 2D-M16:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.16\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{45}=-0.27\hat{i}+0.32\hat{j}-0.91\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result160.tex <==
{\tiny 2D-M160:}

$\hat{n}_{14}=-0.24\hat{i}-0.94\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{23}=0.65\hat{i}-0.65\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.11\hat{i}-0.7\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{45}=-0.51\hat{i}+0.46\hat{j}+0.73\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result161.tex <==
{\tiny 2D-M161:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.14\hat{i}+0.36\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.48\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{34}=0.66\hat{i}+0.34\hat{j}-0.67\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result162.tex <==
{\tiny 2D-M162:}

$\hat{n}_{14}=0.16\hat{i}+0.5\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{23}=0.65\hat{i}-0.38\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.5\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{45}=0.72\hat{i}-0.35\hat{j}+0.6\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result163.tex <==
{\tiny 2D-M163:}

$\hat{n}_{14}=-0.0\hat{i}+0.64\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.98\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.67\hat{i}-0.3\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.49\hat{j}-0.87\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result164.tex <==
{\tiny 2D-M164:}

$\hat{n}_{14}=0.55\hat{i}+0.44\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}-0.71\hat{j}-0.07\hat{k}$,\;\;\;$\hat{n}_{34}=0.63\hat{i}+0.74\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{45}=-0.73\hat{i}+0.68\hat{j}+0.1\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result165.tex <==
{\tiny 2D-M165:}

$\hat{n}_{14}=-0.98\hat{i}-0.16\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{23}=-0.32\hat{i}-0.84\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.74\hat{i}+0.36\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}+0.65\hat{j}+0.21\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result166.tex <==
{\tiny 2D-M166:}

$\hat{n}_{14}=0.44\hat{i}+0.11\hat{j}-0.89\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.86\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=-0.62\hat{i}+0.14\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.54\hat{j}-0.84\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result167.tex <==
{\tiny 2D-M167:}

$\hat{n}_{14}=-0.83\hat{i}+0.47\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{23}=-0.67\hat{i}-0.68\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{34}=-0.6\hat{i}+0.6\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{45}=0.67\hat{i}-0.57\hat{j}-0.48\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result168.tex <==
{\tiny 2D-M168:}

$\hat{n}_{14}=-0.0\hat{i}+0.74\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.6\hat{i}-0.54\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{34}=-0.64\hat{i}-0.54\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.45\hat{j}-0.89\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result169.tex <==
{\tiny 2D-M169:}

$\hat{n}_{14}=-0.49\hat{i}-0.87\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=0.41\hat{i}+0.91\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.49\hat{i}+0.53\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result17.tex <==
{\tiny 2D-M17:}

$\hat{n}_{13}=0.71\hat{i}-0.11\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result170.tex <==
{\tiny 2D-M170:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.36\hat{i}+0.86\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.92\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result171.tex <==
{\tiny 2D-M171:}

$\hat{n}_{14}=-0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{15}=0.92\hat{i}-0.07\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.48\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result172.tex <==
{\tiny 2D-M172:}

$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{15}=0.0\hat{i}+0.39\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.77\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{34}=-0.8\hat{i}+0.28\hat{j}+0.52\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result173.tex <==
{\tiny 2D-M173:}

$\hat{n}_{14}=0.48\hat{i}+0.68\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{15}=0.02\hat{i}+0.84\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.61\hat{i}-0.78\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.35\hat{j}-0.94\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result174.tex <==
{\tiny 2D-M174:}

$\hat{n}_{14}=0.52\hat{i}-0.77\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{23}=0.4\hat{i}-0.7\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{25}=0.7\hat{i}-0.62\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{34}=0.81\hat{i}+0.29\hat{j}-0.51\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result175.tex <==
{\tiny 2D-M175:}

$\hat{n}_{14}=-0.99\hat{i}+0.16\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{23}=0.8\hat{i}-0.15\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.12\hat{i}-0.53\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{34}=-0.83\hat{i}-0.55\hat{j}-0.09\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result176.tex <==
{\tiny 2D-M176:}

$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.95\hat{i}+0.17\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.22\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{34}=-0.02\hat{i}-0.78\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result177.tex <==
{\tiny 2D-M177:}

$\hat{n}_{14}=0.68\hat{i}+0.71\hat{j}-0.19\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.51\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.26\hat{j}-0.97\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result178.tex <==
{\tiny 2D-M178:}

$\hat{n}_{14}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.87\hat{i}-0.5\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result179.tex <==
{\tiny 2D-M179:}

$\hat{n}_{14}=-0.9\hat{i}-0.44\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.76\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.34\hat{i}+0.93\hat{j}-0.14\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.02\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result18.tex <==
{\tiny 2D-M18:}

$\hat{n}_{13}=-0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.04\hat{i}+0.73\hat{j}+0.68\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result180.tex <==
{\tiny 2D-M180:}

$\hat{n}_{15}=0.92\hat{i}-0.1\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}-0.39\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result181.tex <==
{\tiny 2D-M181:}

$\hat{n}_{15}=-0.71\hat{i}-0.23\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{23}=-0.69\hat{i}+0.02\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{25}=0.68\hat{i}-0.21\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{34}=0.43\hat{i}+0.82\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result182.tex <==
{\tiny 2D-M182:}

$\hat{n}_{15}=-0.62\hat{i}-0.69\hat{j}-0.38\hat{k}$,\;\;\;$\hat{n}_{23}=-0.71\hat{i}+0.67\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{25}=0.78\hat{i}+0.17\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{34}=-0.25\hat{i}-0.8\hat{j}-0.55\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result183.tex <==
{\tiny 2D-M183:}

$\hat{n}_{13}=-0.61\hat{i}-0.5\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{14}=-0.64\hat{i}+0.77\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{25}=0.72\hat{i}-0.69\hat{j}-0.03\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result184.tex <==
{\tiny 2D-M184:}

$\hat{n}_{13}=-0.88\hat{i}-0.06\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{14}=0.48\hat{i}+0.33\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=-0.55\hat{i}-0.59\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{35}=-0.64\hat{i}+0.75\hat{j}-0.19\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result185.tex <==
{\tiny 2D-M185:}

$\hat{n}_{13}=-0.62\hat{i}+0.62\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{14}=0.66\hat{i}-0.03\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.72\hat{i}-0.03\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.57\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result186.tex <==
{\tiny 2D-M186:}

$\hat{n}_{13}=-0.26\hat{i}+0.46\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{14}=-0.66\hat{i}-0.53\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{24}=0.27\hat{i}+0.88\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result187.tex <==
{\tiny 2D-M187:}

$\hat{n}_{13}=0.72\hat{i}-0.48\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{14}=0.8\hat{i}-0.25\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.14\hat{i}+0.67\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{35}=-0.07\hat{i}+0.73\hat{j}-0.68\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result188.tex <==
{\tiny 2D-M188:}

$\hat{n}_{13}=0.0\hat{i}+0.5\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{14}=-0.67\hat{i}+0.67\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{25}=0.9\hat{i}+0.11\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result189.tex <==
{\tiny 2D-M189:}

$\hat{n}_{13}=0.65\hat{i}-0.65\hat{j}-0.38\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}+0.61\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.87\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.84\hat{j}+0.55\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result19.tex <==
{\tiny 2D-M19:}

$\hat{n}_{13}=-0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result190.tex <==
{\tiny 2D-M190:}

$\hat{n}_{13}=0.02\hat{i}-0.58\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{14}=-0.84\hat{i}-0.33\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{23}=-0.13\hat{i}-0.9\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{35}=-0.36\hat{i}+0.37\hat{j}-0.86\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=2.49\hat{i}+4.03\hat{j}+6.6\hat{k}$,\;\;\;$\vec{r}_{23}=2.43\hat{i}+3.38\hat{j}+6.05\hat{k}$,\;\;\;$\vec{r}_{24}=3.44\hat{i}+3.7\hat{j}+2.4\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result191.tex <==
{\tiny 2D-M191:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{23}=-0.88\hat{i}-0.3\hat{j}-0.36\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result192.tex <==
{\tiny 2D-M192:}

$\hat{n}_{13}=0.04\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.48\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.7\hat{i}+0.23\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.89\hat{i}+0.46\hat{j}+0.03\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result193.tex <==
{\tiny 2D-M193:}

$\hat{n}_{13}=-0.0\hat{i}+0.51\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.62\hat{i}-0.48\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result194.tex <==
{\tiny 2D-M194:}

$\hat{n}_{13}=-0.68\hat{i}-0.73\hat{j}+0.06\hat{k}$,\;\;\;$\hat{n}_{14}=-0.46\hat{i}-0.83\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{24}=0.49\hat{i}+0.05\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{25}=-0.33\hat{i}+0.62\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result195.tex <==
{\tiny 2D-M195:}

$\hat{n}_{13}=0.0\hat{i}+0.53\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{14}=-0.76\hat{i}+0.63\hat{j}-0.19\hat{k}$,\;\;\;$\hat{n}_{24}=-0.15\hat{i}-0.45\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{35}=0.64\hat{i}+0.46\hat{j}-0.61\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result196.tex <==
{\tiny 2D-M196:}

$\hat{n}_{13}=-0.38\hat{i}-0.4\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{14}=0.72\hat{i}+0.0\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.7\hat{i}-0.08\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{35}=0.56\hat{i}+0.54\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result197.tex <==
{\tiny 2D-M197:}

$\hat{n}_{13}=-0.17\hat{i}+0.74\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{14}=0.79\hat{i}-0.59\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{25}=0.31\hat{i}+0.6\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{35}=-0.53\hat{i}-0.57\hat{j}-0.63\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result198.tex <==
{\tiny 2D-M198:}

$\hat{n}_{13}=-0.78\hat{i}+0.61\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{14}=-0.68\hat{i}-0.51\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.02\hat{i}+0.69\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{25}=-0.9\hat{i}-0.27\hat{j}+0.33\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result199.tex <==
{\tiny 2D-M199:}

$\hat{n}_{13}=-1.0\hat{i}+0.02\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.46\hat{j}-0.89\hat{k}$,\;\;\;$\hat{n}_{45}=0.09\hat{i}+0.72\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result2.tex <==
{\tiny 2D-M2:}

$\hat{n}_{14}=-0.31\hat{i}+0.43\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}-0.01\hat{j}+0.72\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result20.tex <==
{\tiny 2D-M20:}

$\hat{n}_{13}=0.28\hat{i}-0.83\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+9.95\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result200.tex <==
{\tiny 2D-M200:}

$\hat{n}_{13}=0.66\hat{i}-0.03\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.51\hat{i}-0.45\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.72\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result201.tex <==
{\tiny 2D-M201:}

$\hat{n}_{13}=-0.45\hat{i}+0.37\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.06\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.44\hat{j}-0.9\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result202.tex <==
{\tiny 2D-M202:}

$\hat{n}_{13}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.65\hat{i}+0.11\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{23}=-0.5\hat{i}-0.81\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{45}=0.13\hat{i}-0.77\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result203.tex <==
{\tiny 2D-M203:}

$\hat{n}_{13}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.89\hat{i}-0.4\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.51\hat{i}-0.77\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{35}=0.83\hat{i}+0.55\hat{j}+0.11\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.28\hat{i}+4.6\hat{j}+5.29\hat{k}$,\;\;\;$\vec{r}_{24}=5.29\hat{i}+5.38\hat{j}+4.64\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result204.tex <==
{\tiny 2D-M204:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.68\hat{i}+0.43\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.78\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{25}=0.66\hat{i}-0.02\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+6.32\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result205.tex <==
{\tiny 2D-M205:}

$\hat{n}_{13}=-0.0\hat{i}+0.81\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{14}=-0.51\hat{i}-0.48\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.76\hat{i}-0.0\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{45}=0.72\hat{i}+0.22\hat{j}+0.66\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result206.tex <==
{\tiny 2D-M206:}

$\hat{n}_{13}=-0.0\hat{i}+0.41\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{14}=-0.14\hat{i}+0.59\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.81\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.6\hat{i}+0.18\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result207.tex <==
{\tiny 2D-M207:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.11\hat{i}-0.65\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=0.81\hat{i}+0.5\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{45}=-0.06\hat{i}+0.56\hat{j}+0.83\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result208.tex <==
{\tiny 2D-M208:}

$\hat{n}_{13}=0.36\hat{i}+0.64\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{14}=-0.01\hat{i}-0.52\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{24}=0.52\hat{i}+0.04\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{35}=0.81\hat{i}+0.05\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.3\hat{i}+4.88\hat{j}+5.01\hat{k}$,\;\;\;$\vec{r}_{24}=3.68\hat{i}+4.58\hat{j}+4.75\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result209.tex <==
{\tiny 2D-M209:}

$\hat{n}_{13}=-0.7\hat{i}-0.01\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}-0.82\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}-0.58\hat{j}+0.82\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result21.tex <==
{\tiny 2D-M21:}

$\hat{n}_{14}=0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{24}=-0.68\hat{i}+0.06\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result210.tex <==
{\tiny 2D-M210:}

$\hat{n}_{13}=-0.7\hat{i}-0.7\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{14}=0.46\hat{i}-0.36\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.35\hat{i}-0.4\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.57\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result211.tex <==
{\tiny 2D-M211:}

$\hat{n}_{13}=-0.0\hat{i}+0.59\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{14}=0.62\hat{i}+0.35\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.04\hat{i}+0.83\hat{j}-0.56\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+8.83\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result212.tex <==
{\tiny 2D-M212:}

$\hat{n}_{13}=0.47\hat{i}+0.0\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{14}=-0.94\hat{i}-0.04\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.22\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{25}=0.66\hat{i}+0.54\hat{j}-0.52\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result213.tex <==
{\tiny 2D-M213:}

$\hat{n}_{13}=-0.57\hat{i}-0.42\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.88\hat{i}+0.45\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{24}=-0.82\hat{i}+0.36\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{35}=-0.13\hat{i}+0.77\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.57\hat{i}+2.56\hat{j}+7.35\hat{k}$,\;\;\;$\vec{r}_{25}=2.49\hat{i}+4.52\hat{j}+2.78\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result214.tex <==
{\tiny 2D-M214:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.57\hat{i}+0.52\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.71\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{35}=-0.43\hat{i}-0.46\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result215.tex <==
{\tiny 2D-M215:}

$\hat{n}_{13}=0.46\hat{i}-0.33\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{14}=-0.64\hat{i}+0.67\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{25}=0.79\hat{i}-0.55\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{35}=-0.71\hat{i}+0.12\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=8.26\hat{i}+4.82\hat{j}+7.98\hat{k}$,\;\;\;$\vec{r}_{24}=7.31\hat{i}+1.36\hat{j}+7.25\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result216.tex <==
{\tiny 2D-M216:}

$\hat{n}_{13}=0.68\hat{i}-0.08\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.72\hat{i}-0.69\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}-0.52\hat{j}+0.24\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+5.72\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result217.tex <==
{\tiny 2D-M217:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.81\hat{i}-0.41\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{23}=0.43\hat{i}-0.64\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{45}=-0.01\hat{i}-0.7\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.2\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result218.tex <==
{\tiny 2D-M218:}

$\hat{n}_{13}=0.78\hat{i}+0.17\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{14}=0.02\hat{i}-0.83\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{23}=-0.64\hat{i}-0.64\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{45}=-0.87\hat{i}-0.24\hat{j}+0.44\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result219.tex <==
{\tiny 2D-M219:}

$\hat{n}_{13}=0.67\hat{i}+0.26\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{14}=-0.92\hat{i}-0.37\hat{j}+0.13\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}-0.91\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{35}=0.68\hat{i}+0.46\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=2.68\hat{i}+4.94\hat{j}+6.84\hat{k}$,\;\;\;$\vec{r}_{23}=8.18\hat{i}+7.07\hat{j}+1.99\hat{k}$,\;\;\;$\vec{r}_{24}=8.1\hat{i}+8.25\hat{j}+5.88\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result22.tex <==
{\tiny 2D-M22:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.62\hat{j}+0.79\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.03\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result220.tex <==
{\tiny 2D-M220:}

$\hat{n}_{13}=-0.52\hat{i}+0.15\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.63\hat{i}-0.54\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result221.tex <==
{\tiny 2D-M221:}

$\hat{n}_{13}=-0.0\hat{i}+0.43\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{14}=0.54\hat{i}+0.68\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.52\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result222.tex <==
{\tiny 2D-M222:}

$\hat{n}_{13}=-0.0\hat{i}+0.97\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.6\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=-0.52\hat{i}+0.75\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{45}=-0.82\hat{i}-0.0\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result223.tex <==
{\tiny 2D-M223:}

$\hat{n}_{13}=0.8\hat{i}+0.54\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{14}=-0.17\hat{i}+0.61\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.81\hat{i}-0.44\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result224.tex <==
{\tiny 2D-M224:}

$\hat{n}_{13}=-0.69\hat{i}-0.5\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{14}=-0.91\hat{i}-0.41\hat{j}+0.11\hat{k}$,\;\;\;$\hat{n}_{23}=0.87\hat{i}+0.46\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{35}=-0.03\hat{i}+0.87\hat{j}-0.5\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.02\hat{i}+5.79\hat{j}+6.14\hat{k}$,\;\;\;$\vec{r}_{24}=3.41\hat{i}+5.22\hat{j}+4.98\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result225.tex <==
{\tiny 2D-M225:}

$\hat{n}_{13}=-0.0\hat{i}+0.61\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.99\hat{i}-0.07\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}+0.52\hat{j}-0.25\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result226.tex <==
{\tiny 2D-M226:}

$\hat{n}_{13}=0.62\hat{i}+0.62\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{14}=0.79\hat{i}+0.24\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.59\hat{i}-0.52\hat{j}+0.62\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result227.tex <==
{\tiny 2D-M227:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}-0.79\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.79\hat{i}-0.61\hat{j}+0.03\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result228.tex <==
{\tiny 2D-M228:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.8\hat{i}-0.25\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.05\hat{i}-0.93\hat{j}-0.36\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result229.tex <==
{\tiny 2D-M229:}

$\hat{n}_{13}=0.07\hat{i}+0.61\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{14}=-0.63\hat{i}-0.46\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=0.3\hat{i}+0.07\hat{j}+0.95\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result23.tex <==
{\tiny 2D-M23:}

$\hat{n}_{14}=0.0\hat{i}+0.79\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.73\hat{j}+0.69\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result230.tex <==
{\tiny 2D-M230:}

$\hat{n}_{13}=0.5\hat{i}+0.61\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{14}=-0.03\hat{i}-0.73\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.43\hat{j}-0.9\hat{k}$,\;\;\;$\hat{n}_{25}=0.21\hat{i}+0.04\hat{j}+0.98\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result231.tex <==
{\tiny 2D-M231:}

$\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.75\hat{i}-0.43\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.67\hat{i}+0.05\hat{j}+0.74\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result232.tex <==
{\tiny 2D-M232:}

$\hat{n}_{13}=-0.5\hat{i}-0.18\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{14}=-0.45\hat{i}+0.89\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{24}=-0.13\hat{i}+0.94\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{35}=0.05\hat{i}-0.83\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=7.26\hat{i}+2.37\hat{j}+4.72\hat{k}$,\;\;\;$\vec{r}_{23}=0.91\hat{i}+0.23\hat{j}+9.74\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result233.tex <==
{\tiny 2D-M233:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.44\hat{i}+0.36\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{24}=-0.53\hat{i}+0.64\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.44\hat{j}-0.9\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result234.tex <==
{\tiny 2D-M234:}

$\hat{n}_{13}=-0.75\hat{i}+0.66\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}-0.56\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{35}=-0.69\hat{i}+0.72\hat{j}-0.03\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result235.tex <==
{\tiny 2D-M235:}

$\hat{n}_{13}=0.31\hat{i}-0.6\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=0.63\hat{i}+0.55\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.19\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{35}=0.71\hat{i}-0.69\hat{j}-0.13\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result236.tex <==
{\tiny 2D-M236:}

$\hat{n}_{13}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}-0.63\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{25}=0.79\hat{i}+0.56\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{35}=-0.29\hat{i}+0.5\hat{j}-0.82\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result237.tex <==
{\tiny 2D-M237:}

$\hat{n}_{13}=-0.17\hat{i}+0.67\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.19\hat{i}-0.97\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}-0.33\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{35}=-0.71\hat{i}+0.1\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=2.89\hat{i}+3.46\hat{j}+8.02\hat{k}$,\;\;\;$\vec{r}_{25}=3.92\hat{i}+1.58\hat{j}+8.22\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result238.tex <==
{\tiny 2D-M238:}

$\hat{n}_{13}=0.53\hat{i}+0.67\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.83\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=-0.76\hat{i}-0.0\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.45\hat{j}-0.68\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result239.tex <==
{\tiny 2D-M239:}

$\hat{n}_{13}=-0.02\hat{i}+0.57\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=0.47\hat{i}-0.88\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.02\hat{i}-0.98\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{35}=0.68\hat{i}+0.54\hat{j}+0.5\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.13\hat{i}+6.46\hat{j}+3.38\hat{k}$,\;\;\;$\vec{r}_{24}=2.82\hat{i}+5.36\hat{j}+3.17\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result24.tex <==
{\tiny 2D-M24:}

$\hat{n}_{14}=0.21\hat{i}+0.81\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+3.96\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result240.tex <==
{\tiny 2D-M240:}

$\hat{n}_{13}=-0.69\hat{i}-0.54\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.22\hat{i}-0.69\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{45}=-0.78\hat{i}+0.2\hat{j}-0.6\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result241.tex <==
{\tiny 2D-M241:}

$\hat{n}_{13}=-0.03\hat{i}+0.84\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.47\hat{i}-0.59\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.66\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result242.tex <==
{\tiny 2D-M242:}

$\hat{n}_{13}=-0.72\hat{i}+0.05\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{23}=-0.71\hat{i}+0.01\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}-0.54\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{45}=0.27\hat{i}+0.43\hat{j}+0.86\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result243.tex <==
{\tiny 2D-M243:}

$\hat{n}_{13}=-0.45\hat{i}-0.23\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{23}=-0.13\hat{i}-0.92\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{24}=-0.94\hat{i}-0.18\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{35}=0.37\hat{i}+0.14\hat{j}+0.92\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.12\hat{i}+5.39\hat{j}+4.42\hat{k}$,\;\;\;$\vec{r}_{23}=5.78\hat{i}+4.24\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{24}=5.54\hat{i}+5.62\hat{j}+5.4\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result244.tex <==
{\tiny 2D-M244:}

$\hat{n}_{13}=0.22\hat{i}+0.43\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{23}=0.57\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.21\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.14\hat{i}+0.37\hat{j}+0.92\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result245.tex <==
{\tiny 2D-M245:}

$\hat{n}_{13}=0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.64\hat{i}+0.56\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{25}=-0.81\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}+0.49\hat{j}+0.52\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result246.tex <==
{\tiny 2D-M246:}

$\hat{n}_{13}=0.0\hat{i}+0.49\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{23}=0.55\hat{i}+0.63\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.69\hat{i}+0.04\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.91\hat{j}-0.42\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result247.tex <==
{\tiny 2D-M247:}

$\hat{n}_{13}=0.43\hat{i}-0.44\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result248.tex <==
{\tiny 2D-M248:}

$\hat{n}_{13}=0.05\hat{i}+0.84\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{23}=-0.23\hat{i}-0.91\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=0.26\hat{i}-0.96\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{35}=-0.63\hat{i}+0.73\hat{j}-0.26\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.95\hat{i}+3.34\hat{j}+4.38\hat{k}$,\;\;\;$\vec{r}_{24}=3.26\hat{i}+3.75\hat{j}+6.05\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result249.tex <==
{\tiny 2D-M249:}

$\hat{n}_{13}=0.0\hat{i}+0.77\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.5\hat{i}-0.5\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{25}=0.54\hat{i}+0.67\hat{j}-0.51\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result25.tex <==
{\tiny 2D-M25:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.26\hat{i}-0.46\hat{j}+0.85\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result250.tex <==
{\tiny 2D-M250:}

$\hat{n}_{13}=0.52\hat{i}-0.84\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{23}=-0.73\hat{i}+0.01\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{45}=-0.57\hat{i}-0.51\hat{j}-0.64\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result251.tex <==
{\tiny 2D-M251:}

$\hat{n}_{13}=-0.33\hat{i}+0.54\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}+0.73\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{25}=0.2\hat{i}+0.67\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{45}=-0.65\hat{i}-0.65\hat{j}-0.38\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result252.tex <==
{\tiny 2D-M252:}

$\hat{n}_{13}=-0.0\hat{i}+0.64\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.52\hat{i}-0.71\hat{j}-0.47\hat{k}$,\;\;\;$\hat{n}_{24}=-0.08\hat{i}-0.68\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result253.tex <==
{\tiny 2D-M253:}

$\hat{n}_{13}=0.63\hat{i}+0.02\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=0.91\hat{i}+0.23\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{24}=0.88\hat{i}+0.24\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{35}=-0.18\hat{i}-0.57\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=6.56\hat{i}+4.75\hat{j}+6.38\hat{k}$,\;\;\;$\vec{r}_{23}=6.53\hat{i}+2.55\hat{j}+7.74\hat{k}$,\;\;\;$\vec{r}_{24}=5.03\hat{i}+4.39\hat{j}+6.92\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result254.tex <==
{\tiny 2D-M254:}

$\hat{n}_{13}=-0.42\hat{i}-0.76\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{23}=0.37\hat{i}+0.8\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{24}=-0.68\hat{i}+0.68\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{25}=0.85\hat{i}+0.17\hat{j}+0.5\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result255.tex <==
{\tiny 2D-M255:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.76\hat{i}+0.63\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}+0.55\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.64\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result256.tex <==
{\tiny 2D-M256:}

$\hat{n}_{13}=0.01\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.88\hat{i}+0.31\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{24}=-0.8\hat{i}+0.07\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}-0.48\hat{j}-0.32\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.41\hat{i}+1.17\hat{j}+1.95\hat{k}$,\;\;\;$\vec{r}_{23}=6.6\hat{i}+8.7\hat{j}+2.72\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result257.tex <==
{\tiny 2D-M257:}

$\hat{n}_{13}=0.57\hat{i}+0.14\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.64\hat{i}-0.74\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}+0.74\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.61\hat{j}+0.79\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result258.tex <==
{\tiny 2D-M258:}

$\hat{n}_{13}=0.64\hat{i}+0.35\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{14}=0.66\hat{i}-0.05\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.57\hat{j}-0.1\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.76\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result259.tex <==
{\tiny 2D-M259:}

$\hat{n}_{13}=-0.1\hat{i}+0.76\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{14}=-0.93\hat{i}+0.38\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{24}=0.48\hat{i}-0.74\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{35}=0.68\hat{i}+0.44\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result26.tex <==
{\tiny 2D-M26:}

$\hat{n}_{14}=-0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result260.tex <==
{\tiny 2D-M260:}

$\hat{n}_{13}=-0.97\hat{i}+0.07\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{14}=-0.89\hat{i}+0.46\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=0.11\hat{i}+0.76\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{35}=-0.59\hat{i}-0.52\hat{j}+0.62\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result261.tex <==
{\tiny 2D-M261:}

$\hat{n}_{13}=0.0\hat{i}+0.49\hat{j}-0.87\hat{k}$,\;\;\;$\hat{n}_{14}=-0.03\hat{i}+0.4\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.6\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=-0.64\hat{i}+0.54\hat{j}+0.54\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result262.tex <==
{\tiny 2D-M262:}

$\hat{n}_{13}=0.84\hat{i}-0.32\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{14}=0.6\hat{i}-0.43\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{23}=0.79\hat{i}+0.56\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{45}=0.06\hat{i}-0.82\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result263.tex <==
{\tiny 2D-M263:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.73\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.65\hat{j}+0.76\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+8.19\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result264.tex <==
{\tiny 2D-M264:}

$\hat{n}_{13}=-0.33\hat{i}-0.07\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{14}=-0.99\hat{i}-0.15\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=-0.57\hat{i}-0.81\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{35}=0.35\hat{i}+0.65\hat{j}-0.67\hat{k}$,\newline
$\vec{r}_{14}=5.08\hat{i}+4.91\hat{j}+5.17\hat{k}$,\;\;\;$\vec{r}_{23}=4.91\hat{i}+5.3\hat{j}+4.76\hat{k}$,\;\;\;$\vec{r}_{24}=5.32\hat{i}+5.1\hat{j}+5.01\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result265.tex <==
{\tiny 2D-M265:}

$\hat{n}_{13}=0.31\hat{i}+0.52\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.24\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{23}=-0.65\hat{i}-0.39\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=0.26\hat{i}+0.41\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result266.tex <==
{\tiny 2D-M266:}

$\hat{n}_{13}=0.0\hat{i}+0.73\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{14}=0.53\hat{i}-0.66\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{25}=0.76\hat{i}+0.64\hat{j}-0.13\hat{k}$,\;\;\;$\hat{n}_{45}=0.78\hat{i}+0.63\hat{j}-0.01\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result267.tex <==
{\tiny 2D-M267:}

$\hat{n}_{13}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.53\hat{i}+0.6\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.24\hat{i}+0.42\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result268.tex <==
{\tiny 2D-M268:}

$\hat{n}_{13}=-0.03\hat{i}+0.34\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{14}=-0.09\hat{i}-0.97\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{24}=0.91\hat{i}-0.36\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{35}=0.11\hat{i}+0.51\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=4.96\hat{i}+5.0\hat{j}+5.04\hat{k}$,\;\;\;$\vec{r}_{23}=4.9\hat{i}+4.92\hat{j}+5.09\hat{k}$,\;\;\;$\vec{r}_{24}=6.07\hat{i}+5.07\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result269.tex <==
{\tiny 2D-M269:}

$\hat{n}_{13}=-0.58\hat{i}+0.17\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{14}=0.7\hat{i}+0.02\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.31\hat{i}+0.72\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+5.51\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result27.tex <==
{\tiny 2D-M27:}

$\hat{n}_{14}=-0.1\hat{i}-0.04\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{25}=-0.73\hat{i}-0.61\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{45}=-0.27\hat{i}-0.4\hat{j}-0.88\hat{k}$,\;\;\;$\vec{r}_{23}=5.31\hat{i}+4.46\hat{j}+4.41\hat{k}$,\newline
$\vec{r}_{34}=4.99\hat{i}+4.55\hat{j}+5.58\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result270.tex <==
{\tiny 2D-M270:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.02\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.48\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{35}=0.85\hat{i}-0.48\hat{j}+0.22\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result271.tex <==
{\tiny 2D-M271:}

$\hat{n}_{13}=0.0\hat{i}+0.94\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}+0.71\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=0.61\hat{i}+0.64\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{35}=-0.72\hat{i}+0.69\hat{j}+0.02\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result272.tex <==
{\tiny 2D-M272:}

$\hat{n}_{13}=0.27\hat{i}+0.68\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{24}=-0.88\hat{i}+0.48\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=0.12\hat{i}+0.76\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{35}=0.68\hat{i}+0.44\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result273.tex <==
{\tiny 2D-M273:}

$\hat{n}_{13}=0.79\hat{i}-0.46\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{23}=-0.93\hat{i}-0.37\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{25}=-0.59\hat{i}+0.55\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{45}=-0.59\hat{i}+0.2\hat{j}-0.78\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result274.tex <==
{\tiny 2D-M274:}

$\hat{n}_{13}=-0.0\hat{i}+0.95\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{23}=-0.06\hat{i}+0.26\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.31\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{45}=-0.64\hat{i}+0.43\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result275.tex <==
{\tiny 2D-M275:}

$\hat{n}_{13}=-0.77\hat{i}-0.46\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{23}=0.78\hat{i}-0.61\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{24}=-0.43\hat{i}-0.13\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{45}=-0.7\hat{i}+0.1\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result276.tex <==
{\tiny 2D-M276:}

$\hat{n}_{13}=0.28\hat{i}+0.29\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{23}=0.67\hat{i}+0.73\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{24}=-0.52\hat{i}-0.26\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{35}=-0.33\hat{i}-0.35\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=4.74\hat{i}+4.95\hat{j}+5.1\hat{k}$,\;\;\;$\vec{r}_{23}=6.26\hat{i}+5.85\hat{j}+6.44\hat{k}$,\;\;\;$\vec{r}_{24}=4.75\hat{i}+4.71\hat{j}+5.03\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result277.tex <==
{\tiny 2D-M277:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.5\hat{j}+0.86\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result278.tex <==
{\tiny 2D-M278:}

$\hat{n}_{13}=-0.0\hat{i}+0.6\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=0.52\hat{i}-0.72\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.47\hat{i}+0.63\hat{j}-0.63\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result279.tex <==
{\tiny 2D-M279:}

$\hat{n}_{13}=-0.97\hat{i}-0.25\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.64\hat{i}+0.57\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{45}=0.73\hat{i}-0.14\hat{j}+0.67\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result28.tex <==
{\tiny 2D-M28:}

$\hat{n}_{14}=-0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result280.tex <==
{\tiny 2D-M280:}

$\hat{n}_{13}=0.72\hat{i}+0.46\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.57\hat{i}-0.76\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{24}=-0.19\hat{i}-0.67\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{35}=0.65\hat{i}-0.72\hat{j}-0.23\hat{k}$,\newline
$\vec{r}_{14}=6.07\hat{i}+5.03\hat{j}+3.9\hat{k}$,\;\;\;$\vec{r}_{23}=6.94\hat{i}+7.02\hat{j}+2.92\hat{k}$,\;\;\;$\vec{r}_{24}=2.83\hat{i}+3.65\hat{j}+7.09\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result281.tex <==
{\tiny 2D-M281:}

$\hat{n}_{13}=-0.58\hat{i}-0.36\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.9\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{24}=-0.8\hat{i}+0.0\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+6.03\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result282.tex <==
{\tiny 2D-M282:}

$\hat{n}_{13}=0.82\hat{i}+0.52\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{24}=-0.69\hat{i}-0.22\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}+0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{35}=-0.57\hat{i}+0.65\hat{j}-0.51\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result283.tex <==
{\tiny 2D-M283:}

$\hat{n}_{13}=0.2\hat{i}+0.9\hat{j}-0.38\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.38\hat{j}-0.92\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.89\hat{j}+0.46\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result284.tex <==
{\tiny 2D-M284:}

$\hat{n}_{13}=-0.79\hat{i}-0.19\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.5\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.8\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{35}=-0.75\hat{i}-0.19\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result285.tex <==
{\tiny 2D-M285:}

$\hat{n}_{13}=0.0\hat{i}+0.82\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}-0.21\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.66\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{45}=0.97\hat{i}-0.24\hat{j}-0.07\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result286.tex <==
{\tiny 2D-M286:}

$\hat{n}_{13}=-0.43\hat{i}+0.84\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}-0.57\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.77\hat{i}+0.45\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result287.tex <==
{\tiny 2D-M287:}

$\hat{n}_{13}=-0.79\hat{i}+0.51\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{23}=0.08\hat{i}+0.56\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{24}=-0.65\hat{i}+0.37\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result288.tex <==
{\tiny 2D-M288:}

$\hat{n}_{13}=-0.53\hat{i}-0.53\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}-0.62\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.18\hat{i}+0.9\hat{j}-0.4\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.29\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result289.tex <==
{\tiny 2D-M289:}

$\hat{n}_{13}=0.0\hat{i}+0.27\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=-0.53\hat{i}+0.18\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.42\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result29.tex <==
{\tiny 2D-M29:}

$\hat{n}_{14}=0.52\hat{i}-0.5\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{34}=-0.13\hat{i}-0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{45}=-0.25\hat{i}+0.91\hat{j}-0.35\hat{k}$,\;\;\;$\vec{r}_{23}=3.3\hat{i}+3.38\hat{j}+6.5\hat{k}$,\newline
$\vec{r}_{25}=4.87\hat{i}+6.69\hat{j}+6.68\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result290.tex <==
{\tiny 2D-M290:}

$\hat{n}_{13}=0.22\hat{i}+0.8\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{23}=0.51\hat{i}+0.62\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{24}=-0.54\hat{i}+0.58\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.23\hat{i}-0.69\hat{j}-0.69\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result291.tex <==
{\tiny 2D-M291:}

$\hat{n}_{13}=0.36\hat{i}+0.81\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{23}=0.73\hat{i}+0.06\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.24\hat{i}-0.74\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result292.tex <==
{\tiny 2D-M292:}

$\hat{n}_{13}=-0.37\hat{i}-0.55\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{23}=-0.72\hat{i}+0.69\hat{j}-0.07\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}-0.6\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{25}=-0.81\hat{i}-0.57\hat{j}+0.15\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result293.tex <==
{\tiny 2D-M293:}

$\hat{n}_{13}=0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.67\hat{i}+0.05\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{45}=0.41\hat{i}-0.82\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result294.tex <==
{\tiny 2D-M294:}

$\hat{n}_{13}=-0.37\hat{i}+0.44\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.71\hat{i}-0.11\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result295.tex <==
{\tiny 2D-M295:}

$\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.25\hat{i}-0.67\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result296.tex <==
{\tiny 2D-M296:}

$\hat{n}_{13}=0.7\hat{i}-0.01\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.35\hat{i}+0.66\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{25}=-0.61\hat{i}+0.09\hat{j}-0.79\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result297.tex <==
{\tiny 2D-M297:}

$\hat{n}_{14}=-0.0\hat{i}+0.62\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.3\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.92\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}+0.23\hat{j}+0.67\hat{k}$,\newline
$\hat{n}_{35}=-0.73\hat{i}+0.34\hat{j}+0.59\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result298.tex <==
{\tiny 2D-M298:}

$\hat{n}_{14}=-0.47\hat{i}-0.21\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.09\hat{i}-0.59\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=0.78\hat{i}+0.14\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{34}=0.79\hat{i}+0.46\hat{j}-0.39\hat{k}$,\newline
$\hat{n}_{35}=-0.59\hat{i}+0.63\hat{j}-0.51\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result299.tex <==
{\tiny 2D-M299:}

$\hat{n}_{14}=0.57\hat{i}+0.67\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.56\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.23\hat{i}+0.94\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{34}=0.42\hat{i}-0.8\hat{j}-0.42\hat{k}$,\newline
$\hat{n}_{45}=-0.71\hat{i}-0.0\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=5.33\hat{i}+2.14\hat{j}+5.86\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result3.tex <==
{\tiny 2D-M3:}

$\hat{n}_{14}=-0.56\hat{i}+0.74\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.69\hat{i}-0.01\hat{j}+0.73\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result30.tex <==
{\tiny 2D-M30:}

$\hat{n}_{13}=0.81\hat{i}-0.38\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result300.tex <==
{\tiny 2D-M300:}

$\hat{n}_{14}=0.77\hat{i}+0.04\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.56\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.42\hat{i}+0.8\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{34}=-0.23\hat{i}-0.94\hat{j}-0.23\hat{k}$,\newline
$\hat{n}_{45}=0.71\hat{i}+0.0\hat{j}-0.71\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=4.56\hat{i}+5.47\hat{j}+4.32\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result301.tex <==
{\tiny 2D-M301:}

$\hat{n}_{14}=0.13\hat{i}-0.65\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{23}=0.98\hat{i}-0.18\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.19\hat{i}-0.78\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.04\hat{i}-0.59\hat{j}+0.8\hat{k}$,\newline
$\hat{n}_{45}=0.55\hat{i}-0.24\hat{j}+0.8\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.39\hat{i}+4.79\hat{j}+5.38\hat{k}$,\;\;\;$\vec{r}_{25}=4.53\hat{i}+5.13\hat{j}+7.95\hat{k}$,\newline
$\vec{r}_{34}=5.37\hat{i}+4.62\hat{j}+5.27\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result302.tex <==
{\tiny 2D-M302:}

$\hat{n}_{14}=-0.6\hat{i}-0.79\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{15}=-0.59\hat{i}-0.79\hat{j}-0.16\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}-0.43\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.64\hat{i}-0.58\hat{j}+0.5\hat{k}$,\newline
$\hat{n}_{34}=0.45\hat{i}-0.17\hat{j}-0.88\hat{k}$,\;\;\;$\vec{r}_{14}=6.47\hat{i}+3.62\hat{j}+4.11\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result303.tex <==
{\tiny 2D-M303:}

$\hat{n}_{14}=-0.05\hat{i}-0.76\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{15}=-0.8\hat{i}-0.35\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}-0.91\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{25}=0.78\hat{i}+0.38\hat{j}+0.5\hat{k}$,\newline
$\hat{n}_{34}=-0.5\hat{i}-0.12\hat{j}+0.86\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=4.09\hat{i}+6.24\hat{j}+6.18\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result304.tex <==
{\tiny 2D-M304:}

$\hat{n}_{14}=-0.11\hat{i}+0.76\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{15}=0.11\hat{i}-0.76\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{23}=-0.89\hat{i}+0.22\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=0.49\hat{i}+0.6\hat{j}+0.63\hat{k}$,\newline
$\hat{n}_{34}=0.56\hat{i}-0.49\hat{j}-0.67\hat{k}$,\;\;\;$\vec{r}_{14}=4.93\hat{i}+5.16\hat{j}+4.85\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result305.tex <==
{\tiny 2D-M305:}

$\hat{n}_{14}=-0.9\hat{i}-0.42\hat{j}-0.11\hat{k}$,\;\;\;$\hat{n}_{15}=0.34\hat{i}-0.6\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=0.63\hat{i}+0.73\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{25}=-0.36\hat{i}+0.57\hat{j}+0.74\hat{k}$,\newline
$\hat{n}_{34}=-0.27\hat{i}+0.69\hat{j}-0.67\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=4.72\hat{i}+4.85\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result306.tex <==
{\tiny 2D-M306:}

$\hat{n}_{14}=-0.8\hat{i}-0.47\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{15}=0.05\hat{i}-0.66\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}-0.59\hat{j}-0.57\hat{k}$,\newline
$\hat{n}_{34}=0.95\hat{i}-0.24\hat{j}-0.22\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result307.tex <==
{\tiny 2D-M307:}

$\hat{n}_{14}=0.49\hat{i}+0.66\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{15}=-0.04\hat{i}-0.63\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.89\hat{i}-0.36\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}-0.66\hat{j}+0.51\hat{k}$,\newline
$\hat{n}_{34}=-0.0\hat{i}+0.63\hat{j}+0.77\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result308.tex <==
{\tiny 2D-M308:}

$\hat{n}_{13}=-0.7\hat{i}-0.05\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{14}=-0.56\hat{i}-0.56\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{24}=-0.29\hat{i}-0.9\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.61\hat{i}+0.49\hat{j}+0.63\hat{k}$,\newline
$\hat{n}_{35}=0.73\hat{i}+0.02\hat{j}+0.68\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result309.tex <==
{\tiny 2D-M309:}

$\hat{n}_{13}=0.02\hat{i}-0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.8\hat{i}+0.4\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{24}=-0.94\hat{i}+0.25\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}-0.61\hat{j}-0.56\hat{k}$,\newline
$\hat{n}_{35}=-0.05\hat{i}-0.69\hat{j}+0.72\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result31.tex <==
{\tiny 2D-M31:}

$\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.01\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result310.tex <==
{\tiny 2D-M310:}

$\hat{n}_{13}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.57\hat{i}-0.82\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.83\hat{i}+0.06\hat{j}-0.56\hat{k}$,\newline
$\hat{n}_{35}=-0.8\hat{i}+0.61\hat{j}-0.01\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+2.36\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+2.5\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result311.tex <==
{\tiny 2D-M311:}

$\hat{n}_{13}=0.71\hat{i}-0.09\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{14}=-0.48\hat{i}-0.86\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{24}=-0.91\hat{i}-0.42\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{25}=0.47\hat{i}-0.89\hat{j}-0.02\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.44\hat{i}+1.75\hat{j}+1.53\hat{k}$,\;\;\;$\vec{r}_{24}=3.06\hat{i}+6.64\hat{j}+4.6\hat{k}$,\newline
$\vec{r}_{25}=4.99\hat{i}+1.52\hat{j}+1.51\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+7.73\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result312.tex <==
{\tiny 2D-M312:}

$\hat{n}_{13}=-0.54\hat{i}+0.76\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{14}=0.44\hat{i}+0.54\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{23}=0.14\hat{i}+0.63\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{25}=-0.34\hat{i}-0.72\hat{j}+0.61\hat{k}$,\newline
$\hat{n}_{45}=-0.88\hat{i}+0.47\hat{j}+0.12\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result313.tex <==
{\tiny 2D-M313:}

$\hat{n}_{13}=-0.79\hat{i}+0.17\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{14}=-0.42\hat{i}+0.66\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{23}=-0.32\hat{i}+0.5\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=0.84\hat{i}-0.0\hat{j}-0.54\hat{k}$,\newline
$\hat{n}_{45}=0.73\hat{i}+0.68\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result314.tex <==
{\tiny 2D-M314:}

$\hat{n}_{13}=0.9\hat{i}-0.42\hat{j}+0.06\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.83\hat{i}-0.54\hat{j}+0.11\hat{k}$,\;\;\;$\hat{n}_{25}=0.51\hat{i}-0.85\hat{j}+0.09\hat{k}$,\newline
$\hat{n}_{45}=-0.0\hat{i}+0.34\hat{j}+0.94\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+2.38\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result315.tex <==
{\tiny 2D-M315:}

$\hat{n}_{13}=0.0\hat{i}+0.61\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{14}=-0.41\hat{i}-0.02\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}-0.67\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=-0.92\hat{i}-0.37\hat{j}-0.1\hat{k}$,\newline
$\hat{n}_{35}=0.0\hat{i}+0.83\hat{j}-0.56\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.86\hat{i}+5.62\hat{j}+6.15\hat{k}$,\;\;\;$\vec{r}_{23}=5.03\hat{i}+4.98\hat{j}+5.21\hat{k}$,\newline
$\vec{r}_{24}=5.31\hat{i}+5.28\hat{j}+4.75\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result316.tex <==
{\tiny 2D-M316:}

$\hat{n}_{13}=-0.83\hat{i}-0.08\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{14}=-0.31\hat{i}+0.77\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{23}=0.93\hat{i}+0.36\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{24}=0.28\hat{i}-0.5\hat{j}+0.82\hat{k}$,\newline
$\hat{n}_{25}=-0.51\hat{i}+0.74\hat{j}-0.43\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result317.tex <==
{\tiny 2D-M317:}

$\hat{n}_{13}=-0.6\hat{i}+0.68\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{14}=0.18\hat{i}+0.62\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=0.41\hat{i}+0.5\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{25}=0.91\hat{i}-0.38\hat{j}+0.17\hat{k}$,\newline
$\hat{n}_{35}=-0.74\hat{i}-0.37\hat{j}-0.56\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result318.tex <==
{\tiny 2D-M318:}

$\hat{n}_{13}=0.84\hat{i}-0.16\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{14}=0.55\hat{i}+0.26\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.94\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.93\hat{j}-0.36\hat{k}$,\newline
$\hat{n}_{35}=0.78\hat{i}+0.04\hat{j}-0.62\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result319.tex <==
{\tiny 2D-M319:}

$\hat{n}_{13}=0.85\hat{i}+0.13\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{14}=0.51\hat{i}-0.51\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=0.13\hat{i}+0.87\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{25}=-0.3\hat{i}-0.53\hat{j}-0.79\hat{k}$,\newline
$\hat{n}_{35}=-0.88\hat{i}-0.4\hat{j}+0.26\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result32.tex <==
{\tiny 2D-M32:}

$\hat{n}_{13}=0.09\hat{i}-0.77\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{14}=0.21\hat{i}-0.82\hat{j}+0.53\hat{k}$,\;\;\;$\hat{n}_{45}=-0.82\hat{i}-0.45\hat{j}-0.36\hat{k}$,\;\;\;$\vec{r}_{13}=6.51\hat{i}+3.35\hat{j}+4.18\hat{k}$,\newline
$\vec{r}_{23}=4.5\hat{i}+6.92\hat{j}+6.91\hat{k}$,\;\;\;$\vec{r}_{24}=4.66\hat{i}+4.14\hat{j}+6.71\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result320.tex <==
{\tiny 2D-M320:}

$\hat{n}_{14}=-0.2\hat{i}+0.68\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.35\hat{i}+0.47\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.16\hat{i}+0.61\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result321.tex <==
{\tiny 2D-M321:}

$\hat{n}_{14}=0.63\hat{i}+0.7\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{24}=0.78\hat{i}+0.6\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.37\hat{i}+0.45\hat{j}-0.82\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result322.tex <==
{\tiny 2D-M322:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.22\hat{i}+0.64\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{34}=0.52\hat{i}-0.51\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result323.tex <==
{\tiny 2D-M323:}

$\hat{n}_{14}=0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.72\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.78\hat{i}-0.61\hat{j}-0.14\hat{k}$,\;\;\;$\hat{n}_{35}=-0.37\hat{i}+0.74\hat{j}-0.56\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result324.tex <==
{\tiny 2D-M324:}

$\hat{n}_{14}=-0.17\hat{i}-0.47\hat{j}-0.87\hat{k}$,\;\;\;$\hat{n}_{24}=0.31\hat{i}+0.57\hat{j}+0.76\hat{k}$,\;\;\;$\hat{n}_{34}=0.95\hat{i}-0.17\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result325.tex <==
{\tiny 2D-M325:}

$\hat{n}_{14}=0.0\hat{i}+0.63\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{24}=-0.16\hat{i}-0.89\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.42\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result326.tex <==
{\tiny 2D-M326:}

$\hat{n}_{14}=-0.04\hat{i}+0.56\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result327.tex <==
{\tiny 2D-M327:}

$\hat{n}_{14}=-0.0\hat{i}+0.47\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{23}=0.29\hat{i}+0.47\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.61\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.66\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result328.tex <==
{\tiny 2D-M328:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}-0.33\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.73\hat{j}+0.68\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+4.15\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result329.tex <==
{\tiny 2D-M329:}

$\hat{n}_{14}=-0.45\hat{i}-0.89\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.55\hat{i}+0.8\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result33.tex <==
{\tiny 2D-M33:}

$\hat{n}_{13}=-0.7\hat{i}+0.01\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.54\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result330.tex <==
{\tiny 2D-M330:}

$\hat{n}_{14}=0.37\hat{i}-0.39\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.67\hat{i}+0.67\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{45}=-0.34\hat{i}+0.34\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result331.tex <==
{\tiny 2D-M331:}

$\hat{n}_{14}=0.9\hat{i}+0.25\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result332.tex <==
{\tiny 2D-M332:}

$\hat{n}_{14}=-0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{23}=-0.78\hat{i}-0.14\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.87\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.52\hat{j}-0.63\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result333.tex <==
{\tiny 2D-M333:}

$\hat{n}_{14}=-0.79\hat{i}+0.28\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{23}=-0.95\hat{i}+0.21\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result334.tex <==
{\tiny 2D-M334:}

$\hat{n}_{14}=0.36\hat{i}+0.32\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}+0.8\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result335.tex <==
{\tiny 2D-M335:}

$\hat{n}_{14}=-0.79\hat{i}+0.29\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}-0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result336.tex <==
{\tiny 2D-M336:}

$\hat{n}_{14}=-0.81\hat{i}+0.38\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.01\hat{i}+0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result337.tex <==
{\tiny 2D-M337:}

$\hat{n}_{14}=-0.68\hat{i}-0.53\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{25}=0.57\hat{i}+0.23\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result338.tex <==
{\tiny 2D-M338:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{15}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result339.tex <==
{\tiny 2D-M339:}

$\hat{n}_{14}=0.81\hat{i}-0.29\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.81\hat{i}+0.29\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result34.tex <==
{\tiny 2D-M34:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.04\hat{i}-0.73\hat{j}+0.68\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result340.tex <==
{\tiny 2D-M340:}

$\hat{n}_{14}=-0.0\hat{i}+0.48\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{15}=-0.74\hat{i}+0.67\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.63\hat{i}-0.78\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result341.tex <==
{\tiny 2D-M341:}

$\hat{n}_{14}=0.12\hat{i}+0.81\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{14}=5.93\hat{i}+3.77\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result342.tex <==
{\tiny 2D-M342:}

$\hat{n}_{14}=0.91\hat{i}+0.32\hat{j}-0.28\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}-0.43\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.66\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.61\hat{j}+0.54\hat{k}$,\newline
$\vec{r}_{14}=4.11\hat{i}+7.58\hat{j}+7.9\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result343.tex <==
{\tiny 2D-M343:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.85\hat{i}-0.47\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{25}=0.49\hat{i}+0.87\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=0.42\hat{i}+5.85\hat{j}+6.72\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result344.tex <==
{\tiny 2D-M344:}

$\hat{n}_{14}=-0.1\hat{i}+0.5\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.64\hat{i}-0.33\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.97\hat{j}-0.22\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.14\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result345.tex <==
{\tiny 2D-M345:}

$\hat{n}_{14}=0.0\hat{i}+0.03\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.25\hat{i}+0.47\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.64\hat{i}+0.13\hat{j}+0.76\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result346.tex <==
{\tiny 2D-M346:}

$\hat{n}_{14}=0.1\hat{i}-0.09\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.89\hat{i}+0.44\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+5.28\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result347.tex <==
{\tiny 2D-M347:}

$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.31\hat{i}+0.36\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{25}=0.81\hat{i}-0.47\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result348.tex <==
{\tiny 2D-M348:}

$\hat{n}_{14}=0.32\hat{i}-0.67\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}+0.42\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.02\hat{i}+0.7\hat{j}-0.72\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result349.tex <==
{\tiny 2D-M349:}

$\hat{n}_{14}=0.52\hat{i}+0.01\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{24}=-0.71\hat{i}+0.06\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.25\hat{i}-0.67\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{35}=-0.03\hat{i}+0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result35.tex <==
{\tiny 2D-M35:}

$\hat{n}_{13}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.08\hat{i}+0.62\hat{j}-0.78\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result350.tex <==
{\tiny 2D-M350:}

$\hat{n}_{14}=0.25\hat{i}+0.21\hat{j}+0.94\hat{k}$,\;\;\;$\hat{n}_{24}=0.59\hat{i}+0.57\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.37\hat{i}-0.31\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{34}=-0.78\hat{i}+0.6\hat{j}+0.19\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result351.tex <==
{\tiny 2D-M351:}

$\hat{n}_{14}=-0.12\hat{i}+0.83\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.6\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{35}=-0.04\hat{i}+0.66\hat{j}-0.75\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result352.tex <==
{\tiny 2D-M352:}

$\hat{n}_{14}=0.01\hat{i}+0.02\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.7\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{35}=0.4\hat{i}+0.41\hat{j}+0.82\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result353.tex <==
{\tiny 2D-M353:}

$\hat{n}_{14}=-0.45\hat{i}+0.89\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=-0.62\hat{i}+0.44\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{34}=0.27\hat{i}+0.77\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.71\hat{i}-0.14\hat{j}-0.69\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result354.tex <==
{\tiny 2D-M354:}

$\hat{n}_{14}=0.02\hat{i}+0.98\hat{j}+0.19\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{25}=-0.78\hat{i}+0.27\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}+0.49\hat{j}+0.65\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result355.tex <==
{\tiny 2D-M355:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+9.99\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result356.tex <==
{\tiny 2D-M356:}

$\hat{n}_{14}=0.68\hat{i}-0.52\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.37\hat{i}-0.92\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.6\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{34}=0.69\hat{i}+0.02\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result357.tex <==
{\tiny 2D-M357:}

$\hat{n}_{14}=-0.04\hat{i}+0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.62\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.89\hat{i}+0.1\hat{j}-0.44\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result358.tex <==
{\tiny 2D-M358:}

$\hat{n}_{14}=0.25\hat{i}+0.09\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.49\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{25}=-0.79\hat{i}-0.58\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{34}=0.57\hat{i}-0.56\hat{j}+0.6\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result359.tex <==
{\tiny 2D-M359:}

$\hat{n}_{14}=0.37\hat{i}-0.62\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}+0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.55\hat{i}+0.63\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=-0.45\hat{i}-0.77\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result36.tex <==
{\tiny 2D-M36:}

$\hat{n}_{14}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+1.0\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result360.tex <==
{\tiny 2D-M360:}

$\hat{n}_{14}=0.0\hat{i}+0.28\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}-0.55\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.78\hat{i}-0.6\hat{j}+0.18\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result361.tex <==
{\tiny 2D-M361:}

$\hat{n}_{14}=-0.65\hat{i}+0.76\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}+0.66\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{34}=0.88\hat{i}+0.27\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result362.tex <==
{\tiny 2D-M362:}

$\hat{n}_{14}=-0.01\hat{i}+0.17\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.74\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.93\hat{i}-0.37\hat{j}+0.05\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+9.3\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result363.tex <==
{\tiny 2D-M363:}

$\hat{n}_{14}=0.01\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.93\hat{i}-0.25\hat{j}-0.25\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result364.tex <==
{\tiny 2D-M364:}

$\hat{n}_{14}=-0.5\hat{i}-0.58\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+5.83\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result365.tex <==
{\tiny 2D-M365:}

$\hat{n}_{14}=0.26\hat{i}+0.45\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}-0.78\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.13\hat{i}-0.95\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{45}=-0.44\hat{i}-0.24\hat{j}+0.87\hat{k}$,\newline
$\vec{r}_{25}=6.53\hat{i}+5.84\hat{j}+4.67\hat{k}$,\;\;\;$\vec{r}_{34}=5.22\hat{i}+3.7\hat{j}+6.69\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result366.tex <==
{\tiny 2D-M366:}

$\hat{n}_{14}=-0.31\hat{i}+0.95\hat{j}-0.06\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.63\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.96\hat{j}+0.29\hat{k}$,\;\;\;$\hat{n}_{45}=-0.85\hat{i}-0.1\hat{j}+0.52\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result367.tex <==
{\tiny 2D-M367:}

$\hat{n}_{14}=-0.1\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.95\hat{i}+0.21\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{45}=-0.24\hat{i}-0.42\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result368.tex <==
{\tiny 2D-M368:}

$\hat{n}_{14}=-0.5\hat{i}+0.75\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}-0.19\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.59\hat{i}-0.68\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{34}=-0.59\hat{i}-0.56\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result369.tex <==
{\tiny 2D-M369:}

$\hat{n}_{14}=0.04\hat{i}+0.72\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{23}=-0.9\hat{i}-0.31\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.44\hat{i}+0.64\hat{j}-0.64\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result37.tex <==
{\tiny 2D-M37:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result370.tex <==
{\tiny 2D-M370:}

$\hat{n}_{14}=-0.25\hat{i}+0.84\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=-0.79\hat{i}-0.56\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.56\hat{j}-0.13\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result371.tex <==
{\tiny 2D-M371:}

$\hat{n}_{14}=-0.41\hat{i}+0.2\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.74\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=-0.02\hat{i}-0.11\hat{j}+0.99\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{23}=3.16\hat{i}+2.97\hat{j}+6.41\hat{k}$,\;\;\;$\vec{r}_{34}=3.07\hat{i}+6.34\hat{j}+6.83\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+4.66\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result372.tex <==
{\tiny 2D-M372:}

$\hat{n}_{14}=-0.72\hat{i}-0.7\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{23}=0.55\hat{i}-0.55\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{34}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.45\hat{i}-0.45\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result373.tex <==
{\tiny 2D-M373:}

$\hat{n}_{14}=0.62\hat{i}+0.59\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=-0.13\hat{i}-0.8\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.02\hat{i}-0.94\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{45}=0.51\hat{i}-0.74\hat{j}-0.43\hat{k}$,\newline
$\vec{r}_{23}=3.72\hat{i}+3.44\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{25}=6.54\hat{i}+6.37\hat{j}+3.86\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result374.tex <==
{\tiny 2D-M374:}

$\hat{n}_{14}=0.06\hat{i}+0.93\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{25}=-0.63\hat{i}+0.76\hat{j}+0.13\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.52\hat{i}+0.29\hat{j}+0.81\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result375.tex <==
{\tiny 2D-M375:}

$\hat{n}_{14}=-0.74\hat{i}-0.3\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.55\hat{i}-0.55\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{45}=-0.45\hat{i}-0.45\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result376.tex <==
{\tiny 2D-M376:}

$\hat{n}_{14}=0.08\hat{i}+0.11\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{25}=0.57\hat{i}-0.48\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.83\hat{j}+0.55\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.01\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result377.tex <==
{\tiny 2D-M377:}

$\hat{n}_{14}=0.14\hat{i}-0.01\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{25}=-1.0\hat{i}+0.03\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{34}=0.56\hat{i}-0.83\hat{j}-0.06\hat{k}$,\;\;\;$\hat{n}_{45}=0.14\hat{i}-0.52\hat{j}+0.84\hat{k}$,\newline
$\vec{r}_{23}=3.17\hat{i}+3.41\hat{j}+4.4\hat{k}$,\;\;\;$\vec{r}_{34}=7.03\hat{i}+7.38\hat{j}+5.37\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result378.tex <==
{\tiny 2D-M378:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.43\hat{i}+0.46\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{34}=-0.62\hat{i}+0.48\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{45}=-0.11\hat{i}-0.92\hat{j}-0.37\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result379.tex <==
{\tiny 2D-M379:}

$\hat{n}_{14}=-0.75\hat{i}-0.41\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{25}=0.13\hat{i}-0.82\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{34}=-0.29\hat{i}-0.73\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.65\hat{i}-0.72\hat{j}+0.23\hat{k}$,\newline
$\vec{r}_{23}=6.7\hat{i}+6.71\hat{j}+3.56\hat{k}$,\;\;\;$\vec{r}_{25}=3.87\hat{i}+6.71\hat{j}+6.83\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result38.tex <==
{\tiny 2D-M38:}

$\hat{n}_{14}=0.39\hat{i}-0.82\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result380.tex <==
{\tiny 2D-M380:}

$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{15}=-0.0\hat{i}+0.57\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=-0.39\hat{i}-0.43\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{25}=-0.64\hat{i}-0.7\hat{j}-0.31\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result381.tex <==
{\tiny 2D-M381:}

$\hat{n}_{14}=-0.61\hat{i}-0.61\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{15}=-0.18\hat{i}+0.76\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.14\hat{i}+0.55\hat{j}+0.82\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+9.59\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result382.tex <==
{\tiny 2D-M382:}

$\hat{n}_{14}=-0.41\hat{i}-0.41\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{15}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.56\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result383.tex <==
{\tiny 2D-M383:}

$\hat{n}_{14}=0.53\hat{i}-0.85\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{15}=-0.68\hat{i}+0.51\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.53\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result384.tex <==
{\tiny 2D-M384:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result385.tex <==
{\tiny 2D-M385:}

$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{15}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.41\hat{i}+0.41\hat{j}+0.82\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.26\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result386.tex <==
{\tiny 2D-M386:}

$\hat{n}_{14}=-0.62\hat{i}-0.77\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{23}=0.73\hat{i}+0.62\hat{j}-0.28\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{34}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.72\hat{i}+3.59\hat{j}+6.36\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result387.tex <==
{\tiny 2D-M387:}

$\hat{n}_{14}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.08\hat{i}+0.62\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.96\hat{i}+4.18\hat{j}+6.17\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result388.tex <==
{\tiny 2D-M388:}

$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.12\hat{i}-0.81\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=3.34\hat{i}+2.57\hat{j}+6.67\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result389.tex <==
{\tiny 2D-M389:}

$\hat{n}_{14}=-0.82\hat{i}+0.43\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.61\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.67\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{34}=-0.82\hat{i}+0.43\hat{j}-0.38\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=3.03\hat{i}+6.87\hat{j}+5.52\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result39.tex <==
{\tiny 2D-M39:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result390.tex <==
{\tiny 2D-M390:}

$\hat{n}_{14}=-0.82\hat{i}-0.38\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=-0.69\hat{i}-0.48\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}+0.54\hat{j}-0.61\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=3.66\hat{i}+6.37\hat{j}+4.46\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result391.tex <==
{\tiny 2D-M391:}

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.94\hat{i}-0.28\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.88\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{34}=0.12\hat{i}-0.78\hat{j}-0.61\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=1.2\hat{i}+1.39\hat{j}+9.93\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result392.tex <==
{\tiny 2D-M392:}

$\hat{n}_{14}=-0.76\hat{i}-0.65\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{23}=-0.37\hat{i}+0.39\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.59\hat{i}-0.7\hat{j}+0.39\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.57\hat{i}+7.23\hat{j}+6.35\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result393.tex <==
{\tiny 2D-M393:}

$\hat{n}_{14}=0.76\hat{i}+0.65\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.37\hat{i}-0.39\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{34}=0.59\hat{i}-0.7\hat{j}+0.39\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=6.29\hat{i}+5.68\hat{j}+2.58\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result394.tex <==
{\tiny 2D-M394:}

$\hat{n}_{14}=-0.34\hat{i}+0.88\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{23}=-0.93\hat{i}-0.35\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.66\hat{i}+0.03\hat{j}-0.75\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=4.97\hat{i}+5.13\hat{j}+4.93\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result395.tex <==
{\tiny 2D-M395:}

$\hat{n}_{15}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.07\hat{i}+0.74\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{25}=-0.07\hat{i}+0.74\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result396.tex <==
{\tiny 2D-M396:}

$\hat{n}_{15}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.56\hat{i}+0.23\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.56\hat{i}+0.23\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result397.tex <==
{\tiny 2D-M397:}

$\hat{n}_{15}=0.0\hat{i}+0.28\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.19\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{25}=-0.74\hat{i}+0.65\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{34}=-0.5\hat{i}+0.31\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result398.tex <==
{\tiny 2D-M398:}

$\hat{n}_{13}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}-0.69\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.79\hat{i}+0.59\hat{j}+0.18\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result399.tex <==
{\tiny 2D-M399:}

$\hat{n}_{13}=-0.72\hat{i}+0.59\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.85\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{24}=-0.55\hat{i}-0.51\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{35}=0.08\hat{i}-0.79\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result4.tex <==
{\tiny 2D-M4:}

$\hat{n}_{13}=-0.59\hat{i}+0.81\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.04\hat{i}-0.74\hat{j}-0.67\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result40.tex <==
{\tiny 2D-M40:}

$\hat{n}_{13}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.22\hat{i}+0.97\hat{j}-0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result400.tex <==
{\tiny 2D-M400:}

$\hat{n}_{13}=0.42\hat{i}-0.4\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}+0.76\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.59\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result401.tex <==
2D-M401:

$\hat{n}_{13}=-0.73\hat{i}-0.62\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result402.tex <==
2D-M402:

$\hat{n}_{13}=0.0\hat{i}+0.48\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.72\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{35}=0.17\hat{i}-0.47\hat{j}+0.87\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result403.tex <==
2D-M403:

$\hat{n}_{13}=-0.0\hat{i}+0.82\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.72\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=0.95\hat{i}-0.25\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.73\hat{j}+0.68\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result404.tex <==
2D-M404:

$\hat{n}_{13}=-0.11\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{14}=0.56\hat{i}+0.64\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.54\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.81\hat{i}+0.39\hat{j}-0.44\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result405.tex <==
2D-M405:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.48\hat{i}+0.53\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.52\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.8\hat{j}+0.6\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+6.19\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result406.tex <==
2D-M406:

$\hat{n}_{13}=0.67\hat{i}-0.34\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{14}=-0.27\hat{i}-0.83\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{23}=-0.38\hat{i}+0.86\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result407.tex <==
2D-M407:

$\hat{n}_{13}=0.67\hat{i}+0.67\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{14}=0.8\hat{i}+0.6\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.91\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result408.tex <==
2D-M408:

$\hat{n}_{13}=0.69\hat{i}-0.21\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{14}=-0.59\hat{i}-0.71\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.47\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{45}=0.33\hat{i}+0.21\hat{j}+0.92\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result409.tex <==
2D-M409:

$\hat{n}_{13}=-0.8\hat{i}-0.57\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{14}=0.17\hat{i}-0.72\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{23}=0.04\hat{i}-0.93\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{35}=-0.46\hat{i}+0.71\hat{j}+0.53\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=6.94\hat{i}+4.88\hat{j}+3.97\hat{k}$,\;\;\;$\vec{r}_{24}=2.96\hat{i}+7.08\hat{j}+6.42\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result41.tex <==
{\tiny 2D-M41:}

$\hat{n}_{14}=0.81\hat{i}-0.55\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.51\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{25}=-0.32\hat{i}+0.65\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{34}=0.36\hat{i}-0.31\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result410.tex <==
2D-M410:

$\hat{n}_{13}=-0.83\hat{i}-0.55\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{14}=0.53\hat{i}-0.48\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.17\hat{i}-0.62\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{25}=0.69\hat{i}-0.72\hat{j}-0.07\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result411.tex <==
2D-M411:

$\hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{14}=0.36\hat{i}+0.72\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.69\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{45}=0.93\hat{i}-0.26\hat{j}-0.24\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result412.tex <==
2D-M412:

$\hat{n}_{13}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.77\hat{i}-0.48\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.81\hat{i}-0.31\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{45}=-0.11\hat{i}+0.76\hat{j}-0.65\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result413.tex <==
2D-M413:

$\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.7\hat{i}+0.7\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{24}=0.16\hat{i}+0.16\hat{j}-0.97\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result414.tex <==
2D-M414:

$\hat{n}_{13}=-0.16\hat{i}+0.51\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{14}=-0.22\hat{i}-0.97\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{24}=-0.74\hat{i}-0.67\hat{j}-0.06\hat{k}$,\;\;\;$\hat{n}_{35}=-0.16\hat{i}+0.1\hat{j}+0.98\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.3\hat{i}+3.55\hat{j}+5.79\hat{k}$,\;\;\;$\vec{r}_{24}=7.0\hat{i}+7.51\hat{j}+6.9\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result415.tex <==
2D-M415:

$\hat{n}_{13}=-0.35\hat{i}-0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.7\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+5.94\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result416.tex <==
2D-M416:

$\hat{n}_{13}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result417.tex <==
2D-M417:

$\hat{n}_{13}=-0.79\hat{i}+0.28\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{14}=-0.93\hat{i}+0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{24}=0.36\hat{i}+0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result418.tex <==
2D-M418:

$\hat{n}_{13}=0.36\hat{i}+0.32\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{14}=-0.66\hat{i}+0.74\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result419.tex <==
2D-M419:

$\hat{n}_{13}=-0.0\hat{i}+0.8\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.41\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{25}=0.74\hat{i}+0.67\hat{j}+0.09\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+9.66\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result42.tex <==
{\tiny 2D-M42:}

$\hat{n}_{14}=0.0\hat{i}+0.95\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.68\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{35}=0.8\hat{i}+0.57\hat{j}-0.2\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+1.2\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result420.tex <==
2D-M420:

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.61\hat{i}-0.61\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{45}=-0.57\hat{i}-0.57\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+9.49\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result421.tex <==
2D-M421:

$\hat{n}_{13}=-0.41\hat{i}+0.41\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result422.tex <==
2D-M422:

$\hat{n}_{13}=-0.51\hat{i}+0.32\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.9\hat{i}-0.21\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{23}=-0.48\hat{i}-0.56\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{35}=-0.37\hat{i}+0.25\hat{j}+0.89\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.23\hat{i}+2.59\hat{j}+4.81\hat{k}$,\;\;\;$\vec{r}_{24}=6.61\hat{i}+8.27\hat{j}+8.93\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result423.tex <==
2D-M423:

$\hat{n}_{13}=-0.0\hat{i}+0.45\hat{j}+0.9\hat{k}$,\;\;\;$\hat{n}_{14}=0.68\hat{i}-0.71\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{23}=0.49\hat{i}+0.67\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{25}=-0.01\hat{i}+0.25\hat{j}+0.97\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result424.tex <==
2D-M424:

$\hat{n}_{13}=-0.81\hat{i}+0.29\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.93\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{25}=0.37\hat{i}+0.63\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+9.68\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result425.tex <==
2D-M425:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result426.tex <==
2D-M426:

$\hat{n}_{13}=-0.32\hat{i}-0.67\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{14}=-0.46\hat{i}-0.88\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{24}=0.28\hat{i}-0.96\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{35}=0.38\hat{i}+0.55\hat{j}-0.74\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.68\hat{i}+6.31\hat{j}+4.84\hat{k}$,\;\;\;$\vec{r}_{23}=3.98\hat{i}+3.51\hat{j}+1.89\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result427.tex <==
2D-M427:

$\hat{n}_{13}=-0.0\hat{i}+0.18\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.83\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}+0.45\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result428.tex <==
2D-M428:

$\hat{n}_{13}=-0.52\hat{i}-0.11\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{24}=0.04\hat{i}-0.63\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{25}=0.59\hat{i}-0.61\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.65\hat{j}-0.76\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result429.tex <==
2D-M429:

$\hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=-0.91\hat{i}+0.14\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{35}=-0.29\hat{i}-0.6\hat{j}+0.74\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result43.tex <==
{\tiny 2D-M43:}

$\hat{n}_{14}=0.68\hat{i}+0.56\hat{j}-0.47\hat{k}$,\;\;\;$\hat{n}_{24}=-0.42\hat{i}-0.62\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.14\hat{i}+0.82\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.84\hat{j}+0.54\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result430.tex <==
2D-M430:

$\hat{n}_{13}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.9\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.6\hat{i}-0.34\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result431.tex <==
2D-M431:

$\hat{n}_{13}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}+0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.6\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=0.04\hat{i}-0.66\hat{j}-0.75\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result432.tex <==
2D-M432:

$\hat{n}_{13}=0.68\hat{i}+0.55\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{23}=-0.78\hat{i}-0.54\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{25}=0.42\hat{i}-0.83\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{45}=-0.59\hat{i}-0.56\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result433.tex <==
2D-M433:

$\hat{n}_{13}=0.26\hat{i}-0.46\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.2\hat{i}-0.59\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result434.tex <==
2D-M434:

$\hat{n}_{13}=0.4\hat{i}+0.67\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{23}=-0.22\hat{i}-0.97\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}-0.76\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}+0.2\hat{j}+0.79\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.67\hat{i}+5.1\hat{j}+4.86\hat{k}$,\;\;\;$\vec{r}_{24}=5.46\hat{i}+4.73\hat{j}+5.25\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result435.tex <==
2D-M435:

$\hat{n}_{13}=0.81\hat{i}-0.22\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.49\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{24}=0.01\hat{i}-0.9\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result436.tex <==
2D-M436:

$\hat{n}_{13}=0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result437.tex <==
2D-M437:

$\hat{n}_{13}=0.63\hat{i}-0.02\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.88\hat{i}+0.35\hat{j}-0.31\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result438.tex <==
2D-M438:

$\hat{n}_{13}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.04\hat{i}-0.67\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{24}=0.13\hat{i}-0.38\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{35}=0.01\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+3.41\hat{k}$,\;\;\;$\vec{r}_{14}=4.67\hat{i}+5.79\hat{j}+5.32\hat{k}$,\;\;\;$\vec{r}_{23}=5.13\hat{i}+3.54\hat{j}+6.94\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result439.tex <==
2D-M439:

$\hat{n}_{13}=0.17\hat{i}+0.67\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{23}=0.72\hat{i}-0.66\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}-0.61\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.01\hat{i}+0.61\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result44.tex <==
{\tiny 2D-M44:}

$\hat{n}_{14}=0.7\hat{i}-0.1\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=0.74\hat{i}-0.18\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=-0.87\hat{i}-0.07\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{35}=-0.19\hat{i}-0.59\hat{j}+0.78\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result440.tex <==
2D-M440:

$\hat{n}_{13}=0.0\hat{i}+0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{14}=-0.21\hat{i}+0.03\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.11\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{25}=-0.49\hat{i}-0.87\hat{j}+0.08\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result441.tex <==
2D-M441:

$\hat{n}_{13}=-0.44\hat{i}-0.65\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{35}=0.06\hat{i}-0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result442.tex <==
2D-M442:

$\hat{n}_{13}=-0.5\hat{i}-0.62\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{14}=-0.78\hat{i}-0.62\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=-0.52\hat{i}+0.61\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.78\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result443.tex <==
2D-M443:

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.72\hat{i}-0.68\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.21\hat{j}+0.98\hat{k}$,\;\;\;$\hat{n}_{35}=0.46\hat{i}-0.61\hat{j}-0.65\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result444.tex <==
2D-M444:

$\hat{n}_{13}=0.0\hat{i}+0.97\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.37\hat{i}-0.66\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{35}=0.34\hat{i}+0.03\hat{j}-0.94\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result445.tex <==
2D-M445:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.5\hat{i}+0.51\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.12\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result446.tex <==
2D-M446:

$\hat{n}_{13}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.44\hat{i}+0.64\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.9\hat{i}+0.31\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{45}=-0.81\hat{i}+0.36\hat{j}-0.46\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result447.tex <==
2D-M447:

$\hat{n}_{13}=-0.33\hat{i}-0.07\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{14}=-0.39\hat{i}-0.92\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{23}=-0.34\hat{i}-0.94\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.09\hat{i}-0.53\hat{j}+0.84\hat{k}$,\newline
$\vec{r}_{23}=6.79\hat{i}+4.98\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{24}=4.49\hat{i}+5.46\hat{j}+4.46\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result448.tex <==
2D-M448:

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.54\hat{i}-0.58\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{23}=-0.77\hat{i}+0.64\hat{j}+0.07\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}-0.43\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result449.tex <==
2D-M449:

$\hat{n}_{13}=0.0\hat{i}+0.02\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.43\hat{i}+0.38\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+9.97\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result45.tex <==
{\tiny 2D-M45:}

$\hat{n}_{14}=-0.4\hat{i}-0.28\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{24}=0.63\hat{i}+0.63\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}-0.2\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{35}=0.12\hat{i}-0.64\hat{j}+0.76\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result450.tex <==
2D-M450:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.55\hat{i}+0.37\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.57\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.65\hat{i}+0.76\hat{j}+0.06\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result451.tex <==
2D-M451:

$\hat{n}_{13}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.52\hat{i}+0.66\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.81\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+9.14\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result452.tex <==
2D-M452:

$\hat{n}_{13}=-0.22\hat{i}-0.25\hat{j}+0.94\hat{k}$,\;\;\;$\hat{n}_{14}=-0.05\hat{i}-0.91\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=-0.13\hat{i}-0.99\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.23\hat{j}-0.78\hat{k}$,\newline
$\vec{r}_{14}=6.43\hat{i}+5.67\hat{j}+3.93\hat{k}$,\;\;\;$\vec{r}_{25}=5.8\hat{i}+5.18\hat{j}+4.73\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result453.tex <==
2D-M453:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.57\hat{i}-0.36\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=0.11\hat{i}-0.7\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}+0.51\hat{j}+0.25\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result454.tex <==
2D-M454:

$\hat{n}_{13}=0.73\hat{i}+0.19\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{14}=-0.07\hat{i}-0.92\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{25}=-0.5\hat{i}-0.75\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{35}=-0.82\hat{i}-0.06\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=3.86\hat{i}+3.2\hat{j}+5.51\hat{k}$,\;\;\;$\vec{r}_{24}=3.91\hat{i}+5.01\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result455.tex <==
2D-M455:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.34\hat{i}+0.34\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{23}=0.46\hat{i}-0.4\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=-0.67\hat{i}+0.67\hat{j}-0.33\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result456.tex <==
2D-M456:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}-0.48\hat{j}-0.31\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}-0.55\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{45}=-0.56\hat{i}+0.55\hat{j}+0.62\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result457.tex <==
2D-M457:

$\hat{n}_{13}=0.0\hat{i}+0.81\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.27\hat{i}+0.2\hat{j}+0.94\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result458.tex <==
2D-M458:

$\hat{n}_{13}=-0.71\hat{i}-0.69\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{14}=0.06\hat{i}-0.96\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.95\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{35}=0.66\hat{i}-0.72\hat{j}+0.22\hat{k}$,\newline
$\vec{r}_{14}=3.78\hat{i}+4.2\hat{j}+4.49\hat{k}$,\;\;\;$\vec{r}_{23}=3.7\hat{i}+4.48\hat{j}+5.93\hat{k}$,\;\;\;$\vec{r}_{24}=5.24\hat{i}+4.23\hat{j}+5.86\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result459.tex <==
2D-M459:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.86\hat{i}+0.15\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.2\hat{i}+0.58\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=0.35\hat{i}+0.93\hat{j}+0.09\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result46.tex <==
{\tiny 2D-M46:}

$\hat{n}_{14}=-0.62\hat{i}-0.71\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.71\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{25}=0.55\hat{i}-0.12\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{35}=0.13\hat{i}-0.7\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result460.tex <==
2D-M460:

$\hat{n}_{13}=0.61\hat{i}-0.59\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.02\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.61\hat{i}+0.77\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{25}=-0.17\hat{i}-0.98\hat{j}+0.06\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result461.tex <==
2D-M461:

$\hat{n}_{13}=0.12\hat{i}+0.65\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=-0.21\hat{i}-0.59\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{23}=-0.65\hat{i}-0.52\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.8\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result462.tex <==
2D-M462:

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.79\hat{i}-0.28\hat{j}+0.55\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result463.tex <==
2D-M463:

$\hat{n}_{13}=-0.24\hat{i}+0.33\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{14}=-0.16\hat{i}-0.98\hat{j}-0.1\hat{k}$,\;\;\;$\hat{n}_{23}=-0.52\hat{i}-0.86\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{35}=-0.3\hat{i}+0.44\hat{j}+0.85\hat{k}$,\newline
$\vec{r}_{14}=5.64\hat{i}+4.51\hat{j}+4.3\hat{k}$,\;\;\;$\vec{r}_{24}=5.55\hat{i}+5.55\hat{j}+4.32\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result464.tex <==
2D-M464:

$\hat{n}_{13}=0.67\hat{i}+0.74\hat{j}-0.07\hat{k}$,\;\;\;$\hat{n}_{14}=0.12\hat{i}+0.76\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.36\hat{i}-0.32\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result465.tex <==
2D-M465:

$\hat{n}_{13}=-0.51\hat{i}-0.51\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{14}=-0.89\hat{i}+0.44\hat{j}-0.07\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.8\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.21\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result466.tex <==
2D-M466:

$\hat{n}_{13}=0.98\hat{i}-0.13\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{14}=-0.91\hat{i}+0.42\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{45}=0.91\hat{i}+0.16\hat{j}-0.38\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result467.tex <==
2D-M467:

$\hat{n}_{13}=-0.28\hat{i}-0.61\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.26\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}+0.2\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.01\hat{i}+0.92\hat{j}-0.4\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result468.tex <==
2D-M468:

$\hat{n}_{13}=0.72\hat{i}+0.09\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{14}=-0.05\hat{i}-0.99\hat{j}+0.09\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.75\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{35}=0.14\hat{i}-0.99\hat{j}-0.01\hat{k}$,\newline
$\vec{r}_{14}=5.58\hat{i}+5.0\hat{j}+5.4\hat{k}$,\;\;\;$\vec{r}_{23}=4.72\hat{i}+4.21\hat{j}+4.43\hat{k}$,\;\;\;$\vec{r}_{24}=4.1\hat{i}+5.81\hat{j}+5.4\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result469.tex <==
2D-M469:

$\hat{n}_{13}=-0.42\hat{i}+0.43\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.25\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}+0.71\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{25}=-0.95\hat{i}-0.14\hat{j}-0.26\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result47.tex <==
{\tiny 2D-M47:}

$\hat{n}_{14}=0.82\hat{i}-0.53\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.85\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.38\hat{i}+0.92\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+9.45\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result470.tex <==
2D-M470:

$\hat{n}_{13}=-0.82\hat{i}-0.39\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}+0.39\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.9\hat{i}+0.27\hat{j}+0.34\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result471.tex <==
2D-M471:

$\hat{n}_{13}=-0.18\hat{i}-0.16\hat{j}+0.97\hat{k}$,\;\;\;$\hat{n}_{14}=-0.93\hat{i}-0.29\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{24}=-0.68\hat{i}-0.67\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{35}=0.28\hat{i}+0.39\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{14}=3.6\hat{i}+6.7\hat{j}+2.67\hat{k}$,\;\;\;$\vec{r}_{23}=3.29\hat{i}+3.72\hat{j}+2.54\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result472.tex <==
2D-M472:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.5\hat{i}+0.32\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.22\hat{i}-0.48\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result473.tex <==
2D-M473:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.07\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.55\hat{i}+0.53\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{35}=0.6\hat{i}+0.79\hat{j}+0.11\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result474.tex <==
2D-M474:

$\hat{n}_{13}=-0.19\hat{i}-0.52\hat{j}-0.84\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.63\hat{i}-0.55\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{35}=-0.77\hat{i}-0.45\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result475.tex <==
2D-M475:

$\hat{n}_{13}=0.48\hat{i}-0.68\hat{j}-0.55\hat{k}$,\;\;\;$\hat{n}_{24}=-0.6\hat{i}+0.55\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}+0.77\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{35}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result476.tex <==
2D-M476:

$\hat{n}_{13}=0.25\hat{i}-0.31\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{24}=-0.36\hat{i}-0.58\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{25}=-0.53\hat{i}-0.81\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{35}=0.04\hat{i}-0.6\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=3.13\hat{i}+7.06\hat{j}+4.74\hat{k}$,\;\;\;$\vec{r}_{25}=3.36\hat{i}+3.16\hat{j}+7.01\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result477.tex <==
2D-M477:

$\hat{n}_{13}=-0.56\hat{i}-0.15\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=-0.55\hat{i}+0.63\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.45\hat{i}-0.77\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result478.tex <==
2D-M478:

$\hat{n}_{13}=0.02\hat{i}+0.13\hat{j}-0.99\hat{k}$,\;\;\;$\hat{n}_{24}=-0.36\hat{i}-0.76\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.27\hat{i}-0.96\hat{j}-0.11\hat{k}$,\;\;\;$\hat{n}_{35}=-0.18\hat{i}+0.5\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=4.23\hat{i}+5.03\hat{j}+5.58\hat{k}$,\;\;\;$\vec{r}_{24}=4.93\hat{i}+4.37\hat{j}+4.76\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result479.tex <==
2D-M479:

$\hat{n}_{13}=0.47\hat{i}+0.34\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.46\hat{j}+0.89\hat{k}$,\;\;\;$\hat{n}_{25}=0.47\hat{i}+0.68\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{45}=-0.68\hat{i}+0.72\hat{j}-0.16\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result48.tex <==
{\tiny 2D-M48:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.64\hat{i}+0.64\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.09\hat{i}-0.7\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{45}=-0.49\hat{i}+0.5\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result480.tex <==
2D-M480:

$\hat{n}_{13}=0.85\hat{i}-0.29\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{23}=0.83\hat{i}+0.44\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.22\hat{i}+0.56\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{45}=-0.56\hat{i}+0.56\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result481.tex <==
2D-M481:

$\hat{n}_{13}=0.77\hat{i}-0.28\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{23}=0.64\hat{i}-0.74\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.9\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+1.0\hat{j}+0.05\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result482.tex <==
2D-M482:

$\hat{n}_{13}=-0.8\hat{i}-0.4\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.67\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.46\hat{i}-0.89\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.68\hat{j}-0.45\hat{k}$,\newline
$\vec{r}_{14}=2.75\hat{i}+2.95\hat{j}+7.74\hat{k}$,\;\;\;$\vec{r}_{23}=7.76\hat{i}+7.17\hat{j}+2.98\hat{k}$,\;\;\;$\vec{r}_{24}=5.72\hat{i}+2.73\hat{j}+2.31\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result483.tex <==
2D-M483:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.0\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=0.97\hat{i}+0.22\hat{j}-0.07\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result484.tex <==
2D-M484:

$\hat{n}_{13}=0.66\hat{i}-0.71\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}-0.7\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.8\hat{j}-0.13\hat{k}$,\;\;\;$\hat{n}_{45}=-0.16\hat{i}-0.07\hat{j}-0.98\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result485.tex <==
2D-M485:

$\hat{n}_{13}=0.19\hat{i}+0.98\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.92\hat{i}-0.18\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{45}=-0.13\hat{i}+0.76\hat{j}-0.63\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result486.tex <==
2D-M486:

$\hat{n}_{13}=-0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.43\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.57\hat{j}-0.82\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result487.tex <==
2D-M487:

$\hat{n}_{13}=0.02\hat{i}-0.35\hat{j}+0.94\hat{k}$,\;\;\;$\hat{n}_{23}=-0.7\hat{i}-0.67\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{24}=-0.84\hat{i}-0.53\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{35}=0.11\hat{i}+0.51\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=6.14\hat{i}+7.67\hat{j}+6.57\hat{k}$,\;\;\;$\vec{r}_{24}=7.74\hat{i}+4.9\hat{j}+3.93\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result488.tex <==
2D-M488:

$\hat{n}_{13}=-1.0\hat{i}-0.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.93\hat{i}-0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{25}=0.75\hat{i}-0.66\hat{j}+0.02\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result489.tex <==
2D-M489:

$\hat{n}_{13}=-0.59\hat{i}-0.3\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{23}=0.8\hat{i}-0.31\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.18\hat{i}-0.55\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{45}=0.56\hat{i}+0.59\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result49.tex <==
{\tiny 2D-M49:}

$\hat{n}_{14}=0.82\hat{i}+0.55\hat{j}-0.11\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{25}=0.67\hat{i}-0.3\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{34}=-0.71\hat{i}+0.0\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result490.tex <==
2D-M490:

$\hat{n}_{13}=-0.0\hat{i}+0.72\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{23}=0.78\hat{i}+0.43\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{25}=-0.63\hat{i}+0.55\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.71\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result491.tex <==
2D-M491:

$\hat{n}_{13}=-0.39\hat{i}+0.89\hat{j}+0.24\hat{k}$,\;\;\;$\hat{n}_{23}=-0.91\hat{i}-0.34\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.77\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result492.tex <==
2D-M492:

$\hat{n}_{13}=-0.73\hat{i}-0.64\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}-0.85\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}-0.76\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{35}=0.62\hat{i}-0.77\hat{j}+0.16\hat{k}$,\newline
$\vec{r}_{14}=4.11\hat{i}+5.6\hat{j}+4.22\hat{k}$,\;\;\;$\vec{r}_{23}=5.14\hat{i}+5.98\hat{j}+5.75\hat{k}$,\;\;\;$\vec{r}_{24}=5.63\hat{i}+5.96\hat{j}+4.02\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result493.tex <==
2D-M493:

$\hat{n}_{13}=0.7\hat{i}+0.36\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{23}=0.29\hat{i}-0.93\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{24}=0.7\hat{i}-0.0\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+1.0\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result494.tex <==
2D-M494:

$\hat{n}_{13}=-0.82\hat{i}-0.38\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.54\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.56\hat{i}-0.74\hat{j}-0.37\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result495.tex <==
2D-M495:

$\hat{n}_{13}=0.64\hat{i}-0.04\hat{j}+0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.39\hat{i}-0.8\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{24}=0.14\hat{i}-0.86\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{35}=0.33\hat{i}-0.72\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=4.04\hat{i}+3.89\hat{j}+4.19\hat{k}$,\;\;\;$\vec{r}_{23}=5.86\hat{i}+6.12\hat{j}+4.73\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result496.tex <==
2D-M496:

$\hat{n}_{13}=0.52\hat{i}-0.56\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.76\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}+0.49\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.77\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result497.tex <==
2D-M497:

$\hat{n}_{13}=-0.82\hat{i}-0.34\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.64\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.57\hat{i}+0.55\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result498.tex <==
2D-M498:

$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.57\hat{i}+0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}-0.56\hat{j}-0.59\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result499.tex <==
2D-M499:

$\hat{n}_{13}=-0.48\hat{i}-0.31\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=0.38\hat{i}+0.41\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{25}=0.54\hat{i}+0.63\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.63\hat{j}+0.78\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result5.tex <==
{\tiny 2D-M5:}

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.02\hat{i}-0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{45}=0.71\hat{i}-0.11\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result50.tex <==
{\tiny 2D-M50:}

$\hat{n}_{14}=-0.3\hat{i}+0.61\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.77\hat{i}+0.62\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.53\hat{i}-0.06\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{45}=-0.49\hat{i}-0.54\hat{j}+0.68\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result500.tex <==
2D-M500:

$\hat{n}_{13}=-0.75\hat{i}+0.66\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=0.5\hat{i}+0.0\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.45\hat{i}+0.67\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result501.tex <==
2D-M501:

$\hat{n}_{13}=0.59\hat{i}+0.19\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.68\hat{j}-0.44\hat{k}$,\;\;\;$\hat{n}_{24}=-0.59\hat{i}-0.56\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.14\hat{i}+0.98\hat{j}-0.14\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result502.tex <==
2D-M502:

$\hat{n}_{13}=0.78\hat{i}-0.6\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}+0.55\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=-0.12\hat{i}+0.13\hat{j}-0.98\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result503.tex <==
2D-M503:

$\hat{n}_{13}=0.72\hat{i}-0.66\hat{j}+0.23\hat{k}$,\;\;\;$\hat{n}_{23}=0.17\hat{i}+0.67\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}-0.61\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{25}=0.22\hat{i}-0.58\hat{j}-0.78\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result504.tex <==
2D-M504:

$\hat{n}_{13}=-0.78\hat{i}-0.25\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.57\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{25}=-0.09\hat{i}-0.62\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{45}=-0.47\hat{i}+0.17\hat{j}-0.87\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result505.tex <==
2D-M505:

$\hat{n}_{13}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}-0.77\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.62\hat{i}-0.77\hat{j}+0.15\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result506.tex <==
2D-M506:

$\hat{n}_{13}=-0.0\hat{i}+0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+9.98\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result507.tex <==
2D-M507:

$\hat{n}_{13}=-0.37\hat{i}+0.44\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.73\hat{i}+0.69\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{35}=0.24\hat{i}+0.89\hat{j}+0.37\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result508.tex <==
2D-M508:

$\hat{n}_{13}=-0.79\hat{i}-0.58\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.56\hat{j}+0.83\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result509.tex <==
2D-M509:

$\hat{n}_{13}=0.94\hat{i}+0.17\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.73\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.69\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{45}=-0.2\hat{i}+0.68\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result51.tex <==
{\tiny 2D-M51:}

$\hat{n}_{14}=0.28\hat{i}-0.63\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}-0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.37\hat{i}-0.37\hat{j}-0.85\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result510.tex <==
2D-M510:

$\hat{n}_{13}=-0.82\hat{i}+0.19\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{23}=-0.85\hat{i}+0.44\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.53\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+3.67\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result511.tex <==
2D-M511:

$\hat{n}_{13}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=0.57\hat{i}+0.49\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.59\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{25}=-0.38\hat{i}-0.3\hat{j}+0.87\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result512.tex <==
2D-M512:

$\hat{n}_{14}=-0.65\hat{i}-0.65\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{24}=0.97\hat{i}+0.15\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{25}=-0.04\hat{i}-0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}-0.47\hat{j}+0.5\hat{k}$,\newline
$\hat{n}_{35}=0.68\hat{i}-0.54\hat{j}+0.49\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=5.09\hat{i}+4.91\hat{j}+4.99\hat{k}$,\;\;\;$\vec{r}_{34}=5.11\hat{i}+4.91\hat{j}+5.0\hat{k}$,\newline
$\vec{r}_{35}=5.08\hat{i}+5.03\hat{j}+4.93\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result513.tex <==
2D-M513:

$\hat{n}_{14}=0.66\hat{i}-0.72\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{24}=0.5\hat{i}+0.79\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{25}=-0.84\hat{i}+0.35\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{34}=0.67\hat{i}-0.1\hat{j}-0.73\hat{k}$,\newline
$\hat{n}_{35}=-0.55\hat{i}+0.6\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=4.85\hat{i}+4.97\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{34}=4.85\hat{i}+5.11\hat{j}+5.32\hat{k}$,\newline
$\vec{r}_{35}=4.88\hat{i}+5.11\hat{j}+4.95\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result514.tex <==
2D-M514:

$\hat{n}_{14}=-0.69\hat{i}-0.46\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.58\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.58\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=-0.71\hat{i}-0.58\hat{j}+0.41\hat{k}$,\newline
$\hat{n}_{45}=0.0\hat{i}+0.58\hat{j}+0.82\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=4.91\hat{i}+5.04\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{34}=4.92\hat{i}+5.13\hat{j}+5.13\hat{k}$,\newline
$\vec{r}_{45}=4.95\hat{i}+4.99\hat{j}+4.77\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result515.tex <==
2D-M515:

$\hat{n}_{14}=-0.79\hat{i}+0.28\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{23}=0.29\hat{i}-0.55\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{25}=0.91\hat{i}-0.11\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{34}=-0.31\hat{i}-0.83\hat{j}-0.47\hat{k}$,\newline
$\hat{n}_{45}=-0.91\hat{i}+0.11\hat{j}+0.41\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.19\hat{i}+4.83\hat{j}+5.04\hat{k}$,\;\;\;$\vec{r}_{34}=5.19\hat{i}+5.16\hat{j}+4.96\hat{k}$,\newline
$\vec{r}_{45}=5.19\hat{i}+5.18\hat{j}+5.07\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result516.tex <==
2D-M516:

$\hat{n}_{14}=-0.4\hat{i}-0.67\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{23}=-0.36\hat{i}+0.04\hat{j}-0.93\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}-0.14\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{34}=0.12\hat{i}-0.99\hat{j}-0.08\hat{k}$,\newline
$\hat{n}_{45}=0.12\hat{i}-0.99\hat{j}-0.08\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=2.78\hat{i}+7.13\hat{j}+5.98\hat{k}$,\;\;\;$\vec{r}_{25}=2.95\hat{i}+2.59\hat{j}+6.99\hat{k}$,\newline
$\vec{r}_{45}=6.19\hat{i}+6.76\hat{j}+5.93\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result517.tex <==
2D-M517:

$\hat{n}_{14}=0.66\hat{i}-0.72\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{23}=0.29\hat{i}-0.67\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{25}=0.45\hat{i}-0.53\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.84\hat{i}-0.52\hat{j}-0.15\hat{k}$,\newline
$\hat{n}_{45}=0.22\hat{i}-0.97\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.99\hat{i}+4.87\hat{j}+4.99\hat{k}$,\;\;\;$\vec{r}_{25}=4.99\hat{i}+4.93\hat{j}+5.12\hat{k}$,\newline
$\vec{r}_{34}=5.08\hat{i}+5.07\hat{j}+5.09\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result518.tex <==
2D-M518:

$\hat{n}_{14}=0.8\hat{i}-0.31\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{15}=-0.8\hat{i}+0.31\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=-0.8\hat{i}+0.31\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}-0.69\hat{j}+0.45\hat{k}$,\newline
$\hat{n}_{34}=0.22\hat{i}-0.65\hat{j}-0.72\hat{k}$,\;\;\;$\vec{r}_{14}=5.05\hat{i}+5.06\hat{j}+5.07\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=5.08\hat{i}+5.01\hat{j}+5.01\hat{k}$,\newline
$\vec{r}_{34}=4.95\hat{i}+5.09\hat{j}+4.94\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result519.tex <==
2D-M519:

$\hat{n}_{14}=0.77\hat{i}-0.64\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{15}=0.77\hat{i}-0.64\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{23}=-0.49\hat{i}-0.62\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{25}=-0.41\hat{i}-0.45\hat{j}-0.79\hat{k}$,\newline
$\hat{n}_{34}=0.77\hat{i}-0.64\hat{j}-0.03\hat{k}$,\;\;\;$\vec{r}_{14}=5.13\hat{i}+4.73\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.73\hat{i}+4.93\hat{j}+5.0\hat{k}$,\newline
$\vec{r}_{25}=5.18\hat{i}+5.26\hat{j}+5.24\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result52.tex <==
{\tiny 2D-M52:}

$\hat{n}_{14}=-0.72\hat{i}+0.08\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}-0.19\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.8\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}+0.17\hat{j}+0.8\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result520.tex <==
2D-M520:

$\hat{n}_{14}=0.74\hat{i}-0.53\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{24}=-0.8\hat{i}-0.6\hat{j}-0.05\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}+0.23\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{34}=-0.39\hat{i}+0.73\hat{j}-0.55\hat{k}$,\newline
$\hat{n}_{35}=-0.34\hat{i}+0.42\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result521.tex <==
2D-M521:

$\hat{n}_{14}=-0.28\hat{i}+0.06\hat{j}-0.96\hat{k}$,\;\;\;$\hat{n}_{23}=-0.71\hat{i}-0.71\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.76\hat{i}-0.51\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{34}=-0.73\hat{i}-0.55\hat{j}-0.4\hat{k}$,\newline
$\hat{n}_{45}=0.48\hat{i}-0.37\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{23}=3.91\hat{i}+4.94\hat{j}+2.63\hat{k}$,\;\;\;$\vec{r}_{25}=3.26\hat{i}+3.3\hat{j}+4.41\hat{k}$,\;\;\;$\vec{r}_{34}=4.82\hat{i}+8.11\hat{j}+7.6\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result522.tex <==
2D-M522:

$\hat{n}_{14}=-0.66\hat{i}-0.28\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{15}=0.66\hat{i}+0.28\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.66\hat{i}-0.28\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}-0.07\hat{j}+0.7\hat{k}$,\newline
$\hat{n}_{34}=0.24\hat{i}-0.96\hat{j}+0.15\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.9\hat{i}+5.02\hat{j}+4.99\hat{k}$,\;\;\;$\vec{r}_{25}=4.98\hat{i}+4.98\hat{j}+4.98\hat{k}$,\newline
$\vec{r}_{34}=4.77\hat{i}+4.96\hat{j}+4.55\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result523.tex <==
2D-M523:

$\hat{n}_{14}=-0.64\hat{i}-0.31\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{15}=0.64\hat{i}+0.31\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=0.63\hat{i}+0.31\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-0.44\hat{i}+0.9\hat{j}+0.0\hat{k}$,\newline
$\hat{n}_{34}=0.64\hat{i}+0.31\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.8\hat{i}+4.95\hat{j}+5.4\hat{k}$,\;\;\;$\vec{r}_{25}=4.13\hat{i}+5.81\hat{j}+5.24\hat{k}$,\newline
$\vec{r}_{34}=5.88\hat{i}+5.51\hat{j}+5.09\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result524.tex <==
2D-M524:

$\hat{n}_{14}=0.97\hat{i}-0.26\hat{j}+0.03\hat{k}$,\;\;\;$\hat{n}_{15}=-0.26\hat{i}-0.93\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{23}=0.26\hat{i}+0.93\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{25}=-0.26\hat{i}-0.93\hat{j}+0.25\hat{k}$,\newline
$\hat{n}_{34}=-0.03\hat{i}-0.25\hat{j}-0.97\hat{k}$,\;\;\;$\vec{r}_{14}=4.83\hat{i}+5.06\hat{j}+4.87\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.76\hat{i}+5.11\hat{j}+4.74\hat{k}$,\newline
$\vec{r}_{34}=4.59\hat{i}+4.77\hat{j}+5.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result525.tex <==
2D-M525:

$\hat{n}_{14}=0.62\hat{i}+0.78\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{15}=-0.52\hat{i}+0.3\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{23}=0.52\hat{i}-0.3\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=-0.59\hat{i}+0.56\hat{j}-0.59\hat{k}$,\newline
$\hat{n}_{34}=0.52\hat{i}-0.3\hat{j}-0.8\hat{k}$,\;\;\;$\vec{r}_{14}=5.42\hat{i}+5.0\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.88\hat{i}+5.04\hat{j}+4.86\hat{k}$,\newline
$\vec{r}_{25}=5.12\hat{i}+5.09\hat{j}+4.89\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result526.tex <==
2D-M526:

$\hat{n}_{14}=-0.54\hat{i}-0.38\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{15}=-0.73\hat{i}+0.65\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.73\hat{i}+0.65\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{25}=-0.73\hat{i}+0.65\hat{j}-0.2\hat{k}$,\newline
$\hat{n}_{34}=0.42\hat{i}+0.66\hat{j}+0.63\hat{k}$,\;\;\;$\vec{r}_{14}=5.0\hat{i}+4.99\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=4.98\hat{i}+5.01\hat{j}+5.0\hat{k}$,\newline
$\vec{r}_{34}=5.0\hat{i}+5.0\hat{j}+5.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result527.tex <==
2D-M527:

$\hat{n}_{14}=-0.67\hat{i}+0.21\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{15}=-0.38\hat{i}-0.92\hat{j}+0.09\hat{k}$,\;\;\;$\hat{n}_{23}=-0.38\hat{i}-0.92\hat{j}+0.09\hat{k}$,\;\;\;$\hat{n}_{25}=0.64\hat{i}-0.34\hat{j}-0.69\hat{k}$,\newline
$\hat{n}_{34}=0.38\hat{i}+0.92\hat{j}-0.09\hat{k}$,\;\;\;$\vec{r}_{14}=5.47\hat{i}+4.86\hat{j}+5.19\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=4.97\hat{i}+4.57\hat{j}+5.17\hat{k}$,\newline
$\vec{r}_{34}=4.95\hat{i}+5.09\hat{j}+4.54\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result528.tex <==
2D-M528:

$\hat{n}_{14}=0.75\hat{i}-0.54\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{15}=0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.66\hat{i}-0.61\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}-0.58\hat{j}-0.81\hat{k}$,\newline
$\hat{n}_{34}=-0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\vec{r}_{14}=5.73\hat{i}+5.7\hat{j}+5.77\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.6\hat{i}+4.7\hat{j}+4.35\hat{k}$,\newline
$\vec{r}_{25}=5.72\hat{i}+4.61\hat{j}+5.19\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result529.tex <==
2D-M529:

$\hat{n}_{14}=0.34\hat{i}-0.16\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{15}=-0.82\hat{i}+0.44\hat{j}+0.37\hat{k}$,\;\;\;$\hat{n}_{23}=0.46\hat{i}+0.89\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}-0.44\hat{j}-0.37\hat{k}$,\newline
$\hat{n}_{34}=0.82\hat{i}-0.44\hat{j}-0.37\hat{k}$,\;\;\;$\vec{r}_{14}=5.06\hat{i}+5.11\hat{j}+5.03\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.14\hat{i}+5.03\hat{j}+5.14\hat{k}$,\newline
$\vec{r}_{34}=5.04\hat{i}+5.0\hat{j}+5.12\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result53.tex <==
{\tiny 2D-M53:}

$\hat{n}_{14}=0.25\hat{i}+0.41\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.21\hat{j}-0.98\hat{k}$,\;\;\;$\hat{n}_{25}=0.66\hat{i}-0.62\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{34}=-0.64\hat{i}+0.56\hat{j}+0.52\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result530.tex <==
2D-M530:

$\hat{n}_{13}=0.03\hat{i}-0.67\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{14}=0.04\hat{i}+0.75\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{24}=0.06\hat{i}-0.67\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{25}=1.0\hat{i}+0.01\hat{j}-0.07\hat{k}$,\newline
$\hat{n}_{35}=-0.05\hat{i}-0.75\hat{j}-0.66\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=5.04\hat{i}+5.04\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{25}=4.93\hat{i}+5.1\hat{j}+5.09\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result531.tex <==
2D-M531:

$\hat{n}_{13}=-0.66\hat{i}-0.72\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{14}=-0.57\hat{i}+0.49\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.81\hat{j}+0.11\hat{k}$,\;\;\;$\hat{n}_{25}=0.59\hat{i}-0.32\hat{j}+0.74\hat{k}$,\newline
$\hat{n}_{35}=-0.56\hat{i}-0.82\hat{j}+0.1\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.79\hat{i}+5.0\hat{j}+5.1\hat{k}$,\;\;\;$\vec{r}_{25}=5.07\hat{i}+5.02\hat{j}+4.79\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result532.tex <==
2D-M532:

$\hat{n}_{13}=0.06\hat{i}-0.73\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{14}=-0.5\hat{i}-0.64\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{24}=0.87\hat{i}-0.36\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}-0.68\hat{j}+0.74\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}+0.67\hat{j}-0.74\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.48\hat{i}+4.46\hat{j}+4.21\hat{k}$,\;\;\;$\vec{r}_{24}=4.62\hat{i}+5.53\hat{j}+4.44\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result533.tex <==
2D-M533:

$\hat{n}_{13}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.06\hat{i}-0.94\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{24}=-0.9\hat{i}-0.44\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{25}=-0.08\hat{i}-0.8\hat{j}-0.59\hat{k}$,\newline
$\hat{n}_{35}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=1.77\hat{i}+2.39\hat{j}+8.5\hat{k}$,\;\;\;$\vec{r}_{24}=6.02\hat{i}+6.41\hat{j}+1.13\hat{k}$,\newline
$\vec{r}_{25}=2.33\hat{i}+7.66\hat{j}+6.24\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result534.tex <==
2D-M534:

$\hat{n}_{13}=0.25\hat{i}-0.91\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{14}=0.4\hat{i}-0.29\hat{j}-0.87\hat{k}$,\;\;\;$\hat{n}_{23}=-0.61\hat{i}+0.45\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=0.55\hat{i}+0.83\hat{j}-0.06\hat{k}$,\newline
$\hat{n}_{45}=0.78\hat{i}-0.36\hat{j}+0.51\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result535.tex <==
2D-M535:

$\hat{n}_{13}=-0.0\hat{i}+0.7\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{14}=0.75\hat{i}-0.43\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{23}=-0.57\hat{i}-0.82\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{25}=-0.44\hat{i}+0.31\hat{j}-0.84\hat{k}$,\newline
$\hat{n}_{45}=0.44\hat{i}-0.27\hat{j}-0.86\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result536.tex <==
2D-M536:

$\hat{n}_{13}=0.71\hat{i}+0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{23}=-0.19\hat{i}-0.6\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{25}=-0.78\hat{i}+0.6\hat{j}-0.19\hat{k}$,\newline
$\hat{n}_{45}=0.48\hat{i}-0.81\hat{j}-0.33\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.21\hat{i}+5.43\hat{j}+4.46\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result537.tex <==
2D-M537:

$\hat{n}_{13}=-0.23\hat{i}-0.94\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}-0.8\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.56\hat{j}+0.58\hat{k}$,\newline
$\hat{n}_{45}=0.01\hat{i}-1.0\hat{j}+0.01\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.01\hat{i}+4.97\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result538.tex <==
2D-M538:

$\hat{n}_{13}=-0.0\hat{i}+0.42\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{14}=-0.55\hat{i}-0.67\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}-0.84\hat{j}-0.09\hat{k}$,\;\;\;$\hat{n}_{24}=-0.99\hat{i}-0.08\hat{j}-0.14\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=6.34\hat{i}+1.41\hat{j}+3.89\hat{k}$,\;\;\;$\vec{r}_{23}=4.42\hat{i}+4.13\hat{j}+2.91\hat{k}$,\newline
$\vec{r}_{24}=2.54\hat{i}+7.19\hat{j}+8.33\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result539.tex <==
2D-M539:

$\hat{n}_{13}=0.71\hat{i}-0.71\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}+0.58\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{24}=-0.23\hat{i}+0.23\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{25}=-0.42\hat{i}+0.42\hat{j}+0.8\hat{k}$,\newline
$\hat{n}_{35}=0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=5.15\hat{i}+5.24\hat{j}+4.97\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result54.tex <==
{\tiny 2D-M54:}

$\hat{n}_{14}=0.41\hat{i}+0.67\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{23}=0.66\hat{i}+0.6\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.71\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{45}=-0.69\hat{i}+0.72\hat{j}-0.04\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result540.tex <==
2D-M540:

$\hat{n}_{13}=0.76\hat{i}-0.46\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{14}=0.8\hat{i}-0.42\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{24}=0.56\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.94\hat{i}-0.23\hat{j}+0.23\hat{k}$,\newline
$\hat{n}_{35}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=5.21\hat{i}+5.03\hat{j}+5.18\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result541.tex <==
2D-M541:

$\hat{n}_{13}=-0.15\hat{i}-0.31\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{14}=0.12\hat{i}-0.88\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{24}=-0.25\hat{i}-0.83\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{25}=0.07\hat{i}-0.68\hat{j}+0.73\hat{k}$,\newline
$\hat{n}_{35}=0.67\hat{i}+0.13\hat{j}+0.73\hat{k}$,\;\;\;$\vec{r}_{14}=6.24\hat{i}+3.46\hat{j}+3.16\hat{k}$,\;\;\;$\vec{r}_{24}=3.45\hat{i}+3.71\hat{j}+3.74\hat{k}$,\;\;\;$\vec{r}_{25}=5.31\hat{i}+6.47\hat{j}+6.68\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result542.tex <==
2D-M542:

$\hat{n}_{13}=0.64\hat{i}-0.4\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.45\hat{i}-0.21\hat{j}+0.87\hat{k}$,\;\;\;$\hat{n}_{23}=0.18\hat{i}-0.93\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=0.49\hat{i}+0.87\hat{j}+0.05\hat{k}$,\newline
$\hat{n}_{45}=0.72\hat{i}-0.46\hat{j}-0.51\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result543.tex <==
2D-M543:

$\hat{n}_{13}=0.57\hat{i}+0.4\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}+0.47\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{23}=0.27\hat{i}+0.74\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{25}=0.16\hat{i}-0.63\hat{j}-0.76\hat{k}$,\newline
$\hat{n}_{45}=-0.54\hat{i}-0.45\hat{j}+0.72\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result544.tex <==
2D-M544:

$\hat{n}_{13}=-0.65\hat{i}-0.74\hat{j}-0.19\hat{k}$,\;\;\;$\hat{n}_{14}=-0.66\hat{i}-0.72\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.76\hat{i}+0.63\hat{j}+0.16\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.25\hat{j}-0.97\hat{k}$,\newline
$\hat{n}_{45}=-0.56\hat{i}-0.82\hat{j}-0.1\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=5.73\hat{i}+2.72\hat{j}+3.96\hat{k}$,\;\;\;$\vec{r}_{25}=3.27\hat{i}+2.79\hat{j}+2.7\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result545.tex <==
2D-M545:

$\hat{n}_{13}=-0.16\hat{i}-0.91\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{14}=-0.16\hat{i}-0.91\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{23}=0.31\hat{i}-0.41\hat{j}+0.86\hat{k}$,\;\;\;$\hat{n}_{24}=0.94\hat{i}-0.03\hat{j}-0.35\hat{k}$,\newline
$\hat{n}_{45}=0.16\hat{i}-0.66\hat{j}-0.73\hat{k}$,\;\;\;$\vec{r}_{14}=4.95\hat{i}+4.99\hat{j}+5.02\hat{k}$,\;\;\;$\vec{r}_{23}=5.0\hat{i}+5.13\hat{j}+4.97\hat{k}$,\;\;\;$\vec{r}_{24}=5.07\hat{i}+4.88\hat{j}+4.86\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result546.tex <==
2D-M546:

$\hat{n}_{13}=0.19\hat{i}-0.98\hat{j}-0.05\hat{k}$,\;\;\;$\hat{n}_{14}=0.88\hat{i}-0.45\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{23}=-0.4\hat{i}-0.62\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{24}=-0.23\hat{i}-0.64\hat{j}+0.73\hat{k}$,\newline
$\hat{n}_{35}=0.41\hat{i}-0.89\hat{j}+0.21\hat{k}$,\;\;\;$\vec{r}_{14}=4.91\hat{i}+4.92\hat{j}+5.06\hat{k}$,\;\;\;$\vec{r}_{23}=4.99\hat{i}+4.92\hat{j}+4.96\hat{k}$,\;\;\;$\vec{r}_{24}=5.07\hat{i}+5.07\hat{j}+5.17\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result547.tex <==
2D-M547:

$\hat{n}_{13}=-0.01\hat{i}-0.01\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.2\hat{i}-0.98\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.98\hat{i}-0.2\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{24}=-0.01\hat{i}-0.01\hat{j}-1.0\hat{k}$,\newline
$\hat{n}_{25}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\vec{r}_{14}=6.43\hat{i}+7.63\hat{j}+2.17\hat{k}$,\;\;\;$\vec{r}_{23}=2.2\hat{i}+5.86\hat{j}+6.27\hat{k}$,\;\;\;$\vec{r}_{24}=2.38\hat{i}+6.94\hat{j}+2.16\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+7.76\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result548.tex <==
2D-M548:

$\hat{n}_{13}=-0.4\hat{i}+0.52\hat{j}+0.76\hat{k}$,\;\;\;$\hat{n}_{14}=-0.9\hat{i}-0.34\hat{j}-0.28\hat{k}$,\;\;\;$\hat{n}_{24}=0.88\hat{i}-0.47\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=0.43\hat{i}-0.75\hat{j}-0.5\hat{k}$,\newline
$\hat{n}_{35}=0.0\hat{i}+0.81\hat{j}-0.59\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result549.tex <==
2D-M549:

$\hat{n}_{13}=0.71\hat{i}+0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.23\hat{i}-0.23\hat{j}-0.94\hat{k}$,\;\;\;$\hat{n}_{25}=0.42\hat{i}-0.42\hat{j}+0.8\hat{k}$,\newline
$\hat{n}_{35}=0.7\hat{i}-0.7\hat{j}+0.12\hat{k}$,\;\;\;$\vec{r}_{13}=2.94\hat{i}+5.77\hat{j}+5.56\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result55.tex <==
{\tiny 2D-M55:}

$\hat{n}_{14}=0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.46\hat{i}+0.48\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{34}=0.9\hat{i}-0.44\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.7\hat{i}+0.11\hat{j}-0.7\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result550.tex <==
2D-M550:

$\hat{n}_{13}=-0.19\hat{i}+0.86\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{14}=0.67\hat{i}-0.25\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}-0.65\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.26\hat{j}-0.96\hat{k}$,\newline
$\hat{n}_{35}=-0.78\hat{i}-0.45\hat{j}-0.44\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result551.tex <==
2D-M551:

$\hat{n}_{13}=-0.08\hat{i}-0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.61\hat{i}-0.53\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{24}=0.07\hat{i}+0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=0.79\hat{i}-0.47\hat{j}-0.39\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}+0.77\hat{j}-0.64\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.99\hat{i}+4.98\hat{j}+4.98\hat{k}$,\;\;\;$\vec{r}_{25}=5.01\hat{i}+4.99\hat{j}+5.01\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result552.tex <==
2D-M552:

$\hat{n}_{13}=-0.71\hat{i}+0.0\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.56\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}-0.8\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{25}=0.23\hat{i}+0.94\hat{j}+0.23\hat{k}$,\newline
$\hat{n}_{35}=-0.05\hat{i}-1.0\hat{j}-0.05\hat{k}$,\;\;\;$\vec{r}_{13}=4.97\hat{i}+4.99\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result553.tex <==
2D-M553:

$\hat{n}_{13}=0.27\hat{i}+0.95\hat{j}-0.13\hat{k}$,\;\;\;$\hat{n}_{14}=0.72\hat{i}-0.1\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{24}=0.66\hat{i}-0.23\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{25}=0.23\hat{i}+0.97\hat{j}-0.09\hat{k}$,\newline
$\hat{n}_{35}=-0.16\hat{i}+0.94\hat{j}+0.29\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.05\hat{i}+4.92\hat{j}+4.92\hat{k}$,\;\;\;$\vec{r}_{24}=5.05\hat{i}+5.0\hat{j}+4.99\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result554.tex <==
2D-M554:

$\hat{n}_{13}=-0.64\hat{i}-0.14\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{14}=0.57\hat{i}-0.74\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{23}=0.57\hat{i}-0.74\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}+0.66\hat{j}+0.56\hat{k}$,\newline
$\hat{n}_{45}=0.03\hat{i}-1.0\hat{j}-0.06\hat{k}$,\;\;\;$\vec{r}_{13}=4.92\hat{i}+5.04\hat{j}+4.91\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.98\hat{i}+4.91\hat{j}+4.97\hat{k}$,\newline
$\vec{r}_{24}=4.94\hat{i}+5.08\hat{j}+4.94\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result555.tex <==
2D-M555:

$\hat{n}_{13}=0.16\hat{i}-0.75\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{14}=0.44\hat{i}-0.53\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.16\hat{i}-0.75\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{24}=-0.89\hat{i}-0.39\hat{j}-0.24\hat{k}$,\newline
$\hat{n}_{35}=0.6\hat{i}-0.8\hat{j}+0.07\hat{k}$,\;\;\;$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=5.03\hat{i}+4.83\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{23}=4.81\hat{i}+4.8\hat{j}+5.08\hat{k}$,\newline
$\vec{r}_{24}=4.89\hat{i}+4.91\hat{j}+5.2\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result556.tex <==
2D-M556:

$\hat{n}_{13}=0.27\hat{i}-0.66\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{14}=-0.64\hat{i}+0.41\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{23}=-0.78\hat{i}-0.36\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{24}=-0.72\hat{i}-0.57\hat{j}-0.41\hat{k}$,\newline
$\hat{n}_{25}=-0.73\hat{i}-0.66\hat{j}+0.18\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result557.tex <==
2D-M557:

$\hat{n}_{13}=0.74\hat{i}+0.35\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=-0.62\hat{i}+0.67\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{23}=0.62\hat{i}-0.67\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{24}=-0.24\hat{i}-0.65\hat{j}+0.72\hat{k}$,\newline
$\hat{n}_{45}=0.88\hat{i}+0.18\hat{j}+0.44\hat{k}$,\;\;\;$\vec{r}_{13}=4.95\hat{i}+4.94\hat{j}+5.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.95\hat{i}+4.95\hat{j}+4.95\hat{k}$,\;\;\;$\vec{r}_{24}=5.06\hat{i}+5.05\hat{j}+5.06\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result558.tex <==
2D-M558:

$\hat{n}_{13}=-0.01\hat{i}-0.88\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.38\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{23}=-0.01\hat{i}-0.88\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.28\hat{j}-0.5\hat{k}$,\newline
$\hat{n}_{35}=0.8\hat{i}-0.59\hat{j}+0.14\hat{k}$,\;\;\;$\vec{r}_{13}=5.0\hat{i}+5.04\hat{j}+4.87\hat{k}$,\;\;\;$\vec{r}_{14}=5.14\hat{i}+4.88\hat{j}+4.93\hat{k}$,\;\;\;$\vec{r}_{24}=5.06\hat{i}+5.14\hat{j}+4.94\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result559.tex <==
2D-M559:

$\hat{n}_{13}=-0.52\hat{i}+0.68\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{14}=0.69\hat{i}+0.69\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{23}=-0.39\hat{i}-0.72\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}-0.24\hat{j}+0.83\hat{k}$,\newline
$\hat{n}_{25}=-0.8\hat{i}+0.34\hat{j}-0.49\hat{k}$,\;\;\;$\vec{r}_{13}=5.36\hat{i}+4.71\hat{j}+5.12\hat{k}$,\;\;\;$\vec{r}_{14}=5.38\hat{i}+5.66\hat{j}+5.16\hat{k}$,\;\;\;$\vec{r}_{24}=5.07\hat{i}+4.73\hat{j}+5.36\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result56.tex <==
{\tiny 2D-M56:}

$\hat{n}_{14}=0.82\hat{i}-0.52\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=-0.93\hat{i}-0.25\hat{j}+0.25\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+9.98\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result560.tex <==
2D-M560:

$\hat{n}_{14}=-0.13\hat{i}+0.58\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.6\hat{i}+0.6\hat{j}+0.53\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result561.tex <==
2D-M561:

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.69\hat{i}+0.56\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.82\hat{j}-0.57\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result562.tex <==
2D-M562:

$\hat{n}_{14}=-0.08\hat{i}-0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=-0.48\hat{i}+0.68\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{25}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{34}=0.6\hat{i}-0.55\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result563.tex <==
2D-M563:

$\hat{n}_{14}=-0.03\hat{i}+0.77\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{24}=-0.37\hat{i}+0.56\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{25}=-0.93\hat{i}-0.17\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.69\hat{j}-0.72\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result564.tex <==
2D-M564:

$\hat{n}_{14}=-0.26\hat{i}+0.79\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}-0.56\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result565.tex <==
2D-M565:

$\hat{n}_{14}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.67\hat{i}+0.74\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.72\hat{i}-0.7\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+1.02\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+9.32\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result566.tex <==
2D-M566:

$\hat{n}_{14}=-0.0\hat{i}-0.91\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.59\hat{i}+0.7\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{34}=-0.76\hat{i}-0.65\hat{j}+0.02\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result567.tex <==
2D-M567:

$\hat{n}_{14}=0.27\hat{i}+0.67\hat{j}-0.69\hat{k}$,\;\;\;$\hat{n}_{23}=-0.01\hat{i}-0.71\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.01\hat{i}+0.71\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result568.tex <==
2D-M568:

$\hat{n}_{14}=-0.64\hat{i}+0.57\hat{j}-0.52\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result569.tex <==
2D-M569:

$\hat{n}_{14}=-0.01\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.21\hat{i}+0.79\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result57.tex <==
{\tiny 2D-M57:}

$\hat{n}_{14}=-0.7\hat{i}+0.09\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{25}=0.6\hat{i}+0.6\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}+0.67\hat{j}-0.3\hat{k}$,\;\;\;$\hat{n}_{45}=-0.72\hat{i}-0.5\hat{j}+0.48\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result570.tex <==
2D-M570:

$\hat{n}_{14}=0.98\hat{i}-0.12\hat{j}+0.13\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.7\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result571.tex <==
2D-M571:

$\hat{n}_{14}=-0.05\hat{i}+1.0\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=0.63\hat{i}+0.63\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result572.tex <==
2D-M572:

$\hat{n}_{14}=-0.68\hat{i}+0.34\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{23}=0.53\hat{i}-0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}+0.77\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result573.tex <==
2D-M573:

$\hat{n}_{14}=-0.65\hat{i}+0.76\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.6\hat{i}-0.6\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{25}=-0.38\hat{i}+0.38\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result574.tex <==
2D-M574:

$\hat{n}_{14}=-0.45\hat{i}-0.89\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.63\hat{i}-0.63\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result575.tex <==
2D-M575:

$\hat{n}_{14}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{25}=-1.0\hat{i}+0.0\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.93\hat{i}-0.25\hat{j}-0.25\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result576.tex <==
2D-M576:

$\hat{n}_{14}=-0.95\hat{i}-0.23\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{25}=0.36\hat{i}+0.66\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{34}=-0.93\hat{i}+0.25\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result577.tex <==
2D-M577:

$\hat{n}_{14}=0.15\hat{i}-0.85\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.8\hat{i}+0.33\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{34}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=-0.0\hat{i}+0.52\hat{j}-0.86\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result578.tex <==
2D-M578:

$\hat{n}_{14}=0.19\hat{i}+0.77\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{15}=-0.84\hat{i}+0.09\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.98\hat{i}-0.15\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.62\hat{j}+0.78\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result579.tex <==
2D-M579:

$\hat{n}_{14}=-0.81\hat{i}-0.27\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{15}=0.0\hat{i}+0.75\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{23}=0.12\hat{i}+0.8\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}+0.54\hat{j}-0.61\hat{k}$,\newline
$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result58.tex <==
{\tiny 2D-M58:}

$\hat{n}_{14}=-0.0\hat{i}+0.85\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{25}=0.34\hat{i}-0.23\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{34}=-0.48\hat{i}-0.73\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{45}=-0.76\hat{i}-0.64\hat{j}-0.01\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result580.tex <==
2D-M580:

$\hat{n}_{14}=-0.49\hat{i}+0.81\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{15}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.65\hat{i}+0.1\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result581.tex <==
2D-M581:

$\hat{n}_{15}=0.53\hat{i}-0.27\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}+0.42\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.01\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{34}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result582.tex <==
2D-M582:

$\hat{n}_{13}=0.23\hat{i}-0.75\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result583.tex <==
2D-M583:

$\hat{n}_{13}=-0.67\hat{i}+0.45\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{14}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=0.56\hat{i}-0.6\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{35}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result584.tex <==
2D-M584:

$\hat{n}_{13}=-0.25\hat{i}-0.55\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}-0.38\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{24}=0.0\hat{i}+0.75\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.54\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result585.tex <==
2D-M585:

$\hat{n}_{13}=-0.02\hat{i}+0.7\hat{j}-0.72\hat{k}$,\;\;\;$\hat{n}_{14}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{24}=0.8\hat{i}+0.52\hat{j}+0.28\hat{k}$,\;\;\;$\hat{n}_{35}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result586.tex <==
2D-M586:

$\hat{n}_{13}=-0.57\hat{i}-0.49\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.59\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result587.tex <==
2D-M587:

$\hat{n}_{13}=-0.05\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.36\hat{i}-0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.93\hat{i}-0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result588.tex <==
2D-M588:

$\hat{n}_{13}=0.36\hat{i}+0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.93\hat{i}+0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{45}=-0.05\hat{i}-0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result589.tex <==
2D-M589:

$\hat{n}_{13}=0.97\hat{i}-0.11\hat{j}+0.2\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.7\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{23}=0.48\hat{i}-0.87\hat{j}+0.06\hat{k}$,\;\;\;$\hat{n}_{35}=-0.19\hat{i}-0.87\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{23}=4.03\hat{i}+6.0\hat{j}+5.93\hat{k}$,\;\;\;$\vec{r}_{24}=6.07\hat{i}+6.19\hat{j}+4.65\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result59.tex <==
{\tiny 2D-M59:}

$\hat{n}_{14}=-0.79\hat{i}-0.21\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{15}=-0.4\hat{i}-0.12\hat{j}+0.91\hat{k}$,\;\;\;$\hat{n}_{23}=-0.63\hat{i}-0.63\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result590.tex <==
2D-M590:

$\hat{n}_{13}=0.57\hat{i}+0.49\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{14}=-0.58\hat{i}-0.59\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{23}=0.82\hat{i}-0.41\hat{j}-0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.26\hat{i}-0.84\hat{j}+0.47\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result591.tex <==
2D-M591:

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.53\hat{i}+0.27\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{24}=-0.62\hat{i}-0.77\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result592.tex <==
2D-M592:

$\hat{n}_{13}=0.76\hat{i}+0.65\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.63\hat{i}+0.63\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{24}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result593.tex <==
2D-M593:

$\hat{n}_{13}=0.03\hat{i}+0.87\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{14}=0.55\hat{i}-0.55\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.45\hat{i}+0.45\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result594.tex <==
2D-M594:

$\hat{n}_{13}=0.01\hat{i}+0.7\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=0.47\hat{i}+0.35\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.82\hat{i}+0.42\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result595.tex <==
2D-M595:

$\hat{n}_{13}=0.58\hat{i}-0.82\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.34\hat{i}+0.47\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.6\hat{i}-0.56\hat{j}+0.57\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result596.tex <==
2D-M596:

$\hat{n}_{13}=-0.81\hat{i}-0.48\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{14}=-0.81\hat{i}-0.48\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.06\hat{i}+0.64\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result597.tex <==
2D-M597:

$\hat{n}_{13}=-0.84\hat{i}-0.37\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{14}=-0.13\hat{i}-0.99\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{23}=-0.19\hat{i}-0.98\hat{j}-0.03\hat{k}$,\;\;\;$\hat{n}_{35}=0.32\hat{i}-0.93\hat{j}-0.17\hat{k}$,\newline
$\vec{r}_{14}=5.77\hat{i}+4.06\hat{j}+3.99\hat{k}$,\;\;\;$\vec{r}_{24}=5.34\hat{i}+4.63\hat{j}+6.04\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result598.tex <==
2D-M598:

$\hat{n}_{13}=-0.71\hat{i}+0.71\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.07\hat{i}-0.67\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result599.tex <==
2D-M599:

$\hat{n}_{13}=0.65\hat{i}+0.55\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.4\hat{i}-0.34\hat{j}-0.85\hat{k}$,\;\;\;$\hat{n}_{45}=0.7\hat{i}+0.71\hat{j}-0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+2.98\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+5.77\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result6.tex <==
{\tiny 2D-M6:}

$\hat{n}_{14}=0.74\hat{i}-0.67\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{24}=-0.37\hat{i}-0.31\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}-0.57\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result60.tex <==
{\tiny 2D-M60:}

$\hat{n}_{14}=0.8\hat{i}-0.54\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{15}=0.35\hat{i}+0.91\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{34}=-0.16\hat{i}-0.62\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result600.tex <==
2D-M600:

$\hat{n}_{13}=-0.21\hat{i}+0.58\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{14}=0.21\hat{i}-0.58\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.01\hat{i}+0.81\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result601.tex <==
2D-M601:

$\hat{n}_{13}=-0.77\hat{i}-0.63\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{14}=-0.82\hat{i}-0.58\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.35\hat{i}-0.91\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{35}=0.63\hat{i}-0.77\hat{j}+0.03\hat{k}$,\newline
$\vec{r}_{14}=4.03\hat{i}+4.08\hat{j}+4.09\hat{k}$,\;\;\;$\vec{r}_{23}=4.01\hat{i}+5.96\hat{j}+5.94\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result602.tex <==
2D-M602:

$\hat{n}_{13}=0.57\hat{i}+0.49\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.59\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{25}=0.57\hat{i}+0.29\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result603.tex <==
2D-M603:

$\hat{n}_{13}=-0.57\hat{i}-0.64\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{25}=0.58\hat{i}+0.56\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{35}=0.82\hat{i}-0.41\hat{j}+0.41\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result604.tex <==
2D-M604:

$\hat{n}_{13}=-0.03\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.36\hat{i}+0.66\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.93\hat{i}+0.25\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.71\hat{j}+0.71\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result605.tex <==
2D-M605:

$\hat{n}_{13}=0.04\hat{i}+0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{24}=0.93\hat{i}+0.25\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{25}=-0.36\hat{i}+0.66\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{35}=0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result606.tex <==
2D-M606:

$\hat{n}_{13}=0.82\hat{i}+0.38\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{23}=-0.04\hat{i}-0.72\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{25}=-0.58\hat{i}+0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.07\hat{i}+0.67\hat{j}-0.74\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result607.tex <==
2D-M607:

$\hat{n}_{13}=-0.02\hat{i}+0.65\hat{j}+0.76\hat{k}$,\;\;\;$\hat{n}_{23}=1.0\hat{i}+0.0\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}+0.76\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{45}=-0.58\hat{i}-0.53\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result608.tex <==
2D-M608:

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.7\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{24}=0.76\hat{i}+0.65\hat{j}-0.02\hat{k}$,\;\;\;$\hat{n}_{45}=-0.1\hat{i}-0.92\hat{j}-0.39\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result609.tex <==
2D-M609:

$\hat{n}_{13}=0.79\hat{i}+0.27\hat{j}+0.55\hat{k}$,\;\;\;$\hat{n}_{23}=-0.11\hat{i}-0.98\hat{j}+0.18\hat{k}$,\;\;\;$\hat{n}_{24}=-0.02\hat{i}-0.99\hat{j}+0.11\hat{k}$,\;\;\;$\hat{n}_{35}=-0.6\hat{i}+0.19\hat{j}+0.77\hat{k}$,\newline
$\vec{r}_{14}=3.89\hat{i}+5.76\hat{j}+4.46\hat{k}$,\;\;\;$\vec{r}_{24}=3.89\hat{i}+5.39\hat{j}+6.11\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result61.tex <==
{\tiny 2D-M61:}

$\hat{n}_{14}=-0.67\hat{i}-0.3\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{15}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.3\hat{i}+0.67\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{34}=0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+0.0\hat{j}+7.65\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result610.tex <==
2D-M610:

$\hat{n}_{13}=0.45\hat{i}+0.36\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.58\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{24}=-0.33\hat{i}-0.48\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{25}=-0.44\hat{i}-0.71\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result611.tex <==
2D-M611:

$\hat{n}_{13}=0.37\hat{i}-0.93\hat{j}-0.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.93\hat{i}+0.37\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}+0.79\hat{j}+0.61\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result612.tex <==
2D-M612:

$\hat{n}_{13}=-0.82\hat{i}-0.38\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.75\hat{j}-0.66\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}+0.54\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{45}=0.41\hat{i}+0.36\hat{j}-0.84\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result613.tex <==
2D-M613:

$\hat{n}_{13}=0.76\hat{i}-0.62\hat{j}-0.18\hat{k}$,\;\;\;$\hat{n}_{23}=-0.09\hat{i}-0.83\hat{j}-0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.21\hat{i}-0.89\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{35}=-0.55\hat{i}-0.77\hat{j}+0.33\hat{k}$,\newline
$\vec{r}_{14}=6.72\hat{i}+5.99\hat{j}+6.41\hat{k}$,\;\;\;$\vec{r}_{23}=3.54\hat{i}+3.37\hat{j}+3.29\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result614.tex <==
2D-M614:

$\hat{n}_{13}=0.75\hat{i}-0.5\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{23}=-0.13\hat{i}+0.52\hat{j}+0.84\hat{k}$,\;\;\;$\hat{n}_{24}=-0.61\hat{i}+0.71\hat{j}-0.35\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result615.tex <==
2D-M615:

$\hat{n}_{13}=0.83\hat{i}+0.22\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{24}=0.89\hat{i}+0.46\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.58\hat{j}-0.82\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result616.tex <==
2D-M616:

$\hat{n}_{13}=-0.56\hat{i}+0.63\hat{j}+0.54\hat{k}$,\;\;\;$\hat{n}_{23}=-0.56\hat{i}-0.77\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{25}=0.61\hat{i}-0.13\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result617.tex <==
2D-M617:

$\hat{n}_{13}=-0.82\hat{i}+0.41\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{45}=-0.03\hat{i}+0.78\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result618.tex <==
2D-M618:

$\hat{n}_{13}=-0.7\hat{i}+0.71\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{23}=0.7\hat{i}-0.71\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{24}=-0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{35}=0.01\hat{i}-0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result619.tex <==
2D-M619:

$\hat{n}_{13}=-0.46\hat{i}-0.21\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{23}=-0.58\hat{i}-0.67\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{24}=-0.7\hat{i}-0.63\hat{j}+0.33\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result62.tex <==
{\tiny 2D-M62:}

$\hat{n}_{14}=0.81\hat{i}-0.54\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{23}=-0.37\hat{i}-0.15\hat{j}-0.91\hat{k}$,\;\;\;$\hat{n}_{25}=0.26\hat{i}+0.72\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{34}=-0.48\hat{i}-0.06\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result620.tex <==
2D-M620:

$\hat{n}_{14}=-0.28\hat{i}-0.96\hat{j}+0.04\hat{k}$,\;\;\;$\hat{n}_{24}=0.96\hat{i}-0.28\hat{j}+0.07\hat{k}$,\;\;\;$\hat{n}_{25}=-0.18\hat{i}-0.76\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{34}=-0.8\hat{i}-0.26\hat{j}+0.54\hat{k}$,\newline
$\hat{n}_{35}=0.57\hat{i}-0.6\hat{j}+0.56\hat{k}$,\;\;\;$\vec{r}_{25}=5.33\hat{i}+4.37\hat{j}+4.5\hat{k}$,\;\;\;$\vec{r}_{34}=5.5\hat{i}+5.08\hat{j}+4.04\hat{k}$,\;\;\;$\vec{r}_{35}=5.23\hat{i}+5.61\hat{j}+4.85\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result621.tex <==
2D-M621:

$\hat{n}_{14}=-0.12\hat{i}-0.92\hat{j}-0.37\hat{k}$,\;\;\;$\hat{n}_{24}=-0.05\hat{i}-0.64\hat{j}+0.76\hat{k}$,\;\;\;$\hat{n}_{25}=0.99\hat{i}-0.12\hat{j}-0.04\hat{k}$,\;\;\;$\hat{n}_{34}=-0.54\hat{i}-0.63\hat{j}-0.56\hat{k}$,\newline
$\hat{n}_{35}=0.84\hat{i}-0.44\hat{j}-0.32\hat{k}$,\;\;\;$\vec{r}_{24}=5.61\hat{i}+4.52\hat{j}+4.72\hat{k}$,\;\;\;$\vec{r}_{34}=5.32\hat{i}+4.61\hat{j}+5.69\hat{k}$,\;\;\;$\vec{r}_{35}=5.68\hat{i}+4.49\hat{j}+4.87\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result622.tex <==
2D-M622:

$\hat{n}_{14}=0.13\hat{i}-0.96\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{23}=-0.74\hat{i}-0.27\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{25}=-0.55\hat{i}-0.3\hat{j}+0.78\hat{k}$,\;\;\;$\hat{n}_{34}=0.39\hat{i}-0.92\hat{j}-0.07\hat{k}$,\newline
$\hat{n}_{45}=0.74\hat{i}+0.27\hat{j}+0.62\hat{k}$,\;\;\;$\vec{r}_{25}=5.57\hat{i}+2.78\hat{j}+5.57\hat{k}$,\;\;\;$\vec{r}_{34}=5.22\hat{i}+5.68\hat{j}+5.16\hat{k}$,\;\;\;$\vec{r}_{45}=4.79\hat{i}+5.09\hat{j}+5.42\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result623.tex <==
2D-M623:

$\hat{n}_{14}=-0.62\hat{i}-0.79\hat{j}+0.02\hat{k}$,\;\;\;$\hat{n}_{23}=-0.19\hat{i}-0.57\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{25}=0.76\hat{i}-0.59\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{34}=-0.62\hat{i}-0.56\hat{j}+0.55\hat{k}$,\newline
$\hat{n}_{45}=0.76\hat{i}-0.59\hat{j}+0.25\hat{k}$,\;\;\;$\vec{r}_{23}=5.03\hat{i}+5.53\hat{j}+5.53\hat{k}$,\;\;\;$\vec{r}_{34}=5.47\hat{i}+5.5\hat{j}+5.13\hat{k}$,\;\;\;$\vec{r}_{45}=4.75\hat{i}+4.83\hat{j}+4.97\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result624.tex <==
2D-M624:

$\hat{n}_{14}=0.28\hat{i}-0.95\hat{j}-0.15\hat{k}$,\;\;\;$\hat{n}_{23}=-0.65\hat{i}+0.36\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.88\hat{j}-0.47\hat{k}$,\;\;\;$\hat{n}_{34}=-0.76\hat{i}-0.31\hat{j}+0.57\hat{k}$,\newline
$\hat{n}_{45}=0.76\hat{i}+0.31\hat{j}-0.57\hat{k}$,\;\;\;$\vec{r}_{23}=5.46\hat{i}+4.8\hat{j}+4.59\hat{k}$,\;\;\;$\vec{r}_{25}=5.47\hat{i}+5.47\hat{j}+5.46\hat{k}$,\;\;\;$\vec{r}_{45}=5.41\hat{i}+4.87\hat{j}+4.83\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result625.tex <==
2D-M625:

$\hat{n}_{14}=-0.82\hat{i}-0.53\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{23}=-0.72\hat{i}-0.55\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.13\hat{i}-0.71\hat{j}+0.69\hat{k}$,\;\;\;$\hat{n}_{34}=0.68\hat{i}-0.44\hat{j}-0.58\hat{k}$,\newline
$\hat{n}_{45}=0.55\hat{i}-0.83\hat{j}+0.08\hat{k}$,\;\;\;$\vec{r}_{23}=5.29\hat{i}+5.23\hat{j}+4.71\hat{k}$,\;\;\;$\vec{r}_{25}=5.24\hat{i}+4.87\hat{j}+4.94\hat{k}$,\;\;\;$\vec{r}_{34}=5.27\hat{i}+4.71\hat{j}+4.75\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result626.tex <==
2D-M626:

$\hat{n}_{13}=0.92\hat{i}-0.21\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{24}=-0.7\hat{i}+0.38\hat{j}+0.61\hat{k}$,\;\;\;$\hat{n}_{25}=0.72\hat{i}+0.37\hat{j}+0.59\hat{k}$,\newline
$\hat{n}_{35}=-0.0\hat{i}+0.85\hat{j}-0.53\hat{k}$,\;\;\;$\vec{r}_{24}=5.1\hat{i}+5.02\hat{j}+4.88\hat{k}$,\;\;\;$\vec{r}_{25}=4.98\hat{i}+4.97\hat{j}+4.7\hat{k}$,\;\;\;$\vec{r}_{35}=5.0\hat{i}+5.34\hat{j}+4.97\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result627.tex <==
2D-M627:

$\hat{n}_{13}=-0.3\hat{i}-0.95\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{14}=-0.14\hat{i}-0.97\hat{j}+0.21\hat{k}$,\;\;\;$\hat{n}_{24}=0.76\hat{i}-0.24\hat{j}-0.61\hat{k}$,\;\;\;$\hat{n}_{25}=0.64\hat{i}+0.07\hat{j}+0.77\hat{k}$,\newline
$\hat{n}_{35}=-0.76\hat{i}+0.24\hat{j}+0.61\hat{k}$,\;\;\;$\vec{r}_{14}=4.84\hat{i}+5.25\hat{j}+5.19\hat{k}$,\;\;\;$\vec{r}_{25}=4.92\hat{i}+4.76\hat{j}+4.77\hat{k}$,\;\;\;$\vec{r}_{35}=5.12\hat{i}+4.84\hat{j}+5.2\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result628.tex <==
2D-M628:

$\hat{n}_{13}=0.29\hat{i}-0.93\hat{j}-0.21\hat{k}$,\;\;\;$\hat{n}_{14}=0.37\hat{i}-0.59\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{24}=0.12\hat{i}-0.74\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=-0.92\hat{i}-0.33\hat{j}+0.2\hat{k}$,\newline
$\hat{n}_{35}=-0.92\hat{i}-0.33\hat{j}+0.2\hat{k}$,\;\;\;$\vec{r}_{14}=6.32\hat{i}+6.38\hat{j}+4.93\hat{k}$,\;\;\;$\vec{r}_{24}=6.43\hat{i}+6.16\hat{j}+4.07\hat{k}$,\;\;\;$\vec{r}_{35}=6.02\hat{i}+5.53\hat{j}+6.45\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result629.tex <==
2D-M629:

$\hat{n}_{13}=0.74\hat{i}-0.68\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{14}=-0.89\hat{i}-0.36\hat{j}+0.27\hat{k}$,\;\;\;$\hat{n}_{24}=0.12\hat{i}-0.77\hat{j}-0.62\hat{k}$,\;\;\;$\hat{n}_{25}=0.43\hat{i}-0.52\hat{j}+0.73\hat{k}$,\newline
$\hat{n}_{35}=-0.68\hat{i}-0.74\hat{j}-0.01\hat{k}$,\;\;\;$\vec{r}_{14}=5.03\hat{i}+4.8\hat{j}+5.77\hat{k}$,\;\;\;$\vec{r}_{24}=5.76\hat{i}+4.26\hat{j}+5.22\hat{k}$,\;\;\;$\vec{r}_{25}=4.62\hat{i}+4.42\hat{j}+4.9\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result63.tex <==
{\tiny 2D-M63:}

$\hat{n}_{14}=0.68\hat{i}+0.52\hat{j}+0.52\hat{k}$,\;\;\;$\hat{n}_{23}=0.84\hat{i}+0.1\hat{j}-0.53\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{34}=-0.0\hat{i}+0.16\hat{j}-0.99\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+1.8\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result630.tex <==
2D-M630:

$\hat{n}_{13}=0.8\hat{i}-0.38\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{14}=-0.48\hat{i}+0.78\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{23}=0.09\hat{i}-0.68\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{25}=0.59\hat{i}+0.62\hat{j}+0.51\hat{k}$,\newline
$\hat{n}_{45}=0.65\hat{i}+0.01\hat{j}-0.76\hat{k}$,\;\;\;$\vec{r}_{14}=4.7\hat{i}+5.66\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{25}=6.03\hat{i}+5.58\hat{j}+4.55\hat{k}$,\;\;\;$\vec{r}_{45}=4.74\hat{i}+5.38\hat{j}+4.36\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result631.tex <==
2D-M631:

$\hat{n}_{13}=-0.6\hat{i}-0.75\hat{j}+0.26\hat{k}$,\;\;\;$\hat{n}_{14}=0.13\hat{i}-0.83\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{23}=0.68\hat{i}-0.32\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.41\hat{i}-0.57\hat{j}-0.71\hat{k}$,\newline
$\hat{n}_{45}=-0.72\hat{i}-0.45\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{14}=4.8\hat{i}+5.04\hat{j}+5.14\hat{k}$,\;\;\;$\vec{r}_{23}=4.8\hat{i}+5.08\hat{j}+5.19\hat{k}$,\;\;\;$\vec{r}_{45}=4.8\hat{i}+4.92\hat{j}+5.14\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result632.tex <==
2D-M632:

$\hat{n}_{13}=-0.55\hat{i}+0.61\hat{j}+0.57\hat{k}$,\;\;\;$\hat{n}_{14}=0.55\hat{i}-0.61\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{23}=0.66\hat{i}-0.1\hat{j}+0.74\hat{k}$,\;\;\;$\hat{n}_{25}=-0.51\hat{i}-0.79\hat{j}+0.35\hat{k}$,\newline
$\hat{n}_{45}=0.82\hat{i}+0.25\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{14}=5.03\hat{i}+5.08\hat{j}+4.43\hat{k}$,\;\;\;$\vec{r}_{23}=4.96\hat{i}+4.92\hat{j}+4.61\hat{k}$,\;\;\;$\vec{r}_{25}=4.99\hat{i}+5.5\hat{j}+4.97\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result633.tex <==
2D-M633:

$\hat{n}_{13}=-0.22\hat{i}-0.66\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.22\hat{i}-0.66\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{23}=-0.94\hat{i}-0.06\hat{j}-0.34\hat{k}$,\;\;\;$\hat{n}_{24}=0.27\hat{i}-0.74\hat{j}-0.61\hat{k}$,\newline
$\hat{n}_{45}=0.43\hat{i}-0.72\hat{j}-0.54\hat{k}$,\;\;\;$\vec{r}_{14}=5.81\hat{i}+4.94\hat{j}+5.59\hat{k}$,\;\;\;$\vec{r}_{23}=5.82\hat{i}+5.62\hat{j}+5.68\hat{k}$,\;\;\;$\vec{r}_{24}=5.41\hat{i}+5.81\hat{j}+4.83\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result634.tex <==
2D-M634:

$\hat{n}_{13}=-0.36\hat{i}-0.72\hat{j}-0.59\hat{k}$,\;\;\;$\hat{n}_{14}=-0.83\hat{i}-0.54\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{23}=0.14\hat{i}-0.98\hat{j}+0.1\hat{k}$,\;\;\;$\hat{n}_{24}=-0.05\hat{i}-0.98\hat{j}-0.19\hat{k}$,\newline
$\hat{n}_{35}=0.91\hat{i}-0.41\hat{j}-0.05\hat{k}$,\;\;\;$\vec{r}_{14}=5.41\hat{i}+6.3\hat{j}+5.72\hat{k}$,\;\;\;$\vec{r}_{23}=6.29\hat{i}+4.07\hat{j}+4.39\hat{k}$,\;\;\;$\vec{r}_{24}=4.55\hat{i}+5.87\hat{j}+5.73\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result635.tex <==
2D-M635:

$\hat{n}_{13}=-0.64\hat{i}-0.34\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{14}=0.82\hat{i}-0.35\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{23}=-0.56\hat{i}-0.4\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=-0.08\hat{i}-0.85\hat{j}+0.52\hat{k}$,\newline
$\hat{n}_{25}=0.53\hat{i}-0.84\hat{j}+0.08\hat{k}$,\;\;\;$\vec{r}_{14}=5.14\hat{i}+4.94\hat{j}+4.73\hat{k}$,\;\;\;$\vec{r}_{23}=4.92\hat{i}+4.92\hat{j}+5.18\hat{k}$,\;\;\;$\vec{r}_{24}=5.28\hat{i}+5.07\hat{j}+4.34\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result636.tex <==
2D-M636:

$\hat{n}_{13}=0.71\hat{i}+0.58\hat{j}+0.41\hat{k}$,\;\;\;$\hat{n}_{14}=0.1\hat{i}-0.65\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.92\hat{i}-0.23\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{25}=-0.38\hat{i}-0.72\hat{j}-0.58\hat{k}$,\newline
$\hat{n}_{35}=-0.7\hat{i}+0.49\hat{j}+0.52\hat{k}$,\;\;\;$\vec{r}_{13}=5.53\hat{i}+4.39\hat{j}+5.47\hat{k}$,\;\;\;$\vec{r}_{14}=5.67\hat{i}+4.41\hat{j}+5.69\hat{k}$,\;\;\;$\vec{r}_{35}=4.4\hat{i}+5.62\hat{j}+4.11\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result637.tex <==
2D-M637:

$\hat{n}_{13}=-0.23\hat{i}-0.83\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{14}=0.39\hat{i}-0.56\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{24}=-0.23\hat{i}-0.83\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.89\hat{i}+0.03\hat{j}+0.45\hat{k}$,\newline
$\hat{n}_{35}=-0.97\hat{i}+0.18\hat{j}-0.14\hat{k}$,\;\;\;$\vec{r}_{13}=3.21\hat{i}+4.86\hat{j}+5.67\hat{k}$,\;\;\;$\vec{r}_{14}=5.98\hat{i}+4.92\hat{j}+3.95\hat{k}$,\;\;\;$\vec{r}_{25}=5.09\hat{i}+4.22\hat{j}+5.31\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result638.tex <==
2D-M638:

$\hat{n}_{13}=0.38\hat{i}-0.92\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{14}=0.47\hat{i}+0.08\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{24}=-0.79\hat{i}-0.4\hat{j}-0.46\hat{k}$,\;\;\;$\hat{n}_{25}=0.38\hat{i}-0.92\hat{j}+0.12\hat{k}$,\newline
$\hat{n}_{35}=-0.91\hat{i}-0.35\hat{j}+0.22\hat{k}$,\;\;\;$\vec{r}_{13}=5.58\hat{i}+5.48\hat{j}+5.37\hat{k}$,\;\;\;$\vec{r}_{14}=5.7\hat{i}+4.44\hat{j}+4.83\hat{k}$,\;\;\;$\vec{r}_{24}=4.21\hat{i}+5.3\hat{j}+5.78\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result639.tex <==
2D-M639:

$\hat{n}_{13}=0.77\hat{i}-0.16\hat{j}+0.62\hat{k}$,\;\;\;$\hat{n}_{14}=0.42\hat{i}-0.6\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}-0.6\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{24}=-0.48\hat{i}-0.79\hat{j}+0.4\hat{k}$,\newline
$\hat{n}_{45}=-0.6\hat{i}-0.75\hat{j}+0.29\hat{k}$,\;\;\;$\vec{r}_{13}=4.51\hat{i}+5.52\hat{j}+4.98\hat{k}$,\;\;\;$\vec{r}_{14}=4.46\hat{i}+5.27\hat{j}+5.44\hat{k}$,\;\;\;$\vec{r}_{24}=4.6\hat{i}+5.54\hat{j}+5.22\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result64.tex <==
{\tiny 2D-M64:}

$\hat{n}_{14}=0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{23}=-0.88\hat{i}+0.23\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{25}=0.47\hat{i}-0.32\hat{j}+0.82\hat{k}$,\;\;\;$\hat{n}_{34}=-0.7\hat{i}-0.67\hat{j}-0.26\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result640.tex <==
2D-M640:

$\hat{n}_{13}=0.83\hat{i}-0.46\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{14}=-0.21\hat{i}-0.78\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{23}=0.83\hat{i}-0.46\hat{j}+0.31\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}-0.43\hat{j}+0.74\hat{k}$,\newline
$\hat{n}_{35}=-0.5\hat{i}-0.86\hat{j}+0.06\hat{k}$,\;\;\;$\vec{r}_{13}=4.66\hat{i}+5.31\hat{j}+5.3\hat{k}$,\;\;\;$\vec{r}_{14}=4.67\hat{i}+5.05\hat{j}+4.71\hat{k}$,\;\;\;$\vec{r}_{24}=5.26\hat{i}+4.83\hat{j}+4.96\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result641.tex <==
2D-M641:

$\hat{n}_{13}=-0.59\hat{i}-0.49\hat{j}+0.64\hat{k}$,\;\;\;$\hat{n}_{14}=0.81\hat{i}-0.38\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{23}=0.69\hat{i}-0.72\hat{j}+0.08\hat{k}$,\;\;\;$\hat{n}_{24}=-0.02\hat{i}-0.78\hat{j}-0.62\hat{k}$,\newline
$\hat{n}_{25}=-0.72\hat{i}-0.68\hat{j}+0.09\hat{k}$,\;\;\;$\vec{r}_{13}=5.42\hat{i}+5.52\hat{j}+5.21\hat{k}$,\;\;\;$\vec{r}_{14}=5.48\hat{i}+4.49\hat{j}+5.19\hat{k}$,\;\;\;$\vec{r}_{24}=5.53\hat{i}+5.39\hat{j}+5.46\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result65.tex <==
{\tiny 2D-M65:}

$\hat{n}_{14}=0.31\hat{i}-0.9\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{23}=0.77\hat{i}+0.37\hat{j}-0.51\hat{k}$,\;\;\;$\hat{n}_{25}=0.32\hat{i}+0.66\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{34}=0.13\hat{i}-0.63\hat{j}-0.76\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{15}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result66.tex <==
{\tiny 2D-M66:}

$\hat{n}_{15}=-0.0\hat{i}+0.86\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{23}=0.7\hat{i}-0.7\hat{j}+0.17\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.5\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{34}=-0.15\hat{i}-0.62\hat{j}-0.77\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{15}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result67.tex <==
{\tiny 2D-M67:}

$\hat{n}_{13}=0.14\hat{i}+0.99\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.39\hat{i}+0.52\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{24}=0.79\hat{i}+0.57\hat{j}-0.23\hat{k}$,\;\;\;$\hat{n}_{25}=-0.61\hat{i}-0.01\hat{j}-0.79\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result68.tex <==
{\tiny 2D-M68:}

$\hat{n}_{13}=0.61\hat{i}+0.15\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{14}=0.57\hat{i}-0.22\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{24}=0.42\hat{i}+0.64\hat{j}-0.64\hat{k}$,\;\;\;$\hat{n}_{35}=-0.52\hat{i}-0.82\hat{j}-0.24\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result69.tex <==
{\tiny 2D-M69:}

$\hat{n}_{13}=0.69\hat{i}-0.03\hat{j}+0.72\hat{k}$,\;\;\;$\hat{n}_{14}=-0.33\hat{i}+0.9\hat{j}+0.29\hat{k}$,\;\;\;$\hat{n}_{24}=-0.51\hat{i}-0.85\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{25}=0.34\hat{i}+0.69\hat{j}-0.64\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result7.tex <==
{\tiny 2D-M7:}

$\hat{n}_{14}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.71\hat{i}+0.11\hat{j}-0.7\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result70.tex <==
{\tiny 2D-M70:}

$\hat{n}_{13}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.6\hat{i}+0.54\hat{j}+0.6\hat{k}$,\;\;\;$\hat{n}_{24}=-0.67\hat{i}-0.3\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{35}=0.6\hat{i}+0.49\hat{j}+0.64\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+2.68\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result71.tex <==
{\tiny 2D-M71:}

$\hat{n}_{13}=-0.0\hat{i}+0.68\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{14}=0.7\hat{i}-0.18\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{25}=-0.15\hat{i}+0.7\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{35}=0.5\hat{i}+0.78\hat{j}+0.37\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result72.tex <==
{\tiny 2D-M72:}

$\hat{n}_{13}=0.81\hat{i}-0.4\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{14}=-0.0\hat{i}+0.73\hat{j}+0.68\hat{k}$,\;\;\;$\hat{n}_{25}=0.95\hat{i}+0.13\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{35}=0.03\hat{i}+0.76\hat{j}+0.65\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result73.tex <==
{\tiny 2D-M73:}

$\hat{n}_{13}=0.0\hat{i}+0.05\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.71\hat{i}-0.05\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.59\hat{i}+0.46\hat{j}+0.67\hat{k}$,\;\;\;$\hat{n}_{45}=0.0\hat{i}-0.86\hat{j}-0.51\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result74.tex <==
{\tiny 2D-M74:}

$\hat{n}_{13}=0.0\hat{i}-0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{14}=-0.02\hat{i}-0.9\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{23}=-0.94\hat{i}-0.11\hat{j}-0.33\hat{k}$,\;\;\;$\hat{n}_{35}=-0.87\hat{i}-0.5\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=7.25\hat{i}+5.1\hat{j}+3.87\hat{k}$,\;\;\;$\vec{r}_{23}=8.61\hat{i}+8.77\hat{j}+6.23\hat{k}$,\;\;\;$\vec{r}_{24}=1.63\hat{i}+6.13\hat{j}+3.88\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result75.tex <==
{\tiny 2D-M75:}

$\hat{n}_{13}=0.05\hat{i}+0.55\hat{j}-0.83\hat{k}$,\;\;\;$\hat{n}_{14}=0.65\hat{i}-0.39\hat{j}-0.65\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.25\hat{j}-0.97\hat{k}$,\;\;\;$\hat{n}_{25}=0.48\hat{i}-0.37\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result76.tex <==
{\tiny 2D-M76:}

$\hat{n}_{13}=0.7\hat{i}-0.14\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{14}=-0.52\hat{i}+0.82\hat{j}+0.25\hat{k}$,\;\;\;$\hat{n}_{24}=0.22\hat{i}-0.18\hat{j}-0.96\hat{k}$,\;\;\;$\hat{n}_{25}=0.36\hat{i}-0.63\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result77.tex <==
{\tiny 2D-M77:}

$\hat{n}_{13}=0.73\hat{i}+0.15\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{14}=-0.91\hat{i}+0.3\hat{j}-0.28\hat{k}$,\;\;\;$\hat{n}_{24}=-0.47\hat{i}-0.47\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.67\hat{j}+0.74\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result78.tex <==
{\tiny 2D-M78:}

$\hat{n}_{13}=-0.67\hat{i}-0.6\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{14}=-0.71\hat{i}-0.18\hat{j}-0.68\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{35}=-0.67\hat{i}+0.49\hat{j}+0.56\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+9.99\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result79.tex <==
{\tiny 2D-M79:}

$\hat{n}_{13}=0.0\hat{i}+0.62\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{14}=0.43\hat{i}-0.88\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{23}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{25}=0.77\hat{i}+0.12\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result8.tex <==
{\tiny 2D-M8:}

$\hat{n}_{14}=-0.46\hat{i}+0.74\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.71\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{45}=0.58\hat{i}-0.58\hat{j}-0.58\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result80.tex <==
{\tiny 2D-M80:}

$\hat{n}_{13}=0.04\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{14}=-0.86\hat{i}-0.35\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{23}=0.81\hat{i}-0.31\hat{j}+0.5\hat{k}$,\;\;\;$\hat{n}_{45}=0.01\hat{i}-0.72\hat{j}-0.69\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result81.tex <==
{\tiny 2D-M81:}

$\hat{n}_{13}=-0.0\hat{i}+0.87\hat{j}-0.5\hat{k}$,\;\;\;$\hat{n}_{14}=0.0\hat{i}+0.28\hat{j}+0.96\hat{k}$,\;\;\;$\hat{n}_{23}=-0.49\hat{i}-0.73\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{45}=-0.08\hat{i}+0.55\hat{j}+0.83\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result82.tex <==
{\tiny 2D-M82:}

$\hat{n}_{13}=-0.51\hat{i}+0.31\hat{j}+0.8\hat{k}$,\;\;\;$\hat{n}_{14}=-0.04\hat{i}-0.6\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{23}=0.37\hat{i}-0.47\hat{j}-0.8\hat{k}$,\;\;\;$\hat{n}_{35}=-0.02\hat{i}+0.6\hat{j}-0.8\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=4.5\hat{i}+2.54\hat{j}+7.9\hat{k}$,\;\;\;$\vec{r}_{23}=8.09\hat{i}+8.34\hat{j}+4.68\hat{k}$,\;\;\;$\vec{r}_{24}=9.23\hat{i}+8.25\hat{j}+1.09\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result83.tex <==
{\tiny 2D-M83:}

$\hat{n}_{13}=0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{14}=0.79\hat{i}-0.21\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.58\hat{j}-0.58\hat{k}$,\;\;\;$\hat{n}_{25}=-0.82\hat{i}+0.47\hat{j}+0.33\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result84.tex <==
{\tiny 2D-M84:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{14}=0.48\hat{i}+0.77\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{25}=0.71\hat{i}-0.0\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{45}=0.5\hat{i}+0.61\hat{j}-0.62\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result85.tex <==
{\tiny 2D-M85:}

$\hat{n}_{13}=-0.65\hat{i}+0.65\hat{j}-0.4\hat{k}$,\;\;\;$\hat{n}_{14}=-0.48\hat{i}+0.45\hat{j}+0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.63\hat{i}+0.46\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{45}=0.01\hat{i}+0.58\hat{j}-0.81\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result86.tex <==
{\tiny 2D-M86:}

$\hat{n}_{13}=-0.16\hat{i}-0.63\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{14}=-0.22\hat{i}-0.92\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{24}=1.0\hat{i}-0.08\hat{j}-0.01\hat{k}$,\;\;\;$\hat{n}_{35}=-0.71\hat{i}+0.1\hat{j}+0.7\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=7.61\hat{i}+1.62\hat{j}+8.23\hat{k}$,\;\;\;$\vec{r}_{23}=1.68\hat{i}+5.11\hat{j}+6.63\hat{k}$,\;\;\;$\vec{r}_{24}=5.61\hat{i}+4.8\hat{j}+3.36\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result87.tex <==
{\tiny 2D-M87:}

$\hat{n}_{13}=0.66\hat{i}-0.66\hat{j}+0.36\hat{k}$,\;\;\;$\hat{n}_{14}=0.52\hat{i}-0.42\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{24}=0.12\hat{i}-0.71\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{25}=0.68\hat{i}+0.16\hat{j}+0.72\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result88.tex <==
{\tiny 2D-M88:}

$\hat{n}_{13}=0.0\hat{i}+0.62\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}+0.42\hat{j}+0.39\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.7\hat{j}+0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.0\hat{i}+0.7\hat{j}-0.72\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result89.tex <==
{\tiny 2D-M89:}

$\hat{n}_{13}=-0.0\hat{i}-0.58\hat{j}-0.82\hat{k}$,\;\;\;$\hat{n}_{24}=0.65\hat{i}-0.54\hat{j}-0.54\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}+0.38\hat{j}-0.92\hat{k}$,\;\;\;$\hat{n}_{35}=-0.58\hat{i}+0.51\hat{j}+0.63\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result9.tex <==
{\tiny 2D-M9:}

$\hat{n}_{14}=-0.0\hat{i}+0.58\hat{j}+0.81\hat{k}$,\;\;\;$\hat{n}_{25}=-0.36\hat{i}-0.93\hat{j}-0.05\hat{k}$,\;\;\;$\hat{n}_{45}=0.71\hat{i}-0.1\hat{j}+0.7\hat{k}$,\;\;\;$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=6.41\hat{i}+3.46\hat{j}+3.55\hat{k}$,\;\;\;$\vec{r}_{34}=6.26\hat{i}+6.53\hat{j}+1.95\hat{k}$,\;\;\;$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result90.tex <==
{\tiny 2D-M90:}

$\hat{n}_{13}=0.71\hat{i}-0.1\hat{j}+0.7\hat{k}$,\;\;\;$\hat{n}_{24}=0.3\hat{i}+0.67\hat{j}-0.67\hat{k}$,\;\;\;$\hat{n}_{25}=0.0\hat{i}-0.71\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{35}=-0.03\hat{i}+0.68\hat{j}+0.73\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result91.tex <==
{\tiny 2D-M91:}

$\hat{n}_{13}=-0.85\hat{i}+0.47\hat{j}-0.25\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.0\hat{j}+1.0\hat{k}$,\;\;\;$\hat{n}_{25}=-0.13\hat{i}-0.63\hat{j}-0.76\hat{k}$,\;\;\;$\hat{n}_{45}=-0.33\hat{i}-0.9\hat{j}+0.29\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result92.tex <==
{\tiny 2D-M92:}

$\hat{n}_{13}=0.0\hat{i}+0.0\hat{j}-1.0\hat{k}$,\;\;\;$\hat{n}_{23}=0.25\hat{i}-0.44\hat{j}-0.86\hat{k}$,\;\;\;$\hat{n}_{25}=0.41\hat{i}+0.2\hat{j}-0.89\hat{k}$,\;\;\;$\hat{n}_{45}=0.75\hat{i}-0.65\hat{j}+0.11\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+9.97\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result93.tex <==
{\tiny 2D-M93:}

$\hat{n}_{13}=-0.32\hat{i}+0.6\hat{j}-0.74\hat{k}$,\;\;\;$\hat{n}_{23}=-0.71\hat{i}-0.71\hat{j}+0.0\hat{k}$,\;\;\;$\hat{n}_{24}=0.33\hat{i}-0.33\hat{j}-0.89\hat{k}$,\;\;\;$\hat{n}_{45}=-0.29\hat{i}-0.38\hat{j}+0.88\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result94.tex <==
{\tiny 2D-M94:}

$\hat{n}_{13}=0.6\hat{i}-0.11\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{23}=0.13\hat{i}-0.76\hat{j}-0.63\hat{k}$,\;\;\;$\hat{n}_{24}=-0.28\hat{i}+0.27\hat{j}+0.92\hat{k}$,\;\;\;$\hat{n}_{35}=0.13\hat{i}-0.65\hat{j}+0.75\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=6.57\hat{i}+7.46\hat{j}+8.53\hat{k}$,\;\;\;$\vec{r}_{23}=7.76\hat{i}+9.05\hat{j}+0.95\hat{k}$,\;\;\;$\vec{r}_{24}=8.61\hat{i}+8.08\hat{j}+6.19\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result95.tex <==
{\tiny 2D-M95:}

$\hat{n}_{13}=0.82\hat{i}-0.38\hat{j}+0.42\hat{k}$,\;\;\;$\hat{n}_{23}=0.58\hat{i}+0.6\hat{j}+0.56\hat{k}$,\;\;\;$\hat{n}_{24}=0.77\hat{i}-0.22\hat{j}-0.6\hat{k}$,\;\;\;$\hat{n}_{25}=0.3\hat{i}-0.62\hat{j}-0.73\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result96.tex <==
{\tiny 2D-M96:}

$\hat{n}_{13}=0.07\hat{i}-0.81\hat{j}+0.58\hat{k}$,\;\;\;$\hat{n}_{23}=0.35\hat{i}-0.92\hat{j}+0.15\hat{k}$,\;\;\;$\hat{n}_{25}=-0.39\hat{i}-0.83\hat{j}-0.39\hat{k}$,\;\;\;$\hat{n}_{45}=0.75\hat{i}-0.47\hat{j}+0.47\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result97.tex <==
{\tiny 2D-M97:}

$\hat{n}_{13}=-0.69\hat{i}-0.36\hat{j}+0.63\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.36\hat{j}+0.93\hat{k}$,\;\;\;$\hat{n}_{24}=-0.67\hat{i}-0.35\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{45}=0.9\hat{i}+0.28\hat{j}+0.33\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{24}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{45}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result98.tex <==
{\tiny 2D-M98:}

$\hat{n}_{13}=0.67\hat{i}+0.12\hat{j}+0.73\hat{k}$,\;\;\;$\hat{n}_{23}=0.83\hat{i}+0.3\hat{j}+0.48\hat{k}$,\;\;\;$\hat{n}_{24}=-0.87\hat{i}+0.24\hat{j}+0.43\hat{k}$,\;\;\;$\hat{n}_{35}=-0.17\hat{i}+0.67\hat{j}-0.73\hat{k}$,\newline
$\vec{r}_{13}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{14}=3.35\hat{i}+7.41\hat{j}+8.14\hat{k}$,\;\;\;$\vec{r}_{23}=2.65\hat{i}+5.33\hat{j}+4.37\hat{k}$,\;\;\;$\vec{r}_{24}=1.81\hat{i}+5.97\hat{j}+8.77\hat{k}$,\newline
$\vec{r}_{35}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof2_2/result99.tex <==
{\tiny 2D-M99:}

$\hat{n}_{13}=0.48\hat{i}+0.77\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{23}=-0.7\hat{i}-0.56\hat{j}+0.44\hat{k}$,\;\;\;$\hat{n}_{24}=0.64\hat{i}-0.64\hat{j}-0.42\hat{k}$,\;\;\;$\hat{n}_{25}=-0.0\hat{i}+0.48\hat{j}-0.88\hat{k}$,\newline
$\vec{r}_{13}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{14}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof3/result1.tex <==
{\tiny 3D-M1:}

$\hat{n}_{13}=-0.71\hat{i}+0.11\hat{j}-0.7\hat{k}$,\;\;\;$\hat{n}_{23}=-0.0\hat{i}+0.58\hat{j}-0.81\hat{k}$,\;\;\;$\hat{n}_{24}=0.82\hat{i}-0.46\hat{j}-0.34\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof3/result2.tex <==
{\tiny 3D-M2:}

$\hat{n}_{13}=-0.8\hat{i}+0.33\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{23}=-0.17\hat{i}+0.67\hat{j}-0.73\hat{k}$,\;\;\;$\hat{n}_{24}=-0.57\hat{i}-0.67\hat{j}-0.48\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof3/result3.tex <==
{\tiny 3D-M3:}

$\hat{n}_{13}=-0.8\hat{i}+0.58\hat{j}+0.14\hat{k}$,\;\;\;$\hat{n}_{23}=-0.74\hat{i}-0.51\hat{j}-0.43\hat{k}$,\;\;\;$\hat{n}_{24}=0.51\hat{i}+0.16\hat{j}+0.84\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof3/result4.tex <==
{\tiny 3D-M4:}

$\hat{n}_{13}=-0.57\hat{i}-0.67\hat{j}-0.48\hat{k}$,\;\;\;$\hat{n}_{23}=-0.31\hat{i}-0.36\hat{j}-0.88\hat{k}$,\;\;\;$\hat{n}_{24}=0.76\hat{i}-0.65\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\newline
$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof3/result5.tex <==
{\tiny 3D-M5:}

$\hat{n}_{13}=0.5\hat{i}+0.18\hat{j}+0.85\hat{k}$,\;\;\;$\hat{n}_{23}=-0.76\hat{i}-0.61\hat{j}-0.24\hat{k}$,\;\;\;$\hat{n}_{24}=0.03\hat{i}+0.33\hat{j}-0.94\hat{k}$,\;\;\;$\vec{r}_{13}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof3/result6.tex <==
{\tiny 3D-M6:}

$\hat{n}_{13}=-0.6\hat{i}-0.76\hat{j}-0.26\hat{k}$,\;\;\;$\hat{n}_{23}=0.26\hat{i}+0.4\hat{j}+0.88\hat{k}$,\;\;\;$\hat{n}_{24}=-0.21\hat{i}-0.17\hat{j}+0.96\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof3/result7.tex <==
{\tiny 3D-M7:}

$\hat{n}_{13}=-0.54\hat{i}-0.83\hat{j}+0.12\hat{k}$,\;\;\;$\hat{n}_{23}=0.18\hat{i}-0.26\hat{j}-0.95\hat{k}$,\;\;\;$\hat{n}_{24}=-0.04\hat{i}-0.56\hat{j}-0.83\hat{k}$,\;\;\;$\vec{r}_{24}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof3/result8.tex <==
{\tiny 3D-M8:}

$\hat{n}_{13}=0.41\hat{i}+0.89\hat{j}-0.2\hat{k}$,\;\;\;$\hat{n}_{23}=-0.62\hat{i}+0.11\hat{j}-0.78\hat{k}$,\;\;\;$\hat{n}_{24}=-0.67\hat{i}+0.44\hat{j}+0.59\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result1.tex <==
{\tiny 4D-M1:}

$\hat{n}_{14}=-0.29\hat{i}+0.57\hat{j}-0.77\hat{k}$,\;\;\;$\hat{n}_{23}=0.75\hat{i}-0.53\hat{j}+0.4\hat{k}$,\;\;\;$\hat{n}_{25}=-0.34\hat{i}+0.83\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{34}=-0.72\hat{i}+0.12\hat{j}+0.69\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result10.tex <==
{\tiny 4D-M10:}

$\hat{n}_{14}=-0.63\hat{i}-0.76\hat{j}-0.17\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.56\hat{i}+0.59\hat{j}-0.57\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result11.tex <==
{\tiny 4D-M11:}

$\hat{n}_{14}=-0.32\hat{i}+0.81\hat{j}-0.49\hat{k}$,\;\;\;$\hat{n}_{23}=0.78\hat{i}+0.52\hat{j}+0.35\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.54\hat{i}+0.84\hat{j}+0.08\hat{k}$,\newline
$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result12.tex <==
{\tiny 4D-M12:}

$\hat{n}_{14}=0.09\hat{i}-1.0\hat{j}+0.05\hat{k}$,\;\;\;$\hat{n}_{23}=0.67\hat{i}+0.35\hat{j}+0.66\hat{k}$,\;\;\;$\hat{n}_{25}=0.01\hat{i}-0.88\hat{j}+0.47\hat{k}$,\;\;\;$\hat{n}_{34}=-0.75\hat{i}+0.31\hat{j}+0.59\hat{k}$,\newline
$\vec{r}_{14}=4.0\hat{i}+2.99\hat{j}+5.94\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result13.tex <==
{\tiny 4D-M13:}

$\hat{n}_{14}=-0.94\hat{i}-0.18\hat{j}-0.29\hat{k}$,\;\;\;$\hat{n}_{23}=0.32\hat{i}-0.95\hat{j}+0.01\hat{k}$,\;\;\;$\hat{n}_{25}=-0.03\hat{i}-0.8\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=0.34\hat{i}-0.57\hat{j}-0.75\hat{k}$,\newline
$\vec{r}_{23}=7.59\hat{i}+3.33\hat{j}+4.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result14.tex <==
{\tiny 4D-M14:}

$\hat{n}_{14}=-0.38\hat{i}-0.54\hat{j}-0.75\hat{k}$,\;\;\;$\hat{n}_{23}=-0.54\hat{i}-0.53\hat{j}+0.65\hat{k}$,\;\;\;$\hat{n}_{25}=0.34\hat{i}-0.93\hat{j}-0.12\hat{k}$,\;\;\;$\hat{n}_{34}=0.75\hat{i}-0.65\hat{j}+0.1\hat{k}$,\newline
$\vec{r}_{25}=3.55\hat{i}+6.33\hat{j}+6.15\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result15.tex <==
{\tiny 4D-M15:}

$\hat{n}_{14}=-0.19\hat{i}-0.68\hat{j}-0.71\hat{k}$,\;\;\;$\hat{n}_{23}=0.56\hat{i}-0.67\hat{j}+0.49\hat{k}$,\;\;\;$\hat{n}_{25}=-0.8\hat{i}-0.3\hat{j}+0.51\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}-0.54\hat{j}+0.05\hat{k}$,\newline
$\vec{r}_{34}=3.99\hat{i}+5.66\hat{j}+6.62\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result2.tex <==
{\tiny 4D-M2:}

$\hat{n}_{14}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{23}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{25}=-0.42\hat{i}-0.85\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{34}=0.57\hat{i}+0.69\hat{j}+0.45\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result3.tex <==
{\tiny 4D-M3:}

$\hat{n}_{14}=0.39\hat{i}+0.47\hat{j}-0.79\hat{k}$,\;\;\;$\hat{n}_{23}=-0.42\hat{i}-0.85\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=-0.57\hat{i}-0.69\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.49\hat{j}-0.3\hat{k}$,\newline
$\vec{r}_{14}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result4.tex <==
{\tiny 4D-M4:}

$\hat{n}_{14}=0.42\hat{i}+0.85\hat{j}-0.32\hat{k}$,\;\;\;$\hat{n}_{23}=-0.57\hat{i}-0.69\hat{j}+0.45\hat{k}$,\;\;\;$\hat{n}_{25}=-0.39\hat{i}-0.47\hat{j}+0.79\hat{k}$,\;\;\;$\hat{n}_{34}=0.82\hat{i}+0.49\hat{j}-0.3\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result5.tex <==
{\tiny 4D-M5:}

$\hat{n}_{14}=-0.57\hat{i}-0.69\hat{j}-0.45\hat{k}$,\;\;\;$\hat{n}_{23}=0.42\hat{i}+0.85\hat{j}+0.32\hat{k}$,\;\;\;$\hat{n}_{25}=0.82\hat{i}+0.49\hat{j}+0.3\hat{k}$,\;\;\;$\hat{n}_{34}=-0.39\hat{i}-0.47\hat{j}-0.79\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+10.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result6.tex <==
{\tiny 4D-M6:}

$\hat{n}_{14}=-0.54\hat{i}-0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.68\hat{i}-0.7\hat{j}-0.22\hat{k}$,\;\;\;$\hat{n}_{25}=0.62\hat{i}-0.53\hat{j}+0.59\hat{k}$,\;\;\;$\hat{n}_{34}=-0.58\hat{i}-0.81\hat{j}-0.12\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+10.0\hat{k}$,\;\;\;$\vec{r}_{23}=10.0\hat{i}+0.0\hat{j}+0.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result7.tex <==
{\tiny 4D-M7:}

$\hat{n}_{14}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.05\hat{i}+0.94\hat{j}+0.34\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=0.84\hat{i}+0.22\hat{j}-0.49\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result8.tex <==
{\tiny 4D-M8:}

$\hat{n}_{14}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{23}=-0.26\hat{i}+0.85\hat{j}+0.46\hat{k}$,\;\;\;$\hat{n}_{25}=-0.8\hat{i}-0.46\hat{j}+0.38\hat{k}$,\;\;\;$\hat{n}_{34}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\newline
$\vec{r}_{14}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{34}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.



==> contentfolder/mechanisms2/result/dof4/result9.tex <==
{\tiny 4D-M9:}

$\hat{n}_{14}=-0.08\hat{i}-0.96\hat{j}-0.27\hat{k}$,\;\;\;$\hat{n}_{23}=0.54\hat{i}+0.84\hat{j}-0.08\hat{k}$,\;\;\;$\hat{n}_{25}=-0.68\hat{i}-0.7\hat{j}+0.22\hat{k}$,\;\;\;$\hat{n}_{34}=-0.84\hat{i}-0.08\hat{j}+0.53\hat{k}$,\newline
$\vec{r}_{23}=0.0\hat{i}+10.0\hat{j}+0.0\hat{k}$,\;\;\;$\vec{r}_{25}=10.0\hat{i}+0.0\hat{j}+10.0\hat{k}$.


